Aliquot sequences with small starting values

We describe the results of the computation of aliquot sequences with small starting values. In particular all sequences with starting values less than a million have been computed until either termination occurred (at 1 or a cycle), or an entry of 100 decimal digits was encountered. All dependencies were recorded, and numerous statistics, curiosities, and records are reported.

==> H004788 <==
\addplot[color=blue] coordinates{
( 6460, 3.6801 )
( 6461, 3.9900 )
( 6462, 3.9925 )
( 6463, 4.3331 )
( 6464, 4.3342 )
( 6465, 4.5588 )
( 6466, 4.7822 )
( 6467, 5.0229 )
( 6468, 5.3679 )
( 6469, 5.5900 )
( 6470, 5.8724 )
( 6471, 6.1307 )
( 6472, 6.3527 )
( 6473, 6.4440 )
( 6474, 6.4605 )
( 6475, 6.4605 )
( 6476, 6.8815 )
( 6477, 7.1033 )
( 6478, 7.3604 )
( 6479, 7.6213 )
( 6480, 7.9638 )
( 6481, 8.1857 )
( 6482, 8.4664 )
( 6483, 8.7428 )
( 6484, 9.0151 )
( 6485, 9.4584 )
( 6486, 9.6897 )
( 6487, 9.9119 )
( 6488, 10.267 )
( 6489, 10.555 )
( 6490, 10.724 )
( 6491, 10.969 )
( 6492, 11.139 )
( 6493, 11.274 )
( 6494, 11.341 )
( 6495, 11.663 )
( 6496, 11.978 )
( 6497, 12.286 )
( 6498, 12.489 )
( 6499, 12.643 )
( 6500, 12.766 )
( 6501, 12.877 )
( 6502, 12.975 )
( 6503, 13.182 )
( 6504, 13.278 )
( 6505, 13.512 )
( 6506, 13.505 )
( 6507, 13.204 )
( 6508, 12.905 )
( 6509, 12.628 )
( 6510, 12.327 )
( 6511, 12.411 )
( 6512, 12.641 )
( 6513, 12.840 )
( 6514, 13.236 )
( 6515, 13.566 )
( 6516, 13.561 )
( 6517, 13.584 )
( 6518, 13.556 )
( 6519, 13.578 )
( 6520, 13.577 )
( 6521, 13.519 )
( 6522, 13.394 )
( 6523, 13.269 )
( 6524, 13.068 )
( 6525, 12.855 )
( 6526, 12.582 )
( 6527, 12.303 )
( 6528, 12.011 )
( 6529, 11.710 )
( 6530, 11.879 )
( 6531, 12.026 )
( 6532, 12.052 )
( 6533, 12.052 )
( 6534, 12.126 )
( 6535, 12.370 )
( 6536, 12.541 )
( 6537, 12.582 )
( 6538, 12.582 )
( 6539, 12.597 )
( 6540, 12.736 )
( 6541, 12.446 )
( 6542, 12.230 )
( 6543, 11.988 )
( 6544, 11.702 )
( 6545, 11.454 )
( 6546, 11.244 )
( 6547, 11.262 )
( 6548, 11.235 )
( 6549, 11.202 )
( 6550, 11.152 )
( 6551, 11.055 )
( 6552, 10.792 )
( 6553, 10.491 )
( 6554, 10.190 )
( 6555, 10.309 )
( 6556, 10.362 )
( 6557, 10.237 )
( 6558, 10.304 )
( 6559, 10.246 )
( 6560, 10.142 )
( 6561, 9.8503 )
( 6562, 9.6681 )
( 6563, 9.3685 )
( 6564, 9.0676 )
( 6565, 8.7751 )
( 6566, 8.4745 )
( 6567, 8.2043 )
( 6568, 7.9302 )
( 6569, 7.6301 )
( 6570, 7.3320 )
( 6571, 7.0310 )
( 6572, 7.0291 )
( 6573, 6.9600 )
( 6574, 6.9849 )
( 6575, 6.8694 )
( 6576, 6.7460 )
( 6577, 6.9301 )
( 6578, 6.9315 )
( 6579, 6.9433 )
( 6580, 6.9433 )
( 6581, 7.2543 )
( 6582, 7.4141 )
( 6583, 7.5739 )
( 6584, 7.9464 )
( 6585, 8.2183 )
( 6586, 8.3622 )
( 6587, 8.3622 )
( 6588, 8.3767 )
( 6589, 8.3767 )
( 6590, 8.3907 )
( 6591, 8.3990 )
( 6592, 8.4152 )
( 6593, 8.5736 )
( 6594, 8.6829 )
( 6595, 8.9738 )
( 6596, 9.2261 )
( 6597, 9.2344 )
( 6598, 9.2852 )
( 6599, 9.3365 )
( 6600, 9.3850 )
( 6601, 9.5077 )
( 6602, 9.5077 )
( 6603, 9.5757 )
( 6604, 9.5757 )
( 6605, 9.5902 )
( 6606, 9.6217 )
( 6607, 9.6217 )
( 6608, 9.6886 )
( 6609, 9.8518 )
( 6610, 9.9971 )
( 6611, 10.223 )
( 6612, 10.410 )
( 6613, 10.535 )
( 6614, 10.670 )
( 6615, 10.545 )
( 6616, 10.531 )
( 6617, 10.590 )
( 6618, 10.667 )
( 6619, 10.782 )
( 6620, 10.786 )
( 6621, 10.759 )
( 6622, 10.775 )
( 6623, 11.079 )
( 6624, 11.298 )
( 6625, 11.531 )
( 6626, 11.890 )
( 6627, 12.187 )
( 6628, 12.472 )
( 6629, 12.648 )
( 6630, 12.983 )
( 6631, 13.247 )
( 6632, 13.509 )
( 6633, 13.769 )
( 6634, 13.816 )
( 6635, 13.879 )
( 6636, 13.821 )
( 6637, 13.879 )
( 6638, 13.954 )
( 6639, 14.044 )
( 6640, 14.059 )
( 6641, 14.117 )
( 6642, 14.084 )
( 6643, 14.026 )
( 6644, 13.996 )
( 6645, 13.984 )
( 6646, 13.956 )
( 6647, 13.725 )
( 6648, 13.662 )
( 6649, 13.361 )
( 6650, 13.087 )
( 6651, 12.947 )
( 6652, 12.904 )
( 6653, 12.807 )
( 6654, 12.876 )
( 6655, 12.849 )
( 6656, 12.754 )
( 6657, 12.657 )
( 6658, 12.357 )
( 6659, 12.099 )
( 6660, 11.798 )
( 6661, 11.497 )
( 6662, 11.731 )
( 6663, 11.910 )
( 6664, 12.036 )
( 6665, 12.200 )
( 6666, 12.334 )
( 6667, 12.547 )
( 6668, 12.682 )
( 6669, 12.708 )
( 6670, 12.449 )
( 6671, 12.149 )
( 6672, 11.848 )
( 6673, 11.861 )
( 6674, 11.844 )
( 6675, 11.719 )
( 6676, 11.865 )
( 6677, 11.990 )
( 6678, 11.865 )
( 6679, 11.837 )
( 6680, 11.837 )
( 6681, 12.027 )
( 6682, 12.216 )
( 6683, 12.362 )
( 6684, 12.367 )
( 6685, 12.652 )
( 6686, 12.903 )
( 6687, 13.252 )
( 6688, 13.672 )
( 6689, 14.087 )
( 6690, 14.310 )
( 6691, 14.565 )
( 6692, 14.858 )
( 6693, 14.858 )
( 6694, 14.858 )
( 6695, 14.859 )
( 6696, 14.868 )
( 6697, 14.868 )
( 6698, 14.868 )
( 6699, 14.868 )
( 6700, 14.898 )
( 6701, 14.898 )
( 6702, 15.164 )
( 6703, 15.386 )
( 6704, 15.386 )
( 6705, 15.826 )
( 6706, 16.213 )
( 6707, 16.555 )
( 6708, 16.780 )
( 6709, 17.002 )
( 6710, 17.038 )
( 6711, 17.059 )
( 6712, 17.121 )
( 6713, 17.164 )
( 6714, 17.208 )
( 6715, 17.211 )
( 6716, 17.448 )
( 6717, 17.619 )
( 6718, 17.766 )
( 6719, 17.923 )
( 6720, 18.069 )
( 6721, 18.288 )
( 6722, 18.387 )
( 6723, 18.388 )
( 6724, 18.394 )
( 6725, 18.395 )
( 6726, 18.395 )
( 6727, 18.572 )
( 6728, 18.742 )
( 6729, 18.758 )
( 6730, 18.848 )
( 6731, 18.863 )
( 6732, 18.767 )
( 6733, 18.790 )
( 6734, 18.724 )
( 6735, 18.599 )
( 6736, 18.351 )
( 6737, 18.051 )
( 6738, 17.750 )
( 6739, 17.451 )
( 6740, 17.150 )
( 6741, 16.913 )
( 6742, 16.827 )
( 6743, 16.529 )
( 6744, 16.322 )
( 6745, 16.051 )
( 6746, 15.954 )
( 6747, 15.675 )
( 6748, 15.596 )
( 6749, 15.460 )
( 6750, 15.191 )
( 6751, 14.895 )
( 6752, 14.835 )
( 6753, 14.770 )
( 6754, 14.645 )
( 6755, 14.694 )
( 6756, 14.810 )
( 6757, 14.846 )
( 6758, 14.769 )
( 6759, 14.721 )
( 6760, 14.768 )
( 6761, 14.815 )
( 6762, 14.912 )
( 6763, 15.095 )
( 6764, 15.347 )
( 6765, 15.557 )
( 6766, 15.780 )
( 6767, 15.902 )
( 6768, 15.785 )
( 6769, 15.723 )
( 6770, 15.855 )
( 6771, 15.981 )
( 6772, 16.106 )
( 6773, 16.453 )
( 6774, 16.578 )
( 6775, 16.800 )
( 6776, 16.925 )
( 6777, 17.168 )
( 6778, 17.404 )
( 6779, 17.394 )
( 6780, 17.286 )
( 6781, 17.175 )
( 6782, 17.106 )
( 6783, 17.117 )
( 6784, 17.110 )
( 6785, 17.207 )
( 6786, 17.355 )
( 6787, 17.502 )
( 6788, 17.356 )
( 6789, 17.055 )
( 6790, 16.807 )
( 6791, 16.668 )
( 6792, 16.521 )
( 6793, 16.367 )
( 6794, 16.134 )
( 6795, 15.839 )
( 6796, 15.711 )
( 6797, 15.614 )
( 6798, 15.517 )
( 6799, 15.346 )
( 6800, 15.217 )
( 6801, 14.916 )
( 6802, 14.849 )
( 6803, 14.555 )
( 6804, 14.318 )
( 6805, 14.017 )
( 6806, 13.716 )
( 6807, 13.520 )
( 6808, 13.219 )
( 6809, 12.990 )
( 6810, 12.819 )
( 6811, 12.822 )
( 6812, 12.757 )
( 6813, 12.781 )
( 6814, 12.635 )
( 6815, 12.383 )
( 6816, 12.095 )
( 6817, 11.813 )
( 6818, 11.527 )
( 6819, 11.226 )
( 6820, 10.927 )
( 6821, 10.626 )
( 6822, 10.885 )
( 6823, 11.182 )
( 6824, 11.316 )
( 6825, 11.439 )
( 6826, 11.537 )
( 6827, 11.637 )
( 6828, 11.834 )
( 6829, 12.056 )
( 6830, 12.181 )
( 6831, 12.280 )
( 6832, 12.386 )
( 6833, 12.484 )
( 6834, 12.581 )
( 6835, 12.767 )
( 6836, 13.001 )
( 6837, 13.258 )
( 6838, 13.380 )
( 6839, 13.326 )
( 6840, 13.268 )
( 6841, 13.261 )
( 6842, 13.233 )
( 6843, 13.108 )
( 6844, 12.941 )
( 6845, 12.880 )
( 6846, 12.815 )
( 6847, 12.815 )
( 6848, 12.962 )
( 6849, 13.185 )
( 6850, 13.203 )
( 6851, 13.275 )
( 6852, 13.275 )
( 6853, 13.448 )
( 6854, 13.448 )
( 6855, 13.673 )
( 6856, 13.895 )
( 6857, 14.147 )
( 6858, 14.381 )
( 6859, 14.609 )
( 6860, 14.609 )
( 6861, 14.845 )
( 6862, 15.067 )
( 6863, 15.288 )
( 6864, 15.308 )
( 6865, 15.311 )
( 6866, 15.356 )
( 6867, 15.399 )
( 6868, 15.415 )
( 6869, 15.562 )
( 6870, 15.562 )
( 6871, 15.639 )
( 6872, 15.655 )
( 6873, 15.672 )
( 6874, 15.695 )
( 6875, 15.695 )
( 6876, 15.992 )
( 6877, 16.337 )
( 6878, 16.652 )
( 6879, 16.963 )
( 6880, 17.270 )
( 6881, 17.494 )
( 6882, 17.770 )
( 6883, 17.992 )
( 6884, 18.214 )
( 6885, 18.524 )
( 6886, 18.530 )
( 6887, 18.545 )
( 6888, 18.562 )
( 6889, 18.605 )
( 6890, 18.605 )
( 6891, 18.605 )
( 6892, 18.945 )
( 6893, 19.242 )
( 6894, 19.476 )
( 6895, 19.899 )
( 6896, 20.186 )
( 6897, 20.643 )
( 6898, 20.899 )
( 6899, 21.292 )
( 6900, 21.514 )
( 6901, 21.736 )
( 6902, 22.156 )
( 6903, 22.548 )
( 6904, 22.841 )
( 6905, 23.128 )
( 6906, 23.360 )
( 6907, 23.702 )
( 6908, 24.044 )
( 6909, 24.367 )
( 6910, 24.423 )
( 6911, 24.423 )
( 6912, 24.479 )
( 6913, 24.527 )
( 6914, 24.705 )
( 6915, 24.851 )
( 6916, 24.913 )
( 6917, 24.913 )
( 6918, 24.920 )
( 6919, 24.920 )
( 6920, 24.920 )
( 6921, 25.347 )
( 6922, 25.646 )
( 6923, 25.877 )
( 6924, 26.178 )
( 6925, 26.400 )
( 6926, 26.730 )
( 6927, 27.070 )
( 6928, 27.438 )
( 6929, 27.715 )
( 6930, 27.875 )
( 6931, 28.023 )
( 6932, 28.025 )
( 6933, 28.026 )
( 6934, 28.173 )
( 6935, 28.173 )
( 6936, 28.173 )
( 6937, 28.218 )
( 6938, 28.242 )
( 6939, 28.257 )
( 6940, 28.315 )
( 6941, 28.399 )
( 6942, 28.352 )
( 6943, 28.294 )
( 6944, 28.236 )
( 6945, 28.178 )
( 6946, 28.134 )
( 6947, 28.130 )
( 6948, 28.118 )
( 6949, 28.188 )
( 6950, 28.311 )
( 6951, 28.253 )
( 6952, 28.215 )
( 6953, 28.168 )
( 6954, 28.113 )
( 6955, 28.179 )
( 6956, 28.241 )
( 6957, 28.371 )
( 6958, 28.428 )
( 6959, 28.418 )
( 6960, 28.361 )
( 6961, 28.465 )
( 6962, 28.420 )
( 6963, 28.363 )
( 6964, 28.307 )
( 6965, 28.496 )
( 6966, 28.604 )
( 6967, 28.619 )
( 6968, 28.613 )
( 6969, 28.606 )
( 6970, 28.665 )
( 6971, 28.764 )
( 6972, 28.706 )
( 6973, 28.665 )
( 6974, 28.607 )
( 6975, 28.558 )
( 6976, 28.520 )
( 6977, 28.525 )
( 6978, 28.519 )
( 6979, 28.516 )
( 6980, 28.516 )
( 6981, 28.528 )
( 6982, 28.537 )
( 6983, 28.518 )
( 6984, 28.493 )
( 6985, 28.577 )
( 6986, 28.553 )
( 6987, 28.555 )
( 6988, 28.527 )
( 6989, 28.499 )
( 6990, 28.198 )
( 6991, 27.898 )
( 6992, 27.597 )
( 6993, 27.459 )
( 6994, 27.159 )
( 6995, 26.858 )
( 6996, 26.571 )
( 6997, 26.272 )
( 6998, 26.062 )
( 6999, 25.866 )
( 7000, 25.594 )
( 7001, 25.315 )
( 7002, 25.055 )
( 7003, 24.846 )
( 7004, 24.749 )
( 7005, 24.736 )
( 7006, 24.639 )
( 7007, 24.513 )
( 7008, 24.215 )
( 7009, 24.005 )
( 7010, 23.794 )
( 7011, 23.654 )
( 7012, 23.384 )
( 7013, 23.094 )
( 7014, 22.857 )
( 7015, 22.577 )
( 7016, 22.383 )
( 7017, 22.286 )
( 7018, 22.140 )
( 7019, 22.051 )
( 7020, 21.750 )
( 7021, 21.448 )
( 7022, 21.303 )
( 7023, 21.002 )
( 7024, 20.713 )
( 7025, 20.412 )
( 7026, 20.111 )
( 7027, 19.986 )
( 7028, 19.887 )
( 7029, 19.779 )
( 7030, 19.655 )
( 7031, 19.530 )
( 7032, 19.408 )
( 7033, 19.304 )
( 7034, 19.359 )
( 7035, 19.401 )
( 7036, 19.451 )
( 7037, 19.492 )
( 7038, 19.368 )
( 7039, 19.243 )
( 7040, 19.428 )
( 7041, 19.612 )
( 7042, 19.614 )
( 7043, 19.798 )
( 7044, 20.010 )
( 7045, 20.105 )
( 7046, 20.177 )
( 7047, 20.265 )
( 7048, 20.383 )
( 7049, 20.471 )
( 7050, 20.604 )
( 7051, 20.708 )
( 7052, 20.811 )
( 7053, 21.003 )
( 7054, 21.084 )
( 7055, 21.184 )
( 7056, 21.302 )
( 7057, 21.368 )
( 7058, 21.436 )
( 7059, 21.503 )
( 7060, 21.807 )
( 7061, 22.022 )
( 7062, 22.229 )
( 7063, 22.487 )
( 7064, 22.744 )
( 7065, 22.956 )
( 7066, 23.438 )
( 7067, 23.878 )
( 7068, 24.094 )
( 7069, 24.485 )
( 7070, 24.807 )
( 7071, 25.088 )
( 7072, 25.358 )
( 7073, 25.569 )
( 7074, 25.785 )
( 7075, 25.996 )
( 7076, 26.207 )
( 7077, 26.425 )
( 7078, 26.785 )
( 7079, 27.126 )
( 7080, 27.326 )
( 7081, 27.526 )
( 7082, 27.725 )
( 7083, 27.990 )
( 7084, 28.190 )
( 7085, 28.162 )
( 7086, 28.271 )
( 7087, 28.244 )
( 7088, 28.635 )
( 7089, 29.071 )
( 7090, 29.459 )
( 7091, 29.906 )
( 7092, 30.298 )
( 7093, 30.693 )
( 7094, 31.086 )
( 7095, 31.409 )
( 7096, 31.909 )
( 7097, 32.298 )
( 7098, 32.707 )
( 7099, 33.142 )
( 7100, 33.550 )
( 7101, 33.919 )
( 7102, 34.241 )
( 7103, 34.532 )
( 7104, 34.752 )
( 7105, 34.956 )
( 7106, 35.247 )
( 7107, 35.455 )
( 7108, 35.654 )
( 7109, 35.832 )
( 7110, 35.868 )
( 7111, 35.854 )
( 7112, 35.827 )
( 7113, 35.769 )
( 7114, 35.795 )
( 7115, 35.712 )
( 7116, 35.629 )
( 7117, 35.757 )
( 7118, 35.798 )
( 7119, 35.752 )
( 7120, 35.699 )
( 7121, 35.648 )
( 7122, 35.634 )
( 7123, 35.567 )
( 7124, 35.442 )
( 7125, 35.486 )
( 7126, 35.361 )
( 7127, 35.730 )
( 7128, 36.062 )
( 7129, 36.404 )
( 7130, 36.772 )
( 7131, 36.973 )
( 7132, 37.224 )
( 7133, 37.526 )
( 7134, 37.903 )
( 7135, 38.226 )
( 7136, 38.465 )
( 7137, 38.710 )
( 7138, 39.060 )
( 7139, 39.409 )
( 7140, 39.743 )
( 7141, 40.033 )
( 7142, 40.235 )
( 7143, 40.453 )
( 7144, 40.671 )
( 7145, 40.877 )
( 7146, 41.168 )
( 7147, 41.369 )
( 7148, 41.585 )
( 7149, 41.845 )
( 7150, 42.189 )
( 7151, 42.511 )
( 7152, 42.772 )
( 7153, 43.126 )
( 7154, 43.381 )
( 7155, 43.631 )
( 7156, 43.977 )
( 7157, 44.299 )
( 7158, 44.629 )
( 7159, 44.951 )
( 7160, 45.265 )
( 7161, 45.578 )
( 7162, 45.891 )
( 7163, 46.175 )
( 7164, 46.494 )
( 7165, 46.804 )
( 7166, 47.036 )
( 7167, 47.351 )
( 7168, 47.659 )
( 7169, 47.952 )
( 7170, 48.254 )
( 7171, 48.549 )
( 7172, 48.782 )
( 7173, 49.197 )
( 7174, 49.575 )
( 7175, 49.847 )
( 7176, 50.222 )
( 7177, 50.603 )
( 7178, 50.923 )
( 7179, 51.211 )
( 7180, 51.470 )
( 7181, 51.670 )
( 7182, 51.931 )
( 7183, 52.131 )
( 7184, 52.330 )
( 7185, 52.654 )
( 7186, 52.905 )
( 7187, 53.117 )
( 7188, 53.318 )
( 7189, 53.531 )
( 7190, 53.805 )
( 7191, 54.041 )
( 7192, 54.265 )
( 7193, 54.663 )
( 7194, 55.035 )
( 7195, 55.389 )
( 7196, 55.760 )
( 7197, 56.082 )
( 7198, 56.337 )
( 7199, 56.680 )
( 7200, 56.971 )
( 7201, 57.170 )
( 7202, 57.370 )
( 7203, 57.633 )
( 7204, 57.926 )
( 7205, 58.392 )
( 7206, 58.745 )
( 7207, 58.754 )
( 7208, 58.776 )
( 7209, 58.786 )
( 7210, 59.082 )
( 7211, 59.390 )
( 7212, 59.692 )
( 7213, 59.919 )
( 7214, 59.906 )
( 7215, 59.790 )
( 7216, 59.665 )
( 7217, 59.563 )
( 7218, 59.478 )
( 7219, 59.481 )
( 7220, 59.377 )
( 7221, 59.253 )
( 7222, 59.134 )
( 7223, 59.009 )
( 7224, 58.884 )
( 7225, 59.020 )
( 7226, 58.895 )
( 7227, 58.820 )
( 7228, 58.737 )
( 7229, 58.617 )
( 7230, 58.576 )
( 7231, 58.451 )
( 7232, 58.326 )
( 7233, 58.239 )
( 7234, 58.114 )
( 7235, 57.989 )
( 7236, 57.998 )
( 7237, 58.007 )
( 7238, 58.005 )
( 7239, 57.977 )
( 7240, 57.950 )
( 7241, 57.892 )
( 7242, 57.835 )
( 7243, 57.777 )
( 7244, 57.503 )
( 7245, 57.202 )
( 7246, 56.972 )
( 7247, 56.721 )
( 7248, 56.420 )
( 7249, 56.274 )
( 7250, 56.146 )
( 7251, 56.008 )
( 7252, 55.708 )
( 7253, 55.622 )
( 7254, 55.566 )
( 7255, 55.430 )
( 7256, 55.293 )
( 7257, 55.257 )
( 7258, 54.957 )
( 7259, 54.655 )
( 7260, 54.360 )
( 7261, 54.095 )
( 7262, 53.794 )
( 7263, 53.512 )
( 7264, 53.210 )
( 7265, 53.000 )
( 7266, 52.699 )
( 7267, 52.868 )
( 7268, 52.861 )
( 7269, 52.847 )
( 7270, 52.896 )
( 7271, 52.777 )
( 7272, 52.694 )
( 7273, 52.573 )
( 7274, 52.451 )
( 7275, 52.493 )
( 7276, 52.379 )
( 7277, 52.354 )
( 7278, 52.230 )
( 7279, 52.341 )
( 7280, 52.216 )
( 7281, 51.915 )
( 7282, 51.657 )
( 7283, 51.356 )
( 7284, 51.403 )
( 7285, 51.512 )
( 7286, 51.415 )
( 7287, 51.180 )
( 7288, 50.882 )
( 7289, 50.581 )
( 7290, 50.318 )
( 7291, 50.017 )
( 7292, 49.847 )
( 7293, 49.795 )
( 7294, 49.698 )
( 7295, 49.397 )
( 7296, 49.146 )
( 7297, 48.852 )
( 7298, 48.551 )
( 7299, 48.250 )
( 7300, 48.327 )
( 7301, 48.356 )
( 7302, 48.359 )
( 7303, 48.396 )
( 7304, 48.410 )
( 7305, 48.411 )
( 7306, 48.458 )
( 7307, 48.458 )
( 7308, 48.458 )
( 7309, 48.531 )
( 7310, 48.723 )
( 7311, 48.881 )
( 7312, 48.951 )
( 7313, 49.170 )
( 7314, 49.173 )
( 7315, 49.174 )
( 7316, 49.174 )
( 7317, 49.174 )
( 7318, 49.324 )
( 7319, 49.324 )
( 7320, 49.339 )
( 7321, 49.354 )
( 7322, 49.432 )
( 7323, 49.172 )
( 7324, 49.056 )
( 7325, 48.756 )
( 7326, 48.463 )
( 7327, 48.172 )
( 7328, 47.896 )
( 7329, 47.594 )
( 7330, 47.450 )
( 7331, 47.305 )
( 7332, 47.003 )
( 7333, 46.767 )
( 7334, 46.466 )
( 7335, 46.165 )
( 7336, 46.024 )
( 7337, 45.890 )
( 7338, 45.863 )
( 7339, 45.836 )
( 7340, 45.535 )
( 7341, 45.234 )
( 7342, 44.936 )
( 7343, 44.635 )
( 7344, 44.375 )
( 7345, 44.195 )
( 7346, 43.915 )
( 7347, 43.719 )
( 7348, 43.573 )
( 7349, 43.532 )
( 7350, 43.231 )
( 7351, 42.931 )
( 7352, 42.931 )
( 7353, 42.667 )
( 7354, 42.426 )
( 7355, 42.135 )
( 7356, 41.834 )
( 7357, 41.551 )
( 7358, 41.250 )
( 7359, 41.063 )
( 7360, 40.762 )
( 7361, 40.465 )
( 7362, 40.164 )
( 7363, 39.863 )
( 7364, 39.615 )
( 7365, 39.518 )
( 7366, 39.421 )
( 7367, 39.120 )
( 7368, 38.891 )
( 7369, 38.771 )
( 7370, 38.577 )
( 7371, 38.429 )
( 7372, 38.146 )
( 7373, 37.944 )
( 7374, 37.648 )
( 7375, 37.503 )
( 7376, 37.213 )
( 7377, 36.912 )
( 7378, 36.825 )
( 7379, 36.524 )
( 7380, 36.235 )
( 7381, 35.965 )
( 7382, 35.978 )
( 7383, 35.676 )
( 7384, 35.565 )
( 7385, 35.419 )
( 7386, 35.119 )
( 7387, 34.819 )
( 7388, 34.759 )
( 7389, 34.499 )
( 7390, 34.198 )
( 7391, 33.967 )
( 7392, 33.800 )
( 7393, 33.676 )
( 7394, 33.637 )
( 7395, 33.407 )
( 7396, 33.139 )
( 7397, 32.847 )
( 7398, 32.750 )
( 7399, 32.456 )
( 7400, 32.398 )
( 7401, 32.324 )
( 7402, 32.250 )
( 7403, 32.054 )
( 7404, 31.801 )
( 7405, 31.500 )
( 7406, 31.200 )
( 7407, 30.899 )
( 7408, 30.599 )
( 7409, 30.325 )
( 7410, 30.228 )
( 7411, 29.947 )
( 7412, 29.796 )
( 7413, 29.495 )
( 7414, 29.519 )
( 7415, 29.414 )
( 7416, 29.113 )
( 7417, 28.817 )
( 7418, 28.756 )
( 7419, 28.660 )
( 7420, 28.567 )
( 7421, 28.523 )
( 7422, 28.468 )
( 7423, 28.411 )
( 7424, 28.110 )
( 7425, 27.809 )
( 7426, 27.508 )
( 7427, 27.365 )
( 7428, 27.219 )
( 7429, 26.918 )
( 7430, 26.617 )
( 7431, 26.466 )
( 7432, 26.345 )
( 7433, 26.278 )
( 7434, 26.188 )
( 7435, 25.887 )
( 7436, 25.777 )
( 7437, 25.652 )
( 7438, 25.527 )
( 7439, 25.595 )
( 7440, 25.720 )
( 7441, 25.845 )
( 7442, 25.970 )
( 7443, 26.269 )
( 7444, 26.577 )
( 7445, 26.988 )
( 7446, 27.402 )
( 7447, 27.809 )
( 7448, 28.240 )
( 7449, 28.646 )
( 7450, 29.056 )
( 7451, 29.462 )
( 7452, 29.892 )
( 7453, 30.323 )
( 7454, 30.766 )
( 7455, 31.171 )
( 7456, 31.655 )
( 7457, 32.080 )
( 7458, 32.471 )
( 7459, 32.863 )
( 7460, 33.272 )
( 7461, 33.683 )
( 7462, 34.089 )
( 7463, 34.373 )
( 7464, 34.648 )
( 7465, 34.774 )
( 7466, 34.923 )
( 7467, 35.059 )
( 7468, 35.184 )
( 7469, 35.111 )
( 7470, 34.999 )
( 7471, 34.921 )
( 7472, 34.797 )
( 7473, 34.672 )
( 7474, 34.643 )
( 7475, 34.588 )
( 7476, 34.530 )
( 7477, 34.595 )
( 7478, 34.654 )
( 7479, 34.721 )
( 7480, 34.714 )
( 7481, 34.721 )
( 7482, 34.874 )
( 7483, 34.906 )
( 7484, 34.975 )
( 7485, 35.011 )
( 7486, 34.998 )
( 7487, 34.984 )
( 7488, 34.956 )
( 7489, 35.107 )
( 7490, 35.304 )
( 7491, 35.464 )
( 7492, 35.698 )
( 7493, 35.853 )
( 7494, 35.975 )
( 7495, 35.947 )
( 7496, 35.919 )
( 7497, 35.861 )
( 7498, 35.803 )
( 7499, 35.797 )
( 7500, 35.739 )
( 7501, 35.482 )
( 7502, 35.193 )
( 7503, 34.892 )
( 7504, 34.591 )
( 7505, 34.298 )
( 7506, 34.028 )
( 7507, 33.727 )
( 7508, 33.579 )
( 7509, 33.278 )
( 7510, 33.182 )
( 7511, 32.977 )
( 7512, 32.780 )
( 7513, 32.522 )
( 7514, 32.235 )
( 7515, 31.935 )
( 7516, 31.634 )
( 7517, 31.756 )
( 7518, 31.799 )
( 7519, 31.702 )
( 7520, 31.402 )
( 7521, 31.101 )
( 7522, 30.890 )
( 7523, 30.591 )
( 7524, 30.290 )
( 7525, 30.023 )
( 7526, 29.828 )
( 7527, 29.527 )
( 7528, 29.241 )
( 7529, 28.943 )
( 7530, 28.642 )
( 7531, 28.341 )
( 7532, 28.195 )
( 7533, 28.195 )
( 7534, 27.948 )
( 7535, 27.646 )
( 7536, 27.646 )
( 7537, 27.858 )
( 7538, 28.004 )
( 7539, 28.004 )
( 7540, 28.150 )
( 7541, 28.174 )
( 7542, 28.189 )
( 7543, 28.208 )
( 7544, 28.285 )
( 7545, 28.372 )
( 7546, 28.374 )
( 7547, 28.374 )
( 7548, 28.477 )
( 7549, 28.482 )
( 7550, 28.485 )
( 7551, 28.539 )
( 7552, 28.539 )
( 7553, 28.790 )
( 7554, 29.056 )
( 7555, 29.283 )
( 7556, 29.505 )
( 7557, 29.982 )
( 7558, 30.409 )
( 7559, 30.691 )
( 7560, 30.969 )
( 7561, 31.005 )
( 7562, 31.007 )
( 7563, 31.007 )
( 7564, 31.153 )
( 7565, 31.153 )
( 7566, 31.153 )
( 7567, 31.300 )
( 7568, 31.325 )
( 7569, 31.325 )
( 7570, 31.387 )
( 7571, 31.449 )
( 7572, 31.449 )
( 7573, 31.560 )
( 7574, 31.625 )
( 7575, 31.728 )
( 7576, 31.967 )
( 7577, 32.193 )
( 7578, 32.417 )
( 7579, 32.642 )
( 7580, 32.864 )
( 7581, 33.131 )
( 7582, 33.354 )
( 7583, 33.575 )
( 7584, 33.797 )
( 7585, 34.133 )
( 7586, 34.488 )
( 7587, 34.842 )
( 7588, 35.156 )
( 7589, 35.451 )
( 7590, 35.744 )
( 7591, 35.984 )
( 7592, 36.212 )
( 7593, 36.436 )
( 7594, 36.647 )
( 7595, 36.806 )
( 7596, 36.806 )
( 7597, 36.806 )
( 7598, 36.806 )
( 7599, 36.904 )
( 7600, 36.909 )
( 7601, 36.958 )
( 7602, 37.175 )
( 7603, 37.385 )
( 7604, 37.580 )
( 7605, 37.758 )
( 7606, 37.917 )
( 7607, 37.917 )
( 7608, 37.946 )
( 7609, 37.946 )
( 7610, 37.947 )
( 7611, 37.987 )
( 7612, 38.008 )
( 7613, 38.009 )
( 7614, 38.231 )
( 7615, 38.465 )
( 7616, 38.722 )
( 7617, 38.722 )
( 7618, 38.722 )
( 7619, 38.722 )
( 7620, 38.737 )
( 7621, 38.755 )
( 7622, 38.796 )
( 7623, 38.847 )
( 7624, 38.904 )
( 7625, 38.961 )
( 7626, 39.020 )
( 7627, 39.097 )
( 7628, 39.159 )
( 7629, 39.267 )
( 7630, 39.356 )
( 7631, 39.396 )
( 7632, 39.556 )
( 7633, 39.591 )
( 7634, 39.625 )
( 7635, 39.654 )
( 7636, 39.717 )
( 7637, 39.779 )
( 7638, 40.123 )
( 7639, 40.512 )
( 7640, 40.872 )
( 7641, 41.231 )
( 7642, 41.574 )
( 7643, 41.805 )
( 7644, 42.128 )
( 7645, 42.418 )
( 7646, 42.705 )
( 7647, 42.988 )
( 7648, 43.278 )
( 7649, 43.676 )
( 7650, 43.963 )
( 7651, 44.225 )
( 7652, 44.448 )
( 7653, 44.671 )
( 7654, 44.910 )
( 7655, 44.921 )
( 7656, 45.143 )
( 7657, 45.143 )
( 7658, 45.143 )
( 7659, 45.143 )
( 7660, 45.143 )
( 7661, 45.292 )
( 7662, 45.444 )
( 7663, 45.590 )
( 7664, 45.590 )
( 7665, 45.630 )
( 7666, 45.654 )
( 7667, 45.654 )
( 7668, 45.666 )
( 7669, 45.667 )
( 7670, 45.713 )
( 7671, 45.722 )
( 7672, 45.722 )
( 7673, 45.772 )
( 7674, 45.772 )
( 7675, 45.918 )
( 7676, 46.070 )
( 7677, 46.119 )
( 7678, 46.331 )
( 7679, 46.418 )
( 7680, 46.491 )
( 7681, 46.554 )
( 7682, 46.645 )
( 7683, 46.646 )
( 7684, 46.698 )
( 7685, 46.771 )
( 7686, 46.771 )
( 7687, 46.771 )
( 7688, 46.771 )
( 7689, 46.836 )
( 7690, 46.836 )
( 7691, 47.179 )
( 7692, 47.531 )
( 7693, 47.753 )
( 7694, 47.753 )
( 7695, 47.987 )
( 7696, 48.309 )
( 7697, 48.564 )
( 7698, 48.838 )
( 7699, 49.093 )
( 7700, 49.327 )
( 7701, 49.570 )
( 7702, 49.801 )
( 7703, 50.026 )
( 7704, 50.196 )
( 7705, 50.521 )
( 7706, 50.815 )
( 7707, 51.087 )
( 7708, 51.422 )
( 7709, 51.777 )
( 7710, 52.145 )
( 7711, 52.504 )
( 7712, 52.813 )
( 7713, 53.106 )
( 7714, 53.118 )
( 7715, 53.167 )
( 7716, 53.313 )
( 7717, 53.357 )
( 7718, 53.365 )
( 7719, 53.371 )
( 7720, 53.375 )
( 7721, 53.376 )
( 7722, 53.376 )
( 7723, 53.457 )
( 7724, 53.530 )
( 7725, 53.592 )
( 7726, 53.608 )
( 7727, 53.662 )
( 7728, 53.662 )
( 7729, 53.662 )
( 7730, 53.835 )
( 7731, 53.982 )
( 7732, 54.004 )
( 7733, 54.055 )
( 7734, 54.225 )
( 7735, 54.384 )
( 7736, 54.531 )
( 7737, 54.731 )
( 7738, 54.731 )
( 7739, 54.733 )
( 7740, 54.879 )
( 7741, 54.955 )
( 7742, 54.955 )
( 7743, 55.006 )
( 7744, 55.006 )
( 7745, 55.036 )
( 7746, 55.036 )
( 7747, 55.036 )
( 7748, 55.039 )
( 7749, 55.231 )
( 7750, 55.377 )
( 7751, 55.535 )
( 7752, 55.681 )
( 7753, 55.753 )
( 7754, 55.899 )
( 7755, 55.915 )
( 7756, 56.020 )
( 7757, 56.039 )
( 7758, 56.101 )
( 7759, 56.176 )
( 7760, 56.176 )
( 7761, 56.239 )
( 7762, 56.305 )
( 7763, 56.368 )
( 7764, 56.750 )
( 7765, 57.133 )
( 7766, 57.459 )
( 7767, 57.839 )
( 7768, 58.168 )
( 7769, 58.557 )
( 7770, 58.924 )
( 7771, 59.324 )
( 7772, 59.559 )
( 7773, 59.933 )
( 7774, 60.286 )
( 7775, 60.510 )
( 7776, 60.731 )
( 7777, 60.959 )
( 7778, 61.203 )
( 7779, 61.425 )
( 7780, 61.648 )
( 7781, 61.880 )
( 7782, 62.141 )
( 7783, 62.387 )
( 7784, 62.633 )
( 7785, 62.854 )
( 7786, 63.095 )
( 7787, 63.096 )
( 7788, 63.132 )
( 7789, 63.195 )
( 7790, 63.352 )
( 7791, 63.498 )
( 7792, 63.675 )
( 7793, 63.711 )
( 7794, 63.773 )
( 7795, 63.817 )
( 7796, 63.820 )
( 7797, 63.820 )
( 7798, 63.993 )
( 7799, 64.149 )
( 7800, 64.179 )
( 7801, 64.260 )
( 7802, 64.309 )
( 7803, 64.309 )
( 7804, 64.331 )
( 7805, 64.410 )
( 7806, 64.410 )
( 7807, 64.410 )
( 7808, 64.410 )
( 7809, 64.439 )
( 7810, 64.439 )
( 7811, 64.439 )
( 7812, 64.449 )
( 7813, 64.449 )
( 7814, 64.464 )
( 7815, 64.384 )
( 7816, 64.083 )
( 7817, 63.784 )
( 7818, 63.809 )
( 7819, 63.833 )
( 7820, 63.784 )
( 7821, 63.489 )
( 7822, 63.194 )
( 7823, 62.963 )
( 7824, 62.669 )
( 7825, 62.736 )
( 7826, 62.640 )
( 7827, 62.429 )
( 7828, 62.158 )
( 7829, 61.858 )
( 7830, 61.560 )
( 7831, 61.494 )
( 7832, 61.338 )
( 7833, 61.049 )
( 7834, 60.954 )
( 7835, 60.862 )
( 7836, 60.768 )
( 7837, 60.724 )
( 7838, 60.627 )
( 7839, 60.536 )
( 7840, 60.439 )
( 7841, 60.146 )
( 7842, 60.087 )
( 7843, 60.059 )
( 7844, 59.815 )
( 7845, 59.613 )
( 7846, 59.313 )
( 7847, 59.042 )
( 7848, 58.742 )
( 7849, 58.441 )
( 7850, 58.245 )
( 7851, 58.050 )
( 7852, 57.958 )
( 7853, 57.861 )
( 7854, 57.796 )
( 7855, 57.699 )
( 7856, 57.398 )
( 7857, 57.339 )
( 7858, 57.294 )
( 7859, 56.994 )
( 7860, 56.694 )
( 7861, 56.398 )
( 7862, 56.097 )
( 7863, 55.796 )
( 7864, 55.538 )
( 7865, 55.250 )
( 7866, 55.043 )
( 7867, 54.743 )
( 7868, 54.442 )
( 7869, 54.296 )
( 7870, 54.114 )
( 7871, 53.918 )
( 7872, 53.722 )
( 7873, 53.421 )
( 7874, 53.161 )
( 7875, 52.860 )
( 7876, 52.755 )
( 7877, 52.467 )
( 7878, 52.209 )
( 7879, 51.981 )
( 7880, 51.753 )
( 7881, 51.494 )
( 7882, 51.200 )
( 7883, 50.908 )
( 7884, 50.607 )
( 7885, 50.306 )
( 7886, 50.279 )
( 7887, 50.182 )
( 7888, 50.185 )
( 7889, 50.136 )
( 7890, 50.190 )
( 7891, 50.054 )
( 7892, 49.753 )
( 7893, 49.452 )
( 7894, 49.355 )
( 7895, 49.314 )
( 7896, 49.222 )
( 7897, 48.923 )
( 7898, 48.712 )
( 7899, 48.682 )
( 7900, 48.584 )
( 7901, 48.438 )
( 7902, 48.179 )
( 7903, 47.879 )
( 7904, 47.744 )
( 7905, 47.598 )
( 7906, 47.470 )
( 7907, 47.181 )
( 7908, 46.955 )
( 7909, 46.722 )
( 7910, 46.492 )
( 7911, 46.191 )
( 7912, 45.961 )
( 7913, 45.661 )
( 7914, 45.360 )
( 7915, 45.059 )
( 7916, 44.855 )
( 7917, 44.554 )
( 7918, 44.361 )
( 7919, 44.065 )
( 7920, 43.980 )
( 7921, 43.885 )
( 7922, 43.815 )
( 7923, 43.722 )
( 7924, 43.685 )
( 7925, 43.587 )
( 7926, 43.596 )
( 7927, 43.532 )
( 7928, 43.469 )
( 7929, 43.290 )
( 7930, 42.989 )
( 7931, 42.705 )
( 7932, 42.568 )
( 7933, 42.541 )
( 7934, 42.240 )
( 7935, 42.029 )
( 7936, 41.811 )
( 7937, 41.510 )
( 7938, 41.209 )
( 7939, 40.908 )
( 7940, 40.609 )
( 7941, 40.468 )
( 7942, 40.565 )
( 7943, 40.264 )
( 7944, 40.027 )
( 7945, 39.886 )
( 7946, 39.742 )
( 7947, 39.560 )
( 7948, 39.432 )
( 7949, 39.139 )
( 7950, 38.881 )
( 7951, 38.735 )
( 7952, 38.621 )
( 7953, 38.645 )
( 7954, 38.586 )
( 7955, 38.599 )
( 7956, 38.299 )
( 7957, 38.103 )
( 7958, 37.802 )
( 7959, 37.774 )
( 7960, 37.756 )
( 7961, 37.729 )
( 7962, 37.777 )
( 7963, 37.750 )
( 7964, 37.723 )
( 7965, 37.777 )
( 7966, 37.750 )
( 7967, 37.650 )
( 7968, 37.525 )
( 7969, 37.495 )
( 7970, 37.423 )
( 7971, 37.348 )
( 7972, 37.257 )
( 7973, 37.201 )
( 7974, 37.089 )
( 7975, 36.964 )
( 7976, 36.865 )
( 7977, 36.980 )
( 7978, 36.911 )
( 7979, 36.872 )
( 7980, 36.748 )
( 7981, 36.446 )
( 7982, 36.146 )
( 7983, 35.984 )
( 7984, 35.788 )
( 7985, 35.812 )
( 7986, 35.715 )
( 7987, 35.649 )
( 7988, 35.584 )
( 7989, 35.368 )
( 7990, 35.067 )
( 7991, 34.970 )
( 7992, 34.778 )
( 7993, 34.570 )
( 7994, 34.333 )
( 7995, 34.032 )
( 7996, 33.886 )
( 7997, 33.587 )
( 7998, 33.566 )
( 7999, 33.470 )
( 8000, 33.383 )
( 8001, 33.288 )
( 8002, 32.987 )
( 8003, 32.686 )
( 8004, 32.385 )
( 8005, 32.189 )
( 8006, 32.078 )
( 8007, 31.777 )
( 8008, 31.487 )
( 8009, 31.257 )
( 8010, 30.962 )
( 8011, 30.661 )
( 8012, 30.465 )
( 8013, 30.319 )
( 8014, 30.018 )
( 8015, 29.718 )
( 8016, 29.493 )
( 8017, 29.192 )
( 8018, 29.064 )
( 8019, 28.764 )
( 8020, 28.503 )
( 8021, 28.209 )
( 8022, 27.979 )
( 8023, 27.678 )
( 8024, 27.377 )
( 8025, 27.082 )
( 8026, 27.104 )
( 8027, 26.822 )
( 8028, 26.628 )
( 8029, 26.328 )
( 8030, 26.247 )
( 8031, 26.073 )
( 8032, 25.772 )
( 8033, 25.503 )
( 8034, 25.255 )
( 8035, 25.025 )
( 8036, 24.766 )
( 8037, 24.495 )
( 8038, 24.194 )
( 8039, 24.048 )
( 8040, 23.764 )
( 8041, 23.464 )
( 8042, 23.163 )
( 8043, 22.862 )
( 8044, 22.682 )
( 8045, 22.434 )
( 8046, 22.224 )
( 8047, 22.165 )
( 8048, 22.068 )
( 8049, 21.983 )
( 8050, 21.929 )
( 8051, 21.681 )
( 8052, 21.386 )
( 8053, 21.140 )
( 8054, 20.868 )
( 8055, 20.567 )
( 8056, 20.309 )
( 8057, 20.008 )
( 8058, 19.707 )
( 8059, 19.465 )
( 8060, 19.217 )
( 8061, 19.095 )
( 8062, 18.965 )
( 8063, 18.819 )
( 8064, 18.750 )
( 8065, 18.656 )
( 8066, 18.355 )
( 8067, 18.157 )
( 8068, 18.060 )
( 8069, 17.963 )
( 8070, 17.776 )
( 8071, 17.824 )
( 8072, 17.809 )
( 8073, 17.782 )
( 8074, 18.105 )
( 8075, 18.448 )
( 8076, 18.508 )
( 8077, 18.480 )
( 8078, 18.250 )
( 8079, 17.954 )
( 8080, 17.653 )
( 8081, 17.609 )
( 8082, 17.481 )
( 8083, 17.408 )
( 8084, 17.433 )
( 8085, 17.517 )
( 8086, 17.416 )
( 8087, 17.269 )
( 8088, 16.968 )
( 8089, 16.871 )
( 8090, 16.712 )
( 8091, 16.413 )
( 8092, 16.321 )
( 8093, 16.224 )
( 8094, 16.291 )
( 8095, 16.203 )
( 8096, 16.112 )
( 8097, 15.811 )
( 8098, 15.553 )
( 8099, 15.281 )
( 8100, 14.980 )
( 8101, 14.852 )
( 8102, 14.727 )
( 8103, 14.435 )
( 8104, 14.134 )
( 8105, 13.937 )
( 8106, 13.863 )
( 8107, 13.579 )
( 8108, 13.349 )
( 8109, 13.165 )
( 8110, 12.866 )
( 8111, 12.618 )
( 8112, 12.317 )
( 8113, 12.412 )
( 8114, 12.111 )
( 8115, 11.844 )
( 8116, 11.543 )
( 8117, 11.446 )
( 8118, 11.386 )
( 8119, 11.294 )
( 8120, 10.993 )
( 8121, 11.238 )
( 8122, 11.408 )
( 8123, 11.370 )
( 8124, 11.266 )
( 8125, 11.141 )
( 8126, 10.842 )
( 8127, 10.551 )
( 8128, 10.251 )
( 8129, 10.109 )
( 8130, 9.8615 )
( 8131, 9.5635 )
( 8132, 9.4979 )
( 8133, 9.4058 )
( 8134, 9.1246 )
( 8135, 8.8236 )
( 8136, 8.5513 )
( 8137, 8.2502 )
( 8138, 7.9492 )
( 8139, 7.8315 )
( 8140, 7.7110 )
( 8141, 7.8951 )
( 8142, 7.8951 )
( 8143, 7.8999 )
( 8144, 7.9096 )
( 8145, 7.9096 )
( 8146, 8.2892 )
( 8147, 8.5588 )
( 8148, 8.8129 )
( 8149, 8.8129 )
( 8150, 8.9038 )
( 8151, 9.0081 )
( 8152, 9.0952 )
( 8153, 9.2043 )
( 8154, 9.3766 )
( 8155, 9.4994 )
( 8156, 9.5001 )
( 8157, 9.5858 )
( 8158, 9.5858 )
( 8159, 9.6479 )
( 8160, 9.6482 )
( 8161, 9.6609 )
( 8162, 9.7338 )
( 8163, 9.7483 )
( 8164, 9.7777 )
( 8165, 9.7777 )
( 8166, 9.9255 )
( 8167, 9.9335 )
( 8168, 9.9956 )
( 8169, 9.9956 )
( 8170, 10.230 )
( 8171, 10.381 )
( 8172, 10.479 )
( 8173, 10.690 )
( 8174, 10.776 )
( 8175, 10.870 )
( 8176, 11.253 )
( 8177, 11.527 )
( 8178, 11.706 )
( 8179, 11.903 )
( 8180, 12.100 )
( 8181, 12.290 )
( 8182, 12.505 )
( 8183, 12.736 )
( 8184, 12.912 )
( 8185, 13.119 )
( 8186, 13.295 )
( 8187, 13.512 )
( 8188, 13.688 )
( 8189, 13.943 )
( 8190, 14.131 )
( 8191, 14.308 )
( 8192, 14.557 )
( 8193, 14.734 )
( 8194, 14.921 )
( 8195, 15.265 )
( 8196, 15.520 )
( 8197, 15.657 )
( 8198, 15.783 )
( 8199, 16.108 )
( 8200, 16.427 )
( 8201, 16.691 )
( 8202, 16.817 )
( 8203, 16.692 )
( 8204, 16.484 )
( 8205, 16.183 )
( 8206, 15.913 )
( 8207, 15.763 )
( 8208, 15.532 )
( 8209, 15.436 )
( 8210, 15.475 )
( 8211, 15.188 )
( 8212, 14.946 )
( 8213, 14.645 )
( 8214, 14.687 )
( 8215, 14.552 )
( 8216, 14.256 )
( 8217, 13.955 )
( 8218, 13.654 )
( 8219, 13.823 )
( 8220, 13.896 )
( 8221, 13.896 )
( 8222, 14.042 )
( 8223, 14.042 )
( 8224, 14.246 )
( 8225, 14.381 )
( 8226, 14.392 )
( 8227, 14.404 )
( 8228, 14.408 )
( 8229, 14.408 )
( 8230, 14.408 )
( 8231, 14.438 )
( 8232, 14.714 )
( 8233, 14.714 )
( 8234, 14.735 )
( 8235, 14.735 )
( 8236, 14.965 )
( 8237, 14.965 )
( 8238, 14.965 )
( 8239, 14.965 )
( 8240, 15.127 )
( 8241, 15.318 )
( 8242, 15.530 )
( 8243, 15.705 )
( 8244, 15.875 )
( 8245, 15.935 )
( 8246, 15.936 )
( 8247, 15.959 )
( 8248, 16.105 )
( 8249, 16.251 )
( 8250, 16.452 )
( 8251, 16.514 )
( 8252, 16.514 )
( 8253, 16.937 )
( 8254, 17.335 )
( 8255, 17.728 )
( 8256, 18.153 )
( 8257, 18.453 )
( 8258, 18.848 )
( 8259, 19.355 )
( 8260, 19.791 )
( 8261, 20.196 )
( 8262, 20.640 )
( 8263, 21.033 )
( 8264, 21.502 )
( 8265, 21.906 )
( 8266, 22.199 )
( 8267, 22.492 )
( 8268, 22.787 )
( 8269, 23.119 )
( 8270, 23.407 )
( 8271, 23.823 )
( 8272, 24.049 )
( 8273, 24.302 )
( 8274, 24.648 )
( 8275, 24.995 )
( 8276, 25.261 )
( 8277, 25.487 )
( 8278, 25.708 )
( 8279, 25.930 )
( 8280, 26.200 )
( 8281, 26.422 )
( 8282, 26.764 )
( 8283, 27.112 )
( 8284, 27.385 )
( 8285, 27.678 )
( 8286, 27.910 )
( 8287, 28.142 )
( 8288, 28.364 )
( 8289, 28.708 )
( 8290, 29.001 )
( 8291, 29.354 )
( 8292, 29.650 )
( 8293, 29.886 )
( 8294, 30.167 )
( 8295, 30.448 )
( 8296, 30.670 )
( 8297, 30.894 )
( 8298, 31.115 )
( 8299, 31.379 )
( 8300, 31.603 )
( 8301, 31.825 )
( 8302, 32.143 )
( 8303, 32.426 )
( 8304, 32.708 )
( 8305, 32.941 )
( 8306, 33.090 )
( 8307, 33.090 )
( 8308, 33.090 )
( 8309, 33.103 )
( 8310, 33.103 )
( 8311, 33.131 )
( 8312, 33.131 )
( 8313, 33.131 )
( 8314, 33.421 )
( 8315, 33.742 )
( 8316, 33.975 )
( 8317, 34.215 )
( 8318, 34.448 )
( 8319, 34.696 )
( 8320, 34.885 )
( 8321, 35.077 )
( 8322, 35.253 )
( 8323, 35.432 )
( 8324, 35.619 )
( 8325, 35.795 )
( 8326, 35.972 )
( 8327, 36.148 )
( 8328, 36.386 )
( 8329, 36.655 )
( 8330, 37.057 )
( 8331, 37.394 )
( 8332, 37.696 )
( 8333, 37.946 )
( 8334, 38.283 )
( 8335, 38.624 )
( 8336, 38.874 )
( 8337, 39.169 )
( 8338, 39.419 )
( 8339, 39.675 )
( 8340, 39.912 )
( 8341, 40.167 )
( 8342, 40.422 )
( 8343, 40.692 )
( 8344, 40.924 )
( 8345, 41.131 )
( 8346, 41.339 )
( 8347, 41.283 )
( 8348, 41.238 )
( 8349, 41.180 )
( 8350, 41.122 )
( 8351, 41.095 )
( 8352, 41.192 )
( 8353, 41.354 )
( 8354, 41.498 )
( 8355, 41.602 )
( 8356, 41.949 )
( 8357, 42.238 )
( 8358, 42.469 )
( 8359, 42.569 )
( 8360, 42.750 )
( 8361, 42.861 )
( 8362, 42.976 )
( 8363, 43.113 )
( 8364, 43.265 )
( 8365, 43.393 )
( 8366, 43.489 )
( 8367, 43.586 )
( 8368, 43.683 )
( 8369, 43.782 )
( 8370, 43.879 )
( 8371, 43.989 )
( 8372, 44.245 )
( 8373, 44.478 )
( 8374, 44.608 )
( 8375, 44.580 )
( 8376, 44.732 )
( 8377, 44.855 )
( 8378, 44.827 )
( 8379, 44.949 )
( 8380, 45.072 )
( 8381, 45.251 )
( 8382, 45.432 )
( 8383, 45.556 )
( 8384, 45.640 )
( 8385, 45.614 )
( 8386, 45.639 )
( 8387, 45.625 )
( 8388, 45.702 )
( 8389, 45.733 )
( 8390, 45.719 )
( 8391, 45.854 )
( 8392, 45.849 )
( 8393, 45.835 )
( 8394, 45.794 )
( 8395, 45.669 )
( 8396, 45.545 )
( 8397, 45.308 )
( 8398, 45.006 )
( 8399, 44.706 )
( 8400, 44.608 )
( 8401, 44.633 )
( 8402, 44.332 )
( 8403, 44.094 )
( 8404, 43.998 )
( 8405, 44.039 )
( 8406, 44.075 )
( 8407, 44.027 )
( 8408, 43.930 )
( 8409, 43.629 )
( 8410, 43.769 )
( 8411, 43.893 )
( 8412, 43.868 )
( 8413, 43.840 )
( 8414, 43.813 )
( 8415, 43.835 )
( 8416, 43.933 )
( 8417, 44.103 )
( 8418, 44.187 )
( 8419, 44.352 )
( 8420, 44.492 )
( 8421, 44.635 )
( 8422, 44.863 )
( 8423, 44.975 )
( 8424, 45.075 )
( 8425, 45.244 )
( 8426, 45.397 )
( 8427, 45.548 )
( 8428, 45.774 )
( 8429, 45.985 )
( 8430, 46.201 )
( 8431, 46.410 )
( 8432, 46.662 )
( 8433, 46.909 )
( 8434, 47.170 )
( 8435, 47.431 )
( 8436, 47.639 )
( 8437, 47.802 )
( 8438, 47.900 )
( 8439, 47.997 )
( 8440, 48.140 )
( 8441, 48.291 )
( 8442, 48.432 )
( 8443, 48.441 )
( 8444, 48.488 )
( 8445, 48.465 )
( 8446, 48.487 )
( 8447, 48.603 )
( 8448, 48.664 )
( 8449, 48.783 )
( 8450, 48.799 )
( 8451, 48.799 )
( 8452, 48.813 )
( 8453, 48.805 )
( 8454, 48.951 )
( 8455, 49.045 )
( 8456, 49.128 )
( 8457, 49.138 )
( 8458, 49.129 )
( 8459, 49.172 )
( 8460, 49.159 )
( 8461, 49.217 )
( 8462, 49.472 )
( 8463, 49.734 )
( 8464, 50.003 )
( 8465, 50.269 )
( 8466, 50.562 )
( 8467, 50.935 )
( 8468, 51.308 )
( 8469, 51.793 )
( 8470, 52.261 )
( 8471, 52.633 )
( 8472, 53.018 )
( 8473, 53.391 )
( 8474, 53.767 )
( 8475, 54.154 )
( 8476, 54.531 )
( 8477, 54.906 )
( 8478, 55.283 )
( 8479, 55.670 )
( 8480, 55.972 )
( 8481, 56.273 )
( 8482, 56.602 )
( 8483, 56.902 )
( 8484, 57.204 )
( 8485, 57.514 )
( 8486, 57.814 )
( 8487, 58.137 )
( 8488, 58.627 )
( 8489, 58.950 )
( 8490, 59.254 )
( 8491, 59.576 )
( 8492, 59.920 )
( 8493, 60.279 )
( 8494, 60.603 )
( 8495, 61.041 )
( 8496, 61.397 )
( 8497, 61.792 )
( 8498, 62.155 )
( 8499, 62.611 )
( 8500, 62.945 )
( 8501, 63.246 )
( 8502, 63.547 )
( 8503, 63.849 )
( 8504, 64.171 )
( 8505, 64.481 )
( 8506, 64.783 )
( 8507, 65.094 )
( 8508, 65.395 )
( 8509, 65.783 )
( 8510, 66.090 )
( 8511, 66.406 )
( 8512, 66.836 )
( 8513, 67.278 )
( 8514, 67.588 )
( 8515, 67.889 )
( 8516, 68.258 )
( 8517, 68.562 )
( 8518, 68.868 )
( 8519, 69.200 )
( 8520, 69.501 )
( 8521, 69.835 )
( 8522, 70.173 )
( 8523, 70.489 )
( 8524, 70.812 )
( 8525, 71.134 )
( 8526, 71.436 )
( 8527, 71.754 )
( 8528, 72.076 )
( 8529, 72.493 )
( 8530, 72.892 )
( 8531, 73.196 )
( 8532, 73.498 )
( 8533, 73.799 )
( 8534, 74.102 )
( 8535, 74.410 )
( 8536, 74.728 )
( 8537, 75.064 )
( 8538, 75.450 )
( 8539, 75.853 )
( 8540, 76.250 )
( 8541, 76.638 )
( 8542, 76.946 )
( 8543, 77.286 )
( 8544, 77.608 )
( 8545, 77.938 )
( 8546, 78.280 )
( 8547, 78.603 )
( 8548, 78.958 )
( 8549, 79.335 )
( 8550, 79.683 )
( 8551, 80.005 )
( 8552, 80.382 )
( 8553, 80.683 )
( 8554, 81.082 )
( 8555, 81.461 )
( 8556, 81.840 )
( 8557, 82.172 )
( 8558, 82.590 )
( 8559, 82.987 )
( 8560, 83.386 )
( 8561, 83.804 )
( 8562, 84.202 )
( 8563, 84.600 )
( 8564, 85.015 )
( 8565, 85.418 )
( 8566, 85.828 )
( 8567, 86.226 )
( 8568, 86.627 )
( 8569, 87.058 )
( 8570, 87.471 )
( 8571, 87.901 )
( 8572, 88.337 )
( 8573, 88.737 )
( 8574, 89.144 )
( 8575, 89.543 )
( 8576, 89.976 )
( 8577, 90.374 )
( 8578, 90.772 )
( 8579, 91.218 )
( 8580, 91.616 )
( 8581, 92.066 )
( 8582, 92.466 )
( 8583, 92.898 )
( 8584, 93.296 )
( 8585, 93.721 )
( 8586, 94.119 )
( 8587, 94.517 )
( 8588, 94.915 )
( 8589, 95.339 )
( 8590, 95.736 )
( 8591, 96.148 )
( 8592, 96.547 )
( 8593, 96.944 )
( 8594, 97.343 )
( 8595, 97.773 )
( 8596, 98.191 )
( 8597, 98.603 )
( 8598, 99.025 )
};


==> H144984 <==
\addplot[color=red] coordinates{
    ( 0.00000, 5.1613 )
    ( 1.0000, 5.4310 )
    ( 2.0000, 5.6071 )
    ( 3.0000, 5.8361 )
    ( 4.0000, 6.0827 )
    ( 5.0000, 6.3613 )
    ( 6.0000, 6.3895 )
    ( 7.0000, 6.3896 )
    ( 8.0000, 6.5835 )
    ( 9.0000, 6.5836 )
    ( 10.000, 6.6046 )
    ( 11.000, 6.6047 )
    ( 12.000, 6.7646 )
    ( 13.000, 7.0414 )
    ( 14.000, 7.0568 )
    ( 15.000, 7.2278 )
    ( 16.000, 7.6207 )
    ( 17.000, 7.9018 )
    ( 18.000, 8.1891 )
    ( 19.000, 8.4875 )
    ( 20.000, 8.5311 )
    ( 21.000, 8.6375 )
    ( 22.000, 8.7466 )
    ( 23.000, 8.9879 )
    ( 24.000, 8.9894 )
    ( 25.000, 9.1356 )
    ( 26.000, 9.3446 )
    ( 27.000, 9.4586 )
    ( 28.000, 9.8033 )
    ( 29.000, 10.181 )
    ( 30.000, 10.403 )
    ( 31.000, 10.453 )
    ( 32.000, 10.538 )
    ( 33.000, 10.560 )
    ( 34.000, 10.560 )
    ( 35.000, 10.802 )
    ( 36.000, 11.043 )
    ( 37.000, 11.097 )
    ( 38.000, 11.217 )
    ( 39.000, 11.217 )
    ( 40.000, 11.217 )
    ( 41.000, 11.528 )
    ( 42.000, 11.754 )
    ( 43.000, 12.061 )
    ( 44.000, 12.360 )
    ( 45.000, 12.637 )
    ( 46.000, 12.772 )
    ( 47.000, 13.014 )
    ( 48.000, 13.183 )
    ( 49.000, 13.329 )
    ( 50.000, 13.571 )
    ( 51.000, 13.846 )
    ( 52.000, 13.853 )
    ( 53.000, 13.920 )
    ( 54.000, 14.195 )
    ( 55.000, 14.503 )
    ( 56.000, 14.874 )
    ( 57.000, 15.216 )
    ( 58.000, 15.593 )
    ( 59.000, 15.914 )
    ( 60.000, 16.288 )
    ( 61.000, 16.602 )
    ( 62.000, 16.921 )
    ( 63.000, 17.140 )
    ( 64.000, 17.373 )
    ( 65.000, 17.566 )
    ( 66.000, 17.752 )
    ( 67.000, 17.975 )
    ( 68.000, 18.320 )
    ( 69.000, 18.610 )
    ( 70.000, 18.903 )
    ( 71.000, 19.170 )
    ( 72.000, 19.403 )
    ( 73.000, 19.619 )
    ( 74.000, 19.743 )
    ( 75.000, 19.619 )
    ( 76.000, 19.504 )
    ( 77.000, 19.658 )
    ( 78.000, 19.826 )
    ( 79.000, 20.019 )
    ( 80.000, 20.162 )
    ( 81.000, 20.287 )
    ( 82.000, 20.412 )
    ( 83.000, 20.598 )
    ( 84.000, 20.822 )
    ( 85.000, 20.990 )
    ( 86.000, 21.167 )
    ( 87.000, 21.292 )
    ( 88.000, 21.417 )
    ( 89.000, 21.673 )
    ( 90.000, 21.966 )
    ( 91.000, 22.091 )
    ( 92.000, 22.234 )
    ( 93.000, 22.436 )
    ( 94.000, 22.571 )
    ( 95.000, 22.809 )
    ( 96.000, 22.976 )
    ( 97.000, 23.232 )
    ( 98.000, 23.587 )
    ( 99.000, 23.943 )
    ( 100.00, 24.268 )
    ( 101.00, 24.152 )
    ( 102.00, 24.028 )
    ( 103.00, 24.070 )
    ( 104.00, 24.116 )
    ( 105.00, 24.204 )
    ( 106.00, 24.253 )
    ( 107.00, 24.294 )
    ( 108.00, 24.335 )
    ( 109.00, 24.377 )
    ( 110.00, 24.420 )
    ( 111.00, 24.524 )
    ( 112.00, 24.582 )
    ( 113.00, 24.524 )
    ( 114.00, 24.400 )
    ( 115.00, 24.275 )
    ( 116.00, 24.179 )
    ( 117.00, 24.163 )
    ( 118.00, 24.103 )
    ( 119.00, 23.802 )
    ( 120.00, 23.905 )
    ( 121.00, 23.958 )
    ( 122.00, 23.833 )
    ( 123.00, 24.022 )
    ( 124.00, 24.230 )
    ( 125.00, 24.398 )
    ( 126.00, 24.570 )
    ( 127.00, 24.698 )
    ( 128.00, 24.828 )
    ( 129.00, 24.984 )
    ( 130.00, 25.164 )
    ( 131.00, 25.289 )
    ( 132.00, 25.526 )
    ( 133.00, 25.712 )
    ( 134.00, 25.907 )
    ( 135.00, 26.100 )
    ( 136.00, 26.318 )
    ( 137.00, 26.515 )
    ( 138.00, 26.720 )
    ( 139.00, 26.611 )
    ( 140.00, 26.828 )
    ( 141.00, 27.083 )
    ( 142.00, 27.407 )
    ( 143.00, 27.667 )
    ( 144.00, 27.948 )
    ( 145.00, 28.282 )
    ( 146.00, 28.545 )
    ( 147.00, 28.872 )
    ( 148.00, 28.866 )
    ( 149.00, 28.859 )
    ( 150.00, 28.904 )
    ( 151.00, 28.980 )
    ( 152.00, 28.986 )
    ( 153.00, 28.958 )
    ( 154.00, 29.011 )
    ( 155.00, 29.190 )
    ( 156.00, 29.344 )
    ( 157.00, 29.491 )
    ( 158.00, 29.614 )
    ( 159.00, 29.650 )
    ( 160.00, 29.679 )
    ( 161.00, 29.675 )
    ( 162.00, 29.825 )
    ( 163.00, 29.959 )
    ( 164.00, 29.901 )
    ( 165.00, 29.895 )
    ( 166.00, 29.954 )
    ( 167.00, 30.053 )
    ( 168.00, 30.036 )
    ( 169.00, 29.990 )
    ( 170.00, 29.933 )
    ( 171.00, 30.013 )
    ( 172.00, 30.022 )
    ( 173.00, 30.077 )
    ( 174.00, 30.075 )
    ( 175.00, 30.227 )
    ( 176.00, 30.424 )
    ( 177.00, 30.720 )
    ( 178.00, 30.907 )
    ( 179.00, 31.076 )
    ( 180.00, 31.226 )
    ( 181.00, 31.412 )
    ( 182.00, 31.453 )
    ( 183.00, 31.466 )
    ( 184.00, 31.455 )
    ( 185.00, 31.644 )
    ( 186.00, 31.729 )
    ( 187.00, 31.752 )
    ( 188.00, 31.738 )
    ( 189.00, 31.690 )
    ( 190.00, 31.633 )
    ( 191.00, 31.604 )
    ( 192.00, 31.357 )
    ( 193.00, 31.056 )
    ( 194.00, 30.972 )
    ( 195.00, 30.671 )
    ( 196.00, 30.574 )
    ( 197.00, 30.641 )
    ( 198.00, 30.654 )
    ( 199.00, 30.386 )
    ( 200.00, 30.301 )
    ( 201.00, 30.010 )
    ( 202.00, 29.913 )
    ( 203.00, 29.613 )
    ( 204.00, 29.355 )
    ( 205.00, 29.209 )
    ( 206.00, 28.922 )
    ( 207.00, 28.684 )
    ( 208.00, 28.383 )
    ( 209.00, 28.187 )
    ( 210.00, 27.886 )
    ( 211.00, 27.585 )
    ( 212.00, 27.530 )
    ( 213.00, 27.471 )
    ( 214.00, 27.452 )
    ( 215.00, 27.403 )
    ( 216.00, 27.476 )
    ( 217.00, 27.551 )
    ( 218.00, 27.493 )
    ( 219.00, 27.500 )
    ( 220.00, 27.486 )
    ( 221.00, 27.472 )
    ( 222.00, 27.475 )
    ( 223.00, 27.599 )
    ( 224.00, 27.735 )
    ( 225.00, 27.832 )
    ( 226.00, 27.956 )
    ( 227.00, 28.097 )
    ( 228.00, 28.317 )
    ( 229.00, 28.536 )
    ( 230.00, 28.652 )
    ( 231.00, 28.749 )
    ( 232.00, 28.860 )
    ( 233.00, 28.979 )
    ( 234.00, 29.115 )
    ( 235.00, 29.233 )
    ( 236.00, 29.292 )
    ( 237.00, 29.171 )
    ( 238.00, 29.050 )
    ( 239.00, 28.958 )
    ( 240.00, 28.959 )
    ( 241.00, 28.834 )
    ( 242.00, 28.709 )
    ( 243.00, 28.834 )
    ( 244.00, 29.092 )
    ( 245.00, 29.396 )
    ( 246.00, 29.602 )
    ( 247.00, 29.788 )
    ( 248.00, 30.186 )
    ( 249.00, 30.495 )
    ( 250.00, 30.836 )
    ( 251.00, 31.152 )
    ( 252.00, 31.494 )
    ( 253.00, 31.806 )
    ( 254.00, 31.990 )
    ( 255.00, 32.031 )
    ( 256.00, 32.073 )
    ( 257.00, 31.999 )
    ( 258.00, 31.877 )
    ( 259.00, 31.754 )
    ( 260.00, 31.640 )
    ( 261.00, 31.521 )
    ( 262.00, 31.403 )
    ( 263.00, 31.430 )
    ( 264.00, 31.411 )
    ( 265.00, 31.452 )
    ( 266.00, 31.530 )
    ( 267.00, 31.602 )
    ( 268.00, 31.728 )
    ( 269.00, 31.771 )
    ( 270.00, 31.813 )
    ( 271.00, 31.928 )
    ( 272.00, 31.969 )
    ( 273.00, 32.035 )
    ( 274.00, 32.095 )
    ( 275.00, 32.000 )
    ( 276.00, 31.931 )
    ( 277.00, 31.815 )
    ( 278.00, 31.743 )
    ( 279.00, 31.619 )
    ( 280.00, 31.520 )
    ( 281.00, 31.471 )
    ( 282.00, 31.347 )
    ( 283.00, 31.305 )
    ( 284.00, 31.181 )
    ( 285.00, 31.056 )
    ( 286.00, 30.932 )
    ( 287.00, 30.991 )
    ( 288.00, 30.866 )
    ( 289.00, 30.886 )
    ( 290.00, 30.919 )
    ( 291.00, 30.861 )
    ( 292.00, 30.787 )
    ( 293.00, 30.662 )
    ( 294.00, 30.537 )
    ( 295.00, 30.597 )
    ( 296.00, 30.623 )
    ( 297.00, 30.633 )
    ( 298.00, 30.643 )
    ( 299.00, 30.648 )
    ( 300.00, 30.642 )
    ( 301.00, 30.547 )
    ( 302.00, 30.246 )
    ( 303.00, 30.098 )
    ( 304.00, 29.821 )
    ( 305.00, 29.590 )
    ( 306.00, 29.290 )
    ( 307.00, 29.229 )
    ( 308.00, 29.169 )
    ( 309.00, 29.329 )
    ( 310.00, 29.055 )
    ( 311.00, 28.760 )
    ( 312.00, 28.570 )
    ( 313.00, 28.374 )
    ( 314.00, 28.178 )
    ( 315.00, 27.940 )
    ( 316.00, 27.639 )
    ( 317.00, 27.339 )
    ( 318.00, 27.070 )
    ( 319.00, 27.094 )
    ( 320.00, 26.864 )
    ( 321.00, 26.564 )
    ( 322.00, 26.303 )
    ( 323.00, 26.248 )
    ( 324.00, 26.348 )
    ( 325.00, 26.346 )
    ( 326.00, 26.261 )
    ( 327.00, 26.196 )
    ( 328.00, 25.895 )
    ( 329.00, 25.717 )
    ( 330.00, 25.480 )
    ( 331.00, 25.269 )
    ( 332.00, 24.980 )
    ( 333.00, 24.838 )
    ( 334.00, 24.715 )
    ( 335.00, 24.577 )
    ( 336.00, 24.276 )
    ( 337.00, 23.975 )
    ( 338.00, 23.674 )
    ( 339.00, 23.526 )
    ( 340.00, 23.315 )
    ( 341.00, 23.104 )
    ( 342.00, 22.810 )
    ( 343.00, 22.509 )
    ( 344.00, 22.212 )
    ( 345.00, 21.911 )
    ( 346.00, 21.670 )
    ( 347.00, 21.369 )
    ( 348.00, 21.068 )
    ( 349.00, 21.000 )
    ( 350.00, 20.857 )
    ( 351.00, 20.624 )
    ( 352.00, 20.365 )
    ( 353.00, 20.318 )
    ( 354.00, 20.187 )
    ( 355.00, 20.040 )
    ( 356.00, 19.894 )
    ( 357.00, 19.750 )
    ( 358.00, 19.449 )
    ( 359.00, 19.253 )
    ( 360.00, 19.188 )
    ( 361.00, 18.898 )
    ( 362.00, 18.702 )
    ( 363.00, 18.564 )
    ( 364.00, 18.278 )
    ( 365.00, 18.083 )
    ( 366.00, 17.846 )
    ( 367.00, 17.617 )
    ( 368.00, 17.317 )
    ( 369.00, 17.161 )
    ( 370.00, 16.860 )
    ( 371.00, 16.898 )
    ( 372.00, 16.844 )
    ( 373.00, 16.792 )
    ( 374.00, 16.811 )
    ( 375.00, 16.820 )
    ( 376.00, 16.900 )
    ( 377.00, 16.872 )
    ( 378.00, 16.827 )
    ( 379.00, 16.783 )
    ( 380.00, 16.842 )
    ( 381.00, 16.868 )
    ( 382.00, 16.744 )
    ( 383.00, 16.623 )
    ( 384.00, 16.929 )
    ( 385.00, 17.207 )
    ( 386.00, 17.462 )
    ( 387.00, 17.718 )
    ( 388.00, 18.049 )
    ( 389.00, 18.375 )
    ( 390.00, 18.700 )
    ( 391.00, 19.008 )
    ( 392.00, 19.217 )
    ( 393.00, 19.426 )
    ( 394.00, 19.427 )
    ( 395.00, 19.465 )
    ( 396.00, 19.589 )
    ( 397.00, 19.601 )
    ( 398.00, 19.601 )
    ( 399.00, 20.091 )
    ( 400.00, 20.652 )
    ( 401.00, 20.963 )
    ( 402.00, 21.256 )
    ( 403.00, 21.545 )
    ( 404.00, 21.822 )
    ( 405.00, 22.098 )
    ( 406.00, 22.374 )
    ( 407.00, 22.597 )
    ( 408.00, 22.877 )
    ( 409.00, 23.103 )
    ( 410.00, 23.364 )
    ( 411.00, 23.585 )
    ( 412.00, 23.878 )
    ( 413.00, 23.880 )
    ( 414.00, 23.909 )
    ( 415.00, 23.920 )
    ( 416.00, 23.920 )
    ( 417.00, 24.030 )
    ( 418.00, 24.030 )
    ( 419.00, 24.031 )
    ( 420.00, 24.054 )
    ( 421.00, 24.066 )
    ( 422.00, 24.066 )
    ( 423.00, 24.129 )
    ( 424.00, 24.380 )
    ( 425.00, 24.728 )
    ( 426.00, 25.191 )
    ( 427.00, 25.534 )
    ( 428.00, 25.970 )
    ( 429.00, 26.192 )
    ( 430.00, 26.488 )
    ( 431.00, 26.836 )
    ( 432.00, 27.112 )
    ( 433.00, 27.335 )
    ( 434.00, 27.564 )
    ( 435.00, 27.915 )
    ( 436.00, 27.915 )
    ( 437.00, 27.915 )
    ( 438.00, 27.926 )
    ( 439.00, 27.926 )
    ( 440.00, 28.072 )
    ( 441.00, 28.224 )
    ( 442.00, 28.439 )
    ( 443.00, 28.481 )
    ( 444.00, 28.502 )
    ( 445.00, 28.517 )
    ( 446.00, 28.561 )
    ( 447.00, 28.561 )
    ( 448.00, 28.670 )
    ( 449.00, 28.670 )
    ( 450.00, 28.819 )
    ( 451.00, 28.819 )
    ( 452.00, 28.819 )
    ( 453.00, 28.829 )
    ( 454.00, 28.887 )
    ( 455.00, 28.936 )
    ( 456.00, 29.082 )
    ( 457.00, 29.253 )
    ( 458.00, 29.253 )
    ( 459.00, 29.284 )
    ( 460.00, 29.284 )
    ( 461.00, 29.284 )
    ( 462.00, 29.286 )
    ( 463.00, 29.402 )
    ( 464.00, 29.439 )
    ( 465.00, 29.548 )
    ( 466.00, 29.641 )
    ( 467.00, 29.913 )
    ( 468.00, 30.176 )
    ( 469.00, 30.542 )
    ( 470.00, 31.014 )
    ( 471.00, 31.503 )
    ( 472.00, 31.800 )
    ( 473.00, 32.021 )
    ( 474.00, 32.250 )
    ( 475.00, 32.473 )
    ( 476.00, 32.715 )
    ( 477.00, 33.000 )
    ( 478.00, 33.230 )
    ( 479.00, 33.462 )
    ( 480.00, 33.694 )
    ( 481.00, 33.971 )
    ( 482.00, 34.193 )
    ( 483.00, 34.415 )
    ( 484.00, 34.637 )
    ( 485.00, 34.909 )
    ( 486.00, 35.162 )
    ( 487.00, 35.384 )
    ( 488.00, 35.389 )
    ( 489.00, 35.522 )
    ( 490.00, 35.713 )
    ( 491.00, 35.729 )
    ( 492.00, 35.823 )
    ( 493.00, 35.953 )
    ( 494.00, 36.005 )
    ( 495.00, 36.146 )
    ( 496.00, 36.190 )
    ( 497.00, 36.210 )
    ( 498.00, 36.210 )
    ( 499.00, 36.282 )
    ( 500.00, 36.365 )
    ( 501.00, 36.365 )
    ( 502.00, 36.394 )
    ( 503.00, 36.394 )
    ( 504.00, 36.447 )
    ( 505.00, 36.600 )
    ( 506.00, 36.601 )
    ( 507.00, 36.601 )
    ( 508.00, 36.609 )
    ( 509.00, 36.773 )
    ( 510.00, 36.975 )
    ( 511.00, 37.181 )
    ( 512.00, 37.356 )
    ( 513.00, 37.534 )
    ( 514.00, 37.552 )
    ( 515.00, 37.662 )
    ( 516.00, 37.665 )
    ( 517.00, 37.730 )
    ( 518.00, 38.075 )
    ( 519.00, 38.298 )
    ( 520.00, 38.611 )
    ( 521.00, 38.833 )
    ( 522.00, 39.111 )
    ( 523.00, 39.504 )
    ( 524.00, 39.787 )
    ( 525.00, 40.081 )
    ( 526.00, 40.303 )
    ( 527.00, 40.686 )
    ( 528.00, 40.965 )
    ( 529.00, 41.373 )
    ( 530.00, 41.767 )
    ( 531.00, 41.989 )
    ( 532.00, 42.247 )
    ( 533.00, 42.476 )
    ( 534.00, 42.701 )
    ( 535.00, 42.923 )
    ( 536.00, 43.204 )
    ( 537.00, 43.618 )
    ( 538.00, 43.898 )
    ( 539.00, 44.137 )
    ( 540.00, 44.475 )
    ( 541.00, 44.812 )
    ( 542.00, 44.861 )
    ( 543.00, 44.861 )
    ( 544.00, 44.890 )
    ( 545.00, 44.890 )
    ( 546.00, 44.934 )
    ( 547.00, 44.963 )
    ( 548.00, 44.969 )
    ( 549.00, 45.018 )
    ( 550.00, 45.018 )
    ( 551.00, 45.018 )
    ( 552.00, 45.018 )
    ( 553.00, 45.067 )
    ( 554.00, 45.078 )
    ( 555.00, 45.083 )
    ( 556.00, 45.100 )
    ( 557.00, 45.110 )
    ( 558.00, 45.262 )
    ( 559.00, 45.298 )
    ( 560.00, 45.298 )
    ( 561.00, 45.455 )
    ( 562.00, 45.613 )
    ( 563.00, 45.614 )
    ( 564.00, 45.628 )
    ( 565.00, 45.649 )
    ( 566.00, 45.658 )
    ( 567.00, 45.658 )
    ( 568.00, 45.909 )
    ( 569.00, 46.221 )
    ( 570.00, 46.459 )
    ( 571.00, 46.684 )
    ( 572.00, 46.911 )
    ( 573.00, 47.133 )
    ( 574.00, 47.355 )
    ( 575.00, 47.733 )
    ( 576.00, 47.955 )
    ( 577.00, 48.238 )
    ( 578.00, 48.519 )
    ( 579.00, 48.763 )
    ( 580.00, 48.996 )
    ( 581.00, 49.218 )
    ( 582.00, 49.533 )
    ( 583.00, 49.755 )
    ( 584.00, 49.978 )
    ( 585.00, 50.290 )
    ( 586.00, 50.589 )
    ( 587.00, 50.923 )
    ( 588.00, 51.252 )
    ( 589.00, 51.602 )
    ( 590.00, 51.896 )
    ( 591.00, 52.117 )
    ( 592.00, 52.480 )
    ( 593.00, 52.823 )
    ( 594.00, 53.104 )
    ( 595.00, 53.326 )
    ( 596.00, 53.437 )
    ( 597.00, 53.437 )
    ( 598.00, 53.437 )
    ( 599.00, 53.800 )
    ( 600.00, 54.143 )
    ( 601.00, 54.545 )
    ( 602.00, 54.867 )
    ( 603.00, 55.150 )
    ( 604.00, 55.396 )
    ( 605.00, 55.712 )
    ( 606.00, 56.169 )
    ( 607.00, 56.512 )
    ( 608.00, 56.941 )
    ( 609.00, 57.284 )
    ( 610.00, 57.703 )
    ( 611.00, 58.067 )
    ( 612.00, 58.418 )
    ( 613.00, 58.827 )
    ( 614.00, 59.048 )
    ( 615.00, 59.271 )
    ( 616.00, 59.528 )
    ( 617.00, 59.804 )
    ( 618.00, 59.815 )
    ( 619.00, 59.822 )
    ( 620.00, 59.903 )
    ( 621.00, 59.953 )
    ( 622.00, 59.954 )
    ( 623.00, 59.963 )
    ( 624.00, 59.963 )
    ( 625.00, 60.144 )
    ( 626.00, 60.145 )
    ( 627.00, 60.145 )
    ( 628.00, 60.160 )
    ( 629.00, 60.309 )
    ( 630.00, 60.531 )
    ( 631.00, 60.753 )
    ( 632.00, 61.014 )
    ( 633.00, 61.236 )
    ( 634.00, 61.459 )
    ( 635.00, 61.681 )
    ( 636.00, 61.902 )
    ( 637.00, 62.245 )
    ( 638.00, 62.680 )
    ( 639.00, 62.969 )
    ( 640.00, 63.193 )
    ( 641.00, 63.570 )
    ( 642.00, 63.919 )
    ( 643.00, 64.311 )
    ( 644.00, 64.656 )
    ( 645.00, 64.999 )
    ( 646.00, 65.221 )
    ( 647.00, 65.442 )
    ( 648.00, 65.784 )
    ( 649.00, 66.096 )
    ( 650.00, 66.317 )
    ( 651.00, 66.569 )
    ( 652.00, 66.800 )
    ( 653.00, 67.109 )
    ( 654.00, 67.414 )
    ( 655.00, 67.732 )
    ( 656.00, 67.732 )
    ( 657.00, 67.732 )
    ( 658.00, 67.732 )
    ( 659.00, 67.956 )
    ( 660.00, 68.242 )
    ( 661.00, 68.503 )
    ( 662.00, 68.748 )
    ( 663.00, 68.971 )
    ( 664.00, 69.192 )
    ( 665.00, 69.414 )
    ( 666.00, 69.637 )
    ( 667.00, 69.918 )
    ( 668.00, 70.232 )
    ( 669.00, 70.521 )
    ( 670.00, 70.814 )
    ( 671.00, 71.092 )
    ( 672.00, 71.397 )
    ( 673.00, 71.673 )
    ( 674.00, 71.949 )
    ( 675.00, 72.182 )
    ( 676.00, 72.403 )
    ( 677.00, 72.691 )
    ( 678.00, 72.929 )
    ( 679.00, 73.151 )
    ( 680.00, 73.373 )
    ( 681.00, 73.520 )
    ( 682.00, 73.635 )
    ( 683.00, 73.743 )
    ( 684.00, 74.055 )
    ( 685.00, 74.056 )
    ( 686.00, 74.057 )
    ( 687.00, 74.079 )
    ( 688.00, 74.079 )
    ( 689.00, 74.065 )
    ( 690.00, 74.038 )
    ( 691.00, 74.042 )
    ( 692.00, 74.014 )
    ( 693.00, 74.098 )
    ( 694.00, 74.249 )
    ( 695.00, 74.343 )
    ( 696.00, 74.315 )
    ( 697.00, 74.020 )
    ( 698.00, 73.782 )
    ( 699.00, 73.641 )
    ( 700.00, 73.514 )
    ( 701.00, 73.367 )
    ( 702.00, 73.272 )
    ( 703.00, 73.295 )
    ( 704.00, 73.215 )
    ( 705.00, 73.150 )
    ( 706.00, 73.175 )
    ( 707.00, 73.078 )
    ( 708.00, 72.777 )
    ( 709.00, 72.477 )
    ( 710.00, 72.237 )
    ( 711.00, 72.182 )
    ( 712.00, 72.166 )
    ( 713.00, 72.068 )
    ( 714.00, 72.048 )
    ( 715.00, 71.800 )
    ( 716.00, 71.589 )
    ( 717.00, 71.378 )
    ( 718.00, 71.077 )
    ( 719.00, 70.809 )
    ( 720.00, 70.663 )
    ( 721.00, 70.362 )
    ( 722.00, 70.062 )
    ( 723.00, 69.762 )
    ( 724.00, 69.479 )
    ( 725.00, 69.179 )
    ( 726.00, 68.973 )
    ( 727.00, 68.764 )
    ( 728.00, 68.672 )
    ( 729.00, 68.575 )
    ( 730.00, 68.386 )
    ( 731.00, 68.239 )
    ( 732.00, 68.067 )
    ( 733.00, 68.019 )
    ( 734.00, 67.922 )
    ( 735.00, 67.825 )
    ( 736.00, 67.524 )
    ( 737.00, 67.223 )
    ( 738.00, 67.140 )
    ( 739.00, 66.838 )
    ( 740.00, 66.714 )
    ( 741.00, 66.589 )
    ( 742.00, 66.532 )
    ( 743.00, 66.407 )
    ( 744.00, 66.125 )
    ( 745.00, 65.824 )
    ( 746.00, 65.540 )
    ( 747.00, 65.239 )
    ( 748.00, 65.144 )
    ( 749.00, 65.078 )
    ( 750.00, 64.783 )
    ( 751.00, 64.719 )
    ( 752.00, 64.798 )
    ( 753.00, 64.738 )
    ( 754.00, 64.511 )
    ( 755.00, 64.210 )
    ( 756.00, 64.123 )
    ( 757.00, 64.027 )
    ( 758.00, 63.727 )
    ( 759.00, 63.516 )
    ( 760.00, 63.215 )
    ( 761.00, 62.915 )
    ( 762.00, 62.973 )
    ( 763.00, 63.024 )
    ( 764.00, 63.010 )
    ( 765.00, 62.997 )
    ( 766.00, 62.985 )
    ( 767.00, 62.973 )
    ( 768.00, 62.960 )
    ( 769.00, 62.956 )
    ( 770.00, 62.942 )
    ( 771.00, 62.886 )
    ( 772.00, 62.839 )
    ( 773.00, 62.828 )
    ( 774.00, 62.973 )
    ( 775.00, 63.118 )
    ( 776.00, 63.245 )
    ( 777.00, 63.187 )
    ( 778.00, 63.145 )
    ( 779.00, 63.167 )
    ( 780.00, 63.145 )
    ( 781.00, 63.020 )
    ( 782.00, 62.896 )
    ( 783.00, 62.781 )
    ( 784.00, 62.683 )
    ( 785.00, 62.754 )
    ( 786.00, 62.797 )
    ( 787.00, 62.673 )
    ( 788.00, 62.693 )
    ( 789.00, 62.653 )
    ( 790.00, 62.627 )
    ( 791.00, 62.757 )
    ( 792.00, 62.874 )
    ( 793.00, 62.934 )
    ( 794.00, 62.876 )
    ( 795.00, 62.857 )
    ( 796.00, 62.886 )
    ( 797.00, 62.829 )
    ( 798.00, 62.771 )
    ( 799.00, 62.830 )
    ( 800.00, 62.779 )
    ( 801.00, 62.727 )
    ( 802.00, 62.896 )
    ( 803.00, 62.956 )
    ( 804.00, 62.899 )
    ( 805.00, 62.853 )
    ( 806.00, 62.861 )
    ( 807.00, 62.804 )
    ( 808.00, 62.747 )
    ( 809.00, 62.755 )
    ( 810.00, 62.631 )
    ( 811.00, 62.680 )
    ( 812.00, 62.748 )
    ( 813.00, 62.817 )
    ( 814.00, 62.918 )
    ( 815.00, 62.961 )
    ( 816.00, 63.003 )
    ( 817.00, 63.101 )
    ( 818.00, 63.068 )
    ( 819.00, 62.996 )
    ( 820.00, 62.871 )
    ( 821.00, 62.746 )
    ( 822.00, 62.627 )
    ( 823.00, 62.502 )
    ( 824.00, 62.543 )
    ( 825.00, 62.585 )
    ( 826.00, 62.626 )
    ( 827.00, 62.740 )
    ( 828.00, 62.781 )
    ( 829.00, 62.896 )
    ( 830.00, 62.771 )
    ( 831.00, 62.646 )
    ( 832.00, 62.521 )
    ( 833.00, 62.396 )
    ( 834.00, 62.276 )
    ( 835.00, 62.151 )
    ( 836.00, 62.026 )
    ( 837.00, 61.902 )
    ( 838.00, 61.778 )
    ( 839.00, 61.653 )
    ( 840.00, 61.531 )
    ( 841.00, 61.423 )
    ( 842.00, 61.311 )
    ( 843.00, 61.529 )
    ( 844.00, 61.709 )
    ( 845.00, 61.850 )
    ( 846.00, 61.975 )
    ( 847.00, 62.103 )
    ( 848.00, 62.239 )
    ( 849.00, 62.484 )
    ( 850.00, 62.668 )
    ( 851.00, 62.864 )
    ( 852.00, 62.989 )
    ( 853.00, 63.178 )
    ( 854.00, 63.306 )
    ( 855.00, 63.618 )
    ( 856.00, 63.874 )
    ( 857.00, 64.169 )
    ( 858.00, 64.334 )
    ( 859.00, 64.509 )
    ( 860.00, 64.725 )
    ( 861.00, 64.917 )
    ( 862.00, 65.097 )
    ( 863.00, 65.226 )
    ( 864.00, 65.376 )
    ( 865.00, 65.501 )
    ( 866.00, 65.686 )
    ( 867.00, 65.869 )
    ( 868.00, 65.970 )
    ( 869.00, 66.043 )
    ( 870.00, 66.266 )
    ( 871.00, 66.471 )
    ( 872.00, 66.553 )
    ( 873.00, 66.620 )
    ( 874.00, 66.721 )
    ( 875.00, 66.825 )
    ( 876.00, 66.922 )
    ( 877.00, 67.016 )
    ( 878.00, 67.110 )
    ( 879.00, 67.316 )
    ( 880.00, 67.404 )
    ( 881.00, 67.535 )
    ( 882.00, 67.622 )
    ( 883.00, 67.712 )
    ( 884.00, 67.913 )
    ( 885.00, 68.112 )
    ( 886.00, 68.200 )
    ( 887.00, 68.200 )
    ( 888.00, 68.200 )
    ( 889.00, 68.243 )
    ( 890.00, 68.243 )
    ( 891.00, 68.243 )
    ( 892.00, 68.243 )
    ( 893.00, 68.243 )
    ( 894.00, 68.418 )
    ( 895.00, 68.595 )
    ( 896.00, 68.770 )
    ( 897.00, 68.773 )
    ( 898.00, 68.868 )
    ( 899.00, 68.955 )
    ( 900.00, 69.021 )
    ( 901.00, 69.226 )
    ( 902.00, 69.293 )
    ( 903.00, 69.540 )
    ( 904.00, 69.750 )
    ( 905.00, 70.017 )
    ( 906.00, 70.225 )
    ( 907.00, 70.478 )
    ( 908.00, 70.680 )
    ( 909.00, 70.863 )
    ( 910.00, 71.168 )
    ( 911.00, 71.406 )
    ( 912.00, 71.591 )
    ( 913.00, 71.785 )
    ( 914.00, 71.971 )
    ( 915.00, 72.159 )
    ( 916.00, 72.344 )
    ( 917.00, 72.512 )
    ( 918.00, 72.636 )
    ( 919.00, 72.846 )
    ( 920.00, 73.029 )
    ( 921.00, 73.071 )
    ( 922.00, 72.952 )
    ( 923.00, 72.842 )
    ( 924.00, 72.736 )
    ( 925.00, 72.631 )
    ( 926.00, 72.614 )
    ( 927.00, 72.588 )
    ( 928.00, 72.463 )
    ( 929.00, 72.390 )
    ( 930.00, 72.315 )
    ( 931.00, 72.191 )
    ( 932.00, 72.101 )
    ( 933.00, 71.976 )
    ( 934.00, 71.854 )
    ( 935.00, 71.729 )
    ( 936.00, 71.655 )
    ( 937.00, 71.603 )
    ( 938.00, 71.478 )
    ( 939.00, 71.355 )
    ( 940.00, 71.233 )
    ( 941.00, 71.109 )
    ( 942.00, 70.984 )
    ( 943.00, 70.955 )
    ( 944.00, 70.840 )
    ( 945.00, 70.716 )
    ( 946.00, 70.604 )
    ( 947.00, 70.479 )
    ( 948.00, 70.420 )
    ( 949.00, 70.417 )
    ( 950.00, 70.398 )
    ( 951.00, 70.383 )
    ( 952.00, 70.414 )
    ( 953.00, 70.386 )
    ( 954.00, 70.405 )
    ( 955.00, 70.399 )
    ( 956.00, 70.536 )
    ( 957.00, 70.509 )
    ( 958.00, 70.497 )
    ( 959.00, 70.469 )
    ( 960.00, 70.512 )
    ( 961.00, 70.506 )
    ( 962.00, 70.499 )
    ( 963.00, 70.441 )
    ( 964.00, 70.383 )
    ( 965.00, 70.422 )
    ( 966.00, 70.363 )
    ( 967.00, 70.451 )
    ( 968.00, 70.538 )
    ( 969.00, 70.556 )
    ( 970.00, 70.527 )
    ( 971.00, 70.539 )
    ( 972.00, 70.513 )
    ( 973.00, 70.485 )
    ( 974.00, 70.457 )
    ( 975.00, 70.445 )
    ( 976.00, 70.439 )
    ( 977.00, 70.382 )
    ( 978.00, 70.348 )
    ( 979.00, 70.296 )
    ( 980.00, 70.284 )
    ( 981.00, 70.226 )
    ( 982.00, 70.101 )
    ( 983.00, 70.094 )
    ( 984.00, 70.067 )
    ( 985.00, 69.857 )
    ( 986.00, 69.646 )
    ( 987.00, 69.436 )
    ( 988.00, 69.164 )
    ( 989.00, 68.905 )
    ( 990.00, 68.710 )
    ( 991.00, 68.409 )
    ( 992.00, 68.107 )
    ( 993.00, 67.860 )
    ( 994.00, 67.696 )
    ( 995.00, 67.396 )
    ( 996.00, 67.121 )
    ( 997.00, 67.015 )
    ( 998.00, 66.756 )
    ( 999.00, 66.638 )
    ( 1000, 66.554 )
    ( 1001, 66.408 )
    ( 1002, 66.262 )
    ( 1003, 65.961 )
    ( 1004, 65.681 )
    ( 1005, 65.470 )
    ( 1006, 65.260 )
    ( 1007, 64.959 )
    ( 1008, 64.729 )
    ( 1009, 64.462 )
    ( 1010, 64.162 )
    ( 1011, 63.976 )
    ( 1012, 63.701 )
    ( 1013, 63.403 )
    ( 1014, 63.371 )
    ( 1015, 63.110 )
    ( 1016, 62.845 )
    ( 1017, 62.547 )
    ( 1018, 62.246 )
    ( 1019, 62.092 )
    ( 1020, 61.921 )
    ( 1021, 61.975 )
    ( 1022, 61.674 )
    ( 1023, 61.528 )
    ( 1024, 61.382 )
    ( 1025, 61.186 )
    ( 1026, 60.885 )
    ( 1027, 60.584 )
    ( 1028, 60.283 )
    ( 1029, 60.196 )
    ( 1030, 59.896 )
    ( 1031, 59.700 )
    ( 1032, 59.398 )
    ( 1033, 59.098 )
    ( 1034, 58.896 )
    ( 1035, 58.622 )
    ( 1036, 58.320 )
    ( 1037, 58.027 )
    ( 1038, 57.968 )
    ( 1039, 57.904 )
    ( 1040, 57.860 )
    ( 1041, 57.764 )
    ( 1042, 57.710 )
    ( 1043, 57.409 )
    ( 1044, 57.164 )
    ( 1045, 56.954 )
    ( 1046, 56.920 )
    ( 1047, 56.944 )
    ( 1048, 56.895 )
    ( 1049, 56.863 )
    ( 1050, 56.807 )
    ( 1051, 56.786 )
    ( 1052, 56.549 )
    ( 1053, 56.251 )
    ( 1054, 55.950 )
    ( 1055, 55.921 )
    ( 1056, 55.993 )
    ( 1057, 55.935 )
    ( 1058, 55.877 )
    ( 1059, 55.755 )
    ( 1060, 55.664 )
    ( 1061, 55.539 )
    ( 1062, 55.498 )
    ( 1063, 55.374 )
    ( 1064, 55.415 )
    ( 1065, 55.457 )
    ( 1066, 55.515 )
    ( 1067, 55.398 )
    ( 1068, 55.291 )
    ( 1069, 55.166 )
    ( 1070, 55.097 )
    ( 1071, 54.972 )
    ( 1072, 54.847 )
    ( 1073, 54.722 )
    ( 1074, 54.605 )
    ( 1075, 54.480 )
    ( 1076, 54.355 )
    ( 1077, 54.254 )
    ( 1078, 54.142 )
    ( 1079, 54.053 )
    ( 1080, 54.000 )
    ( 1081, 53.925 )
    ( 1082, 53.815 )
    ( 1083, 53.718 )
    ( 1084, 53.671 )
    ( 1085, 53.739 )
    ( 1086, 53.935 )
    ( 1087, 54.046 )
    ( 1088, 54.099 )
    ( 1089, 54.140 )
    ( 1090, 54.029 )
    ( 1091, 53.921 )
    ( 1092, 53.852 )
    ( 1093, 54.059 )
    ( 1094, 54.330 )
    ( 1095, 54.536 )
    ( 1096, 54.723 )
    ( 1097, 54.846 )
    ( 1098, 55.001 )
    ( 1099, 55.139 )
    ( 1100, 55.303 )
    ( 1101, 55.275 )
    ( 1102, 55.225 )
    ( 1103, 55.109 )
    ( 1104, 54.990 )
    ( 1105, 55.185 )
    ( 1106, 55.330 )
    ( 1107, 55.497 )
    ( 1108, 55.704 )
    ( 1109, 55.909 )
    ( 1110, 56.109 )
    ( 1111, 56.234 )
    ( 1112, 56.359 )
    ( 1113, 56.501 )
    ( 1114, 56.706 )
    ( 1115, 56.831 )
    ( 1116, 57.076 )
    ( 1117, 57.260 )
    ( 1118, 57.462 )
    ( 1119, 57.698 )
    ( 1120, 57.905 )
    ( 1121, 57.780 )
    ( 1122, 57.673 )
    ( 1123, 57.572 )
    ( 1124, 57.616 )
    ( 1125, 57.492 )
    ( 1126, 57.295 )
    ( 1127, 57.039 )
    ( 1128, 56.910 )
    ( 1129, 56.765 )
    ( 1130, 56.619 )
    ( 1131, 56.475 )
    ( 1132, 56.329 )
    ( 1133, 56.232 )
    ( 1134, 56.176 )
    ( 1135, 56.160 )
    ( 1136, 56.067 )
    ( 1137, 56.036 )
    ( 1138, 55.836 )
    ( 1139, 55.536 )
    ( 1140, 55.305 )
    ( 1141, 55.084 )
    ( 1142, 54.822 )
    ( 1143, 54.610 )
    ( 1144, 54.576 )
    ( 1145, 54.354 )
    ( 1146, 54.054 )
    ( 1147, 53.988 )
    ( 1148, 53.891 )
    ( 1149, 53.592 )
    ( 1150, 53.355 )
    ( 1151, 53.058 )
    ( 1152, 52.762 )
    ( 1153, 52.566 )
    ( 1154, 52.266 )
    ( 1155, 52.171 )
    ( 1156, 51.875 )
    ( 1157, 51.587 )
    ( 1158, 51.510 )
    ( 1159, 51.417 )
    ( 1160, 51.401 )
    ( 1161, 51.205 )
    ( 1162, 50.904 )
    ( 1163, 50.610 )
    ( 1164, 50.463 )
    ( 1165, 50.163 )
    ( 1166, 49.967 )
    ( 1167, 49.667 )
    ( 1168, 49.368 )
    ( 1169, 49.067 )
    ( 1170, 48.778 )
    ( 1171, 48.535 )
    ( 1172, 48.298 )
    ( 1173, 48.117 )
    ( 1174, 47.828 )
    ( 1175, 47.526 )
    ( 1176, 47.226 )
    ( 1177, 46.924 )
    ( 1178, 46.906 )
    ( 1179, 46.894 )
    ( 1180, 46.943 )
    ( 1181, 46.968 )
    ( 1182, 47.026 )
    ( 1183, 46.968 )
    ( 1184, 46.910 )
    ( 1185, 46.859 )
    ( 1186, 46.948 )
    ( 1187, 47.021 )
    ( 1188, 47.000 )
    ( 1189, 47.102 )
    ( 1190, 47.074 )
    ( 1191, 47.116 )
    ( 1192, 47.088 )
    ( 1193, 47.403 )
    ( 1194, 47.731 )
    ( 1195, 48.032 )
    ( 1196, 48.284 )
    ( 1197, 48.520 )
    ( 1198, 48.917 )
    ( 1199, 49.178 )
    ( 1200, 49.399 )
    ( 1201, 49.665 )
    ( 1202, 49.886 )
    ( 1203, 50.201 )
    ( 1204, 50.501 )
    ( 1205, 50.538 )
    ( 1206, 50.556 )
    ( 1207, 50.632 )
    ( 1208, 50.732 )
    ( 1209, 51.006 )
    ( 1210, 51.160 )
    ( 1211, 51.313 )
    ( 1212, 51.313 )
    ( 1213, 51.313 )
    ( 1214, 51.314 )
    ( 1215, 51.387 )
    ( 1216, 51.425 )
    ( 1217, 51.463 )
    ( 1218, 51.475 )
    ( 1219, 51.475 )
    ( 1220, 51.707 )
    ( 1221, 51.952 )
    ( 1222, 52.245 )
    ( 1223, 52.253 )
    ( 1224, 52.291 )
    ( 1225, 52.322 )
    ( 1226, 52.325 )
    ( 1227, 52.397 )
    ( 1228, 52.398 )
    ( 1229, 52.620 )
    ( 1230, 52.875 )
    ( 1231, 53.105 )
    ( 1232, 53.368 )
    ( 1233, 53.649 )
    ( 1234, 54.060 )
    ( 1235, 54.408 )
    ( 1236, 54.689 )
    ( 1237, 54.975 )
    ( 1238, 55.146 )
    ( 1239, 55.365 )
    ( 1240, 55.365 )
    ( 1241, 55.365 )
    ( 1242, 55.379 )
    ( 1243, 55.392 )
    ( 1244, 55.428 )
    ( 1245, 55.428 )
    ( 1246, 55.430 )
    ( 1247, 55.446 )
    ( 1248, 55.446 )
    ( 1249, 55.707 )
    ( 1250, 55.995 )
    ( 1251, 56.253 )
    ( 1252, 56.475 )
    ( 1253, 56.712 )
    ( 1254, 56.938 )
    ( 1255, 56.953 )
    ( 1256, 56.953 )
    ( 1257, 56.953 )
    ( 1258, 56.954 )
    ( 1259, 57.017 )
    ( 1260, 57.082 )
    ( 1261, 57.169 )
    ( 1262, 57.185 )
    ( 1263, 57.323 )
    ( 1264, 57.449 )
    ( 1265, 57.507 )
    ( 1266, 57.474 )
    ( 1267, 57.416 )
    ( 1268, 57.358 )
    ( 1269, 57.300 )
    ( 1270, 57.242 )
    ( 1271, 57.117 )
    ( 1272, 57.048 )
    ( 1273, 56.964 )
    ( 1274, 56.841 )
    ( 1275, 56.722 )
    ( 1276, 56.600 )
    ( 1277, 56.475 )
    ( 1278, 56.350 )
    ( 1279, 56.537 )
    ( 1280, 56.845 )
    ( 1281, 57.041 )
    ( 1282, 57.225 )
    ( 1283, 56.923 )
    ( 1284, 56.623 )
    ( 1285, 56.757 )
    ( 1286, 56.921 )
    ( 1287, 57.174 )
    ( 1288, 57.296 )
    ( 1289, 57.268 )
    ( 1290, 57.328 )
    ( 1291, 57.388 )
    ( 1292, 57.379 )
    ( 1293, 57.353 )
    ( 1294, 57.329 )
    ( 1295, 57.333 )
    ( 1296, 57.305 )
    ( 1297, 57.319 )
    ( 1298, 57.443 )
    ( 1299, 57.566 )
    ( 1300, 57.692 )
    ( 1301, 57.854 )
    ( 1302, 58.033 )
    ( 1303, 58.210 )
    ( 1304, 58.185 )
    ( 1305, 58.440 )
    ( 1306, 58.724 )
    ( 1307, 58.980 )
    ( 1308, 59.256 )
    ( 1309, 59.527 )
    ( 1310, 59.805 )
    ( 1311, 60.060 )
    ( 1312, 60.335 )
    ( 1313, 60.626 )
    ( 1314, 60.861 )
    ( 1315, 61.096 )
    ( 1316, 61.358 )
    ( 1317, 61.607 )
    ( 1318, 61.841 )
    ( 1319, 62.186 )
    ( 1320, 62.458 )
    ( 1321, 62.729 )
    ( 1322, 62.961 )
    ( 1323, 63.197 )
    ( 1324, 63.441 )
    ( 1325, 63.774 )
    ( 1326, 64.107 )
    ( 1327, 64.398 )
    ( 1328, 64.757 )
    ( 1329, 65.104 )
    ( 1330, 65.442 )
    ( 1331, 65.733 )
    ( 1332, 66.061 )
    ( 1333, 66.383 )
    ( 1334, 66.883 )
    ( 1335, 67.288 )
    ( 1336, 67.706 )
    ( 1337, 68.083 )
    ( 1338, 68.406 )
    ( 1339, 68.684 )
    ( 1340, 68.868 )
    ( 1341, 69.197 )
    ( 1342, 69.072 )
    ( 1343, 69.052 )
    ( 1344, 69.177 )
    ( 1345, 69.135 )
    ( 1346, 69.106 )
    ( 1347, 69.066 )
    ( 1348, 68.946 )
    ( 1349, 68.842 )
    ( 1350, 68.884 )
    ( 1351, 68.871 )
    ( 1352, 68.901 )
    ( 1353, 68.938 )
    ( 1354, 68.932 )
    ( 1355, 68.873 )
    ( 1356, 68.749 )
    ( 1357, 68.660 )
    ( 1358, 68.535 )
    ( 1359, 68.413 )
    ( 1360, 68.297 )
    ( 1361, 68.172 )
    ( 1362, 68.131 )
    ( 1363, 68.010 )
    ( 1364, 67.885 )
    ( 1365, 67.932 )
    ( 1366, 68.052 )
    ( 1367, 68.047 )
    ( 1368, 68.047 )
    ( 1369, 68.019 )
    ( 1370, 68.016 )
    ( 1371, 68.021 )
    ( 1372, 68.003 )
    ( 1373, 67.946 )
    ( 1374, 67.821 )
    ( 1375, 67.753 )
    ( 1376, 67.629 )
    ( 1377, 67.505 )
    ( 1378, 67.403 )
    ( 1379, 67.280 )
    ( 1380, 67.173 )
    ( 1381, 67.119 )
    ( 1382, 66.994 )
    ( 1383, 66.955 )
    ( 1384, 66.913 )
    ( 1385, 66.792 )
    ( 1386, 66.705 )
    ( 1387, 66.734 )
    ( 1388, 66.666 )
    ( 1389, 66.597 )
    ( 1390, 66.479 )
    ( 1391, 66.415 )
    ( 1392, 66.341 )
    ( 1393, 66.220 )
    ( 1394, 66.139 )
    ( 1395, 66.014 )
    ( 1396, 65.889 )
    ( 1397, 65.823 )
    ( 1398, 65.771 )
    ( 1399, 65.679 )
    ( 1400, 65.582 )
    ( 1401, 65.522 )
    ( 1402, 65.433 )
    ( 1403, 65.133 )
    ( 1404, 64.841 )
    ( 1405, 64.541 )
    ( 1406, 64.240 )
    ( 1407, 63.960 )
    ( 1408, 63.764 )
    ( 1409, 63.499 )
    ( 1410, 63.198 )
    ( 1411, 62.958 )
    ( 1412, 62.813 )
    ( 1413, 62.667 )
    ( 1414, 62.366 )
    ( 1415, 62.135 )
    ( 1416, 61.897 )
    ( 1417, 61.660 )
    ( 1418, 61.459 )
    ( 1419, 61.263 )
    ( 1420, 60.997 )
    ( 1421, 60.704 )
    ( 1422, 60.570 )
    ( 1423, 60.269 )
    ( 1424, 60.138 )
    ( 1425, 59.992 )
    ( 1426, 59.897 )
    ( 1427, 59.772 )
    ( 1428, 59.471 )
    ( 1429, 59.260 )
    ( 1430, 59.023 )
    ( 1431, 58.803 )
    ( 1432, 58.502 )
    ( 1433, 58.208 )
    ( 1434, 57.931 )
    ( 1435, 57.632 )
    ( 1436, 57.343 )
    ( 1437, 57.049 )
    ( 1438, 56.812 )
    ( 1439, 56.615 )
    ( 1440, 56.314 )
    ( 1441, 56.054 )
    ( 1442, 55.794 )
    ( 1443, 55.525 )
    ( 1444, 55.224 )
    ( 1445, 55.166 )
    ( 1446, 55.232 )
    ( 1447, 55.309 )
    ( 1448, 55.387 )
    ( 1449, 55.513 )
    ( 1450, 55.533 )
    ( 1451, 55.575 )
    ( 1452, 55.521 )
    ( 1453, 55.468 )
    ( 1454, 55.477 )
    ( 1455, 55.490 )
    ( 1456, 55.217 )
    ( 1457, 55.108 )
    ( 1458, 54.808 )
    ( 1459, 54.772 )
    ( 1460, 54.682 )
    ( 1461, 54.381 )
    ( 1462, 54.081 )
    ( 1463, 53.780 )
    ( 1464, 53.546 )
    ( 1465, 53.245 )
    ( 1466, 53.408 )
    ( 1467, 53.404 )
    ( 1468, 53.286 )
    ( 1469, 53.188 )
    ( 1470, 53.072 )
    ( 1471, 52.979 )
    ( 1472, 52.858 )
    ( 1473, 52.844 )
    ( 1474, 52.735 )
    ( 1475, 52.610 )
    ( 1476, 52.735 )
    ( 1477, 52.956 )
    ( 1478, 53.130 )
    ( 1479, 53.293 )
    ( 1480, 53.485 )
    ( 1481, 53.610 )
    ( 1482, 53.735 )
    ( 1483, 53.892 )
    ( 1484, 54.094 )
    ( 1485, 54.306 )
    ( 1486, 54.490 )
    ( 1487, 54.824 )
    ( 1488, 55.161 )
    ( 1489, 55.495 )
    ( 1490, 55.874 )
    ( 1491, 56.204 )
    ( 1492, 56.459 )
    ( 1493, 56.584 )
    ( 1494, 56.727 )
    ( 1495, 56.911 )
    ( 1496, 57.050 )
    ( 1497, 57.239 )
    ( 1498, 57.368 )
    ( 1499, 57.535 )
    ( 1500, 57.660 )
    ( 1501, 57.786 )
    ( 1502, 57.922 )
    ( 1503, 58.047 )
    ( 1504, 58.240 )
    ( 1505, 58.365 )
    ( 1506, 58.514 )
    ( 1507, 58.639 )
    ( 1508, 58.586 )
    ( 1509, 58.628 )
    ( 1510, 58.728 )
    ( 1511, 58.826 )
    ( 1512, 58.739 )
    ( 1513, 58.615 )
    ( 1514, 58.503 )
    ( 1515, 58.544 )
    ( 1516, 58.476 )
    ( 1517, 58.401 )
    ( 1518, 58.327 )
    ( 1519, 58.210 )
    ( 1520, 58.336 )
    ( 1521, 58.461 )
    ( 1522, 58.595 )
    ( 1523, 58.808 )
    ( 1524, 58.933 )
    ( 1525, 59.118 )
    ( 1526, 59.481 )
    ( 1527, 59.790 )
    ( 1528, 60.098 )
    ( 1529, 60.427 )
    ( 1530, 60.778 )
    ( 1531, 61.123 )
    ( 1532, 61.468 )
    ( 1533, 61.776 )
    ( 1534, 61.991 )
    ( 1535, 62.175 )
    ( 1536, 62.364 )
    ( 1537, 62.652 )
    ( 1538, 62.964 )
    ( 1539, 63.243 )
    ( 1540, 63.515 )
    ( 1541, 63.770 )
    ( 1542, 64.155 )
    ( 1543, 64.527 )
    ( 1544, 65.000 )
    ( 1545, 65.473 )
    ( 1546, 65.845 )
    ( 1547, 66.096 )
    ( 1548, 66.285 )
    ( 1549, 66.480 )
    ( 1550, 66.605 )
    ( 1551, 66.861 )
    ( 1552, 67.116 )
    ( 1553, 67.399 )
    ( 1554, 67.679 )
    ( 1555, 67.935 )
    ( 1556, 68.243 )
    ( 1557, 68.552 )
    ( 1558, 68.860 )
    ( 1559, 69.185 )
    ( 1560, 69.466 )
    ( 1561, 69.780 )
    ( 1562, 70.035 )
    ( 1563, 70.349 )
    ( 1564, 70.626 )
    ( 1565, 70.761 )
    ( 1566, 70.886 )
    ( 1567, 71.010 )
    ( 1568, 70.958 )
    ( 1569, 70.847 )
    ( 1570, 70.973 )
    ( 1571, 71.098 )
    ( 1572, 71.224 )
    ( 1573, 71.461 )
    ( 1574, 71.646 )
    ( 1575, 71.770 )
    ( 1576, 71.959 )
    ( 1577, 72.259 )
    ( 1578, 72.536 )
    ( 1579, 72.900 )
    ( 1580, 73.025 )
    ( 1581, 73.176 )
    ( 1582, 73.301 )
    ( 1583, 73.426 )
    ( 1584, 73.598 )
    ( 1585, 73.857 )
    ( 1586, 74.131 )
    ( 1587, 74.386 )
    ( 1588, 74.643 )
    ( 1589, 74.768 )
    ( 1590, 74.935 )
    ( 1591, 75.078 )
    ( 1592, 75.203 )
    ( 1593, 75.328 )
    ( 1594, 75.514 )
    ( 1595, 75.639 )
    ( 1596, 75.514 )
    ( 1597, 75.461 )
    ( 1598, 75.336 )
    ( 1599, 75.222 )
    ( 1600, 75.152 )
    ( 1601, 75.329 )
    ( 1602, 75.461 )
    ( 1603, 75.608 )
    ( 1604, 75.705 )
    ( 1605, 75.896 )
    ( 1606, 76.044 )
    ( 1607, 76.201 )
    ( 1608, 76.397 )
    ( 1609, 76.521 )
    ( 1610, 76.646 )
    ( 1611, 76.769 )
    ( 1612, 76.865 )
    ( 1613, 76.983 )
    ( 1614, 77.081 )
    ( 1615, 77.262 )
    ( 1616, 77.358 )
    ( 1617, 77.493 )
    ( 1618, 77.529 )
    ( 1619, 77.490 )
    ( 1620, 77.434 )
    ( 1621, 77.455 )
    ( 1622, 77.475 )
    ( 1623, 77.494 )
    ( 1624, 77.440 )
    ( 1625, 77.383 )
    ( 1626, 77.390 )
    ( 1627, 77.396 )
    ( 1628, 77.382 )
    ( 1629, 77.257 )
    ( 1630, 77.383 )
    ( 1631, 77.571 )
    ( 1632, 77.696 )
    ( 1633, 77.957 )
    ( 1634, 78.197 )
    ( 1635, 78.366 )
    ( 1636, 78.665 )
    ( 1637, 78.795 )
    ( 1638, 79.033 )
    ( 1639, 79.260 )
    ( 1640, 79.227 )
    ( 1641, 79.220 )
    ( 1642, 79.211 )
    ( 1643, 79.175 )
    ( 1644, 79.117 )
    ( 1645, 79.170 )
    ( 1646, 79.112 )
    ( 1647, 79.174 )
    ( 1648, 79.116 )
    ( 1649, 79.109 )
    ( 1650, 79.104 )
    ( 1651, 79.098 )
    ( 1652, 79.251 )
    ( 1653, 79.342 )
    ( 1654, 79.283 )
    ( 1655, 79.226 )
    ( 1656, 79.144 )
    ( 1657, 79.042 )
    ( 1658, 78.995 )
    ( 1659, 78.942 )
    ( 1660, 78.818 )
    ( 1661, 78.693 )
    ( 1662, 78.569 )
    ( 1663, 78.444 )
    ( 1664, 78.523 )
    ( 1665, 78.592 )
    ( 1666, 78.468 )
    ( 1667, 78.356 )
    ( 1668, 78.287 )
    ( 1669, 78.312 )
    ( 1670, 78.300 )
    ( 1671, 78.286 )
    ( 1672, 78.277 )
    ( 1673, 78.215 )
    ( 1674, 78.119 )
    ( 1675, 78.170 )
    ( 1676, 78.143 )
    ( 1677, 77.850 )
    ( 1678, 77.549 )
    ( 1679, 77.264 )
    ( 1680, 77.067 )
    ( 1681, 76.769 )
    ( 1682, 76.472 )
    ( 1683, 76.192 )
    ( 1684, 75.893 )
    ( 1685, 75.592 )
    ( 1686, 75.321 )
    ( 1687, 75.020 )
    ( 1688, 74.720 )
    ( 1689, 74.472 )
    ( 1690, 74.215 )
    ( 1691, 74.130 )
    ( 1692, 73.946 )
    ( 1693, 73.759 )
    ( 1694, 73.467 )
    ( 1695, 73.165 )
    ( 1696, 73.072 )
    ( 1697, 72.771 )
    ( 1698, 72.471 )
    ( 1699, 72.170 )
    ( 1700, 72.074 )
    ( 1701, 71.778 )
    ( 1702, 71.555 )
    ( 1703, 71.253 )
    ( 1704, 71.032 )
    ( 1705, 70.837 )
    ( 1706, 70.583 )
    ( 1707, 70.438 )
    ( 1708, 70.292 )
    ( 1709, 70.171 )
    ( 1710, 69.870 )
    ( 1711, 69.806 )
    ( 1712, 69.761 )
    ( 1713, 69.797 )
    ( 1714, 69.848 )
    ( 1715, 69.873 )
    ( 1716, 69.938 )
    ( 1717, 69.939 )
    ( 1718, 69.692 )
    ( 1719, 69.421 )
    ( 1720, 69.150 )
    ( 1721, 68.954 )
    ( 1722, 68.945 )
    ( 1723, 68.649 )
    ( 1724, 68.348 )
    ( 1725, 68.096 )
    ( 1726, 67.798 )
    ( 1727, 67.539 )
    ( 1728, 67.238 )
    ( 1729, 67.111 )
    ( 1730, 66.979 )
    ( 1731, 66.679 )
    ( 1732, 66.434 )
    ( 1733, 66.173 )
    ( 1734, 65.964 )
    ( 1735, 65.923 )
    ( 1736, 65.669 )
    ( 1737, 65.400 )
    ( 1738, 65.100 )
    ( 1739, 64.862 )
    ( 1740, 64.565 )
    ( 1741, 64.265 )
    ( 1742, 63.963 )
    ( 1743, 64.015 )
    ( 1744, 64.030 )
    ( 1745, 64.103 )
    ( 1746, 64.165 )
    ( 1747, 64.208 )
    ( 1748, 64.209 )
    ( 1749, 64.209 )
    ( 1750, 64.245 )
    ( 1751, 64.255 )
    ( 1752, 64.257 )
    ( 1753, 64.278 )
    ( 1754, 64.281 )
    ( 1755, 64.322 )
    ( 1756, 64.322 )
    ( 1757, 64.329 )
    ( 1758, 64.329 )
    ( 1759, 64.329 )
    ( 1760, 64.392 )
    ( 1761, 64.407 )
    ( 1762, 64.408 )
    ( 1763, 64.437 )
    ( 1764, 64.437 )
    ( 1765, 64.592 )
    ( 1766, 64.738 )
    ( 1767, 64.738 )
    ( 1768, 64.794 )
    ( 1769, 64.921 )
    ( 1770, 64.995 )
    ( 1771, 65.092 )
    ( 1772, 65.154 )
    ( 1773, 65.234 )
    ( 1774, 65.234 )
    ( 1775, 65.244 )
    ( 1776, 65.244 )
    ( 1777, 65.392 )
    ( 1778, 65.603 )
    ( 1779, 65.812 )
    ( 1780, 66.056 )
    ( 1781, 66.215 )
    ( 1782, 66.302 )
    ( 1783, 66.364 )
    ( 1784, 66.380 )
    ( 1785, 66.396 )
    ( 1786, 66.406 )
    ( 1787, 66.408 )
    ( 1788, 66.420 )
    ( 1789, 66.421 )
    ( 1790, 66.465 )
    ( 1791, 66.465 )
    ( 1792, 66.493 )
    ( 1793, 66.493 )
    ( 1794, 66.495 )
    ( 1795, 66.499 )
    ( 1796, 66.543 )
    ( 1797, 66.621 )
    ( 1798, 66.622 )
    ( 1799, 66.649 )
    ( 1800, 66.662 )
    ( 1801, 66.662 )
    ( 1802, 66.734 )
    ( 1803, 66.740 )
    ( 1804, 66.761 )
    ( 1805, 66.762 )
    ( 1806, 66.804 )
    ( 1807, 66.822 )
    ( 1808, 66.845 )
    ( 1809, 66.847 )
    ( 1810, 66.847 )
    ( 1811, 66.993 )
    ( 1812, 67.156 )
    ( 1813, 67.157 )
    ( 1814, 67.157 )
    ( 1815, 67.157 )
    ( 1816, 67.197 )
    ( 1817, 67.200 )
    ( 1818, 67.203 )
    ( 1819, 67.264 )
    ( 1820, 67.268 )
    ( 1821, 67.302 )
    ( 1822, 67.323 )
    ( 1823, 67.339 )
    ( 1824, 67.376 )
    ( 1825, 67.573 )
    ( 1826, 67.680 )
    ( 1827, 67.679 )
    ( 1828, 67.471 )
    ( 1829, 67.429 )
    ( 1830, 67.332 )
    ( 1831, 67.085 )
    ( 1832, 66.783 )
    ( 1833, 66.487 )
    ( 1834, 66.187 )
    ( 1835, 65.896 )
    ( 1836, 65.626 )
    ( 1837, 65.354 )
    ( 1838, 65.066 )
    ( 1839, 65.040 )
    ( 1840, 64.781 )
    ( 1841, 64.480 )
    ( 1842, 64.210 )
    ( 1843, 63.909 )
    ( 1844, 63.614 )
    ( 1845, 63.313 )
    ( 1846, 63.279 )
    ( 1847, 63.408 )
    ( 1848, 63.633 )
    ( 1849, 63.853 )
    ( 1850, 63.979 )
    ( 1851, 64.104 )
    ( 1852, 64.229 )
    ( 1853, 64.392 )
    ( 1854, 64.521 )
    ( 1855, 64.671 )
    ( 1856, 64.798 )
    ( 1857, 65.092 )
    ( 1858, 65.347 )
    ( 1859, 65.473 )
    ( 1860, 65.662 )
    ( 1861, 65.870 )
    ( 1862, 66.039 )
    ( 1863, 66.316 )
    ( 1864, 66.195 )
    ( 1865, 66.298 )
    ( 1866, 66.258 )
    ( 1867, 66.208 )
    ( 1868, 66.230 )
    ( 1869, 66.213 )
    ( 1870, 66.198 )
    ( 1871, 66.312 )
    ( 1872, 66.360 )
    ( 1873, 66.418 )
    ( 1874, 66.329 )
    ( 1875, 66.407 )
    ( 1876, 66.449 )
    ( 1877, 66.490 )
    ( 1878, 66.646 )
    ( 1879, 66.708 )
    ( 1880, 66.750 )
    ( 1881, 66.818 )
    ( 1882, 66.693 )
    ( 1883, 66.640 )
    ( 1884, 66.682 )
    ( 1885, 66.724 )
    ( 1886, 66.786 )
    ( 1887, 66.705 )
    ( 1888, 66.586 )
    ( 1889, 66.484 )
    ( 1890, 66.393 )
    ( 1891, 66.311 )
    ( 1892, 66.217 )
    ( 1893, 66.115 )
    ( 1894, 66.120 )
    ( 1895, 66.017 )
    ( 1896, 65.900 )
    ( 1897, 65.789 )
    ( 1898, 65.979 )
    ( 1899, 66.104 )
    ( 1900, 66.036 )
    ( 1901, 65.919 )
    ( 1902, 65.808 )
    ( 1903, 65.683 )
    ( 1904, 65.597 )
    ( 1905, 65.747 )
    ( 1906, 65.623 )
    ( 1907, 65.524 )
    ( 1908, 65.399 )
    ( 1909, 65.381 )
    ( 1910, 65.333 )
    ( 1911, 65.300 )
    ( 1912, 65.243 )
    ( 1913, 65.188 )
    ( 1914, 65.337 )
    ( 1915, 65.485 )
    ( 1916, 65.543 )
    ( 1917, 65.487 )
    ( 1918, 65.433 )
    ( 1919, 65.375 )
    ( 1920, 65.432 )
    ( 1921, 65.375 )
    ( 1922, 65.334 )
    ( 1923, 65.308 )
    ( 1924, 65.250 )
    ( 1925, 65.262 )
    ( 1926, 65.261 )
    ( 1927, 65.247 )
    ( 1928, 65.382 )
    ( 1929, 65.526 )
    ( 1930, 65.525 )
    ( 1931, 65.523 )
    ( 1932, 65.910 )
    ( 1933, 66.121 )
    ( 1934, 66.332 )
    ( 1935, 66.573 )
    ( 1936, 66.784 )
    ( 1937, 67.117 )
    ( 1938, 67.449 )
    ( 1939, 67.791 )
    ( 1940, 68.134 )
    ( 1941, 68.474 )
    ( 1942, 68.818 )
    ( 1943, 69.225 )
    ( 1944, 69.563 )
    ( 1945, 69.938 )
    ( 1946, 70.344 )
    ( 1947, 70.705 )
    ( 1948, 71.077 )
    ( 1949, 71.384 )
    ( 1950, 71.503 )
    ( 1951, 71.496 )
    ( 1952, 71.482 )
    ( 1953, 71.474 )
    ( 1954, 71.546 )
    ( 1955, 71.574 )
    ( 1956, 71.590 )
    ( 1957, 71.589 )
    ( 1958, 71.579 )
    ( 1959, 71.726 )
    ( 1960, 71.697 )
    ( 1961, 71.556 )
    ( 1962, 71.256 )
    ( 1963, 71.199 )
    ( 1964, 71.244 )
    ( 1965, 71.272 )
    ( 1966, 71.176 )
    ( 1967, 71.079 )
    ( 1968, 70.778 )
    ( 1969, 70.584 )
    ( 1970, 70.392 )
    ( 1971, 70.091 )
    ( 1972, 69.963 )
    ( 1973, 69.662 )
    ( 1974, 69.361 )
    ( 1975, 69.188 )
    ( 1976, 68.977 )
    ( 1977, 68.949 )
    ( 1978, 68.922 )
    ( 1979, 68.837 )
    ( 1980, 68.884 )
    ( 1981, 68.688 )
    ( 1982, 68.398 )
    ( 1983, 68.121 )
    ( 1984, 67.850 )
    ( 1985, 67.613 )
    ( 1986, 67.312 )
    ( 1987, 67.247 )
    ( 1988, 67.190 )
    ( 1989, 67.171 )
    ( 1990, 67.122 )
    ( 1991, 67.116 )
    ( 1992, 66.825 )
    ( 1993, 66.614 )
    ( 1994, 66.403 )
    ( 1995, 66.255 )
    ( 1996, 66.035 )
    ( 1997, 65.739 )
    ( 1998, 65.438 )
    ( 1999, 65.138 )
    ( 2000, 64.850 )
    ( 2001, 64.661 )
    ( 2002, 64.491 )
    ( 2003, 64.327 )
    ( 2004, 64.069 )
    ( 2005, 63.839 )
    ( 2006, 63.538 )
    ( 2007, 63.237 )
    ( 2008, 62.936 )
    ( 2009, 62.635 )
    ( 2010, 62.362 )
    ( 2011, 62.151 )
    ( 2012, 62.054 )
    ( 2013, 62.006 )
    ( 2014, 61.910 )
    ( 2015, 61.619 )
    ( 2016, 61.473 )
    ( 2017, 61.176 )
    ( 2018, 60.875 )
    ( 2019, 60.592 )
    ( 2020, 60.436 )
    ( 2021, 60.289 )
    ( 2022, 60.157 )
    ( 2023, 60.039 )
    ( 2024, 59.893 )
    ( 2025, 59.866 )
    ( 2026, 59.670 )
    ( 2027, 59.374 )
    ( 2028, 59.077 )
    ( 2029, 58.816 )
    ( 2030, 58.523 )
    ( 2031, 58.245 )
    ( 2032, 57.949 )
    ( 2033, 57.648 )
    ( 2034, 57.445 )
    ( 2035, 57.144 )
    ( 2036, 57.186 )
    ( 2037, 57.253 )
    ( 2038, 57.129 )
    ( 2039, 57.004 )
    ( 2040, 56.879 )
    ( 2041, 56.754 )
    ( 2042, 56.682 )
    ( 2043, 56.557 )
    ( 2044, 56.812 )
    ( 2045, 56.938 )
    ( 2046, 57.083 )
    ( 2047, 57.209 )
    ( 2048, 57.408 )
    ( 2049, 57.534 )
    ( 2050, 57.728 )
    ( 2051, 57.856 )
    ( 2052, 57.981 )
    ( 2053, 58.141 )
    ( 2054, 58.271 )
    ( 2055, 58.396 )
    ( 2056, 58.521 )
    ( 2057, 58.719 )
    ( 2058, 58.908 )
    ( 2059, 59.106 )
    ( 2060, 59.250 )
    ( 2061, 59.434 )
    ( 2062, 59.635 )
    ( 2063, 59.819 )
    ( 2064, 60.012 )
    ( 2065, 60.196 )
    ( 2066, 60.398 )
    ( 2067, 60.531 )
    ( 2068, 60.695 )
    ( 2069, 60.880 )
    ( 2070, 61.196 )
    ( 2071, 61.504 )
    ( 2072, 61.749 )
    ( 2073, 62.014 )
    ( 2074, 62.218 )
    ( 2075, 62.484 )
    ( 2076, 62.708 )
    ( 2077, 62.916 )
    ( 2078, 63.181 )
    ( 2079, 63.481 )
    ( 2080, 63.692 )
    ( 2081, 63.903 )
    ( 2082, 64.153 )
    ( 2083, 64.365 )
    ( 2084, 64.576 )
    ( 2085, 64.854 )
    ( 2086, 65.074 )
    ( 2087, 65.304 )
    ( 2088, 65.636 )
    ( 2089, 65.984 )
    ( 2090, 66.356 )
    ( 2091, 66.747 )
    ( 2092, 66.994 )
    ( 2093, 67.269 )
    ( 2094, 67.490 )
    ( 2095, 67.723 )
    ( 2096, 67.938 )
    ( 2097, 67.961 )
    ( 2098, 67.985 )
    ( 2099, 67.979 )
    ( 2100, 67.854 )
    ( 2101, 67.781 )
    ( 2102, 67.662 )
    ( 2103, 67.537 )
    ( 2104, 67.496 )
    ( 2105, 67.371 )
    ( 2106, 67.284 )
    ( 2107, 67.221 )
    ( 2108, 67.146 )
    ( 2109, 67.145 )
    ( 2110, 67.258 )
    ( 2111, 67.330 )
    ( 2112, 67.440 )
    ( 2113, 67.434 )
    ( 2114, 67.361 )
    ( 2115, 67.316 )
    ( 2116, 67.207 )
    ( 2117, 67.155 )
    ( 2118, 67.088 )
    ( 2119, 67.040 )
    ( 2120, 66.916 )
    ( 2121, 66.875 )
    ( 2122, 66.868 )
    ( 2123, 66.938 )
    ( 2124, 67.024 )
    ( 2125, 67.079 )
    ( 2126, 67.142 )
    ( 2127, 67.017 )
    ( 2128, 66.896 )
    ( 2129, 66.771 )
    ( 2130, 66.698 )
    ( 2131, 66.573 )
    ( 2132, 66.273 )
    ( 2133, 65.973 )
    ( 2134, 65.672 )
    ( 2135, 65.436 )
    ( 2136, 65.207 )
    ( 2137, 64.915 )
    ( 2138, 64.614 )
    ( 2139, 64.332 )
    ( 2140, 64.121 )
    ( 2141, 63.928 )
    ( 2142, 63.626 )
    ( 2143, 63.360 )
    ( 2144, 63.183 )
    ( 2145, 63.139 )
    ( 2146, 62.838 )
    ( 2147, 62.542 )
    ( 2148, 62.242 )
    ( 2149, 61.941 )
    ( 2150, 61.809 )
    ( 2151, 61.724 )
    ( 2152, 61.681 )
    ( 2153, 61.455 )
    ( 2154, 61.196 )
    ( 2155, 61.057 )
    ( 2156, 60.779 )
    ( 2157, 60.480 )
    ( 2158, 60.195 )
    ( 2159, 59.911 )
    ( 2160, 59.700 )
    ( 2161, 59.462 )
    ( 2162, 59.422 )
    ( 2163, 59.122 )
    ( 2164, 59.038 )
    ( 2165, 58.737 )
    ( 2166, 58.436 )
    ( 2167, 58.225 )
    ( 2168, 57.933 )
    ( 2169, 57.722 )
    ( 2170, 57.421 )
    ( 2171, 57.120 )
    ( 2172, 56.819 )
    ( 2173, 56.537 )
    ( 2174, 56.586 )
    ( 2175, 56.476 )
    ( 2176, 56.382 )
    ( 2177, 56.081 )
    ( 2178, 55.932 )
    ( 2179, 55.721 )
    ( 2180, 55.658 )
    ( 2181, 55.357 )
    ( 2182, 55.056 )
    ( 2183, 54.846 )
    ( 2184, 54.545 )
    ( 2185, 54.502 )
    ( 2186, 54.456 )
    ( 2187, 54.155 )
    ( 2188, 53.934 )
    ( 2189, 53.644 )
    ( 2190, 53.367 )
    ( 2191, 53.066 )
    ( 2192, 52.766 )
    ( 2193, 52.551 )
    ( 2194, 52.323 )
    ( 2195, 52.044 )
    ( 2196, 51.743 )
    ( 2197, 51.502 )
    ( 2198, 51.399 )
    ( 2199, 51.110 )
    ( 2200, 50.811 )
    ( 2201, 50.528 )
    ( 2202, 50.432 )
    ( 2203, 50.210 )
    ( 2204, 49.910 )
    ( 2205, 49.633 )
    ( 2206, 49.332 )
    ( 2207, 49.061 )
    ( 2208, 48.963 )
    ( 2209, 48.867 )
    ( 2210, 48.565 )
    ( 2211, 48.315 )
    ( 2212, 48.014 )
    ( 2213, 47.731 )
    ( 2214, 47.430 )
    ( 2215, 47.137 )
    ( 2216, 46.858 )
    ( 2217, 46.561 )
    ( 2218, 46.260 )
    ( 2219, 46.049 )
    ( 2220, 45.752 )
    ( 2221, 45.454 )
    ( 2222, 45.152 )
    ( 2223, 44.885 )
    ( 2224, 44.586 )
    ( 2225, 44.285 )
    ( 2226, 44.402 )
    ( 2227, 44.406 )
    ( 2228, 44.409 )
    ( 2229, 44.490 )
    ( 2230, 44.490 )
    ( 2231, 44.765 )
    ( 2232, 45.044 )
    ( 2233, 45.360 )
    ( 2234, 45.653 )
    ( 2235, 45.985 )
    ( 2236, 46.272 )
    ( 2237, 46.322 )
    ( 2238, 46.322 )
    ( 2239, 46.548 )
    ( 2240, 46.826 )
    ( 2241, 47.123 )
    ( 2242, 47.399 )
    ( 2243, 47.675 )
    ( 2244, 47.951 )
    ( 2245, 47.959 )
    ( 2246, 48.009 )
    ( 2247, 48.009 )
    ( 2248, 48.027 )
    ( 2249, 48.076 )
    ( 2250, 48.076 )
    ( 2251, 48.415 )
    ( 2252, 48.751 )
    ( 2253, 49.201 )
    ( 2254, 49.651 )
    ( 2255, 50.105 )
    ( 2256, 50.436 )
    ( 2257, 50.794 )
    ( 2258, 51.154 )
    ( 2259, 51.478 )
    ( 2260, 51.817 )
    ( 2261, 52.151 )
    ( 2262, 52.475 )
    ( 2263, 52.784 )
    ( 2264, 53.056 )
    ( 2265, 53.319 )
    ( 2266, 53.542 )
    ( 2267, 53.542 )
    ( 2268, 53.840 )
    ( 2269, 54.063 )
    ( 2270, 54.339 )
    ( 2271, 54.652 )
    ( 2272, 54.745 )
    ( 2273, 54.771 )
    ( 2274, 54.793 )
    ( 2275, 54.809 )
    ( 2276, 54.821 )
    ( 2277, 54.821 )
    ( 2278, 54.821 )
    ( 2279, 54.821 )
    ( 2280, 54.884 )
    ( 2281, 54.915 )
    ( 2282, 54.915 )
    ( 2283, 54.940 )
    ( 2284, 55.001 )
    ( 2285, 55.134 )
    ( 2286, 55.216 )
    ( 2287, 55.319 )
    ( 2288, 55.320 )
    ( 2289, 55.364 )
    ( 2290, 55.371 )
    ( 2291, 55.371 )
    ( 2292, 55.372 )
    ( 2293, 55.372 )
    ( 2294, 55.410 )
    ( 2295, 55.411 )
    ( 2296, 55.415 )
    ( 2297, 55.415 )
    ( 2298, 55.433 )
    ( 2299, 55.580 )
    ( 2300, 55.750 )
    ( 2301, 55.896 )
    ( 2302, 56.100 )
    ( 2303, 56.100 )
    ( 2304, 56.106 )
    ( 2305, 56.179 )
    ( 2306, 56.179 )
    ( 2307, 56.179 )
    ( 2308, 56.195 )
    ( 2309, 56.195 )
    ( 2310, 56.282 )
    ( 2311, 56.284 )
    ( 2312, 56.299 )
    ( 2313, 56.352 )
    ( 2314, 56.391 )
    ( 2315, 56.414 )
    ( 2316, 56.573 )
    ( 2317, 56.730 )
    ( 2318, 56.843 )
    ( 2319, 56.849 )
    ( 2320, 56.821 )
    ( 2321, 57.021 )
    ( 2322, 57.225 )
    ( 2323, 57.425 )
    ( 2324, 57.396 )
    ( 2325, 57.149 )
    ( 2326, 56.854 )
    ( 2327, 56.657 )
    ( 2328, 56.546 )
    ( 2329, 56.524 )
    ( 2330, 56.464 )
    ( 2331, 56.169 )
    ( 2332, 55.868 )
    ( 2333, 55.723 )
    ( 2334, 55.596 )
    ( 2335, 55.484 )
    ( 2336, 55.183 )
    ( 2337, 54.882 )
    ( 2338, 54.624 )
    ( 2339, 54.341 )
    ( 2340, 54.041 )
    ( 2341, 53.749 )
    ( 2342, 53.448 )
    ( 2343, 53.390 )
    ( 2344, 53.181 )
    ( 2345, 52.970 )
    ( 2346, 52.668 )
    ( 2347, 52.368 )
    ( 2348, 52.158 )
    ( 2349, 51.931 )
    ( 2350, 51.649 )
    ( 2351, 51.348 )
    ( 2352, 51.202 )
    ( 2353, 50.938 )
    ( 2354, 50.660 )
    ( 2355, 50.359 )
    ( 2356, 50.163 )
    ( 2357, 49.892 )
    ( 2358, 49.654 )
    ( 2359, 49.388 )
    ( 2360, 49.091 )
    ( 2361, 48.790 )
    ( 2362, 48.489 )
    ( 2363, 48.436 )
    ( 2364, 48.620 )
    ( 2365, 48.953 )
    ( 2366, 49.142 )
    ( 2367, 49.326 )
    ( 2368, 49.368 )
    ( 2369, 49.419 )
    ( 2370, 49.531 )
    ( 2371, 49.572 )
    ( 2372, 49.498 )
    ( 2373, 49.374 )
    ( 2374, 49.302 )
    ( 2375, 49.178 )
    ( 2376, 49.077 )
    ( 2377, 48.952 )
    ( 2378, 48.685 )
    ( 2379, 48.474 )
    ( 2380, 48.227 )
    ( 2381, 48.014 )
    ( 2382, 47.868 )
    ( 2383, 47.566 )
    ( 2384, 47.266 )
    ( 2385, 46.964 )
    ( 2386, 46.973 )
    ( 2387, 46.921 )
    ( 2388, 46.863 )
    ( 2389, 46.807 )
    ( 2390, 46.840 )
    ( 2391, 46.812 )
    ( 2392, 46.755 )
    ( 2393, 46.697 )
    ( 2394, 46.669 )
    ( 2395, 46.565 )
    ( 2396, 46.616 )
    ( 2397, 46.717 )
    ( 2398, 46.843 )
    ( 2399, 46.719 )
    ( 2400, 46.619 )
    ( 2401, 46.502 )
    ( 2402, 46.434 )
    ( 2403, 46.324 )
    ( 2404, 46.533 )
    ( 2405, 46.569 )
    ( 2406, 46.579 )
    ( 2407, 46.565 )
    ( 2408, 46.625 )
    ( 2409, 46.611 )
    ( 2410, 46.598 )
    ( 2411, 46.659 )
    ( 2412, 46.740 )
    ( 2413, 46.833 )
    ( 2414, 46.916 )
    ( 2415, 46.916 )
    ( 2416, 46.905 )
    ( 2417, 46.907 )
    ( 2418, 46.906 )
    ( 2419, 46.976 )
    ( 2420, 46.980 )
    ( 2421, 46.973 )
    ( 2422, 46.948 )
    ( 2423, 47.051 )
    ( 2424, 47.137 )
    ( 2425, 47.108 )
    ( 2426, 47.181 )
    ( 2427, 47.241 )
    ( 2428, 47.293 )
    ( 2429, 47.280 )
    ( 2430, 47.324 )
    ( 2431, 47.310 )
    ( 2432, 47.283 )
    ( 2433, 47.255 )
    ( 2434, 47.292 )
    ( 2435, 47.264 )
    ( 2436, 47.206 )
    ( 2437, 47.222 )
    ( 2438, 47.280 )
    ( 2439, 47.222 )
    ( 2440, 47.276 )
    ( 2441, 47.332 )
    ( 2442, 47.367 )
    ( 2443, 47.412 )
    ( 2444, 47.452 )
    ( 2445, 47.528 )
    ( 2446, 47.470 )
    ( 2447, 47.183 )
    ( 2448, 46.882 )
    ( 2449, 46.656 )
    ( 2450, 46.354 )
    ( 2451, 46.054 )
    ( 2452, 45.759 )
    ( 2453, 45.458 )
    ( 2454, 45.184 )
    ( 2455, 44.932 )
    ( 2456, 44.631 )
    ( 2457, 44.351 )
    ( 2458, 44.051 )
    ( 2459, 43.859 )
    ( 2460, 43.663 )
    ( 2461, 43.369 )
    ( 2462, 43.068 )
    ( 2463, 42.768 )
    ( 2464, 42.493 )
    ( 2465, 42.297 )
    ( 2466, 42.244 )
    ( 2467, 42.100 )
    ( 2468, 41.955 )
    ( 2469, 41.654 )
    ( 2470, 41.836 )
    ( 2471, 41.987 )
    ( 2472, 41.931 )
    ( 2473, 41.893 )
    ( 2474, 41.850 )
    ( 2475, 41.836 )
    ( 2476, 41.935 )
    ( 2477, 41.984 )
    ( 2478, 42.085 )
    ( 2479, 42.131 )
    ( 2480, 42.006 )
    ( 2481, 41.960 )
    ( 2482, 41.946 )
    ( 2483, 41.821 )
    ( 2484, 41.876 )
    ( 2485, 41.922 )
    ( 2486, 41.963 )
    ( 2487, 42.005 )
    ( 2488, 42.106 )
    ( 2489, 41.981 )
    ( 2490, 41.856 )
    ( 2491, 41.732 )
    ( 2492, 41.874 )
    ( 2493, 41.837 )
    ( 2494, 41.796 )
    ( 2495, 41.727 )
    ( 2496, 41.686 )
    ( 2497, 41.617 )
    ( 2498, 41.496 )
    ( 2499, 41.384 )
    ( 2500, 41.460 )
    ( 2501, 41.532 )
    ( 2502, 41.434 )
    ( 2503, 41.314 )
    ( 2504, 41.191 )
    ( 2505, 41.066 )
    ( 2506, 40.941 )
    ( 2507, 40.910 )
    ( 2508, 40.785 )
    ( 2509, 40.540 )
    ( 2510, 40.239 )
    ( 2511, 40.142 )
    ( 2512, 40.045 )
    ( 2513, 39.751 )
    ( 2514, 39.504 )
    ( 2515, 39.477 )
    ( 2516, 39.470 )
    ( 2517, 39.374 )
    ( 2518, 39.228 )
    ( 2519, 39.082 )
    ( 2520, 38.938 )
    ( 2521, 38.751 )
    ( 2522, 38.580 )
    ( 2523, 38.473 )
    ( 2524, 38.287 )
    ( 2525, 37.993 )
    ( 2526, 37.804 )
    ( 2527, 37.608 )
    ( 2528, 37.458 )
    ( 2529, 37.157 )
    ( 2530, 36.960 )
    ( 2531, 36.731 )
    ( 2532, 36.771 )
    ( 2533, 36.675 )
    ( 2534, 36.445 )
    ( 2535, 36.248 )
    ( 2536, 36.038 )
    ( 2537, 35.746 )
    ( 2538, 35.505 )
    ( 2539, 35.204 )
    ( 2540, 34.994 )
    ( 2541, 34.692 )
    ( 2542, 34.564 )
    ( 2543, 34.379 )
    ( 2544, 34.108 )
    ( 2545, 33.837 )
    ( 2546, 33.539 )
    ( 2547, 33.301 )
    ( 2548, 33.003 )
    ( 2549, 32.922 )
    ( 2550, 32.916 )
    ( 2551, 32.615 )
    ( 2552, 32.521 )
    ( 2553, 32.423 )
    ( 2554, 32.438 )
    ( 2555, 32.379 )
    ( 2556, 32.352 )
    ( 2557, 32.368 )
    ( 2558, 32.271 )
    ( 2559, 32.258 )
    ( 2560, 32.208 )
    ( 2561, 32.142 )
    ( 2562, 32.076 )
    ( 2563, 31.980 )
    ( 2564, 31.684 )
    ( 2565, 31.384 )
    ( 2566, 31.083 )
    ( 2567, 30.788 )
    ( 2568, 30.557 )
    ( 2569, 30.265 )
    ( 2570, 30.113 )
    ( 2571, 29.995 )
    ( 2572, 29.715 )
    ( 2573, 29.443 )
    ( 2574, 29.148 )
    ( 2575, 28.932 )
    ( 2576, 28.649 )
    ( 2577, 28.353 )
    ( 2578, 28.052 )
    ( 2579, 27.751 )
    ( 2580, 27.555 )
    ( 2581, 27.254 )
    ( 2582, 27.278 )
    ( 2583, 27.197 )
    ( 2584, 27.217 )
    ( 2585, 27.130 )
    ( 2586, 27.033 )
    ( 2587, 26.938 )
    ( 2588, 27.011 )
    ( 2589, 26.865 )
    ( 2590, 26.564 )
    ( 2591, 26.263 )
    ( 2592, 26.047 )
    ( 2593, 25.763 )
    ( 2594, 25.477 )
    ( 2595, 25.304 )
    ( 2596, 25.130 )
    ( 2597, 24.829 )
    ( 2598, 24.656 )
    ( 2599, 24.355 )
    ( 2600, 24.208 )
    ( 2601, 23.917 )
    ( 2602, 23.685 )
    ( 2603, 23.389 )
    ( 2604, 23.128 )
    ( 2605, 23.031 )
    ( 2606, 22.794 )
    ( 2607, 22.601 )
    ( 2608, 22.495 )
    ( 2609, 22.355 )
    ( 2610, 22.055 )
    ( 2611, 21.754 )
    ( 2612, 21.622 )
    ( 2613, 21.321 )
    ( 2614, 21.028 )
    ( 2615, 20.727 )
    ( 2616, 20.570 )
    ( 2617, 20.416 )
    ( 2618, 20.178 )
    ( 2619, 19.898 )
    ( 2620, 19.802 )
    ( 2621, 19.561 )
    ( 2622, 19.260 )
    ( 2623, 19.135 )
    ( 2624, 19.017 )
    ( 2625, 18.716 )
    ( 2626, 18.502 )
    ( 2627, 18.416 )
    ( 2628, 18.116 )
    ( 2629, 17.815 )
    ( 2630, 17.731 )
    ( 2631, 17.715 )
    ( 2632, 17.427 )
    ( 2633, 17.160 )
    ( 2634, 17.024 )
    ( 2635, 16.839 )
    ( 2636, 16.611 )
    ( 2637, 16.310 )
    ( 2638, 16.327 )
    ( 2639, 16.344 )
    ( 2640, 16.520 )
    ( 2641, 16.793 )
    ( 2642, 17.086 )
    ( 2643, 17.359 )
    ( 2644, 17.598 )
    ( 2645, 17.861 )
    ( 2646, 17.861 )
    ( 2647, 17.861 )
    ( 2648, 18.108 )
    ( 2649, 18.380 )
    ( 2650, 18.784 )
    ( 2651, 19.137 )
    ( 2652, 19.363 )
    ( 2653, 19.732 )
    ( 2654, 20.008 )
    ( 2655, 20.033 )
    ( 2656, 20.056 )
    ( 2657, 20.056 )
    ( 2658, 20.056 )
    ( 2659, 20.228 )
    ( 2660, 20.413 )
    ( 2661, 20.604 )
    ( 2662, 20.750 )
    ( 2663, 20.896 )
    ( 2664, 20.924 )
    ( 2665, 21.041 )
    ( 2666, 21.043 )
    ( 2667, 21.120 )
    ( 2668, 21.183 )
    ( 2669, 21.226 )
    ( 2670, 21.242 )
    ( 2671, 21.314 )
    ( 2672, 21.213 )
    ( 2673, 21.132 )
    ( 2674, 21.039 )
    ( 2675, 20.914 )
    ( 2676, 21.114 )
    ( 2677, 21.374 )
    ( 2678, 21.665 )
    ( 2679, 21.865 )
    ( 2680, 22.064 )
    ( 2681, 22.264 )
    ( 2682, 22.464 )
    ( 2683, 22.678 )
    ( 2684, 22.940 )
    ( 2685, 23.151 )
    ( 2686, 23.350 )
    ( 2687, 23.622 )
    ( 2688, 23.894 )
    ( 2689, 24.172 )
    ( 2690, 24.252 )
    ( 2691, 24.392 )
    ( 2692, 24.479 )
    ( 2693, 24.624 )
    ( 2694, 24.711 )
    ( 2695, 24.884 )
    ( 2696, 25.082 )
    ( 2697, 25.194 )
    ( 2698, 25.281 )
    ( 2699, 25.408 )
    ( 2700, 25.580 )
    ( 2701, 25.835 )
    ( 2702, 26.021 )
    ( 2703, 26.091 )
    ( 2704, 26.158 )
    ( 2705, 26.246 )
    ( 2706, 26.355 )
    ( 2707, 26.466 )
    ( 2708, 26.469 )
    ( 2709, 26.582 )
    ( 2710, 26.625 )
    ( 2711, 26.894 )
    ( 2712, 27.042 )
    ( 2713, 27.042 )
    ( 2714, 27.182 )
    ( 2715, 27.307 )
    ( 2716, 27.478 )
    ( 2717, 27.565 )
    ( 2718, 27.565 )
    ( 2719, 27.729 )
    ( 2720, 27.735 )
    ( 2721, 27.744 )
    ( 2722, 27.744 )
    ( 2723, 27.816 )
    ( 2724, 27.816 )
    ( 2725, 27.831 )
    ( 2726, 27.873 )
    ( 2727, 27.909 )
    ( 2728, 27.909 )
    ( 2729, 28.145 )
    ( 2730, 28.367 )
    ( 2731, 28.662 )
    ( 2732, 28.949 )
    ( 2733, 29.184 )
    ( 2734, 29.443 )
    ( 2735, 29.621 )
    ( 2736, 29.822 )
    ( 2737, 30.108 )
    ( 2738, 30.400 )
    ( 2739, 30.674 )
    ( 2740, 30.986 )
    ( 2741, 31.258 )
    ( 2742, 31.480 )
    ( 2743, 31.777 )
    ( 2744, 32.039 )
    ( 2745, 32.281 )
    ( 2746, 32.518 )
    ( 2747, 32.662 )
    ( 2748, 32.801 )
    ( 2749, 32.868 )
    ( 2750, 32.961 )
    ( 2751, 33.040 )
    ( 2752, 33.209 )
    ( 2753, 33.384 )
    ( 2754, 33.452 )
    ( 2755, 33.522 )
    ( 2756, 33.769 )
    ( 2757, 34.041 )
    ( 2758, 34.297 )
    ( 2759, 34.418 )
    ( 2760, 34.512 )
    ( 2761, 34.615 )
    ( 2762, 34.687 )
    ( 2763, 34.754 )
    ( 2764, 34.878 )
    ( 2765, 35.033 )
    ( 2766, 35.147 )
    ( 2767, 35.227 )
    ( 2768, 35.416 )
    ( 2769, 35.631 )
    ( 2770, 35.831 )
    ( 2771, 36.045 )
    ( 2772, 36.112 )
    ( 2773, 36.179 )
    ( 2774, 36.246 )
    ( 2775, 36.339 )
    ( 2776, 36.433 )
    ( 2777, 36.439 )
    ( 2778, 36.458 )
    ( 2779, 36.604 )
    ( 2780, 36.750 )
    ( 2781, 36.896 )
    ( 2782, 36.937 )
    ( 2783, 36.950 )
    ( 2784, 36.950 )
    ( 2785, 36.971 )
    ( 2786, 37.008 )
    ( 2787, 37.009 )
    ( 2788, 37.009 )
    ( 2789, 37.121 )
    ( 2790, 37.230 )
    ( 2791, 37.230 )
    ( 2792, 37.239 )
    ( 2793, 37.239 )
    ( 2794, 37.239 )
    ( 2795, 37.335 )
    ( 2796, 37.335 )
    ( 2797, 37.408 )
    ( 2798, 37.472 )
    ( 2799, 37.534 )
    ( 2800, 37.607 )
    ( 2801, 37.626 )
    ( 2802, 37.740 )
    ( 2803, 37.827 )
    ( 2804, 37.874 )
    ( 2805, 37.910 )
    ( 2806, 37.911 )
    ( 2807, 37.923 )
    ( 2808, 37.923 )
    ( 2809, 38.137 )
    ( 2810, 38.284 )
    ( 2811, 38.430 )
    ( 2812, 38.560 )
    ( 2813, 38.787 )
    ( 2814, 38.927 )
    ( 2815, 39.083 )
    ( 2816, 39.208 )
    ( 2817, 39.343 )
    ( 2818, 39.473 )
    ( 2819, 39.634 )
    ( 2820, 39.846 )
    ( 2821, 40.041 )
    ( 2822, 40.353 )
    ( 2823, 40.478 )
    ( 2824, 40.612 )
    ( 2825, 40.737 )
    ( 2826, 40.863 )
    ( 2827, 41.001 )
    ( 2828, 41.196 )
    ( 2829, 41.516 )
    ( 2830, 41.650 )
    ( 2831, 41.800 )
    ( 2832, 41.978 )
    ( 2833, 42.128 )
    ( 2834, 42.197 )
    ( 2835, 42.269 )
    ( 2836, 42.341 )
    ( 2837, 42.415 )
    ( 2838, 42.491 )
    ( 2839, 42.561 )
    ( 2840, 42.801 )
    ( 2841, 43.034 )
    ( 2842, 43.305 )
    ( 2843, 43.532 )
    ( 2844, 43.533 )
    ( 2845, 43.533 )
    ( 2846, 43.679 )
    ( 2847, 43.822 )
    ( 2848, 43.858 )
    ( 2849, 43.859 )
    ( 2850, 43.859 )
    ( 2851, 43.859 )
    ( 2852, 43.888 )
    ( 2853, 43.890 )
    ( 2854, 43.917 )
    ( 2855, 43.917 )
    ( 2856, 43.925 )
    ( 2857, 44.035 )
    ( 2858, 44.035 )
    ( 2859, 44.035 )
    ( 2860, 44.255 )
    ( 2861, 44.519 )
    ( 2862, 44.596 )
    ( 2863, 44.690 )
    ( 2864, 44.763 )
    ( 2865, 44.875 )
    ( 2866, 44.957 )
    ( 2867, 45.170 )
    ( 2868, 45.248 )
    ( 2869, 45.453 )
    ( 2870, 45.657 )
    ( 2871, 45.878 )
    ( 2872, 46.092 )
    ( 2873, 46.342 )
    ( 2874, 46.561 )
    ( 2875, 46.792 )
    ( 2876, 47.019 )
    ( 2877, 47.247 )
    ( 2878, 47.313 )
    ( 2879, 47.387 )
    ( 2880, 47.593 )
    ( 2881, 47.799 )
    ( 2882, 48.003 )
    ( 2883, 48.182 )
    ( 2884, 48.265 )
    ( 2885, 48.359 )
    ( 2886, 48.446 )
    ( 2887, 48.597 )
    ( 2888, 48.766 )
    ( 2889, 48.935 )
    ( 2890, 49.116 )
    ( 2891, 49.141 )
    ( 2892, 49.192 )
    ( 2893, 49.192 )
    ( 2894, 49.433 )
    ( 2895, 49.556 )
    ( 2896, 49.665 )
    ( 2897, 49.958 )
    ( 2898, 50.235 )
    ( 2899, 50.255 )
    ( 2900, 50.255 )
    ( 2901, 50.256 )
    ( 2902, 50.256 )
    ( 2903, 50.323 )
    ( 2904, 50.527 )
    ( 2905, 50.754 )
    ( 2906, 51.018 )
    ( 2907, 51.187 )
    ( 2908, 51.356 )
    ( 2909, 51.450 )
    ( 2910, 51.557 )
    ( 2911, 51.763 )
    ( 2912, 51.932 )
    ( 2913, 52.028 )
    ( 2914, 52.123 )
    ( 2915, 52.125 )
    ( 2916, 52.173 )
    ( 2917, 52.316 )
    ( 2918, 52.450 )
    ( 2919, 52.478 )
    ( 2920, 52.555 )
    ( 2921, 52.557 )
    ( 2922, 52.557 )
    ( 2923, 52.557 )
    ( 2924, 52.593 )
    ( 2925, 52.778 )
    ( 2926, 52.925 )
    ( 2927, 52.987 )
    ( 2928, 53.049 )
    ( 2929, 53.214 )
    ( 2930, 53.360 )
    ( 2931, 53.507 )
    ( 2932, 53.654 )
    ( 2933, 53.833 )
    ( 2934, 53.943 )
    ( 2935, 53.986 )
    ( 2936, 53.986 )
    ( 2937, 53.986 )
    ( 2938, 54.065 )
    ( 2939, 54.065 )
    ( 2940, 54.065 )
    ( 2941, 54.127 )
    ( 2942, 54.190 )
    ( 2943, 54.258 )
    ( 2944, 54.370 )
    ( 2945, 54.581 )
    ( 2946, 54.585 )
    ( 2947, 54.626 )
    ( 2948, 54.755 )
    ( 2949, 54.763 )
    ( 2950, 54.926 )
    ( 2951, 54.963 )
    ( 2952, 55.109 )
    ( 2953, 55.255 )
    ( 2954, 55.462 )
    ( 2955, 55.476 )
    ( 2956, 55.515 )
    ( 2957, 55.633 )
    ( 2958, 55.691 )
    ( 2959, 55.858 )
    ( 2960, 56.045 )
    ( 2961, 56.267 )
    ( 2962, 56.468 )
    ( 2963, 56.577 )
    ( 2964, 56.587 )
    ( 2965, 56.617 )
    ( 2966, 56.636 )
    ( 2967, 56.663 )
    ( 2968, 56.700 )
    ( 2969, 56.700 )
    ( 2970, 56.702 )
    ( 2971, 56.811 )
    ( 2972, 56.920 )
    ( 2973, 56.943 )
    ( 2974, 56.943 )
    ( 2975, 56.958 )
    ( 2976, 57.006 )
    ( 2977, 57.006 )
    ( 2978, 57.122 )
    ( 2979, 57.274 )
    ( 2980, 57.274 )
    ( 2981, 57.363 )
    ( 2982, 57.363 )
    ( 2983, 57.407 )
    ( 2984, 57.489 )
    ( 2985, 57.525 )
    ( 2986, 57.525 )
    ( 2987, 57.610 )
    ( 2988, 57.610 )
    ( 2989, 57.610 )
    ( 2990, 57.630 )
    ( 2991, 57.630 )
    ( 2992, 57.736 )
    ( 2993, 57.829 )
    ( 2994, 57.923 )
    ( 2995, 58.011 )
    ( 2996, 58.198 )
    ( 2997, 58.325 )
    ( 2998, 58.414 )
    ( 2999, 58.566 )
    ( 3000, 58.710 )
    ( 3001, 58.847 )
    ( 3002, 58.943 )
    ( 3003, 59.061 )
    ( 3004, 59.306 )
    ( 3005, 59.418 )
    ( 3006, 59.658 )
    ( 3007, 59.864 )
    ( 3008, 60.157 )
    ( 3009, 60.444 )
    ( 3010, 60.732 )
    ( 3011, 60.827 )
    ( 3012, 60.921 )
    ( 3013, 61.008 )
    ( 3014, 61.097 )
    ( 3015, 61.197 )
    ( 3016, 61.291 )
    ( 3017, 61.401 )
    ( 3018, 61.495 )
    ( 3019, 61.583 )
    ( 3020, 61.770 )
    ( 3021, 61.770 )
    ( 3022, 61.798 )
    ( 3023, 61.865 )
    ( 3024, 61.932 )
    ( 3025, 62.040 )
    ( 3026, 62.270 )
    ( 3027, 62.404 )
    ( 3028, 62.492 )
    ( 3029, 62.585 )
    ( 3030, 62.754 )
    ( 3031, 62.826 )
    ( 3032, 62.913 )
    ( 3033, 63.002 )
    ( 3034, 63.107 )
    ( 3035, 63.203 )
    ( 3036, 63.281 )
    ( 3037, 63.349 )
    ( 3038, 63.416 )
    ( 3039, 63.483 )
    ( 3040, 63.550 )
    ( 3041, 63.657 )
    ( 3042, 63.785 )
    ( 3043, 64.051 )
    ( 3044, 64.158 )
    ( 3045, 64.287 )
    ( 3046, 64.287 )
    ( 3047, 64.368 )
    ( 3048, 64.436 )
    ( 3049, 64.436 )
    ( 3050, 64.451 )
    ( 3051, 64.453 )
    ( 3052, 64.455 )
    ( 3053, 64.569 )
    ( 3054, 64.688 )
    ( 3055, 64.725 )
    ( 3056, 64.725 )
    ( 3057, 64.743 )
    ( 3058, 64.762 )
    ( 3059, 64.839 )
    ( 3060, 64.996 )
    ( 3061, 65.109 )
    ( 3062, 65.194 )
    ( 3063, 65.394 )
    ( 3064, 65.548 )
    ( 3065, 65.728 )
    ( 3066, 65.877 )
    ( 3067, 65.877 )
    ( 3068, 65.990 )
    ( 3069, 66.170 )
    ( 3070, 66.465 )
    ( 3071, 66.634 )
    ( 3072, 66.932 )
    ( 3073, 67.223 )
    ( 3074, 67.532 )
    ( 3075, 67.719 )
    ( 3076, 67.955 )
    ( 3077, 68.155 )
    ( 3078, 68.360 )
    ( 3079, 68.408 )
    ( 3080, 68.464 )
    ( 3081, 68.536 )
    ( 3082, 68.609 )
    ( 3083, 68.609 )
    ( 3084, 68.611 )
    ( 3085, 68.772 )
    ( 3086, 68.823 )
    ( 3087, 68.877 )
    ( 3088, 68.943 )
    ( 3089, 68.951 )
    ( 3090, 68.951 )
    ( 3091, 69.062 )
    ( 3092, 69.081 )
    ( 3093, 69.081 )
    ( 3094, 69.081 )
    ( 3095, 69.084 )
    ( 3096, 69.112 )
    ( 3097, 69.142 )
    ( 3098, 69.252 )
    ( 3099, 69.295 )
    ( 3100, 69.295 )
    ( 3101, 69.529 )
    ( 3102, 69.755 )
    ( 3103, 70.006 )
    ( 3104, 70.291 )
    ( 3105, 70.588 )
    ( 3106, 70.865 )
    ( 3107, 70.997 )
    ( 3108, 71.126 )
    ( 3109, 71.250 )
    ( 3110, 71.381 )
    ( 3111, 71.526 )
    ( 3112, 71.651 )
    ( 3113, 71.785 )
    ( 3114, 71.929 )
    ( 3115, 72.054 )
    ( 3116, 72.186 )
    ( 3117, 72.311 )
    ( 3118, 72.436 )
    ( 3119, 72.561 )
    ( 3120, 72.686 )
    ( 3121, 73.003 )
    ( 3122, 73.192 )
    ( 3123, 73.354 )
    ( 3124, 73.546 )
    ( 3125, 73.681 )
    ( 3126, 73.918 )
    ( 3127, 74.114 )
    ( 3128, 74.249 )
    ( 3129, 74.312 )
    ( 3130, 74.312 )
    ( 3131, 74.312 )
    ( 3132, 74.318 )
    ( 3133, 74.318 )
    ( 3134, 74.361 )
    ( 3135, 74.389 )
    ( 3136, 74.402 )
    ( 3137, 74.403 )
    ( 3138, 74.405 )
    ( 3139, 74.407 )
    ( 3140, 74.517 )
    ( 3141, 74.626 )
    ( 3142, 74.771 )
    ( 3143, 74.885 )
    ( 3144, 75.223 )
    ( 3145, 75.369 )
    ( 3146, 75.560 )
    ( 3147, 75.725 )
    ( 3148, 75.871 )
    ( 3149, 75.920 )
    ( 3150, 75.920 )
    ( 3151, 75.923 )
    ( 3152, 75.930 )
    ( 3153, 75.936 )
    ( 3154, 75.938 )
    ( 3155, 76.000 )
    ( 3156, 76.034 )
    ( 3157, 76.034 )
    ( 3158, 76.049 )
    ( 3159, 76.049 )
    ( 3160, 76.122 )
    ( 3161, 76.194 )
    ( 3162, 76.200 )
    ( 3163, 76.370 )
    ( 3164, 76.540 )
    ( 3165, 76.648 )
    ( 3166, 76.667 )
    ( 3167, 76.681 )
    ( 3168, 76.827 )
    ( 3169, 77.014 )
    ( 3170, 77.164 )
    ( 3171, 77.322 )
    ( 3172, 77.479 )
    ( 3173, 77.656 )
    ( 3174, 77.729 )
    ( 3175, 77.758 )
    ( 3176, 77.775 )
    ( 3177, 77.819 )
    ( 3178, 77.887 )
    ( 3179, 77.991 )
    ( 3180, 78.195 )
    ( 3181, 78.446 )
    ( 3182, 78.673 )
    ( 3183, 78.937 )
    ( 3184, 79.142 )
    ( 3185, 79.346 )
    ( 3186, 79.580 )
    ( 3187, 79.785 )
    ( 3188, 80.015 )
    ( 3189, 80.254 )
    ( 3190, 80.468 )
    ( 3191, 80.694 )
    ( 3192, 80.790 )
    ( 3193, 81.052 )
    ( 3194, 81.285 )
    ( 3195, 81.521 )
    ( 3196, 81.743 )
    ( 3197, 81.966 )
    ( 3198, 82.188 )
    ( 3199, 82.499 )
    ( 3200, 82.721 )
    ( 3201, 82.948 )
    ( 3202, 83.179 )
    ( 3203, 83.400 )
    ( 3204, 83.644 )
    ( 3205, 83.882 )
    ( 3206, 84.120 )
    ( 3207, 84.353 )
    ( 3208, 84.575 )
    ( 3209, 84.835 )
    ( 3210, 85.122 )
    ( 3211, 85.374 )
    ( 3212, 85.604 )
    ( 3213, 85.825 )
    ( 3214, 86.047 )
    ( 3215, 86.270 )
    ( 3216, 86.492 )
    ( 3217, 86.780 )
    ( 3218, 87.089 )
    ( 3219, 87.189 )
    ( 3220, 87.309 )
    ( 3221, 87.309 )
    ( 3222, 87.338 )
    ( 3223, 87.367 )
    ( 3224, 87.375 )
    ( 3225, 87.438 )
    ( 3226, 87.500 )
    ( 3227, 87.562 )
    ( 3228, 87.576 )
    ( 3229, 87.577 )
    ( 3230, 87.578 )
    ( 3231, 87.581 )
    ( 3232, 87.644 )
    ( 3233, 87.706 )
    ( 3234, 87.744 )
    ( 3235, 87.795 )
    ( 3236, 87.797 )
    ( 3237, 87.906 )
    ( 3238, 88.022 )
    ( 3239, 88.277 )
    ( 3240, 88.461 )
    ( 3241, 88.606 )
    ( 3242, 88.777 )
    ( 3243, 88.990 )
    ( 3244, 89.244 )
    ( 3245, 89.391 )
    ( 3246, 89.396 )
    ( 3247, 89.428 )
    ( 3248, 89.451 )
    ( 3249, 89.532 )
    ( 3250, 89.533 )
    ( 3251, 89.576 )
    ( 3252, 89.577 )
    ( 3253, 89.604 )
    ( 3254, 89.653 )
    ( 3255, 89.678 )
    ( 3256, 89.691 )
    ( 3257, 89.691 )
    ( 3258, 89.720 )
    ( 3259, 89.720 )
    ( 3260, 89.721 )
    ( 3261, 89.723 )
    ( 3262, 89.729 )
    ( 3263, 89.801 )
    ( 3264, 89.806 )
    ( 3265, 89.887 )
    ( 3266, 89.924 )
    ( 3267, 90.185 )
    ( 3268, 90.278 )
    ( 3269, 90.365 )
    ( 3270, 90.540 )
    ( 3271, 90.724 )
    ( 3272, 90.791 )
    ( 3273, 90.956 )
    ( 3274, 91.023 )
    ( 3275, 91.158 )
    ( 3276, 91.371 )
    ( 3277, 91.547 )
    ( 3278, 91.716 )
    ( 3279, 91.886 )
    ( 3280, 92.055 )
    ( 3281, 92.137 )
    ( 3282, 92.204 )
    ( 3283, 92.271 )
    ( 3284, 92.349 )
    ( 3285, 92.483 )
    ( 3286, 92.576 )
    ( 3287, 92.684 )
    ( 3288, 92.844 )
    ( 3289, 92.979 )
    ( 3290, 93.092 )
    ( 3291, 93.261 )
    ( 3292, 93.331 )
    ( 3293, 93.397 )
    ( 3294, 93.468 )
    ( 3295, 93.712 )
    ( 3296, 93.922 )
    ( 3297, 93.989 )
    ( 3298, 94.082 )
    ( 3299, 94.276 )
    ( 3300, 94.594 )
    ( 3301, 94.910 )
    ( 3302, 95.128 )
    ( 3303, 95.332 )
    ( 3304, 95.536 )
    ( 3305, 95.741 )
    ( 3306, 95.969 )
    ( 3307, 96.173 )
    ( 3308, 96.377 )
    ( 3309, 96.604 )
    ( 3310, 96.678 )
    ( 3311, 96.744 )
    ( 3312, 96.947 )
    ( 3313, 97.158 )
    ( 3314, 97.362 )
    ( 3315, 97.566 )
    ( 3316, 97.770 )
    ( 3317, 97.972 )
    ( 3318, 98.156 )
    ( 3319, 98.364 )
    ( 3320, 98.549 )
    ( 3321, 98.424 )
    ( 3322, 98.299 )
    ( 3323, 98.174 )
    ( 3324, 98.105 )
    ( 3325, 98.039 )
    ( 3326, 97.914 )
    ( 3327, 97.791 )
    ( 3328, 97.695 )
    ( 3329, 97.821 )
    ( 3330, 97.954 )
    ( 3331, 98.080 )
    ( 3332, 98.215 )
    ( 3333, 98.340 )
    ( 3334, 98.465 )
    ( 3335, 98.347 )
    ( 3336, 98.222 )
    ( 3337, 97.921 )
    ( 3338, 97.853 )
    ( 3339, 97.552 )
    ( 3340, 97.263 )
    ( 3341, 96.969 )
    ( 3342, 96.668 )
    ( 3343, 96.367 )
    ( 3344, 96.066 )
    ( 3345, 95.789 )
    ( 3346, 95.522 )
    ( 3347, 95.252 )
    ( 3348, 94.957 )
    ( 3349, 94.659 )
    ( 3350, 94.359 )
    ( 3351, 94.060 )
    ( 3352, 93.823 )
    ( 3353, 93.528 )
    ( 3354, 93.228 )
    ( 3355, 93.116 )
    ( 3356, 92.815 )
    ( 3357, 92.514 )
    ( 3358, 92.455 )
    ( 3359, 92.516 )
    ( 3360, 92.411 )
    ( 3361, 92.163 )
    ( 3362, 91.862 )
    ( 3363, 91.579 )
    ( 3364, 91.287 )
    ( 3365, 91.050 )
    ( 3366, 90.905 )
    ( 3367, 90.604 )
    ( 3368, 90.328 )
    ( 3369, 90.028 )
    ( 3370, 89.728 )
    ( 3371, 89.427 )
    ( 3372, 89.354 )
    ( 3373, 89.281 )
    ( 3374, 89.138 )
    ( 3375, 88.844 )
    ( 3376, 88.545 )
    ( 3377, 88.284 )
    ( 3378, 88.067 )
    ( 3379, 87.819 )
    ( 3380, 87.667 )
    ( 3381, 87.456 )
    ( 3382, 87.155 )
    ( 3383, 87.047 )
    ( 3384, 86.903 )
    ( 3385, 86.927 )
    ( 3386, 86.862 )
    ( 3387, 86.847 )
    ( 3388, 86.871 )
    ( 3389, 86.638 )
    ( 3390, 86.377 )
    ( 3391, 86.076 )
    ( 3392, 85.775 )
    ( 3393, 85.475 )
    ( 3394, 85.200 )
    ( 3395, 84.899 )
    ( 3396, 84.703 )
    ( 3397, 84.402 )
    ( 3398, 84.102 )
    ( 3399, 83.801 )
    ( 3400, 83.521 )
    ( 3401, 83.221 )
    ( 3402, 82.922 )
    ( 3403, 82.825 )
    ( 3404, 82.744 )
    ( 3405, 82.833 )
    ( 3406, 82.851 )
    ( 3407, 82.824 )
    ( 3408, 82.797 )
    ( 3409, 82.713 )
    ( 3410, 82.445 )
    ( 3411, 82.145 )
    ( 3412, 81.923 )
    ( 3413, 81.696 )
    ( 3414, 81.396 )
    ( 3415, 81.319 )
    ( 3416, 81.018 )
    ( 3417, 80.724 )
    ( 3418, 80.422 )
    ( 3419, 80.141 )
    ( 3420, 79.840 )
    ( 3421, 79.632 )
    ( 3422, 79.330 )
    ( 3423, 79.233 )
    ( 3424, 79.139 )
    ( 3425, 79.042 )
    ( 3426, 78.741 )
    ( 3427, 78.595 )
    ( 3428, 78.534 )
    ( 3429, 78.469 )
    ( 3430, 78.170 )
    ( 3431, 77.936 )
    ( 3432, 77.712 )
    ( 3433, 77.590 )
    ( 3434, 77.289 )
    ( 3435, 76.987 )
    ( 3436, 76.691 )
    ( 3437, 76.390 )
    ( 3438, 76.198 )
    ( 3439, 75.904 )
    ( 3440, 75.637 )
    ( 3441, 75.336 )
    ( 3442, 75.035 )
    ( 3443, 74.737 )
    ( 3444, 74.444 )
    ( 3445, 74.188 )
    ( 3446, 73.888 )
    ( 3447, 73.683 )
    ( 3448, 73.390 )
    ( 3449, 73.159 )
    ( 3450, 73.188 )
    ( 3451, 73.216 )
    ( 3452, 73.118 )
    ( 3453, 72.889 )
    ( 3454, 72.600 )
    ( 3455, 72.535 )
    ( 3456, 72.389 )
    ( 3457, 72.088 )
    ( 3458, 71.830 )
    ( 3459, 71.539 )
    ( 3460, 71.301 )
    ( 3461, 71.116 )
    ( 3462, 70.905 )
    ( 3463, 70.696 )
    ( 3464, 70.600 )
    ( 3465, 70.305 )
    ( 3466, 70.003 )
    ( 3467, 70.036 )
    ( 3468, 69.735 )
    ( 3469, 69.442 )
    ( 3470, 69.141 )
    ( 3471, 68.949 )
    ( 3472, 68.648 )
    ( 3473, 68.358 )
    ( 3474, 68.068 )
    ( 3475, 67.864 )
    ( 3476, 67.563 )
    ( 3477, 67.262 )
    ( 3478, 66.961 )
    ( 3479, 66.751 )
    ( 3480, 66.575 )
    ( 3481, 66.345 )
    ( 3482, 66.123 )
    ( 3483, 65.823 )
    ( 3484, 65.521 )
    ( 3485, 65.222 )
    ( 3486, 64.921 )
    ( 3487, 64.698 )
    ( 3488, 64.398 )
    ( 3489, 64.205 )
    ( 3490, 64.087 )
    ( 3491, 63.990 )
    ( 3492, 63.689 )
    ( 3493, 63.388 )
    ( 3494, 63.358 )
    ( 3495, 63.230 )
    ( 3496, 63.084 )
    ( 3497, 63.029 )
    ( 3498, 63.053 )
    ( 3499, 62.968 )
    ( 3500, 62.823 )
    ( 3501, 62.776 )
    ( 3502, 62.630 )
    ( 3503, 62.329 )
    ( 3504, 62.028 )
    ( 3505, 62.150 )
    ( 3506, 62.123 )
    ( 3507, 62.270 )
    ( 3508, 62.211 )
    ( 3509, 62.153 )
    ( 3510, 62.110 )
    ( 3511, 62.055 )
    ( 3512, 61.997 )
    ( 3513, 62.069 )
    ( 3514, 62.041 )
    ( 3515, 61.916 )
    ( 3516, 61.799 )
    ( 3517, 61.674 )
    ( 3518, 61.858 )
    ( 3519, 62.098 )
    ( 3520, 62.275 )
    ( 3521, 62.451 )
    ( 3522, 62.702 )
    ( 3523, 63.040 )
    ( 3524, 63.378 )
    ( 3525, 63.721 )
    ( 3526, 63.971 )
    ( 3527, 64.204 )
    ( 3528, 64.459 )
    ( 3529, 64.750 )
    ( 3530, 64.983 )
    ( 3531, 65.216 )
    ( 3532, 65.449 )
    ( 3533, 65.685 )
    ( 3534, 65.918 )
    ( 3535, 66.214 )
    ( 3536, 66.449 )
    ( 3537, 66.741 )
    ( 3538, 66.974 )
    ( 3539, 67.256 )
    ( 3540, 67.607 )
    ( 3541, 67.912 )
    ( 3542, 68.216 )
    ( 3543, 68.511 )
    ( 3544, 68.805 )
    ( 3545, 69.101 )
    ( 3546, 69.407 )
    ( 3547, 69.631 )
    ( 3548, 69.920 )
    ( 3549, 70.179 )
    ( 3550, 70.558 )
    ( 3551, 70.921 )
    ( 3552, 71.282 )
    ( 3553, 71.502 )
    ( 3554, 71.795 )
    ( 3555, 72.061 )
    ( 3556, 72.326 )
    ( 3557, 72.646 )
    ( 3558, 72.922 )
    ( 3559, 73.305 )
    ( 3560, 73.689 )
    ( 3561, 73.955 )
    ( 3562, 74.237 )
    ( 3563, 74.515 )
    ( 3564, 74.788 )
    ( 3565, 75.045 )
    ( 3566, 75.301 )
    ( 3567, 75.556 )
    ( 3568, 75.899 )
    ( 3569, 76.154 )
    ( 3570, 76.414 )
    ( 3571, 76.671 )
    ( 3572, 77.057 )
    ( 3573, 77.330 )
    ( 3574, 77.602 )
    ( 3575, 77.801 )
    ( 3576, 77.809 )
    ( 3577, 77.812 )
    ( 3578, 77.834 )
    ( 3579, 77.807 )
    ( 3580, 77.855 )
    ( 3581, 77.905 )
    ( 3582, 77.896 )
    ( 3583, 77.909 )
    ( 3584, 77.977 )
    ( 3585, 77.962 )
    ( 3586, 77.937 )
    ( 3587, 78.166 )
    ( 3588, 78.251 )
    ( 3589, 78.224 )
    ( 3590, 78.255 )
    ( 3591, 78.305 )
    ( 3592, 78.487 )
    ( 3593, 78.609 )
    ( 3594, 78.581 )
    ( 3595, 78.630 )
    ( 3596, 78.812 )
    ( 3597, 78.968 )
    ( 3598, 79.095 )
    ( 3599, 79.131 )
    ( 3600, 79.114 )
    ( 3601, 79.095 )
    ( 3602, 79.184 )
    ( 3603, 79.156 )
    ( 3604, 79.200 )
    ( 3605, 79.365 )
    ( 3606, 79.382 )
    ( 3607, 79.479 )
    ( 3608, 79.575 )
    ( 3609, 79.673 )
    ( 3610, 79.890 )
    ( 3611, 80.113 )
    ( 3612, 80.323 )
    ( 3613, 80.625 )
    ( 3614, 80.886 )
    ( 3615, 81.046 )
    ( 3616, 81.205 )
    ( 3617, 81.400 )
    ( 3618, 81.593 )
    ( 3619, 81.730 )
    ( 3620, 81.747 )
    ( 3621, 81.769 )
    ( 3622, 81.765 )
    ( 3623, 81.695 )
    ( 3624, 81.783 )
    ( 3625, 81.884 )
    ( 3626, 81.926 )
    ( 3627, 81.967 )
    ( 3628, 81.842 )
    ( 3629, 81.723 )
    ( 3630, 81.599 )
    ( 3631, 81.360 )
    ( 3632, 81.160 )
    ( 3633, 80.859 )
    ( 3634, 80.558 )
    ( 3635, 80.257 )
    ( 3636, 79.969 )
    ( 3637, 79.670 )
    ( 3638, 79.449 )
    ( 3639, 79.258 )
    ( 3640, 79.094 )
    ( 3641, 78.924 )
    ( 3642, 78.714 )
    ( 3643, 78.417 )
    ( 3644, 78.137 )
    ( 3645, 78.044 )
    ( 3646, 77.966 )
    ( 3647, 78.002 )
    ( 3648, 78.048 )
    ( 3649, 78.032 )
    ( 3650, 77.989 )
    ( 3651, 77.692 )
    ( 3652, 77.465 )
    ( 3653, 77.220 )
    ( 3654, 76.926 )
    ( 3655, 76.658 )
    ( 3656, 76.369 )
    ( 3657, 76.149 )
    ( 3658, 76.133 )
    ( 3659, 76.021 )
    ( 3660, 75.877 )
    ( 3661, 75.783 )
    ( 3662, 75.481 )
    ( 3663, 75.202 )
    ( 3664, 75.009 )
    ( 3665, 74.864 )
    ( 3666, 74.581 )
    ( 3667, 74.280 )
    ( 3668, 73.980 )
    ( 3669, 73.884 )
    ( 3670, 73.790 )
    ( 3671, 73.757 )
    ( 3672, 73.729 )
    ( 3673, 73.684 )
    ( 3674, 73.587 )
    ( 3675, 73.490 )
    ( 3676, 73.444 )
    ( 3677, 73.485 )
    ( 3678, 73.414 )
    ( 3679, 73.188 )
    ( 3680, 72.978 )
    ( 3681, 72.729 )
    ( 3682, 72.429 )
    ( 3683, 72.154 )
    ( 3684, 72.009 )
    ( 3685, 71.731 )
    ( 3686, 71.464 )
    ( 3687, 71.163 )
    ( 3688, 70.967 )
    ( 3689, 70.729 )
    ( 3690, 70.429 )
    ( 3691, 70.162 )
    ( 3692, 69.907 )
    ( 3693, 69.812 )
    ( 3694, 69.888 )
    ( 3695, 69.770 )
    ( 3696, 69.469 )
    ( 3697, 69.168 )
    ( 3698, 68.873 )
    ( 3699, 68.637 )
    ( 3700, 68.525 )
    ( 3701, 68.225 )
    ( 3702, 68.128 )
    ( 3703, 67.834 )
    ( 3704, 67.688 )
    ( 3705, 67.560 )
    ( 3706, 67.463 )
    ( 3707, 67.373 )
    ( 3708, 67.276 )
    ( 3709, 66.976 )
    ( 3710, 66.729 )
    ( 3711, 66.499 )
    ( 3712, 66.229 )
    ( 3713, 65.928 )
    ( 3714, 65.631 )
    ( 3715, 65.394 )
    ( 3716, 65.093 )
    ( 3717, 65.126 )
    ( 3718, 65.061 )
    ( 3719, 64.762 )
    ( 3720, 64.528 )
    ( 3721, 64.228 )
    ( 3722, 63.980 )
    ( 3723, 63.682 )
    ( 3724, 63.471 )
    ( 3725, 63.375 )
    ( 3726, 63.148 )
    ( 3727, 62.847 )
    ( 3728, 62.550 )
    ( 3729, 62.454 )
    ( 3730, 62.356 )
    ( 3731, 62.056 )
    ( 3732, 61.958 )
    ( 3733, 61.894 )
    ( 3734, 61.626 )
    ( 3735, 61.327 )
    ( 3736, 61.130 )
    ( 3737, 60.935 )
    ( 3738, 60.751 )
    ( 3739, 60.457 )
    ( 3740, 60.156 )
    ( 3741, 59.855 )
    ( 3742, 59.598 )
    ( 3743, 59.389 )
    ( 3744, 59.122 )
    ( 3745, 59.016 )
    ( 3746, 58.803 )
    ( 3747, 58.531 )
    ( 3748, 58.230 )
    ( 3749, 57.930 )
    ( 3750, 57.682 )
    ( 3751, 57.508 )
    ( 3752, 57.207 )
    ( 3753, 56.906 )
    ( 3754, 56.646 )
    ( 3755, 56.349 )
    ( 3756, 56.048 )
    ( 3757, 55.844 )
    ( 3758, 55.697 )
    ( 3759, 55.397 )
    ( 3760, 55.108 )
    ( 3761, 54.807 )
    ( 3762, 54.611 )
    ( 3763, 54.310 )
    ( 3764, 54.019 )
    ( 3765, 53.718 )
    ( 3766, 53.758 )
    ( 3767, 53.784 )
    ( 3768, 53.688 )
    ( 3769, 53.592 )
    ( 3770, 53.620 )
    ( 3771, 53.604 )
    ( 3772, 53.303 )
    ( 3773, 53.002 )
    ( 3774, 52.827 )
    ( 3775, 52.617 )
    ( 3776, 52.506 )
    ( 3777, 52.205 )
    ( 3778, 51.904 )
    ( 3779, 51.604 )
    ( 3780, 51.393 )
    ( 3781, 51.189 )
    ( 3782, 50.888 )
    ( 3783, 50.617 )
    ( 3784, 50.576 )
    ( 3785, 50.577 )
    ( 3786, 50.484 )
    ( 3787, 50.508 )
    ( 3788, 50.557 )
    ( 3789, 50.460 )
    ( 3790, 50.484 )
    ( 3791, 50.207 )
    ( 3792, 49.936 )
    ( 3793, 49.730 )
    ( 3794, 49.522 )
    ( 3795, 49.359 )
    ( 3796, 49.058 )
    ( 3797, 48.862 )
    ( 3798, 48.615 )
    ( 3799, 48.314 )
    ( 3800, 48.178 )
    ( 3801, 48.046 )
    ( 3802, 47.745 )
    ( 3803, 47.649 )
    ( 3804, 47.559 )
    ( 3805, 47.510 )
    ( 3806, 47.415 )
    ( 3807, 47.318 )
    ( 3808, 47.270 )
    ( 3809, 47.124 )
    ( 3810, 47.136 )
    ( 3811, 47.039 )
    ( 3812, 46.944 )
    ( 3813, 46.849 )
    ( 3814, 46.704 )
    ( 3815, 46.481 )
    ( 3816, 46.181 )
    ( 3817, 45.954 )
    ( 3818, 45.806 )
    ( 3819, 45.758 )
    ( 3820, 45.721 )
    ( 3821, 45.641 )
    ( 3822, 45.600 )
    ( 3823, 45.333 )
    ( 3824, 45.032 )
    ( 3825, 44.731 )
    ( 3826, 44.704 )
    ( 3827, 44.625 )
    ( 3828, 44.565 )
    ( 3829, 44.419 )
    ( 3830, 44.312 )
    ( 3831, 44.141 )
    ( 3832, 43.930 )
    ( 3833, 43.634 )
    ( 3834, 43.333 )
    ( 3835, 43.194 )
    ( 3836, 42.957 )
    ( 3837, 42.869 )
    ( 3838, 42.568 )
    ( 3839, 42.684 )
    ( 3840, 42.783 )
    ( 3841, 42.885 )
    ( 3842, 43.067 )
    ( 3843, 43.185 )
    ( 3844, 43.282 )
    ( 3845, 43.396 )
    ( 3846, 43.534 )
    ( 3847, 43.646 )
    ( 3848, 43.752 )
    ( 3849, 43.950 )
    ( 3850, 44.048 )
    ( 3851, 44.211 )
    ( 3852, 44.308 )
    ( 3853, 44.451 )
    ( 3854, 44.552 )
    ( 3855, 44.715 )
    ( 3856, 44.869 )
    ( 3857, 44.966 )
    ( 3858, 45.062 )
    ( 3859, 45.160 )
    ( 3860, 45.259 )
    ( 3861, 45.414 )
    ( 3862, 45.553 )
    ( 3863, 45.712 )
    ( 3864, 45.887 )
    ( 3865, 46.064 )
    ( 3866, 46.057 )
    ( 3867, 46.081 )
    ( 3868, 46.026 )
    ( 3869, 46.035 )
    ( 3870, 46.059 )
    ( 3871, 46.034 )
    ( 3872, 46.058 )
    ( 3873, 46.120 )
    ( 3874, 46.066 )
    ( 3875, 46.008 )
    ( 3876, 45.951 )
    ( 3877, 45.937 )
    ( 3878, 46.071 )
    ( 3879, 46.058 )
    ( 3880, 46.042 )
    ( 3881, 46.035 )
    ( 3882, 45.978 )
    ( 3883, 45.949 )
    ( 3884, 45.891 )
    ( 3885, 45.768 )
    ( 3886, 45.667 )
    ( 3887, 45.710 )
    ( 3888, 45.797 )
    ( 3889, 45.840 )
    ( 3890, 45.715 )
    ( 3891, 45.593 )
    ( 3892, 45.474 )
    ( 3893, 45.349 )
    ( 3894, 45.395 )
    ( 3895, 45.569 )
    ( 3896, 45.611 )
    ( 3897, 45.676 )
    ( 3898, 45.717 )
    ( 3899, 45.955 )
    ( 3900, 46.023 )
    ( 3901, 46.066 )
    ( 3902, 46.137 )
    ( 3903, 46.179 )
    ( 3904, 46.267 )
    ( 3905, 46.358 )
    ( 3906, 46.411 )
    ( 3907, 46.464 )
    ( 3908, 46.339 )
    ( 3909, 46.237 )
    ( 3910, 46.219 )
    ( 3911, 46.095 )
    ( 3912, 46.053 )
    ( 3913, 46.000 )
    ( 3914, 45.898 )
    ( 3915, 45.773 )
    ( 3916, 45.681 )
    ( 3917, 45.556 )
    ( 3918, 45.487 )
    ( 3919, 45.366 )
    ( 3920, 45.241 )
    ( 3921, 45.447 )
    ( 3922, 45.322 )
    ( 3923, 45.197 )
    ( 3924, 45.126 )
    ( 3925, 45.073 )
    ( 3926, 45.056 )
    ( 3927, 44.958 )
    ( 3928, 44.857 )
    ( 3929, 44.838 )
    ( 3930, 44.836 )
    ( 3931, 44.779 )
    ( 3932, 44.750 )
    ( 3933, 44.714 )
    ( 3934, 44.657 )
    ( 3935, 44.599 )
    ( 3936, 44.604 )
    ( 3937, 44.784 )
    ( 3938, 44.871 )
    ( 3939, 44.886 )
    ( 3940, 44.986 )
    ( 3941, 44.986 )
    ( 3942, 44.987 )
    ( 3943, 44.987 )
    ( 3944, 45.001 )
    ( 3945, 45.038 )
    ( 3946, 45.038 )
    ( 3947, 45.038 )
    ( 3948, 45.121 )
    ( 3949, 45.250 )
    ( 3950, 45.313 )
    ( 3951, 45.416 )
    ( 3952, 45.416 )
    ( 3953, 45.421 )
    ( 3954, 45.462 )
    ( 3955, 45.498 )
    ( 3956, 45.575 )
    ( 3957, 45.638 )
    ( 3958, 45.664 )
    ( 3959, 45.712 )
    ( 3960, 45.712 )
    ( 3961, 45.713 )
    ( 3962, 45.859 )
    ( 3963, 46.030 )
    ( 3964, 46.320 )
    ( 3965, 46.520 )
    ( 3966, 46.520 )
    ( 3967, 46.667 )
    ( 3968, 46.828 )
    ( 3969, 46.829 )
    ( 3970, 46.829 )
    ( 3971, 46.829 )
    ( 3972, 46.976 )
    ( 3973, 47.146 )
    ( 3974, 47.357 )
    ( 3975, 47.357 )
    ( 3976, 47.430 )
    ( 3977, 47.505 )
    ( 3978, 47.509 )
    ( 3979, 47.509 )
    ( 3980, 47.559 )
    ( 3981, 47.559 )
    ( 3982, 47.582 )
    ( 3983, 47.612 )
    ( 3984, 47.666 )
    ( 3985, 47.676 )
    ( 3986, 47.676 )
    ( 3987, 47.725 )
    ( 3988, 47.740 )
    ( 3989, 47.899 )
    ( 3990, 48.070 )
    ( 3991, 48.228 )
    ( 3992, 48.375 )
    ( 3993, 48.404 )
    ( 3994, 48.404 )
    ( 3995, 48.412 )
    ( 3996, 48.440 )
    ( 3997, 48.506 )
    ( 3998, 48.608 )
    ( 3999, 48.719 )
    ( 4000, 48.739 )
    ( 4001, 48.750 )
    ( 4002, 48.812 )
    ( 4003, 48.874 )
    ( 4004, 48.875 )
    ( 4005, 48.898 )
    ( 4006, 48.919 )
    ( 4007, 48.941 )
    ( 4008, 48.984 )
    ( 4009, 49.021 )
    ( 4010, 49.025 )
    ( 4011, 49.025 )
    ( 4012, 49.025 )
    ( 4013, 49.042 )
    ( 4014, 49.104 )
    ( 4015, 49.205 )
    ( 4016, 49.177 )
    ( 4017, 49.210 )
    ( 4018, 49.231 )
    ( 4019, 49.191 )
    ( 4020, 49.133 )
    ( 4021, 49.075 )
    ( 4022, 49.104 )
    ( 4023, 49.126 )
    ( 4024, 49.072 )
    ( 4025, 49.016 )
    ( 4026, 48.987 )
    ( 4027, 48.960 )
    ( 4028, 48.968 )
    ( 4029, 48.910 )
    ( 4030, 48.882 )
    ( 4031, 48.869 )
    ( 4032, 48.855 )
    ( 4033, 48.904 )
    ( 4034, 48.891 )
    ( 4035, 48.884 )
    ( 4036, 48.775 )
    ( 4037, 48.653 )
    ( 4038, 48.657 )
    ( 4039, 48.532 )
    ( 4040, 48.518 )
    ( 4041, 48.443 )
    ( 4042, 48.581 )
    ( 4043, 48.708 )
    ( 4044, 48.837 )
    ( 4045, 49.024 )
    ( 4046, 49.149 )
    ( 4047, 49.274 )
    ( 4048, 49.406 )
    ( 4049, 49.533 )
    ( 4050, 49.675 )
    ( 4051, 49.802 )
    ( 4052, 49.934 )
    ( 4053, 50.059 )
    ( 4054, 50.199 )
    ( 4055, 50.436 )
    ( 4056, 50.581 )
    ( 4057, 50.760 )
    ( 4058, 50.887 )
    ( 4059, 51.012 )
    ( 4060, 51.137 )
    ( 4061, 51.328 )
    ( 4062, 51.287 )
    ( 4063, 51.395 )
    ( 4064, 51.485 )
    ( 4065, 51.527 )
    ( 4066, 51.613 )
    ( 4067, 51.488 )
    ( 4068, 51.447 )
    ( 4069, 51.356 )
    ( 4070, 51.458 )
    ( 4071, 51.526 )
    ( 4072, 51.568 )
    ( 4073, 51.610 )
    ( 4074, 51.651 )
    ( 4075, 51.703 )
    ( 4076, 51.745 )
    ( 4077, 51.620 )
    ( 4078, 51.661 )
    ( 4079, 51.536 )
    ( 4080, 51.433 )
    ( 4081, 51.309 )
    ( 4082, 51.333 )
    ( 4083, 51.208 )
    ( 4084, 50.909 )
    ( 4085, 50.608 )
    ( 4086, 50.316 )
    ( 4087, 50.016 )
    ( 4088, 50.012 )
    ( 4089, 50.048 )
    ( 4090, 50.083 )
    ( 4091, 50.106 )
    ( 4092, 50.172 )
    ( 4093, 50.114 )
    ( 4094, 50.056 )
    ( 4095, 50.012 )
    ( 4096, 49.955 )
    ( 4097, 49.904 )
    ( 4098, 49.856 )
    ( 4099, 49.836 )
    ( 4100, 49.808 )
    ( 4101, 49.755 )
    ( 4102, 49.764 )
    ( 4103, 49.809 )
    ( 4104, 49.750 )
    ( 4105, 49.837 )
    ( 4106, 49.822 )
    ( 4107, 49.785 )
    ( 4108, 49.876 )
    ( 4109, 49.841 )
    ( 4110, 49.783 )
    ( 4111, 49.586 )
    ( 4112, 49.427 )
    ( 4113, 49.126 )
    ( 4114, 48.827 )
    ( 4115, 48.591 )
    ( 4116, 48.524 )
    ( 4117, 48.377 )
    ( 4118, 48.300 )
    ( 4119, 48.276 )
    ( 4120, 48.210 )
    ( 4121, 48.145 )
    ( 4122, 48.178 )
    ( 4123, 48.149 )
    ( 4124, 48.052 )
    ( 4125, 47.891 )
    ( 4126, 47.589 )
    ( 4127, 47.328 )
    ( 4128, 47.044 )
    ( 4129, 46.749 )
    ( 4130, 46.447 )
    ( 4131, 46.148 )
    ( 4132, 46.002 )
    ( 4133, 45.702 )
    ( 4134, 45.400 )
    ( 4135, 45.100 )
    ( 4136, 44.808 )
    ( 4137, 44.524 )
    ( 4138, 44.223 )
    ( 4139, 44.279 )
    ( 4140, 44.321 )
    ( 4141, 44.257 )
    ( 4142, 44.204 )
    ( 4143, 44.401 )
    ( 4144, 44.526 )
    ( 4145, 44.651 )
    ( 4146, 44.964 )
    ( 4147, 45.089 )
    ( 4148, 45.293 )
    ( 4149, 45.461 )
    ( 4150, 45.640 )
    ( 4151, 45.825 )
    ( 4152, 46.003 )
    ( 4153, 46.170 )
    ( 4154, 46.295 )
    ( 4155, 46.504 )
    ( 4156, 46.722 )
    ( 4157, 46.924 )
    ( 4158, 46.799 )
    ( 4159, 46.674 )
    ( 4160, 46.591 )
    ( 4161, 46.490 )
    ( 4162, 46.547 )
    ( 4163, 46.630 )
    ( 4164, 46.792 )
    ( 4165, 46.906 )
    ( 4166, 46.989 )
    ( 4167, 47.031 )
    ( 4168, 47.072 )
    ( 4169, 46.979 )
    ( 4170, 46.874 )
    ( 4171, 47.058 )
    ( 4172, 47.252 )
    ( 4173, 47.130 )
    ( 4174, 47.005 )
    ( 4175, 46.936 )
    ( 4176, 46.828 )
    ( 4177, 46.733 )
    ( 4178, 46.612 )
    ( 4179, 46.576 )
    ( 4180, 46.511 )
    ( 4181, 46.397 )
    ( 4182, 46.272 )
    ( 4183, 46.230 )
    ( 4184, 46.106 )
    ( 4185, 46.065 )
    ( 4186, 45.940 )
    ( 4187, 45.821 )
    ( 4188, 45.706 )
    ( 4189, 45.721 )
    ( 4190, 45.824 )
    ( 4191, 45.865 )
    ( 4192, 45.803 )
    ( 4193, 45.678 )
    ( 4194, 45.555 )
    ( 4195, 45.448 )
    ( 4196, 45.325 )
    ( 4197, 45.201 )
    ( 4198, 45.076 )
    ( 4199, 45.113 )
    ( 4200, 45.085 )
    ( 4201, 45.058 )
    ( 4202, 45.031 )
    ( 4203, 45.122 )
    ( 4204, 45.139 )
    ( 4205, 45.263 )
    ( 4206, 45.371 )
    ( 4207, 45.466 )
    ( 4208, 45.585 )
    ( 4209, 45.781 )
    ( 4210, 45.980 )
    ( 4211, 45.979 )
    ( 4212, 46.017 )
    ( 4213, 46.013 )
    ( 4214, 46.013 )
    ( 4215, 45.711 )
    ( 4216, 45.472 )
    ( 4217, 45.180 )
    ( 4218, 44.919 )
    ( 4219, 44.658 )
    ( 4220, 44.411 )
    ( 4221, 44.265 )
    ( 4222, 44.092 )
    ( 4223, 43.896 )
    ( 4224, 43.648 )
    ( 4225, 43.369 )
    ( 4226, 43.067 )
    ( 4227, 43.041 )
    ( 4228, 42.956 )
    ( 4229, 42.913 )
    ( 4230, 42.816 )
    ( 4231, 42.544 )
    ( 4232, 42.273 )
    ( 4233, 42.324 )
    ( 4234, 42.216 )
    ( 4235, 42.021 )
    ( 4236, 41.810 )
    ( 4237, 41.647 )
    ( 4238, 41.373 )
    ( 4239, 41.099 )
    ( 4240, 40.798 )
    ( 4241, 40.570 )
    ( 4242, 40.319 )
    ( 4243, 40.246 )
    ( 4244, 40.271 )
    ( 4245, 40.175 )
    ( 4246, 39.897 )
    ( 4247, 39.597 )
    ( 4248, 39.451 )
    ( 4249, 39.149 )
    ( 4250, 38.919 )
    ( 4251, 38.618 )
    ( 4252, 38.318 )
    ( 4253, 38.239 )
    ( 4254, 38.144 )
    ( 4255, 38.065 )
    ( 4256, 37.764 )
    ( 4257, 37.622 )
    ( 4258, 37.321 )
    ( 4259, 37.054 )
    ( 4260, 36.908 )
    ( 4261, 36.704 )
    ( 4262, 36.626 )
    ( 4263, 36.392 )
    ( 4264, 36.091 )
    ( 4265, 35.790 )
    ( 4266, 35.726 )
    ( 4267, 35.536 )
    ( 4268, 35.235 )
    ( 4269, 34.935 )
    ( 4270, 34.652 )
    ( 4271, 34.352 )
    ( 4272, 34.051 )
    ( 4273, 33.803 )
    ( 4274, 33.502 )
    ( 4275, 33.228 )
    ( 4276, 33.288 )
    ( 4277, 33.261 )
    ( 4278, 33.169 )
    ( 4279, 33.074 )
    ( 4280, 32.932 )
    ( 4281, 32.839 )
    ( 4282, 32.632 )
    ( 4283, 32.365 )
    ( 4284, 32.079 )
    ( 4285, 31.791 )
    ( 4286, 31.503 )
    ( 4287, 31.202 )
    ( 4288, 30.901 )
    ( 4289, 30.600 )
    ( 4290, 30.404 )
    ( 4291, 30.276 )
    ( 4292, 30.009 )
    ( 4293, 29.742 )
    ( 4294, 29.456 )
    ( 4295, 29.155 )
    ( 4296, 29.208 )
    ( 4297, 29.257 )
    ( 4298, 29.229 )
    ( 4299, 29.201 )
    ( 4300, 29.352 )
    ( 4301, 29.539 )
    ( 4302, 29.770 )
    ( 4303, 29.905 )
    ( 4304, 30.027 )
    ( 4305, 30.155 )
    ( 4306, 30.252 )
    ( 4307, 30.349 )
    ( 4308, 30.447 )
    ( 4309, 30.670 )
    ( 4310, 30.886 )
    ( 4311, 30.985 )
    ( 4312, 31.127 )
    ( 4313, 31.228 )
    ( 4314, 31.325 )
    ( 4315, 31.422 )
    ( 4316, 31.520 )
    ( 4317, 31.637 )
    ( 4318, 31.839 )
    ( 4319, 32.035 )
    ( 4320, 32.273 )
    ( 4321, 32.475 )
    ( 4322, 32.572 )
    ( 4323, 32.756 )
    ( 4324, 32.854 )
    ( 4325, 32.951 )
    ( 4326, 33.048 )
    ( 4327, 33.225 )
    ( 4328, 33.348 )
    ( 4329, 33.256 )
    ( 4330, 33.161 )
    ( 4331, 33.059 )
    ( 4332, 32.976 )
    ( 4333, 32.868 )
    ( 4334, 32.749 )
    ( 4335, 32.634 )
    ( 4336, 32.509 )
    ( 4337, 32.384 )
    ( 4338, 32.260 )
    ( 4339, 32.139 )
    ( 4340, 32.064 )
    ( 4341, 31.958 )
    ( 4342, 31.833 )
    ( 4343, 31.708 )
    ( 4344, 31.653 )
    ( 4345, 31.474 )
    ( 4346, 31.216 )
    ( 4347, 31.063 )
    ( 4348, 30.917 )
    ( 4349, 30.616 )
    ( 4350, 30.449 )
    ( 4351, 30.148 )
    ( 4352, 29.854 )
    ( 4353, 29.690 )
    ( 4354, 29.706 )
    ( 4355, 29.609 )
    ( 4356, 29.308 )
    ( 4357, 29.007 )
    ( 4358, 28.706 )
    ( 4359, 28.846 )
    ( 4360, 29.003 )
    ( 4361, 29.087 )
    ( 4362, 29.228 )
    ( 4363, 29.251 )
    ( 4364, 29.310 )
    ( 4365, 29.366 )
    ( 4366, 29.308 )
    ( 4367, 29.250 )
    ( 4368, 29.309 )
    ( 4369, 29.414 )
    ( 4370, 29.550 )
    ( 4371, 29.676 )
    ( 4372, 29.618 )
    ( 4373, 29.521 )
    ( 4374, 29.422 )
    ( 4375, 29.297 )
    ( 4376, 29.269 )
    ( 4377, 29.423 )
    ( 4378, 29.563 )
    ( 4379, 29.858 )
    ( 4380, 30.018 )
    ( 4381, 30.161 )
    ( 4382, 30.258 )
    ( 4383, 30.557 )
    ( 4384, 30.799 )
    ( 4385, 31.041 )
    ( 4386, 31.317 )
    ( 4387, 31.603 )
    ( 4388, 31.887 )
    ( 4389, 32.157 )
    ( 4390, 32.414 )
    ( 4391, 32.655 )
    ( 4392, 32.811 )
    ( 4393, 32.900 )
    ( 4394, 32.969 )
    ( 4395, 32.974 )
    ( 4396, 32.963 )
    ( 4397, 32.905 )
    ( 4398, 32.847 )
    ( 4399, 32.847 )
    ( 4400, 32.895 )
    ( 4401, 32.897 )
    ( 4402, 32.897 )
    ( 4403, 33.029 )
    ( 4404, 33.166 )
    ( 4405, 33.301 )
    ( 4406, 33.301 )
    ( 4407, 33.416 )
    ( 4408, 33.416 )
    ( 4409, 33.418 )
    ( 4410, 33.418 )
    ( 4411, 33.438 )
    ( 4412, 33.494 )
    ( 4413, 33.494 )
    ( 4414, 33.719 )
    ( 4415, 33.961 )
    ( 4416, 34.183 )
    ( 4417, 34.406 )
    ( 4418, 34.645 )
    ( 4419, 34.973 )
    ( 4420, 35.300 )
    ( 4421, 35.569 )
    ( 4422, 35.812 )
    ( 4423, 36.062 )
    ( 4424, 36.312 )
    ( 4425, 36.585 )
    ( 4426, 36.921 )
    ( 4427, 37.154 )
    ( 4428, 37.357 )
    ( 4429, 37.559 )
    ( 4430, 37.535 )
    ( 4431, 37.602 )
    ( 4432, 37.477 )
    ( 4433, 37.403 )
    ( 4434, 37.296 )
    ( 4435, 37.222 )
    ( 4436, 37.097 )
    ( 4437, 36.972 )
    ( 4438, 36.866 )
    ( 4439, 36.748 )
    ( 4440, 36.623 )
    ( 4441, 36.502 )
    ( 4442, 36.396 )
    ( 4443, 36.271 )
    ( 4444, 36.188 )
    ( 4445, 36.098 )
    ( 4446, 35.976 )
    ( 4447, 35.854 )
    ( 4448, 35.730 )
    ( 4449, 35.711 )
    ( 4450, 35.770 )
    ( 4451, 35.884 )
    ( 4452, 35.898 )
    ( 4453, 35.860 )
    ( 4454, 35.805 )
    ( 4455, 35.747 )
    ( 4456, 35.689 )
    ( 4457, 35.631 )
    ( 4458, 35.330 )
    ( 4459, 35.052 )
    ( 4460, 34.845 )
    ( 4461, 34.750 )
    ( 4462, 34.604 )
    ( 4463, 34.332 )
    ( 4464, 34.186 )
    ( 4465, 34.089 )
    ( 4466, 34.108 )
    ( 4467, 34.047 )
    ( 4468, 34.098 )
    ( 4469, 34.133 )
    ( 4470, 34.171 )
    ( 4471, 34.075 )
    ( 4472, 34.037 )
    ( 4473, 33.770 )
    ( 4474, 33.620 )
    ( 4475, 33.318 )
    ( 4476, 33.089 )
    ( 4477, 32.911 )
    ( 4478, 32.663 )
    ( 4479, 32.474 )
    ( 4480, 32.192 )
    ( 4481, 31.891 )
    ( 4482, 31.757 )
    ( 4483, 31.647 )
    ( 4484, 31.523 )
    ( 4485, 31.353 )
    ( 4486, 31.184 )
    ( 4487, 30.883 )
    ( 4488, 30.582 )
    ( 4489, 30.310 )
    ( 4490, 30.042 )
    ( 4491, 29.746 )
    ( 4492, 29.445 )
    ( 4493, 29.215 )
    ( 4494, 28.938 )
    ( 4495, 28.741 )
    ( 4496, 28.595 )
    ( 4497, 28.330 )
    ( 4498, 28.062 )
    ( 4499, 27.762 )
    ( 4500, 27.471 )
    ( 4501, 27.406 )
    ( 4502, 27.132 )
    ( 4503, 27.066 )
    ( 4504, 27.023 )
    ( 4505, 26.722 )
    ( 4506, 26.448 )
    ( 4507, 26.302 )
    ( 4508, 26.206 )
    ( 4509, 26.170 )
    ( 4510, 25.897 )
    ( 4511, 25.625 )
    ( 4512, 25.333 )
    ( 4513, 25.165 )
    ( 4514, 24.898 )
    ( 4515, 24.598 )
    ( 4516, 24.313 )
    ( 4517, 24.276 )
    ( 4518, 24.212 )
    ( 4519, 24.209 )
    ( 4520, 24.189 )
    ( 4521, 24.141 )
    ( 4522, 24.048 )
    ( 4523, 23.751 )
    ( 4524, 23.450 )
    ( 4525, 23.410 )
    ( 4526, 23.313 )
    ( 4527, 23.125 )
    ( 4528, 22.842 )
    ( 4529, 22.541 )
    ( 4530, 22.241 )
    ( 4531, 22.053 )
    ( 4532, 21.766 )
    ( 4533, 21.477 )
    ( 4534, 21.285 )
    ( 4535, 21.141 )
    ( 4536, 20.995 )
    ( 4537, 20.694 )
    ( 4538, 20.397 )
    ( 4539, 20.096 )
    ( 4540, 19.794 )
    ( 4541, 19.496 )
    ( 4542, 19.195 )
    ( 4543, 19.437 )
    ( 4544, 19.634 )
    ( 4545, 19.795 )
    ( 4546, 20.015 )
    ( 4547, 20.059 )
    ( 4548, 20.159 )
    ( 4549, 20.172 )
    ( 4550, 20.178 )
    ( 4551, 20.178 )
    ( 4552, 20.410 )
    ( 4553, 20.708 )
    ( 4554, 21.007 )
    ( 4555, 21.229 )
    ( 4556, 21.463 )
    ( 4557, 21.769 )
    ( 4558, 22.057 )
    ( 4559, 22.420 )
    ( 4560, 22.437 )
    ( 4561, 22.437 )
    ( 4562, 22.437 )
    ( 4563, 22.664 )
    ( 4564, 22.886 )
    ( 4565, 23.228 )
    ( 4566, 23.656 )
    ( 4567, 24.021 )
    ( 4568, 24.247 )
    ( 4569, 24.547 )
    ( 4570, 24.824 )
    ( 4571, 25.152 )
    ( 4572, 25.449 )
    ( 4573, 25.727 )
    ( 4574, 26.039 )
    ( 4575, 26.315 )
    ( 4576, 26.339 )
    ( 4577, 26.354 )
    ( 4578, 26.527 )
    ( 4579, 26.610 )
    ( 4580, 26.677 )
    ( 4581, 26.672 )
    ( 4582, 26.817 )
    ( 4583, 26.878 )
    ( 4584, 26.894 )
    ( 4585, 26.836 )
    ( 4586, 26.790 )
    ( 4587, 26.848 )
    ( 4588, 26.861 )
    ( 4589, 26.804 )
    ( 4590, 26.790 )
    ( 4591, 26.665 )
    ( 4592, 26.377 )
    ( 4593, 26.231 )
    ( 4594, 25.970 )
    ( 4595, 25.752 )
    ( 4596, 25.451 )
    ( 4597, 25.567 )
    ( 4598, 25.668 )
    ( 4599, 25.782 )
    ( 4600, 25.880 )
    ( 4601, 25.977 )
    ( 4602, 26.099 )
    ( 4603, 26.003 )
    ( 4604, 25.765 )
    ( 4605, 25.464 )
    ( 4606, 25.179 )
    ( 4607, 24.890 )
    ( 4608, 24.799 )
    ( 4609, 24.708 )
    ( 4610, 24.407 )
    ( 4611, 24.106 )
    ( 4612, 23.805 )
    ( 4613, 23.669 )
    ( 4614, 23.368 )
    ( 4615, 23.310 )
    ( 4616, 23.185 )
    ( 4617, 23.060 )
    ( 4618, 22.939 )
    ( 4619, 22.864 )
    ( 4620, 22.790 )
    ( 4621, 22.915 )
    ( 4622, 22.956 )
    ( 4623, 22.843 )
    ( 4624, 22.829 )
    ( 4625, 22.535 )
    ( 4626, 22.237 )
    ( 4627, 21.936 )
    ( 4628, 21.875 )
    ( 4629, 21.602 )
    ( 4630, 21.530 )
    ( 4631, 21.474 )
    ( 4632, 21.498 )
    ( 4633, 21.436 )
    ( 4634, 21.318 )
    ( 4635, 21.019 )
    ( 4636, 20.860 )
    ( 4637, 20.649 )
    ( 4638, 20.348 )
    ( 4639, 20.449 )
    ( 4640, 20.517 )
    ( 4641, 20.680 )
    ( 4642, 20.843 )
    ( 4643, 20.979 )
    ( 4644, 21.078 )
    ( 4645, 21.246 )
    ( 4646, 21.346 )
    ( 4647, 21.444 )
    ( 4648, 21.557 )
    ( 4649, 21.671 )
    ( 4650, 21.940 )
    ( 4651, 22.045 )
    ( 4652, 22.142 )
    ( 4653, 22.241 )
    ( 4654, 22.338 )
    ( 4655, 22.443 )
    ( 4656, 22.550 )
    ( 4657, 22.647 )
    ( 4658, 22.749 )
    ( 4659, 22.871 )
    ( 4660, 22.969 )
    ( 4661, 23.091 )
    ( 4662, 23.208 )
    ( 4663, 23.323 )
    ( 4664, 23.453 )
    ( 4665, 23.575 )
    ( 4666, 23.697 )
    ( 4667, 23.844 )
    ( 4668, 23.795 )
    ( 4669, 23.791 )
    ( 4670, 23.763 )
    ( 4671, 23.709 )
    ( 4672, 23.652 )
    ( 4673, 23.597 )
    ( 4674, 23.581 )
    ( 4675, 23.667 )
    ( 4676, 23.740 )
    ( 4677, 23.798 )
    ( 4678, 23.746 )
    ( 4679, 23.688 )
    ( 4680, 23.713 )
    ( 4681, 23.699 )
    ( 4682, 23.398 )
    ( 4683, 23.214 )
    ( 4684, 22.920 )
    ( 4685, 22.640 )
    ( 4686, 22.574 )
    ( 4687, 22.531 )
    ( 4688, 22.441 )
    ( 4689, 22.140 )
    ( 4690, 22.000 )
    ( 4691, 21.804 )
    ( 4692, 21.540 )
    ( 4693, 21.443 )
    ( 4694, 21.358 )
    ( 4695, 21.133 )
    ( 4696, 20.865 )
    ( 4697, 20.564 )
    ( 4698, 20.267 )
    ( 4699, 20.044 )
    ( 4700, 19.774 )
    ( 4701, 19.511 )
    ( 4702, 19.281 )
    ( 4703, 19.146 )
    ( 4704, 18.845 )
    ( 4705, 18.718 )
    ( 4706, 18.417 )
    ( 4707, 18.116 )
    ( 4708, 17.927 )
    ( 4709, 17.626 )
    ( 4710, 17.678 )
    ( 4711, 17.404 )
    ( 4712, 17.143 )
    ( 4713, 16.895 )
    ( 4714, 16.594 )
    ( 4715, 16.295 )
    ( 4716, 15.994 )
    ( 4717, 15.693 )
    ( 4718, 15.408 )
    ( 4719, 15.116 )
    ( 4720, 14.906 )
    ( 4721, 14.606 )
    ( 4722, 14.357 )
    ( 4723, 14.150 )
    ( 4724, 14.168 )
    ( 4725, 13.972 )
    ( 4726, 13.674 )
    ( 4727, 13.608 )
    ( 4728, 13.349 )
    ( 4729, 13.254 )
    ( 4730, 13.157 )
    ( 4731, 13.031 )
    ( 4732, 12.820 )
    ( 4733, 12.546 )
    ( 4734, 12.325 )
    ( 4735, 12.024 )
    ( 4736, 11.723 )
    ( 4737, 11.666 )
    ( 4738, 11.573 )
    ( 4739, 11.272 )
    ( 4740, 11.273 )
    ( 4741, 11.266 )
    ( 4742, 11.474 )
    ( 4743, 11.516 )
    ( 4744, 11.553 )
    ( 4745, 11.598 )
    ( 4746, 11.587 )
    ( 4747, 11.715 )
    ( 4748, 11.757 )
    ( 4749, 11.633 )
    ( 4750, 11.580 )
    ( 4751, 11.532 )
    ( 4752, 11.407 )
    ( 4753, 11.463 )
    ( 4754, 11.466 )
    ( 4755, 11.481 )
    ( 4756, 11.483 )
    ( 4757, 11.416 )
    ( 4758, 11.323 )
    ( 4759, 11.209 )
    ( 4760, 11.091 )
    ( 4761, 10.967 )
    ( 4762, 10.978 )
    ( 4763, 11.008 )
    ( 4764, 10.957 )
    ( 4765, 10.882 )
    ( 4766, 10.831 )
    ( 4767, 10.963 )
    ( 4768, 11.088 )
    ( 4769, 11.021 )
    ( 4770, 10.984 )
    ( 4771, 11.026 )
    ( 4772, 10.908 )
    ( 4773, 11.056 )
    ( 4774, 10.931 )
    ( 4775, 10.867 )
    ( 4776, 10.801 )
    ( 4777, 10.724 )
    ( 4778, 10.682 )
    ( 4779, 10.618 )
    ( 4780, 10.521 )
    ( 4781, 10.325 )
    ( 4782, 10.024 )
    ( 4783, 10.125 )
    ( 4784, 9.9784 )
    ( 4785, 9.8324 )
    ( 4786, 9.5754 )
    ( 4787, 9.5848 )
    ( 4788, 9.4694 )
    ( 4789, 9.5850 )
    ( 4790, 9.4601 )
    ( 4791, 9.4265 )
    ( 4792, 9.3016 )
    ( 4793, 9.2994 )
    ( 4794, 9.3472 )
    ( 4795, 9.3191 )
    ( 4796, 9.1984 )
    ( 4797, 9.0870 )
    ( 4798, 8.9945 )
    ( 4799, 8.8986 )
    ( 4800, 8.8453 )
    ( 4801, 9.0569 )
    ( 4802, 9.1819 )
    ( 4803, 9.3068 )
    ( 4804, 9.5840 )
    ( 4805, 9.7681 )
    ( 4806, 9.6454 )
    ( 4807, 9.6547 )
    ( 4808, 9.6268 )
    ( 4809, 9.7429 )
    ( 4810, 9.8120 )
    ( 4811, 9.9794 )
    ( 4812, 10.023 )
    ( 4813, 9.8979 )
    ( 4814, 9.8013 )
    ( 4815, 9.6287 )
    ( 4816, 9.3276 )
    ( 4817, 9.3206 )
    ( 4818, 9.1958 )
    ( 4819, 9.4457 )
    ( 4820, 9.7401 )
    ( 4821, 10.016 )
    ( 4822, 10.296 )
    ( 4823, 10.526 )
    ( 4824, 10.717 )
    ( 4825, 10.917 )
    ( 4826, 11.093 )
    ( 4827, 11.372 )
    ( 4828, 11.633 )
    ( 4829, 11.867 )
    ( 4830, 12.123 )
    ( 4831, 12.388 )
    ( 4832, 12.455 )
    ( 4833, 12.455 )
    ( 4834, 12.499 )
    ( 4835, 12.499 )
    ( 4836, 12.499 )
    ( 4837, 12.501 )
    ( 4838, 12.685 )
    ( 4839, 12.831 )
    ( 4840, 13.013 )
    ( 4841, 13.159 )
    ( 4842, 13.415 )
    ( 4843, 13.566 )
    ( 4844, 13.780 )
    ( 4845, 13.942 )
    ( 4846, 13.942 )
    ( 4847, 14.148 )
    ( 4848, 14.412 )
    ( 4849, 14.582 )
    ( 4850, 14.728 )
    ( 4851, 14.816 )
    ( 4852, 14.945 )
    ( 4853, 15.012 )
    ( 4854, 15.012 )
    ( 4855, 15.089 )
    ( 4856, 15.152 )
    ( 4857, 15.259 )
    ( 4858, 15.276 )
    ( 4859, 15.315 )
    ( 4860, 15.315 )
    ( 4861, 15.323 )
    ( 4862, 15.326 )
    ( 4863, 15.336 )
    ( 4864, 15.380 )
    ( 4865, 15.528 )
    ( 4866, 15.579 )
    ( 4867, 15.692 )
    ( 4868, 15.815 )
    ( 4869, 15.821 )
    ( 4870, 15.839 )
    ( 4871, 15.911 )
    ( 4872, 15.959 )
    ( 4873, 15.971 )
    ( 4874, 15.971 )
    ( 4875, 15.971 )
    ( 4876, 16.168 )
    ( 4877, 16.168 )
    ( 4878, 16.189 )
    ( 4879, 16.189 )
    ( 4880, 16.336 )
    ( 4881, 16.360 )
    ( 4882, 16.360 )
    ( 4883, 16.507 )
    ( 4884, 16.517 )
    ( 4885, 16.523 )
    ( 4886, 16.523 )
    ( 4887, 16.524 )
    ( 4888, 16.768 )
    ( 4889, 16.990 )
    ( 4890, 17.216 )
    ( 4891, 17.538 )
    ( 4892, 17.774 )
    ( 4893, 17.996 )
    ( 4894, 18.218 )
    ( 4895, 18.453 )
    ( 4896, 18.684 )
    ( 4897, 18.938 )
    ( 4898, 19.161 )
    ( 4899, 19.464 )
    ( 4900, 19.696 )
    ( 4901, 19.884 )
    ( 4902, 19.951 )
    ( 4903, 20.159 )
    ( 4904, 20.393 )
    ( 4905, 20.626 )
    ( 4906, 20.810 )
    ( 4907, 20.935 )
    ( 4908, 21.024 )
    ( 4909, 20.974 )
    ( 4910, 20.860 )
    ( 4911, 20.739 )
    ( 4912, 20.614 )
    ( 4913, 20.748 )
    ( 4914, 20.649 )
    ( 4915, 20.604 )
    ( 4916, 20.845 )
    ( 4917, 21.046 )
    ( 4918, 21.250 )
    ( 4919, 21.375 )
    ( 4920, 21.500 )
    ( 4921, 21.638 )
    ( 4922, 21.764 )
    ( 4923, 21.921 )
    ( 4924, 22.046 )
    ( 4925, 22.332 )
    ( 4926, 22.600 )
    ( 4927, 22.732 )
    ( 4928, 22.948 )
    ( 4929, 23.073 )
    ( 4930, 23.351 )
    ( 4931, 23.606 )
    ( 4932, 23.958 )
    ( 4933, 24.235 )
    ( 4934, 24.430 )
    ( 4935, 24.612 )
    ( 4936, 24.753 )
    ( 4937, 24.878 )
    ( 4938, 25.003 )
    ( 4939, 24.911 )
    ( 4940, 24.976 )
    ( 4941, 25.017 )
    ( 4942, 25.059 )
    ( 4943, 24.953 )
    ( 4944, 24.929 )
    ( 4945, 24.804 )
    ( 4946, 24.686 )
    ( 4947, 24.561 )
    ( 4948, 24.460 )
    ( 4949, 24.535 )
    ( 4950, 24.632 )
    ( 4951, 24.738 )
    ( 4952, 24.874 )
    ( 4953, 25.097 )
    ( 4954, 25.194 )
    ( 4955, 25.249 )
    ( 4956, 25.124 )
    ( 4957, 25.001 )
    ( 4958, 24.883 )
    ( 4959, 24.758 )
    ( 4960, 24.645 )
    ( 4961, 24.555 )
    ( 4962, 24.430 )
    ( 4963, 24.347 )
    ( 4964, 24.283 )
    ( 4965, 24.158 )
    ( 4966, 24.033 )
    ( 4967, 24.236 )
    ( 4968, 24.440 )
    ( 4969, 24.601 )
    ( 4970, 24.906 )
    ( 4971, 25.257 )
    ( 4972, 25.465 )
    ( 4973, 25.673 )
    ( 4974, 25.897 )
    ( 4975, 26.207 )
    ( 4976, 26.515 )
    ( 4977, 26.713 )
    ( 4978, 26.938 )
    ( 4979, 27.205 )
    ( 4980, 27.331 )
    ( 4981, 27.586 )
    ( 4982, 27.841 )
    ( 4983, 28.098 )
    ( 4984, 28.356 )
    ( 4985, 28.616 )
    ( 4986, 28.740 )
    ( 4987, 28.930 )
    ( 4988, 29.123 )
    ( 4989, 29.379 )
    ( 4990, 29.635 )
    ( 4991, 29.893 )
    ( 4992, 30.177 )
    ( 4993, 30.451 )
    ( 4994, 30.727 )
    ( 4995, 30.877 )
    ( 4996, 31.002 )
    ( 4997, 31.137 )
    ( 4998, 31.262 )
    ( 4999, 31.429 )
    ( 5000, 31.555 )
    ( 5001, 31.690 )
    ( 5002, 31.823 )
    ( 5003, 31.955 )
    ( 5004, 32.084 )
    ( 5005, 32.209 )
    ( 5006, 32.337 )
    ( 5007, 32.380 )
    ( 5008, 32.448 )
    ( 5009, 32.519 )
    ( 5010, 32.421 )
    ( 5011, 32.309 )
    ( 5012, 32.197 )
    ( 5013, 32.162 )
    ( 5014, 32.156 )
    ( 5015, 32.151 )
    ( 5016, 32.093 )
    ( 5017, 31.797 )
    ( 5018, 31.504 )
    ( 5019, 31.478 )
    ( 5020, 31.381 )
    ( 5021, 31.369 )
    ( 5022, 31.068 )
    ( 5023, 30.920 )
    ( 5024, 30.823 )
    ( 5025, 30.535 )
    ( 5026, 30.261 )
    ( 5027, 29.960 )
    ( 5028, 29.660 )
    ( 5029, 29.388 )
    ( 5030, 29.183 )
    ( 5031, 28.882 )
    ( 5032, 28.615 )
    ( 5033, 28.331 )
    ( 5034, 28.234 )
    ( 5035, 28.035 )
    ( 5036, 27.735 )
    ( 5037, 27.493 )
    ( 5038, 27.192 )
    ( 5039, 26.936 )
    ( 5040, 26.635 )
    ( 5041, 26.405 )
    ( 5042, 26.280 )
    ( 5043, 25.979 )
    ( 5044, 25.707 )
    ( 5045, 25.406 )
    ( 5046, 25.309 )
    ( 5047, 25.431 )
    ( 5048, 25.365 )
    ( 5049, 25.388 )
    ( 5050, 25.291 )
    ( 5051, 25.145 )
    ( 5052, 24.861 )
    ( 5053, 24.571 )
    ( 5054, 24.360 )
    ( 5055, 24.063 )
    ( 5056, 23.987 )
    ( 5057, 23.920 )
    ( 5058, 23.823 )
    ( 5059, 23.825 )
    ( 5060, 23.571 )
    ( 5061, 23.504 )
    ( 5062, 23.205 )
    ( 5063, 23.108 )
    ( 5064, 22.912 )
    ( 5065, 22.838 )
    ( 5066, 22.741 )
    ( 5067, 22.677 )
    ( 5068, 22.376 )
    ( 5069, 22.280 )
    ( 5070, 21.979 )
    ( 5071, 21.887 )
    ( 5072, 21.813 )
    ( 5073, 21.611 )
    ( 5074, 21.311 )
    ( 5075, 21.293 )
    ( 5076, 21.200 )
    ( 5077, 21.187 )
    ( 5078, 21.200 )
    ( 5079, 21.073 )
    ( 5080, 20.945 )
    ( 5081, 20.644 )
    ( 5082, 20.501 )
    ( 5083, 20.359 )
    ( 5084, 20.265 )
    ( 5085, 19.973 )
    ( 5086, 19.777 )
    ( 5087, 19.535 )
    ( 5088, 19.235 )
    ( 5089, 18.968 )
    ( 5090, 18.772 )
    ( 5091, 18.475 )
    ( 5092, 18.174 )
    ( 5093, 17.890 )
    ( 5094, 17.589 )
    ( 5095, 17.288 )
    ( 5096, 17.010 )
    ( 5097, 16.714 )
    ( 5098, 16.515 )
    ( 5099, 16.319 )
    ( 5100, 16.022 )
    ( 5101, 15.729 )
    ( 5102, 15.649 )
    ( 5103, 15.552 )
    ( 5104, 15.251 )
    ( 5105, 15.269 )
    ( 5106, 15.168 )
    ( 5107, 15.043 )
    ( 5108, 15.071 )
    ( 5109, 15.008 )
    ( 5110, 14.736 )
    ( 5111, 14.475 )
    ( 5112, 14.174 )
    ( 5113, 14.170 )
    ( 5114, 13.869 )
    ( 5115, 13.808 )
    ( 5116, 13.507 )
    ( 5117, 13.397 )
    ( 5118, 13.272 )
    ( 5119, 13.196 )
    ( 5120, 13.220 )
    ( 5121, 12.926 )
    ( 5122, 12.650 )
    ( 5123, 12.349 )
    ( 5124, 12.169 )
    ( 5125, 11.878 )
    ( 5126, 11.609 )
    ( 5127, 11.489 )
    ( 5128, 11.278 )
    ( 5129, 11.272 )
    ( 5130, 10.971 )
    ( 5131, 10.825 )
    ( 5132, 10.524 )
    ( 5133, 10.224 )
    ( 5134, 9.9894 )
    ( 5135, 10.287 )
    ( 5136, 10.552 )
    ( 5137, 10.823 )
    ( 5138, 10.809 )
    ( 5139, 10.807 )
    ( 5140, 10.817 )
    ( 5141, 10.973 )
    ( 5142, 10.947 )
    ( 5143, 11.055 )
    ( 5144, 11.156 )
    ( 5145, 11.214 )
    ( 5146, 11.457 )
    ( 5147, 11.726 )
    ( 5148, 11.927 )
    ( 5149, 12.144 )
    ( 5150, 12.321 )
    ( 5151, 12.520 )
    ( 5152, 12.801 )
    ( 5153, 12.977 )
    ( 5154, 13.190 )
    ( 5155, 13.381 )
    ( 5156, 13.568 )
    ( 5157, 13.754 )
    ( 5158, 13.958 )
    ( 5159, 14.135 )
    ( 5160, 14.311 )
    ( 5161, 14.492 )
    ( 5162, 14.672 )
    ( 5163, 14.956 )
    ( 5164, 15.224 )
    ( 5165, 15.549 )
    ( 5166, 15.808 )
    ( 5167, 15.984 )
    ( 5168, 16.231 )
    ( 5169, 16.452 )
    ( 5170, 16.671 )
    ( 5171, 16.902 )
    ( 5172, 17.145 )
    ( 5173, 17.366 )
    ( 5174, 17.715 )
    ( 5175, 18.057 )
    ( 5176, 18.328 )
    ( 5177, 18.027 )
    ( 5178, 17.735 )
    ( 5179, 17.539 )
    ( 5180, 17.352 )
    ( 5181, 17.324 )
    ( 5182, 17.023 )
    ( 5183, 16.879 )
    ( 5184, 16.578 )
    ( 5185, 16.308 )
    ( 5186, 16.078 )
    ( 5187, 15.819 )
    ( 5188, 15.689 )
    ( 5189, 15.664 )
    ( 5190, 15.607 )
    ( 5191, 15.461 )
    ( 5192, 15.289 )
    ( 5193, 14.988 )
    ( 5194, 14.863 )
    ( 5195, 14.701 )
    ( 5196, 14.564 )
    ( 5197, 14.367 )
    ( 5198, 14.067 )
    ( 5199, 13.766 )
    ( 5200, 13.663 )
    ( 5201, 13.432 )
    ( 5202, 13.132 )
    ( 5203, 13.029 )
    ( 5204, 12.845 )
    ( 5205, 12.544 )
    ( 5206, 12.243 )
    ( 5207, 11.954 )
    ( 5208, 11.809 )
    ( 5209, 11.834 )
    ( 5210, 11.577 )
    ( 5211, 11.276 )
    ( 5212, 11.132 )
    ( 5213, 11.059 )
    ( 5214, 11.090 )
    ( 5215, 10.814 )
    ( 5216, 10.521 )
    ( 5217, 10.220 )
    ( 5218, 10.154 )
    ( 5219, 10.240 )
    ( 5220, 10.366 )
    ( 5221, 10.398 )
    ( 5222, 10.371 )
    ( 5223, 10.401 )
    ( 5224, 10.420 )
    ( 5225, 10.393 )
    ( 5226, 10.351 )
    ( 5227, 10.228 )
    ( 5228, 10.154 )
    ( 5229, 10.311 )
    ( 5230, 10.467 )
    ( 5231, 10.592 )
    ( 5232, 10.523 )
    ( 5233, 10.465 )
    ( 5234, 10.164 )
    ( 5235, 10.033 )
    ( 5236, 9.7589 )
    ( 5237, 9.6472 )
    ( 5238, 9.3774 )
    ( 5239, 9.0953 )
    ( 5240, 8.8000 )
    ( 5241, 8.5518 )
    ( 5242, 8.2639 )
    ( 5243, 8.0848 )
    ( 5244, 7.9363 )
    ( 5245, 7.7137 )
    ( 5246, 7.6976 )
    ( 5247, 7.4602 )
    ( 5248, 7.1772 )
    ( 5249, 6.9878 )
    ( 5250, 6.9904 )
    ( 5251, 7.0237 )
    ( 5252, 6.8776 )
    ( 5253, 6.6127 )
    ( 5254, 6.3146 )
    ( 5255, 6.0135 )
    ( 5256, 6.2350 )
    ( 5257, 6.2609 )
    ( 5258, 6.2823 )
    ( 5259, 6.5587 )
    ( 5260, 6.8340 )
    ( 5261, 7.0231 )
    ( 5262, 7.3524 )
    ( 5263, 7.4277 )
    ( 5264, 7.6553 )
    ( 5265, 7.9654 )
    ( 5266, 8.2197 )
    ( 5267, 8.4269 )
    ( 5268, 8.5637 )
    ( 5269, 8.5796 )
    ( 5270, 8.5900 )
    ( 5271, 8.5908 )
    ( 5272, 8.5908 )
    ( 5273, 8.7438 )
    ( 5274, 8.8827 )
    ( 5275, 8.9498 )
    ( 5276, 9.0389 )
    ( 5277, 9.1990 )
    ( 5278, 9.4039 )
    ( 5279, 9.6987 )
    ( 5280, 9.7744 )
    ( 5281, 9.8693 )
    ( 5282, 9.9937 )
    ( 5283, 10.066 )
    ( 5284, 10.138 )
    ( 5285, 10.378 )
    ( 5286, 10.582 )
    ( 5287, 10.846 )
    ( 5288, 11.134 )
    ( 5289, 11.303 )
    ( 5290, 11.407 )
    ( 5291, 11.514 )
    ( 5292, 11.589 )
    ( 5293, 11.709 )
    ( 5294, 11.776 )
    ( 5295, 11.927 )
    ( 5296, 12.096 )
    ( 5297, 12.335 )
    ( 5298, 12.623 )
    ( 5299, 12.880 )
    ( 5300, 13.069 )
    ( 5301, 13.255 )
    ( 5302, 13.380 )
    ( 5303, 13.505 )
    ( 5304, 13.635 )
    ( 5305, 13.894 )
    ( 5306, 14.172 )
    ( 5307, 14.316 )
    ( 5308, 14.383 )
    ( 5309, 14.477 )
    ( 5310, 14.740 )
    ( 5311, 14.999 )
    ( 5312, 15.297 )
    ( 5313, 15.596 )
    ( 5314, 15.900 )
    ( 5315, 16.230 )
    ( 5316, 16.539 )
    ( 5317, 16.789 )
    ( 5318, 17.113 )
    ( 5319, 17.448 )
    ( 5320, 17.704 )
    ( 5321, 17.937 )
    ( 5322, 18.221 )
    ( 5323, 18.397 )
    ( 5324, 18.789 )
    ( 5325, 19.090 )
    ( 5326, 19.391 )
    ( 5327, 19.886 )
    ( 5328, 20.234 )
    ( 5329, 20.541 )
    ( 5330, 20.842 )
    ( 5331, 21.144 )
    ( 5332, 21.446 )
    ( 5333, 21.747 )
    ( 5334, 22.049 )
    ( 5335, 22.391 )
    ( 5336, 22.694 )
    ( 5337, 22.996 )
    ( 5338, 23.320 )
    ( 5339, 23.625 )
    ( 5340, 23.961 )
    ( 5341, 24.263 )
    ( 5342, 24.564 )
    ( 5343, 24.865 )
    ( 5344, 25.177 )
    ( 5345, 25.526 )
    ( 5346, 25.852 )
    ( 5347, 26.251 )
    ( 5348, 26.623 )
    ( 5349, 26.893 )
    ( 5350, 27.121 )
    ( 5351, 27.322 )
    ( 5352, 27.586 )
    ( 5353, 27.766 )
    ( 5354, 28.016 )
    ( 5355, 28.201 )
    ( 5356, 28.523 )
    ( 5357, 28.844 )
    ( 5358, 29.182 )
    ( 5359, 29.437 )
    ( 5360, 29.739 )
    ( 5361, 30.015 )
    ( 5362, 30.378 )
    ( 5363, 30.740 )
    ( 5364, 31.073 )
    ( 5365, 31.371 )
    ( 5366, 31.379 )
    ( 5367, 31.379 )
    ( 5368, 31.380 )
    ( 5369, 31.380 )
    ( 5370, 31.380 )
    ( 5371, 31.453 )
    ( 5372, 31.470 )
    ( 5373, 31.658 )
    ( 5374, 31.730 )
    ( 5375, 31.731 )
    ( 5376, 31.470 )
    ( 5377, 31.180 )
    ( 5378, 30.879 )
    ( 5379, 30.578 )
    ( 5380, 30.664 )
    ( 5381, 30.606 )
    ( 5382, 30.498 )
    ( 5383, 30.412 )
    ( 5384, 30.321 )
    ( 5385, 30.202 )
    ( 5386, 30.077 )
    ( 5387, 29.953 )
    ( 5388, 29.837 )
    ( 5389, 29.716 )
    ( 5390, 29.591 )
    ( 5391, 29.516 )
    ( 5392, 29.700 )
    ( 5393, 29.875 )
    ( 5394, 30.042 )
    ( 5395, 30.167 )
    ( 5396, 30.513 )
    ( 5397, 30.817 )
    ( 5398, 31.085 )
    ( 5399, 31.341 )
    ( 5400, 31.618 )
    ( 5401, 31.873 )
    ( 5402, 32.183 )
    ( 5403, 32.311 )
    ( 5404, 32.470 )
    ( 5405, 32.595 )
    ( 5406, 32.782 )
    ( 5407, 32.657 )
    ( 5408, 32.553 )
    ( 5409, 32.428 )
    ( 5410, 32.338 )
    ( 5411, 32.306 )
    ( 5412, 32.191 )
    ( 5413, 32.144 )
    ( 5414, 32.185 )
    ( 5415, 32.060 )
    ( 5416, 32.196 )
    ( 5417, 32.080 )
    ( 5418, 31.956 )
    ( 5419, 31.831 )
    ( 5420, 32.103 )
    ( 5421, 32.076 )
    ( 5422, 32.048 )
    ( 5423, 31.907 )
    ( 5424, 31.762 )
    ( 5425, 31.461 )
    ( 5426, 31.161 )
    ( 5427, 30.861 )
    ( 5428, 30.561 )
    ( 5429, 30.330 )
    ( 5430, 30.029 )
    ( 5431, 29.883 )
    ( 5432, 29.742 )
    ( 5433, 29.443 )
    ( 5434, 29.220 )
    ( 5435, 29.078 )
    ( 5436, 28.852 )
    ( 5437, 28.595 )
    ( 5438, 28.314 )
    ( 5439, 28.014 )
    ( 5440, 27.820 )
    ( 5441, 27.519 )
    ( 5442, 27.218 )
    ( 5443, 27.037 )
    ( 5444, 26.738 )
    ( 5445, 26.762 )
    ( 5446, 26.673 )
    ( 5447, 26.599 )
    ( 5448, 26.480 )
    ( 5449, 26.428 )
    ( 5450, 26.331 )
    ( 5451, 26.097 )
    ( 5452, 26.256 )
    ( 5453, 26.135 )
    ( 5454, 26.013 )
    ( 5455, 25.888 )
    ( 5456, 25.997 )
    ( 5457, 26.106 )
    ( 5458, 26.149 )
    ( 5459, 26.263 )
    ( 5460, 26.331 )
    ( 5461, 26.586 )
    ( 5462, 26.775 )
    ( 5463, 27.017 )
    ( 5464, 27.284 )
    ( 5465, 27.563 )
    ( 5466, 27.808 )
    ( 5467, 28.178 )
    ( 5468, 28.513 )
    ( 5469, 28.843 )
    ( 5470, 29.208 )
    ( 5471, 29.392 )
    ( 5472, 29.681 )
    ( 5473, 29.936 )
    ( 5474, 30.125 )
    ( 5475, 30.250 )
    ( 5476, 30.430 )
    ( 5477, 30.610 )
    ( 5478, 30.580 )
    ( 5479, 30.581 )
    ( 5480, 30.483 )
    ( 5481, 30.728 )
    ( 5482, 30.912 )
    ( 5483, 31.126 )
    ( 5484, 31.318 )
    ( 5485, 31.555 )
    ( 5486, 31.788 )
    ( 5487, 31.987 )
    ( 5488, 32.207 )
    ( 5489, 32.438 )
    ( 5490, 32.646 )
    ( 5491, 32.856 )
    ( 5492, 32.981 )
    ( 5493, 33.221 )
    ( 5494, 33.498 )
    ( 5495, 33.753 )
    ( 5496, 33.930 )
    ( 5497, 34.098 )
    ( 5498, 34.248 )
    ( 5499, 34.432 )
    ( 5500, 34.640 )
    ( 5501, 34.765 )
    ( 5502, 34.899 )
    ( 5503, 35.041 )
    ( 5504, 35.229 )
    ( 5505, 35.455 )
    ( 5506, 35.580 )
    ( 5507, 35.835 )
    ( 5508, 35.984 )
    ( 5509, 36.109 )
    ( 5510, 36.313 )
    ( 5511, 36.447 )
    ( 5512, 36.574 )
    ( 5513, 36.501 )
    ( 5514, 36.391 )
    ( 5515, 36.278 )
    ( 5516, 36.234 )
    ( 5517, 36.139 )
    ( 5518, 36.268 )
    ( 5519, 36.373 )
    ( 5520, 36.416 )
    ( 5521, 36.292 )
    ( 5522, 36.334 )
    ( 5523, 36.420 )
    ( 5524, 36.533 )
    ( 5525, 36.574 )
    ( 5526, 36.693 )
    ( 5527, 36.749 )
    ( 5528, 36.666 )
    ( 5529, 36.564 )
    ( 5530, 36.607 )
    ( 5531, 36.490 )
    ( 5532, 36.557 )
    ( 5533, 36.630 )
    ( 5534, 36.529 )
    ( 5535, 36.419 )
    ( 5536, 36.317 )
    ( 5537, 36.200 )
    ( 5538, 36.084 )
    ( 5539, 35.993 )
    ( 5540, 35.868 )
    ( 5541, 35.744 )
    ( 5542, 35.630 )
    ( 5543, 35.515 )
    ( 5544, 35.390 )
    ( 5545, 35.298 )
    ( 5546, 35.236 )
    ( 5547, 35.130 )
    ( 5548, 35.005 )
    ( 5549, 35.199 )
    ( 5550, 35.400 )
    ( 5551, 35.595 )
    ( 5552, 35.779 )
    ( 5553, 35.707 )
    ( 5554, 35.587 )
    ( 5555, 35.478 )
    ( 5556, 35.437 )
    ( 5557, 35.313 )
    ( 5558, 35.188 )
    ( 5559, 35.443 )
    ( 5560, 35.646 )
    ( 5561, 35.846 )
    ( 5562, 36.022 )
    ( 5563, 36.281 )
    ( 5564, 36.519 )
    ( 5565, 36.712 )
    ( 5566, 36.891 )
    ( 5567, 37.067 )
    ( 5568, 37.296 )
    ( 5569, 37.472 )
    ( 5570, 37.658 )
    ( 5571, 38.061 )
    ( 5572, 38.429 )
    ( 5573, 38.798 )
    ( 5574, 39.167 )
    ( 5575, 39.544 )
    ( 5576, 39.926 )
    ( 5577, 40.305 )
    ( 5578, 40.673 )
    ( 5579, 41.041 )
    ( 5580, 41.439 )
    ( 5581, 41.807 )
    ( 5582, 42.196 )
    ( 5583, 42.517 )
    ( 5584, 42.750 )
    ( 5585, 42.780 )
    ( 5586, 42.781 )
    ( 5587, 42.808 )
    ( 5588, 42.836 )
    ( 5589, 42.836 )
    ( 5590, 42.836 )
    ( 5591, 42.899 )
    ( 5592, 42.961 )
    ( 5593, 43.107 )
    ( 5594, 43.253 )
    ( 5595, 43.312 )
    ( 5596, 43.312 )
    ( 5597, 43.362 )
    ( 5598, 43.362 )
    ( 5599, 43.449 )
    ( 5600, 43.542 )
    ( 5601, 43.611 )
    ( 5602, 43.697 )
    ( 5603, 43.940 )
    ( 5604, 44.145 )
    ( 5605, 44.212 )
    ( 5606, 44.354 )
    ( 5607, 44.421 )
    ( 5608, 44.653 )
    ( 5609, 44.936 )
    ( 5610, 45.275 )
    ( 5611, 45.558 )
    ( 5612, 45.863 )
    ( 5613, 46.155 )
    ( 5614, 46.453 )
    ( 5615, 46.745 )
    ( 5616, 47.235 )
    ( 5617, 47.671 )
    ( 5618, 48.100 )
    ( 5619, 48.491 )
    ( 5620, 48.867 )
    ( 5621, 49.228 )
    ( 5622, 49.545 )
    ( 5623, 49.855 )
    ( 5624, 50.077 )
    ( 5625, 50.302 )
    ( 5626, 50.530 )
    ( 5627, 50.774 )
    ( 5628, 50.996 )
    ( 5629, 51.219 )
    ( 5630, 51.440 )
    ( 5631, 51.663 )
    ( 5632, 51.948 )
    ( 5633, 52.169 )
    ( 5634, 52.392 )
    ( 5635, 52.611 )
    ( 5636, 52.834 )
    ( 5637, 53.057 )
    ( 5638, 53.288 )
    ( 5639, 53.500 )
    ( 5640, 53.711 )
    ( 5641, 53.926 )
    ( 5642, 54.136 )
    ( 5643, 54.349 )
    ( 5644, 54.559 )
    ( 5645, 54.785 )
    ( 5646, 54.996 )
    ( 5647, 55.254 )
    ( 5648, 55.472 )
    ( 5649, 55.683 )
    ( 5650, 56.015 )
    ( 5651, 56.226 )
    ( 5652, 56.460 )
    ( 5653, 56.695 )
    ( 5654, 56.965 )
    ( 5655, 57.195 )
    ( 5656, 57.529 )
    ( 5657, 57.762 )
    ( 5658, 57.992 )
    ( 5659, 58.211 )
    ( 5660, 58.422 )
    ( 5661, 58.622 )
    ( 5662, 58.833 )
    ( 5663, 59.168 )
    ( 5664, 59.515 )
    ( 5665, 60.018 )
    ( 5666, 60.423 )
    ( 5667, 60.825 )
    ( 5668, 61.221 )
    ( 5669, 61.479 )
    ( 5670, 61.852 )
    ( 5671, 62.329 )
    ( 5672, 62.301 )
    ( 5673, 62.418 )
    ( 5674, 62.528 )
    ( 5675, 62.625 )
    ( 5676, 62.788 )
    ( 5677, 62.884 )
    ( 5678, 62.996 )
    ( 5679, 63.125 )
    ( 5680, 63.248 )
    ( 5681, 63.459 )
    ( 5682, 63.639 )
    ( 5683, 63.736 )
    ( 5684, 63.833 )
    ( 5685, 63.930 )
    ( 5686, 64.051 )
    ( 5687, 64.147 )
    ( 5688, 64.245 )
    ( 5689, 64.342 )
    ( 5690, 64.439 )
    ( 5691, 64.536 )
    ( 5692, 64.687 )
    ( 5693, 64.810 )
    ( 5694, 64.933 )
    ( 5695, 65.055 )
    ( 5696, 65.188 )
    ( 5697, 65.324 )
    ( 5698, 65.458 )
    ( 5699, 65.637 )
    ( 5700, 65.737 )
    ( 5701, 65.837 )
    ( 5702, 65.971 )
    ( 5703, 66.146 )
    ( 5704, 66.140 )
    ( 5705, 66.429 )
    ( 5706, 66.525 )
    ( 5707, 66.610 )
    ( 5708, 66.997 )
    ( 5709, 67.241 )
    ( 5710, 67.492 )
    ( 5711, 67.735 )
    ( 5712, 67.958 )
    ( 5713, 68.179 )
    ( 5714, 68.380 )
    ( 5715, 68.670 )
    ( 5716, 68.961 )
    ( 5717, 69.160 )
    ( 5718, 69.369 )
    ( 5719, 69.590 )
    ( 5720, 69.790 )
    ( 5721, 69.990 )
    ( 5722, 70.241 )
    ( 5723, 70.493 )
    ( 5724, 70.692 )
    ( 5725, 71.078 )
    ( 5726, 71.506 )
    ( 5727, 71.932 )
    ( 5728, 72.227 )
    ( 5729, 72.530 )
    ( 5730, 72.811 )
    ( 5731, 73.186 )
    ( 5732, 73.474 )
    ( 5733, 73.772 )
    ( 5734, 74.023 )
    ( 5735, 74.271 )
    ( 5736, 74.515 )
    ( 5737, 74.738 )
    ( 5738, 74.957 )
    ( 5739, 75.179 )
    ( 5740, 75.462 )
    ( 5741, 75.663 )
    ( 5742, 76.107 )
    ( 5743, 76.489 )
    ( 5744, 76.862 )
    ( 5745, 77.255 )
    ( 5746, 77.582 )
    ( 5747, 77.943 )
    ( 5748, 78.287 )
    ( 5749, 78.434 )
    ( 5750, 78.534 )
    ( 5751, 78.647 )
    ( 5752, 78.749 )
    ( 5753, 78.871 )
    ( 5754, 79.039 )
    ( 5755, 79.156 )
    ( 5756, 79.319 )
    ( 5757, 79.582 )
    ( 5758, 79.733 )
    ( 5759, 79.870 )
    ( 5760, 79.971 )
    ( 5761, 80.134 )
    ( 5762, 80.230 )
    ( 5763, 80.327 )
    ( 5764, 80.524 )
    ( 5765, 80.671 )
    ( 5766, 80.816 )
    ( 5767, 80.859 )
    ( 5768, 80.847 )
    ( 5769, 80.873 )
    ( 5770, 80.859 )
    ( 5771, 80.846 )
    ( 5772, 80.839 )
    ( 5773, 80.889 )
    ( 5774, 80.951 )
    ( 5775, 80.948 )
    ( 5776, 80.823 )
    ( 5777, 80.698 )
    ( 5778, 80.647 )
    ( 5779, 80.523 )
    ( 5780, 80.635 )
    ( 5781, 80.735 )
    ( 5782, 80.658 )
    ( 5783, 80.644 )
    ( 5784, 80.539 )
    ( 5785, 80.415 )
    ( 5786, 80.362 )
    ( 5787, 80.241 )
    ( 5788, 80.145 )
    ( 5789, 80.021 )
    ( 5790, 79.948 )
    ( 5791, 79.823 )
    ( 5792, 79.699 )
    ( 5793, 79.630 )
    ( 5794, 79.565 )
    ( 5795, 79.590 )
    ( 5796, 79.553 )
    ( 5797, 79.483 )
    ( 5798, 79.358 )
    ( 5799, 79.237 )
    ( 5800, 79.162 )
    ( 5801, 79.120 )
    ( 5802, 78.995 )
    ( 5803, 78.871 )
    ( 5804, 79.320 )
    ( 5805, 79.762 )
    ( 5806, 80.091 )
    ( 5807, 80.466 )
    ( 5808, 80.811 )
    ( 5809, 81.133 )
    ( 5810, 81.455 )
    ( 5811, 81.700 )
    ( 5812, 81.913 )
    ( 5813, 82.122 )
    ( 5814, 82.344 )
    ( 5815, 82.560 )
    ( 5816, 82.535 )
    ( 5817, 82.516 )
    ( 5818, 82.523 )
    ( 5819, 82.500 )
    ( 5820, 82.585 )
    ( 5821, 82.587 )
    ( 5822, 82.573 )
    ( 5823, 82.560 )
    ( 5824, 82.585 )
    ( 5825, 82.461 )
    ( 5826, 82.505 )
    ( 5827, 82.588 )
    ( 5828, 82.464 )
    ( 5829, 82.339 )
    ( 5830, 82.234 )
    ( 5831, 82.109 )
    ( 5832, 82.026 )
    ( 5833, 81.901 )
    ( 5834, 81.776 )
    ( 5835, 81.770 )
    ( 5836, 81.989 )
    ( 5837, 82.193 )
    ( 5838, 82.505 )
    ( 5839, 82.716 )
    ( 5840, 82.946 )
    ( 5841, 83.205 )
    ( 5842, 83.405 )
    ( 5843, 83.379 )
    ( 5844, 83.539 )
    ( 5845, 83.747 )
    ( 5846, 83.896 )
    ( 5847, 84.030 )
    ( 5848, 84.166 )
    ( 5849, 84.284 )
    ( 5850, 84.300 )
    ( 5851, 84.295 )
    ( 5852, 84.236 )
    ( 5853, 84.184 )
    ( 5854, 84.126 )
    ( 5855, 83.879 )
    ( 5856, 83.732 )
    ( 5857, 83.587 )
    ( 5858, 83.285 )
    ( 5859, 83.140 )
    ( 5860, 82.839 )
    ( 5861, 82.557 )
    ( 5862, 82.266 )
    ( 5863, 81.986 )
    ( 5864, 81.838 )
    ( 5865, 81.629 )
    ( 5866, 81.341 )
    ( 5867, 81.195 )
    ( 5868, 80.895 )
    ( 5869, 80.624 )
    ( 5870, 80.341 )
    ( 5871, 80.040 )
    ( 5872, 79.850 )
    ( 5873, 79.557 )
    ( 5874, 79.312 )
    ( 5875, 79.151 )
    ( 5876, 78.862 )
    ( 5877, 78.790 )
    ( 5878, 78.645 )
    ( 5879, 78.438 )
    ( 5880, 78.228 )
    ( 5881, 78.074 )
    ( 5882, 77.886 )
    ( 5883, 77.587 )
    ( 5884, 77.497 )
    ( 5885, 77.441 )
    ( 5886, 77.352 )
    ( 5887, 77.256 )
    ( 5888, 77.203 )
    ( 5889, 76.905 )
    ( 5890, 76.604 )
    ( 5891, 76.305 )
    ( 5892, 76.159 )
    ( 5893, 75.869 )
    ( 5894, 75.591 )
    ( 5895, 75.320 )
    ( 5896, 75.050 )
    ( 5897, 74.819 )
    ( 5898, 74.715 )
    ( 5899, 74.438 )
    ( 5900, 74.207 )
    ( 5901, 73.979 )
    ( 5902, 73.749 )
    ( 5903, 73.457 )
    ( 5904, 73.167 )
    ( 5905, 72.865 )
    ( 5906, 72.564 )
    ( 5907, 72.264 )
    ( 5908, 72.167 )
    ( 5909, 72.184 )
    ( 5910, 71.883 )
    ( 5911, 71.582 )
    ( 5912, 71.299 )
    ( 5913, 71.012 )
    ( 5914, 70.866 )
    ( 5915, 70.890 )
    ( 5916, 70.793 )
    ( 5917, 70.492 )
    ( 5918, 70.420 )
    ( 5919, 70.349 )
    ( 5920, 70.292 )
    ( 5921, 70.096 )
    ( 5922, 69.795 )
    ( 5923, 69.495 )
    ( 5924, 69.196 )
    ( 5925, 68.896 )
    ( 5926, 68.614 )
    ( 5927, 68.335 )
    ( 5928, 68.202 )
    ( 5929, 68.120 )
    ( 5930, 67.819 )
    ( 5931, 67.518 )
    ( 5932, 67.231 )
    ( 5933, 67.021 )
    ( 5934, 66.720 )
    ( 5935, 66.489 )
    ( 5936, 66.188 )
    ( 5937, 65.887 )
    ( 5938, 65.677 )
    ( 5939, 65.375 )
    ( 5940, 65.093 )
    ( 5941, 64.791 )
    ( 5942, 64.507 )
    ( 5943, 64.228 )
    ( 5944, 64.138 )
    ( 5945, 63.991 )
    ( 5946, 63.846 )
    ( 5947, 63.546 )
    ( 5948, 63.373 )
    ( 5949, 63.075 )
    ( 5950, 62.837 )
    ( 5951, 62.536 )
    ( 5952, 62.254 )
    ( 5953, 61.953 )
    ( 5954, 61.663 )
    ( 5955, 61.362 )
    ( 5956, 61.124 )
    ( 5957, 60.978 )
    ( 5958, 60.930 )
    ( 5959, 60.730 )
    ( 5960, 60.520 )
    ( 5961, 60.357 )
    ( 5962, 60.121 )
    ( 5963, 59.824 )
    ( 5964, 59.544 )
    ( 5965, 59.568 )
    ( 5966, 59.422 )
    ( 5967, 59.309 )
    ( 5968, 59.315 )
    ( 5969, 59.243 )
    ( 5970, 58.943 )
    ( 5971, 58.924 )
    ( 5972, 58.806 )
    ( 5973, 58.595 )
    ( 5974, 58.345 )
    ( 5975, 58.136 )
    ( 5976, 57.899 )
    ( 5977, 57.725 )
    ( 5978, 57.424 )
    ( 5979, 57.297 )
    ( 5980, 57.003 )
    ( 5981, 56.702 )
    ( 5982, 56.409 )
    ( 5983, 56.366 )
    ( 5984, 56.135 )
    ( 5985, 55.990 )
    ( 5986, 55.759 )
    ( 5987, 55.586 )
    ( 5988, 55.292 )
    ( 5989, 54.996 )
    ( 5990, 54.744 )
    ( 5991, 54.556 )
    ( 5992, 54.254 )
    ( 5993, 53.954 )
    ( 5994, 53.655 )
    ( 5995, 53.354 )
    ( 5996, 53.144 )
    ( 5997, 52.858 )
    ( 5998, 52.588 )
    ( 5999, 52.402 )
    ( 6000, 52.151 )
    ( 6001, 52.005 )
    ( 6002, 51.859 )
    ( 6003, 51.559 )
    ( 6004, 51.261 )
    ( 6005, 51.078 )
    ( 6006, 50.812 )
    ( 6007, 50.641 )
    ( 6008, 50.380 )
    ( 6009, 50.081 )
    ( 6010, 49.850 )
    ( 6011, 49.556 )
    ( 6012, 49.454 )
    ( 6013, 49.360 )
    ( 6014, 49.099 )
    ( 6015, 48.803 )
    ( 6016, 48.606 )
    ( 6017, 48.315 )
    ( 6018, 48.114 )
    ( 6019, 47.813 )
    ( 6020, 47.512 )
    ( 6021, 47.211 )
    ( 6022, 47.114 )
    ( 6023, 47.039 )
    ( 6024, 46.865 )
    ( 6025, 46.574 )
    ( 6026, 46.307 )
    ( 6027, 46.114 )
    ( 6028, 45.853 )
    ( 6029, 45.562 )
    ( 6030, 45.439 )
    ( 6031, 45.334 )
    ( 6032, 45.188 )
    ( 6033, 44.949 )
    ( 6034, 44.648 )
    ( 6035, 44.355 )
    ( 6036, 44.054 )
    ( 6037, 43.753 )
    ( 6038, 43.500 )
    ( 6039, 43.200 )
    ( 6040, 42.903 )
    ( 6041, 42.606 )
    ( 6042, 42.306 )
    ( 6043, 42.004 )
    ( 6044, 41.711 )
    ( 6045, 41.565 )
    ( 6046, 41.295 )
    ( 6047, 41.023 )
    ( 6048, 41.066 )
    ( 6049, 40.941 )
    ( 6050, 40.948 )
    ( 6051, 40.893 )
    ( 6052, 40.866 )
    ( 6053, 40.875 )
    ( 6054, 40.817 )
    ( 6055, 40.850 )
    ( 6056, 41.031 )
    ( 6057, 41.188 )
    ( 6058, 41.345 )
    ( 6059, 41.429 )
    ( 6060, 41.520 )
    ( 6061, 41.612 )
    ( 6062, 41.697 )
    ( 6063, 42.054 )
    ( 6064, 42.271 )
    ( 6065, 42.495 )
    ( 6066, 42.774 )
    ( 6067, 43.084 )
    ( 6068, 43.384 )
    ( 6069, 43.659 )
    ( 6070, 43.945 )
    ( 6071, 44.211 )
    ( 6072, 44.433 )
    ( 6073, 44.732 )
    ( 6074, 44.954 )
    ( 6075, 45.234 )
    ( 6076, 45.457 )
    ( 6077, 45.678 )
    ( 6078, 45.922 )
    ( 6079, 46.180 )
    ( 6080, 46.436 )
    ( 6081, 46.663 )
    ( 6082, 46.915 )
    ( 6083, 47.150 )
    ( 6084, 47.390 )
    ( 6085, 47.594 )
    ( 6086, 47.798 )
    ( 6087, 47.872 )
    ( 6088, 47.946 )
    ( 6089, 48.126 )
    ( 6090, 48.249 )
    ( 6091, 48.249 )
    ( 6092, 48.280 )
    ( 6093, 48.280 )
    ( 6094, 48.379 )
    ( 6095, 48.626 )
    ( 6096, 48.634 )
    ( 6097, 48.749 )
    ( 6098, 48.838 )
    ( 6099, 48.925 )
    ( 6100, 49.127 )
    ( 6101, 49.218 )
    ( 6102, 49.306 )
    ( 6103, 49.437 )
    ( 6104, 49.676 )
    ( 6105, 49.854 )
    ( 6106, 49.962 )
    ( 6107, 50.059 )
    ( 6108, 50.126 )
    ( 6109, 50.220 )
    ( 6110, 50.289 )
    ( 6111, 50.381 )
    ( 6112, 50.635 )
    ( 6113, 50.801 )
    ( 6114, 50.956 )
    ( 6115, 51.103 )
    ( 6116, 51.253 )
    ( 6117, 51.448 )
    ( 6118, 51.594 )
    ( 6119, 51.728 )
    ( 6120, 51.854 )
    ( 6121, 52.061 )
    ( 6122, 52.294 )
    ( 6123, 52.640 )
    ( 6124, 52.841 )
    ( 6125, 53.011 )
    ( 6126, 53.122 )
    ( 6127, 53.190 )
    ( 6128, 53.305 )
    ( 6129, 53.400 )
    ( 6130, 53.498 )
    ( 6131, 53.585 )
    ( 6132, 53.673 )
    ( 6133, 53.770 )
    ( 6134, 53.837 )
    ( 6135, 54.041 )
    ( 6136, 54.246 )
    ( 6137, 54.472 )
    ( 6138, 54.772 )
    ( 6139, 55.055 )
    ( 6140, 55.277 )
    ( 6141, 55.532 )
    ( 6142, 55.782 )
    ( 6143, 56.031 )
    ( 6144, 56.346 )
    ( 6145, 56.688 )
    ( 6146, 57.024 )
    ( 6147, 57.375 )
    ( 6148, 57.605 )
    ( 6149, 57.830 )
    ( 6150, 58.090 )
    ( 6151, 58.313 )
    ( 6152, 58.594 )
    ( 6153, 58.816 )
    ( 6154, 59.090 )
    ( 6155, 59.312 )
    ( 6156, 59.533 )
    ( 6157, 59.802 )
    ( 6158, 59.946 )
    ( 6159, 60.014 )
    ( 6160, 60.241 )
    ( 6161, 60.452 )
    ( 6162, 60.661 )
    ( 6163, 60.919 )
    ( 6164, 61.134 )
    ( 6165, 61.201 )
    ( 6166, 61.268 )
    ( 6167, 61.335 )
    ( 6168, 61.416 )
    ( 6169, 61.497 )
    ( 6170, 61.563 )
    ( 6171, 61.630 )
    ( 6172, 61.632 )
    ( 6173, 61.675 )
    ( 6174, 61.680 )
    ( 6175, 61.683 )
    ( 6176, 61.745 )
    ( 6177, 61.892 )
    ( 6178, 61.894 )
    ( 6179, 61.894 )
    ( 6180, 62.003 )
    ( 6181, 62.003 )
    ( 6182, 62.003 )
    ( 6183, 62.003 )
    ( 6184, 62.003 )
    ( 6185, 62.027 )
    ( 6186, 62.094 )
    ( 6187, 62.162 )
    ( 6188, 62.341 )
    ( 6189, 62.408 )
    ( 6190, 62.476 )
    ( 6191, 62.634 )
    ( 6192, 62.769 )
    ( 6193, 62.904 )
    ( 6194, 62.996 )
    ( 6195, 63.088 )
    ( 6196, 63.156 )
    ( 6197, 63.225 )
    ( 6198, 63.394 )
    ( 6199, 63.481 )
    ( 6200, 63.579 )
    ( 6201, 63.674 )
    ( 6202, 63.808 )
    ( 6203, 63.896 )
    ( 6204, 64.034 )
    ( 6205, 64.133 )
    ( 6206, 64.228 )
    ( 6207, 64.381 )
    ( 6208, 64.473 )
    ( 6209, 64.654 )
    ( 6210, 64.743 )
    ( 6211, 64.830 )
    ( 6212, 64.947 )
    ( 6213, 65.020 )
    ( 6214, 65.090 )
    ( 6215, 65.160 )
    ( 6216, 65.235 )
    ( 6217, 65.324 )
    ( 6218, 65.412 )
    ( 6219, 65.499 )
    ( 6220, 65.652 )
    ( 6221, 65.807 )
    ( 6222, 65.893 )
    ( 6223, 65.960 )
    ( 6224, 66.065 )
    ( 6225, 66.152 )
    ( 6226, 66.284 )
    ( 6227, 66.411 )
    ( 6228, 66.596 )
    ( 6229, 66.765 )
    ( 6230, 66.996 )
    ( 6231, 67.200 )
    ( 6232, 67.267 )
    ( 6233, 67.439 )
    ( 6234, 67.628 )
    ( 6235, 67.694 )
    ( 6236, 67.762 )
    ( 6237, 67.849 )
    ( 6238, 67.995 )
    ( 6239, 68.134 )
    ( 6240, 68.282 )
    ( 6241, 68.443 )
    ( 6242, 68.591 )
    ( 6243, 68.711 )
    ( 6244, 68.839 )
    ( 6245, 68.944 )
    ( 6246, 69.034 )
    ( 6247, 69.276 )
    ( 6248, 69.479 )
    ( 6249, 69.689 )
    ( 6250, 69.897 )
    ( 6251, 70.066 )
    ( 6252, 70.134 )
    ( 6253, 70.134 )
    ( 6254, 70.200 )
    ( 6255, 70.287 )
    ( 6256, 70.378 )
    ( 6257, 70.378 )
    ( 6258, 70.450 )
    ( 6259, 70.451 )
    ( 6260, 70.514 )
    ( 6261, 70.578 )
    ( 6262, 70.780 )
    ( 6263, 70.950 )
    ( 6264, 70.950 )
    ( 6265, 71.073 )
    ( 6266, 71.198 )
    ( 6267, 71.280 )
    ( 6268, 71.285 )
    ( 6269, 71.308 )
    ( 6270, 71.462 )
    ( 6271, 71.549 )
    ( 6272, 71.616 )
    ( 6273, 71.684 )
    ( 6274, 71.758 )
    ( 6275, 71.825 )
    ( 6276, 71.994 )
    ( 6277, 71.994 )
    ( 6278, 72.119 )
    ( 6279, 72.119 )
    ( 6280, 72.203 )
    ( 6281, 72.222 )
    ( 6282, 72.399 )
    ( 6283, 72.523 )
    ( 6284, 72.647 )
    ( 6285, 72.648 )
    ( 6286, 72.799 )
    ( 6287, 72.848 )
    ( 6288, 73.010 )
    ( 6289, 73.251 )
    ( 6290, 73.313 )
    ( 6291, 73.328 )
    ( 6292, 73.330 )
    ( 6293, 73.438 )
    ( 6294, 73.501 )
    ( 6295, 73.568 )
    ( 6296, 73.644 )
    ( 6297, 73.705 )
    ( 6298, 73.715 )
    ( 6299, 73.843 )
    ( 6300, 73.983 )
    ( 6301, 74.199 )
    ( 6302, 74.418 )
    ( 6303, 74.583 )
    ( 6304, 74.692 )
    ( 6305, 74.739 )
    ( 6306, 74.764 )
    ( 6307, 74.839 )
    ( 6308, 74.839 )
    ( 6309, 75.013 )
    ( 6310, 75.120 )
    ( 6311, 75.229 )
    ( 6312, 75.340 )
    ( 6313, 75.449 )
    ( 6314, 75.559 )
    ( 6315, 75.566 )
    ( 6316, 75.566 )
    ( 6317, 75.566 )
    ( 6318, 75.658 )
    ( 6319, 75.694 )
    ( 6320, 75.858 )
    ( 6321, 76.006 )
    ( 6322, 76.152 )
    ( 6323, 76.262 )
    ( 6324, 76.439 )
    ( 6325, 76.613 )
    ( 6326, 76.752 )
    ( 6327, 76.753 )
    ( 6328, 76.899 )
    ( 6329, 76.912 )
    ( 6330, 76.917 )
    ( 6331, 76.917 )
    ( 6332, 76.934 )
    ( 6333, 76.941 )
    ( 6334, 76.991 )
    ( 6335, 77.041 )
    ( 6336, 77.049 )
    ( 6337, 77.050 )
    ( 6338, 77.098 )
    ( 6339, 77.166 )
    ( 6340, 77.167 )
    ( 6341, 77.276 )
    ( 6342, 77.423 )
    ( 6343, 77.569 )
    ( 6344, 77.715 )
    ( 6345, 77.875 )
    ( 6346, 78.065 )
    ( 6347, 78.149 )
    ( 6348, 78.159 )
    ( 6349, 78.164 )
    ( 6350, 78.165 )
    ( 6351, 78.184 )
    ( 6352, 78.330 )
    ( 6353, 78.334 )
    ( 6354, 78.334 )
    ( 6355, 78.334 )
    ( 6356, 78.532 )
    ( 6357, 78.697 )
    ( 6358, 78.810 )
    ( 6359, 78.932 )
    ( 6360, 78.955 )
    ( 6361, 78.992 )
    ( 6362, 79.191 )
    ( 6363, 79.201 )
    ( 6364, 79.201 )
    ( 6365, 79.218 )
    ( 6366, 79.327 )
    ( 6367, 79.327 )
    ( 6368, 79.327 )
    ( 6369, 79.372 )
    ( 6370, 79.395 )
    ( 6371, 79.432 )
    ( 6372, 79.554 )
    ( 6373, 79.599 )
    ( 6374, 79.599 )
    ( 6375, 79.603 )
    ( 6376, 79.603 )
    ( 6377, 79.653 )
    ( 6378, 79.716 )
    ( 6379, 79.720 )
    ( 6380, 79.782 )
    ( 6381, 79.793 )
    ( 6382, 79.868 )
    ( 6383, 79.868 )
    ( 6384, 80.123 )
    ( 6385, 80.352 )
    ( 6386, 80.441 )
    ( 6387, 80.562 )
    ( 6388, 80.697 )
    ( 6389, 80.784 )
    ( 6390, 80.890 )
    ( 6391, 80.983 )
    ( 6392, 80.984 )
    ( 6393, 81.057 )
    ( 6394, 81.057 )
    ( 6395, 81.298 )
    ( 6396, 81.444 )
    ( 6397, 81.591 )
    ( 6398, 81.752 )
    ( 6399, 81.968 )
    ( 6400, 82.114 )
    ( 6401, 82.272 )
    ( 6402, 82.419 )
    ( 6403, 82.567 )
    ( 6404, 82.774 )
    ( 6405, 82.920 )
    ( 6406, 83.066 )
    ( 6407, 83.237 )
    ( 6408, 83.403 )
    ( 6409, 83.405 )
    ( 6410, 83.405 )
    ( 6411, 83.406 )
    ( 6412, 83.442 )
    ( 6413, 83.617 )
    ( 6414, 83.617 )
    ( 6415, 83.812 )
    ( 6416, 84.034 )
    ( 6417, 84.181 )
    ( 6418, 84.181 )
    ( 6419, 84.182 )
    ( 6420, 84.327 )
    ( 6421, 84.474 )
    ( 6422, 84.626 )
    ( 6423, 84.771 )
    ( 6424, 84.953 )
    ( 6425, 85.101 )
    ( 6426, 85.423 )
    ( 6427, 85.692 )
    ( 6428, 85.692 )
    ( 6429, 85.702 )
    ( 6430, 85.702 )
    ( 6431, 85.751 )
    ( 6432, 85.896 )
    ( 6433, 85.896 )
    ( 6434, 85.899 )
    ( 6435, 86.044 )
    ( 6436, 86.131 )
    ( 6437, 86.148 )
    ( 6438, 86.148 )
    ( 6439, 86.185 )
    ( 6440, 86.294 )
    ( 6441, 86.500 )
    ( 6442, 86.630 )
    ( 6443, 86.759 )
    ( 6444, 86.868 )
    ( 6445, 86.868 )
    ( 6446, 86.868 )
    ( 6447, 86.869 )
    ( 6448, 86.871 )
    ( 6449, 87.075 )
    ( 6450, 87.245 )
    ( 6451, 87.415 )
    ( 6452, 87.524 )
    ( 6453, 87.528 )
    ( 6454, 87.529 )
    ( 6455, 87.679 )
    ( 6456, 87.825 )
    ( 6457, 87.877 )
    ( 6458, 87.929 )
    ( 6459, 87.935 )
    ( 6460, 87.935 )
    ( 6461, 87.950 )
    ( 6462, 88.020 )
    ( 6463, 88.092 )
    ( 6464, 88.238 )
    ( 6465, 88.245 )
    ( 6466, 88.299 )
    ( 6467, 88.445 )
    ( 6468, 88.452 )
    ( 6469, 88.470 )
    ( 6470, 88.495 )
    ( 6471, 88.596 )
    ( 6472, 88.645 )
    ( 6473, 88.730 )
    ( 6474, 88.748 )
    ( 6475, 88.748 )
    ( 6476, 88.857 )
    ( 6477, 89.026 )
    ( 6478, 89.195 )
    ( 6479, 89.275 )
    ( 6480, 89.343 )
    ( 6481, 89.462 )
    ( 6482, 89.706 )
    ( 6483, 89.910 )
    ( 6484, 89.982 )
    ( 6485, 90.090 )
    ( 6486, 90.183 )
    ( 6487, 90.313 )
    ( 6488, 90.501 )
    ( 6489, 90.568 )
    ( 6490, 90.635 )
    ( 6491, 90.702 )
    ( 6492, 90.949 )
    ( 6493, 91.186 )
    ( 6494, 91.416 )
    ( 6495, 91.524 )
    ( 6496, 91.591 )
    ( 6497, 91.591 )
    ( 6498, 91.758 )
    ( 6499, 91.873 )
    ( 6500, 91.982 )
    ( 6501, 91.992 )
    ( 6502, 91.993 )
    ( 6503, 91.993 )
    ( 6504, 92.215 )
    ( 6505, 92.526 )
    ( 6506, 92.750 )
    ( 6507, 92.973 )
    ( 6508, 93.251 )
    ( 6509, 93.532 )
    ( 6510, 93.782 )
    ( 6511, 93.998 )
    ( 6512, 94.099 )
    ( 6513, 94.183 )
    ( 6514, 94.249 )
    ( 6515, 94.529 )
    ( 6516, 94.901 )
    ( 6517, 95.314 )
    ( 6518, 95.714 )
    ( 6519, 96.100 )
    ( 6520, 96.494 )
    ( 6521, 96.887 )
    ( 6522, 97.260 )
    ( 6523, 97.633 )
    ( 6524, 98.025 )
    ( 6525, 98.443 )
    ( 6526, 98.843 )
    ( 6527, 99.181 )
};


==> H314718 <==
\addplot[color=yellow] coordinates{
    ( 0, 5.4979 )
    ( 1, 5.4979 )
    ( 2, 5.7557 )
    ( 3, 6.0124 )
    ( 4, 6.1375 )
    ( 5, 6.4745 )
    ( 6, 6.7335 )
    ( 7, 6.8796 )
    ( 8, 6.9694 )
    ( 9, 7.0464 )
    ( 10, 7.0464 )
    ( 11, 7.3787 )
    ( 12, 7.6057 )
    ( 13, 7.7991 )
    ( 14, 7.9683 )
    ( 15, 8.0624 )
    ( 16, 8.1603 )
    ( 17, 8.1658 )
    ( 18, 8.2296 )
    ( 19, 8.3232 )
    ( 20, 8.3529 )
    ( 21, 8.4487 )
    ( 22, 8.5181 )
    ( 23, 8.5543 )
    ( 24, 8.5994 )
    ( 25, 8.6078 )
    ( 26, 8.7584 )
    ( 27, 8.7584 )
    ( 28, 8.7780 )
    ( 29, 8.7780 )
    ( 30, 8.7906 )
    ( 31, 8.8646 )
    ( 32, 8.8651 )
    ( 33, 9.1128 )
    ( 34, 9.2808 )
    ( 35, 9.3175 )
    ( 36, 9.4917 )
    ( 37, 9.4917 )
    ( 38, 9.5792 )
    ( 39, 9.6461 )
    ( 40, 9.8303 )
    ( 41, 9.7085 )
    ( 42, 9.8842 )
    ( 43, 10.009 )
    ( 44, 10.200 )
    ( 45, 10.326 )
    ( 46, 10.594 )
    ( 47, 10.724 )
    ( 48, 10.655 )
    ( 49, 10.755 )
    ( 50, 10.779 )
    ( 51, 10.738 )
    ( 52, 10.615 )
    ( 53, 10.801 )
    ( 54, 10.986 )
    ( 55, 11.255 )
    ( 56, 11.431 )
    ( 57, 11.644 )
    ( 58, 11.915 )
    ( 59, 12.184 )
    ( 60, 12.397 )
    ( 61, 12.596 )
    ( 62, 12.846 )
    ( 63, 13.153 )
    ( 64, 13.390 )
    ( 65, 13.644 )
    ( 66, 13.903 )
    ( 67, 14.161 )
    ( 68, 14.397 )
    ( 69, 14.666 )
    ( 70, 14.939 )
    ( 71, 15.222 )
    ( 72, 15.508 )
    ( 73, 15.786 )
    ( 74, 15.827 )
    ( 75, 15.895 )
    ( 76, 16.012 )
    ( 77, 16.072 )
    ( 78, 16.113 )
    ( 79, 15.988 )
    ( 80, 16.050 )
    ( 81, 16.041 )
    ( 82, 16.057 )
    ( 83, 16.066 )
    ( 84, 16.038 )
    ( 85, 16.188 )
    ( 86, 16.411 )
    ( 87, 16.384 )
    ( 88, 16.325 )
    ( 89, 16.201 )
    ( 90, 16.076 )
    ( 91, 16.130 )
    ( 92, 16.129 )
    ( 93, 16.308 )
    ( 94, 16.319 )
    ( 95, 16.299 )
    ( 96, 16.310 )
    ( 97, 16.256 )
    ( 98, 16.198 )
    ( 99, 16.142 )
    ( 100, 16.218 )
    ( 101, 16.230 )
    ( 102, 16.230 )
    ( 103, 16.323 )
    ( 104, 16.395 )
    ( 105, 16.427 )
    ( 106, 16.484 )
    ( 107, 16.528 )
    ( 108, 16.750 )
    ( 109, 17.048 )
    ( 110, 17.071 )
    ( 111, 17.159 )
    ( 112, 17.226 )
    ( 113, 17.315 )
    ( 114, 17.323 )
    ( 115, 17.339 )
    ( 116, 17.357 )
    ( 117, 17.357 )
    ( 118, 17.534 )
    ( 119, 17.535 )
    ( 120, 17.575 )
    ( 121, 17.577 )
    ( 122, 17.606 )
    ( 123, 17.612 )
    ( 124, 17.613 )
    ( 125, 17.686 )
    ( 126, 17.730 )
    ( 127, 18.033 )
    ( 128, 18.037 )
    ( 129, 18.037 )
    ( 130, 18.408 )
    ( 131, 18.771 )
    ( 132, 19.066 )
    ( 133, 19.379 )
    ( 134, 19.678 )
    ( 135, 19.929 )
    ( 136, 20.185 )
    ( 137, 20.531 )
    ( 138, 20.884 )
    ( 139, 21.237 )
    ( 140, 21.600 )
    ( 141, 21.600 )
    ( 142, 21.648 )
    ( 143, 21.663 )
    ( 144, 21.695 )
    ( 145, 21.766 )
    ( 146, 21.776 )
    ( 147, 21.792 )
    ( 148, 21.647 )
    ( 149, 21.550 )
    ( 150, 21.320 )
    ( 151, 21.019 )
    ( 152, 20.894 )
    ( 153, 20.649 )
    ( 154, 20.349 )
    ( 155, 20.202 )
    ( 156, 20.084 )
    ( 157, 19.783 )
    ( 158, 19.482 )
    ( 159, 19.603 )
    ( 160, 19.650 )
    ( 161, 19.692 )
    ( 162, 19.806 )
    ( 163, 19.931 )
    ( 164, 19.810 )
    ( 165, 19.694 )
    ( 166, 19.569 )
    ( 167, 19.449 )
    ( 168, 19.634 )
    ( 169, 19.878 )
    ( 170, 20.118 )
    ( 171, 20.281 )
    ( 172, 20.241 )
    ( 173, 20.116 )
    ( 174, 20.047 )
    ( 175, 20.118 )
    ( 176, 19.993 )
    ( 177, 19.868 )
    ( 178, 19.828 )
    ( 179, 19.703 )
    ( 180, 19.612 )
    ( 181, 19.498 )
    ( 182, 19.376 )
    ( 183, 19.337 )
    ( 184, 19.212 )
    ( 185, 19.115 )
    ( 186, 19.020 )
    ( 187, 19.035 )
    ( 188, 18.969 )
    ( 189, 19.047 )
    ( 190, 19.060 )
    ( 191, 19.060 )
    ( 192, 19.403 )
    ( 193, 19.683 )
    ( 194, 19.942 )
    ( 195, 20.166 )
    ( 196, 20.506 )
    ( 197, 20.943 )
    ( 198, 21.206 )
    ( 199, 21.451 )
    ( 200, 21.733 )
    ( 201, 22.009 )
    ( 202, 22.087 )
    ( 203, 22.102 )
    ( 204, 22.126 )
    ( 205, 21.837 )
    ( 206, 21.536 )
    ( 207, 21.485 )
    ( 208, 21.388 )
    ( 209, 21.292 )
    ( 210, 21.195 )
    ( 211, 20.901 )
    ( 212, 20.812 )
    ( 213, 20.511 )
    ( 214, 20.344 )
    ( 215, 20.117 )
    ( 216, 19.826 )
    ( 217, 19.540 )
    ( 218, 19.245 )
    ( 219, 18.944 )
    ( 220, 18.688 )
    ( 221, 18.578 )
    ( 222, 18.681 )
    ( 223, 18.610 )
    ( 224, 18.542 )
    ( 225, 18.485 )
    ( 226, 18.341 )
    ( 227, 18.232 )
    ( 228, 18.100 )
    ( 229, 17.869 )
    ( 230, 17.601 )
    ( 231, 17.350 )
    ( 232, 17.080 )
    ( 233, 16.883 )
    ( 234, 16.688 )
    ( 235, 16.455 )
    ( 236, 16.196 )
    ( 237, 15.904 )
    ( 238, 15.603 )
    ( 239, 15.514 )
    ( 240, 15.215 )
    ( 241, 14.921 )
    ( 242, 14.945 )
    ( 243, 14.848 )
    ( 244, 14.780 )
    ( 245, 14.479 )
    ( 246, 14.178 )
    ( 247, 13.883 )
    ( 248, 13.584 )
    ( 249, 13.283 )
    ( 250, 13.148 )
    ( 251, 13.101 )
    ( 252, 13.183 )
    ( 253, 13.155 )
    ( 254, 13.088 )
    ( 255, 12.787 )
    ( 256, 12.772 )
    ( 257, 12.721 )
    ( 258, 12.664 )
    ( 259, 12.617 )
    ( 260, 12.737 )
    ( 261, 12.761 )
    ( 262, 12.843 )
    ( 263, 13.059 )
    ( 264, 13.262 )
    ( 265, 13.397 )
    ( 266, 13.272 )
    ( 267, 13.170 )
    ( 268, 13.474 )
    ( 269, 13.720 )
    ( 270, 13.905 )
    ( 271, 14.166 )
    ( 272, 14.330 )
    ( 273, 14.455 )
    ( 274, 14.612 )
    ( 275, 14.798 )
    ( 276, 14.978 )
    ( 277, 15.244 )
    ( 278, 15.430 )
    ( 279, 15.614 )
    ( 280, 15.579 )
    ( 281, 15.521 )
    ( 282, 15.493 )
    ( 283, 15.473 )
    ( 284, 15.415 )
    ( 285, 15.449 )
    ( 286, 15.472 )
    ( 287, 15.458 )
    ( 288, 15.157 )
    ( 289, 14.856 )
    ( 290, 14.751 )
    ( 291, 14.565 )
    ( 292, 14.369 )
    ( 293, 14.158 )
    ( 294, 14.127 )
    ( 295, 14.044 )
    ( 296, 13.848 )
    ( 297, 13.547 )
    ( 298, 13.453 )
    ( 299, 13.188 )
    ( 300, 13.042 )
    ( 301, 12.770 )
    ( 302, 12.676 )
    ( 303, 12.620 )
    ( 304, 12.318 )
    ( 305, 12.246 )
    ( 306, 12.373 )
    ( 307, 12.568 )
    ( 308, 12.809 )
    ( 309, 13.005 )
    ( 310, 13.135 )
    ( 311, 13.260 )
    ( 312, 13.420 )
    ( 313, 13.594 )
    ( 314, 13.735 )
    ( 315, 13.965 )
    ( 316, 14.294 )
    ( 317, 14.629 )
    ( 318, 14.959 )
    ( 319, 15.268 )
    ( 320, 15.593 )
    ( 321, 15.848 )
    ( 322, 15.975 )
    ( 323, 16.163 )
    ( 324, 16.347 )
    ( 325, 16.068 )
    ( 326, 15.766 )
    ( 327, 15.913 )
    ( 328, 15.885 )
    ( 329, 15.689 )
    ( 330, 15.456 )
    ( 331, 15.157 )
    ( 332, 14.875 )
    ( 333, 14.602 )
    ( 334, 14.371 )
    ( 335, 14.074 )
    ( 336, 13.773 )
    ( 337, 13.472 )
    ( 338, 13.414 )
    ( 339, 13.178 )
    ( 340, 12.877 )
    ( 341, 12.582 )
    ( 342, 12.415 )
    ( 343, 12.318 )
    ( 344, 12.108 )
    ( 345, 11.837 )
    ( 346, 11.771 )
    ( 347, 11.487 )
    ( 348, 11.512 )
    ( 349, 11.493 )
    ( 350, 11.238 )
    ( 351, 11.045 )
    ( 352, 10.798 )
    ( 353, 10.497 )
    ( 354, 10.277 )
    ( 355, 9.9758 )
    ( 356, 9.7385 )
    ( 357, 9.6719 )
    ( 358, 9.4611 )
    ( 359, 9.2731 )
    ( 360, 9.2759 )
    ( 361, 9.1874 )
    ( 362, 9.1460 )
    ( 363, 9.0210 )
    ( 364, 9.1432 )
    ( 365, 9.0852 )
    ( 366, 9.0115 )
    ( 367, 8.8870 )
    ( 368, 8.7643 )
    ( 369, 8.6959 )
    ( 370, 8.7052 )
    ( 371, 8.5817 )
    ( 372, 8.5126 )
    ( 373, 8.6129 )
    ( 374, 8.8385 )
    ( 375, 8.9229 )
    ( 376, 9.1437 )
    ( 377, 9.1224 )
    ( 378, 9.1086 )
    ( 379, 9.0508 )
    ( 380, 9.0327 )
    ( 381, 9.1346 )
    ( 382, 9.1428 )
    ( 383, 9.1240 )
    ( 384, 9.1708 )
    ( 385, 9.1128 )
    ( 386, 9.0144 )
    ( 387, 9.1393 )
    ( 388, 9.2969 )
    ( 389, 9.5221 )
    ( 390, 9.7650 )
    ( 391, 9.9861 )
    ( 392, 10.194 )
    ( 393, 9.9526 )
    ( 394, 9.6549 )
    ( 395, 9.4120 )
    ( 396, 9.2010 )
    ( 397, 8.9000 )
    ( 398, 9.0336 )
    ( 399, 9.1398 )
    ( 400, 9.1438 )
    ( 401, 9.1367 )
    ( 402, 9.2598 )
    ( 403, 9.3585 )
    ( 404, 9.5331 )
    ( 405, 9.6300 )
    ( 406, 9.6714 )
    ( 407, 9.5790 )
    ( 408, 9.2780 )
    ( 409, 9.4366 )
    ( 410, 9.6160 )
    ( 411, 9.8159 )
    ( 412, 9.8448 )
    ( 413, 9.8816 )
    ( 414, 9.8827 )
    ( 415, 9.9244 )
    ( 416, 9.9244 )
    ( 417, 10.011 )
    ( 418, 10.101 )
    ( 419, 10.130 )
    ( 420, 10.292 )
    ( 421, 10.325 )
    ( 422, 10.356 )
    ( 423, 10.356 )
    ( 424, 10.356 )
    ( 425, 10.379 )
    ( 426, 10.380 )
    ( 427, 10.384 )
    ( 428, 10.662 )
    ( 429, 10.919 )
    ( 430, 11.151 )
    ( 431, 11.377 )
    ( 432, 11.600 )
    ( 433, 11.995 )
    ( 434, 12.473 )
    ( 435, 12.831 )
    ( 436, 13.052 )
    ( 437, 13.117 )
    ( 438, 13.145 )
    ( 439, 13.321 )
    ( 440, 13.467 )
    ( 441, 13.637 )
    ( 442, 13.637 )
    ( 443, 13.637 )
    ( 444, 13.765 )
    ( 445, 13.975 )
    ( 446, 14.001 )
    ( 447, 14.262 )
    ( 448, 14.490 )
    ( 449, 14.770 )
    ( 450, 15.045 )
    ( 451, 15.338 )
    ( 452, 15.679 )
    ( 453, 15.679 )
    ( 454, 15.694 )
    ( 455, 15.840 )
    ( 456, 15.840 )
    ( 457, 16.158 )
    ( 458, 16.467 )
    ( 459, 16.743 )
    ( 460, 17.041 )
    ( 461, 17.216 )
    ( 462, 17.268 )
    ( 463, 17.307 )
    ( 464, 17.344 )
    ( 465, 17.344 )
    ( 466, 17.387 )
    ( 467, 17.475 )
    ( 468, 17.475 )
    ( 469, 17.475 )
    ( 470, 17.475 )
    ( 471, 17.490 )
    ( 472, 17.513 )
    ( 473, 17.704 )
    ( 474, 18.041 )
    ( 475, 18.138 )
    ( 476, 18.254 )
    ( 477, 18.421 )
    ( 478, 18.696 )
    ( 479, 18.933 )
    ( 480, 19.164 )
    ( 481, 19.312 )
    ( 482, 19.409 )
    ( 483, 19.539 )
    ( 484, 19.636 )
    ( 485, 19.846 )
    ( 486, 19.839 )
    ( 487, 19.965 )
    ( 488, 19.958 )
    ( 489, 19.835 )
    ( 490, 19.794 )
    ( 491, 19.757 )
    ( 492, 19.675 )
    ( 493, 19.560 )
    ( 494, 19.781 )
    ( 495, 20.211 )
    ( 496, 20.552 )
    ( 497, 20.773 )
    ( 498, 20.772 )
    ( 499, 20.759 )
    ( 500, 20.745 )
    ( 501, 20.977 )
    ( 502, 21.012 )
    ( 503, 20.893 )
    ( 504, 20.768 )
    ( 505, 20.643 )
    ( 506, 20.617 )
    ( 507, 20.590 )
    ( 508, 20.471 )
    ( 509, 20.459 )
    ( 510, 20.335 )
    ( 511, 20.502 )
    ( 512, 20.632 )
    ( 513, 20.759 )
    ( 514, 20.926 )
    ( 515, 21.051 )
    ( 516, 21.179 )
    ( 517, 21.303 )
    ( 518, 21.637 )
    ( 519, 21.971 )
    ( 520, 22.184 )
    ( 521, 22.488 )
    ( 522, 22.696 )
    ( 523, 22.638 )
    ( 524, 22.442 )
    ( 525, 22.143 )
    ( 526, 21.997 )
    ( 527, 21.699 )
    ( 528, 21.407 )
    ( 529, 21.182 )
    ( 530, 20.932 )
    ( 531, 20.787 )
    ( 532, 20.486 )
    ( 533, 20.260 )
    ( 534, 19.983 )
    ( 535, 19.942 )
    ( 536, 19.848 )
    ( 537, 19.638 )
    ( 538, 19.338 )
    ( 539, 19.077 )
    ( 540, 18.781 )
    ( 541, 18.571 )
    ( 542, 18.270 )
    ( 543, 18.074 )
    ( 544, 17.781 )
    ( 545, 17.635 )
    ( 546, 17.398 )
    ( 547, 17.097 )
    ( 548, 16.836 )
    ( 549, 16.535 )
    ( 550, 16.500 )
    ( 551, 16.199 )
    ( 552, 16.102 )
    ( 553, 16.005 )
    ( 554, 15.908 )
    ( 555, 15.830 )
    ( 556, 15.551 )
    ( 557, 15.305 )
    ( 558, 15.005 )
    ( 559, 14.703 )
    ( 560, 14.558 )
    ( 561, 14.347 )
    ( 562, 14.134 )
    ( 563, 13.838 )
    ( 564, 13.642 )
    ( 565, 13.341 )
    ( 566, 13.040 )
    ( 567, 13.225 )
    ( 568, 13.433 )
    ( 569, 13.623 )
    ( 570, 13.685 )
    ( 571, 14.088 )
    ( 572, 14.394 )
    ( 573, 14.397 )
    ( 574, 14.463 )
    ( 575, 14.483 )
    ( 576, 14.492 )
    ( 577, 14.495 )
    ( 578, 14.641 )
    ( 579, 14.787 )
    ( 580, 15.047 )
    ( 581, 15.194 )
    ( 582, 15.194 )
    ( 583, 15.212 )
    ( 584, 15.267 )
    ( 585, 15.283 )
    ( 586, 15.355 )
    ( 587, 15.539 )
    ( 588, 15.723 )
    ( 589, 15.870 )
    ( 590, 16.016 )
    ( 591, 16.018 )
    ( 592, 16.040 )
    ( 593, 16.055 )
    ( 594, 16.114 )
    ( 595, 16.172 )
    ( 596, 16.114 )
    ( 597, 16.056 )
    ( 598, 16.002 )
    ( 599, 16.099 )
    ( 600, 16.157 )
    ( 601, 16.099 )
    ( 602, 16.105 )
    ( 603, 16.116 )
    ( 604, 16.303 )
    ( 605, 16.400 )
    ( 606, 16.497 )
    ( 607, 16.656 )
    ( 608, 16.773 )
    ( 609, 16.811 )
    ( 610, 16.961 )
    ( 611, 17.144 )
    ( 612, 17.144 )
    ( 613, 17.213 )
    ( 614, 17.297 )
    ( 615, 17.370 )
    ( 616, 17.516 )
    ( 617, 17.522 )
    ( 618, 17.551 )
    ( 619, 17.634 )
    ( 620, 17.748 )
    ( 621, 17.748 )
    ( 622, 17.796 )
    ( 623, 17.797 )
    ( 624, 17.797 )
    ( 625, 18.019 )
    ( 626, 18.348 )
    ( 627, 18.749 )
    ( 628, 19.033 )
    ( 629, 19.215 )
    ( 630, 19.362 )
    ( 631, 19.362 )
    ( 632, 19.660 )
    ( 633, 20.003 )
    ( 634, 20.345 )
    ( 635, 20.688 )
    ( 636, 21.017 )
    ( 637, 21.305 )
    ( 638, 21.495 )
    ( 639, 21.626 )
    ( 640, 21.780 )
    ( 641, 21.896 )
    ( 642, 22.077 )
    ( 643, 22.277 )
    ( 644, 22.362 )
    ( 645, 22.430 )
    ( 646, 22.514 )
    ( 647, 22.581 )
    ( 648, 22.852 )
    ( 649, 23.056 )
    ( 650, 23.308 )
    ( 651, 23.528 )
    ( 652, 23.778 )
    ( 653, 23.880 )
    ( 654, 23.967 )
    ( 655, 24.058 )
    ( 656, 24.170 )
    ( 657, 24.311 )
    ( 658, 24.379 )
    ( 659, 24.414 )
    ( 660, 24.669 )
    ( 661, 24.815 )
    ( 662, 25.015 )
    ( 663, 25.161 )
    ( 664, 25.161 )
    ( 665, 25.401 )
    ( 666, 25.597 )
    ( 667, 25.903 )
    ( 668, 26.226 )
    ( 669, 26.395 )
    ( 670, 26.465 )
    ( 671, 26.532 )
    ( 672, 26.641 )
    ( 673, 26.646 )
    ( 674, 26.646 )
    ( 675, 26.740 )
    ( 676, 26.740 )
    ( 677, 26.740 )
    ( 678, 26.807 )
    ( 679, 26.879 )
    ( 680, 27.014 )
    ( 681, 27.088 )
    ( 682, 27.159 )
    ( 683, 27.227 )
    ( 684, 27.228 )
    ( 685, 27.423 )
    ( 686, 27.686 )
    ( 687, 27.795 )
    ( 688, 27.904 )
    ( 689, 27.991 )
    ( 690, 28.079 )
    ( 691, 28.146 )
    ( 692, 28.271 )
    ( 693, 28.410 )
    ( 694, 28.530 )
    ( 695, 28.637 )
    ( 696, 28.724 )
    ( 697, 28.828 )
    ( 698, 28.922 )
    ( 699, 29.009 )
    ( 700, 29.103 )
    ( 701, 29.190 )
    ( 702, 29.277 )
    ( 703, 29.328 )
    ( 704, 29.328 )
    ( 705, 29.484 )
    ( 706, 29.557 )
    ( 707, 29.710 )
    ( 708, 29.711 )
    ( 709, 29.905 )
    ( 710, 29.937 )
    ( 711, 29.937 )
    ( 712, 30.004 )
    ( 713, 30.139 )
    ( 714, 30.308 )
    ( 715, 30.386 )
    ( 716, 30.480 )
    ( 717, 30.568 )
    ( 718, 30.677 )
    ( 719, 30.744 )
    ( 720, 30.913 )
    ( 721, 31.091 )
    ( 722, 31.158 )
    ( 723, 31.228 )
    ( 724, 31.421 )
    ( 725, 31.515 )
    ( 726, 31.635 )
    ( 727, 31.791 )
    ( 728, 31.878 )
    ( 729, 32.045 )
    ( 730, 32.045 )
    ( 731, 32.131 )
    ( 732, 32.204 )
    ( 733, 32.205 )
    ( 734, 32.211 )
    ( 735, 32.374 )
    ( 736, 32.437 )
    ( 737, 32.464 )
    ( 738, 32.544 )
    ( 739, 32.620 )
    ( 740, 32.691 )
    ( 741, 32.870 )
    ( 742, 32.986 )
    ( 743, 33.218 )
    ( 744, 33.423 )
    ( 745, 33.654 )
    ( 746, 33.721 )
    ( 747, 33.933 )
    ( 748, 34.069 )
    ( 749, 33.944 )
    ( 750, 33.886 )
    ( 751, 33.828 )
    ( 752, 33.805 )
    ( 753, 33.758 )
    ( 754, 33.816 )
    ( 755, 33.810 )
    ( 756, 33.826 )
    ( 757, 33.820 )
    ( 758, 33.762 )
    ( 759, 33.552 )
    ( 760, 33.263 )
    ( 761, 32.992 )
    ( 762, 32.896 )
    ( 763, 32.596 )
    ( 764, 32.297 )
    ( 765, 32.031 )
    ( 766, 31.730 )
    ( 767, 31.431 )
    ( 768, 31.285 )
    ( 769, 31.061 )
    ( 770, 30.772 )
    ( 771, 30.471 )
    ( 772, 30.170 )
    ( 773, 29.869 )
    ( 774, 29.782 )
    ( 775, 29.659 )
    ( 776, 29.534 )
    ( 777, 29.617 )
    ( 778, 29.658 )
    ( 779, 29.727 )
    ( 780, 29.674 )
    ( 781, 29.582 )
    ( 782, 29.465 )
    ( 783, 29.382 )
    ( 784, 29.257 )
    ( 785, 29.270 )
    ( 786, 29.145 )
    ( 787, 29.063 )
    ( 788, 28.938 )
    ( 789, 28.828 )
    ( 790, 28.713 )
    ( 791, 28.588 )
    ( 792, 28.463 )
    ( 793, 28.338 )
    ( 794, 28.215 )
    ( 795, 28.508 )
    ( 796, 28.763 )
    ( 797, 29.056 )
    ( 798, 29.236 )
    ( 799, 29.169 )
    ( 800, 29.147 )
    ( 801, 29.106 )
    ( 802, 29.079 )
    ( 803, 29.040 )
    ( 804, 29.011 )
    ( 805, 28.886 )
    ( 806, 28.928 )
    ( 807, 28.894 )
    ( 808, 28.787 )
    ( 809, 28.823 )
    ( 810, 28.817 )
    ( 811, 28.795 )
    ( 812, 29.035 )
    ( 813, 29.267 )
    ( 814, 29.548 )
    ( 815, 29.821 )
    ( 816, 30.056 )
    ( 817, 30.311 )
    ( 818, 30.544 )
    ( 819, 30.776 )
    ( 820, 31.017 )
    ( 821, 31.258 )
    ( 822, 31.565 )
    ( 823, 31.798 )
    ( 824, 32.053 )
    ( 825, 32.318 )
    ( 826, 32.632 )
    ( 827, 32.916 )
    ( 828, 33.206 )
    ( 829, 33.478 )
    ( 830, 33.733 )
    ( 831, 33.933 )
    ( 832, 34.022 )
    ( 833, 34.281 )
    ( 834, 34.468 )
    ( 835, 34.633 )
    ( 836, 34.860 )
    ( 837, 34.832 )
    ( 838, 34.714 )
    ( 839, 34.770 )
    ( 840, 34.743 )
    ( 841, 34.827 )
    ( 842, 34.867 )
    ( 843, 34.838 )
    ( 844, 34.814 )
    ( 845, 34.759 )
    ( 846, 34.718 )
    ( 847, 34.660 )
    ( 848, 34.602 )
    ( 849, 34.575 )
    ( 850, 34.569 )
    ( 851, 34.589 )
    ( 852, 34.570 )
    ( 853, 34.552 )
    ( 854, 34.494 )
    ( 855, 34.508 )
    ( 856, 34.565 )
    ( 857, 34.558 )
    ( 858, 34.563 )
    ( 859, 34.605 )
    ( 860, 34.586 )
    ( 861, 34.558 )
    ( 862, 34.547 )
    ( 863, 34.602 )
    ( 864, 34.588 )
    ( 865, 34.575 )
    ( 866, 34.539 )
    ( 867, 34.480 )
    ( 868, 34.180 )
    ( 869, 33.960 )
    ( 870, 33.663 )
    ( 871, 33.374 )
    ( 872, 33.073 )
    ( 873, 32.771 )
    ( 874, 32.511 )
    ( 875, 32.314 )
    ( 876, 32.137 )
    ( 877, 31.990 )
    ( 878, 31.906 )
    ( 879, 31.809 )
    ( 880, 31.832 )
    ( 881, 31.881 )
    ( 882, 31.763 )
    ( 883, 31.462 )
    ( 884, 31.394 )
    ( 885, 31.093 )
    ( 886, 30.996 )
    ( 887, 30.908 )
    ( 888, 30.957 )
    ( 889, 31.008 )
    ( 890, 30.943 )
    ( 891, 30.806 )
    ( 892, 30.656 )
    ( 893, 30.355 )
    ( 894, 30.056 )
    ( 895, 29.770 )
    ( 896, 29.469 )
    ( 897, 29.283 )
    ( 898, 29.110 )
    ( 899, 28.811 )
    ( 900, 28.514 )
    ( 901, 28.214 )
    ( 902, 27.913 )
    ( 903, 28.128 )
    ( 904, 28.129 )
    ( 905, 28.496 )
    ( 906, 28.858 )
    ( 907, 28.980 )
    ( 908, 29.137 )
    ( 909, 29.257 )
    ( 910, 29.339 )
    ( 911, 29.339 )
    ( 912, 29.351 )
    ( 913, 29.423 )
    ( 914, 29.566 )
    ( 915, 29.566 )
    ( 916, 29.566 )
    ( 917, 29.576 )
    ( 918, 29.576 )
    ( 919, 29.649 )
    ( 920, 29.674 )
    ( 921, 29.675 )
    ( 922, 29.675 )
    ( 923, 29.687 )
    ( 924, 29.842 )
    ( 925, 29.990 )
    ( 926, 30.033 )
    ( 927, 30.033 )
    ( 928, 30.095 )
    ( 929, 30.162 )
    ( 930, 30.162 )
    ( 931, 30.226 )
    ( 932, 30.226 )
    ( 933, 30.228 )
    ( 934, 30.251 )
    ( 935, 30.251 )
    ( 936, 30.251 )
    ( 937, 30.300 )
    ( 938, 30.361 )
    ( 939, 30.411 )
    ( 940, 30.455 )
    ( 941, 30.842 )
    ( 942, 31.118 )
    ( 943, 31.192 )
    ( 944, 31.344 )
    ( 945, 31.494 )
    ( 946, 31.694 )
    ( 947, 31.737 )
    ( 948, 31.810 )
    ( 949, 31.858 )
    ( 950, 31.865 )
    ( 951, 32.020 )
    ( 952, 32.048 )
    ( 953, 32.048 )
    ( 954, 32.048 )
    ( 955, 32.071 )
    ( 956, 32.078 )
    ( 957, 32.117 )
    ( 958, 32.117 )
    ( 959, 32.226 )
    ( 960, 32.226 )
    ( 961, 32.235 )
    ( 962, 32.271 )
    ( 963, 32.392 )
    ( 964, 32.501 )
    ( 965, 32.785 )
    ( 966, 33.007 )
    ( 967, 33.288 )
    ( 968, 33.547 )
    ( 969, 33.771 )
    ( 970, 33.999 )
    ( 971, 34.220 )
    ( 972, 34.446 )
    ( 973, 34.799 )
    ( 974, 35.021 )
    ( 975, 35.396 )
    ( 976, 35.738 )
    ( 977, 36.042 )
    ( 978, 36.350 )
    ( 979, 36.571 )
    ( 980, 36.834 )
    ( 981, 37.128 )
    ( 982, 37.502 )
    ( 983, 37.977 )
    ( 984, 38.376 )
    ( 985, 38.769 )
    ( 986, 39.161 )
    ( 987, 39.553 )
    ( 988, 39.829 )
    ( 989, 40.114 )
    ( 990, 40.391 )
    ( 991, 40.463 )
    ( 992, 40.463 )
    ( 993, 40.572 )
    ( 994, 40.794 )
    ( 995, 41.020 )
    ( 996, 41.259 )
    ( 997, 41.481 )
    ( 998, 41.894 )
    ( 999, 42.293 )
    ( 1000, 42.688 )
    ( 1001, 42.965 )
    ( 1002, 42.973 )
    ( 1003, 42.974 )
    ( 1004, 43.096 )
    ( 1005, 43.235 )
    ( 1006, 43.235 )
    ( 1007, 43.235 )
    ( 1008, 43.235 )
    ( 1009, 43.235 )
    ( 1010, 43.392 )
    ( 1011, 43.392 )
    ( 1012, 43.422 )
    ( 1013, 43.422 )
    ( 1014, 43.691 )
    ( 1015, 43.692 )
    ( 1016, 43.758 )
    ( 1017, 43.769 )
    ( 1018, 43.813 )
    ( 1019, 43.813 )
    ( 1020, 43.813 )
    ( 1021, 43.879 )
    ( 1022, 44.060 )
    ( 1023, 44.210 )
    ( 1024, 44.239 )
    ( 1025, 44.239 )
    ( 1026, 44.364 )
    ( 1027, 44.510 )
    ( 1028, 44.514 )
    ( 1029, 44.540 )
    ( 1030, 44.590 )
    ( 1031, 44.590 )
    ( 1032, 44.736 )
    ( 1033, 44.784 )
    ( 1034, 44.862 )
    ( 1035, 44.863 )
    ( 1036, 45.020 )
    ( 1037, 45.195 )
    ( 1038, 45.365 )
    ( 1039, 45.536 )
    ( 1040, 45.707 )
    ( 1041, 45.716 )
    ( 1042, 45.890 )
    ( 1043, 45.926 )
    ( 1044, 45.926 )
    ( 1045, 45.926 )
    ( 1046, 45.926 )
    ( 1047, 45.928 )
    ( 1048, 46.038 )
    ( 1049, 46.214 )
    ( 1050, 46.389 )
    ( 1051, 46.563 )
    ( 1052, 46.728 )
    ( 1053, 46.851 )
    ( 1054, 47.029 )
    ( 1055, 47.321 )
    ( 1056, 47.430 )
    ( 1057, 47.766 )
    ( 1058, 48.110 )
    ( 1059, 48.332 )
    ( 1060, 48.554 )
    ( 1061, 48.794 )
    ( 1062, 49.016 )
    ( 1063, 49.352 )
    ( 1064, 49.663 )
    ( 1065, 49.996 )
    ( 1066, 50.271 )
    ( 1067, 50.661 )
    ( 1068, 51.003 )
    ( 1069, 51.359 )
    ( 1070, 51.790 )
    ( 1071, 52.214 )
    ( 1072, 52.589 )
    ( 1073, 53.053 )
    ( 1074, 53.397 )
    ( 1075, 53.683 )
    ( 1076, 54.016 )
    ( 1077, 54.357 )
    ( 1078, 54.693 )
    ( 1079, 55.050 )
    ( 1080, 55.357 )
    ( 1081, 55.700 )
    ( 1082, 55.977 )
    ( 1083, 56.414 )
    ( 1084, 56.805 )
    ( 1085, 57.200 )
    ( 1086, 57.578 )
    ( 1087, 57.863 )
    ( 1088, 58.085 )
    ( 1089, 58.378 )
    ( 1090, 58.655 )
    ( 1091, 58.931 )
    ( 1092, 59.273 )
    ( 1093, 59.648 )
    ( 1094, 60.008 )
    ( 1095, 60.351 )
    ( 1096, 60.694 )
    ( 1097, 61.072 )
    ( 1098, 61.414 )
    ( 1099, 61.757 )
    ( 1100, 62.169 )
    ( 1101, 62.353 )
    ( 1102, 62.530 )
    ( 1103, 62.601 )
    ( 1104, 62.637 )
    ( 1105, 62.686 )
    ( 1106, 62.843 )
    ( 1107, 62.906 )
    ( 1108, 62.824 )
    ( 1109, 62.713 )
    ( 1110, 62.663 )
    ( 1111, 62.569 )
    ( 1112, 62.697 )
    ( 1113, 62.822 )
    ( 1114, 62.947 )
    ( 1115, 62.889 )
    ( 1116, 62.828 )
    ( 1117, 62.775 )
    ( 1118, 62.773 )
    ( 1119, 62.899 )
    ( 1120, 62.846 )
    ( 1121, 62.800 )
    ( 1122, 62.944 )
    ( 1123, 63.064 )
    ( 1124, 63.165 )
    ( 1125, 63.337 )
    ( 1126, 63.440 )
    ( 1127, 63.320 )
    ( 1128, 63.313 )
    ( 1129, 63.306 )
    ( 1130, 63.305 )
    ( 1131, 63.375 )
    ( 1132, 63.375 )
    ( 1133, 63.377 )
    ( 1134, 63.376 )
    ( 1135, 63.285 )
    ( 1136, 63.250 )
    ( 1137, 63.153 )
    ( 1138, 63.221 )
    ( 1139, 63.178 )
    ( 1140, 63.124 )
    ( 1141, 63.068 )
    ( 1142, 63.092 )
    ( 1143, 62.804 )
    ( 1144, 62.513 )
    ( 1145, 62.275 )
    ( 1146, 61.974 )
    ( 1147, 61.690 )
    ( 1148, 61.416 )
    ( 1149, 61.144 )
    ( 1150, 60.843 )
    ( 1151, 60.542 )
    ( 1152, 60.271 )
    ( 1153, 60.244 )
    ( 1154, 60.147 )
    ( 1155, 60.076 )
    ( 1156, 59.775 )
    ( 1157, 59.610 )
    ( 1158, 59.470 )
    ( 1159, 59.343 )
    ( 1160, 59.156 )
    ( 1161, 59.130 )
    ( 1162, 58.829 )
    ( 1163, 58.528 )
    ( 1164, 58.227 )
    ( 1165, 57.932 )
    ( 1166, 57.630 )
    ( 1167, 57.362 )
    ( 1168, 57.132 )
    ( 1169, 57.119 )
    ( 1170, 56.819 )
    ( 1171, 56.586 )
    ( 1172, 56.288 )
    ( 1173, 56.214 )
    ( 1174, 55.932 )
    ( 1175, 55.809 )
    ( 1176, 55.663 )
    ( 1177, 55.362 )
    ( 1178, 55.063 )
    ( 1179, 54.762 )
    ( 1180, 54.461 )
    ( 1181, 54.534 )
    ( 1182, 54.634 )
    ( 1183, 54.735 )
    ( 1184, 54.785 )
    ( 1185, 54.671 )
    ( 1186, 54.547 )
    ( 1187, 54.478 )
    ( 1188, 54.610 )
    ( 1189, 54.735 )
    ( 1190, 54.886 )
    ( 1191, 55.029 )
    ( 1192, 55.154 )
    ( 1193, 55.297 )
    ( 1194, 55.490 )
    ( 1195, 55.615 )
    ( 1196, 55.741 )
    ( 1197, 55.667 )
    ( 1198, 55.636 )
    ( 1199, 55.511 )
    ( 1200, 55.389 )
    ( 1201, 55.264 )
    ( 1202, 55.181 )
    ( 1203, 55.062 )
    ( 1204, 54.954 )
    ( 1205, 54.854 )
    ( 1206, 54.762 )
    ( 1207, 54.693 )
    ( 1208, 54.594 )
    ( 1209, 54.778 )
    ( 1210, 55.079 )
    ( 1211, 55.355 )
    ( 1212, 55.612 )
    ( 1213, 55.737 )
    ( 1214, 55.876 )
    ( 1215, 56.002 )
    ( 1216, 55.922 )
    ( 1217, 55.797 )
    ( 1218, 55.734 )
    ( 1219, 55.622 )
    ( 1220, 55.620 )
    ( 1221, 55.496 )
    ( 1222, 55.407 )
    ( 1223, 55.307 )
    ( 1224, 55.183 )
    ( 1225, 55.468 )
    ( 1226, 55.788 )
    ( 1227, 56.013 )
    ( 1228, 56.236 )
    ( 1229, 56.459 )
    ( 1230, 56.682 )
    ( 1231, 56.903 )
    ( 1232, 57.179 )
    ( 1233, 57.455 )
    ( 1234, 57.676 )
    ( 1235, 57.953 )
    ( 1236, 58.336 )
    ( 1237, 58.718 )
    ( 1238, 59.104 )
    ( 1239, 59.518 )
    ( 1240, 59.963 )
    ( 1241, 60.218 )
    ( 1242, 60.496 )
    ( 1243, 60.760 )
    ( 1244, 61.048 )
    ( 1245, 61.304 )
    ( 1246, 61.504 )
    ( 1247, 61.704 )
    ( 1248, 61.964 )
    ( 1249, 62.171 )
    ( 1250, 62.372 )
    ( 1251, 62.611 )
    ( 1252, 62.925 )
    ( 1253, 63.219 )
    ( 1254, 63.418 )
    ( 1255, 63.709 )
    ( 1256, 64.000 )
    ( 1257, 64.291 )
    ( 1258, 64.495 )
    ( 1259, 64.819 )
    ( 1260, 65.200 )
    ( 1261, 65.533 )
    ( 1262, 65.856 )
    ( 1263, 66.056 )
    ( 1264, 66.017 )
    ( 1265, 66.013 )
    ( 1266, 66.032 )
    ( 1267, 66.131 )
    ( 1268, 66.152 )
    ( 1269, 66.161 )
    ( 1270, 66.103 )
    ( 1271, 66.055 )
    ( 1272, 65.997 )
    ( 1273, 65.938 )
    ( 1274, 65.997 )
    ( 1275, 66.059 )
    ( 1276, 66.116 )
    ( 1277, 66.181 )
    ( 1278, 66.127 )
    ( 1279, 66.069 )
    ( 1280, 66.137 )
    ( 1281, 66.079 )
    ( 1282, 65.888 )
    ( 1283, 65.772 )
    ( 1284, 65.576 )
    ( 1285, 65.282 )
    ( 1286, 64.981 )
    ( 1287, 64.719 )
    ( 1288, 64.460 )
    ( 1289, 64.388 )
    ( 1290, 64.315 )
    ( 1291, 64.238 )
    ( 1292, 64.097 )
    ( 1293, 63.951 )
    ( 1294, 63.721 )
    ( 1295, 63.566 )
    ( 1296, 63.356 )
    ( 1297, 63.333 )
    ( 1298, 63.096 )
    ( 1299, 62.798 )
    ( 1300, 62.557 )
    ( 1301, 62.255 )
    ( 1302, 61.955 )
    ( 1303, 61.872 )
    ( 1304, 61.571 )
    ( 1305, 61.270 )
    ( 1306, 61.160 )
    ( 1307, 60.988 )
    ( 1308, 60.687 )
    ( 1309, 60.387 )
    ( 1310, 60.203 )
    ( 1311, 59.937 )
    ( 1312, 59.653 )
    ( 1313, 59.396 )
    ( 1314, 59.135 )
    ( 1315, 58.869 )
    ( 1316, 58.633 )
    ( 1317, 58.333 )
    ( 1318, 58.065 )
    ( 1319, 57.764 )
    ( 1320, 57.465 )
    ( 1321, 57.182 )
    ( 1322, 56.911 )
    ( 1323, 56.767 )
    ( 1324, 56.621 )
    ( 1325, 56.475 )
    ( 1326, 56.333 )
    ( 1327, 56.032 )
    ( 1328, 55.836 )
    ( 1329, 55.739 )
    ( 1330, 55.498 )
    ( 1331, 55.287 )
    ( 1332, 55.062 )
    ( 1333, 54.825 )
    ( 1334, 54.525 )
    ( 1335, 54.464 )
    ( 1336, 54.164 )
    ( 1337, 53.862 )
    ( 1338, 53.562 )
    ( 1339, 53.417 )
    ( 1340, 53.157 )
    ( 1341, 52.855 )
    ( 1342, 52.932 )
    ( 1343, 52.704 )
    ( 1344, 52.500 )
    ( 1345, 52.290 )
    ( 1346, 51.991 )
    ( 1347, 51.915 )
    ( 1348, 51.887 )
    ( 1349, 51.790 )
    ( 1350, 51.490 )
    ( 1351, 51.193 )
    ( 1352, 51.184 )
    ( 1353, 50.883 )
    ( 1354, 50.582 )
    ( 1355, 50.361 )
    ( 1356, 50.170 )
    ( 1357, 49.869 )
    ( 1358, 49.568 )
    ( 1359, 49.274 )
    ( 1360, 48.981 )
    ( 1361, 49.068 )
    ( 1362, 49.080 )
    ( 1363, 48.778 )
    ( 1364, 48.538 )
    ( 1365, 48.259 )
    ( 1366, 47.958 )
    ( 1367, 47.659 )
    ( 1368, 47.357 )
    ( 1369, 47.229 )
    ( 1370, 46.929 )
    ( 1371, 46.628 )
    ( 1372, 46.514 )
    ( 1373, 46.318 )
    ( 1374, 46.070 )
    ( 1375, 45.974 )
    ( 1376, 45.915 )
    ( 1377, 45.845 )
    ( 1378, 45.748 )
    ( 1379, 45.715 )
    ( 1380, 45.648 )
    ( 1381, 45.583 )
    ( 1382, 45.372 )
    ( 1383, 45.071 )
    ( 1384, 45.064 )
    ( 1385, 44.820 )
    ( 1386, 44.558 )
    ( 1387, 44.306 )
    ( 1388, 44.122 )
    ( 1389, 43.821 )
    ( 1390, 43.530 )
    ( 1391, 43.229 )
    ( 1392, 43.049 )
    ( 1393, 42.748 )
    ( 1394, 42.739 )
    ( 1395, 42.480 )
    ( 1396, 42.181 )
    ( 1397, 42.119 )
    ( 1398, 42.055 )
    ( 1399, 41.990 )
    ( 1400, 41.933 )
    ( 1401, 41.633 )
    ( 1402, 41.332 )
    ( 1403, 41.244 )
    ( 1404, 41.147 )
    ( 1405, 40.879 )
    ( 1406, 40.582 )
    ( 1407, 40.418 )
    ( 1408, 40.222 )
    ( 1409, 39.921 )
    ( 1410, 39.621 )
    ( 1411, 39.422 )
    ( 1412, 39.121 )
    ( 1413, 39.094 )
    ( 1414, 39.179 )
    ( 1415, 39.134 )
    ( 1416, 39.239 )
    ( 1417, 39.309 )
    ( 1418, 39.367 )
    ( 1419, 39.309 )
    ( 1420, 39.320 )
    ( 1421, 39.342 )
    ( 1422, 39.285 )
    ( 1423, 39.344 )
    ( 1424, 39.287 )
    ( 1425, 39.229 )
    ( 1426, 39.251 )
    ( 1427, 39.271 )
    ( 1428, 39.267 )
    ( 1429, 39.256 )
    ( 1430, 39.271 )
    ( 1431, 39.219 )
    ( 1432, 39.190 )
    ( 1433, 39.132 )
    ( 1434, 38.834 )
    ( 1435, 38.744 )
    ( 1436, 38.769 )
    ( 1437, 38.798 )
    ( 1438, 38.587 )
    ( 1439, 38.286 )
    ( 1440, 37.992 )
    ( 1441, 37.781 )
    ( 1442, 37.489 )
    ( 1443, 37.188 )
    ( 1444, 37.043 )
    ( 1445, 36.861 )
    ( 1446, 36.561 )
    ( 1447, 36.260 )
    ( 1448, 36.024 )
    ( 1449, 35.723 )
    ( 1450, 35.550 )
    ( 1451, 35.374 )
    ( 1452, 35.073 )
    ( 1453, 34.877 )
    ( 1454, 34.578 )
    ( 1455, 34.487 )
    ( 1456, 34.187 )
    ( 1457, 34.097 )
    ( 1458, 34.158 )
    ( 1459, 34.076 )
    ( 1460, 34.019 )
    ( 1461, 33.773 )
    ( 1462, 33.507 )
    ( 1463, 33.410 )
    ( 1464, 33.313 )
    ( 1465, 33.297 )
    ( 1466, 33.200 )
    ( 1467, 33.147 )
    ( 1468, 32.958 )
    ( 1469, 32.683 )
    ( 1470, 32.519 )
    ( 1471, 32.219 )
    ( 1472, 31.918 )
    ( 1473, 31.724 )
    ( 1474, 31.500 )
    ( 1475, 31.416 )
    ( 1476, 31.185 )
    ( 1477, 30.884 )
    ( 1478, 30.588 )
    ( 1479, 30.451 )
    ( 1480, 30.357 )
    ( 1481, 30.254 )
    ( 1482, 29.965 )
    ( 1483, 29.666 )
    ( 1484, 29.457 )
    ( 1485, 29.164 )
    ( 1486, 28.884 )
    ( 1487, 28.583 )
    ( 1488, 28.486 )
    ( 1489, 28.510 )
    ( 1490, 28.226 )
    ( 1491, 27.930 )
    ( 1492, 27.648 )
    ( 1493, 27.352 )
    ( 1494, 27.051 )
    ( 1495, 26.834 )
    ( 1496, 26.578 )
    ( 1497, 26.277 )
    ( 1498, 26.167 )
    ( 1499, 25.987 )
    ( 1500, 25.686 )
    ( 1501, 25.442 )
    ( 1502, 25.211 )
    ( 1503, 24.992 )
    ( 1504, 24.759 )
    ( 1505, 24.461 )
    ( 1506, 24.224 )
    ( 1507, 23.936 )
    ( 1508, 23.658 )
    ( 1509, 23.357 )
    ( 1510, 23.056 )
    ( 1511, 23.243 )
    ( 1512, 23.486 )
    ( 1513, 23.597 )
    ( 1514, 23.696 )
    ( 1515, 23.713 )
    ( 1516, 23.776 )
    ( 1517, 23.778 )
    ( 1518, 23.793 )
    ( 1519, 23.793 )
    ( 1520, 24.015 )
    ( 1521, 24.016 )
    ( 1522, 24.104 )
    ( 1523, 24.167 )
    ( 1524, 24.355 )
    ( 1525, 24.368 )
    ( 1526, 24.436 )
    ( 1527, 24.451 )
    ( 1528, 24.562 )
    ( 1529, 24.415 )
    ( 1530, 24.318 )
    ( 1531, 24.017 )
    ( 1532, 23.740 )
    ( 1533, 23.439 )
    ( 1534, 23.424 )
    ( 1535, 23.153 )
    ( 1536, 22.916 )
    ( 1537, 22.619 )
    ( 1538, 22.346 )
    ( 1539, 22.116 )
    ( 1540, 21.844 )
    ( 1541, 21.543 )
    ( 1542, 21.263 )
    ( 1543, 21.315 )
    ( 1544, 21.015 )
    ( 1545, 20.714 )
    ( 1546, 20.427 )
    ( 1547, 20.133 )
    ( 1548, 19.902 )
    ( 1549, 19.603 )
    ( 1550, 19.457 )
    ( 1551, 19.156 )
    ( 1552, 19.111 )
    ( 1553, 18.906 )
    ( 1554, 18.605 )
    ( 1555, 18.397 )
    ( 1556, 18.111 )
    ( 1557, 17.826 )
    ( 1558, 17.729 )
    ( 1559, 17.525 )
    ( 1560, 17.315 )
    ( 1561, 17.119 )
    ( 1562, 16.954 )
    ( 1563, 16.653 )
    ( 1564, 16.556 )
    ( 1565, 16.256 )
    ( 1566, 16.080 )
    ( 1567, 15.864 )
    ( 1568, 15.582 )
    ( 1569, 15.311 )
    ( 1570, 15.010 )
    ( 1571, 14.864 )
    ( 1572, 14.633 )
    ( 1573, 14.358 )
    ( 1574, 14.147 )
    ( 1575, 13.936 )
    ( 1576, 13.931 )
    ( 1577, 13.850 )
    ( 1578, 13.753 )
    ( 1579, 13.497 )
    ( 1580, 13.208 )
    ( 1581, 13.054 )
    ( 1582, 12.753 )
    ( 1583, 12.641 )
    ( 1584, 12.516 )
    ( 1585, 12.659 )
    ( 1586, 12.857 )
    ( 1587, 12.874 )
    ( 1588, 13.073 )
    ( 1589, 13.333 )
    ( 1590, 13.570 )
    ( 1591, 13.793 )
    ( 1592, 14.016 )
    ( 1593, 14.244 )
    ( 1594, 14.457 )
    ( 1595, 14.679 )
    ( 1596, 14.899 )
    ( 1597, 15.173 )
    ( 1598, 15.392 )
    ( 1599, 15.610 )
    ( 1600, 15.790 )
    ( 1601, 16.098 )
    ( 1602, 16.326 )
    ( 1603, 16.527 )
    ( 1604, 16.713 )
    ( 1605, 16.958 )
    ( 1606, 17.135 )
    ( 1607, 17.311 )
    ( 1608, 17.602 )
    ( 1609, 17.783 )
    ( 1610, 17.970 )
    ( 1611, 18.149 )
    ( 1612, 18.336 )
    ( 1613, 18.605 )
    ( 1614, 18.935 )
    ( 1615, 19.207 )
    ( 1616, 19.427 )
    ( 1617, 19.616 )
    ( 1618, 19.874 )
    ( 1619, 20.119 )
    ( 1620, 20.305 )
    ( 1621, 20.430 )
    ( 1622, 20.594 )
    ( 1623, 20.774 )
    ( 1624, 20.707 )
    ( 1625, 20.654 )
    ( 1626, 20.659 )
    ( 1627, 20.534 )
    ( 1628, 20.493 )
    ( 1629, 20.470 )
    ( 1630, 20.419 )
    ( 1631, 20.294 )
    ( 1632, 20.345 )
    ( 1633, 20.536 )
    ( 1634, 20.638 )
    ( 1635, 20.590 )
    ( 1636, 20.532 )
    ( 1637, 20.414 )
    ( 1638, 20.289 )
    ( 1639, 20.034 )
    ( 1640, 19.746 )
    ( 1641, 19.466 )
    ( 1642, 19.165 )
    ( 1643, 18.865 )
    ( 1644, 18.745 )
    ( 1645, 18.444 )
    ( 1646, 18.143 )
    ( 1647, 17.850 )
    ( 1648, 17.550 )
    ( 1649, 17.510 )
    ( 1650, 17.348 )
    ( 1651, 17.047 )
    ( 1652, 16.922 )
    ( 1653, 16.799 )
    ( 1654, 16.811 )
    ( 1655, 16.800 )
    ( 1656, 16.786 )
    ( 1657, 16.689 )
    ( 1658, 16.544 )
    ( 1659, 16.243 )
    ( 1660, 16.173 )
    ( 1661, 15.901 )
    ( 1662, 15.601 )
    ( 1663, 15.300 )
    ( 1664, 15.377 )
    ( 1665, 15.327 )
    ( 1666, 15.425 )
    ( 1667, 15.522 )
    ( 1668, 15.619 )
    ( 1669, 15.720 )
    ( 1670, 15.973 )
    ( 1671, 16.072 )
    ( 1672, 16.361 )
    ( 1673, 16.533 )
    ( 1674, 16.687 )
    ( 1675, 16.784 )
    ( 1676, 16.965 )
    ( 1677, 17.062 )
    ( 1678, 17.147 )
    ( 1679, 17.226 )
    ( 1680, 17.369 )
    ( 1681, 17.454 )
    ( 1682, 17.572 )
    ( 1683, 17.758 )
    ( 1684, 17.881 )
    ( 1685, 17.854 )
    ( 1686, 17.796 )
    ( 1687, 17.781 )
    ( 1688, 17.739 )
    ( 1689, 17.637 )
    ( 1690, 17.524 )
    ( 1691, 17.423 )
    ( 1692, 17.298 )
    ( 1693, 17.175 )
    ( 1694, 17.050 )
    ( 1695, 17.246 )
    ( 1696, 17.430 )
    ( 1697, 17.575 )
    ( 1698, 17.700 )
    ( 1699, 18.149 )
    ( 1700, 18.505 )
    ( 1701, 18.910 )
    ( 1702, 19.268 )
    ( 1703, 19.539 )
    ( 1704, 19.815 )
    ( 1705, 20.052 )
    ( 1706, 20.268 )
    ( 1707, 20.448 )
    ( 1708, 20.652 )
    ( 1709, 20.801 )
    ( 1710, 20.990 )
    ( 1711, 21.115 )
    ( 1712, 21.240 )
    ( 1713, 21.390 )
    ( 1714, 21.516 )
    ( 1715, 21.672 )
    ( 1716, 21.813 )
    ( 1717, 21.939 )
    ( 1718, 22.064 )
    ( 1719, 22.150 )
    ( 1720, 22.251 )
    ( 1721, 22.126 )
    ( 1722, 22.168 )
    ( 1723, 22.043 )
    ( 1724, 22.060 )
    ( 1725, 22.318 )
    ( 1726, 22.603 )
    ( 1727, 22.844 )
    ( 1728, 23.077 )
    ( 1729, 23.462 )
    ( 1730, 23.815 )
    ( 1731, 24.061 )
    ( 1732, 24.302 )
    ( 1733, 24.611 )
    ( 1734, 24.877 )
    ( 1735, 25.097 )
    ( 1736, 25.492 )
    ( 1737, 25.836 )
    ( 1738, 26.086 )
    ( 1739, 26.306 )
    ( 1740, 26.563 )
    ( 1741, 26.849 )
    ( 1742, 27.082 )
    ( 1743, 27.258 )
    ( 1744, 27.458 )
    ( 1745, 27.693 )
    ( 1746, 27.997 )
    ( 1747, 28.248 )
    ( 1748, 28.516 )
    ( 1749, 28.771 )
    ( 1750, 29.027 )
    ( 1751, 29.284 )
    ( 1752, 29.484 )
    ( 1753, 29.460 )
    ( 1754, 29.508 )
    ( 1755, 29.450 )
    ( 1756, 29.489 )
    ( 1757, 29.511 )
    ( 1758, 29.510 )
    ( 1759, 29.482 )
    ( 1760, 29.186 )
    ( 1761, 28.971 )
    ( 1762, 28.734 )
    ( 1763, 28.548 )
    ( 1764, 28.353 )
    ( 1765, 28.258 )
    ( 1766, 27.958 )
    ( 1767, 27.706 )
    ( 1768, 27.424 )
    ( 1769, 27.297 )
    ( 1770, 27.151 )
    ( 1771, 26.850 )
    ( 1772, 26.772 )
    ( 1773, 26.503 )
    ( 1774, 26.202 )
    ( 1775, 25.972 )
    ( 1776, 25.950 )
    ( 1777, 26.004 )
    ( 1778, 25.705 )
    ( 1779, 25.405 )
    ( 1780, 25.138 )
    ( 1781, 25.106 )
    ( 1782, 25.128 )
    ( 1783, 25.063 )
    ( 1784, 24.917 )
    ( 1785, 24.617 )
    ( 1786, 24.321 )
    ( 1787, 24.020 )
    ( 1788, 23.923 )
    ( 1789, 23.826 )
    ( 1790, 23.848 )
    ( 1791, 23.730 )
    ( 1792, 23.458 )
    ( 1793, 23.157 )
    ( 1794, 23.011 )
    ( 1795, 22.710 )
    ( 1796, 22.719 )
    ( 1797, 22.623 )
    ( 1798, 22.476 )
    ( 1799, 22.269 )
    ( 1800, 21.969 )
    ( 1801, 21.669 )
    ( 1802, 21.373 )
    ( 1803, 21.072 )
    ( 1804, 20.771 )
    ( 1805, 20.930 )
    ( 1806, 21.076 )
    ( 1807, 21.159 )
    ( 1808, 21.180 )
    ( 1809, 21.180 )
    ( 1810, 21.224 )
    ( 1811, 21.297 )
    ( 1812, 21.303 )
    ( 1813, 21.390 )
    ( 1814, 21.439 )
    ( 1815, 21.488 )
    ( 1816, 21.648 )
    ( 1817, 21.731 )
    ( 1818, 21.779 )
    ( 1819, 21.935 )
    ( 1820, 22.110 )
    ( 1821, 22.207 )
    ( 1822, 22.339 )
    ( 1823, 22.344 )
    ( 1824, 22.344 )
    ( 1825, 22.344 )
    ( 1826, 22.358 )
    ( 1827, 22.377 )
    ( 1828, 22.377 )
    ( 1829, 22.378 )
    ( 1830, 22.427 )
    ( 1831, 22.427 )
    ( 1832, 22.514 )
    ( 1833, 22.534 )
    ( 1834, 22.534 )
    ( 1835, 22.557 )
    ( 1836, 22.559 )
    ( 1837, 22.559 )
    ( 1838, 22.902 )
    ( 1839, 23.132 )
    ( 1840, 23.354 )
    ( 1841, 23.630 )
    ( 1842, 23.852 )
    ( 1843, 24.219 )
    ( 1844, 24.457 )
    ( 1845, 24.712 )
    ( 1846, 24.947 )
    ( 1847, 25.220 )
    ( 1848, 25.442 )
    ( 1849, 25.494 )
    ( 1850, 25.556 )
    ( 1851, 25.556 )
    ( 1852, 25.594 )
    ( 1853, 25.603 )
    ( 1854, 25.774 )
    ( 1855, 25.776 )
    ( 1856, 25.776 )
    ( 1857, 25.821 )
    ( 1858, 25.834 )
    ( 1859, 25.834 )
    ( 1860, 26.123 )
    ( 1861, 26.493 )
    ( 1862, 26.856 )
    ( 1863, 27.258 )
    ( 1864, 27.600 )
    ( 1865, 27.876 )
    ( 1866, 28.152 )
    ( 1867, 28.451 )
    ( 1868, 28.673 )
    ( 1869, 28.895 )
    ( 1870, 29.291 )
    ( 1871, 29.644 )
    ( 1872, 29.866 )
    ( 1873, 30.117 )
    ( 1874, 30.354 )
    ( 1875, 30.644 )
    ( 1876, 30.925 )
    ( 1877, 31.159 )
    ( 1878, 31.431 )
    ( 1879, 31.656 )
    ( 1880, 31.877 )
    ( 1881, 32.100 )
    ( 1882, 32.493 )
    ( 1883, 32.885 )
    ( 1884, 33.325 )
    ( 1885, 33.625 )
    ( 1886, 33.918 )
    ( 1887, 34.211 )
    ( 1888, 34.560 )
    ( 1889, 34.836 )
    ( 1890, 34.888 )
    ( 1891, 34.960 )
    ( 1892, 34.961 )
    ( 1893, 35.211 )
    ( 1894, 35.420 )
    ( 1895, 35.500 )
    ( 1896, 35.588 )
    ( 1897, 35.604 )
    ( 1898, 35.755 )
    ( 1899, 35.984 )
    ( 1900, 35.984 )
    ( 1901, 35.984 )
    ( 1902, 36.057 )
    ( 1903, 36.057 )
    ( 1904, 36.119 )
    ( 1905, 36.124 )
    ( 1906, 36.400 )
    ( 1907, 36.677 )
    ( 1908, 37.069 )
    ( 1909, 37.345 )
    ( 1910, 37.627 )
    ( 1911, 37.903 )
    ( 1912, 37.958 )
    ( 1913, 37.958 )
    ( 1914, 37.958 )
    ( 1915, 38.169 )
    ( 1916, 38.315 )
    ( 1917, 38.473 )
    ( 1918, 38.480 )
    ( 1919, 38.507 )
    ( 1920, 38.507 )
    ( 1921, 38.653 )
    ( 1922, 38.710 )
    ( 1923, 38.710 )
    ( 1924, 38.783 )
    ( 1925, 38.799 )
    ( 1926, 38.881 )
    ( 1927, 38.908 )
    ( 1928, 38.928 )
    ( 1929, 38.928 )
    ( 1930, 38.971 )
    ( 1931, 38.971 )
    ( 1932, 39.036 )
    ( 1933, 39.036 )
    ( 1934, 39.105 )
    ( 1935, 39.105 )
    ( 1936, 39.105 )
    ( 1937, 39.184 )
    ( 1938, 39.184 )
    ( 1939, 39.227 )
    ( 1940, 39.229 )
    ( 1941, 39.229 )
    ( 1942, 39.229 )
    ( 1943, 39.244 )
    ( 1944, 39.332 )
    ( 1945, 39.528 )
    ( 1946, 39.732 )
    ( 1947, 39.878 )
    ( 1948, 40.043 )
    ( 1949, 40.094 )
    ( 1950, 40.094 )
    ( 1951, 40.106 )
    ( 1952, 40.280 )
    ( 1953, 40.429 )
    ( 1954, 40.642 )
    ( 1955, 40.723 )
    ( 1956, 40.922 )
    ( 1957, 40.947 )
    ( 1958, 40.953 )
    ( 1959, 40.953 )
    ( 1960, 41.016 )
    ( 1961, 41.078 )
    ( 1962, 41.384 )
    ( 1963, 41.385 )
    ( 1964, 41.447 )
    ( 1965, 41.593 )
    ( 1966, 41.655 )
    ( 1967, 41.709 )
    ( 1968, 41.954 )
    ( 1969, 42.187 )
    ( 1970, 42.421 )
    ( 1971, 42.643 )
    ( 1972, 42.883 )
    ( 1973, 43.173 )
    ( 1974, 43.450 )
    ( 1975, 43.754 )
    ( 1976, 44.014 )
    ( 1977, 44.271 )
    ( 1978, 44.560 )
    ( 1979, 44.922 )
    ( 1980, 45.321 )
    ( 1981, 45.719 )
    ( 1982, 46.133 )
    ( 1983, 46.410 )
    ( 1984, 46.690 )
    ( 1985, 46.930 )
    ( 1986, 47.151 )
    ( 1987, 47.408 )
    ( 1988, 47.708 )
    ( 1989, 47.930 )
    ( 1990, 48.152 )
    ( 1991, 48.375 )
    ( 1992, 48.411 )
    ( 1993, 48.450 )
    ( 1994, 48.509 )
    ( 1995, 48.509 )
    ( 1996, 48.509 )
    ( 1997, 48.587 )
    ( 1998, 48.605 )
    ( 1999, 48.626 )
    ( 2000, 48.643 )
    ( 2001, 48.643 )
    ( 2002, 48.643 )
    ( 2003, 48.667 )
    ( 2004, 48.734 )
    ( 2005, 48.734 )
    ( 2006, 48.734 )
    ( 2007, 48.811 )
    ( 2008, 48.840 )
    ( 2009, 48.855 )
    ( 2010, 48.879 )
    ( 2011, 49.117 )
    ( 2012, 49.180 )
    ( 2013, 49.255 )
    ( 2014, 49.545 )
    ( 2015, 49.825 )
    ( 2016, 50.198 )
    ( 2017, 50.475 )
    ( 2018, 50.867 )
    ( 2019, 51.088 )
    ( 2020, 51.311 )
    ( 2021, 51.594 )
    ( 2022, 51.987 )
    ( 2023, 52.376 )
    ( 2024, 52.598 )
    ( 2025, 52.824 )
    ( 2026, 53.117 )
    ( 2027, 53.476 )
    ( 2028, 53.835 )
    ( 2029, 54.173 )
    ( 2030, 54.194 )
    ( 2031, 54.194 )
    ( 2032, 54.197 )
    ( 2033, 54.367 )
    ( 2034, 54.539 )
    ( 2035, 54.700 )
    ( 2036, 54.910 )
    ( 2037, 54.911 )
    ( 2038, 54.911 )
    ( 2039, 54.912 )
    ( 2040, 54.922 )
    ( 2041, 54.925 )
    ( 2042, 54.935 )
    ( 2043, 54.987 )
    ( 2044, 54.988 )
    ( 2045, 54.998 )
    ( 2046, 55.008 )
    ( 2047, 55.008 )
    ( 2048, 55.008 )
    ( 2049, 55.008 )
    ( 2050, 55.056 )
    ( 2051, 55.244 )
    ( 2052, 55.390 )
    ( 2053, 55.593 )
    ( 2054, 55.655 )
    ( 2055, 56.074 )
    ( 2056, 56.470 )
    ( 2057, 56.692 )
    ( 2058, 56.969 )
    ( 2059, 57.293 )
    ( 2060, 57.587 )
    ( 2061, 57.809 )
    ( 2062, 58.033 )
    ( 2063, 58.193 )
    ( 2064, 58.426 )
    ( 2065, 58.633 )
    ( 2066, 58.815 )
    ( 2067, 58.977 )
    ( 2068, 59.192 )
    ( 2069, 59.408 )
    ( 2070, 59.555 )
    ( 2071, 59.701 )
    ( 2072, 59.862 )
    ( 2073, 59.885 )
    ( 2074, 60.058 )
    ( 2075, 60.261 )
    ( 2076, 60.407 )
    ( 2077, 60.429 )
    ( 2078, 60.456 )
    ( 2079, 60.471 )
    ( 2080, 60.486 )
    ( 2081, 60.486 )
    ( 2082, 60.491 )
    ( 2083, 60.556 )
    ( 2084, 60.556 )
    ( 2085, 60.898 )
    ( 2086, 61.310 )
    ( 2087, 61.673 )
    ( 2088, 62.003 )
    ( 2089, 62.246 )
    ( 2090, 62.500 )
    ( 2091, 62.722 )
    ( 2092, 62.994 )
    ( 2093, 63.216 )
    ( 2094, 63.439 )
    ( 2095, 63.700 )
    ( 2096, 63.923 )
    ( 2097, 64.157 )
    ( 2098, 64.543 )
    ( 2099, 64.886 )
    ( 2100, 65.245 )
    ( 2101, 65.605 )
    ( 2102, 65.870 )
    ( 2103, 66.106 )
    ( 2104, 66.341 )
    ( 2105, 66.684 )
    ( 2106, 67.026 )
    ( 2107, 67.415 )
    ( 2108, 67.651 )
    ( 2109, 67.873 )
    ( 2110, 68.105 )
    ( 2111, 68.371 )
    ( 2112, 68.594 )
    ( 2113, 68.870 )
    ( 2114, 69.028 )
    ( 2115, 69.175 )
    ( 2116, 69.181 )
    ( 2117, 69.184 )
    ( 2118, 69.212 )
    ( 2119, 69.218 )
    ( 2120, 69.505 )
    ( 2121, 69.529 )
    ( 2122, 69.534 )
    ( 2123, 69.547 )
    ( 2124, 69.823 )
    ( 2125, 69.897 )
    ( 2126, 69.901 )
    ( 2127, 69.905 )
    ( 2128, 69.929 )
    ( 2129, 69.965 )
    ( 2130, 69.965 )
    ( 2131, 70.111 )
    ( 2132, 70.258 )
    ( 2133, 70.258 )
    ( 2134, 70.258 )
    ( 2135, 70.258 )
    ( 2136, 70.544 )
    ( 2137, 70.832 )
    ( 2138, 71.108 )
    ( 2139, 71.447 )
    ( 2140, 71.739 )
    ( 2141, 72.023 )
    ( 2142, 72.328 )
    ( 2143, 72.642 )
    ( 2144, 72.918 )
    ( 2145, 73.210 )
    ( 2146, 73.500 )
    ( 2147, 73.722 )
    ( 2148, 73.989 )
    ( 2149, 74.211 )
    ( 2150, 74.241 )
    ( 2151, 74.350 )
    ( 2152, 74.430 )
    ( 2153, 74.431 )
    ( 2154, 74.431 )
    ( 2155, 74.431 )
    ( 2156, 74.431 )
    ( 2157, 74.431 )
    ( 2158, 74.439 )
    ( 2159, 74.488 )
    ( 2160, 74.551 )
    ( 2161, 74.626 )
    ( 2162, 74.628 )
    ( 2163, 74.646 )
    ( 2164, 74.661 )
    ( 2165, 74.766 )
    ( 2166, 74.867 )
    ( 2167, 74.966 )
    ( 2168, 74.908 )
    ( 2169, 74.904 )
    ( 2170, 74.885 )
    ( 2171, 74.827 )
    ( 2172, 74.727 )
    ( 2173, 74.640 )
    ( 2174, 74.523 )
    ( 2175, 74.405 )
    ( 2176, 74.283 )
    ( 2177, 74.159 )
    ( 2178, 74.060 )
    ( 2179, 73.993 )
    ( 2180, 73.927 )
    ( 2181, 73.802 )
    ( 2182, 73.690 )
    ( 2183, 73.572 )
    ( 2184, 73.613 )
    ( 2185, 73.765 )
    ( 2186, 73.866 )
    ( 2187, 73.907 )
    ( 2188, 73.804 )
    ( 2189, 73.679 )
    ( 2190, 73.565 )
    ( 2191, 73.502 )
    ( 2192, 73.451 )
    ( 2193, 73.328 )
    ( 2194, 73.213 )
    ( 2195, 73.088 )
    ( 2196, 72.993 )
    ( 2197, 72.892 )
    ( 2198, 72.799 )
    ( 2199, 72.701 )
    ( 2200, 72.576 )
    ( 2201, 72.516 )
    ( 2202, 72.391 )
    ( 2203, 72.266 )
    ( 2204, 72.167 )
    ( 2205, 72.126 )
    ( 2206, 72.052 )
    ( 2207, 71.969 )
    ( 2208, 71.844 )
    ( 2209, 71.796 )
    ( 2210, 71.783 )
    ( 2211, 71.768 )
    ( 2212, 71.466 )
    ( 2213, 71.277 )
    ( 2214, 71.050 )
    ( 2215, 70.749 )
    ( 2216, 70.472 )
    ( 2217, 70.559 )
    ( 2218, 70.462 )
    ( 2219, 70.167 )
    ( 2220, 69.874 )
    ( 2221, 69.728 )
    ( 2222, 69.496 )
    ( 2223, 69.195 )
    ( 2224, 68.895 )
    ( 2225, 68.633 )
    ( 2226, 68.353 )
    ( 2227, 68.053 )
    ( 2228, 68.077 )
    ( 2229, 67.775 )
    ( 2230, 67.505 )
    ( 2231, 67.234 )
    ( 2232, 67.070 )
    ( 2233, 67.070 )
    ( 2234, 66.974 )
    ( 2235, 66.673 )
    ( 2236, 66.372 )
    ( 2237, 66.135 )
    ( 2238, 65.919 )
    ( 2239, 65.716 )
    ( 2240, 65.485 )
    ( 2241, 65.212 )
    ( 2242, 64.933 )
    ( 2243, 64.632 )
    ( 2244, 64.330 )
    ( 2245, 64.193 )
    ( 2246, 64.111 )
    ( 2247, 63.965 )
    ( 2248, 63.667 )
    ( 2249, 63.480 )
    ( 2250, 63.191 )
    ( 2251, 62.892 )
    ( 2252, 62.672 )
    ( 2253, 62.371 )
    ( 2254, 62.078 )
    ( 2255, 61.777 )
    ( 2256, 61.476 )
    ( 2257, 61.452 )
    ( 2258, 61.505 )
    ( 2259, 61.409 )
    ( 2260, 61.111 )
    ( 2261, 60.810 )
    ( 2262, 60.509 )
    ( 2263, 60.208 )
    ( 2264, 60.051 )
    ( 2265, 59.762 )
    ( 2266, 59.699 )
    ( 2267, 59.398 )
    ( 2268, 59.470 )
    ( 2269, 59.273 )
    ( 2270, 58.974 )
    ( 2271, 58.897 )
    ( 2272, 58.660 )
    ( 2273, 58.360 )
    ( 2274, 58.101 )
    ( 2275, 57.833 )
    ( 2276, 57.669 )
    ( 2277, 57.473 )
    ( 2278, 57.242 )
    ( 2279, 57.155 )
    ( 2280, 56.854 )
    ( 2281, 56.565 )
    ( 2282, 56.340 )
    ( 2283, 56.109 )
    ( 2284, 55.900 )
    ( 2285, 55.856 )
    ( 2286, 55.555 )
    ( 2287, 55.259 )
    ( 2288, 55.141 )
    ( 2289, 54.995 )
    ( 2290, 54.694 )
    ( 2291, 54.498 )
    ( 2292, 54.197 )
    ( 2293, 54.051 )
    ( 2294, 54.108 )
    ( 2295, 54.093 )
    ( 2296, 53.826 )
    ( 2297, 53.524 )
    ( 2298, 53.238 )
    ( 2299, 52.948 )
    ( 2300, 52.760 )
    ( 2301, 52.529 )
    ( 2302, 52.229 )
    ( 2303, 52.189 )
    ( 2304, 51.959 )
    ( 2305, 51.661 )
    ( 2306, 51.395 )
    ( 2307, 51.111 )
    ( 2308, 50.811 )
    ( 2309, 50.510 )
    ( 2310, 50.212 )
    ( 2311, 49.912 )
    ( 2312, 49.884 )
    ( 2313, 49.787 )
    ( 2314, 49.487 )
    ( 2315, 49.250 )
    ( 2316, 48.979 )
    ( 2317, 48.678 )
    ( 2318, 48.581 )
    ( 2319, 48.279 )
    ( 2320, 48.086 )
    ( 2321, 47.908 )
    ( 2322, 47.821 )
    ( 2323, 47.675 )
    ( 2324, 47.405 )
    ( 2325, 47.104 )
    ( 2326, 46.834 )
    ( 2327, 46.636 )
    ( 2328, 46.411 )
    ( 2329, 46.190 )
    ( 2330, 46.049 )
    ( 2331, 45.768 )
    ( 2332, 45.680 )
    ( 2333, 45.566 )
    ( 2334, 45.329 )
    ( 2335, 45.146 )
    ( 2336, 44.847 )
    ( 2337, 44.701 )
    ( 2338, 44.545 )
    ( 2339, 44.448 )
    ( 2340, 44.351 )
    ( 2341, 44.050 )
    ( 2342, 43.750 )
    ( 2343, 43.558 )
    ( 2344, 43.256 )
    ( 2345, 42.956 )
    ( 2346, 42.975 )
    ( 2347, 42.939 )
    ( 2348, 42.911 )
    ( 2349, 42.853 )
    ( 2350, 42.839 )
    ( 2351, 42.795 )
    ( 2352, 42.777 )
    ( 2353, 42.753 )
    ( 2354, 42.971 )
    ( 2355, 43.165 )
    ( 2356, 43.301 )
    ( 2357, 43.437 )
    ( 2358, 43.595 )
    ( 2359, 43.725 )
    ( 2360, 43.697 )
    ( 2361, 43.815 )
    ( 2362, 43.913 )
    ( 2363, 44.027 )
    ( 2364, 44.112 )
    ( 2365, 44.105 )
    ( 2366, 44.141 )
    ( 2367, 44.223 )
    ( 2368, 44.314 )
    ( 2369, 44.332 )
    ( 2370, 44.318 )
    ( 2371, 44.348 )
    ( 2372, 44.369 )
    ( 2373, 44.362 )
    ( 2374, 44.062 )
    ( 2375, 43.777 )
    ( 2376, 43.476 )
    ( 2377, 43.202 )
    ( 2378, 42.902 )
    ( 2379, 42.613 )
    ( 2380, 42.312 )
    ( 2381, 42.116 )
    ( 2382, 41.920 )
    ( 2383, 41.627 )
    ( 2384, 41.327 )
    ( 2385, 41.039 )
    ( 2386, 40.892 )
    ( 2387, 40.599 )
    ( 2388, 40.369 )
    ( 2389, 40.272 )
    ( 2390, 40.260 )
    ( 2391, 40.188 )
    ( 2392, 40.042 )
    ( 2393, 39.867 )
    ( 2394, 39.595 )
    ( 2395, 39.602 )
    ( 2396, 39.391 )
    ( 2397, 39.130 )
    ( 2398, 38.830 )
    ( 2399, 38.599 )
    ( 2400, 38.314 )
    ( 2401, 38.103 )
    ( 2402, 37.848 )
    ( 2403, 37.703 )
    ( 2404, 37.561 )
    ( 2405, 37.276 )
    ( 2406, 37.050 )
    ( 2407, 36.750 )
    ( 2408, 36.449 )
    ( 2409, 36.148 )
    ( 2410, 35.847 )
    ( 2411, 35.617 )
    ( 2412, 35.319 )
    ( 2413, 35.347 )
    ( 2414, 35.309 )
    ( 2415, 35.230 )
    ( 2416, 34.931 )
    ( 2417, 34.673 )
    ( 2418, 34.372 )
    ( 2419, 34.120 )
    ( 2420, 33.819 )
    ( 2421, 33.522 )
    ( 2422, 33.221 )
    ( 2423, 32.934 )
    ( 2424, 32.836 )
    ( 2425, 32.536 )
    ( 2426, 32.339 )
    ( 2427, 32.148 )
    ( 2428, 31.961 )
    ( 2429, 31.765 )
    ( 2430, 31.464 )
    ( 2431, 31.163 )
    ( 2432, 30.934 )
    ( 2433, 30.634 )
    ( 2434, 30.488 )
    ( 2435, 30.277 )
    ( 2436, 30.029 )
    ( 2437, 30.053 )
    ( 2438, 29.865 )
    ( 2439, 29.953 )
    ( 2440, 29.828 )
    ( 2441, 29.996 )
    ( 2442, 30.159 )
    ( 2443, 30.284 )
    ( 2444, 30.441 )
    ( 2445, 30.593 )
    ( 2446, 30.779 )
    ( 2447, 30.964 )
    ( 2448, 30.839 )
    ( 2449, 30.791 )
    ( 2450, 30.737 )
    ( 2451, 30.720 )
    ( 2452, 30.693 )
    ( 2453, 30.686 )
    ( 2454, 30.719 )
    ( 2455, 30.717 )
    ( 2456, 30.840 )
    ( 2457, 30.826 )
    ( 2458, 30.868 )
    ( 2459, 30.862 )
    ( 2460, 30.920 )
    ( 2461, 30.978 )
    ( 2462, 30.920 )
    ( 2463, 30.892 )
    ( 2464, 31.014 )
    ( 2465, 31.136 )
    ( 2466, 31.233 )
    ( 2467, 31.336 )
    ( 2468, 31.461 )
    ( 2469, 31.571 )
    ( 2470, 31.720 )
    ( 2471, 31.883 )
    ( 2472, 32.029 )
    ( 2473, 32.117 )
    ( 2474, 32.171 )
    ( 2475, 32.047 )
    ( 2476, 31.922 )
    ( 2477, 31.797 )
    ( 2478, 32.011 )
    ( 2479, 32.195 )
    ( 2480, 31.894 )
    ( 2481, 31.861 )
    ( 2482, 31.916 )
    ( 2483, 31.947 )
    ( 2484, 31.967 )
    ( 2485, 31.909 )
    ( 2486, 31.909 )
    ( 2487, 31.902 )
    ( 2488, 31.662 )
    ( 2489, 31.361 )
    ( 2490, 31.060 )
    ( 2491, 30.914 )
    ( 2492, 30.771 )
    ( 2493, 30.471 )
    ( 2494, 30.189 )
    ( 2495, 29.888 )
    ( 2496, 29.587 )
    ( 2497, 29.286 )
    ( 2498, 29.094 )
    ( 2499, 28.972 )
    ( 2500, 28.906 )
    ( 2501, 28.711 )
    ( 2502, 28.529 )
    ( 2503, 28.389 )
    ( 2504, 28.243 )
    ( 2505, 28.170 )
    ( 2506, 28.194 )
    ( 2507, 28.097 )
    ( 2508, 27.796 )
    ( 2509, 27.563 )
    ( 2510, 27.298 )
    ( 2511, 27.066 )
    ( 2512, 26.805 )
    ( 2513, 26.575 )
    ( 2514, 26.287 )
    ( 2515, 26.190 )
    ( 2516, 25.889 )
    ( 2517, 25.906 )
    ( 2518, 25.809 )
    ( 2519, 25.712 )
    ( 2520, 25.413 )
    ( 2521, 25.267 )
    ( 2522, 25.131 )
    ( 2523, 24.996 )
    ( 2524, 24.902 )
    ( 2525, 24.805 )
    ( 2526, 24.587 )
    ( 2527, 24.286 )
    ( 2528, 24.027 )
    ( 2529, 23.831 )
    ( 2530, 23.570 )
    ( 2531, 23.505 )
    ( 2532, 23.204 )
    ( 2533, 22.903 )
    ( 2534, 22.602 )
    ( 2535, 22.302 )
    ( 2536, 22.042 )
    ( 2537, 21.945 )
    ( 2538, 21.695 )
    ( 2539, 21.606 )
    ( 2540, 21.317 )
    ( 2541, 21.037 )
    ( 2542, 20.757 )
    ( 2543, 20.456 )
    ( 2544, 20.155 )
    ( 2545, 19.917 )
    ( 2546, 19.623 )
    ( 2547, 19.331 )
    ( 2548, 19.031 )
    ( 2549, 18.730 )
    ( 2550, 18.779 )
    ( 2551, 18.766 )
    ( 2552, 18.752 )
    ( 2553, 18.667 )
    ( 2554, 18.628 )
    ( 2555, 18.334 )
    ( 2556, 18.037 )
    ( 2557, 17.736 )
    ( 2558, 17.435 )
    ( 2559, 17.134 )
    ( 2560, 16.961 )
    ( 2561, 16.660 )
    ( 2562, 16.359 )
    ( 2563, 16.496 )
    ( 2564, 16.379 )
    ( 2565, 16.311 )
    ( 2566, 16.218 )
    ( 2567, 16.137 )
    ( 2568, 16.045 )
    ( 2569, 15.920 )
    ( 2570, 15.803 )
    ( 2571, 15.697 )
    ( 2572, 15.673 )
    ( 2573, 15.557 )
    ( 2574, 15.432 )
    ( 2575, 15.623 )
    ( 2576, 15.749 )
    ( 2577, 15.943 )
    ( 2578, 16.264 )
    ( 2579, 16.594 )
    ( 2580, 16.879 )
    ( 2581, 17.160 )
    ( 2582, 17.485 )
    ( 2583, 17.864 )
    ( 2584, 18.278 )
    ( 2585, 18.624 )
    ( 2586, 18.966 )
    ( 2587, 19.174 )
    ( 2588, 19.236 )
    ( 2589, 19.238 )
    ( 2590, 19.238 )
    ( 2591, 19.238 )
    ( 2592, 19.355 )
    ( 2593, 19.422 )
    ( 2594, 19.517 )
    ( 2595, 19.585 )
    ( 2596, 19.725 )
    ( 2597, 20.011 )
    ( 2598, 20.078 )
    ( 2599, 20.288 )
    ( 2600, 20.517 )
    ( 2601, 20.605 )
    ( 2602, 20.672 )
    ( 2603, 20.741 )
    ( 2604, 20.810 )
    ( 2605, 20.855 )
    ( 2606, 20.855 )
    ( 2607, 20.863 )
    ( 2608, 20.990 )
    ( 2609, 21.231 )
    ( 2610, 21.253 )
    ( 2611, 21.298 )
    ( 2612, 21.342 )
    ( 2613, 21.370 )
    ( 2614, 21.387 )
    ( 2615, 21.626 )
    ( 2616, 21.879 )
    ( 2617, 22.042 )
    ( 2618, 22.243 )
    ( 2619, 22.489 )
    ( 2620, 22.689 )
    ( 2621, 22.853 )
    ( 2622, 22.853 )
    ( 2623, 22.862 )
    ( 2624, 22.862 )
    ( 2625, 23.008 )
    ( 2626, 23.180 )
    ( 2627, 23.183 )
    ( 2628, 23.210 )
    ( 2629, 23.290 )
    ( 2630, 23.362 )
    ( 2631, 23.689 )
    ( 2632, 23.958 )
    ( 2633, 24.165 )
    ( 2634, 24.339 )
    ( 2635, 24.594 )
    ( 2636, 24.827 )
    ( 2637, 24.998 )
    ( 2638, 25.094 )
    ( 2639, 25.190 )
    ( 2640, 25.316 )
    ( 2641, 25.441 )
    ( 2642, 25.630 )
    ( 2643, 25.864 )
    ( 2644, 25.989 )
    ( 2645, 26.178 )
    ( 2646, 26.303 )
    ( 2647, 26.392 )
    ( 2648, 26.392 )
    ( 2649, 26.393 )
    ( 2650, 26.465 )
    ( 2651, 26.473 )
    ( 2652, 26.667 )
    ( 2653, 26.814 )
    ( 2654, 26.814 )
    ( 2655, 26.814 )
    ( 2656, 26.944 )
    ( 2657, 27.017 )
    ( 2658, 27.060 )
    ( 2659, 27.060 )
    ( 2660, 27.316 )
    ( 2661, 27.441 )
    ( 2662, 27.575 )
    ( 2663, 27.831 )
    ( 2664, 28.097 )
    ( 2665, 28.353 )
    ( 2666, 28.497 )
    ( 2667, 28.589 )
    ( 2668, 28.676 )
    ( 2669, 28.743 )
    ( 2670, 28.810 )
    ( 2671, 28.877 )
    ( 2672, 29.061 )
    ( 2673, 29.207 )
    ( 2674, 29.208 )
    ( 2675, 29.240 )
    ( 2676, 29.296 )
    ( 2677, 29.358 )
    ( 2678, 29.373 )
    ( 2679, 29.374 )
    ( 2680, 29.509 )
    ( 2681, 29.639 )
    ( 2682, 29.652 )
    ( 2683, 29.719 )
    ( 2684, 29.785 )
    ( 2685, 29.853 )
    ( 2686, 29.924 )
    ( 2687, 29.993 )
    ( 2688, 30.073 )
    ( 2689, 30.152 )
    ( 2690, 30.299 )
    ( 2691, 30.498 )
    ( 2692, 30.725 )
    ( 2693, 30.871 )
    ( 2694, 30.871 )
    ( 2695, 30.894 )
    ( 2696, 30.895 )
    ( 2697, 30.943 )
    ( 2698, 30.982 )
    ( 2699, 30.999 )
    ( 2700, 30.999 )
    ( 2701, 31.180 )
    ( 2702, 31.180 )
    ( 2703, 31.393 )
    ( 2704, 31.541 )
    ( 2705, 31.554 )
    ( 2706, 31.555 )
    ( 2707, 31.560 )
    ( 2708, 31.561 )
    ( 2709, 31.561 )
    ( 2710, 31.562 )
    ( 2711, 31.634 )
    ( 2712, 31.634 )
    ( 2713, 31.702 )
    ( 2714, 31.804 )
    ( 2715, 31.941 )
    ( 2716, 32.009 )
    ( 2717, 32.076 )
    ( 2718, 32.245 )
    ( 2719, 32.360 )
    ( 2720, 32.361 )
    ( 2721, 32.361 )
    ( 2722, 32.510 )
    ( 2723, 32.510 )
    ( 2724, 32.547 )
    ( 2725, 32.583 )
    ( 2726, 32.858 )
    ( 2727, 33.099 )
    ( 2728, 33.246 )
    ( 2729, 33.487 )
    ( 2730, 33.487 )
    ( 2731, 33.574 )
    ( 2732, 33.663 )
    ( 2733, 33.750 )
    ( 2734, 33.906 )
    ( 2735, 33.997 )
    ( 2736, 33.997 )
    ( 2737, 33.997 )
    ( 2738, 34.001 )
    ( 2739, 34.001 )
    ( 2740, 34.028 )
    ( 2741, 34.028 )
    ( 2742, 34.229 )
    ( 2743, 34.399 )
    ( 2744, 34.545 )
    ( 2745, 34.545 )
    ( 2746, 34.545 )
    ( 2747, 34.545 )
    ( 2748, 34.560 )
    ( 2749, 34.566 )
    ( 2750, 34.675 )
    ( 2751, 34.675 )
    ( 2752, 34.764 )
    ( 2753, 34.851 )
    ( 2754, 34.945 )
    ( 2755, 35.032 )
    ( 2756, 35.208 )
    ( 2757, 35.295 )
    ( 2758, 35.311 )
    ( 2759, 35.311 )
    ( 2760, 35.461 )
    ( 2761, 35.476 )
    ( 2762, 35.491 )
    ( 2763, 35.500 )
    ( 2764, 35.677 )
    ( 2765, 35.787 )
    ( 2766, 35.796 )
    ( 2767, 35.796 )
    ( 2768, 35.796 )
    ( 2769, 35.972 )
    ( 2770, 36.142 )
    ( 2771, 36.228 )
    ( 2772, 36.295 )
    ( 2773, 36.464 )
    ( 2774, 36.491 )
    ( 2775, 36.519 )
    ( 2776, 36.747 )
    ( 2777, 36.911 )
    ( 2778, 36.919 )
    ( 2779, 36.940 )
    ( 2780, 36.946 )
    ( 2781, 36.963 )
    ( 2782, 37.109 )
    ( 2783, 37.156 )
    ( 2784, 37.337 )
    ( 2785, 37.507 )
    ( 2786, 37.521 )
    ( 2787, 37.521 )
    ( 2788, 37.722 )
    ( 2789, 37.895 )
    ( 2790, 38.104 )
    ( 2791, 38.284 )
    ( 2792, 38.356 )
    ( 2793, 38.356 )
    ( 2794, 38.466 )
    ( 2795, 38.466 )
    ( 2796, 38.509 )
    ( 2797, 38.558 )
    ( 2798, 38.558 )
    ( 2799, 38.594 )
    ( 2800, 38.594 )
    ( 2801, 38.740 )
    ( 2802, 38.816 )
    ( 2803, 38.853 )
    ( 2804, 38.963 )
    ( 2805, 39.036 )
    ( 2806, 39.039 )
    ( 2807, 39.039 )
    ( 2808, 39.075 )
    ( 2809, 39.185 )
    ( 2810, 39.308 )
    ( 2811, 39.387 )
    ( 2812, 39.596 )
    ( 2813, 39.743 )
    ( 2814, 39.865 )
    ( 2815, 39.865 )
    ( 2816, 39.885 )
    ( 2817, 39.885 )
    ( 2818, 39.934 )
    ( 2819, 39.936 )
    ( 2820, 40.086 )
    ( 2821, 40.233 )
    ( 2822, 40.346 )
    ( 2823, 40.456 )
    ( 2824, 40.504 )
    ( 2825, 40.504 )
    ( 2826, 40.504 )
    ( 2827, 40.595 )
    ( 2828, 40.595 )
    ( 2829, 40.598 )
    ( 2830, 40.618 )
    ( 2831, 40.658 )
    ( 2832, 40.721 )
    ( 2833, 40.810 )
    ( 2834, 40.899 )
    ( 2835, 41.069 )
    ( 2836, 41.215 )
    ( 2837, 41.416 )
    ( 2838, 41.606 )
    ( 2839, 41.781 )
    ( 2840, 41.927 )
    ( 2841, 42.097 )
    ( 2842, 42.133 )
    ( 2843, 42.169 )
    ( 2844, 42.347 )
    ( 2845, 42.348 )
    ( 2846, 42.348 )
    ( 2847, 42.348 )
    ( 2848, 42.384 )
    ( 2849, 42.498 )
    ( 2850, 42.663 )
    ( 2851, 42.772 )
    ( 2852, 42.772 )
    ( 2853, 42.772 )
    ( 2854, 42.775 )
    ( 2855, 42.792 )
    ( 2856, 42.792 )
    ( 2857, 42.833 )
    ( 2858, 42.896 )
    ( 2859, 42.967 )
    ( 2860, 42.967 )
    ( 2861, 43.137 )
    ( 2862, 43.209 )
    ( 2863, 43.362 )
    ( 2864, 43.487 )
    ( 2865, 43.596 )
    ( 2866, 43.705 )
    ( 2867, 43.816 )
    ( 2868, 43.818 )
    ( 2869, 43.869 )
    ( 2870, 43.869 )
    ( 2871, 43.941 )
    ( 2872, 43.973 )
    ( 2873, 43.974 )
    ( 2874, 44.081 )
    ( 2875, 44.343 )
    ( 2876, 44.343 )
    ( 2877, 44.343 )
    ( 2878, 44.377 )
    ( 2879, 44.377 )
    ( 2880, 44.378 )
    ( 2881, 44.531 )
    ( 2882, 44.551 )
    ( 2883, 44.618 )
    ( 2884, 44.685 )
    ( 2885, 44.780 )
    ( 2886, 44.912 )
    ( 2887, 44.981 )
    ( 2888, 44.981 )
    ( 2889, 44.982 )
    ( 2890, 44.990 )
    ( 2891, 45.103 )
    ( 2892, 45.106 )
    ( 2893, 45.162 )
    ( 2894, 45.180 )
    ( 2895, 45.181 )
    ( 2896, 45.191 )
    ( 2897, 45.191 )
    ( 2898, 45.220 )
    ( 2899, 45.220 )
    ( 2900, 45.256 )
    ( 2901, 45.302 )
    ( 2902, 45.341 )
    ( 2903, 45.344 )
    ( 2904, 45.377 )
    ( 2905, 45.398 )
    ( 2906, 45.399 )
    ( 2907, 45.399 )
    ( 2908, 45.443 )
    ( 2909, 45.502 )
    ( 2910, 45.502 )
    ( 2911, 45.831 )
    ( 2912, 45.928 )
    ( 2913, 46.043 )
    ( 2914, 46.110 )
    ( 2915, 46.140 )
    ( 2916, 46.140 )
    ( 2917, 46.213 )
    ( 2918, 46.286 )
    ( 2919, 46.312 )
    ( 2920, 46.358 )
    ( 2921, 46.377 )
    ( 2922, 46.393 )
    ( 2923, 46.394 )
    ( 2924, 46.461 )
    ( 2925, 46.529 )
    ( 2926, 46.664 )
    ( 2927, 46.798 )
    ( 2928, 46.933 )
    ( 2929, 47.001 )
    ( 2930, 47.105 )
    ( 2931, 47.194 )
    ( 2932, 47.287 )
    ( 2933, 47.374 )
    ( 2934, 47.461 )
    ( 2935, 47.592 )
    ( 2936, 47.686 )
    ( 2937, 47.848 )
    ( 2938, 48.009 )
    ( 2939, 48.096 )
    ( 2940, 48.186 )
    ( 2941, 48.273 )
    ( 2942, 48.360 )
    ( 2943, 48.466 )
    ( 2944, 48.560 )
    ( 2945, 48.660 )
    ( 2946, 48.747 )
    ( 2947, 48.902 )
    ( 2948, 49.022 )
    ( 2949, 49.117 )
    ( 2950, 49.184 )
    ( 2951, 49.271 )
    ( 2952, 49.358 )
    ( 2953, 49.376 )
    ( 2954, 49.376 )
    ( 2955, 49.377 )
    ( 2956, 49.392 )
    ( 2957, 49.428 )
    ( 2958, 49.575 )
    ( 2959, 49.717 )
    ( 2960, 49.728 )
    ( 2961, 49.729 )
    ( 2962, 49.731 )
    ( 2963, 49.754 )
    ( 2964, 49.833 )
    ( 2965, 49.950 )
    ( 2966, 50.116 )
    ( 2967, 50.290 )
    ( 2968, 50.398 )
    ( 2969, 50.398 )
    ( 2970, 50.613 )
    ( 2971, 50.759 )
    ( 2972, 50.836 )
    ( 2973, 50.844 )
    ( 2974, 50.844 )
    ( 2975, 50.844 )
    ( 2976, 50.845 )
    ( 2977, 50.845 )
    ( 2978, 50.845 )
    ( 2979, 50.845 )
    ( 2980, 50.848 )
    ( 2981, 50.920 )
    ( 2982, 50.920 )
    ( 2983, 51.063 )
    ( 2984, 51.186 )
    ( 2985, 51.188 )
    ( 2986, 51.197 )
    ( 2987, 51.205 )
    ( 2988, 51.234 )
    ( 2989, 51.244 )
    ( 2990, 51.248 )
    ( 2991, 51.253 )
    ( 2992, 51.362 )
    ( 2993, 51.396 )
    ( 2994, 51.412 )
    ( 2995, 51.416 )
    ( 2996, 51.568 )
    ( 2997, 51.568 )
    ( 2998, 51.667 )
    ( 2999, 51.774 )
    ( 3000, 51.941 )
    ( 3001, 52.028 )
    ( 3002, 52.192 )
    ( 3003, 52.292 )
    ( 3004, 52.389 )
    ( 3005, 52.491 )
    ( 3006, 52.621 )
    ( 3007, 52.750 )
    ( 3008, 52.849 )
    ( 3009, 53.009 )
    ( 3010, 53.153 )
    ( 3011, 53.221 )
    ( 3012, 53.308 )
    ( 3013, 53.477 )
    ( 3014, 53.590 )
    ( 3015, 53.751 )
    ( 3016, 53.851 )
    ( 3017, 53.915 )
    ( 3018, 53.939 )
    ( 3019, 53.982 )
    ( 3020, 54.060 )
    ( 3021, 54.060 )
    ( 3022, 54.060 )
    ( 3023, 54.060 )
    ( 3024, 54.197 )
    ( 3025, 54.209 )
    ( 3026, 54.225 )
    ( 3027, 54.251 )
    ( 3028, 54.291 )
    ( 3029, 54.396 )
    ( 3030, 54.661 )
    ( 3031, 54.814 )
    ( 3032, 54.967 )
    ( 3033, 55.114 )
    ( 3034, 55.261 )
    ( 3035, 55.485 )
    ( 3036, 55.660 )
    ( 3037, 55.665 )
    ( 3038, 55.666 )
    ( 3039, 55.668 )
    ( 3040, 55.681 )
    ( 3041, 55.790 )
    ( 3042, 55.836 )
    ( 3043, 55.909 )
    ( 3044, 55.981 )
    ( 3045, 56.160 )
    ( 3046, 56.213 )
    ( 3047, 56.213 )
    ( 3048, 56.215 )
    ( 3049, 56.217 )
    ( 3050, 56.347 )
    ( 3051, 56.414 )
    ( 3052, 56.469 )
    ( 3053, 56.469 )
    ( 3054, 56.469 )
    ( 3055, 56.469 )
    ( 3056, 56.588 )
    ( 3057, 56.588 )
    ( 3058, 56.588 )
    ( 3059, 56.588 )
    ( 3060, 56.735 )
    ( 3061, 56.762 )
    ( 3062, 56.840 )
    ( 3063, 56.913 )
    ( 3064, 56.979 )
    ( 3065, 57.067 )
    ( 3066, 57.155 )
    ( 3067, 57.343 )
    ( 3068, 57.343 )
    ( 3069, 57.358 )
    ( 3070, 57.441 )
    ( 3071, 57.462 )
    ( 3072, 57.463 )
    ( 3073, 57.464 )
    ( 3074, 57.466 )
    ( 3075, 57.597 )
    ( 3076, 57.660 )
    ( 3077, 57.813 )
    ( 3078, 57.880 )
    ( 3079, 58.056 )
    ( 3080, 58.295 )
    ( 3081, 58.528 )
    ( 3082, 58.762 )
    ( 3083, 59.009 )
    ( 3084, 59.241 )
    ( 3085, 59.518 )
    ( 3086, 59.830 )
    ( 3087, 60.085 )
    ( 3088, 60.057 )
    ( 3089, 60.032 )
    ( 3090, 60.264 )
    ( 3091, 60.601 )
    ( 3092, 60.949 )
    ( 3093, 61.247 )
    ( 3094, 61.542 )
    ( 3095, 61.848 )
    ( 3096, 62.151 )
    ( 3097, 62.244 )
    ( 3098, 62.329 )
    ( 3099, 62.411 )
    ( 3100, 62.393 )
    ( 3101, 62.365 )
    ( 3102, 62.708 )
    ( 3103, 63.000 )
    ( 3104, 63.222 )
    ( 3105, 63.585 )
    ( 3106, 63.807 )
    ( 3107, 64.058 )
    ( 3108, 64.391 )
    ( 3109, 64.612 )
    ( 3110, 64.977 )
    ( 3111, 65.319 )
    ( 3112, 65.697 )
    ( 3113, 66.060 )
    ( 3114, 66.416 )
    ( 3115, 66.638 )
    ( 3116, 66.926 )
    ( 3117, 67.214 )
    ( 3118, 67.458 )
    ( 3119, 67.695 )
    ( 3120, 67.918 )
    ( 3121, 68.140 )
    ( 3122, 68.373 )
    ( 3123, 68.657 )
    ( 3124, 68.892 )
    ( 3125, 69.125 )
    ( 3126, 69.416 )
    ( 3127, 69.645 )
    ( 3128, 69.879 )
    ( 3129, 70.123 )
    ( 3130, 70.345 )
    ( 3131, 70.578 )
    ( 3132, 70.800 )
    ( 3133, 71.061 )
    ( 3134, 71.348 )
    ( 3135, 71.629 )
    ( 3136, 71.923 )
    ( 3137, 72.222 )
    ( 3138, 72.506 )
    ( 3139, 72.728 )
    ( 3140, 72.979 )
    ( 3141, 73.200 )
    ( 3142, 73.444 )
    ( 3143, 73.613 )
    ( 3144, 73.760 )
    ( 3145, 73.907 )
    ( 3146, 74.053 )
    ( 3147, 74.155 )
    ( 3148, 74.157 )
    ( 3149, 74.246 )
    ( 3150, 74.328 )
    ( 3151, 74.505 )
    ( 3152, 74.655 )
    ( 3153, 74.802 )
    ( 3154, 74.947 )
    ( 3155, 74.957 )
    ( 3156, 74.957 )
    ( 3157, 74.970 )
    ( 3158, 75.118 )
    ( 3159, 75.307 )
    ( 3160, 75.470 )
    ( 3161, 75.498 )
    ( 3162, 75.629 )
    ( 3163, 75.652 )
    ( 3164, 75.654 )
    ( 3165, 75.654 )
    ( 3166, 75.654 )
    ( 3167, 75.800 )
    ( 3168, 75.987 )
    ( 3169, 76.134 )
    ( 3170, 76.158 )
    ( 3171, 76.158 )
    ( 3172, 76.158 )
    ( 3173, 76.158 )
    ( 3174, 76.403 )
    ( 3175, 76.635 )
    ( 3176, 76.894 )
    ( 3177, 77.136 )
    ( 3178, 77.424 )
    ( 3179, 77.706 )
    ( 3180, 78.103 )
    ( 3181, 78.329 )
    ( 3182, 78.555 )
    ( 3183, 78.776 )
    ( 3184, 79.060 )
    ( 3185, 79.310 )
    ( 3186, 79.532 )
    ( 3187, 79.775 )
    ( 3188, 79.848 )
    ( 3189, 80.048 )
    ( 3190, 80.078 )
    ( 3191, 80.080 )
    ( 3192, 80.087 )
    ( 3193, 80.089 )
    ( 3194, 80.259 )
    ( 3195, 80.405 )
    ( 3196, 80.406 )
    ( 3197, 80.406 )
    ( 3198, 80.586 )
    ( 3199, 80.731 )
    ( 3200, 80.731 )
    ( 3201, 81.043 )
    ( 3202, 81.519 )
    ( 3203, 81.822 )
    ( 3204, 82.145 )
    ( 3205, 82.456 )
    ( 3206, 82.761 )
    ( 3207, 83.068 )
    ( 3208, 83.358 )
    ( 3209, 83.706 )
    ( 3210, 84.019 )
    ( 3211, 84.294 )
    ( 3212, 84.570 )
    ( 3213, 85.004 )
    ( 3214, 85.295 )
    ( 3215, 85.596 )
    ( 3216, 85.894 )
    ( 3217, 86.175 )
    ( 3218, 86.453 )
    ( 3219, 86.735 )
    ( 3220, 87.012 )
    ( 3221, 87.038 )
    ( 3222, 87.039 )
    ( 3223, 87.039 )
    ( 3224, 87.232 )
    ( 3225, 87.232 )
    ( 3226, 87.247 )
    ( 3227, 87.332 )
    ( 3228, 87.304 )
    ( 3229, 87.327 )
    ( 3230, 87.354 )
    ( 3231, 87.354 )
    ( 3232, 87.341 )
    ( 3233, 87.218 )
    ( 3234, 87.094 )
    ( 3235, 86.981 )
    ( 3236, 86.856 )
    ( 3237, 86.743 )
    ( 3238, 86.690 )
    ( 3239, 86.616 )
    ( 3240, 86.491 )
    ( 3241, 86.456 )
    ( 3242, 86.331 )
    ( 3243, 86.238 )
    ( 3244, 86.113 )
    ( 3245, 86.252 )
    ( 3246, 86.404 )
    ( 3247, 86.529 )
    ( 3248, 86.654 )
    ( 3249, 86.835 )
    ( 3250, 86.711 )
    ( 3251, 86.852 )
    ( 3252, 86.990 )
    ( 3253, 87.079 )
    ( 3254, 87.215 )
    ( 3255, 87.287 )
    ( 3256, 87.163 )
    ( 3257, 87.038 )
    ( 3258, 87.009 )
    ( 3259, 86.884 )
    ( 3260, 86.811 )
    ( 3261, 86.820 )
    ( 3262, 86.695 )
    ( 3263, 86.402 )
    ( 3264, 86.165 )
    ( 3265, 85.864 )
    ( 3266, 85.563 )
    ( 3267, 85.263 )
    ( 3268, 84.962 )
    ( 3269, 84.675 )
    ( 3270, 84.470 )
    ( 3271, 84.314 )
    ( 3272, 84.057 )
    ( 3273, 83.766 )
    ( 3274, 83.468 )
    ( 3275, 83.167 )
    ( 3276, 82.866 )
    ( 3277, 82.575 )
    ( 3278, 82.379 )
    ( 3279, 82.221 )
    ( 3280, 82.025 )
    ( 3281, 81.820 )
    ( 3282, 81.525 )
    ( 3283, 81.226 )
    ( 3284, 80.925 )
    ( 3285, 80.624 )
    ( 3286, 80.339 )
    ( 3287, 80.116 )
    ( 3288, 79.918 )
    ( 3289, 79.681 )
    ( 3290, 79.391 )
    ( 3291, 79.206 )
    ( 3292, 78.927 )
    ( 3293, 78.626 )
    ( 3294, 78.368 )
    ( 3295, 78.121 )
    ( 3296, 77.873 )
    ( 3297, 77.572 )
    ( 3298, 77.312 )
    ( 3299, 77.188 )
    ( 3300, 76.908 )
    ( 3301, 76.670 )
    ( 3302, 76.395 )
    ( 3303, 76.138 )
    ( 3304, 75.837 )
    ( 3305, 75.555 )
    ( 3306, 75.254 )
    ( 3307, 74.952 )
    ( 3308, 74.686 )
    ( 3309, 74.385 )
    ( 3310, 74.164 )
    ( 3311, 73.892 )
    ( 3312, 73.592 )
    ( 3313, 73.361 )
    ( 3314, 73.150 )
    ( 3315, 72.850 )
    ( 3316, 72.549 )
    ( 3317, 72.452 )
    ( 3318, 72.375 )
    ( 3319, 72.095 )
    ( 3320, 71.828 )
    ( 3321, 71.852 )
    ( 3322, 71.918 )
    ( 3323, 71.978 )
    ( 3324, 71.884 )
    ( 3325, 71.793 )
    ( 3326, 71.830 )
    ( 3327, 71.765 )
    ( 3328, 71.463 )
    ( 3329, 71.463 )
    ( 3330, 71.648 )
    ( 3331, 71.859 )
    ( 3332, 71.766 )
    ( 3333, 71.854 )
    ( 3334, 71.897 )
    ( 3335, 71.938 )
    ( 3336, 71.980 )
    ( 3337, 71.856 )
    ( 3338, 71.792 )
    ( 3339, 71.680 )
    ( 3340, 71.637 )
    ( 3341, 71.613 )
    ( 3342, 71.488 )
    ( 3343, 71.564 )
    ( 3344, 71.471 )
    ( 3345, 71.347 )
    ( 3346, 71.305 )
    ( 3347, 71.328 )
    ( 3348, 71.379 )
    ( 3349, 71.421 )
    ( 3350, 71.299 )
    ( 3351, 71.340 )
    ( 3352, 71.268 )
    ( 3353, 71.143 )
    ( 3354, 71.018 )
    ( 3355, 71.145 )
    ( 3356, 71.269 )
    ( 3357, 71.516 )
    ( 3358, 71.531 )
    ( 3359, 71.504 )
    ( 3360, 71.477 )
    ( 3361, 71.448 )
    ( 3362, 71.684 )
    ( 3363, 71.911 )
    ( 3364, 72.131 )
    ( 3365, 72.370 )
    ( 3366, 72.698 )
    ( 3367, 72.995 )
    ( 3368, 73.284 )
    ( 3369, 73.553 )
    ( 3370, 73.809 )
    ( 3371, 74.223 )
    ( 3372, 74.614 )
    ( 3373, 75.003 )
    ( 3374, 75.392 )
    ( 3375, 75.717 )
    ( 3376, 75.957 )
    ( 3377, 76.196 )
    ( 3378, 76.398 )
    ( 3379, 76.602 )
    ( 3380, 76.626 )
    ( 3381, 76.661 )
    ( 3382, 76.693 )
    ( 3383, 76.695 )
    ( 3384, 76.640 )
    ( 3385, 76.697 )
    ( 3386, 76.705 )
    ( 3387, 76.700 )
    ( 3388, 76.686 )
    ( 3389, 76.672 )
    ( 3390, 76.371 )
    ( 3391, 76.141 )
    ( 3392, 76.007 )
    ( 3393, 75.707 )
    ( 3394, 75.471 )
    ( 3395, 75.223 )
    ( 3396, 75.012 )
    ( 3397, 74.726 )
    ( 3398, 74.426 )
    ( 3399, 74.140 )
    ( 3400, 73.840 )
    ( 3401, 73.644 )
    ( 3402, 73.420 )
    ( 3403, 73.118 )
    ( 3404, 72.817 )
    ( 3405, 72.677 )
    ( 3406, 72.376 )
    ( 3407, 72.076 )
    ( 3408, 71.774 )
    ( 3409, 71.474 )
    ( 3410, 71.173 )
    ( 3411, 70.872 )
    ( 3412, 70.571 )
    ( 3413, 70.276 )
    ( 3414, 69.976 )
    ( 3415, 69.841 )
    ( 3416, 69.547 )
    ( 3417, 69.323 )
    ( 3418, 69.022 )
    ( 3419, 69.056 )
    ( 3420, 69.081 )
    ( 3421, 68.793 )
    ( 3422, 68.491 )
    ( 3423, 68.190 )
    ( 3424, 67.890 )
    ( 3425, 67.602 )
    ( 3426, 67.301 )
    ( 3427, 67.184 )
    ( 3428, 66.883 )
    ( 3429, 66.583 )
    ( 3430, 66.315 )
    ( 3431, 66.401 )
    ( 3432, 66.406 )
    ( 3433, 66.419 )
    ( 3434, 66.326 )
    ( 3435, 66.128 )
    ( 3436, 66.124 )
    ( 3437, 66.027 )
    ( 3438, 65.780 )
    ( 3439, 65.519 )
    ( 3440, 65.248 )
    ( 3441, 65.011 )
    ( 3442, 64.710 )
    ( 3443, 64.479 )
    ( 3444, 64.250 )
    ( 3445, 64.067 )
    ( 3446, 63.874 )
    ( 3447, 63.677 )
    ( 3448, 63.481 )
    ( 3449, 63.302 )
    ( 3450, 63.022 )
    ( 3451, 62.740 )
    ( 3452, 62.585 )
    ( 3453, 62.284 )
    ( 3454, 62.160 )
    ( 3455, 62.035 )
    ( 3456, 61.910 )
    ( 3457, 61.815 )
    ( 3458, 61.715 )
    ( 3459, 61.626 )
    ( 3460, 61.501 )
    ( 3461, 61.419 )
    ( 3462, 61.294 )
    ( 3463, 61.169 )
    ( 3464, 61.049 )
    ( 3465, 60.927 )
    ( 3466, 60.802 )
    ( 3467, 60.687 )
    ( 3468, 60.562 )
    ( 3469, 60.493 )
    ( 3470, 60.369 )
    ( 3471, 60.327 )
    ( 3472, 60.286 )
    ( 3473, 60.260 )
    ( 3474, 60.135 )
    ( 3475, 60.018 )
    ( 3476, 59.894 )
    ( 3477, 60.081 )
    ( 3478, 60.343 )
    ( 3479, 60.643 )
    ( 3480, 60.845 )
    ( 3481, 60.970 )
    ( 3482, 61.109 )
    ( 3483, 61.366 )
    ( 3484, 61.499 )
    ( 3485, 61.754 )
    ( 3486, 62.012 )
    ( 3487, 62.198 )
    ( 3488, 62.327 )
    ( 3489, 62.567 )
    ( 3490, 62.697 )
    ( 3491, 62.822 )
    ( 3492, 63.006 )
    ( 3493, 62.978 )
    ( 3494, 62.963 )
    ( 3495, 62.935 )
    ( 3496, 62.877 )
    ( 3497, 62.819 )
    ( 3498, 62.827 )
    ( 3499, 62.770 )
    ( 3500, 62.721 )
    ( 3501, 62.663 )
    ( 3502, 62.604 )
    ( 3503, 62.549 )
    ( 3504, 62.513 )
    ( 3505, 62.570 )
    ( 3506, 62.524 )
    ( 3507, 62.467 )
    ( 3508, 62.417 )
    ( 3509, 62.443 )
    ( 3510, 62.525 )
    ( 3511, 62.470 )
    ( 3512, 62.458 )
    ( 3513, 62.499 )
    ( 3514, 62.494 )
    ( 3515, 62.445 )
    ( 3516, 62.450 )
    ( 3517, 62.409 )
    ( 3518, 62.351 )
    ( 3519, 62.317 )
    ( 3520, 62.259 )
    ( 3521, 62.230 )
    ( 3522, 62.208 )
    ( 3523, 62.531 )
    ( 3524, 62.854 )
    ( 3525, 63.203 )
    ( 3526, 63.438 )
    ( 3527, 63.712 )
    ( 3528, 63.952 )
    ( 3529, 64.324 )
    ( 3530, 64.692 )
    ( 3531, 64.893 )
    ( 3532, 65.095 )
    ( 3533, 65.111 )
    ( 3534, 65.167 )
    ( 3535, 65.221 )
    ( 3536, 65.288 )
    ( 3537, 65.274 )
    ( 3538, 65.179 )
    ( 3539, 65.091 )
    ( 3540, 64.994 )
    ( 3541, 64.931 )
    ( 3542, 64.874 )
    ( 3543, 64.690 )
    ( 3544, 64.460 )
    ( 3545, 64.161 )
    ( 3546, 63.889 )
    ( 3547, 63.588 )
    ( 3548, 63.318 )
    ( 3549, 63.017 )
    ( 3550, 62.740 )
    ( 3551, 62.439 )
    ( 3552, 62.202 )
    ( 3553, 62.119 )
    ( 3554, 61.997 )
    ( 3555, 61.925 )
    ( 3556, 61.784 )
    ( 3557, 61.483 )
    ( 3558, 61.182 )
    ( 3559, 60.906 )
    ( 3560, 60.709 )
    ( 3561, 60.529 )
    ( 3562, 60.238 )
    ( 3563, 59.937 )
    ( 3564, 59.816 )
    ( 3565, 59.680 )
    ( 3566, 59.556 )
    ( 3567, 59.410 )
    ( 3568, 59.519 )
    ( 3569, 59.473 )
    ( 3570, 59.379 )
    ( 3571, 59.099 )
    ( 3572, 58.798 )
    ( 3573, 58.718 )
    ( 3574, 58.417 )
    ( 3575, 58.495 )
    ( 3576, 58.563 )
    ( 3577, 58.556 )
    ( 3578, 58.659 )
    ( 3579, 58.806 )
    ( 3580, 58.804 )
    ( 3581, 58.844 )
    ( 3582, 58.852 )
    ( 3583, 58.850 )
    ( 3584, 58.956 )
    ( 3585, 58.953 )
    ( 3586, 58.961 )
    ( 3587, 58.958 )
    ( 3588, 58.955 )
    ( 3589, 58.704 )
    ( 3590, 58.411 )
    ( 3591, 58.331 )
    ( 3592, 58.252 )
    ( 3593, 58.225 )
    ( 3594, 58.015 )
    ( 3595, 57.715 )
    ( 3596, 57.415 )
    ( 3597, 57.245 )
    ( 3598, 56.944 )
    ( 3599, 56.684 )
    ( 3600, 56.567 )
    ( 3601, 56.309 )
    ( 3602, 56.125 )
    ( 3603, 55.825 )
    ( 3604, 55.539 )
    ( 3605, 55.240 )
    ( 3606, 54.940 )
    ( 3607, 54.733 )
    ( 3608, 54.435 )
    ( 3609, 54.163 )
    ( 3610, 53.866 )
    ( 3611, 53.770 )
    ( 3612, 53.573 )
    ( 3613, 53.476 )
    ( 3614, 53.250 )
    ( 3615, 53.040 )
    ( 3616, 52.761 )
    ( 3617, 52.460 )
    ( 3618, 52.211 )
    ( 3619, 51.910 )
    ( 3620, 51.874 )
    ( 3621, 51.780 )
    ( 3622, 51.905 )
    ( 3623, 52.079 )
    ( 3624, 51.971 )
    ( 3625, 51.849 )
    ( 3626, 51.763 )
    ( 3627, 51.638 )
    ( 3628, 51.515 )
    ( 3629, 51.719 )
    ( 3630, 51.818 )
    ( 3631, 51.922 )
    ( 3632, 52.119 )
    ( 3633, 52.215 )
    ( 3634, 52.362 )
    ( 3635, 52.464 )
    ( 3636, 52.561 )
    ( 3637, 52.729 )
    ( 3638, 52.909 )
    ( 3639, 53.046 )
    ( 3640, 53.154 )
    ( 3641, 53.405 )
    ( 3642, 53.701 )
    ( 3643, 53.917 )
    ( 3644, 54.080 )
    ( 3645, 54.177 )
    ( 3646, 54.332 )
    ( 3647, 54.454 )
    ( 3648, 54.555 )
    ( 3649, 54.434 )
    ( 3650, 54.381 )
    ( 3651, 54.267 )
    ( 3652, 54.142 )
    ( 3653, 54.101 )
    ( 3654, 54.097 )
    ( 3655, 54.142 )
    ( 3656, 54.122 )
    ( 3657, 54.102 )
    ( 3658, 53.977 )
    ( 3659, 54.054 )
    ( 3660, 54.165 )
    ( 3661, 54.132 )
    ( 3662, 54.013 )
    ( 3663, 53.888 )
    ( 3664, 53.705 )
    ( 3665, 53.489 )
    ( 3666, 53.508 )
    ( 3667, 53.228 )
    ( 3668, 52.941 )
    ( 3669, 52.655 )
    ( 3670, 52.463 )
    ( 3671, 52.226 )
    ( 3672, 51.952 )
    ( 3673, 51.650 )
    ( 3674, 51.384 )
    ( 3675, 51.085 )
    ( 3676, 50.858 )
    ( 3677, 50.557 )
    ( 3678, 50.261 )
    ( 3679, 50.050 )
    ( 3680, 49.882 )
    ( 3681, 49.628 )
    ( 3682, 49.327 )
    ( 3683, 49.302 )
    ( 3684, 49.071 )
    ( 3685, 49.124 )
    ( 3686, 49.164 )
    ( 3687, 49.096 )
    ( 3688, 49.003 )
    ( 3689, 48.917 )
    ( 3690, 48.899 )
    ( 3691, 48.890 )
    ( 3692, 48.793 )
    ( 3693, 48.583 )
    ( 3694, 48.418 )
    ( 3695, 48.208 )
    ( 3696, 47.997 )
    ( 3697, 47.761 )
    ( 3698, 47.461 )
    ( 3699, 47.336 )
    ( 3700, 47.233 )
    ( 3701, 46.932 )
    ( 3702, 46.636 )
    ( 3703, 46.335 )
    ( 3704, 46.258 )
    ( 3705, 46.163 )
    ( 3706, 45.862 )
    ( 3707, 45.562 )
    ( 3708, 45.357 )
    ( 3709, 45.060 )
    ( 3710, 44.760 )
    ( 3711, 44.460 )
    ( 3712, 44.169 )
    ( 3713, 43.868 )
    ( 3714, 43.567 )
    ( 3715, 43.384 )
    ( 3716, 43.083 )
    ( 3717, 42.954 )
    ( 3718, 42.653 )
    ( 3719, 42.509 )
    ( 3720, 42.363 )
    ( 3721, 42.291 )
    ( 3722, 42.229 )
    ( 3723, 42.166 )
    ( 3724, 42.101 )
    ( 3725, 42.085 )
    ( 3726, 41.989 )
    ( 3727, 41.688 )
    ( 3728, 41.660 )
    ( 3729, 41.381 )
    ( 3730, 41.185 )
    ( 3731, 40.991 )
    ( 3732, 40.795 )
    ( 3733, 40.607 )
    ( 3734, 40.306 )
    ( 3735, 40.363 )
    ( 3736, 40.304 )
    ( 3737, 40.107 )
    ( 3738, 39.840 )
    ( 3739, 39.788 )
    ( 3740, 39.690 )
    ( 3741, 39.390 )
    ( 3742, 39.262 )
    ( 3743, 39.030 )
    ( 3744, 38.965 )
    ( 3745, 38.868 )
    ( 3746, 38.771 )
    ( 3747, 38.674 )
    ( 3748, 38.590 )
    ( 3749, 38.325 )
    ( 3750, 38.023 )
    ( 3751, 37.723 )
    ( 3752, 37.423 )
    ( 3753, 37.122 )
    ( 3754, 36.826 )
    ( 3755, 36.630 )
    ( 3756, 36.329 )
    ( 3757, 36.029 )
    ( 3758, 35.768 )
    ( 3759, 35.525 )
    ( 3760, 35.245 )
    ( 3761, 34.944 )
    ( 3762, 34.884 )
    ( 3763, 34.596 )
    ( 3764, 34.396 )
    ( 3765, 34.095 )
    ( 3766, 34.038 )
    ( 3767, 33.941 )
    ( 3768, 33.844 )
    ( 3769, 33.747 )
    ( 3770, 33.490 )
    ( 3771, 33.189 )
    ( 3772, 32.958 )
    ( 3773, 32.658 )
    ( 3774, 32.357 )
    ( 3775, 32.546 )
    ( 3776, 32.715 )
    ( 3777, 32.898 )
    ( 3778, 33.001 )
    ( 3779, 33.023 )
    ( 3780, 32.996 )
    ( 3781, 32.994 )
    ( 3782, 32.937 )
    ( 3783, 32.931 )
    ( 3784, 32.924 )
    ( 3785, 32.957 )
    ( 3786, 32.956 )
    ( 3787, 32.986 )
    ( 3788, 32.972 )
    ( 3789, 32.958 )
    ( 3790, 33.174 )
    ( 3791, 33.274 )
    ( 3792, 33.499 )
    ( 3793, 33.630 )
    ( 3794, 33.731 )
    ( 3795, 33.828 )
    ( 3796, 34.026 )
    ( 3797, 34.132 )
    ( 3798, 34.232 )
    ( 3799, 34.329 )
    ( 3800, 34.428 )
    ( 3801, 34.577 )
    ( 3802, 34.797 )
    ( 3803, 35.053 )
    ( 3804, 35.180 )
    ( 3805, 35.302 )
    ( 3806, 35.430 )
    ( 3807, 35.591 )
    ( 3808, 35.752 )
    ( 3809, 35.886 )
    ( 3810, 36.072 )
    ( 3811, 36.194 )
    ( 3812, 36.329 )
    ( 3813, 36.271 )
    ( 3814, 36.213 )
    ( 3815, 36.139 )
    ( 3816, 36.104 )
    ( 3817, 36.033 )
    ( 3818, 35.967 )
    ( 3819, 35.921 )
    ( 3820, 35.945 )
    ( 3821, 35.879 )
    ( 3822, 35.755 )
    ( 3823, 35.630 )
    ( 3824, 35.519 )
    ( 3825, 35.394 )
    ( 3826, 35.336 )
    ( 3827, 35.278 )
    ( 3828, 35.280 )
    ( 3829, 35.299 )
    ( 3830, 35.321 )
    ( 3831, 35.321 )
    ( 3832, 35.377 )
    ( 3833, 35.495 )
    ( 3834, 35.570 )
    ( 3835, 35.702 )
    ( 3836, 35.774 )
    ( 3837, 35.774 )
    ( 3838, 35.789 )
    ( 3839, 35.804 )
    ( 3840, 35.840 )
    ( 3841, 35.840 )
    ( 3842, 35.894 )
    ( 3843, 35.970 )
    ( 3844, 35.986 )
    ( 3845, 36.133 )
    ( 3846, 36.138 )
    ( 3847, 36.167 )
    ( 3848, 36.243 )
    ( 3849, 36.322 )
    ( 3850, 36.373 )
    ( 3851, 36.373 )
    ( 3852, 36.379 )
    ( 3853, 36.409 )
    ( 3854, 36.409 )
    ( 3855, 36.830 )
    ( 3856, 37.110 )
    ( 3857, 37.333 )
    ( 3858, 37.555 )
    ( 3859, 37.813 )
    ( 3860, 38.035 )
    ( 3861, 38.268 )
    ( 3862, 38.536 )
    ( 3863, 38.793 )
    ( 3864, 39.015 )
    ( 3865, 39.287 )
    ( 3866, 39.513 )
    ( 3867, 39.997 )
    ( 3868, 40.475 )
    ( 3869, 40.982 )
    ( 3870, 41.420 )
    ( 3871, 41.763 )
    ( 3872, 42.105 )
    ( 3873, 42.468 )
    ( 3874, 42.691 )
    ( 3875, 42.913 )
    ( 3876, 43.135 )
    ( 3877, 43.499 )
    ( 3878, 43.870 )
    ( 3879, 44.156 )
    ( 3880, 44.501 )
    ( 3881, 44.894 )
    ( 3882, 45.182 )
    ( 3883, 45.403 )
    ( 3884, 45.639 )
    ( 3885, 45.861 )
    ( 3886, 46.083 )
    ( 3887, 46.359 )
    ( 3888, 46.645 )
    ( 3889, 46.955 )
    ( 3890, 47.253 )
    ( 3891, 47.563 )
    ( 3892, 47.875 )
    ( 3893, 48.180 )
    ( 3894, 48.474 )
    ( 3895, 48.755 )
    ( 3896, 49.046 )
    ( 3897, 49.328 )
    ( 3898, 49.694 )
    ( 3899, 49.991 )
    ( 3900, 50.296 )
    ( 3901, 50.591 )
    ( 3902, 50.830 )
    ( 3903, 51.063 )
    ( 3904, 51.371 )
    ( 3905, 51.619 )
    ( 3906, 51.853 )
    ( 3907, 52.087 )
    ( 3908, 52.309 )
    ( 3909, 52.532 )
    ( 3910, 52.758 )
    ( 3911, 52.982 )
    ( 3912, 53.207 )
    ( 3913, 53.435 )
    ( 3914, 53.657 )
    ( 3915, 53.879 )
    ( 3916, 53.928 )
    ( 3917, 53.933 )
    ( 3918, 54.120 )
    ( 3919, 54.201 )
    ( 3920, 54.202 )
    ( 3921, 54.202 )
    ( 3922, 54.348 )
    ( 3923, 54.358 )
    ( 3924, 54.471 )
    ( 3925, 54.471 )
    ( 3926, 54.474 )
    ( 3927, 54.475 )
    ( 3928, 54.504 )
    ( 3929, 54.504 )
    ( 3930, 54.655 )
    ( 3931, 54.887 )
    ( 3932, 55.038 )
    ( 3933, 55.184 )
    ( 3934, 55.187 )
    ( 3935, 55.259 )
    ( 3936, 55.325 )
    ( 3937, 55.340 )
    ( 3938, 55.418 )
    ( 3939, 55.525 )
    ( 3940, 55.602 )
    ( 3941, 55.818 )
    ( 3942, 56.075 )
    ( 3943, 56.238 )
    ( 3944, 56.340 )
    ( 3945, 56.556 )
    ( 3946, 56.654 )
    ( 3947, 56.761 )
    ( 3948, 56.927 )
    ( 3949, 57.024 )
    ( 3950, 57.122 )
    ( 3951, 57.288 )
    ( 3952, 57.438 )
    ( 3953, 57.593 )
    ( 3954, 57.736 )
    ( 3955, 57.900 )
    ( 3956, 58.177 )
    ( 3957, 58.262 )
    ( 3958, 58.233 )
    ( 3959, 58.470 )
    ( 3960, 58.704 )
    ( 3961, 58.938 )
    ( 3962, 59.170 )
    ( 3963, 59.403 )
    ( 3964, 59.641 )
    ( 3965, 59.876 )
    ( 3966, 60.111 )
    ( 3967, 60.348 )
    ( 3968, 60.583 )
    ( 3969, 60.854 )
    ( 3970, 61.123 )
    ( 3971, 61.355 )
    ( 3972, 61.588 )
    ( 3973, 61.834 )
    ( 3974, 62.096 )
    ( 3975, 62.338 )
    ( 3976, 62.574 )
    ( 3977, 62.834 )
    ( 3978, 63.012 )
    ( 3979, 63.189 )
    ( 3980, 63.388 )
    ( 3981, 63.571 )
    ( 3982, 63.748 )
    ( 3983, 63.937 )
    ( 3984, 64.113 )
    ( 3985, 64.314 )
    ( 3986, 64.492 )
    ( 3987, 64.668 )
    ( 3988, 64.844 )
    ( 3989, 65.021 )
    ( 3990, 65.293 )
    ( 3991, 65.584 )
    ( 3992, 65.834 )
    ( 3993, 66.066 )
    ( 3994, 66.243 )
    ( 3995, 66.422 )
    ( 3996, 66.604 )
    ( 3997, 66.833 )
    ( 3998, 67.040 )
    ( 3999, 67.282 )
    ( 4000, 67.467 )
    ( 4001, 67.680 )
    ( 4002, 67.892 )
    ( 4003, 68.068 )
    ( 4004, 68.245 )
    ( 4005, 68.422 )
    ( 4006, 68.651 )
    ( 4007, 68.920 )
    ( 4008, 69.151 )
    ( 4009, 69.394 )
    ( 4010, 69.681 )
    ( 4011, 69.863 )
    ( 4012, 70.101 )
    ( 4013, 70.301 )
    ( 4014, 70.479 )
    ( 4015, 70.656 )
    ( 4016, 70.913 )
    ( 4017, 71.154 )
    ( 4018, 71.354 )
    ( 4019, 71.752 )
    ( 4020, 72.146 )
    ( 4021, 72.538 )
    ( 4022, 72.524 )
    ( 4023, 72.511 )
    ( 4024, 72.544 )
    ( 4025, 72.518 )
    ( 4026, 72.509 )
    ( 4027, 72.570 )
    ( 4028, 72.617 )
    ( 4029, 72.664 )
    ( 4030, 72.636 )
    ( 4031, 72.626 )
    ( 4032, 72.721 )
    ( 4033, 72.739 )
    ( 4034, 72.806 )
    ( 4035, 72.792 )
    ( 4036, 72.801 )
    ( 4037, 72.797 )
    ( 4038, 72.814 )
    ( 4039, 72.938 )
    ( 4040, 73.044 )
    ( 4041, 73.042 )
    ( 4042, 73.041 )
    ( 4043, 72.983 )
    ( 4044, 72.961 )
    ( 4045, 72.903 )
    ( 4046, 72.863 )
    ( 4047, 72.857 )
    ( 4048, 72.799 )
    ( 4049, 72.910 )
    ( 4050, 72.882 )
    ( 4051, 72.854 )
    ( 4052, 72.827 )
    ( 4053, 72.799 )
    ( 4054, 72.562 )
    ( 4055, 72.278 )
    ( 4056, 71.978 )
    ( 4057, 71.815 )
    ( 4058, 71.521 )
    ( 4059, 71.291 )
    ( 4060, 71.118 )
    ( 4061, 70.979 )
    ( 4062, 70.791 )
    ( 4063, 70.490 )
    ( 4064, 70.587 )
    ( 4065, 70.783 )
    ( 4066, 70.880 )
    ( 4067, 71.017 )
    ( 4068, 71.236 )
    ( 4069, 71.446 )
    ( 4070, 71.706 )
    ( 4071, 71.902 )
    ( 4072, 72.099 )
    ( 4073, 72.305 )
    ( 4074, 72.501 )
    ( 4075, 72.599 )
    ( 4076, 72.695 )
    ( 4077, 72.792 )
    ( 4078, 72.890 )
    ( 4079, 72.987 )
    ( 4080, 73.084 )
    ( 4081, 73.181 )
    ( 4082, 73.278 )
    ( 4083, 73.465 )
    ( 4084, 73.512 )
    ( 4085, 73.483 )
    ( 4086, 73.541 )
    ( 4087, 73.515 )
    ( 4088, 73.575 )
    ( 4089, 73.638 )
    ( 4090, 73.579 )
    ( 4091, 73.521 )
    ( 4092, 73.239 )
    ( 4093, 72.939 )
    ( 4094, 72.639 )
    ( 4095, 72.338 )
    ( 4096, 72.040 )
    ( 4097, 71.772 )
    ( 4098, 71.499 )
    ( 4099, 71.271 )
    ( 4100, 71.046 )
    ( 4101, 70.782 )
    ( 4102, 70.617 )
    ( 4103, 70.340 )
    ( 4104, 70.039 )
    ( 4105, 69.737 )
    ( 4106, 69.641 )
    ( 4107, 69.383 )
    ( 4108, 69.093 )
    ( 4109, 68.828 )
    ( 4110, 68.534 )
    ( 4111, 68.242 )
    ( 4112, 67.944 )
    ( 4113, 67.661 )
    ( 4114, 67.360 )
    ( 4115, 67.149 )
    ( 4116, 66.938 )
    ( 4117, 66.735 )
    ( 4118, 66.435 )
    ( 4119, 66.292 )
    ( 4120, 65.991 )
    ( 4121, 65.894 )
    ( 4122, 65.851 )
    ( 4123, 65.809 )
    ( 4124, 65.749 )
    ( 4125, 65.448 )
    ( 4126, 65.193 )
    ( 4127, 64.894 )
    ( 4128, 64.594 )
    ( 4129, 64.323 )
    ( 4130, 64.106 )
    ( 4131, 64.025 )
    ( 4132, 63.938 )
    ( 4133, 63.641 )
    ( 4134, 63.544 )
    ( 4135, 63.587 )
    ( 4136, 63.617 )
    ( 4137, 63.712 )
    ( 4138, 63.411 )
    ( 4139, 63.354 )
    ( 4140, 63.429 )
    ( 4141, 63.510 )
    ( 4142, 63.453 )
    ( 4143, 63.395 )
    ( 4144, 63.453 )
    ( 4145, 63.410 )
    ( 4146, 63.439 )
    ( 4147, 63.385 )
    ( 4148, 63.327 )
    ( 4149, 63.351 )
    ( 4150, 63.378 )
    ( 4151, 63.397 )
    ( 4152, 63.339 )
    ( 4153, 63.368 )
    ( 4154, 63.325 )
    ( 4155, 63.271 )
    ( 4156, 63.213 )
    ( 4157, 63.164 )
    ( 4158, 63.110 )
    ( 4159, 63.088 )
    ( 4160, 63.030 )
    ( 4161, 63.049 )
    ( 4162, 63.230 )
    ( 4163, 63.173 )
    ( 4164, 62.872 )
    ( 4165, 62.571 )
    ( 4166, 62.474 )
    ( 4167, 62.478 )
    ( 4168, 62.177 )
    ( 4169, 61.898 )
    ( 4170, 61.661 )
    ( 4171, 61.457 )
    ( 4172, 61.275 )
    ( 4173, 60.975 )
    ( 4174, 60.689 )
    ( 4175, 60.530 )
    ( 4176, 60.273 )
    ( 4177, 60.184 )
    ( 4178, 60.054 )
    ( 4179, 59.909 )
    ( 4180, 59.865 )
    ( 4181, 59.669 )
    ( 4182, 59.479 )
    ( 4183, 59.242 )
    ( 4184, 58.941 )
    ( 4185, 58.844 )
    ( 4186, 58.748 )
    ( 4187, 58.650 )
    ( 4188, 58.374 )
    ( 4189, 58.297 )
    ( 4190, 58.116 )
    ( 4191, 57.850 )
    ( 4192, 57.549 )
    ( 4193, 57.248 )
    ( 4194, 56.951 )
    ( 4195, 56.816 )
    ( 4196, 56.607 )
    ( 4197, 56.306 )
    ( 4198, 56.119 )
    ( 4199, 55.942 )
    ( 4200, 55.747 )
    ( 4201, 55.730 )
    ( 4202, 55.815 )
    ( 4203, 55.687 )
    ( 4204, 55.541 )
    ( 4205, 55.427 )
    ( 4206, 55.281 )
    ( 4207, 54.980 )
    ( 4208, 54.679 )
    ( 4209, 54.611 )
    ( 4210, 54.503 )
    ( 4211, 54.378 )
    ( 4212, 54.253 )
    ( 4213, 54.145 )
    ( 4214, 54.112 )
    ( 4215, 53.987 )
    ( 4216, 53.862 )
    ( 4217, 53.617 )
    ( 4218, 53.351 )
    ( 4219, 53.210 )
    ( 4220, 53.103 )
    ( 4221, 52.836 )
    ( 4222, 52.860 )
    ( 4223, 52.964 )
    ( 4224, 53.091 )
    ( 4225, 53.130 )
    ( 4226, 52.984 )
    ( 4227, 52.684 )
    ( 4228, 52.448 )
    ( 4229, 52.159 )
    ( 4230, 51.858 )
    ( 4231, 51.557 )
    ( 4232, 51.311 )
    ( 4233, 51.046 )
    ( 4234, 50.746 )
    ( 4235, 50.489 )
    ( 4236, 50.230 )
    ( 4237, 49.930 )
    ( 4238, 49.628 )
    ( 4239, 49.720 )
    ( 4240, 49.805 )
    ( 4241, 49.812 )
    ( 4242, 49.798 )
    ( 4243, 49.847 )
    ( 4244, 49.896 )
    ( 4245, 49.946 )
    ( 4246, 49.910 )
    ( 4247, 49.852 )
    ( 4248, 49.875 )
    ( 4249, 49.873 )
    ( 4250, 49.898 )
    ( 4251, 49.840 )
    ( 4252, 49.782 )
    ( 4253, 49.732 )
    ( 4254, 49.763 )
    ( 4255, 49.775 )
    ( 4256, 49.717 )
    ( 4257, 49.698 )
    ( 4258, 49.689 )
    ( 4259, 49.643 )
    ( 4260, 49.647 )
    ( 4261, 49.589 )
    ( 4262, 49.543 )
    ( 4263, 49.486 )
    ( 4264, 49.472 )
    ( 4265, 49.443 )
    ( 4266, 49.414 )
    ( 4267, 49.405 )
    ( 4268, 49.347 )
    ( 4269, 49.289 )
    ( 4270, 49.250 )
    ( 4271, 49.125 )
    ( 4272, 49.352 )
    ( 4273, 49.568 )
    ( 4274, 49.760 )
    ( 4275, 49.982 )
    ( 4276, 50.219 )
    ( 4277, 50.464 )
    ( 4278, 50.709 )
    ( 4279, 50.889 )
    ( 4280, 51.066 )
    ( 4281, 51.299 )
    ( 4282, 51.532 )
    ( 4283, 51.789 )
    ( 4284, 52.039 )
    ( 4285, 52.294 )
    ( 4286, 52.543 )
    ( 4287, 52.775 )
    ( 4288, 52.952 )
    ( 4289, 53.144 )
    ( 4290, 53.319 )
    ( 4291, 53.553 )
    ( 4292, 53.793 )
    ( 4293, 53.969 )
    ( 4294, 54.146 )
    ( 4295, 54.325 )
    ( 4296, 54.500 )
    ( 4297, 54.677 )
    ( 4298, 54.856 )
    ( 4299, 55.032 )
    ( 4300, 55.210 )
    ( 4301, 55.427 )
    ( 4302, 55.604 )
    ( 4303, 55.783 )
    ( 4304, 55.960 )
    ( 4305, 56.136 )
    ( 4306, 56.374 )
    ( 4307, 56.549 )
    ( 4308, 56.818 )
    ( 4309, 57.001 )
    ( 4310, 57.199 )
    ( 4311, 57.380 )
    ( 4312, 57.564 )
    ( 4313, 57.749 )
    ( 4314, 57.925 )
    ( 4315, 58.102 )
    ( 4316, 58.370 )
    ( 4317, 58.662 )
    ( 4318, 58.931 )
    ( 4319, 59.109 )
    ( 4320, 59.288 )
    ( 4321, 59.525 )
    ( 4322, 59.702 )
    ( 4323, 59.939 )
    ( 4324, 60.115 )
    ( 4325, 60.298 )
    ( 4326, 60.476 )
    ( 4327, 60.709 )
    ( 4328, 60.885 )
    ( 4329, 61.062 )
    ( 4330, 61.296 )
    ( 4331, 61.547 )
    ( 4332, 61.785 )
    ( 4333, 62.052 )
    ( 4334, 62.324 )
    ( 4335, 62.557 )
    ( 4336, 62.812 )
    ( 4337, 63.068 )
    ( 4338, 63.323 )
    ( 4339, 63.575 )
    ( 4340, 63.942 )
    ( 4341, 64.329 )
    ( 4342, 64.684 )
    ( 4343, 65.068 )
    ( 4344, 65.335 )
    ( 4345, 65.568 )
    ( 4346, 65.894 )
    ( 4347, 66.126 )
    ( 4348, 66.419 )
    ( 4349, 66.673 )
    ( 4350, 66.905 )
    ( 4351, 67.156 )
    ( 4352, 67.509 )
    ( 4353, 67.915 )
    ( 4354, 68.334 )
    ( 4355, 68.719 )
    ( 4356, 69.111 )
    ( 4357, 69.531 )
    ( 4358, 69.947 )
    ( 4359, 70.318 )
    ( 4360, 70.688 )
    ( 4361, 71.017 )
    ( 4362, 71.391 )
    ( 4363, 71.750 )
    ( 4364, 72.090 )
    ( 4365, 72.417 )
    ( 4366, 72.831 )
    ( 4367, 73.199 )
    ( 4368, 73.526 )
    ( 4369, 73.864 )
    ( 4370, 74.199 )
    ( 4371, 74.535 )
    ( 4372, 74.864 )
    ( 4373, 75.098 )
    ( 4374, 75.330 )
    ( 4375, 75.563 )
    ( 4376, 75.851 )
    ( 4377, 75.920 )
    ( 4378, 76.037 )
    ( 4379, 76.156 )
    ( 4380, 76.264 )
    ( 4381, 76.261 )
    ( 4382, 76.372 )
    ( 4383, 76.441 )
    ( 4384, 76.438 )
    ( 4385, 76.314 )
    ( 4386, 76.189 )
    ( 4387, 76.064 )
    ( 4388, 75.950 )
    ( 4389, 75.996 )
    ( 4390, 76.037 )
    ( 4391, 75.939 )
    ( 4392, 75.818 )
    ( 4393, 75.693 )
    ( 4394, 75.920 )
    ( 4395, 76.127 )
    ( 4396, 76.311 )
    ( 4397, 76.189 )
    ( 4398, 76.196 )
    ( 4399, 76.071 )
    ( 4400, 75.949 )
    ( 4401, 75.824 )
    ( 4402, 75.785 )
    ( 4403, 75.738 )
    ( 4404, 75.613 )
    ( 4405, 75.491 )
    ( 4406, 75.613 )
    ( 4407, 75.674 )
    ( 4408, 75.626 )
    ( 4409, 75.557 )
    ( 4410, 75.457 )
    ( 4411, 75.509 )
    ( 4412, 75.562 )
    ( 4413, 75.441 )
    ( 4414, 75.316 )
    ( 4415, 75.225 )
    ( 4416, 75.155 )
    ( 4417, 75.032 )
    ( 4418, 74.932 )
    ( 4419, 74.807 )
    ( 4420, 74.682 )
    ( 4421, 74.866 )
    ( 4422, 75.050 )
    ( 4423, 75.255 )
    ( 4424, 75.440 )
    ( 4425, 75.686 )
    ( 4426, 75.940 )
    ( 4427, 76.085 )
    ( 4428, 76.210 )
    ( 4429, 76.338 )
    ( 4430, 76.468 )
    ( 4431, 76.593 )
    ( 4432, 76.917 )
    ( 4433, 77.288 )
    ( 4434, 77.613 )
    ( 4435, 77.939 )
    ( 4436, 78.270 )
    ( 4437, 78.690 )
    ( 4438, 79.015 )
    ( 4439, 79.340 )
    ( 4440, 79.664 )
    ( 4441, 79.989 )
    ( 4442, 80.262 )
    ( 4443, 80.518 )
    ( 4444, 80.775 )
    ( 4445, 81.104 )
    ( 4446, 81.412 )
    ( 4447, 81.597 )
    ( 4448, 81.783 )
    ( 4449, 81.968 )
    ( 4450, 81.843 )
    ( 4451, 81.765 )
    ( 4452, 81.652 )
    ( 4453, 81.529 )
    ( 4454, 81.408 )
    ( 4455, 81.360 )
    ( 4456, 81.358 )
    ( 4457, 81.289 )
    ( 4458, 81.164 )
    ( 4459, 81.123 )
    ( 4460, 81.207 )
    ( 4461, 81.118 )
    ( 4462, 81.003 )
    ( 4463, 80.920 )
    ( 4464, 80.837 )
    ( 4465, 80.771 )
    ( 4466, 80.650 )
    ( 4467, 80.615 )
    ( 4468, 80.567 )
    ( 4469, 80.442 )
    ( 4470, 80.425 )
    ( 4471, 80.301 )
    ( 4472, 80.222 )
    ( 4473, 80.112 )
    ( 4474, 79.995 )
    ( 4475, 79.941 )
    ( 4476, 79.816 )
    ( 4477, 79.858 )
    ( 4478, 79.998 )
    ( 4479, 80.055 )
    ( 4480, 80.097 )
    ( 4481, 80.146 )
    ( 4482, 80.038 )
    ( 4483, 79.927 )
    ( 4484, 79.869 )
    ( 4485, 79.744 )
    ( 4486, 79.750 )
    ( 4487, 79.705 )
    ( 4488, 79.702 )
    ( 4489, 79.715 )
    ( 4490, 79.737 )
    ( 4491, 79.746 )
    ( 4492, 79.769 )
    ( 4493, 79.784 )
    ( 4494, 79.727 )
    ( 4495, 79.671 )
    ( 4496, 79.634 )
    ( 4497, 79.576 )
    ( 4498, 79.620 )
    ( 4499, 79.562 )
    ( 4500, 79.505 )
    ( 4501, 79.491 )
    ( 4502, 79.478 )
    ( 4503, 79.593 )
    ( 4504, 79.640 )
    ( 4505, 79.611 )
    ( 4506, 79.583 )
    ( 4507, 79.691 )
    ( 4508, 79.801 )
    ( 4509, 79.936 )
    ( 4510, 79.958 )
    ( 4511, 79.938 )
    ( 4512, 79.812 )
    ( 4513, 79.771 )
    ( 4514, 79.717 )
    ( 4515, 79.688 )
    ( 4516, 79.562 )
    ( 4517, 79.664 )
    ( 4518, 79.711 )
    ( 4519, 79.759 )
    ( 4520, 79.800 )
    ( 4521, 79.677 )
    ( 4522, 79.552 )
    ( 4523, 79.427 )
    ( 4524, 79.307 )
    ( 4525, 79.208 )
    ( 4526, 79.334 )
    ( 4527, 79.402 )
    ( 4528, 79.290 )
    ( 4529, 79.167 )
    ( 4530, 79.126 )
    ( 4531, 79.067 )
    ( 4532, 78.992 )
    ( 4533, 78.868 )
    ( 4534, 78.744 )
    ( 4535, 78.630 )
    ( 4536, 78.515 )
    ( 4537, 78.390 )
    ( 4538, 78.265 )
    ( 4539, 78.213 )
    ( 4540, 78.088 )
    ( 4541, 77.963 )
    ( 4542, 77.838 )
    ( 4543, 77.741 )
    ( 4544, 77.440 )
    ( 4545, 77.196 )
    ( 4546, 77.100 )
    ( 4547, 76.812 )
    ( 4548, 76.531 )
    ( 4549, 76.385 )
    ( 4550, 76.187 )
    ( 4551, 75.886 )
    ( 4552, 75.842 )
    ( 4553, 75.745 )
    ( 4554, 75.660 )
    ( 4555, 75.359 )
    ( 4556, 75.088 )
    ( 4557, 74.805 )
    ( 4558, 74.504 )
    ( 4559, 74.415 )
    ( 4560, 74.115 )
    ( 4561, 73.814 )
    ( 4562, 73.514 )
    ( 4563, 73.213 )
    ( 4564, 73.013 )
    ( 4565, 72.916 )
    ( 4566, 72.727 )
    ( 4567, 72.661 )
    ( 4568, 72.544 )
    ( 4569, 72.351 )
    ( 4570, 72.104 )
    ( 4571, 71.858 )
    ( 4572, 71.662 )
    ( 4573, 71.516 )
    ( 4574, 71.216 )
    ( 4575, 70.916 )
    ( 4576, 70.620 )
    ( 4577, 70.478 )
    ( 4578, 70.218 )
    ( 4579, 69.924 )
    ( 4580, 69.633 )
    ( 4581, 69.413 )
    ( 4582, 69.301 )
    ( 4583, 68.999 )
    ( 4584, 68.874 )
    ( 4585, 68.750 )
    ( 4586, 68.729 )
    ( 4587, 68.618 )
    ( 4588, 68.534 )
    ( 4589, 68.435 )
    ( 4590, 68.334 )
    ( 4591, 68.209 )
    ( 4592, 68.393 )
    ( 4593, 68.587 )
    ( 4594, 68.803 )
    ( 4595, 68.928 )
    ( 4596, 69.053 )
    ( 4597, 69.279 )
    ( 4598, 69.472 )
    ( 4599, 69.660 )
    ( 4600, 69.785 )
    ( 4601, 69.693 )
    ( 4602, 69.731 )
    ( 4603, 69.638 )
    ( 4604, 69.647 )
    ( 4605, 69.595 )
    ( 4606, 69.555 )
    ( 4607, 69.501 )
    ( 4608, 69.439 )
    ( 4609, 69.339 )
    ( 4610, 69.224 )
    ( 4611, 69.133 )
    ( 4612, 69.014 )
    ( 4613, 68.961 )
    ( 4614, 68.841 )
    ( 4615, 68.719 )
    ( 4616, 68.595 )
    ( 4617, 68.470 )
    ( 4618, 68.418 )
    ( 4619, 68.379 )
    ( 4620, 68.388 )
    ( 4621, 68.334 )
    ( 4622, 68.386 )
    ( 4623, 68.413 )
    ( 4624, 68.355 )
    ( 4625, 68.349 )
    ( 4626, 68.291 )
    ( 4627, 68.349 )
    ( 4628, 68.355 )
    ( 4629, 68.328 )
    ( 4630, 68.309 )
    ( 4631, 68.251 )
    ( 4632, 68.193 )
    ( 4633, 68.068 )
    ( 4634, 67.993 )
    ( 4635, 67.902 )
    ( 4636, 67.777 )
    ( 4637, 67.669 )
    ( 4638, 67.561 )
    ( 4639, 67.462 )
    ( 4640, 67.394 )
    ( 4641, 67.354 )
    ( 4642, 67.230 )
    ( 4643, 67.105 )
    ( 4644, 67.311 )
    ( 4645, 67.568 )
    ( 4646, 67.752 )
    ( 4647, 67.646 )
    ( 4648, 67.612 )
    ( 4649, 67.497 )
    ( 4650, 67.390 )
    ( 4651, 67.285 )
    ( 4652, 67.328 )
    ( 4653, 67.203 )
    ( 4654, 67.102 )
    ( 4655, 67.061 )
    ( 4656, 67.019 )
    ( 4657, 67.130 )
    ( 4658, 67.241 )
    ( 4659, 67.401 )
    ( 4660, 67.560 )
    ( 4661, 67.440 )
    ( 4662, 67.328 )
    ( 4663, 67.222 )
    ( 4664, 67.118 )
    ( 4665, 67.078 )
    ( 4666, 66.953 )
    ( 4667, 66.828 )
    ( 4668, 66.770 )
    ( 4669, 66.712 )
    ( 4670, 66.705 )
    ( 4671, 66.691 )
    ( 4672, 66.683 )
    ( 4673, 66.673 )
    ( 4674, 66.661 )
    ( 4675, 66.647 )
    ( 4676, 66.646 )
    ( 4677, 66.651 )
    ( 4678, 66.594 )
    ( 4679, 66.536 )
    ( 4680, 66.519 )
    ( 4681, 66.501 )
    ( 4682, 66.481 )
    ( 4683, 66.425 )
    ( 4684, 66.385 )
    ( 4685, 66.327 )
    ( 4686, 66.269 )
    ( 4687, 66.253 )
    ( 4688, 66.194 )
    ( 4689, 66.137 )
    ( 4690, 66.092 )
    ( 4691, 66.058 )
    ( 4692, 66.021 )
    ( 4693, 65.964 )
    ( 4694, 65.910 )
    ( 4695, 65.853 )
    ( 4696, 65.794 )
    ( 4697, 65.736 )
    ( 4698, 65.695 )
    ( 4699, 65.726 )
    ( 4700, 65.667 )
    ( 4701, 65.611 )
    ( 4702, 65.620 )
    ( 4703, 65.629 )
    ( 4704, 65.572 )
    ( 4705, 65.515 )
    ( 4706, 65.390 )
    ( 4707, 65.438 )
    ( 4708, 65.525 )
    ( 4709, 65.567 )
    ( 4710, 65.442 )
    ( 4711, 65.328 )
    ( 4712, 65.396 )
    ( 4713, 65.271 )
    ( 4714, 65.202 )
    ( 4715, 65.089 )
    ( 4716, 64.987 )
    ( 4717, 64.862 )
    ( 4718, 64.810 )
    ( 4719, 65.040 )
    ( 4720, 65.318 )
    ( 4721, 65.698 )
    ( 4722, 65.976 )
    ( 4723, 66.120 )
    ( 4724, 66.261 )
    ( 4725, 66.416 )
    ( 4726, 66.720 )
    ( 4727, 66.961 )
    ( 4728, 67.086 )
    ( 4729, 67.211 )
    ( 4730, 67.374 )
    ( 4731, 67.505 )
    ( 4732, 67.630 )
    ( 4733, 67.854 )
    ( 4734, 68.079 )
    ( 4735, 68.270 )
    ( 4736, 68.460 )
    ( 4737, 68.646 )
    ( 4738, 68.771 )
    ( 4739, 68.716 )
    ( 4740, 68.598 )
    ( 4741, 68.562 )
    ( 4742, 68.446 )
    ( 4743, 68.321 )
    ( 4744, 68.196 )
    ( 4745, 67.896 )
    ( 4746, 67.595 )
    ( 4747, 67.295 )
    ( 4748, 67.036 )
    ( 4749, 66.762 )
    ( 4750, 66.461 )
    ( 4751, 66.160 )
    ( 4752, 65.923 )
    ( 4753, 65.712 )
    ( 4754, 65.453 )
    ( 4755, 65.392 )
    ( 4756, 65.181 )
    ( 4757, 64.880 )
    ( 4758, 64.587 )
    ( 4759, 64.296 )
    ( 4760, 63.996 )
    ( 4761, 63.724 )
    ( 4762, 63.423 )
    ( 4763, 63.122 )
    ( 4764, 62.850 )
    ( 4765, 62.764 )
    ( 4766, 62.669 )
    ( 4767, 62.399 )
    ( 4768, 62.098 )
    ( 4769, 61.828 )
    ( 4770, 61.581 )
    ( 4771, 61.303 )
    ( 4772, 61.207 )
    ( 4773, 61.110 )
    ( 4774, 61.023 )
    ( 4775, 60.945 )
    ( 4776, 60.848 )
    ( 4777, 60.872 )
    ( 4778, 60.909 )
    ( 4779, 60.845 )
    ( 4780, 60.780 )
    ( 4781, 60.684 )
    ( 4782, 60.537 )
    ( 4783, 60.426 )
    ( 4784, 60.331 )
    ( 4785, 60.202 )
    ( 4786, 60.056 )
    ( 4787, 59.910 )
    ( 4788, 59.800 )
    ( 4789, 59.654 )
    ( 4790, 59.546 )
    ( 4791, 59.253 )
    ( 4792, 58.995 )
    ( 4793, 58.695 )
    ( 4794, 58.397 )
    ( 4795, 58.188 )
    ( 4796, 57.909 )
    ( 4797, 57.608 )
    ( 4798, 57.307 )
    ( 4799, 57.242 )
    ( 4800, 56.940 )
    ( 4801, 56.693 )
    ( 4802, 56.393 )
    ( 4803, 56.109 )
    ( 4804, 55.928 )
    ( 4805, 55.632 )
    ( 4806, 55.331 )
    ( 4807, 55.150 )
    ( 4808, 54.942 )
    ( 4809, 54.716 )
    ( 4810, 54.416 )
    ( 4811, 54.206 )
    ( 4812, 53.935 )
    ( 4813, 53.647 )
    ( 4814, 53.346 )
    ( 4815, 53.138 )
    ( 4816, 52.925 )
    ( 4817, 52.729 )
    ( 4818, 52.440 )
    ( 4819, 52.139 )
    ( 4820, 51.838 )
    ( 4821, 51.537 )
    ( 4822, 51.271 )
    ( 4823, 51.212 )
    ( 4824, 51.148 )
    ( 4825, 50.948 )
    ( 4826, 50.673 )
    ( 4827, 50.376 )
    ( 4828, 50.075 )
    ( 4829, 49.792 )
    ( 4830, 49.664 )
    ( 4831, 49.368 )
    ( 4832, 49.067 )
    ( 4833, 48.766 )
    ( 4834, 48.519 )
    ( 4835, 48.482 )
    ( 4836, 48.439 )
    ( 4837, 48.343 )
    ( 4838, 48.250 )
    ( 4839, 47.949 )
    ( 4840, 47.916 )
    ( 4841, 47.615 )
    ( 4842, 47.315 )
    ( 4843, 47.088 )
    ( 4844, 46.830 )
    ( 4845, 46.534 )
    ( 4846, 46.242 )
    ( 4847, 45.959 )
    ( 4848, 45.723 )
    ( 4849, 45.422 )
    ( 4850, 45.131 )
    ( 4851, 44.989 )
    ( 4852, 44.993 )
    ( 4853, 44.847 )
    ( 4854, 44.791 )
    ( 4855, 44.645 )
    ( 4856, 44.378 )
    ( 4857, 44.077 )
    ( 4858, 43.847 )
    ( 4859, 43.545 )
    ( 4860, 43.247 )
    ( 4861, 43.042 )
    ( 4862, 42.837 )
    ( 4863, 42.536 )
    ( 4864, 42.235 )
    ( 4865, 42.138 )
    ( 4866, 42.027 )
    ( 4867, 41.727 )
    ( 4868, 41.479 )
    ( 4869, 41.240 )
    ( 4870, 40.942 )
    ( 4871, 40.845 )
    ( 4872, 40.755 )
    ( 4873, 40.658 )
    ( 4874, 40.561 )
    ( 4875, 40.464 )
    ( 4876, 40.163 )
    ( 4877, 39.881 )
    ( 4878, 39.622 )
    ( 4879, 39.333 )
    ( 4880, 39.253 )
    ( 4881, 39.156 )
    ( 4882, 39.061 )
    ( 4883, 39.100 )
    ( 4884, 39.002 )
    ( 4885, 38.906 )
    ( 4886, 38.635 )
    ( 4887, 38.611 )
    ( 4888, 38.321 )
    ( 4889, 38.020 )
    ( 4890, 37.737 )
    ( 4891, 37.453 )
    ( 4892, 37.196 )
    ( 4893, 36.895 )
    ( 4894, 36.647 )
    ( 4895, 36.347 )
    ( 4896, 36.047 )
    ( 4897, 35.789 )
    ( 4898, 35.488 )
    ( 4899, 35.521 )
    ( 4900, 35.507 )
    ( 4901, 35.497 )
    ( 4902, 35.382 )
    ( 4903, 35.300 )
    ( 4904, 35.188 )
    ( 4905, 35.321 )
    ( 4906, 35.207 )
    ( 4907, 35.082 )
    ( 4908, 35.207 )
    ( 4909, 35.332 )
    ( 4910, 35.534 )
    ( 4911, 35.736 )
    ( 4912, 35.936 )
    ( 4913, 36.120 )
    ( 4914, 35.819 )
    ( 4915, 35.521 )
    ( 4916, 35.230 )
    ( 4917, 34.929 )
    ( 4918, 34.870 )
    ( 4919, 34.815 )
    ( 4920, 34.749 )
    ( 4921, 34.448 )
    ( 4922, 34.317 )
    ( 4923, 34.184 )
    ( 4924, 33.882 )
    ( 4925, 33.653 )
    ( 4926, 33.352 )
    ( 4927, 33.057 )
    ( 4928, 33.029 )
    ( 4929, 32.729 )
    ( 4930, 32.463 )
    ( 4931, 32.168 )
    ( 4932, 31.980 )
    ( 4933, 31.679 )
    ( 4934, 31.483 )
    ( 4935, 31.204 )
    ( 4936, 30.904 )
    ( 4937, 30.606 )
    ( 4938, 30.412 )
    ( 4939, 30.111 )
    ( 4940, 29.853 )
    ( 4941, 29.577 )
    ( 4942, 29.618 )
    ( 4943, 29.351 )
    ( 4944, 29.052 )
    ( 4945, 28.794 )
    ( 4946, 28.643 )
    ( 4947, 28.447 )
    ( 4948, 28.357 )
    ( 4949, 28.301 )
    ( 4950, 28.000 )
    ( 4951, 27.941 )
    ( 4952, 27.721 )
    ( 4953, 27.421 )
    ( 4954, 27.120 )
    ( 4955, 26.916 )
    ( 4956, 26.617 )
    ( 4957, 26.316 )
    ( 4958, 26.288 )
    ( 4959, 26.324 )
    ( 4960, 26.341 )
    ( 4961, 26.359 )
    ( 4962, 26.365 )
    ( 4963, 26.424 )
    ( 4964, 26.367 )
    ( 4965, 26.323 )
    ( 4966, 26.374 )
    ( 4967, 26.462 )
    ( 4968, 26.435 )
    ( 4969, 26.313 )
    ( 4970, 26.366 )
    ( 4971, 26.408 )
    ( 4972, 26.425 )
    ( 4973, 26.342 )
    ( 4974, 26.304 )
    ( 4975, 26.287 )
    ( 4976, 26.177 )
    ( 4977, 26.052 )
    ( 4978, 26.038 )
    ( 4979, 25.963 )
    ( 4980, 26.088 )
    ( 4981, 26.278 )
    ( 4982, 26.517 )
    ( 4983, 26.728 )
    ( 4984, 26.854 )
    ( 4985, 26.979 )
    ( 4986, 26.939 )
    ( 4987, 26.897 )
    ( 4988, 26.772 )
    ( 4989, 26.835 )
    ( 4990, 27.159 )
    ( 4991, 27.505 )
    ( 4992, 27.534 )
    ( 4993, 27.534 )
    ( 4994, 27.812 )
    ( 4995, 28.117 )
    ( 4996, 28.317 )
    ( 4997, 28.317 )
    ( 4998, 28.692 )
    ( 4999, 29.003 )
    ( 5000, 29.115 )
    ( 5001, 29.224 )
    ( 5002, 29.372 )
    ( 5003, 29.372 )
    ( 5004, 29.372 )
    ( 5005, 29.376 )
    ( 5006, 29.376 )
    ( 5007, 29.598 )
    ( 5008, 29.820 )
    ( 5009, 30.042 )
    ( 5010, 30.151 )
    ( 5011, 30.392 )
    ( 5012, 30.582 )
    ( 5013, 30.731 )
    ( 5014, 30.731 )
    ( 5015, 30.732 )
    ( 5016, 30.703 )
    ( 5017, 30.645 )
    ( 5018, 30.675 )
    ( 5019, 30.693 )
    ( 5020, 30.642 )
    ( 5021, 30.653 )
    ( 5022, 30.595 )
    ( 5023, 30.567 )
    ( 5024, 30.664 )
    ( 5025, 30.749 )
    ( 5026, 30.833 )
    ( 5027, 30.999 )
    ( 5028, 31.035 )
    ( 5029, 31.009 )
    ( 5030, 30.999 )
    ( 5031, 30.975 )
    ( 5032, 31.136 )
    ( 5033, 31.348 )
    ( 5034, 31.495 )
    ( 5035, 31.538 )
    ( 5036, 31.585 )
    ( 5037, 31.610 )
    ( 5038, 31.614 )
    ( 5039, 31.642 )
    ( 5040, 31.759 )
    ( 5041, 31.911 )
    ( 5042, 32.062 )
    ( 5043, 32.209 )
    ( 5044, 32.423 )
    ( 5045, 32.463 )
    ( 5046, 32.507 )
    ( 5047, 32.507 )
    ( 5048, 32.507 )
    ( 5049, 32.729 )
    ( 5050, 32.951 )
    ( 5051, 33.264 )
    ( 5052, 33.657 )
    ( 5053, 33.937 )
    ( 5054, 34.266 )
    ( 5055, 34.708 )
    ( 5056, 34.997 )
    ( 5057, 35.275 )
    ( 5058, 35.585 )
    ( 5059, 35.590 )
    ( 5060, 35.652 )
    ( 5061, 35.723 )
    ( 5062, 35.731 )
    ( 5063, 35.963 )
    ( 5064, 36.354 )
    ( 5065, 36.702 )
    ( 5066, 37.061 )
    ( 5067, 37.312 )
    ( 5068, 37.533 )
    ( 5069, 37.776 )
    ( 5070, 38.017 )
    ( 5071, 38.280 )
    ( 5072, 38.502 )
    ( 5073, 38.787 )
    ( 5074, 39.068 )
    ( 5075, 39.298 )
    ( 5076, 39.521 )
    ( 5077, 39.742 )
    ( 5078, 39.742 )
    ( 5079, 39.746 )
    ( 5080, 39.747 )
    ( 5081, 39.783 )
    ( 5082, 39.783 )
    ( 5083, 40.005 )
    ( 5084, 40.233 )
    ( 5085, 40.494 )
    ( 5086, 40.728 )
    ( 5087, 40.950 )
    ( 5088, 41.172 )
    ( 5089, 41.394 )
    ( 5090, 41.616 )
    ( 5091, 41.804 )
    ( 5092, 41.822 )
    ( 5093, 41.822 )
    ( 5094, 41.995 )
    ( 5095, 42.166 )
    ( 5096, 42.171 )
    ( 5097, 42.181 )
    ( 5098, 42.245 )
    ( 5099, 42.245 )
    ( 5100, 42.245 )
    ( 5101, 42.254 )
    ( 5102, 42.254 )
    ( 5103, 42.442 )
    ( 5104, 42.651 )
    ( 5105, 42.860 )
    ( 5106, 42.875 )
    ( 5107, 42.955 )
    ( 5108, 42.955 )
    ( 5109, 42.982 )
    ( 5110, 43.049 )
    ( 5111, 43.132 )
    ( 5112, 43.318 )
    ( 5113, 43.468 )
    ( 5114, 43.511 )
    ( 5115, 43.541 )
    ( 5116, 43.541 )
    ( 5117, 43.541 )
    ( 5118, 43.553 )
    ( 5119, 43.616 )
    ( 5120, 43.660 )
    ( 5121, 43.661 )
    ( 5122, 43.687 )
    ( 5123, 43.687 )
    ( 5124, 43.687 )
    ( 5125, 43.975 )
    ( 5126, 44.285 )
    ( 5127, 44.501 )
    ( 5128, 44.679 )
    ( 5129, 44.852 )
    ( 5130, 44.969 )
    ( 5131, 45.077 )
    ( 5132, 45.398 )
    ( 5133, 45.716 )
    ( 5134, 46.030 )
    ( 5135, 46.170 )
    ( 5136, 46.287 )
    ( 5137, 46.395 )
    ( 5138, 46.705 )
    ( 5139, 47.023 )
    ( 5140, 47.337 )
    ( 5141, 47.704 )
    ( 5142, 48.016 )
    ( 5143, 48.124 )
    ( 5144, 48.296 )
    ( 5145, 48.455 )
    ( 5146, 48.618 )
    ( 5147, 49.005 )
    ( 5148, 49.282 )
    ( 5149, 49.548 )
    ( 5150, 49.779 )
    ( 5151, 49.882 )
    ( 5152, 49.881 )
    ( 5153, 49.880 )
    ( 5154, 49.900 )
    ( 5155, 49.894 )
    ( 5156, 49.835 )
    ( 5157, 49.777 )
    ( 5158, 49.719 )
    ( 5159, 49.726 )
    ( 5160, 49.902 )
    ( 5161, 49.928 )
    ( 5162, 50.012 )
    ( 5163, 49.988 )
    ( 5164, 50.111 )
    ( 5165, 50.301 )
    ( 5166, 50.487 )
    ( 5167, 50.610 )
    ( 5168, 50.582 )
    ( 5169, 50.699 )
    ( 5170, 50.696 )
    ( 5171, 50.571 )
    ( 5172, 50.461 )
    ( 5173, 50.578 )
    ( 5174, 50.620 )
    ( 5175, 50.679 )
    ( 5176, 50.758 )
    ( 5177, 50.804 )
    ( 5178, 50.679 )
    ( 5179, 50.554 )
    ( 5180, 50.430 )
    ( 5181, 50.308 )
    ( 5182, 50.358 )
    ( 5183, 50.237 )
    ( 5184, 50.113 )
    ( 5185, 49.852 )
    ( 5186, 49.755 )
    ( 5187, 49.671 )
    ( 5188, 49.606 )
    ( 5189, 49.509 )
    ( 5190, 49.215 )
    ( 5191, 48.942 )
    ( 5192, 48.676 )
    ( 5193, 48.381 )
    ( 5194, 48.235 )
    ( 5195, 47.974 )
    ( 5196, 47.877 )
    ( 5197, 47.818 )
    ( 5198, 47.523 )
    ( 5199, 47.372 )
    ( 5200, 47.208 )
    ( 5201, 47.260 )
    ( 5202, 47.211 )
    ( 5203, 47.284 )
    ( 5204, 46.983 )
    ( 5205, 46.682 )
    ( 5206, 46.486 )
    ( 5207, 46.213 )
    ( 5208, 46.110 )
    ( 5209, 45.809 )
    ( 5210, 45.582 )
    ( 5211, 45.352 )
    ( 5212, 45.054 )
    ( 5213, 44.753 )
    ( 5214, 44.466 )
    ( 5215, 44.291 )
    ( 5216, 44.314 )
    ( 5217, 44.217 )
    ( 5218, 43.955 )
    ( 5219, 43.661 )
    ( 5220, 43.450 )
    ( 5221, 43.423 )
    ( 5222, 43.122 )
    ( 5223, 42.992 )
    ( 5224, 42.783 )
    ( 5225, 42.633 )
    ( 5226, 42.438 )
    ( 5227, 42.438 )
    ( 5228, 42.138 )
    ( 5229, 42.050 )
    ( 5230, 41.954 )
    ( 5231, 41.686 )
    ( 5232, 41.385 )
    ( 5233, 41.688 )
    ( 5234, 41.975 )
    ( 5235, 42.248 )
    ( 5236, 42.391 )
    ( 5237, 42.529 )
    ( 5238, 42.657 )
    ( 5239, 42.818 )
    ( 5240, 42.916 )
    ( 5241, 43.019 )
    ( 5242, 43.150 )
    ( 5243, 43.276 )
    ( 5244, 43.373 )
    ( 5245, 43.626 )
    ( 5246, 43.792 )
    ( 5247, 43.920 )
    ( 5248, 44.018 )
    ( 5249, 44.145 )
    ( 5250, 44.242 )
    ( 5251, 44.339 )
    ( 5252, 44.436 )
    ( 5253, 44.551 )
    ( 5254, 44.655 )
    ( 5255, 44.752 )
    ( 5256, 44.868 )
    ( 5257, 44.965 )
    ( 5258, 45.095 )
    ( 5259, 45.291 )
    ( 5260, 45.417 )
    ( 5261, 45.547 )
    ( 5262, 45.644 )
    ( 5263, 45.741 )
    ( 5264, 45.862 )
    ( 5265, 45.970 )
    ( 5266, 46.067 )
    ( 5267, 46.189 )
    ( 5268, 46.335 )
    ( 5269, 46.458 )
    ( 5270, 46.640 )
    ( 5271, 46.615 )
    ( 5272, 46.586 )
    ( 5273, 46.462 )
    ( 5274, 46.472 )
    ( 5275, 46.480 )
    ( 5276, 46.461 )
    ( 5277, 46.428 )
    ( 5278, 46.370 )
    ( 5279, 46.312 )
    ( 5280, 46.331 )
    ( 5281, 46.273 )
    ( 5282, 46.215 )
    ( 5283, 46.224 )
    ( 5284, 46.218 )
    ( 5285, 46.249 )
    ( 5286, 46.194 )
    ( 5287, 46.079 )
    ( 5288, 45.954 )
    ( 5289, 46.299 )
    ( 5290, 46.544 )
    ( 5291, 46.732 )
    ( 5292, 46.916 )
    ( 5293, 47.053 )
    ( 5294, 47.273 )
    ( 5295, 47.398 )
    ( 5296, 47.533 )
    ( 5297, 47.690 )
    ( 5298, 47.856 )
    ( 5299, 47.982 )
    ( 5300, 48.108 )
    ( 5301, 48.275 )
    ( 5302, 48.400 )
    ( 5303, 48.498 )
    ( 5304, 48.636 )
    ( 5305, 48.514 )
    ( 5306, 48.445 )
    ( 5307, 48.477 )
    ( 5308, 48.352 )
    ( 5309, 48.310 )
    ( 5310, 48.341 )
    ( 5311, 48.216 )
    ( 5312, 48.402 )
    ( 5313, 48.504 )
    ( 5314, 48.572 )
    ( 5315, 48.535 )
    ( 5316, 48.563 )
    ( 5317, 48.513 )
    ( 5318, 48.455 )
    ( 5319, 48.345 )
    ( 5320, 48.243 )
    ( 5321, 48.118 )
    ( 5322, 47.997 )
    ( 5323, 47.971 )
    ( 5324, 47.851 )
    ( 5325, 47.726 )
    ( 5326, 47.707 )
    ( 5327, 47.761 )
    ( 5328, 47.720 )
    ( 5329, 47.806 )
    ( 5330, 47.807 )
    ( 5331, 47.781 )
    ( 5332, 47.723 )
    ( 5333, 47.822 )
    ( 5334, 47.767 )
    ( 5335, 47.802 )
    ( 5336, 47.751 )
    ( 5337, 47.753 )
    ( 5338, 47.750 )
    ( 5339, 47.692 )
    ( 5340, 47.707 )
    ( 5341, 47.725 )
    ( 5342, 47.770 )
    ( 5343, 47.818 )
    ( 5344, 47.891 )
    ( 5345, 47.934 )
    ( 5346, 47.934 )
    ( 5347, 47.954 )
    ( 5348, 48.057 )
    ( 5349, 48.085 )
    ( 5350, 48.086 )
    ( 5351, 48.086 )
    ( 5352, 48.087 )
    ( 5353, 48.450 )
    ( 5354, 48.571 )
    ( 5355, 48.634 )
    ( 5356, 48.651 )
    ( 5357, 48.762 )
    ( 5358, 48.825 )
    ( 5359, 48.933 )
    ( 5360, 48.961 )
    ( 5361, 48.967 )
    ( 5362, 48.970 )
    ( 5363, 48.970 )
    ( 5364, 48.985 )
    ( 5365, 49.138 )
    ( 5366, 49.300 )
    ( 5367, 49.300 )
    ( 5368, 49.458 )
    ( 5369, 49.458 )
    ( 5370, 49.588 )
    ( 5371, 49.905 )
    ( 5372, 50.162 )
    ( 5373, 50.244 )
    ( 5374, 50.292 )
    ( 5375, 50.292 )
    ( 5376, 50.326 )
    ( 5377, 50.333 )
    ( 5378, 50.341 )
    ( 5379, 50.356 )
    ( 5380, 50.379 )
    ( 5381, 50.422 )
    ( 5382, 50.471 )
    ( 5383, 50.496 )
    ( 5384, 50.643 )
    ( 5385, 50.815 )
    ( 5386, 50.986 )
    ( 5387, 50.986 )
    ( 5388, 51.013 )
    ( 5389, 51.032 )
    ( 5390, 51.039 )
    ( 5391, 51.039 )
    ( 5392, 51.187 )
    ( 5393, 51.250 )
    ( 5394, 51.340 )
    ( 5395, 51.341 )
    ( 5396, 51.341 )
    ( 5397, 51.374 )
    ( 5398, 51.395 )
    ( 5399, 51.402 )
    ( 5400, 51.440 )
    ( 5401, 51.443 )
    ( 5402, 51.446 )
    ( 5403, 51.458 )
    ( 5404, 51.476 )
    ( 5405, 51.476 )
    ( 5406, 51.477 )
    ( 5407, 51.477 )
    ( 5408, 51.504 )
    ( 5409, 51.520 )
    ( 5410, 51.549 )
    ( 5411, 51.592 )
    ( 5412, 51.636 )
    ( 5413, 51.666 )
    ( 5414, 51.670 )
    ( 5415, 51.706 )
    ( 5416, 51.727 )
    ( 5417, 51.837 )
    ( 5418, 52.035 )
    ( 5419, 52.142 )
    ( 5420, 52.140 )
    ( 5421, 52.137 )
    ( 5422, 52.012 )
    ( 5423, 51.887 )
    ( 5424, 52.074 )
    ( 5425, 52.278 )
    ( 5426, 52.464 )
    ( 5427, 52.596 )
    ( 5428, 52.721 )
    ( 5429, 52.927 )
    ( 5430, 53.052 )
    ( 5431, 52.927 )
    ( 5432, 53.050 )
    ( 5433, 53.201 )
    ( 5434, 53.447 )
    ( 5435, 53.665 )
    ( 5436, 53.641 )
    ( 5437, 53.663 )
    ( 5438, 53.635 )
    ( 5439, 53.607 )
    ( 5440, 53.748 )
    ( 5441, 53.741 )
    ( 5442, 53.739 )
    ( 5443, 53.797 )
    ( 5444, 53.973 )
    ( 5445, 53.966 )
    ( 5446, 53.964 )
    ( 5447, 54.013 )
    ( 5448, 53.915 )
    ( 5449, 53.882 )
    ( 5450, 53.763 )
    ( 5451, 53.661 )
    ( 5452, 53.536 )
    ( 5453, 53.434 )
    ( 5454, 53.310 )
    ( 5455, 53.192 )
    ( 5456, 53.159 )
    ( 5457, 53.120 )
    ( 5458, 52.995 )
    ( 5459, 53.036 )
    ( 5460, 52.979 )
    ( 5461, 52.905 )
    ( 5462, 53.072 )
    ( 5463, 53.213 )
    ( 5464, 53.364 )
    ( 5465, 53.528 )
    ( 5466, 53.668 )
    ( 5467, 53.793 )
    ( 5468, 53.975 )
    ( 5469, 54.114 )
    ( 5470, 54.279 )
    ( 5471, 54.437 )
    ( 5472, 54.561 )
    ( 5473, 54.770 )
    ( 5474, 54.956 )
    ( 5475, 55.140 )
    ( 5476, 55.324 )
    ( 5477, 55.601 )
    ( 5478, 55.482 )
    ( 5479, 55.591 )
    ( 5480, 55.674 )
    ( 5481, 55.727 )
    ( 5482, 55.815 )
    ( 5483, 55.690 )
    ( 5484, 55.566 )
    ( 5485, 55.449 )
    ( 5486, 55.328 )
    ( 5487, 55.383 )
    ( 5488, 55.478 )
    ( 5489, 55.588 )
    ( 5490, 55.630 )
    ( 5491, 55.624 )
    ( 5492, 55.591 )
    ( 5493, 55.467 )
    ( 5494, 55.687 )
    ( 5495, 55.875 )
    ( 5496, 56.060 )
    ( 5497, 55.758 )
    ( 5498, 55.458 )
    ( 5499, 55.156 )
    ( 5500, 54.855 )
    ( 5501, 54.633 )
    ( 5502, 54.667 )
    ( 5503, 54.470 )
    ( 5504, 54.325 )
    ( 5505, 54.228 )
    ( 5506, 54.083 )
    ( 5507, 53.986 )
    ( 5508, 53.958 )
    ( 5509, 53.658 )
    ( 5510, 53.357 )
    ( 5511, 53.057 )
    ( 5512, 52.756 )
    ( 5513, 52.455 )
    ( 5514, 52.218 )
    ( 5515, 51.918 )
    ( 5516, 51.657 )
    ( 5517, 51.448 )
    ( 5518, 51.166 )
    ( 5519, 50.967 )
    ( 5520, 50.669 )
    ( 5521, 50.368 )
    ( 5522, 50.160 )
    ( 5523, 49.999 )
    ( 5524, 49.812 )
    ( 5525, 49.689 )
    ( 5526, 49.443 )
    ( 5527, 49.204 )
    ( 5528, 48.910 )
    ( 5529, 48.757 )
    ( 5530, 48.532 )
    ( 5531, 48.438 )
    ( 5532, 48.414 )
    ( 5533, 48.329 )
    ( 5534, 48.232 )
    ( 5535, 48.146 )
    ( 5536, 48.049 )
    ( 5537, 47.758 )
    ( 5538, 47.457 )
    ( 5539, 47.493 )
    ( 5540, 47.465 )
    ( 5541, 47.355 )
    ( 5542, 47.341 )
    ( 5543, 47.363 )
    ( 5544, 47.238 )
    ( 5545, 47.236 )
    ( 5546, 47.111 )
    ( 5547, 47.081 )
    ( 5548, 46.975 )
    ( 5549, 46.850 )
    ( 5550, 46.600 )
    ( 5551, 46.333 )
    ( 5552, 46.151 )
    ( 5553, 45.850 )
    ( 5554, 45.549 )
    ( 5555, 45.248 )
    ( 5556, 44.947 )
    ( 5557, 44.801 )
    ( 5558, 44.500 )
    ( 5559, 44.200 )
    ( 5560, 43.902 )
    ( 5561, 43.792 )
    ( 5562, 43.681 )
    ( 5563, 43.379 )
    ( 5564, 43.233 )
    ( 5565, 42.936 )
    ( 5566, 42.635 )
    ( 5567, 42.333 )
    ( 5568, 42.188 )
    ( 5569, 41.941 )
    ( 5570, 41.691 )
    ( 5571, 41.510 )
    ( 5572, 41.688 )
    ( 5573, 41.494 )
    ( 5574, 41.473 )
    ( 5575, 41.412 )
    ( 5576, 41.266 )
    ( 5577, 41.299 )
    ( 5578, 41.291 )
    ( 5579, 41.194 )
    ( 5580, 41.146 )
    ( 5581, 41.049 )
    ( 5582, 40.989 )
    ( 5583, 40.689 )
    ( 5584, 40.396 )
    ( 5585, 40.199 )
    ( 5586, 39.903 )
    ( 5587, 39.631 )
    ( 5588, 39.477 )
    ( 5589, 39.216 )
    ( 5590, 38.917 )
    ( 5591, 38.852 )
    ( 5592, 38.755 )
    ( 5593, 38.659 )
    ( 5594, 38.699 )
    ( 5595, 38.723 )
    ( 5596, 38.462 )
    ( 5597, 38.283 )
    ( 5598, 38.097 )
    ( 5599, 37.796 )
    ( 5600, 37.529 )
    ( 5601, 37.234 )
    ( 5602, 36.976 )
    ( 5603, 36.743 )
    ( 5604, 36.442 )
    ( 5605, 36.175 )
    ( 5606, 35.979 )
    ( 5607, 35.681 )
    ( 5608, 35.452 )
    ( 5609, 35.241 )
    ( 5610, 35.030 )
    ( 5611, 34.730 )
    ( 5612, 34.497 )
    ( 5613, 34.196 )
    ( 5614, 34.359 )
    ( 5615, 34.456 )
    ( 5616, 34.741 )
    ( 5617, 34.998 )
    ( 5618, 35.094 )
    ( 5619, 35.390 )
    ( 5620, 35.486 )
    ( 5621, 35.650 )
    ( 5622, 35.772 )
    ( 5623, 35.994 )
    ( 5624, 36.192 )
    ( 5625, 36.179 )
    ( 5626, 36.156 )
    ( 5627, 36.100 )
    ( 5628, 36.042 )
    ( 5629, 35.942 )
    ( 5630, 35.817 )
    ( 5631, 35.692 )
    ( 5632, 35.735 )
    ( 5633, 35.731 )
    ( 5634, 35.755 )
    ( 5635, 35.727 )
    ( 5636, 35.690 )
    ( 5637, 35.640 )
    ( 5638, 35.595 )
    ( 5639, 35.537 )
    ( 5640, 35.480 )
    ( 5641, 35.422 )
    ( 5642, 35.430 )
    ( 5643, 35.373 )
    ( 5644, 35.314 )
    ( 5645, 35.257 )
    ( 5646, 35.245 )
    ( 5647, 35.225 )
    ( 5648, 35.167 )
    ( 5649, 35.226 )
    ( 5650, 35.352 )
    ( 5651, 35.372 )
    ( 5652, 35.313 )
    ( 5653, 35.315 )
    ( 5654, 35.261 )
    ( 5655, 35.203 )
    ( 5656, 34.902 )
    ( 5657, 34.607 )
    ( 5658, 34.516 )
    ( 5659, 34.423 )
    ( 5660, 34.289 )
    ( 5661, 34.099 )
    ( 5662, 33.812 )
    ( 5663, 33.574 )
    ( 5664, 33.312 )
    ( 5665, 33.041 )
    ( 5666, 32.895 )
    ( 5667, 32.599 )
    ( 5668, 32.298 )
    ( 5669, 32.154 )
    ( 5670, 32.110 )
    ( 5671, 32.135 )
    ( 5672, 32.206 )
    ( 5673, 32.067 )
    ( 5674, 31.921 )
    ( 5675, 31.887 )
    ( 5676, 31.846 )
    ( 5677, 31.781 )
    ( 5678, 31.481 )
    ( 5679, 31.180 )
    ( 5680, 30.932 )
    ( 5681, 30.736 )
    ( 5682, 30.436 )
    ( 5683, 30.148 )
    ( 5684, 29.952 )
    ( 5685, 29.651 )
    ( 5686, 29.406 )
    ( 5687, 29.341 )
    ( 5688, 29.143 )
    ( 5689, 28.932 )
    ( 5690, 28.638 )
    ( 5691, 28.337 )
    ( 5692, 28.036 )
    ( 5693, 27.769 )
    ( 5694, 27.469 )
    ( 5695, 27.167 )
    ( 5696, 26.867 )
    ( 5697, 26.860 )
    ( 5698, 26.802 )
    ( 5699, 26.747 )
    ( 5700, 26.446 )
    ( 5701, 26.174 )
    ( 5702, 25.873 )
    ( 5703, 25.784 )
    ( 5704, 25.741 )
    ( 5705, 25.685 )
    ( 5706, 25.625 )
    ( 5707, 25.323 )
    ( 5708, 25.088 )
    ( 5709, 24.794 )
    ( 5710, 24.520 )
    ( 5711, 24.374 )
    ( 5712, 24.169 )
    ( 5713, 23.876 )
    ( 5714, 23.646 )
    ( 5715, 23.540 )
    ( 5716, 23.469 )
    ( 5717, 23.410 )
    ( 5718, 23.173 )
    ( 5719, 23.003 )
    ( 5720, 22.715 )
    ( 5721, 22.625 )
    ( 5722, 22.643 )
    ( 5723, 22.631 )
    ( 5724, 22.588 )
    ( 5725, 22.330 )
    ( 5726, 22.159 )
    ( 5727, 21.893 )
    ( 5728, 21.595 )
    ( 5729, 21.294 )
    ( 5730, 21.237 )
    ( 5731, 21.295 )
    ( 5732, 21.276 )
    ( 5733, 21.218 )
    ( 5734, 21.185 )
    ( 5735, 21.181 )
    ( 5736, 21.205 )
    ( 5737, 21.302 )
    ( 5738, 21.455 )
    ( 5739, 21.712 )
    ( 5740, 21.814 )
    ( 5741, 21.911 )
    ( 5742, 22.015 )
    ( 5743, 22.118 )
    ( 5744, 22.221 )
    ( 5745, 22.225 )
    ( 5746, 22.202 )
    ( 5747, 22.254 )
    ( 5748, 22.231 )
    ( 5749, 22.213 )
    ( 5750, 22.299 )
    ( 5751, 22.383 )
    ( 5752, 22.738 )
    ( 5753, 22.998 )
    ( 5754, 23.286 )
    ( 5755, 23.564 )
    ( 5756, 23.740 )
    ( 5757, 23.916 )
    ( 5758, 24.172 )
    ( 5759, 24.427 )
    ( 5760, 24.720 )
    ( 5761, 24.949 )
    ( 5762, 25.228 )
    ( 5763, 25.489 )
    ( 5764, 25.710 )
    ( 5765, 25.923 )
    ( 5766, 26.122 )
    ( 5767, 26.186 )
    ( 5768, 26.128 )
    ( 5769, 25.836 )
    ( 5770, 25.692 )
    ( 5771, 25.392 )
    ( 5772, 25.246 )
    ( 5773, 24.947 )
    ( 5774, 24.646 )
    ( 5775, 24.345 )
    ( 5776, 24.044 )
    ( 5777, 23.743 )
    ( 5778, 23.442 )
    ( 5779, 23.299 )
    ( 5780, 23.153 )
    ( 5781, 22.856 )
    ( 5782, 22.575 )
    ( 5783, 22.338 )
    ( 5784, 22.045 )
    ( 5785, 21.744 )
    ( 5786, 21.533 )
    ( 5787, 21.232 )
    ( 5788, 20.931 )
    ( 5789, 20.630 )
    ( 5790, 20.329 )
    ( 5791, 20.028 )
    ( 5792, 19.727 )
    ( 5793, 19.909 )
    ( 5794, 20.006 )
    ( 5795, 20.172 )
    ( 5796, 20.297 )
    ( 5797, 20.459 )
    ( 5798, 20.695 )
    ( 5799, 20.948 )
    ( 5800, 21.178 )
    ( 5801, 21.281 )
    ( 5802, 21.386 )
    ( 5803, 21.697 )
    ( 5804, 21.794 )
    ( 5805, 22.088 )
    ( 5806, 22.383 )
    ( 5807, 22.648 )
    ( 5808, 22.848 )
    ( 5809, 22.945 )
    ( 5810, 23.098 )
    ( 5811, 23.220 )
    ( 5812, 23.346 )
    ( 5813, 23.537 )
    ( 5814, 23.683 )
    ( 5815, 23.823 )
    ( 5816, 23.984 )
    ( 5817, 24.228 )
    ( 5818, 24.395 )
    ( 5819, 24.337 )
    ( 5820, 24.224 )
    ( 5821, 24.104 )
    ( 5822, 23.979 )
    ( 5823, 23.948 )
    ( 5824, 23.823 )
    ( 5825, 23.755 )
    ( 5826, 23.630 )
    ( 5827, 23.587 )
    ( 5828, 23.462 )
    ( 5829, 23.167 )
    ( 5830, 22.866 )
    ( 5831, 22.565 )
    ( 5832, 22.500 )
    ( 5833, 22.403 )
    ( 5834, 22.126 )
    ( 5835, 21.916 )
    ( 5836, 21.644 )
    ( 5837, 21.558 )
    ( 5838, 21.567 )
    ( 5839, 21.401 )
    ( 5840, 21.100 )
    ( 5841, 20.852 )
    ( 5842, 20.622 )
    ( 5843, 20.321 )
    ( 5844, 20.281 )
    ( 5845, 19.980 )
    ( 5846, 20.160 )
    ( 5847, 20.408 )
    ( 5848, 20.515 )
    ( 5849, 20.622 )
    ( 5850, 20.748 )
    ( 5851, 20.870 )
    ( 5852, 20.805 )
    ( 5853, 20.504 )
    ( 5854, 20.274 )
    ( 5855, 20.043 )
    ( 5856, 19.773 )
    ( 5857, 19.575 )
    ( 5858, 19.348 )
    ( 5859, 19.124 )
    ( 5860, 18.823 )
    ( 5861, 18.765 )
    ( 5862, 18.712 )
    ( 5863, 18.655 )
    ( 5864, 18.729 )
    ( 5865, 18.723 )
    ( 5866, 18.699 )
    ( 5867, 18.671 )
    ( 5868, 19.033 )
    ( 5869, 19.362 )
    ( 5870, 19.620 )
    ( 5871, 19.855 )
    ( 5872, 19.827 )
    ( 5873, 19.807 )
    ( 5874, 19.779 )
    ( 5875, 19.654 )
    ( 5876, 19.546 )
    ( 5877, 19.421 )
    ( 5878, 19.301 )
    ( 5879, 19.585 )
    ( 5880, 19.830 )
    ( 5881, 19.956 )
    ( 5882, 20.081 )
    ( 5883, 20.039 )
    ( 5884, 19.936 )
    ( 5885, 20.049 )
    ( 5886, 19.982 )
    ( 5887, 20.101 )
    ( 5888, 20.269 )
    ( 5889, 20.391 )
    ( 5890, 20.266 )
    ( 5891, 20.208 )
    ( 5892, 20.282 )
    ( 5893, 20.340 )
    ( 5894, 20.349 )
    ( 5895, 20.358 )
    ( 5896, 20.331 )
    ( 5897, 20.303 )
    ( 5898, 20.178 )
    ( 5899, 20.053 )
    ( 5900, 20.123 )
    ( 5901, 20.234 )
    ( 5902, 20.276 )
    ( 5903, 20.319 )
    ( 5904, 20.360 )
    ( 5905, 20.317 )
    ( 5906, 20.276 )
    ( 5907, 20.408 )
    ( 5908, 20.283 )
    ( 5909, 20.230 )
    ( 5910, 20.105 )
    ( 5911, 20.009 )
    ( 5912, 19.917 )
    ( 5913, 19.853 )
    ( 5914, 19.757 )
    ( 5915, 19.661 )
    ( 5916, 19.564 )
    ( 5917, 19.609 )
    ( 5918, 19.523 )
    ( 5919, 19.427 )
    ( 5920, 19.330 )
    ( 5921, 19.034 )
    ( 5922, 18.738 )
    ( 5923, 18.439 )
    ( 5924, 18.138 )
    ( 5925, 18.052 )
    ( 5926, 17.837 )
    ( 5927, 17.536 )
    ( 5928, 17.235 )
    ( 5929, 17.089 )
    ( 5930, 16.794 )
    ( 5931, 16.526 )
    ( 5932, 16.380 )
    ( 5933, 16.283 )
    ( 5934, 16.015 )
    ( 5935, 15.768 )
    ( 5936, 15.497 )
    ( 5937, 15.267 )
    ( 5938, 15.056 )
    ( 5939, 14.756 )
    ( 5940, 14.546 )
    ( 5941, 14.246 )
    ( 5942, 13.953 )
    ( 5943, 13.664 )
    ( 5944, 13.432 )
    ( 5945, 13.131 )
    ( 5946, 12.934 )
    ( 5947, 12.633 )
    ( 5948, 12.660 )
    ( 5949, 12.359 )
    ( 5950, 12.058 )
    ( 5951, 12.255 )
    ( 5952, 12.489 )
    ( 5953, 12.614 )
    ( 5954, 12.712 )
    ( 5955, 12.842 )
    ( 5956, 12.946 )
    ( 5957, 13.139 )
    ( 5958, 13.336 )
    ( 5959, 13.505 )
    ( 5960, 13.637 )
    ( 5961, 13.759 )
    ( 5962, 13.733 )
    ( 5963, 13.639 )
    ( 5964, 13.542 )
    ( 5965, 13.332 )
    ( 5966, 13.031 )
    ( 5967, 12.990 )
    ( 5968, 12.893 )
    ( 5969, 12.605 )
    ( 5970, 12.304 )
    ( 5971, 12.108 )
    ( 5972, 11.807 )
    ( 5973, 11.918 )
    ( 5974, 12.022 )
    ( 5975, 12.175 )
    ( 5976, 12.277 )
    ( 5977, 12.394 )
    ( 5978, 12.509 )
    ( 5979, 12.630 )
    ( 5980, 12.881 )
    ( 5981, 13.035 )
    ( 5982, 13.095 )
    ( 5983, 13.158 )
    ( 5984, 13.177 )
    ( 5985, 13.310 )
    ( 5986, 13.310 )
    ( 5987, 13.208 )
    ( 5988, 13.083 )
    ( 5989, 12.991 )
    ( 5990, 13.016 )
    ( 5991, 13.069 )
    ( 5992, 13.004 )
    ( 5993, 12.963 )
    ( 5994, 12.838 )
    ( 5995, 12.879 )
    ( 5996, 12.980 )
    ( 5997, 12.862 )
    ( 5998, 12.737 )
    ( 5999, 12.783 )
    ( 6000, 12.832 )
    ( 6001, 12.874 )
    ( 6002, 12.928 )
    ( 6003, 12.875 )
    ( 6004, 13.010 )
    ( 6005, 12.895 )
    ( 6006, 12.770 )
    ( 6007, 12.665 )
    ( 6008, 12.541 )
    ( 6009, 12.427 )
    ( 6010, 12.304 )
    ( 6011, 12.202 )
    ( 6012, 12.319 )
    ( 6013, 12.194 )
    ( 6014, 12.190 )
    ( 6015, 11.889 )
    ( 6016, 11.945 )
    ( 6017, 11.883 )
    ( 6018, 11.786 )
    ( 6019, 11.759 )
    ( 6020, 11.548 )
    ( 6021, 11.248 )
    ( 6022, 11.117 )
    ( 6023, 10.970 )
    ( 6024, 10.673 )
    ( 6025, 10.372 )
    ( 6026, 10.212 )
    ( 6027, 9.9446 )
    ( 6028, 9.8558 )
    ( 6029, 9.7473 )
    ( 6030, 9.5511 )
    ( 6031, 9.3562 )
    ( 6032, 9.2103 )
    ( 6033, 8.9106 )
    ( 6034, 8.8831 )
    ( 6035, 8.6691 )
    ( 6036, 8.3701 )
    ( 6037, 8.0697 )
    ( 6038, 7.7993 )
    ( 6039, 7.4983 )
    ( 6040, 7.5962 )
    ( 6041, 7.6901 )
    ( 6042, 7.7107 )
    ( 6043, 7.9309 )
    ( 6044, 8.0580 )
    ( 6045, 8.1942 )
    ( 6046, 8.3381 )
    ( 6047, 8.4476 )
    ( 6048, 8.5973 )
    ( 6049, 8.9855 )
    ( 6050, 9.3085 )
    ( 6051, 9.5088 )
    ( 6052, 9.8776 )
    ( 6053, 10.141 )
    ( 6054, 10.387 )
    ( 6055, 10.606 )
    ( 6056, 10.826 )
    ( 6057, 11.142 )
    ( 6058, 11.413 )
    ( 6059, 11.112 )
    ( 6060, 11.110 )
    ( 6061, 10.985 )
    ( 6062, 10.728 )
    ( 6063, 10.491 )
    ( 6064, 10.203 )
    ( 6065, 10.269 )
    ( 6066, 10.172 )
    ( 6067, 10.120 )
    ( 6068, 9.8589 )
    ( 6069, 9.5579 )
    ( 6070, 9.3862 )
    ( 6071, 9.0908 )
    ( 6072, 8.7899 )
    ( 6073, 8.6506 )
    ( 6074, 8.3496 )
    ( 6075, 8.2528 )
    ( 6076, 8.0648 )
    ( 6077, 8.2357 )
    ( 6078, 8.4243 )
    ( 6079, 8.3663 )
    ( 6080, 8.0653 )
    ( 6081, 7.9374 )
    ( 6082, 7.9344 )
    ( 6083, 7.9924 )
    ( 6084, 8.0198 )
    ( 6085, 8.0668 )
    ( 6086, 8.0817 )
    ( 6087, 8.0748 )
    ( 6088, 7.9263 )
    ( 6089, 7.6259 )
    ( 6090, 7.3264 )
    ( 6091, 7.0253 )
    ( 6092, 7.0701 )
    ( 6093, 7.0529 )
    ( 6094, 6.9371 )
    ( 6095, 7.1083 )
    ( 6096, 7.2974 )
    ( 6097, 7.4319 )
    ( 6098, 7.5568 )
    ( 6099, 7.7647 )
    ( 6100, 7.6486 )
    ( 6101, 7.6905 )
    ( 6102, 7.6871 )
    ( 6103, 7.3860 )
    ( 6104, 7.2625 )
    ( 6105, 7.2487 )
    ( 6106, 7.1248 )
    ( 6107, 6.9999 )
    ( 6108, 6.9235 )
    ( 6109, 7.0244 )
    ( 6110, 6.8995 )
    ( 6111, 6.6008 )
    ( 6112, 6.3899 )
    ( 6113, 6.0889 )
    ( 6114, 6.0781 )
    ( 6115, 6.0746 )
    ( 6116, 6.0287 )
    ( 6117, 5.9708 )
    ( 6118, 5.9563 )
    ( 6119, 6.0929 )
    ( 6120, 6.2273 )
    ( 6121, 6.2853 )
    ( 6122, 6.3422 )
    ( 6123, 6.3505 )
    ( 6124, 6.2960 )
    ( 6125, 6.2554 )
    ( 6126, 6.2495 )
    ( 6127, 6.1915 )
    ( 6128, 5.8905 )
    ( 6129, 5.9485 )
    ( 6130, 5.8906 )
    ( 6131, 5.8911 )
    ( 6132, 6.1143 )
    ( 6133, 6.1477 )
    ( 6134, 6.1480 )
    ( 6135, 6.6390 )
    ( 6136, 6.8611 )
    ( 6137, 7.1378 )
    ( 6138, 7.3970 )
    ( 6139, 7.3970 )
    ( 6140, 7.4408 )
    ( 6141, 7.5729 )
    ( 6142, 7.6352 )
    ( 6143, 7.7310 )
    ( 6144, 7.7745 )
    ( 6145, 7.7745 )
    ( 6146, 8.1107 )
    ( 6147, 8.3326 )
    ( 6148, 8.6516 )
    ( 6149, 8.9690 )
    ( 6150, 9.2103 )
    ( 6151, 9.4215 )
    ( 6152, 9.5964 )
    ( 6153, 9.8723 )
    ( 6154, 10.043 )
    ( 6155, 10.376 )
    ( 6156, 10.864 )
    ( 6157, 11.205 )
    ( 6158, 11.360 )
    ( 6159, 11.506 )
    ( 6160, 11.514 )
    ( 6161, 11.623 )
    ( 6162, 11.640 )
    ( 6163, 11.640 )
    ( 6164, 11.719 )
    ( 6165, 11.720 )
    ( 6166, 11.619 )
    ( 6167, 11.318 )
    ( 6168, 11.081 )
    ( 6169, 10.820 )
    ( 6170, 10.733 )
    ( 6171, 10.432 )
    ( 6172, 10.379 )
    ( 6173, 10.304 )
    ( 6174, 10.430 )
    ( 6175, 10.555 )
    ( 6176, 10.687 )
    ( 6177, 10.837 )
    ( 6178, 10.712 )
    ( 6179, 10.862 )
    ( 6180, 11.102 )
    ( 6181, 11.284 )
    ( 6182, 11.376 )
    ( 6183, 11.499 )
    ( 6184, 11.633 )
    ( 6185, 11.634 )
    ( 6186, 11.620 )
    ( 6187, 11.644 )
    ( 6188, 11.639 )
    ( 6189, 11.684 )
    ( 6190, 11.746 )
    ( 6191, 11.673 )
    ( 6192, 11.548 )
    ( 6193, 11.557 )
    ( 6194, 11.499 )
    ( 6195, 11.561 )
    ( 6196, 11.559 )
    ( 6197, 11.587 )
    ( 6198, 11.578 )
    ( 6199, 11.550 )
    ( 6200, 11.818 )
    ( 6201, 12.051 )
    ( 6202, 12.235 )
    ( 6203, 12.119 )
    ( 6204, 11.994 )
    ( 6205, 11.869 )
    ( 6206, 12.053 )
    ( 6207, 12.231 )
    ( 6208, 12.514 )
    ( 6209, 12.697 )
    ( 6210, 12.947 )
    ( 6211, 13.180 )
    ( 6212, 13.508 )
    ( 6213, 13.764 )
    ( 6214, 14.040 )
    ( 6215, 14.040 )
    ( 6216, 14.060 )
    ( 6217, 14.075 )
    ( 6218, 13.947 )
    ( 6219, 13.823 )
    ( 6220, 13.522 )
    ( 6221, 13.221 )
    ( 6222, 13.010 )
    ( 6223, 12.780 )
    ( 6224, 12.479 )
    ( 6225, 12.530 )
    ( 6226, 12.523 )
    ( 6227, 12.398 )
    ( 6228, 12.301 )
    ( 6229, 12.003 )
    ( 6230, 11.756 )
    ( 6231, 11.559 )
    ( 6232, 11.364 )
    ( 6233, 11.218 )
    ( 6234, 10.959 )
    ( 6235, 10.658 )
    ( 6236, 10.371 )
    ( 6237, 10.192 )
    ( 6238, 9.9014 )
    ( 6239, 9.7552 )
    ( 6240, 9.5145 )
    ( 6241, 9.3689 )
    ( 6242, 9.4274 )
    ( 6243, 9.2899 )
    ( 6244, 9.1783 )
    ( 6245, 8.8773 )
    ( 6246, 8.8551 )
    ( 6247, 8.8121 )
    ( 6248, 8.7948 )
    ( 6249, 8.8506 )
    ( 6250, 8.8229 )
    ( 6251, 9.1163 )
    ( 6252, 9.3342 )
    ( 6253, 9.5939 )
    ( 6254, 9.8978 )
    ( 6255, 10.153 )
    ( 6256, 10.061 )
    ( 6257, 9.8378 )
    ( 6258, 9.5428 )
    ( 6259, 9.2422 )
    ( 6260, 8.9906 )
    ( 6261, 8.7611 )
    ( 6262, 8.4601 )
    ( 6263, 8.4536 )
    ( 6264, 8.5380 )
    ( 6265, 8.5902 )
    ( 6266, 8.5623 )
    ( 6267, 8.4373 )
    ( 6268, 8.2114 )
    ( 6269, 7.9266 )
    ( 6270, 7.7884 )
    ( 6271, 7.4874 )
    ( 6272, 7.4523 )
    ( 6273, 7.3484 )
    ( 6274, 7.2737 )
    ( 6275, 7.4578 )
    ( 6276, 7.6353 )
    ( 6277, 7.8127 )
    ( 6278, 8.0870 )
    ( 6279, 8.3435 )
    ( 6280, 8.5276 )
    ( 6281, 8.6659 )
    ( 6282, 8.7909 )
    ( 6283, 8.9476 )
    ( 6284, 9.1062 )
    ( 6285, 9.2969 )
    ( 6286, 9.1720 )
    ( 6287, 9.4192 )
    ( 6288, 9.3677 )
    ( 6289, 9.2429 )
    ( 6290, 9.6428 )
    ( 6291, 9.9503 )
    ( 6292, 10.184 )
    ( 6293, 10.439 )
    ( 6294, 10.628 )
    ( 6295, 10.696 )
    ( 6296, 10.865 )
    ( 6297, 10.995 )
    ( 6298, 11.104 )
    ( 6299, 11.201 )
    ( 6300, 11.472 )
    ( 6301, 11.769 )
    ( 6302, 11.893 )
    ( 6303, 12.055 )
    ( 6304, 12.158 )
    ( 6305, 12.259 )
    ( 6306, 12.387 )
    ( 6307, 12.484 )
    ( 6308, 12.589 )
    ( 6309, 12.686 )
    ( 6310, 12.783 )
    ( 6311, 12.880 )
    ( 6312, 13.050 )
    ( 6313, 13.204 )
    ( 6314, 13.373 )
    ( 6315, 13.391 )
    ( 6316, 13.405 )
    ( 6317, 13.347 )
    ( 6318, 13.047 )
    ( 6319, 12.796 )
    ( 6320, 12.735 )
    ( 6321, 12.589 )
    ( 6322, 12.314 )
    ( 6323, 12.043 )
    ( 6324, 11.813 )
    ( 6325, 11.880 )
    ( 6326, 11.786 )
    ( 6327, 11.485 )
    ( 6328, 11.383 )
    ( 6329, 11.304 )
    ( 6330, 11.221 )
    ( 6331, 11.096 )
    ( 6332, 10.971 )
    ( 6333, 10.897 )
    ( 6334, 10.925 )
    ( 6335, 10.979 )
    ( 6336, 10.861 )
    ( 6337, 10.753 )
    ( 6338, 10.628 )
    ( 6339, 10.514 )
    ( 6340, 10.407 )
    ( 6341, 10.282 )
    ( 6342, 10.418 )
    ( 6343, 10.383 )
    ( 6344, 10.325 )
    ( 6345, 10.297 )
    ( 6346, 10.294 )
    ( 6347, 10.179 )
    ( 6348, 10.054 )
    ( 6349, 10.101 )
    ( 6350, 9.9757 )
    ( 6351, 10.124 )
    ( 6352, 10.249 )
    ( 6353, 10.291 )
    ( 6354, 10.229 )
    ( 6355, 10.106 )
    ( 6356, 9.9932 )
    ( 6357, 9.8683 )
    ( 6358, 9.7440 )
    ( 6359, 9.6409 )
    ( 6360, 9.5160 )
    ( 6361, 9.2604 )
    ( 6362, 9.0239 )
    ( 6363, 8.7639 )
    ( 6364, 8.5062 )
    ( 6365, 8.2177 )
    ( 6366, 7.9166 )
    ( 6367, 7.6808 )
    ( 6368, 7.3810 )
    ( 6369, 7.0807 )
    ( 6370, 6.7797 )
    ( 6371, 6.7993 )
    ( 6372, 7.0769 )
    ( 6373, 6.9848 )
    ( 6374, 6.7144 )
    ( 6375, 6.6408 )
    ( 6376, 6.3398 )
    ( 6377, 6.0439 )
    ( 6378, 5.7429 )
    ( 6379, 6.0621 )
    ( 6380, 6.3267 )
    ( 6381, 6.6205 )
    ( 6382, 6.6068 )
    ( 6383, 6.5551 )
    ( 6384, 6.5487 )
    ( 6385, 6.4907 )
    ( 6386, 6.2972 )
    ( 6387, 5.9962 )
    ( 6388, 6.0657 )
    ( 6389, 6.1071 )
    ( 6390, 6.2728 )
    ( 6391, 6.2277 )
    ( 6392, 6.2350 )
    ( 6393, 6.2350 )
    ( 6394, 6.4668 )
    ( 6395, 6.9166 )
    ( 6396, 7.2733 )
    ( 6397, 7.6934 )
    ( 6398, 7.9906 )
    ( 6399, 8.2156 )
    ( 6400, 8.4520 )
    ( 6401, 8.7208 )
    ( 6402, 8.9796 )
    ( 6403, 9.2566 )
    ( 6404, 9.2737 )
    ( 6405, 9.2952 )
    ( 6406, 9.4413 )
    ( 6407, 9.5078 )
    ( 6408, 9.7710 )
    ( 6409, 9.9723 )
    ( 6410, 10.169 )
    ( 6411, 10.392 )
    ( 6412, 10.585 )
    ( 6413, 10.755 )
    ( 6414, 10.771 )
    ( 6415, 10.626 )
    ( 6416, 10.380 )
    ( 6417, 10.169 )
    ( 6418, 9.9192 )
    ( 6419, 9.6183 )
    ( 6420, 9.5754 )
    ( 6421, 9.2789 )
    ( 6422, 8.9790 )
    ( 6423, 8.8558 )
    ( 6424, 8.7108 )
    ( 6425, 8.4098 )
    ( 6426, 8.1128 )
    ( 6427, 7.9166 )
    ( 6428, 7.6932 )
    ( 6429, 7.3948 )
    ( 6430, 7.0938 )
    ( 6431, 7.2170 )
    ( 6432, 7.1752 )
    ( 6433, 7.0782 )
    ( 6434, 6.8478 )
    ( 6435, 6.6606 )
    ( 6436, 6.3644 )
    ( 6437, 6.0634 )
    ( 6438, 6.2599 )
    ( 6439, 6.3568 )
    ( 6440, 6.4678 )
    ( 6441, 6.3688 )
    ( 6442, 6.1821 )
    ( 6443, 5.8906 )
    ( 6444, 5.5895 )
    ( 6445, 5.5537 )
    ( 6446, 5.2527 )
    ( 6447, 5.1526 )
    ( 6448, 5.0278 )
    ( 6449, 5.2222 )
    ( 6450, 5.3070 )
    ( 6451, 5.3485 )
    ( 6452, 5.4583 )
    ( 6453, 5.3334 )
    ( 6454, 5.2702 )
    ( 6455, 5.2432 )
    ( 6456, 4.9422 )
    ( 6457, 4.8996 )
    ( 6458, 4.7036 )
    ( 6459, 4.5078 )
    ( 6460, 4.2068 )
    ( 6461, 4.4077 )
    ( 6462, 4.4897 )
    ( 6463, 4.4905 )
    ( 6464, 4.7302 )
    ( 6465, 4.7818 )
    ( 6466, 4.7822 )
};


==> H414288 <==
\addplot[color=blue] coordinates{
( 0 , 5.617 )
( 1 , 5.980 )
( 2 , 6.180 )
( 3 , 6.355 )
( 4 , 6.532 )
( 5 , 6.712 )
( 6 , 6.888 )
( 7 , 7.139 )
( 8 , 7.493 )
( 9 , 7.676 )
( 10 , 7.905 )
( 11 , 8.100 )
( 12 , 8.476 )
( 13 , 8.708 )
( 14 , 8.775 )
( 15 , 8.861 )
( 16 , 9.021 )
( 17 , 9.193 )
( 18 , 9.286 )
( 19 , 9.355 )
( 20 , 9.560 )
( 21 , 9.647 )
( 22 , 9.647 )
( 23 , 9.647 )
( 24 , 9.715 )
( 25 , 9.721 )
( 26 , 9.721 )
( 27 , 10.02 )
( 28 , 10.25 )
( 29 , 10.56 )
( 30 , 10.85 )
( 31 , 11.01 )
( 32 , 11.15 )
( 33 , 11.29 )
( 34 , 11.36 )
( 35 , 11.44 )
( 36 , 11.61 )
( 37 , 11.76 )
( 38 , 12.00 )
( 39 , 12.00 )
( 40 , 12.03 )
( 41 , 12.04 )
( 42 , 12.11 )
( 43 , 12.22 )
( 44 , 12.23 )
( 45 , 12.23 )
( 46 , 12.40 )
( 47 , 12.40 )
( 48 , 12.57 )
( 49 , 12.79 )
( 50 , 12.89 )
( 51 , 13.06 )
( 52 , 13.14 )
( 53 , 13.25 )
( 54 , 13.41 )
( 55 , 13.65 )
( 56 , 13.74 )
( 57 , 13.91 )
( 58 , 13.99 )
( 59 , 14.09 )
( 60 , 14.22 )
( 61 , 14.31 )
( 62 , 14.38 )
( 63 , 14.44 )
( 64 , 14.78 )
( 65 , 14.96 )
( 66 , 15.18 )
( 67 , 15.35 )
( 68 , 15.53 )
( 69 , 15.71 )
( 70 , 15.92 )
( 71 , 16.15 )
( 72 , 16.34 )
( 73 , 16.52 )
( 74 , 16.78 )
( 75 , 16.96 )
( 76 , 17.14 )
( 77 , 17.37 )
( 78 , 17.55 )
( 79 , 17.77 )
( 80 , 17.94 )
( 81 , 18.21 )
( 82 , 18.57 )
( 83 , 18.91 )
( 84 , 19.24 )
( 85 , 19.55 )
( 86 , 19.89 )
( 87 , 20.21 )
( 88 , 20.52 )
( 89 , 20.91 )
( 90 , 21.26 )
( 91 , 21.52 )
( 92 , 21.77 )
( 93 , 22.04 )
( 94 , 22.31 )
( 95 , 22.36 )
( 96 , 22.40 )
( 97 , 22.37 )
( 98 , 22.25 )
( 99 , 22.25 )
( 100 , 22.19 )
( 101 , 22.13 )
( 102 , 22.09 )
( 103 , 22.07 )
( 104 , 22.01 )
( 105 , 21.90 )
( 106 , 22.03 )
( 107 , 22.38 )
( 108 , 22.64 )
( 109 , 22.77 )
( 110 , 22.64 )
( 111 , 22.60 )
( 112 , 22.56 )
( 113 , 22.52 )
( 114 , 22.61 )
( 115 , 22.65 )
( 116 , 22.53 )
( 117 , 22.40 )
( 118 , 22.33 )
( 119 , 22.20 )
( 120 , 22.08 )
( 121 , 21.96 )
( 122 , 21.92 )
( 123 , 21.88 )
( 124 , 21.84 )
( 125 , 21.79 )
( 126 , 21.84 )
( 127 , 21.89 )
( 128 , 21.93 )
( 129 , 22.05 )
( 130 , 22.18 )
( 131 , 22.30 )
( 132 , 22.44 )
( 133 , 22.37 )
( 134 , 22.26 )
( 135 , 22.14 )
( 136 , 22.01 )
( 137 , 21.93 )
( 138 , 21.80 )
( 139 , 21.78 )
( 140 , 21.77 )
( 141 , 21.47 )
( 142 , 21.17 )
( 143 , 20.96 )
( 144 , 20.75 )
( 145 , 20.56 )
( 146 , 20.60 )
( 147 , 20.59 )
( 148 , 20.58 )
( 149 , 20.64 )
( 150 , 20.70 )
( 151 , 20.69 )
( 152 , 20.71 )
( 153 , 20.69 )
( 154 , 20.68 )
( 155 , 20.62 )
( 156 , 20.56 )
( 157 , 20.53 )
( 158 , 20.49 )
( 159 , 20.45 )
( 160 , 20.44 )
( 161 , 20.39 )
( 162 , 20.33 )
( 163 , 20.35 )
( 164 , 20.36 )
( 165 , 20.32 )
( 166 , 20.36 )
( 167 , 20.37 )
( 168 , 20.38 )
( 169 , 20.38 )
( 170 , 20.08 )
( 171 , 19.82 )
( 172 , 19.56 )
( 173 , 19.30 )
( 174 , 19.07 )
( 175 , 18.77 )
( 176 , 18.55 )
( 177 , 18.25 )
( 178 , 18.11 )
( 179 , 17.82 )
( 180 , 17.68 )
( 181 , 17.38 )
( 182 , 17.08 )
( 183 , 16.93 )
( 184 , 16.63 )
( 185 , 16.35 )
( 186 , 16.05 )
( 187 , 16.04 )
( 188 , 15.74 )
( 189 , 15.44 )
( 190 , 15.14 )
( 191 , 15.36 )
( 192 , 15.53 )
( 193 , 15.64 )
( 194 , 15.74 )
( 195 , 15.89 )
( 196 , 16.03 )
( 197 , 15.97 )
( 198 , 16.03 )
( 199 , 15.97 )
( 200 , 16.06 )
( 201 , 16.16 )
( 202 , 16.35 )
( 203 , 16.39 )
( 204 , 16.43 )
( 205 , 16.52 )
( 206 , 16.53 )
( 207 , 16.50 )
( 208 , 16.53 )
( 209 , 16.52 )
( 210 , 16.54 )
( 211 , 16.49 )
( 212 , 16.55 )
( 213 , 16.61 )
( 214 , 16.55 )
( 215 , 16.51 )
( 216 , 16.45 )
( 217 , 16.39 )
( 218 , 16.41 )
( 219 , 16.40 )
( 220 , 16.38 )
( 221 , 16.35 )
( 222 , 16.43 )
( 223 , 16.37 )
( 224 , 16.43 )
( 225 , 16.44 )
( 226 , 16.41 )
( 227 , 16.52 )
( 228 , 16.69 )
( 229 , 16.96 )
( 230 , 17.21 )
( 231 , 17.45 )
( 232 , 17.54 )
( 233 , 17.65 )
( 234 , 17.65 )
( 235 , 17.65 )
( 236 , 17.65 )
( 237 , 17.95 )
( 238 , 18.25 )
( 239 , 18.56 )
( 240 , 18.85 )
( 241 , 19.08 )
( 242 , 19.30 )
( 243 , 19.65 )
( 244 , 19.92 )
( 245 , 20.32 )
( 246 , 20.57 )
( 247 , 20.80 )
( 248 , 21.15 )
( 249 , 21.47 )
( 250 , 21.74 )
( 251 , 22.00 )
( 252 , 22.00 )
( 253 , 22.15 )
( 254 , 22.15 )
( 255 , 22.39 )
( 256 , 22.61 )
( 257 , 22.83 )
( 258 , 23.05 )
( 259 , 23.36 )
( 260 , 23.58 )
( 261 , 23.80 )
( 262 , 24.08 )
( 263 , 24.35 )
( 264 , 24.58 )
( 265 , 24.81 )
( 266 , 25.04 )
( 267 , 25.26 )
( 268 , 25.60 )
( 269 , 25.84 )
( 270 , 26.11 )
( 271 , 26.34 )
( 272 , 26.68 )
( 273 , 27.02 )
( 274 , 27.42 )
( 275 , 27.79 )
( 276 , 28.09 )
( 277 , 28.39 )
( 278 , 28.72 )
( 279 , 28.98 )
( 280 , 29.23 )
( 281 , 29.46 )
( 282 , 29.70 )
( 283 , 29.92 )
( 284 , 30.22 )
( 285 , 30.28 )
( 286 , 30.28 )
( 287 , 30.48 )
( 288 , 30.52 )
( 289 , 30.54 )
( 290 , 30.54 )
( 291 , 30.54 )
( 292 , 30.54 )
( 293 , 30.59 )
( 294 , 30.82 )
( 295 , 31.06 )
( 296 , 31.28 )
( 297 , 31.28 )
( 298 , 31.36 )
( 299 , 31.44 )
( 300 , 31.47 )
( 301 , 31.53 )
( 302 , 31.61 )
( 303 , 31.62 )
( 304 , 31.64 )
( 305 , 31.65 )
( 306 , 31.67 )
( 307 , 31.73 )
( 308 , 31.83 )
( 309 , 31.90 )
( 310 , 31.90 )
( 311 , 32.11 )
( 312 , 32.17 )
( 313 , 32.23 )
( 314 , 32.26 )
( 315 , 32.26 )
( 316 , 32.34 )
( 317 , 32.34 )
( 318 , 32.71 )
( 319 , 33.06 )
( 320 , 33.40 )
( 321 , 33.77 )
( 322 , 33.94 )
( 323 , 33.94 )
( 324 , 33.94 )
( 325 , 33.97 )
( 326 , 34.02 )
( 327 , 34.05 )
( 328 , 34.10 )
( 329 , 34.18 )
( 330 , 34.20 )
( 331 , 34.26 )
( 332 , 34.24 )
( 333 , 34.20 )
( 334 , 34.17 )
( 335 , 34.12 )
( 336 , 34.06 )
( 337 , 34.06 )
( 338 , 34.00 )
( 339 , 33.96 )
( 340 , 33.92 )
( 341 , 33.95 )
( 342 , 33.90 )
( 343 , 33.87 )
( 344 , 33.85 )
( 345 , 33.79 )
( 346 , 33.85 )
( 347 , 33.80 )
( 348 , 33.85 )
( 349 , 33.80 )
( 350 , 33.81 )
( 351 , 33.79 )
( 352 , 33.73 )
( 353 , 33.68 )
( 354 , 33.62 )
( 355 , 33.59 )
( 356 , 33.71 )
( 357 , 33.95 )
( 358 , 34.20 )
( 359 , 34.39 )
( 360 , 34.39 )
( 361 , 34.38 )
( 362 , 34.34 )
( 363 , 34.33 )
( 364 , 34.30 )
( 365 , 34.27 )
( 366 , 34.25 )
( 367 , 34.22 )
( 368 , 34.49 )
( 369 , 34.78 )
( 370 , 35.06 )
( 371 , 35.34 )
( 372 , 35.59 )
( 373 , 35.90 )
( 374 , 36.18 )
( 375 , 36.43 )
( 376 , 36.67 )
( 377 , 36.85 )
( 378 , 37.00 )
( 379 , 37.13 )
( 380 , 37.26 )
( 381 , 37.39 )
( 382 , 37.60 )
( 383 , 37.75 )
( 384 , 37.91 )
( 385 , 38.03 )
( 386 , 38.17 )
( 387 , 38.05 )
( 388 , 37.93 )
( 389 , 37.87 )
( 390 , 37.74 )
( 391 , 37.62 )
( 392 , 37.59 )
( 393 , 37.64 )
( 394 , 37.68 )
( 395 , 37.57 )
( 396 , 37.45 )
( 397 , 37.32 )
( 398 , 37.40 )
( 399 , 37.39 )
( 400 , 37.34 )
( 401 , 37.23 )
( 402 , 37.12 )
( 403 , 37.00 )
( 404 , 36.88 )
( 405 , 36.84 )
( 406 , 36.86 )
( 407 , 36.82 )
( 408 , 36.77 )
( 409 , 36.71 )
( 410 , 36.69 )
( 411 , 36.67 )
( 412 , 36.65 )
( 413 , 36.68 )
( 414 , 36.64 )
( 415 , 36.62 )
( 416 , 36.59 )
( 417 , 36.74 )
( 418 , 36.86 )
( 419 , 36.84 )
( 420 , 36.81 )
( 421 , 36.85 )
( 422 , 36.86 )
( 423 , 36.80 )
( 424 , 36.74 )
( 425 , 36.69 )
( 426 , 36.75 )
( 427 , 36.82 )
( 428 , 36.88 )
( 429 , 36.90 )
( 430 , 36.88 )
( 431 , 36.82 )
( 432 , 36.76 )
( 433 , 36.79 )
( 434 , 36.79 )
( 435 , 36.80 )
( 436 , 37.02 )
( 437 , 37.26 )
( 438 , 37.68 )
( 439 , 38.12 )
( 440 , 38.44 )
( 441 , 38.77 )
( 442 , 39.20 )
( 443 , 39.51 )
( 444 , 39.73 )
( 445 , 39.95 )
( 446 , 40.02 )
( 447 , 40.10 )
( 448 , 40.24 )
( 449 , 40.30 )
( 450 , 40.52 )
( 451 , 40.75 )
( 452 , 40.97 )
( 453 , 41.20 )
( 454 , 41.54 )
( 455 , 41.82 )
( 456 , 42.04 )
( 457 , 42.29 )
( 458 , 42.52 )
( 459 , 42.84 )
( 460 , 43.21 )
( 461 , 43.61 )
( 462 , 43.98 )
( 463 , 44.28 )
( 464 , 44.61 )
( 465 , 45.00 )
( 466 , 45.38 )
( 467 , 45.69 )
( 468 , 46.07 )
( 469 , 46.42 )
( 470 , 46.64 )
( 471 , 46.87 )
( 472 , 47.09 )
( 473 , 47.31 )
( 474 , 47.55 )
( 475 , 47.77 )
( 476 , 47.99 )
( 477 , 48.21 )
( 478 , 48.27 )
( 479 , 48.33 )
( 480 , 48.36 )
( 481 , 48.47 )
( 482 , 48.52 )
( 483 , 48.74 )
( 484 , 48.75 )
( 485 , 48.75 )
( 486 , 48.75 )
( 487 , 48.98 )
( 488 , 49.29 )
( 489 , 49.51 )
( 490 , 49.79 )
( 491 , 50.04 )
( 492 , 50.29 )
( 493 , 50.40 )
( 494 , 50.40 )
( 495 , 50.42 )
( 496 , 50.45 )
( 497 , 50.60 )
( 498 , 50.78 )
( 499 , 50.78 )
( 500 , 50.78 )
( 501 , 50.78 )
( 502 , 50.79 )
( 503 , 50.96 )
( 504 , 51.11 )
( 505 , 51.32 )
( 506 , 51.39 )
( 507 , 51.40 )
( 508 , 51.47 )
( 509 , 51.55 )
( 510 , 51.70 )
( 511 , 51.86 )
( 512 , 51.86 )
( 513 , 51.86 )
( 514 , 52.00 )
( 515 , 52.22 )
( 516 , 52.43 )
( 517 , 52.57 )
( 518 , 52.57 )
( 519 , 52.57 )
( 520 , 52.57 )
( 521 , 52.57 )
( 522 , 52.57 )
( 523 , 52.59 )
( 524 , 52.59 )
( 525 , 52.59 )
( 526 , 52.59 )
( 527 , 52.77 )
( 528 , 52.77 )
( 529 , 52.78 )
( 530 , 52.89 )
( 531 , 52.89 )
( 532 , 53.17 )
( 533 , 53.17 )
( 534 , 53.18 )
( 535 , 53.18 )
( 536 , 53.18 )
( 537 , 53.18 )
( 538 , 53.30 )
( 539 , 53.30 )
( 540 , 53.45 )
( 541 , 53.60 )
( 542 , 53.60 )
( 543 , 53.91 )
( 544 , 54.30 )
( 545 , 54.72 )
( 546 , 54.96 )
( 547 , 55.05 )
( 548 , 55.05 )
( 549 , 55.21 )
( 550 , 55.36 )
( 551 , 55.51 )
( 552 , 55.69 )
( 553 , 55.69 )
( 554 , 55.69 )
( 555 , 55.69 )
( 556 , 55.83 )
( 557 , 56.09 )
( 558 , 56.25 )
( 559 , 56.57 )
( 560 , 56.81 )
( 561 , 56.99 )
( 562 , 56.99 )
( 563 , 57.04 )
( 564 , 57.04 )
( 565 , 57.18 )
( 566 , 57.33 )
( 567 , 57.35 )
( 568 , 57.38 )
( 569 , 57.38 )
( 570 , 57.38 )
( 571 , 57.38 )
( 572 , 57.38 )
( 573 , 57.38 )
( 574 , 57.53 )
( 575 , 57.53 )
( 576 , 57.53 )
( 577 , 57.68 )
( 578 , 57.83 )
( 579 , 57.98 )
( 580 , 58.12 )
( 581 , 58.32 )
( 582 , 58.47 )
( 583 , 58.58 )
( 584 , 58.64 )
( 585 , 58.64 )
( 586 , 58.68 )
( 587 , 58.70 )
( 588 , 58.71 )
( 589 , 58.84 )
( 590 , 58.91 )
( 591 , 58.93 )
( 592 , 59.04 )
( 593 , 59.25 )
( 594 , 59.25 )
( 595 , 59.35 )
( 596 , 59.43 )
( 597 , 59.43 )
( 598 , 59.43 )
( 599 , 59.45 )
( 600 , 59.72 )
( 601 , 60.02 )
( 602 , 60.15 )
( 603 , 60.24 )
( 604 , 60.37 )
( 605 , 60.44 )
( 606 , 60.47 )
( 607 , 60.47 )
( 608 , 60.48 )
( 609 , 60.59 )
( 610 , 60.62 )
( 611 , 60.74 )
( 612 , 60.99 )
( 613 , 61.23 )
( 614 , 61.43 )
( 615 , 61.61 )
( 616 , 61.61 )
( 617 , 61.61 )
( 618 , 61.89 )
( 619 , 62.16 )
( 620 , 62.32 )
( 621 , 62.47 )
( 622 , 62.49 )
( 623 , 62.49 )
( 624 , 62.49 )
( 625 , 62.61 )
( 626 , 62.61 )
( 627 , 62.61 )
( 628 , 62.62 )
( 629 , 62.62 )
( 630 , 62.77 )
( 631 , 62.78 )
( 632 , 62.91 )
( 633 , 63.04 )
( 634 , 63.15 )
( 635 , 63.15 )
( 636 , 63.15 )
( 637 , 63.17 )
( 638 , 63.23 )
( 639 , 63.30 )
( 640 , 63.30 )
( 641 , 63.31 )
( 642 , 63.31 )
( 643 , 63.34 )
( 644 , 63.50 )
( 645 , 63.65 )
( 646 , 63.81 )
( 647 , 63.83 )
( 648 , 63.89 )
( 649 , 63.89 )
( 650 , 63.89 )
( 651 , 63.92 )
( 652 , 63.95 )
( 653 , 64.05 )
( 654 , 64.27 )
( 655 , 64.51 )
( 656 , 64.48 )
( 657 , 64.45 )
( 658 , 64.53 )
( 659 , 64.52 )
( 660 , 64.55 )
( 661 , 64.63 )
( 662 , 64.76 )
( 663 , 64.73 )
( 664 , 64.70 )
( 665 , 64.68 )
( 666 , 64.77 )
( 667 , 64.74 )
( 668 , 64.75 )
( 669 , 64.77 )
( 670 , 64.71 )
( 671 , 64.71 )
( 672 , 64.70 )
( 673 , 64.65 )
( 674 , 64.61 )
( 675 , 64.55 )
( 676 , 64.49 )
( 677 , 64.37 )
( 678 , 64.27 )
( 679 , 64.14 )
( 680 , 64.02 )
( 681 , 63.89 )
( 682 , 63.77 )
( 683 , 63.64 )
( 684 , 63.52 )
( 685 , 63.40 )
( 686 , 63.27 )
( 687 , 63.49 )
( 688 , 63.70 )
( 689 , 64.02 )
( 690 , 64.28 )
( 691 , 64.49 )
( 692 , 64.71 )
( 693 , 64.84 )
( 694 , 64.96 )
( 695 , 65.12 )
( 696 , 65.30 )
( 697 , 65.42 )
( 698 , 65.55 )
( 699 , 65.67 )
( 700 , 65.55 )
( 701 , 65.62 )
( 702 , 65.69 )
( 703 , 65.57 )
( 704 , 65.45 )
( 705 , 65.35 )
( 706 , 65.23 )
( 707 , 65.41 )
( 708 , 65.59 )
( 709 , 65.52 )
( 710 , 65.40 )
( 711 , 65.27 )
( 712 , 65.33 )
( 713 , 65.37 )
( 714 , 65.49 )
( 715 , 65.53 )
( 716 , 65.41 )
( 717 , 65.35 )
( 718 , 65.24 )
( 719 , 65.14 )
( 720 , 65.14 )
( 721 , 65.26 )
( 722 , 65.37 )
( 723 , 65.29 )
( 724 , 65.17 )
( 725 , 65.05 )
( 726 , 64.98 )
( 727 , 65.10 )
( 728 , 65.23 )
( 729 , 65.34 )
( 730 , 65.41 )
( 731 , 65.47 )
( 732 , 65.51 )
( 733 , 65.59 )
( 734 , 65.53 )
( 735 , 65.49 )
( 736 , 65.38 )
( 737 , 65.26 )
( 738 , 65.13 )
( 739 , 65.01 )
( 740 , 64.91 )
( 741 , 64.79 )
( 742 , 64.71 )
( 743 , 64.59 )
( 744 , 64.67 )
( 745 , 64.76 )
( 746 , 64.88 )
( 747 , 64.92 )
( 748 , 64.80 )
( 749 , 64.67 )
( 750 , 64.87 )
( 751 , 65.02 )
( 752 , 65.16 )
( 753 , 65.27 )
( 754 , 65.46 )
( 755 , 65.73 )
( 756 , 65.97 )
( 757 , 66.10 )
( 758 , 66.20 )
( 759 , 66.30 )
( 760 , 66.41 )
( 761 , 66.54 )
( 762 , 66.73 )
( 763 , 66.82 )
( 764 , 66.97 )
( 765 , 67.14 )
( 766 , 67.30 )
( 767 , 67.42 )
( 768 , 67.55 )
( 769 , 67.81 )
( 770 , 68.02 )
( 771 , 68.34 )
( 772 , 68.59 )
( 773 , 68.75 )
( 774 , 68.88 )
( 775 , 69.11 )
( 776 , 69.21 )
( 777 , 69.32 )
( 778 , 69.45 )
( 779 , 69.55 )
( 780 , 69.50 )
( 781 , 69.46 )
( 782 , 69.43 )
( 783 , 69.38 )
( 784 , 69.44 )
( 785 , 69.38 )
( 786 , 69.32 )
( 787 , 69.25 )
( 788 , 69.12 )
( 789 , 69.08 )
( 790 , 69.01 )
( 791 , 68.90 )
( 792 , 68.77 )
( 793 , 68.66 )
( 794 , 68.84 )
( 795 , 69.03 )
( 796 , 69.23 )
( 797 , 69.44 )
( 798 , 69.66 )
( 799 , 70.07 )
( 800 , 70.31 )
( 801 , 70.59 )
( 802 , 70.82 )
( 803 , 71.05 )
( 804 , 71.30 )
( 805 , 71.54 )
( 806 , 71.81 )
( 807 , 71.76 )
( 808 , 71.63 )
( 809 , 71.83 )
( 810 , 72.02 )
( 811 , 72.21 )
( 812 , 72.40 )
( 813 , 72.62 )
( 814 , 72.75 )
( 815 , 72.88 )
( 816 , 73.00 )
( 817 , 73.20 )
( 818 , 73.32 )
( 819 , 73.59 )
( 820 , 73.88 )
( 821 , 74.13 )
( 822 , 74.27 )
( 823 , 74.42 )
( 824 , 74.68 )
( 825 , 74.82 )
( 826 , 75.08 )
( 827 , 75.26 )
( 828 , 75.45 )
( 829 , 75.60 )
( 830 , 75.73 )
( 831 , 75.98 )
( 832 , 76.27 )
( 833 , 76.54 )
( 834 , 76.68 )
( 835 , 76.82 )
( 836 , 76.95 )
( 837 , 76.96 )
( 838 , 76.89 )
( 839 , 76.84 )
( 840 , 76.77 )
( 841 , 76.73 )
( 842 , 76.62 )
( 843 , 76.49 )
( 844 , 76.37 )
( 845 , 76.34 )
( 846 , 76.21 )
( 847 , 76.09 )
( 848 , 76.03 )
( 849 , 75.92 )
( 850 , 75.80 )
( 851 , 75.67 )
( 852 , 75.55 )
( 853 , 75.49 )
( 854 , 75.37 )
( 855 , 75.24 )
( 856 , 75.12 )
( 857 , 75.06 )
( 858 , 74.94 )
( 859 , 74.64 )
( 860 , 74.34 )
( 861 , 74.10 )
( 862 , 73.80 )
( 863 , 73.74 )
( 864 , 73.69 )
( 865 , 73.64 )
( 866 , 73.59 )
( 867 , 73.64 )
( 868 , 73.70 )
( 869 , 73.72 )
( 870 , 73.66 )
( 871 , 73.60 )
( 872 , 73.55 )
( 873 , 73.52 )
( 874 , 73.50 )
( 875 , 73.45 )
( 876 , 73.55 )
( 877 , 73.53 )
( 878 , 73.55 )
( 879 , 73.49 )
( 880 , 73.46 )
( 881 , 73.42 )
( 882 , 73.43 )
( 883 , 73.48 )
( 884 , 73.42 )
( 885 , 73.37 )
( 886 , 73.30 )
( 887 , 73.25 )
( 888 , 73.23 )
( 889 , 73.23 )
( 890 , 73.18 )
( 891 , 73.12 )
( 892 , 73.16 )
( 893 , 73.34 )
( 894 , 73.48 )
( 895 , 73.48 )
( 896 , 73.46 )
( 897 , 73.65 )
( 898 , 73.84 )
( 899 , 73.88 )
( 900 , 73.88 )
( 901 , 73.85 )
( 902 , 73.82 )
( 903 , 73.82 )
( 904 , 73.85 )
( 905 , 73.85 )
( 906 , 73.85 )
( 907 , 73.87 )
( 908 , 73.90 )
( 909 , 73.94 )
( 910 , 73.98 )
( 911 , 73.99 )
( 912 , 74.09 )
( 913 , 74.20 )
( 914 , 74.29 )
( 915 , 74.40 )
( 916 , 74.63 )
( 917 , 74.80 )
( 918 , 74.90 )
( 919 , 75.02 )
( 920 , 75.19 )
( 921 , 75.29 )
( 922 , 75.42 )
( 923 , 75.52 )
( 924 , 75.62 )
( 925 , 75.72 )
( 926 , 75.83 )
( 927 , 75.88 )
( 928 , 75.83 )
( 929 , 75.88 )
( 930 , 75.84 )
( 931 , 75.80 )
( 932 , 75.73 )
( 933 , 75.64 )
( 934 , 75.37 )
( 935 , 75.06 )
( 936 , 74.77 )
( 937 , 74.48 )
( 938 , 74.17 )
( 939 , 74.08 )
( 940 , 73.89 )
( 941 , 73.78 )
( 942 , 73.48 )
( 943 , 73.19 )
( 944 , 72.92 )
( 945 , 72.68 )
( 946 , 72.58 )
( 947 , 72.48 )
( 948 , 72.40 )
( 949 , 72.30 )
( 950 , 72.20 )
( 951 , 71.91 )
( 952 , 71.60 )
( 953 , 71.30 )
( 954 , 71.16 )
( 955 , 71.03 )
( 956 , 70.76 )
( 957 , 70.56 )
( 958 , 70.52 )
( 959 , 70.24 )
( 960 , 69.95 )
( 961 , 69.79 )
( 962 , 69.48 )
( 963 , 69.19 )
( 964 , 68.88 )
( 965 , 68.64 )
( 966 , 68.35 )
( 967 , 68.28 )
( 968 , 68.21 )
( 969 , 67.92 )
( 970 , 67.62 )
( 971 , 67.39 )
( 972 , 67.19 )
( 973 , 66.98 )
( 974 , 66.79 )
( 975 , 66.48 )
( 976 , 66.19 )
( 977 , 65.88 )
( 978 , 65.82 )
( 979 , 65.73 )
( 980 , 65.42 )
( 981 , 65.12 )
( 982 , 64.82 )
( 983 , 64.52 )
( 984 , 64.22 )
( 985 , 63.92 )
( 986 , 63.82 )
( 987 , 63.71 )
( 988 , 63.57 )
( 989 , 63.27 )
( 990 , 62.97 )
( 991 , 62.81 )
( 992 , 62.81 )
( 993 , 62.62 )
( 994 , 62.43 )
( 995 , 62.17 )
( 996 , 62.08 )
( 997 , 61.79 )
( 998 , 61.49 )
( 999 , 61.19 )
( 1000 , 61.00 )
( 1001 , 60.87 )
( 1002 , 60.68 )
( 1003 , 60.44 )
( 1004 , 60.14 )
( 1005 , 59.84 )
( 1006 , 59.62 )
( 1007 , 59.32 )
( 1008 , 59.02 )
( 1009 , 58.72 )
( 1010 , 58.47 )
( 1011 , 58.22 )
( 1012 , 58.03 )
( 1013 , 57.76 )
( 1014 , 57.47 )
( 1015 , 57.17 )
( 1016 , 56.88 )
( 1017 , 56.61 )
( 1018 , 56.33 )
( 1019 , 56.06 )
( 1020 , 55.77 )
( 1021 , 55.46 )
( 1022 , 55.23 )
( 1023 , 54.93 )
( 1024 , 54.64 )
( 1025 , 54.41 )
( 1026 , 54.21 )
( 1027 , 53.91 )
( 1028 , 53.86 )
( 1029 , 53.71 )
( 1030 , 53.41 )
( 1031 , 53.12 )
( 1032 , 52.83 )
( 1033 , 52.73 )
( 1034 , 52.59 )
( 1035 , 52.29 )
( 1036 , 52.19 )
( 1037 , 52.09 )
( 1038 , 52.21 )
( 1039 , 52.25 )
( 1040 , 52.12 )
( 1041 , 52.04 )
( 1042 , 51.90 )
( 1043 , 51.77 )
( 1044 , 51.56 )
( 1045 , 51.28 )
( 1046 , 51.00 )
( 1047 , 50.70 )
( 1048 , 50.42 )
( 1049 , 50.34 )
( 1050 , 50.25 )
( 1051 , 50.17 )
( 1052 , 49.87 )
( 1053 , 49.61 )
( 1054 , 49.35 )
( 1055 , 49.05 )
( 1056 , 48.90 )
( 1057 , 48.76 )
( 1058 , 48.46 )
( 1059 , 48.17 )
( 1060 , 47.87 )
( 1061 , 47.57 )
( 1062 , 47.28 )
( 1063 , 47.22 )
( 1064 , 46.97 )
( 1065 , 46.67 )
( 1066 , 46.46 )
( 1067 , 46.16 )
( 1068 , 45.86 )
( 1069 , 45.56 )
( 1070 , 45.32 )
( 1071 , 45.02 )
( 1072 , 44.79 )
( 1073 , 44.60 )
( 1074 , 44.30 )
( 1075 , 44.05 )
( 1076 , 43.82 )
( 1077 , 43.52 )
( 1078 , 43.23 )
( 1079 , 42.98 )
( 1080 , 42.73 )
( 1081 , 42.56 )
( 1082 , 42.29 )
( 1083 , 42.21 )
( 1084 , 42.00 )
( 1085 , 41.79 )
( 1086 , 41.49 )
( 1087 , 41.40 )
( 1088 , 41.27 )
( 1089 , 41.07 )
( 1090 , 40.90 )
( 1091 , 40.93 )
( 1092 , 40.62 )
( 1093 , 40.33 )
( 1094 , 40.16 )
( 1095 , 39.88 )
( 1096 , 39.59 )
( 1097 , 39.40 )
( 1098 , 39.21 )
( 1099 , 38.98 )
( 1100 , 38.68 )
( 1101 , 38.66 )
( 1102 , 38.38 )
( 1103 , 38.07 )
( 1104 , 37.90 )
( 1105 , 37.63 )
( 1106 , 37.43 )
( 1107 , 37.14 )
( 1108 , 37.00 )
( 1109 , 36.70 )
( 1110 , 36.46 )
( 1111 , 36.22 )
( 1112 , 35.92 )
( 1113 , 35.72 )
( 1114 , 35.42 )
( 1115 , 35.12 )
( 1116 , 34.88 )
( 1117 , 34.61 )
( 1118 , 34.38 )
( 1119 , 34.30 )
( 1120 , 34.20 )
( 1121 , 34.08 )
( 1122 , 34.13 )
( 1123 , 33.84 )
( 1124 , 33.57 )
( 1125 , 33.43 )
( 1126 , 33.33 )
( 1127 , 33.04 )
( 1128 , 32.73 )
( 1129 , 32.45 )
( 1130 , 32.14 )
( 1131 , 32.00 )
( 1132 , 31.70 )
( 1133 , 31.49 )
( 1134 , 31.34 )
( 1135 , 31.04 )
( 1136 , 31.04 )
( 1137 , 31.19 )
( 1138 , 31.25 )
( 1139 , 31.38 )
( 1140 , 31.50 )
( 1141 , 31.54 )
( 1142 , 31.75 )
( 1143 , 31.96 )
( 1144 , 32.16 )
( 1145 , 32.30 )
( 1146 , 32.42 )
( 1147 , 32.45 )
( 1148 , 32.39 )
( 1149 , 32.29 )
( 1150 , 32.16 )
( 1151 , 32.06 )
( 1152 , 32.20 )
( 1153 , 32.34 )
( 1154 , 32.47 )
( 1155 , 32.64 )
( 1156 , 32.77 )
( 1157 , 32.96 )
( 1158 , 33.20 )
( 1159 , 33.08 )
( 1160 , 32.96 )
( 1161 , 32.92 )
( 1162 , 32.81 )
( 1163 , 32.69 )
( 1164 , 32.67 )
( 1165 , 32.37 )
( 1166 , 32.27 )
( 1167 , 32.12 )
( 1168 , 31.85 )
( 1169 , 31.71 )
( 1170 , 31.41 )
( 1171 , 31.27 )
( 1172 , 31.12 )
( 1173 , 30.98 )
( 1174 , 30.68 )
( 1175 , 30.53 )
( 1176 , 30.32 )
( 1177 , 30.02 )
( 1178 , 29.83 )
( 1179 , 29.68 )
( 1180 , 29.43 )
( 1181 , 29.13 )
( 1182 , 29.24 )
( 1183 , 29.45 )
( 1184 , 29.53 )
( 1185 , 29.52 )
( 1186 , 29.59 )
( 1187 , 29.57 )
( 1188 , 29.73 )
( 1189 , 29.76 )
( 1190 , 29.74 )
( 1191 , 29.89 )
( 1192 , 30.04 )
( 1193 , 30.23 )
( 1194 , 30.21 )
( 1195 , 30.08 )
( 1196 , 30.01 )
( 1197 , 29.89 )
( 1198 , 29.77 )
( 1199 , 29.65 )
( 1200 , 29.56 )
( 1201 , 29.44 )
( 1202 , 29.51 )
( 1203 , 29.50 )
( 1204 , 29.44 )
( 1205 , 29.39 )
( 1206 , 29.54 )
( 1207 , 29.66 )
( 1208 , 29.63 )
( 1209 , 29.76 )
( 1210 , 29.88 )
( 1211 , 30.01 )
( 1212 , 30.17 )
( 1213 , 30.35 )
( 1214 , 30.50 )
( 1215 , 30.47 )
( 1216 , 30.45 )
( 1217 , 30.39 )
( 1218 , 30.33 )
( 1219 , 30.25 )
( 1220 , 30.21 )
( 1221 , 30.28 )
( 1222 , 30.21 )
( 1223 , 30.24 )
( 1224 , 29.96 )
( 1225 , 29.67 )
( 1226 , 29.38 )
( 1227 , 29.12 )
( 1228 , 28.86 )
( 1229 , 28.89 )
( 1230 , 28.82 )
( 1231 , 28.56 )
( 1232 , 28.26 )
( 1233 , 28.17 )
( 1234 , 28.07 )
( 1235 , 28.04 )
( 1236 , 28.11 )
( 1237 , 28.02 )
( 1238 , 27.79 )
( 1239 , 27.49 )
( 1240 , 27.43 )
( 1241 , 27.28 )
( 1242 , 27.10 )
( 1243 , 26.82 )
( 1244 , 26.67 )
( 1245 , 26.58 )
( 1246 , 26.44 )
( 1247 , 26.34 )
( 1248 , 26.04 )
( 1249 , 25.74 )
( 1250 , 25.44 )
( 1251 , 25.17 )
( 1252 , 24.87 )
( 1253 , 24.57 )
( 1254 , 24.44 )
( 1255 , 24.13 )
( 1256 , 23.83 )
( 1257 , 23.53 )
( 1258 , 23.23 )
( 1259 , 23.09 )
( 1260 , 22.99 )
( 1261 , 22.93 )
( 1262 , 22.96 )
( 1263 , 22.69 )
( 1264 , 22.72 )
( 1265 , 22.57 )
( 1266 , 22.51 )
( 1267 , 22.21 )
( 1268 , 21.91 )
( 1269 , 21.61 )
( 1270 , 21.46 )
( 1271 , 21.16 )
( 1272 , 20.89 )
( 1273 , 20.61 )
( 1274 , 20.32 )
( 1275 , 20.05 )
( 1276 , 19.75 )
( 1277 , 19.80 )
( 1278 , 19.65 )
( 1279 , 19.35 )
( 1280 , 19.05 )
( 1281 , 18.75 )
( 1282 , 18.80 )
( 1283 , 18.84 )
( 1284 , 18.84 )
( 1285 , 18.83 )
( 1286 , 18.80 )
( 1287 , 18.69 )
( 1288 , 18.56 )
( 1289 , 18.61 )
( 1290 , 18.72 )
( 1291 , 18.83 )
( 1292 , 18.70 )
( 1293 , 18.66 )
( 1294 , 18.62 )
( 1295 , 18.50 )
( 1296 , 18.73 )
( 1297 , 19.09 )
( 1298 , 19.44 )
( 1299 , 19.35 )
( 1300 , 19.22 )
( 1301 , 19.13 )
( 1302 , 19.04 )
( 1303 , 18.96 )
( 1304 , 18.87 )
( 1305 , 19.00 )
( 1306 , 19.25 )
( 1307 , 19.51 )
( 1308 , 19.77 )
( 1309 , 20.08 )
( 1310 , 20.38 )
( 1311 , 20.59 )
( 1312 , 20.81 )
( 1313 , 21.04 )
( 1314 , 21.31 )
( 1315 , 21.70 )
( 1316 , 22.09 )
( 1317 , 22.45 )
( 1318 , 22.72 )
( 1319 , 23.13 )
( 1320 , 23.49 )
( 1321 , 23.75 )
( 1322 , 23.93 )
( 1323 , 24.11 )
( 1324 , 24.29 )
( 1325 , 24.47 )
( 1326 , 24.70 )
( 1327 , 24.91 )
( 1328 , 25.15 )
( 1329 , 25.42 )
( 1330 , 25.74 )
( 1331 , 26.06 )
( 1332 , 26.31 )
( 1333 , 26.56 )
( 1334 , 26.84 )
( 1335 , 27.05 )
( 1336 , 27.26 )
( 1337 , 27.51 )
( 1338 , 27.75 )
( 1339 , 28.01 )
( 1340 , 28.27 )
( 1341 , 28.58 )
( 1342 , 28.83 )
( 1343 , 29.08 )
( 1344 , 29.35 )
( 1345 , 29.55 )
( 1346 , 29.55 )
( 1347 , 29.64 )
( 1348 , 29.78 )
( 1349 , 29.89 )
( 1350 , 30.09 )
( 1351 , 30.19 )
( 1352 , 30.31 )
( 1353 , 30.40 )
( 1354 , 30.50 )
( 1355 , 30.71 )
( 1356 , 30.81 )
( 1357 , 30.93 )
( 1358 , 31.07 )
( 1359 , 31.21 )
( 1360 , 31.22 )
( 1361 , 31.38 )
( 1362 , 31.38 )
( 1363 , 31.41 )
( 1364 , 31.40 )
( 1365 , 31.54 )
( 1366 , 31.51 )
( 1367 , 31.58 )
( 1368 , 31.57 )
( 1369 , 31.55 )
( 1370 , 31.50 )
( 1371 , 31.53 )
( 1372 , 31.47 )
( 1373 , 31.53 )
( 1374 , 31.47 )
( 1375 , 31.47 )
( 1376 , 31.42 )
( 1377 , 31.46 )
( 1378 , 31.44 )
( 1379 , 31.41 )
( 1380 , 31.35 )
( 1381 , 31.11 )
( 1382 , 30.80 )
( 1383 , 30.58 )
( 1384 , 30.28 )
( 1385 , 29.99 )
( 1386 , 29.71 )
( 1387 , 29.41 )
( 1388 , 29.42 )
( 1389 , 29.28 )
( 1390 , 29.18 )
( 1391 , 28.94 )
( 1392 , 28.63 )
( 1393 , 28.54 )
( 1394 , 28.24 )
( 1395 , 27.95 )
( 1396 , 27.75 )
( 1397 , 27.61 )
( 1398 , 27.30 )
( 1399 , 27.08 )
( 1400 , 26.78 )
( 1401 , 26.49 )
( 1402 , 26.19 )
( 1403 , 25.92 )
( 1404 , 25.66 )
( 1405 , 25.60 )
( 1406 , 25.67 )
( 1407 , 25.37 )
( 1408 , 25.36 )
( 1409 , 25.22 )
( 1410 , 25.07 )
( 1411 , 24.78 )
( 1412 , 24.48 )
( 1413 , 24.31 )
( 1414 , 24.11 )
( 1415 , 23.88 )
( 1416 , 23.65 )
( 1417 , 23.35 )
( 1418 , 23.38 )
( 1419 , 23.14 )
( 1420 , 22.84 )
( 1421 , 22.56 )
( 1422 , 22.26 )
( 1423 , 22.00 )
( 1424 , 21.74 )
( 1425 , 21.44 )
( 1426 , 21.34 )
( 1427 , 21.04 )
( 1428 , 20.74 )
( 1429 , 20.44 )
( 1430 , 20.31 )
( 1431 , 20.02 )
( 1432 , 19.77 )
( 1433 , 19.48 )
( 1434 , 19.19 )
( 1435 , 18.89 )
( 1436 , 18.63 )
( 1437 , 18.33 )
( 1438 , 18.34 )
( 1439 , 18.13 )
( 1440 , 17.93 )
( 1441 , 17.63 )
( 1442 , 17.34 )
( 1443 , 17.04 )
( 1444 , 16.74 )
( 1445 , 16.48 )
( 1446 , 16.19 )
( 1447 , 15.89 )
( 1448 , 15.59 )
( 1449 , 15.52 )
( 1450 , 15.54 )
( 1451 , 15.54 )
( 1452 , 15.54 )
( 1453 , 15.54 )
( 1454 , 15.55 )
( 1455 , 15.59 )
( 1456 , 15.65 )
( 1457 , 15.73 )
( 1458 , 15.73 )
( 1459 , 15.73 )
( 1460 , 16.03 )
( 1461 , 16.33 )
( 1462 , 16.55 )
( 1463 , 16.95 )
( 1464 , 17.17 )
( 1465 , 17.43 )
( 1466 , 17.66 )
( 1467 , 17.88 )
( 1468 , 18.16 )
( 1469 , 18.39 )
( 1470 , 18.67 )
( 1471 , 18.89 )
( 1472 , 18.89 )
( 1473 , 18.93 )
( 1474 , 18.97 )
( 1475 , 18.98 )
( 1476 , 19.20 )
( 1477 , 19.51 )
( 1478 , 19.75 )
( 1479 , 19.98 )
( 1480 , 20.26 )
( 1481 , 20.48 )
( 1482 , 20.72 )
( 1483 , 20.94 )
( 1484 , 21.17 )
( 1485 , 21.45 )
( 1486 , 21.74 )
( 1487 , 21.97 )
( 1488 , 22.34 )
( 1489 , 22.57 )
( 1490 , 22.88 )
( 1491 , 23.12 )
( 1492 , 23.41 )
( 1493 , 23.69 )
( 1494 , 23.98 )
( 1495 , 24.25 )
( 1496 , 24.47 )
( 1497 , 24.76 )
( 1498 , 25.13 )
( 1499 , 25.44 )
( 1500 , 25.74 )
( 1501 , 25.98 )
( 1502 , 26.21 )
( 1503 , 26.58 )
( 1504 , 26.82 )
( 1505 , 27.06 )
( 1506 , 27.40 )
( 1507 , 27.74 )
( 1508 , 28.02 )
( 1509 , 28.30 )
( 1510 , 28.59 )
( 1511 , 28.88 )
( 1512 , 29.11 )
( 1513 , 29.36 )
( 1514 , 29.66 )
( 1515 , 29.68 )
( 1516 , 29.96 )
( 1517 , 30.18 )
( 1518 , 30.27 )
( 1519 , 30.28 )
( 1520 , 30.43 )
( 1521 , 30.58 )
( 1522 , 30.75 )
( 1523 , 30.76 )
( 1524 , 30.81 )
( 1525 , 30.97 )
( 1526 , 31.16 )
( 1527 , 31.16 )
( 1528 , 31.49 )
( 1529 , 31.77 )
( 1530 , 32.07 )
( 1531 , 32.41 )
( 1532 , 32.66 )
( 1533 , 32.96 )
( 1534 , 32.96 )
( 1535 , 32.96 )
( 1536 , 32.99 )
( 1537 , 32.99 )
( 1538 , 33.00 )
( 1539 , 33.00 )
( 1540 , 33.07 )
( 1541 , 33.09 )
( 1542 , 33.09 )
( 1543 , 33.16 )
( 1544 , 33.20 )
( 1545 , 33.20 )
( 1546 , 33.21 )
( 1547 , 33.27 )
( 1548 , 33.31 )
( 1549 , 33.31 )
( 1550 , 33.32 )
( 1551 , 33.19 )
( 1552 , 33.09 )
( 1553 , 32.79 )
( 1554 , 32.49 )
( 1555 , 32.19 )
( 1556 , 31.90 )
( 1557 , 31.65 )
( 1558 , 31.36 )
( 1559 , 31.17 )
( 1560 , 30.90 )
( 1561 , 30.60 )
( 1562 , 30.36 )
( 1563 , 30.09 )
( 1564 , 29.79 )
( 1565 , 29.66 )
( 1566 , 29.54 )
( 1567 , 29.28 )
( 1568 , 28.98 )
( 1569 , 28.68 )
( 1570 , 28.79 )
( 1571 , 28.71 )
( 1572 , 28.67 )
( 1573 , 28.58 )
( 1574 , 28.46 )
( 1575 , 28.42 )
( 1576 , 28.30 )
( 1577 , 28.57 )
( 1578 , 28.55 )
( 1579 , 28.82 )
( 1580 , 29.13 )
( 1581 , 29.37 )
( 1582 , 29.61 )
( 1583 , 29.84 )
( 1584 , 30.02 )
( 1585 , 30.25 )
( 1586 , 30.46 )
( 1587 , 30.69 )
( 1588 , 30.92 )
( 1589 , 31.10 )
( 1590 , 31.32 )
( 1591 , 31.60 )
( 1592 , 31.88 )
( 1593 , 32.29 )
( 1594 , 32.57 )
( 1595 , 32.77 )
( 1596 , 32.97 )
( 1597 , 32.97 )
( 1598 , 33.10 )
( 1599 , 33.10 )
( 1600 , 33.09 )
( 1601 , 33.11 )
( 1602 , 33.21 )
( 1603 , 33.33 )
( 1604 , 33.43 )
( 1605 , 33.52 )
( 1606 , 33.49 )
( 1607 , 33.37 )
( 1608 , 33.24 )
( 1609 , 33.14 )
( 1610 , 33.01 )
( 1611 , 33.02 )
( 1612 , 33.02 )
( 1613 , 33.02 )
( 1614 , 33.00 )
( 1615 , 32.97 )
( 1616 , 33.09 )
( 1617 , 33.07 )
( 1618 , 33.05 )
( 1619 , 32.96 )
( 1620 , 32.86 )
( 1621 , 32.82 )
( 1622 , 32.70 )
( 1623 , 32.57 )
( 1624 , 32.45 )
( 1625 , 32.32 )
( 1626 , 32.20 )
( 1627 , 32.15 )
( 1628 , 32.14 )
( 1629 , 32.09 )
( 1630 , 32.09 )
( 1631 , 31.98 )
( 1632 , 31.85 )
( 1633 , 31.73 )
( 1634 , 31.68 )
( 1635 , 31.62 )
( 1636 , 31.59 )
( 1637 , 31.66 )
( 1638 , 31.61 )
( 1639 , 31.55 )
( 1640 , 31.49 )
( 1641 , 31.48 )
( 1642 , 31.43 )
( 1643 , 31.42 )
( 1644 , 31.36 )
( 1645 , 31.30 )
( 1646 , 31.24 )
( 1647 , 31.13 )
( 1648 , 31.05 )
( 1649 , 30.98 )
( 1650 , 30.87 )
( 1651 , 30.98 )
( 1652 , 30.86 )
( 1653 , 30.80 )
( 1654 , 30.68 )
( 1655 , 30.70 )
( 1656 , 30.64 )
( 1657 , 30.70 )
( 1658 , 30.81 )
( 1659 , 30.83 )
( 1660 , 30.88 )
( 1661 , 30.88 )
( 1662 , 30.91 )
( 1663 , 30.90 )
( 1664 , 31.08 )
( 1665 , 31.25 )
( 1666 , 31.43 )
( 1667 , 31.62 )
( 1668 , 31.80 )
( 1669 , 31.98 )
( 1670 , 32.15 )
( 1671 , 32.42 )
( 1672 , 32.62 )
( 1673 , 32.86 )
( 1674 , 33.07 )
( 1675 , 33.25 )
( 1676 , 33.52 )
( 1677 , 33.70 )
( 1678 , 33.91 )
( 1679 , 34.08 )
( 1680 , 34.31 )
( 1681 , 34.49 )
( 1682 , 34.68 )
( 1683 , 34.85 )
( 1684 , 35.03 )
( 1685 , 35.33 )
( 1686 , 35.61 )
( 1687 , 35.91 )
( 1688 , 36.18 )
( 1689 , 36.38 )
( 1690 , 36.28 )
( 1691 , 36.21 )
( 1692 , 36.15 )
( 1693 , 36.08 )
( 1694 , 35.97 )
( 1695 , 35.87 )
( 1696 , 35.74 )
( 1697 , 35.74 )
( 1698 , 35.61 )
( 1699 , 35.49 )
( 1700 , 35.37 )
( 1701 , 35.26 )
( 1702 , 35.14 )
( 1703 , 35.04 )
( 1704 , 34.95 )
( 1705 , 34.82 )
( 1706 , 34.75 )
( 1707 , 34.68 )
( 1708 , 34.65 )
( 1709 , 34.52 )
( 1710 , 34.57 )
( 1711 , 34.62 )
( 1712 , 34.60 )
( 1713 , 34.75 )
( 1714 , 34.73 )
( 1715 , 35.01 )
( 1716 , 35.30 )
( 1717 , 35.55 )
( 1718 , 35.81 )
( 1719 , 36.07 )
( 1720 , 36.34 )
( 1721 , 36.59 )
( 1722 , 36.88 )
( 1723 , 37.15 )
( 1724 , 37.43 )
( 1725 , 37.41 )
( 1726 , 37.11 )
( 1727 , 36.83 )
( 1728 , 36.53 )
( 1729 , 36.23 )
( 1730 , 35.93 )
( 1731 , 35.74 )
( 1732 , 35.43 )
( 1733 , 35.13 )
( 1734 , 35.04 )
( 1735 , 35.06 )
( 1736 , 34.80 )
( 1737 , 34.50 )
( 1738 , 34.20 )
( 1739 , 33.89 )
( 1740 , 33.98 )
( 1741 , 34.00 )
( 1742 , 33.70 )
( 1743 , 33.40 )
( 1744 , 33.10 )
( 1745 , 32.80 )
( 1746 , 32.50 )
( 1747 , 32.20 )
( 1748 , 31.90 )
( 1749 , 31.69 )
( 1750 , 31.40 )
( 1751 , 31.10 )
( 1752 , 30.86 )
( 1753 , 30.56 )
( 1754 , 30.26 )
( 1755 , 30.38 )
( 1756 , 30.49 )
( 1757 , 30.75 )
( 1758 , 30.88 )
( 1759 , 30.97 )
( 1760 , 31.16 )
( 1761 , 31.25 )
( 1762 , 31.38 )
( 1763 , 31.49 )
( 1764 , 31.60 )
( 1765 , 31.69 )
( 1766 , 31.75 )
( 1767 , 31.86 )
( 1768 , 32.01 )
( 1769 , 32.03 )
( 1770 , 32.14 )
( 1771 , 32.15 )
( 1772 , 32.42 )
( 1773 , 32.57 )
( 1774 , 32.61 )
( 1775 , 32.68 )
( 1776 , 32.70 )
( 1777 , 32.77 )
( 1778 , 32.86 )
( 1779 , 33.00 )
( 1780 , 33.00 )
( 1781 , 33.02 )
( 1782 , 33.15 )
( 1783 , 33.34 )
( 1784 , 33.47 )
( 1785 , 33.60 )
( 1786 , 33.67 )
( 1787 , 33.82 )
( 1788 , 33.98 )
( 1789 , 33.98 )
( 1790 , 33.98 )
( 1791 , 34.00 )
( 1792 , 34.05 )
( 1793 , 34.20 )
( 1794 , 34.38 )
( 1795 , 34.53 )
( 1796 , 34.77 )
( 1797 , 34.77 )
( 1798 , 34.80 )
( 1799 , 34.91 )
( 1800 , 34.98 )
( 1801 , 35.05 )
( 1802 , 35.13 )
( 1803 , 35.20 )
( 1804 , 35.21 )
( 1805 , 35.21 )
( 1806 , 35.22 )
( 1807 , 35.35 )
( 1808 , 35.35 )
( 1809 , 35.36 )
( 1810 , 35.36 )
( 1811 , 35.39 )
( 1812 , 35.40 )
( 1813 , 35.48 )
( 1814 , 35.62 )
( 1815 , 35.79 )
( 1816 , 35.98 )
( 1817 , 36.15 )
( 1818 , 36.32 )
( 1819 , 36.53 )
( 1820 , 36.62 )
( 1821 , 36.74 )
( 1822 , 36.75 )
( 1823 , 36.75 )
( 1824 , 36.90 )
( 1825 , 36.90 )
( 1826 , 36.90 )
( 1827 , 36.96 )
( 1828 , 36.96 )
( 1829 , 37.18 )
( 1830 , 37.34 )
( 1831 , 37.35 )
( 1832 , 37.50 )
( 1833 , 37.66 )
( 1834 , 37.79 )
( 1835 , 37.88 )
( 1836 , 37.97 )
( 1837 , 38.05 )
( 1838 , 38.14 )
( 1839 , 38.23 )
( 1840 , 38.35 )
( 1841 , 38.55 )
( 1842 , 38.76 )
( 1843 , 38.96 )
( 1844 , 39.15 )
( 1845 , 39.30 )
( 1846 , 39.30 )
( 1847 , 39.35 )
( 1848 , 39.35 )
( 1849 , 39.35 )
( 1850 , 39.35 )
( 1851 , 39.36 )
( 1852 , 39.41 )
( 1853 , 39.53 )
( 1854 , 39.64 )
( 1855 , 39.68 )
( 1856 , 39.68 )
( 1857 , 39.90 )
( 1858 , 39.96 )
( 1859 , 40.03 )
( 1860 , 40.10 )
( 1861 , 40.23 )
( 1862 , 40.40 )
( 1863 , 40.61 )
( 1864 , 40.81 )
( 1865 , 40.88 )
( 1866 , 41.14 )
( 1867 , 41.41 )
( 1868 , 41.71 )
( 1869 , 41.84 )
( 1870 , 41.99 )
( 1871 , 42.24 )
( 1872 , 42.50 )
( 1873 , 42.75 )
( 1874 , 43.01 )
( 1875 , 43.14 )
( 1876 , 43.26 )
( 1877 , 43.39 )
( 1878 , 43.64 )
( 1879 , 43.96 )
( 1880 , 44.22 )
( 1881 , 44.48 )
( 1882 , 44.74 )
( 1883 , 44.88 )
( 1884 , 45.06 )
( 1885 , 45.19 )
( 1886 , 45.35 )
( 1887 , 45.54 )
( 1888 , 45.71 )
( 1889 , 45.93 )
( 1890 , 46.17 )
( 1891 , 46.33 )
( 1892 , 46.46 )
( 1893 , 46.63 )
( 1894 , 46.77 )
( 1895 , 47.03 )
( 1896 , 47.27 )
( 1897 , 47.46 )
( 1898 , 47.59 )
( 1899 , 47.72 )
( 1900 , 47.85 )
( 1901 , 47.97 )
( 1902 , 47.88 )
( 1903 , 47.88 )
( 1904 , 47.99 )
( 1905 , 48.18 )
( 1906 , 48.17 )
( 1907 , 48.13 )
( 1908 , 48.02 )
( 1909 , 47.89 )
( 1910 , 47.86 )
( 1911 , 47.82 )
( 1912 , 47.71 )
( 1913 , 47.59 )
( 1914 , 47.66 )
( 1915 , 47.70 )
( 1916 , 47.63 )
( 1917 , 47.55 )
( 1918 , 47.43 )
( 1919 , 47.37 )
( 1920 , 47.25 )
( 1921 , 47.18 )
( 1922 , 47.05 )
( 1923 , 46.96 )
( 1924 , 47.02 )
( 1925 , 47.06 )
( 1926 , 47.02 )
( 1927 , 46.92 )
( 1928 , 46.88 )
( 1929 , 46.84 )
( 1930 , 46.79 )
( 1931 , 46.71 )
( 1932 , 46.79 )
( 1933 , 46.73 )
( 1934 , 46.61 )
( 1935 , 46.48 )
( 1936 , 46.61 )
( 1937 , 46.80 )
( 1938 , 46.93 )
( 1939 , 47.11 )
( 1940 , 47.30 )
( 1941 , 47.17 )
( 1942 , 47.15 )
( 1943 , 47.12 )
( 1944 , 47.09 )
( 1945 , 47.08 )
( 1946 , 47.09 )
( 1947 , 47.06 )
( 1948 , 47.10 )
( 1949 , 47.16 )
( 1950 , 47.34 )
( 1951 , 47.32 )
( 1952 , 47.19 )
( 1953 , 47.32 )
( 1954 , 47.26 )
( 1955 , 47.25 )
( 1956 , 47.39 )
( 1957 , 47.45 )
( 1958 , 47.51 )
( 1959 , 47.39 )
( 1960 , 47.61 )
( 1961 , 47.79 )
( 1962 , 47.98 )
( 1963 , 48.18 )
( 1964 , 48.37 )
( 1965 , 48.50 )
( 1966 , 48.76 )
( 1967 , 48.90 )
( 1968 , 49.03 )
( 1969 , 49.15 )
( 1970 , 49.41 )
( 1971 , 49.60 )
( 1972 , 49.73 )
( 1973 , 49.86 )
( 1974 , 49.98 )
( 1975 , 50.15 )
( 1976 , 50.30 )
( 1977 , 50.43 )
( 1978 , 50.57 )
( 1979 , 50.45 )
( 1980 , 50.35 )
( 1981 , 50.24 )
( 1982 , 50.12 )
( 1983 , 50.00 )
( 1984 , 50.12 )
( 1985 , 50.12 )
( 1986 , 50.14 )
( 1987 , 50.17 )
( 1988 , 50.16 )
( 1989 , 50.16 )
( 1990 , 50.27 )
( 1991 , 50.45 )
( 1992 , 50.57 )
( 1993 , 50.66 )
( 1994 , 50.77 )
( 1995 , 50.92 )
( 1996 , 51.05 )
( 1997 , 51.14 )
( 1998 , 51.29 )
( 1999 , 51.45 )
( 2000 , 51.73 )
( 2001 , 52.01 )
( 2002 , 52.27 )
( 2003 , 52.50 )
( 2004 , 52.76 )
( 2005 , 53.01 )
( 2006 , 53.27 )
( 2007 , 53.41 )
( 2008 , 53.52 )
( 2009 , 53.62 )
( 2010 , 53.76 )
( 2011 , 53.96 )
( 2012 , 54.07 )
( 2013 , 54.17 )
( 2014 , 54.29 )
( 2015 , 54.40 )
( 2016 , 54.50 )
( 2017 , 54.60 )
( 2018 , 54.77 )
( 2019 , 54.86 )
( 2020 , 55.02 )
( 2021 , 55.25 )
( 2022 , 55.40 )
( 2023 , 55.50 )
( 2024 , 55.62 )
( 2025 , 55.66 )
( 2026 , 55.75 )
( 2027 , 55.80 )
( 2028 , 55.87 )
( 2029 , 55.90 )
( 2030 , 55.88 )
( 2031 , 55.84 )
( 2032 , 55.89 )
( 2033 , 55.88 )
( 2034 , 55.93 )
( 2035 , 55.91 )
( 2036 , 55.93 )
( 2037 , 55.93 )
( 2038 , 55.91 )
( 2039 , 55.90 )
( 2040 , 55.84 )
( 2041 , 55.84 )
( 2042 , 55.78 )
( 2043 , 55.72 )
( 2044 , 55.67 )
( 2045 , 55.64 )
( 2046 , 55.62 )
( 2047 , 55.62 )
( 2048 , 55.56 )
( 2049 , 55.51 )
( 2050 , 55.46 )
( 2051 , 55.41 )
( 2052 , 55.40 )
( 2053 , 55.34 )
( 2054 , 55.32 )
( 2055 , 55.28 )
( 2056 , 55.22 )
( 2057 , 55.16 )
( 2058 , 55.11 )
( 2059 , 55.09 )
( 2060 , 55.12 )
( 2061 , 55.16 )
( 2062 , 55.12 )
( 2063 , 55.07 )
( 2064 , 55.02 )
( 2065 , 55.01 )
( 2066 , 55.04 )
( 2067 , 55.01 )
( 2068 , 54.96 )
( 2069 , 55.04 )
( 2070 , 55.12 )
( 2071 , 55.07 )
( 2072 , 55.04 )
( 2073 , 55.02 )
( 2074 , 54.96 )
( 2075 , 55.09 )
( 2076 , 55.09 )
( 2077 , 55.09 )
( 2078 , 55.03 )
( 2079 , 54.99 )
( 2080 , 54.93 )
( 2081 , 54.94 )
( 2082 , 54.88 )
( 2083 , 54.86 )
( 2084 , 54.89 )
( 2085 , 54.86 )
( 2086 , 54.85 )
( 2087 , 54.85 )
( 2088 , 54.85 )
( 2089 , 54.84 )
( 2090 , 54.85 )
( 2091 , 54.86 )
( 2092 , 54.97 )
( 2093 , 55.09 )
( 2094 , 55.17 )
( 2095 , 55.27 )
( 2096 , 55.27 )
( 2097 , 55.49 )
( 2098 , 55.71 )
( 2099 , 55.72 )
( 2100 , 55.73 )
( 2101 , 55.77 )
( 2102 , 55.88 )
( 2103 , 55.95 )
( 2104 , 55.95 )
( 2105 , 55.98 )
( 2106 , 56.00 )
( 2107 , 56.00 )
( 2108 , 56.07 )
( 2109 , 56.11 )
( 2110 , 56.14 )
( 2111 , 56.24 )
( 2112 , 56.31 )
( 2113 , 56.33 )
( 2114 , 56.48 )
( 2115 , 56.62 )
( 2116 , 56.77 )
( 2117 , 56.92 )
( 2118 , 57.07 )
( 2119 , 57.07 )
( 2120 , 57.11 )
( 2121 , 57.12 )
( 2122 , 57.18 )
( 2123 , 57.18 )
( 2124 , 57.19 )
( 2125 , 57.25 )
( 2126 , 57.32 )
( 2127 , 57.38 )
( 2128 , 57.45 )
( 2129 , 57.39 )
( 2130 , 57.37 )
( 2131 , 57.32 )
( 2132 , 57.26 )
( 2133 , 57.24 )
( 2134 , 57.18 )
( 2135 , 57.06 )
( 2136 , 56.94 )
( 2137 , 56.82 )
( 2138 , 56.76 )
( 2139 , 56.64 )
( 2140 , 56.55 )
( 2141 , 56.48 )
( 2142 , 56.37 )
( 2143 , 56.25 )
( 2144 , 56.12 )
( 2145 , 56.00 )
( 2146 , 55.92 )
( 2147 , 55.83 )
( 2148 , 55.71 )
( 2149 , 55.62 )
( 2150 , 55.50 )
( 2151 , 55.38 )
( 2152 , 55.30 )
( 2153 , 55.18 )
( 2154 , 55.05 )
( 2155 , 54.93 )
( 2156 , 54.80 )
( 2157 , 54.68 )
( 2158 , 54.61 )
( 2159 , 54.50 )
( 2160 , 54.40 )
( 2161 , 54.32 )
( 2162 , 54.20 )
( 2163 , 54.13 )
( 2164 , 54.02 )
( 2165 , 53.90 )
( 2166 , 54.13 )
( 2167 , 54.48 )
( 2168 , 54.78 )
( 2169 , 55.03 )
( 2170 , 55.26 )
( 2171 , 55.45 )
( 2172 , 55.67 )
( 2173 , 55.86 )
( 2174 , 56.02 )
( 2175 , 56.14 )
( 2176 , 56.31 )
( 2177 , 56.44 )
( 2178 , 56.58 )
( 2179 , 56.80 )
( 2180 , 57.03 )
( 2181 , 57.40 )
( 2182 , 57.71 )
( 2183 , 58.07 )
( 2184 , 58.29 )
( 2185 , 58.44 )
( 2186 , 58.57 )
( 2187 , 58.70 )
( 2188 , 58.82 )
( 2189 , 59.07 )
( 2190 , 59.33 )
( 2191 , 59.59 )
( 2192 , 59.88 )
( 2193 , 60.18 )
( 2194 , 60.30 )
( 2195 , 60.45 )
( 2196 , 60.72 )
( 2197 , 60.96 )
( 2198 , 61.22 )
( 2199 , 61.48 )
( 2200 , 61.76 )
( 2201 , 61.99 )
( 2202 , 62.23 )
( 2203 , 62.41 )
( 2204 , 62.59 )
( 2205 , 62.47 )
( 2206 , 62.34 )
( 2207 , 62.22 )
( 2208 , 62.16 )
( 2209 , 61.86 )
( 2210 , 61.56 )
( 2211 , 61.26 )
( 2212 , 61.15 )
( 2213 , 61.02 )
( 2214 , 60.90 )
( 2215 , 60.77 )
( 2216 , 60.65 )
( 2217 , 60.52 )
( 2218 , 60.48 )
( 2219 , 60.61 )
( 2220 , 60.53 )
( 2221 , 60.45 )
( 2222 , 60.32 )
( 2223 , 60.31 )
( 2224 , 60.31 )
( 2225 , 60.30 )
( 2226 , 60.49 )
( 2227 , 60.62 )
( 2228 , 60.78 )
( 2229 , 60.90 )
( 2230 , 60.86 )
( 2231 , 60.80 )
( 2232 , 60.80 )
( 2233 , 60.79 )
( 2234 , 60.73 )
( 2235 , 60.84 )
( 2236 , 60.89 )
( 2237 , 61.00 )
( 2238 , 61.09 )
( 2239 , 61.20 )
( 2240 , 61.14 )
( 2241 , 61.09 )
( 2242 , 61.21 )
( 2243 , 61.19 )
( 2244 , 61.27 )
( 2245 , 61.24 )
( 2246 , 61.37 )
( 2247 , 61.38 )
( 2248 , 61.35 )
( 2249 , 61.41 )
( 2250 , 61.39 )
( 2251 , 61.26 )
( 2252 , 61.17 )
( 2253 , 61.04 )
( 2254 , 60.92 )
( 2255 , 60.96 )
( 2256 , 61.02 )
( 2257 , 60.92 )
( 2258 , 60.79 )
( 2259 , 60.67 )
( 2260 , 60.70 )
( 2261 , 60.70 )
( 2262 , 60.71 )
( 2263 , 60.67 )
( 2264 , 60.68 )
( 2265 , 60.64 )
( 2266 , 60.52 )
( 2267 , 60.41 )
( 2268 , 60.31 )
( 2269 , 60.19 )
( 2270 , 60.15 )
( 2271 , 60.03 )
( 2272 , 60.00 )
( 2273 , 59.97 )
( 2274 , 59.95 )
( 2275 , 59.95 )
( 2276 , 59.89 )
( 2277 , 59.91 )
( 2278 , 60.07 )
( 2279 , 60.02 )
( 2280 , 60.01 )
( 2281 , 60.05 )
( 2282 , 60.02 )
( 2283 , 60.00 )
( 2284 , 60.02 )
( 2285 , 60.04 )
( 2286 , 60.01 )
( 2287 , 59.95 )
( 2288 , 59.89 )
( 2289 , 59.84 )
( 2290 , 59.84 )
( 2291 , 59.83 )
( 2292 , 59.93 )
( 2293 , 59.88 )
( 2294 , 59.82 )
( 2295 , 59.77 )
( 2296 , 59.74 )
( 2297 , 59.79 )
( 2298 , 59.73 )
( 2299 , 59.67 )
( 2300 , 59.61 )
( 2301 , 59.58 )
( 2302 , 59.73 )
( 2303 , 59.86 )
( 2304 , 59.98 )
( 2305 , 60.15 )
( 2306 , 60.28 )
( 2307 , 60.48 )
( 2308 , 60.61 )
( 2309 , 60.73 )
( 2310 , 60.70 )
( 2311 , 60.92 )
( 2312 , 61.08 )
( 2313 , 61.09 )
( 2314 , 61.09 )
( 2315 , 61.15 )
( 2316 , 61.23 )
( 2317 , 61.41 )
( 2318 , 61.49 )
( 2319 , 61.57 )
( 2320 , 61.58 )
( 2321 , 61.57 )
( 2322 , 61.52 )
( 2323 , 61.49 )
( 2324 , 61.46 )
( 2325 , 61.34 )
( 2326 , 61.21 )
( 2327 , 61.47 )
( 2328 , 61.76 )
( 2329 , 62.07 )
( 2330 , 62.38 )
( 2331 , 62.66 )
( 2332 , 62.96 )
( 2333 , 63.26 )
( 2334 , 63.26 )
( 2335 , 63.43 )
( 2336 , 63.54 )
( 2337 , 63.54 )
( 2338 , 63.65 )
( 2339 , 63.72 )
( 2340 , 63.83 )
( 2341 , 63.88 )
( 2342 , 63.88 )
( 2343 , 63.97 )
( 2344 , 64.06 )
( 2345 , 64.20 )
( 2346 , 64.34 )
( 2347 , 64.38 )
( 2348 , 64.38 )
( 2349 , 64.49 )
( 2350 , 64.55 )
( 2351 , 64.57 )
( 2352 , 64.57 )
( 2353 , 64.57 )
( 2354 , 64.57 )
( 2355 , 64.57 )
( 2356 , 64.58 )
( 2357 , 64.58 )
( 2358 , 64.65 )
( 2359 , 64.71 )
( 2360 , 64.80 )
( 2361 , 64.98 )
( 2362 , 65.05 )
( 2363 , 65.13 )
( 2364 , 65.39 )
( 2365 , 65.40 )
( 2366 , 65.40 )
( 2367 , 65.60 )
( 2368 , 65.60 )
( 2369 , 65.68 )
( 2370 , 65.80 )
( 2371 , 65.85 )
( 2372 , 65.88 )
( 2373 , 65.91 )
( 2374 , 65.91 )
( 2375 , 65.91 )
( 2376 , 65.95 )
( 2377 , 65.97 )
( 2378 , 65.98 )
( 2379 , 65.98 )
( 2380 , 65.98 )
( 2381 , 65.98 )
( 2382 , 66.16 )
( 2383 , 66.27 )
( 2384 , 66.38 )
( 2385 , 66.54 )
( 2386 , 66.73 )
( 2387 , 66.83 )
( 2388 , 66.91 )
( 2389 , 67.02 )
( 2390 , 67.11 )
( 2391 , 67.20 )
( 2392 , 67.24 )
( 2393 , 67.30 )
( 2394 , 67.31 )
( 2395 , 67.44 )
( 2396 , 67.61 )
( 2397 , 67.84 )
( 2398 , 68.00 )
( 2399 , 68.12 )
( 2400 , 68.23 )
( 2401 , 68.34 )
( 2402 , 68.34 )
( 2403 , 68.34 )
( 2404 , 68.34 )
( 2405 , 68.34 )
( 2406 , 68.44 )
( 2407 , 68.54 )
( 2408 , 68.81 )
( 2409 , 69.03 )
( 2410 , 69.26 )
( 2411 , 69.50 )
( 2412 , 69.79 )
( 2413 , 69.99 )
( 2414 , 70.20 )
( 2415 , 70.50 )
( 2416 , 70.67 )
( 2417 , 70.84 )
( 2418 , 70.84 )
( 2419 , 70.94 )
( 2420 , 71.20 )
( 2421 , 71.38 )
( 2422 , 71.64 )
( 2423 , 71.79 )
( 2424 , 71.79 )
( 2425 , 71.79 )
( 2426 , 71.90 )
( 2427 , 71.90 )
( 2428 , 71.90 )
( 2429 , 71.91 )
( 2430 , 71.95 )
( 2431 , 71.95 )
( 2432 , 72.02 )
( 2433 , 72.09 )
( 2434 , 72.11 )
( 2435 , 72.11 )
( 2436 , 72.38 )
( 2437 , 72.38 )
( 2438 , 72.41 )
( 2439 , 72.41 )
( 2440 , 72.48 )
( 2441 , 72.48 )
( 2442 , 72.48 )
( 2443 , 72.49 )
( 2444 , 72.50 )
( 2445 , 72.50 )
( 2446 , 72.58 )
( 2447 , 72.66 )
( 2448 , 72.66 )
( 2449 , 72.66 )
( 2450 , 72.66 )
( 2451 , 72.66 )
( 2452 , 72.66 )
( 2453 , 72.80 )
( 2454 , 72.94 )
( 2455 , 72.95 )
( 2456 , 73.08 )
( 2457 , 73.08 )
( 2458 , 73.08 )
( 2459 , 73.08 )
( 2460 , 73.08 )
( 2461 , 73.08 )
( 2462 , 73.08 )
( 2463 , 73.29 )
( 2464 , 73.35 )
( 2465 , 73.42 )
( 2466 , 73.62 )
( 2467 , 73.68 )
( 2468 , 73.75 )
( 2469 , 74.05 )
( 2470 , 74.18 )
( 2471 , 74.30 )
( 2472 , 74.58 )
( 2473 , 74.74 )
( 2474 , 74.92 )
( 2475 , 75.05 )
( 2476 , 75.21 )
( 2477 , 75.34 )
( 2478 , 75.53 )
( 2479 , 75.71 )
( 2480 , 75.89 )
( 2481 , 76.10 )
( 2482 , 76.23 )
( 2483 , 76.39 )
( 2484 , 76.55 )
( 2485 , 76.68 )
( 2486 , 76.80 )
( 2487 , 77.06 )
( 2488 , 77.32 )
( 2489 , 77.60 )
( 2490 , 77.86 )
( 2491 , 77.98 )
( 2492 , 78.17 )
( 2493 , 78.33 )
( 2494 , 78.46 )
( 2495 , 78.61 )
( 2496 , 78.76 )
( 2497 , 78.88 )
( 2498 , 79.02 )
( 2499 , 79.14 )
( 2500 , 79.31 )
( 2501 , 79.48 )
( 2502 , 79.60 )
( 2503 , 79.58 )
( 2504 , 79.49 )
( 2505 , 79.37 )
( 2506 , 79.27 )
( 2507 , 79.39 )
( 2508 , 79.30 )
( 2509 , 79.18 )
( 2510 , 79.05 )
( 2511 , 78.95 )
( 2512 , 78.84 )
( 2513 , 78.71 )
( 2514 , 78.62 )
( 2515 , 78.50 )
( 2516 , 78.54 )
( 2517 , 78.65 )
( 2518 , 78.73 )
( 2519 , 78.81 )
( 2520 , 78.89 )
( 2521 , 78.94 )
( 2522 , 78.98 )
( 2523 , 78.88 )
( 2524 , 78.76 )
( 2525 , 78.74 )
( 2526 , 78.65 )
( 2527 , 78.58 )
( 2528 , 78.48 )
( 2529 , 78.40 )
( 2530 , 78.36 )
( 2531 , 78.45 )
( 2532 , 78.48 )
( 2533 , 78.40 )
( 2534 , 78.42 )
( 2535 , 78.32 )
( 2536 , 78.23 )
( 2537 , 77.92 )
( 2538 , 77.63 )
( 2539 , 77.38 )
( 2540 , 77.08 )
( 2541 , 76.99 )
( 2542 , 76.96 )
( 2543 , 76.66 )
( 2544 , 76.54 )
( 2545 , 76.23 )
( 2546 , 76.01 )
( 2547 , 75.77 )
( 2548 , 75.49 )
( 2549 , 75.22 )
( 2550 , 75.01 )
( 2551 , 74.76 )
( 2552 , 74.50 )
( 2553 , 74.21 )
( 2554 , 73.91 )
( 2555 , 73.61 )
( 2556 , 73.47 )
( 2557 , 73.36 )
( 2558 , 73.06 )
( 2559 , 72.76 )
( 2560 , 72.47 )
( 2561 , 72.19 )
( 2562 , 71.88 )
( 2563 , 71.84 )
( 2564 , 71.74 )
( 2565 , 71.73 )
( 2566 , 71.43 )
( 2567 , 71.20 )
( 2568 , 70.89 )
( 2569 , 70.59 )
( 2570 , 70.29 )
( 2571 , 69.99 )
( 2572 , 69.88 )
( 2573 , 69.80 )
( 2574 , 69.68 )
( 2575 , 69.55 )
( 2576 , 69.49 )
( 2577 , 69.39 )
( 2578 , 69.27 )
( 2579 , 69.30 )
( 2580 , 69.19 )
( 2581 , 69.06 )
( 2582 , 69.21 )
( 2583 , 69.41 )
( 2584 , 69.61 )
( 2585 , 69.89 )
( 2586 , 70.02 )
( 2587 , 69.95 )
( 2588 , 69.88 )
( 2589 , 69.83 )
( 2590 , 69.76 )
( 2591 , 69.73 )
( 2592 , 69.62 )
( 2593 , 69.49 )
( 2594 , 69.37 )
( 2595 , 69.26 )
( 2596 , 69.13 )
( 2597 , 69.32 )
( 2598 , 69.49 )
( 2599 , 69.68 )
( 2600 , 69.69 )
( 2601 , 69.74 )
( 2602 , 69.92 )
( 2603 , 70.10 )
( 2604 , 70.27 )
( 2605 , 70.56 )
( 2606 , 70.76 )
( 2607 , 70.95 )
( 2608 , 71.16 )
( 2609 , 71.34 )
( 2610 , 71.53 )
( 2611 , 71.73 )
( 2612 , 71.61 )
( 2613 , 71.48 )
( 2614 , 71.53 )
( 2615 , 71.57 )
( 2616 , 71.62 )
( 2617 , 71.51 )
( 2618 , 71.38 )
( 2619 , 71.26 )
( 2620 , 71.38 )
( 2621 , 71.52 )
( 2622 , 71.66 )
( 2623 , 71.84 )
( 2624 , 71.97 )
( 2625 , 72.10 )
( 2626 , 72.25 )
( 2627 , 72.38 )
( 2628 , 72.53 )
( 2629 , 72.70 )
( 2630 , 72.91 )
( 2631 , 73.17 )
( 2632 , 73.45 )
( 2633 , 73.57 )
( 2634 , 73.82 )
( 2635 , 74.08 )
( 2636 , 74.34 )
( 2637 , 74.60 )
( 2638 , 74.86 )
( 2639 , 75.11 )
( 2640 , 75.39 )
( 2641 , 75.52 )
( 2642 , 75.70 )
( 2643 , 75.89 )
( 2644 , 76.08 )
( 2645 , 76.30 )
( 2646 , 76.42 )
( 2647 , 76.59 )
( 2648 , 76.88 )
( 2649 , 77.16 )
( 2650 , 77.44 )
( 2651 , 77.57 )
( 2652 , 77.70 )
( 2653 , 77.88 )
( 2654 , 78.06 )
( 2655 , 78.21 )
( 2656 , 78.48 )
( 2657 , 78.67 )
( 2658 , 78.87 )
( 2659 , 79.01 )
( 2660 , 79.14 )
( 2661 , 79.30 )
( 2662 , 79.47 )
( 2663 , 79.60 )
( 2664 , 79.73 )
( 2665 , 79.85 )
( 2666 , 79.99 )
( 2667 , 80.27 )
( 2668 , 80.40 )
( 2669 , 80.53 )
( 2670 , 80.66 )
( 2671 , 80.78 )
( 2672 , 80.91 )
( 2673 , 81.03 )
( 2674 , 81.16 )
( 2675 , 81.30 )
( 2676 , 81.44 )
( 2677 , 81.62 )
( 2678 , 81.92 )
( 2679 , 82.05 )
( 2680 , 82.30 )
( 2681 , 82.59 )
( 2682 , 82.92 )
( 2683 , 83.19 )
( 2684 , 83.40 )
( 2685 , 83.60 )
( 2686 , 83.48 )
( 2687 , 83.36 )
( 2688 , 83.23 )
( 2689 , 83.16 )
( 2690 , 83.09 )
( 2691 , 83.13 )
( 2692 , 83.12 )
( 2693 , 83.01 )
( 2694 , 82.91 )
( 2695 , 82.80 )
( 2696 , 82.73 )
( 2697 , 82.60 )
( 2698 , 82.48 )
( 2699 , 82.52 )
( 2700 , 82.40 )
( 2701 , 82.30 )
( 2702 , 82.19 )
( 2703 , 82.09 )
( 2704 , 82.40 )
( 2705 , 82.69 )
( 2706 , 83.02 )
( 2707 , 83.20 )
( 2708 , 83.33 )
( 2709 , 83.21 )
( 2710 , 83.09 )
( 2711 , 82.97 )
( 2712 , 82.84 )
( 2713 , 82.80 )
( 2714 , 82.75 )
( 2715 , 82.86 )
( 2716 , 82.90 )
( 2717 , 82.98 )
( 2718 , 83.08 )
( 2719 , 83.15 )
( 2720 , 83.16 )
( 2721 , 83.16 )
( 2722 , 83.15 )
( 2723 , 83.20 )
( 2724 , 83.18 )
( 2725 , 83.17 )
( 2726 , 82.88 )
( 2727 , 82.58 )
( 2728 , 82.49 )
( 2729 , 82.48 )
( 2730 , 82.39 )
( 2731 , 82.34 )
( 2732 , 82.04 )
( 2733 , 81.89 )
( 2734 , 81.95 )
( 2735 , 81.91 )
( 2736 , 81.84 )
( 2737 , 81.80 )
( 2738 , 81.88 )
( 2739 , 81.84 )
( 2740 , 81.73 )
( 2741 , 81.45 )
( 2742 , 81.16 )
( 2743 , 80.86 )
( 2744 , 80.66 )
( 2745 , 80.55 )
( 2746 , 80.51 )
( 2747 , 80.45 )
( 2748 , 80.43 )
( 2749 , 80.45 )
( 2750 , 80.39 )
( 2751 , 80.34 )
( 2752 , 80.19 )
( 2753 , 79.88 )
( 2754 , 79.59 )
( 2755 , 79.45 )
( 2756 , 79.14 )
( 2757 , 78.84 )
( 2758 , 78.57 )
( 2759 , 78.27 )
( 2760 , 78.29 )
( 2761 , 78.30 )
( 2762 , 78.27 )
( 2763 , 78.25 )
( 2764 , 78.39 )
( 2765 , 78.53 )
( 2766 , 78.69 )
( 2767 , 78.85 )
( 2768 , 79.00 )
( 2769 , 79.15 )
( 2770 , 79.32 )
( 2771 , 79.31 )
( 2772 , 79.26 )
( 2773 , 79.25 )
( 2774 , 79.20 )
( 2775 , 79.13 )
( 2776 , 79.11 )
( 2777 , 79.18 )
( 2778 , 79.26 )
( 2779 , 79.20 )
( 2780 , 79.18 )
( 2781 , 79.16 )
( 2782 , 79.11 )
( 2783 , 79.06 )
( 2784 , 79.12 )
( 2785 , 79.09 )
( 2786 , 79.04 )
( 2787 , 78.98 )
( 2788 , 78.98 )
( 2789 , 78.95 )
( 2790 , 78.91 )
( 2791 , 78.89 )
( 2792 , 79.03 )
( 2793 , 79.27 )
( 2794 , 79.51 )
( 2795 , 79.65 )
( 2796 , 79.89 )
( 2797 , 80.17 )
( 2798 , 80.34 )
( 2799 , 80.38 )
( 2800 , 80.42 )
( 2801 , 80.46 )
( 2802 , 80.50 )
( 2803 , 80.50 )
( 2804 , 80.52 )
( 2805 , 80.68 )
( 2806 , 80.82 )
( 2807 , 81.00 )
( 2808 , 81.22 )
( 2809 , 81.41 )
( 2810 , 81.59 )
( 2811 , 81.62 )
( 2812 , 81.68 )
( 2813 , 81.71 )
( 2814 , 81.76 )
( 2815 , 81.74 )
( 2816 , 81.73 )
( 2817 , 81.72 )
( 2818 , 81.70 )
( 2819 , 81.72 )
( 2820 , 81.73 )
( 2821 , 81.86 )
( 2822 , 81.98 )
( 2823 , 81.96 )
( 2824 , 82.01 )
( 2825 , 81.98 )
( 2826 , 81.97 )
( 2827 , 81.94 )
( 2828 , 81.91 )
( 2829 , 81.91 )
( 2830 , 81.88 )
( 2831 , 81.85 )
( 2832 , 81.84 )
( 2833 , 81.80 )
( 2834 , 81.94 )
( 2835 , 81.88 )
( 2836 , 81.91 )
( 2837 , 81.94 )
( 2838 , 81.96 )
( 2839 , 82.12 )
( 2840 , 82.12 )
( 2841 , 82.07 )
( 2842 , 82.04 )
( 2843 , 81.98 )
( 2844 , 81.95 )
( 2845 , 82.21 )
( 2846 , 82.45 )
( 2847 , 82.64 )
( 2848 , 82.34 )
( 2849 , 82.20 )
( 2850 , 82.05 )
( 2851 , 81.97 )
( 2852 , 81.99 )
( 2853 , 81.70 )
( 2854 , 81.73 )
( 2855 , 81.77 )
( 2856 , 81.68 )
( 2857 , 81.73 )
( 2858 , 81.80 )
( 2859 , 81.66 )
( 2860 , 81.69 )
( 2861 , 81.59 )
( 2862 , 81.34 )
( 2863 , 81.14 )
( 2864 , 80.87 )
( 2865 , 80.57 )
( 2866 , 80.36 )
( 2867 , 80.05 )
( 2868 , 79.76 )
( 2869 , 79.52 )
( 2870 , 79.23 )
( 2871 , 79.02 )
( 2872 , 78.98 )
( 2873 , 79.02 )
( 2874 , 78.99 )
( 2875 , 78.90 )
( 2876 , 78.59 )
( 2877 , 78.45 )
( 2878 , 78.30 )
( 2879 , 78.00 )
( 2880 , 77.72 )
( 2881 , 77.41 )
( 2882 , 77.29 )
( 2883 , 77.14 )
( 2884 , 76.95 )
( 2885 , 76.76 )
( 2886 , 76.45 )
( 2887 , 76.39 )
( 2888 , 76.09 )
( 2889 , 75.80 )
( 2890 , 75.49 )
( 2891 , 75.26 )
( 2892 , 75.16 )
( 2893 , 74.88 )
( 2894 , 74.67 )
( 2895 , 74.44 )
( 2896 , 74.14 )
( 2897 , 73.84 )
( 2898 , 73.54 )
( 2899 , 73.34 )
( 2900 , 73.04 )
( 2901 , 72.74 )
( 2902 , 72.45 )
( 2903 , 72.32 )
( 2904 , 72.20 )
( 2905 , 71.89 )
( 2906 , 71.59 )
( 2907 , 71.30 )
( 2908 , 71.09 )
( 2909 , 70.88 )
( 2910 , 70.69 )
( 2911 , 70.38 )
( 2912 , 70.29 )
( 2913 , 70.23 )
( 2914 , 70.15 )
( 2915 , 69.86 )
( 2916 , 69.84 )
( 2917 , 69.75 )
( 2918 , 69.66 )
( 2919 , 69.41 )
( 2920 , 69.45 )
( 2921 , 69.36 )
( 2922 , 69.35 )
( 2923 , 69.26 )
( 2924 , 68.95 )
( 2925 , 68.67 )
( 2926 , 68.41 )
( 2927 , 68.35 )
( 2928 , 68.09 )
( 2929 , 68.05 )
( 2930 , 67.78 )
( 2931 , 67.48 )
( 2932 , 67.19 )
( 2933 , 66.89 )
( 2934 , 66.64 )
( 2935 , 66.41 )
( 2936 , 66.32 )
( 2937 , 66.22 )
( 2938 , 66.12 )
( 2939 , 66.16 )
( 2940 , 66.17 )
( 2941 , 66.11 )
( 2942 , 66.02 )
( 2943 , 65.72 )
( 2944 , 65.66 )
( 2945 , 65.52 )
( 2946 , 65.38 )
( 2947 , 65.07 )
( 2948 , 65.04 )
( 2949 , 64.84 )
( 2950 , 64.58 )
( 2951 , 64.54 )
( 2952 , 64.42 )
( 2953 , 64.27 )
( 2954 , 64.17 )
( 2955 , 63.96 )
( 2956 , 63.66 )
( 2957 , 63.40 )
( 2958 , 63.10 )
( 2959 , 62.90 )
( 2960 , 62.60 )
( 2961 , 62.54 )
( 2962 , 62.23 )
( 2963 , 62.09 )
( 2964 , 61.92 )
( 2965 , 61.73 )
( 2966 , 61.49 )
( 2967 , 61.23 )
( 2968 , 60.94 )
( 2969 , 60.65 )
( 2970 , 60.35 )
( 2971 , 60.05 )
( 2972 , 59.75 )
( 2973 , 59.45 )
( 2974 , 59.18 )
( 2975 , 59.04 )
( 2976 , 58.75 )
( 2977 , 58.45 )
( 2978 , 58.15 )
( 2979 , 57.92 )
( 2980 , 57.63 )
( 2981 , 57.38 )
( 2982 , 57.15 )
( 2983 , 56.88 )
( 2984 , 56.74 )
( 2985 , 56.62 )
( 2986 , 56.32 )
( 2987 , 56.27 )
( 2988 , 56.21 )
( 2989 , 55.91 )
( 2990 , 55.61 )
( 2991 , 55.32 )
( 2992 , 55.34 )
( 2993 , 55.04 )
( 2994 , 54.74 )
( 2995 , 54.44 )
( 2996 , 54.15 )
( 2997 , 53.86 )
( 2998 , 53.55 )
( 2999 , 53.38 )
( 3000 , 53.18 )
( 3001 , 52.88 )
( 3002 , 52.58 )
( 3003 , 52.28 )
( 3004 , 52.16 )
( 3005 , 51.86 )
( 3006 , 51.56 )
( 3007 , 51.41 )
( 3008 , 51.26 )
( 3009 , 50.97 )
( 3010 , 50.71 )
( 3011 , 50.59 )
( 3012 , 50.66 )
( 3013 , 50.57 )
( 3014 , 50.59 )
( 3015 , 50.62 )
( 3016 , 50.65 )
( 3017 , 50.58 )
( 3018 , 50.52 )
( 3019 , 50.53 )
( 3020 , 50.45 )
( 3021 , 50.41 )
( 3022 , 50.11 )
( 3023 , 49.86 )
( 3024 , 49.59 )
( 3025 , 49.39 )
( 3026 , 49.27 )
( 3027 , 49.01 )
( 3028 , 48.71 )
( 3029 , 48.41 )
( 3030 , 48.36 )
( 3031 , 48.27 )
( 3032 , 48.12 )
( 3033 , 47.92 )
( 3034 , 47.77 )
( 3035 , 47.47 )
( 3036 , 47.17 )
( 3037 , 47.07 )
( 3038 , 46.92 )
( 3039 , 46.72 )
( 3040 , 46.43 )
( 3041 , 46.34 )
( 3042 , 46.04 )
( 3043 , 45.74 )
( 3044 , 45.44 )
( 3045 , 45.14 )
( 3046 , 45.04 )
( 3047 , 44.75 )
( 3048 , 44.61 )
( 3049 , 44.48 )
( 3050 , 44.19 )
( 3051 , 44.04 )
( 3052 , 43.75 )
( 3053 , 43.45 )
( 3054 , 43.14 )
( 3055 , 42.86 )
( 3056 , 42.64 )
( 3057 , 42.34 )
( 3058 , 42.38 )
( 3059 , 42.18 )
( 3060 , 42.07 )
( 3061 , 41.89 )
( 3062 , 41.79 )
( 3063 , 41.49 )
( 3064 , 41.26 )
( 3065 , 40.96 )
( 3066 , 40.79 )
( 3067 , 40.48 )
( 3068 , 40.41 )
( 3069 , 40.15 )
( 3070 , 39.89 )
( 3071 , 39.64 )
( 3072 , 39.41 )
( 3073 , 39.28 )
( 3074 , 38.98 )
( 3075 , 38.75 )
( 3076 , 38.61 )
( 3077 , 38.45 )
( 3078 , 38.25 )
( 3079 , 38.11 )
( 3080 , 37.91 )
( 3081 , 37.61 )
( 3082 , 37.31 )
( 3083 , 37.17 )
( 3084 , 36.88 )
( 3085 , 36.62 )
( 3086 , 36.53 )
( 3087 , 36.43 )
( 3088 , 36.38 )
( 3089 , 36.29 )
( 3090 , 36.20 )
( 3091 , 36.15 )
( 3092 , 36.09 )
( 3093 , 35.79 )
( 3094 , 35.91 )
( 3095 , 36.04 )
( 3096 , 36.17 )
( 3097 , 36.36 )
( 3098 , 36.57 )
( 3099 , 36.80 )
( 3100 , 36.96 )
( 3101 , 37.17 )
( 3102 , 37.38 )
( 3103 , 37.52 )
( 3104 , 37.49 )
( 3105 , 37.46 )
( 3106 , 37.21 )
( 3107 , 36.91 )
( 3108 , 36.84 )
( 3109 , 36.76 )
( 3110 , 36.69 )
( 3111 , 36.39 )
( 3112 , 36.09 )
( 3113 , 35.97 )
( 3114 , 35.67 )
( 3115 , 35.57 )
( 3116 , 35.29 )
( 3117 , 35.18 )
( 3118 , 34.90 )
( 3119 , 34.78 )
( 3120 , 34.72 )
( 3121 , 34.46 )
( 3122 , 34.26 )
( 3123 , 34.02 )
( 3124 , 33.73 )
( 3125 , 33.44 )
( 3126 , 33.14 )
( 3127 , 32.84 )
( 3128 , 32.54 )
( 3129 , 32.24 )
( 3130 , 32.00 )
( 3131 , 31.74 )
( 3132 , 31.79 )
( 3133 , 31.50 )
( 3134 , 31.20 )
( 3135 , 30.89 )
( 3136 , 30.78 )
( 3137 , 30.48 )
( 3138 , 30.25 )
( 3139 , 29.95 )
( 3140 , 29.71 )
( 3141 , 29.55 )
( 3142 , 29.27 )
( 3143 , 29.05 )
( 3144 , 28.75 )
( 3145 , 28.46 )
( 3146 , 28.31 )
( 3147 , 28.10 )
( 3148 , 28.06 )
( 3149 , 27.76 )
( 3150 , 27.51 )
( 3151 , 27.28 )
( 3152 , 27.24 )
( 3153 , 27.30 )
( 3154 , 27.23 )
( 3155 , 27.14 )
( 3156 , 27.04 )
( 3157 , 26.95 )
( 3158 , 26.65 )
( 3159 , 26.60 )
( 3160 , 26.46 )
( 3161 , 26.23 )
( 3162 , 25.93 )
( 3163 , 25.83 )
( 3164 , 25.73 )
( 3165 , 25.49 )
( 3166 , 25.19 )
( 3167 , 25.15 )
( 3168 , 25.05 )
( 3169 , 24.97 )
( 3170 , 24.67 )
( 3171 , 24.37 )
( 3172 , 24.15 )
( 3173 , 23.92 )
( 3174 , 23.62 )
( 3175 , 23.38 )
( 3176 , 23.17 )
( 3177 , 22.87 )
( 3178 , 22.57 )
( 3179 , 22.31 )
( 3180 , 22.04 )
( 3181 , 21.97 )
( 3182 , 21.67 )
( 3183 , 21.46 )
( 3184 , 21.27 )
( 3185 , 21.17 )
( 3186 , 21.14 )
( 3187 , 21.14 )
( 3188 , 20.99 )
( 3189 , 20.96 )
( 3190 , 20.82 )
( 3191 , 20.52 )
( 3192 , 20.37 )
( 3193 , 20.24 )
( 3194 , 19.96 )
( 3195 , 19.66 )
( 3196 , 19.57 )
( 3197 , 19.26 )
( 3198 , 18.96 )
( 3199 , 18.66 )
( 3200 , 18.54 )
( 3201 , 18.25 )
( 3202 , 17.95 )
( 3203 , 17.65 )
( 3204 , 17.35 )
( 3205 , 17.21 )
( 3206 , 17.04 )
( 3207 , 16.77 )
( 3208 , 16.73 )
( 3209 , 16.64 )
( 3210 , 16.35 )
( 3211 , 16.08 )
( 3212 , 16.10 )
( 3213 , 16.05 )
( 3214 , 15.75 )
( 3215 , 15.50 )
( 3216 , 15.40 )
( 3217 , 15.31 )
( 3218 , 15.21 )
( 3219 , 15.08 )
( 3220 , 14.94 )
( 3221 , 14.85 )
( 3222 , 14.75 )
( 3223 , 14.45 )
( 3224 , 14.31 )
( 3225 , 14.16 )
( 3226 , 13.86 )
( 3227 , 13.56 )
( 3228 , 13.37 )
( 3229 , 13.07 )
( 3230 , 12.90 )
( 3231 , 12.68 )
( 3232 , 12.70 )
( 3233 , 12.49 )
( 3234 , 12.25 )
( 3235 , 12.04 )
( 3236 , 11.97 )
( 3237 , 11.87 )
( 3238 , 11.60 )
( 3239 , 11.30 )
( 3240 , 11.45 )
( 3241 , 11.52 )
( 3242 , 11.57 )
( 3243 , 11.57 )
( 3244 , 11.58 )
( 3245 , 11.62 )
( 3246 , 11.66 )
( 3247 , 11.66 )
( 3248 , 11.66 )
( 3249 , 12.01 )
( 3250 , 12.36 )
( 3251 , 12.58 )
( 3252 , 12.80 )
( 3253 , 13.20 )
( 3254 , 13.50 )
( 3255 , 13.75 )
( 3256 , 14.07 )
( 3257 , 14.35 )
( 3258 , 14.74 )
( 3259 , 15.15 )
( 3260 , 15.47 )
( 3261 , 15.75 )
( 3262 , 15.75 )
( 3263 , 15.97 )
( 3264 , 16.39 )
( 3265 , 16.79 )
( 3266 , 17.17 )
( 3267 , 17.54 )
( 3268 , 17.71 )
( 3269 , 17.86 )
( 3270 , 18.08 )
( 3271 , 18.08 )
( 3272 , 18.09 )
( 3273 , 18.10 )
( 3274 , 18.10 )
( 3275 , 18.45 )
( 3276 , 18.94 )
( 3277 , 19.26 )
( 3278 , 19.55 )
( 3279 , 19.84 )
( 3280 , 20.12 )
( 3281 , 20.58 )
( 3282 , 21.03 )
( 3283 , 21.48 )
( 3284 , 21.96 )
( 3285 , 22.37 )
( 3286 , 22.65 )
( 3287 , 22.94 )
( 3288 , 23.02 )
( 3289 , 23.09 )
( 3290 , 23.09 )
( 3291 , 23.12 )
( 3292 , 23.17 )
( 3293 , 23.17 )
( 3294 , 23.59 )
( 3295 , 23.95 )
( 3296 , 24.30 )
( 3297 , 24.52 )
( 3298 , 24.75 )
( 3299 , 25.03 )
( 3300 , 25.29 )
( 3301 , 25.54 )
( 3302 , 25.83 )
( 3303 , 26.05 )
( 3304 , 26.43 )
( 3305 , 26.77 )
( 3306 , 27.05 )
( 3307 , 27.28 )
( 3308 , 27.50 )
( 3309 , 27.72 )
( 3310 , 28.00 )
( 3311 , 28.22 )
( 3312 , 28.46 )
( 3313 , 28.69 )
( 3314 , 28.98 )
( 3315 , 29.28 )
( 3316 , 29.28 )
( 3317 , 29.28 )
( 3318 , 29.30 )
( 3319 , 29.30 )
( 3320 , 29.30 )
( 3321 , 29.45 )
( 3322 , 29.65 )
( 3323 , 29.86 )
( 3324 , 30.00 )
( 3325 , 30.00 )
( 3326 , 30.03 )
( 3327 , 30.03 )
( 3328 , 30.05 )
( 3329 , 30.10 )
( 3330 , 30.31 )
( 3331 , 30.57 )
( 3332 , 30.78 )
( 3333 , 30.94 )
( 3334 , 31.15 )
( 3335 , 31.15 )
( 3336 , 31.15 )
( 3337 , 31.20 )
( 3338 , 31.20 )
( 3339 , 31.27 )
( 3340 , 31.27 )
( 3341 , 31.27 )
( 3342 , 31.27 )
( 3343 , 31.49 )
( 3344 , 31.65 )
( 3345 , 31.71 )
( 3346 , 31.78 )
( 3347 , 31.82 )
( 3348 , 31.84 )
( 3349 , 31.92 )
( 3350 , 31.93 )
( 3351 , 32.00 )
( 3352 , 32.07 )
( 3353 , 32.19 )
( 3354 , 32.19 )
( 3355 , 32.21 )
( 3356 , 32.29 )
( 3357 , 32.33 )
( 3358 , 32.33 )
( 3359 , 32.48 )
( 3360 , 32.55 )
( 3361 , 32.63 )
( 3362 , 32.71 )
( 3363 , 32.77 )
( 3364 , 32.77 )
( 3365 , 32.79 )
( 3366 , 32.79 )
( 3367 , 32.79 )
( 3368 , 32.79 )
( 3369 , 32.82 )
( 3370 , 32.82 )
( 3371 , 32.96 )
( 3372 , 33.11 )
( 3373 , 33.31 )
( 3374 , 33.53 )
( 3375 , 33.59 )
( 3376 , 33.62 )
( 3377 , 33.78 )
( 3378 , 33.93 )
( 3379 , 34.10 )
( 3380 , 34.25 )
( 3381 , 34.25 )
( 3382 , 34.48 )
( 3383 , 34.72 )
( 3384 , 34.96 )
( 3385 , 35.30 )
( 3386 , 35.55 )
( 3387 , 35.86 )
( 3388 , 36.14 )
( 3389 , 36.41 )
( 3390 , 36.73 )
( 3391 , 37.04 )
( 3392 , 37.04 )
( 3393 , 37.04 )
( 3394 , 37.08 )
( 3395 , 37.18 )
( 3396 , 37.18 )
( 3397 , 37.18 )
( 3398 , 37.18 )
( 3399 , 37.18 )
( 3400 , 37.22 )
( 3401 , 37.22 )
( 3402 , 37.67 )
( 3403 , 38.02 )
( 3404 , 38.26 )
( 3405 , 38.52 )
( 3406 , 38.75 )
( 3407 , 38.98 )
( 3408 , 39.27 )
( 3409 , 39.50 )
( 3410 , 39.79 )
( 3411 , 40.11 )
( 3412 , 40.40 )
( 3413 , 40.63 )
( 3414 , 40.91 )
( 3415 , 41.13 )
( 3416 , 41.36 )
( 3417 , 41.61 )
( 3418 , 41.84 )
( 3419 , 42.20 )
( 3420 , 42.54 )
( 3421 , 42.83 )
( 3422 , 42.91 )
( 3423 , 42.91 )
( 3424 , 42.94 )
( 3425 , 42.94 )
( 3426 , 42.97 )
( 3427 , 43.08 )
( 3428 , 43.12 )
( 3429 , 43.12 )
( 3430 , 43.35 )
( 3431 , 43.35 )
( 3432 , 43.35 )
( 3433 , 43.41 )
( 3434 , 43.60 )
( 3435 , 43.80 )
( 3436 , 43.95 )
( 3437 , 44.11 )
( 3438 , 44.25 )
( 3439 , 44.41 )
( 3440 , 44.43 )
( 3441 , 44.43 )
( 3442 , 44.77 )
( 3443 , 45.01 )
( 3444 , 45.23 )
( 3445 , 45.46 )
( 3446 , 45.68 )
( 3447 , 45.92 )
( 3448 , 46.15 )
( 3449 , 46.37 )
( 3450 , 46.38 )
( 3451 , 46.54 )
( 3452 , 46.71 )
( 3453 , 46.86 )
( 3454 , 47.00 )
( 3455 , 47.16 )
( 3456 , 47.36 )
( 3457 , 47.51 )
( 3458 , 47.51 )
( 3459 , 47.56 )
( 3460 , 47.60 )
( 3461 , 47.60 )
( 3462 , 47.61 )
( 3463 , 47.61 )
( 3464 , 47.67 )
( 3465 , 47.67 )
( 3466 , 47.74 )
( 3467 , 47.75 )
( 3468 , 47.75 )
( 3469 , 47.75 )
( 3470 , 47.75 )
( 3471 , 47.92 )
( 3472 , 47.94 )
( 3473 , 47.94 )
( 3474 , 47.94 )
( 3475 , 47.94 )
( 3476 , 47.94 )
( 3477 , 47.94 )
( 3478 , 47.95 )
( 3479 , 48.04 )
( 3480 , 48.08 )
( 3481 , 48.12 )
( 3482 , 48.12 )
( 3483 , 48.14 )
( 3484 , 48.14 )
( 3485 , 48.15 )
( 3486 , 48.22 )
( 3487 , 48.28 )
( 3488 , 48.37 )
( 3489 , 48.52 )
( 3490 , 48.69 )
( 3491 , 48.70 )
( 3492 , 48.70 )
( 3493 , 48.72 )
( 3494 , 48.75 )
( 3495 , 48.75 )
( 3496 , 49.02 )
( 3497 , 49.24 )
( 3498 , 49.46 )
( 3499 , 49.69 )
( 3500 , 50.04 )
( 3501 , 50.37 )
( 3502 , 50.70 )
( 3503 , 50.98 )
( 3504 , 51.20 )
( 3505 , 51.62 )
( 3506 , 51.84 )
( 3507 , 51.84 )
( 3508 , 51.85 )
( 3509 , 51.85 )
( 3510 , 51.88 )
( 3511 , 51.88 )
( 3512 , 51.88 )
( 3513 , 51.88 )
( 3514 , 51.89 )
( 3515 , 51.90 )
( 3516 , 51.93 )
( 3517 , 51.98 )
( 3518 , 51.98 )
( 3519 , 51.98 )
( 3520 , 51.98 )
( 3521 , 51.98 )
( 3522 , 51.98 )
( 3523 , 51.99 )
( 3524 , 52.00 )
( 3525 , 52.02 )
( 3526 , 52.04 )
( 3527 , 52.04 )
( 3528 , 52.39 )
( 3529 , 52.71 )
( 3530 , 53.06 )
( 3531 , 53.42 )
( 3532 , 53.72 )
( 3533 , 54.01 )
( 3534 , 54.29 )
( 3535 , 54.57 )
( 3536 , 54.84 )
( 3537 , 55.07 )
( 3538 , 55.34 )
( 3539 , 55.62 )
( 3540 , 55.70 )
( 3541 , 55.78 )
( 3542 , 55.78 )
( 3543 , 55.78 )
( 3544 , 55.78 )
( 3545 , 55.82 )
( 3546 , 55.82 )
( 3547 , 55.89 )
( 3548 , 55.94 )
( 3549 , 55.94 )
( 3550 , 56.00 )
( 3551 , 56.04 )
( 3552 , 56.04 )
( 3553 , 56.06 )
( 3554 , 56.06 )
( 3555 , 56.06 )
( 3556 , 56.06 )
( 3557 , 56.06 )
( 3558 , 56.07 )
( 3559 , 56.07 )
( 3560 , 56.07 )
( 3561 , 56.15 )
( 3562 , 56.23 )
( 3563 , 56.39 )
( 3564 , 56.39 )
( 3565 , 56.40 )
( 3566 , 56.41 )
( 3567 , 56.41 )
( 3568 , 56.43 )
( 3569 , 56.46 )
( 3570 , 56.53 )
( 3571 , 56.54 )
( 3572 , 56.54 )
( 3573 , 56.54 )
( 3574 , 56.55 )
( 3575 , 56.55 )
( 3576 , 56.55 )
( 3577 , 56.70 )
( 3578 , 56.77 )
( 3579 , 56.77 )
( 3580 , 57.07 )
( 3581 , 57.35 )
( 3582 , 57.63 )
( 3583 , 57.78 )
( 3584 , 57.78 )
( 3585 , 57.96 )
( 3586 , 58.04 )
( 3587 , 58.04 )
( 3588 , 58.04 )
( 3589 , 58.26 )
( 3590 , 58.48 )
( 3591 , 58.71 )
( 3592 , 58.93 )
( 3593 , 59.18 )
( 3594 , 59.40 )
( 3595 , 59.62 )
( 3596 , 59.90 )
( 3597 , 60.14 )
( 3598 , 60.41 )
( 3599 , 60.66 )
( 3600 , 61.02 )
( 3601 , 61.41 )
( 3602 , 61.75 )
( 3603 , 62.09 )
( 3604 , 62.38 )
( 3605 , 62.61 )
( 3606 , 62.84 )
( 3607 , 63.06 )
( 3608 , 63.35 )
( 3609 , 63.58 )
( 3610 , 63.63 )
( 3611 , 63.63 )
( 3612 , 63.71 )
( 3613 , 63.73 )
( 3614 , 63.96 )
( 3615 , 64.25 )
( 3616 , 64.48 )
( 3617 , 64.54 )
( 3618 , 64.62 )
( 3619 , 64.88 )
( 3620 , 65.27 )
( 3621 , 65.50 )
( 3622 , 65.72 )
( 3623 , 66.01 )
( 3624 , 66.21 )
( 3625 , 66.18 )
( 3626 , 66.15 )
( 3627 , 66.27 )
( 3628 , 66.41 )
( 3629 , 66.55 )
( 3630 , 66.67 )
( 3631 , 66.80 )
( 3632 , 66.98 )
( 3633 , 67.10 )
( 3634 , 67.08 )
( 3635 , 67.02 )
( 3636 , 67.05 )
( 3637 , 67.02 )
( 3638 , 66.91 )
( 3639 , 66.78 )
( 3640 , 66.73 )
( 3641 , 66.61 )
( 3642 , 66.62 )
( 3643 , 66.76 )
( 3644 , 66.75 )
( 3645 , 66.73 )
( 3646 , 66.88 )
( 3647 , 66.87 )
( 3648 , 66.88 )
( 3649 , 66.89 )
( 3650 , 66.88 )
( 3651 , 66.84 )
( 3652 , 66.87 )
( 3653 , 66.82 )
( 3654 , 66.77 )
( 3655 , 66.77 )
( 3656 , 66.73 )
( 3657 , 66.67 )
( 3658 , 66.70 )
( 3659 , 66.76 )
( 3660 , 66.80 )
( 3661 , 66.77 )
( 3662 , 66.72 )
( 3663 , 66.67 )
( 3664 , 66.62 )
( 3665 , 66.56 )
( 3666 , 66.52 )
( 3667 , 66.47 )
( 3668 , 66.41 )
( 3669 , 66.36 )
( 3670 , 66.30 )
( 3671 , 66.24 )
( 3672 , 66.19 )
( 3673 , 66.21 )
( 3674 , 66.15 )
( 3675 , 66.09 )
( 3676 , 65.97 )
( 3677 , 65.85 )
( 3678 , 65.73 )
( 3679 , 65.85 )
( 3680 , 65.73 )
( 3681 , 65.60 )
( 3682 , 65.56 )
( 3683 , 65.44 )
( 3684 , 65.31 )
( 3685 , 65.19 )
( 3686 , 65.06 )
( 3687 , 64.98 )
( 3688 , 64.87 )
( 3689 , 64.81 )
( 3690 , 64.71 )
( 3691 , 64.59 )
( 3692 , 64.46 )
( 3693 , 64.36 )
( 3694 , 64.31 )
( 3695 , 64.37 )
( 3696 , 64.24 )
( 3697 , 64.13 )
( 3698 , 64.26 )
( 3699 , 64.52 )
( 3700 , 64.71 )
( 3701 , 64.84 )
( 3702 , 65.00 )
( 3703 , 65.12 )
( 3704 , 65.34 )
( 3705 , 65.53 )
( 3706 , 65.73 )
( 3707 , 65.85 )
( 3708 , 65.98 )
( 3709 , 66.11 )
( 3710 , 66.30 )
( 3711 , 66.42 )
( 3712 , 66.55 )
( 3713 , 66.76 )
( 3714 , 66.91 )
( 3715 , 67.05 )
( 3716 , 67.17 )
( 3717 , 67.30 )
( 3718 , 67.55 )
( 3719 , 67.84 )
( 3720 , 68.09 )
( 3721 , 68.34 )
( 3722 , 68.52 )
( 3723 , 68.57 )
( 3724 , 68.45 )
( 3725 , 68.32 )
( 3726 , 68.20 )
( 3727 , 68.14 )
( 3728 , 68.08 )
( 3729 , 68.01 )
( 3730 , 67.94 )
( 3731 , 67.81 )
( 3732 , 67.96 )
( 3733 , 67.89 )
( 3734 , 67.83 )
( 3735 , 67.70 )
( 3736 , 67.59 )
( 3737 , 67.46 )
( 3738 , 67.59 )
( 3739 , 67.46 )
( 3740 , 67.34 )
( 3741 , 67.45 )
( 3742 , 67.49 )
( 3743 , 67.46 )
( 3744 , 67.37 )
( 3745 , 67.24 )
( 3746 , 67.45 )
( 3747 , 67.58 )
( 3748 , 67.73 )
( 3749 , 67.89 )
( 3750 , 68.13 )
( 3751 , 68.38 )
( 3752 , 68.57 )
( 3753 , 68.77 )
( 3754 , 68.93 )
( 3755 , 69.10 )
( 3756 , 69.27 )
( 3757 , 69.41 )
( 3758 , 69.53 )
( 3759 , 69.66 )
( 3760 , 69.78 )
( 3761 , 69.91 )
( 3762 , 70.20 )
( 3763 , 70.51 )
( 3764 , 70.82 )
( 3765 , 71.12 )
( 3766 , 71.25 )
( 3767 , 71.44 )
( 3768 , 71.63 )
( 3769 , 71.82 )
( 3770 , 72.02 )
( 3771 , 72.21 )
( 3772 , 72.40 )
( 3773 , 72.59 )
( 3774 , 72.77 )
( 3775 , 72.98 )
( 3776 , 73.16 )
( 3777 , 73.29 )
( 3778 , 73.16 )
( 3779 , 73.16 )
( 3780 , 73.14 )
( 3781 , 73.12 )
( 3782 , 72.99 )
( 3783 , 72.87 )
( 3784 , 72.80 )
( 3785 , 72.67 )
( 3786 , 72.74 )
( 3787 , 72.90 )
( 3788 , 73.07 )
( 3789 , 73.16 )
( 3790 , 73.21 )
( 3791 , 73.25 )
( 3792 , 73.30 )
( 3793 , 73.34 )
( 3794 , 73.40 )
( 3795 , 73.29 )
( 3796 , 73.23 )
( 3797 , 73.30 )
( 3798 , 73.38 )
( 3799 , 73.42 )
( 3800 , 73.47 )
( 3801 , 73.34 )
( 3802 , 73.29 )
( 3803 , 73.22 )
( 3804 , 73.17 )
( 3805 , 73.05 )
( 3806 , 72.93 )
( 3807 , 73.05 )
( 3808 , 73.29 )
( 3809 , 73.41 )
( 3810 , 73.54 )
( 3811 , 73.73 )
( 3812 , 73.89 )
( 3813 , 74.02 )
( 3814 , 74.15 )
( 3815 , 74.45 )
( 3816 , 74.73 )
( 3817 , 74.94 )
( 3818 , 75.06 )
( 3819 , 74.94 )
( 3820 , 74.83 )
( 3821 , 74.70 )
( 3822 , 74.59 )
( 3823 , 74.46 )
( 3824 , 74.34 )
( 3825 , 74.38 )
( 3826 , 74.27 )
( 3827 , 74.14 )
( 3828 , 74.34 )
( 3829 , 74.22 )
( 3830 , 74.11 )
( 3831 , 74.00 )
( 3832 , 73.91 )
( 3833 , 73.80 )
( 3834 , 73.67 )
( 3835 , 73.57 )
( 3836 , 73.45 )
( 3837 , 73.32 )
( 3838 , 73.20 )
( 3839 , 73.19 )
( 3840 , 73.19 )
( 3841 , 73.17 )
( 3842 , 73.16 )
( 3843 , 73.21 )
( 3844 , 73.40 )
( 3845 , 73.45 )
( 3846 , 73.43 )
( 3847 , 73.38 )
( 3848 , 73.25 )
( 3849 , 73.15 )
( 3850 , 73.21 )
( 3851 , 73.18 )
( 3852 , 73.05 )
( 3853 , 72.99 )
( 3854 , 72.87 )
( 3855 , 72.75 )
( 3856 , 72.65 )
( 3857 , 72.53 )
( 3858 , 72.41 )
( 3859 , 72.31 )
( 3860 , 72.20 )
( 3861 , 72.23 )
( 3862 , 72.19 )
( 3863 , 72.06 )
( 3864 , 71.94 )
( 3865 , 71.82 )
( 3866 , 71.73 )
( 3867 , 71.61 )
( 3868 , 71.48 )
( 3869 , 71.37 )
( 3870 , 71.34 )
( 3871 , 71.27 )
( 3872 , 71.15 )
( 3873 , 71.02 )
( 3874 , 70.90 )
( 3875 , 70.85 )
( 3876 , 70.73 )
( 3877 , 70.68 )
( 3878 , 70.62 )
( 3879 , 70.53 )
( 3880 , 70.72 )
( 3881 , 70.84 )
( 3882 , 71.06 )
( 3883 , 71.25 )
( 3884 , 71.51 )
( 3885 , 71.70 )
( 3886 , 71.89 )
( 3887 , 72.16 )
( 3888 , 72.36 )
( 3889 , 72.65 )
( 3890 , 72.88 )
( 3891 , 72.85 )
( 3892 , 72.82 )
( 3893 , 72.80 )
( 3894 , 72.83 )
( 3895 , 72.92 )
( 3896 , 73.05 )
( 3897 , 73.02 )
( 3898 , 73.02 )
( 3899 , 73.01 )
( 3900 , 73.08 )
( 3901 , 73.09 )
( 3902 , 73.09 )
( 3903 , 73.12 )
( 3904 , 73.16 )
( 3905 , 73.21 )
( 3906 , 73.25 )
( 3907 , 73.22 )
( 3908 , 73.20 )
( 3909 , 73.01 )
( 3910 , 72.70 )
( 3911 , 72.41 )
( 3912 , 72.11 )
( 3913 , 71.81 )
( 3914 , 71.51 )
( 3915 , 71.24 )
( 3916 , 70.94 )
( 3917 , 70.64 )
( 3918 , 70.34 )
( 3919 , 70.04 )
( 3920 , 69.74 )
( 3921 , 69.68 )
( 3922 , 69.66 )
( 3923 , 69.56 )
( 3924 , 69.36 )
( 3925 , 69.09 )
( 3926 , 68.80 )
( 3927 , 68.70 )
( 3928 , 68.40 )
( 3929 , 68.39 )
( 3930 , 68.12 )
( 3931 , 67.84 )
( 3932 , 67.55 )
( 3933 , 67.27 )
( 3934 , 66.98 )
( 3935 , 66.68 )
( 3936 , 66.45 )
( 3937 , 66.14 )
( 3938 , 65.84 )
( 3939 , 65.72 )
( 3940 , 65.42 )
( 3941 , 65.12 )
( 3942 , 65.16 )
( 3943 , 65.16 )
( 3944 , 65.30 )
( 3945 , 65.45 )
( 3946 , 65.45 )
( 3947 , 65.45 )
( 3948 , 65.46 )
( 3949 , 65.46 )
( 3950 , 65.52 )
( 3951 , 65.54 )
( 3952 , 65.55 )
( 3953 , 65.62 )
( 3954 , 65.68 )
( 3955 , 65.68 )
( 3956 , 65.68 )
( 3957 , 65.70 )
( 3958 , 65.70 )
( 3959 , 65.70 )
( 3960 , 65.70 )
( 3961 , 65.70 )
( 3962 , 65.70 )
( 3963 , 65.70 )
( 3964 , 65.72 )
( 3965 , 65.83 )
( 3966 , 65.90 )
( 3967 , 65.97 )
( 3968 , 65.97 )
( 3969 , 66.02 )
( 3970 , 66.09 )
( 3971 , 66.12 )
( 3972 , 66.12 )
( 3973 , 66.14 )
( 3974 , 66.14 )
( 3975 , 66.19 )
( 3976 , 66.24 )
( 3977 , 66.29 )
( 3978 , 66.30 )
( 3979 , 66.44 )
( 3980 , 66.44 )
( 3981 , 66.44 )
( 3982 , 66.45 )
( 3983 , 66.45 )
( 3984 , 66.51 )
( 3985 , 66.54 )
( 3986 , 66.55 )
( 3987 , 66.59 )
( 3988 , 66.76 )
( 3989 , 66.94 )
( 3990 , 67.00 )
( 3991 , 67.00 )
( 3992 , 67.05 )
( 3993 , 67.05 )
( 3994 , 67.16 )
( 3995 , 67.20 )
( 3996 , 67.35 )
( 3997 , 67.50 )
( 3998 , 67.56 )
( 3999 , 67.69 )
( 4000 , 67.70 )
( 4001 , 67.70 )
( 4002 , 67.70 )
( 4003 , 67.86 )
( 4004 , 68.05 )
( 4005 , 68.22 )
( 4006 , 68.23 )
( 4007 , 68.32 )
( 4008 , 68.32 )
( 4009 , 68.32 )
( 4010 , 68.59 )
( 4011 , 68.88 )
( 4012 , 69.09 )
( 4013 , 69.34 )
( 4014 , 69.56 )
( 4015 , 69.78 )
( 4016 , 69.79 )
( 4017 , 69.79 )
( 4018 , 69.94 )
( 4019 , 69.94 )
( 4020 , 69.95 )
( 4021 , 70.16 )
( 4022 , 70.16 )
( 4023 , 70.18 )
( 4024 , 70.18 )
( 4025 , 70.19 )
( 4026 , 70.38 )
( 4027 , 70.39 )
( 4028 , 70.45 )
( 4029 , 70.46 )
( 4030 , 70.64 )
( 4031 , 70.66 )
( 4032 , 70.66 )
( 4033 , 70.66 )
( 4034 , 70.66 )
( 4035 , 70.66 )
( 4036 , 70.67 )
( 4037 , 70.67 )
( 4038 , 70.67 )
( 4039 , 70.70 )
( 4040 , 70.73 )
( 4041 , 70.73 )
( 4042 , 70.73 )
( 4043 , 70.92 )
( 4044 , 71.06 )
( 4045 , 71.24 )
( 4046 , 71.40 )
( 4047 , 71.40 )
( 4048 , 71.41 )
( 4049 , 71.45 )
( 4050 , 71.45 )
( 4051 , 71.52 )
( 4052 , 71.63 )
( 4053 , 71.63 )
( 4054 , 71.65 )
( 4055 , 71.65 )
( 4056 , 71.66 )
( 4057 , 71.83 )
( 4058 , 72.10 )
( 4059 , 72.26 )
( 4060 , 72.32 )
( 4061 , 72.33 )
( 4062 , 72.33 )
( 4063 , 72.59 )
( 4064 , 72.80 )
( 4065 , 73.15 )
( 4066 , 73.49 )
( 4067 , 73.84 )
( 4068 , 74.23 )
( 4069 , 74.46 )
( 4070 , 74.68 )
( 4071 , 74.91 )
( 4072 , 75.20 )
( 4073 , 75.20 )
( 4074 , 75.23 )
( 4075 , 75.23 )
( 4076 , 75.23 )
( 4077 , 75.48 )
( 4078 , 75.71 )
( 4079 , 75.94 )
( 4080 , 76.16 )
( 4081 , 76.38 )
( 4082 , 76.61 )
( 4083 , 76.83 )
( 4084 , 77.05 )
( 4085 , 77.28 )
( 4086 , 77.52 )
( 4087 , 77.74 )
( 4088 , 78.11 )
( 4089 , 78.45 )
( 4090 , 78.82 )
( 4091 , 79.20 )
( 4092 , 79.42 )
( 4093 , 79.81 )
( 4094 , 80.16 )
( 4095 , 80.57 )
( 4096 , 80.99 )
( 4097 , 80.99 )
( 4098 , 80.99 )
( 4099 , 81.06 )
( 4100 , 81.07 )
( 4101 , 81.09 )
( 4102 , 81.16 )
( 4103 , 81.29 )
( 4104 , 81.39 )
( 4105 , 81.34 )
( 4106 , 81.29 )
( 4107 , 81.23 )
( 4108 , 81.23 )
( 4109 , 81.17 )
( 4110 , 81.11 )
( 4111 , 81.06 )
( 4112 , 81.05 )
( 4113 , 81.00 )
( 4114 , 80.94 )
( 4115 , 80.96 )
( 4116 , 80.98 )
( 4117 , 80.91 )
( 4118 , 80.79 )
( 4119 , 81.12 )
( 4120 , 81.44 )
( 4121 , 81.71 )
( 4122 , 81.98 )
( 4123 , 82.02 )
( 4124 , 81.99 )
( 4125 , 81.96 )
( 4126 , 82.23 )
( 4127 , 82.55 )
( 4128 , 82.84 )
( 4129 , 83.11 )
( 4130 , 83.38 )
( 4131 , 83.62 )
( 4132 , 83.90 )
( 4133 , 83.95 )
( 4134 , 84.01 )
( 4135 , 84.01 )
( 4136 , 83.88 )
( 4137 , 83.76 )
( 4138 , 83.64 )
( 4139 , 83.60 )
( 4140 , 83.48 )
( 4141 , 83.35 )
( 4142 , 83.25 )
( 4143 , 83.12 )
( 4144 , 83.09 )
( 4145 , 83.03 )
( 4146 , 82.91 )
( 4147 , 82.78 )
( 4148 , 82.66 )
( 4149 , 82.54 )
( 4150 , 82.44 )
( 4151 , 82.33 )
( 4152 , 82.21 )
( 4153 , 82.09 )
( 4154 , 81.98 )
( 4155 , 81.91 )
( 4156 , 81.96 )
( 4157 , 82.05 )
( 4158 , 81.99 )
( 4159 , 81.92 )
( 4160 , 81.80 )
( 4161 , 81.84 )
( 4162 , 81.92 )
( 4163 , 82.02 )
( 4164 , 82.19 )
( 4165 , 82.06 )
( 4166 , 81.94 )
( 4167 , 81.84 )
( 4168 , 81.71 )
( 4169 , 81.66 )
( 4170 , 81.64 )
( 4171 , 81.62 )
( 4172 , 81.54 )
( 4173 , 81.48 )
( 4174 , 81.36 )
( 4175 , 81.34 )
( 4176 , 81.21 )
( 4177 , 81.14 )
( 4178 , 81.02 )
( 4179 , 80.96 )
( 4180 , 80.84 )
( 4181 , 80.71 )
( 4182 , 80.66 )
( 4183 , 80.62 )
( 4184 , 80.51 )
( 4185 , 80.48 )
( 4186 , 80.38 )
( 4187 , 80.25 )
( 4188 , 80.31 )
( 4189 , 80.36 )
( 4190 , 80.23 )
( 4191 , 80.11 )
( 4192 , 79.98 )
( 4193 , 79.86 )
( 4194 , 79.73 )
( 4195 , 79.61 )
( 4196 , 79.51 )
( 4197 , 79.39 )
( 4198 , 79.38 )
( 4199 , 79.25 )
( 4200 , 79.06 )
( 4201 , 78.86 )
( 4202 , 78.56 )
( 4203 , 78.26 )
( 4204 , 78.00 )
( 4205 , 77.70 )
( 4206 , 77.50 )
( 4207 , 77.20 )
( 4208 , 76.90 )
( 4209 , 76.63 )
( 4210 , 76.34 )
( 4211 , 76.03 )
( 4212 , 75.73 )
( 4213 , 75.48 )
( 4214 , 75.19 )
( 4215 , 75.17 )
( 4216 , 74.98 )
( 4217 , 74.68 )
( 4218 , 74.38 )
( 4219 , 74.15 )
( 4220 , 73.91 )
( 4221 , 73.84 )
( 4222 , 73.60 )
( 4223 , 73.45 )
( 4224 , 73.15 )
( 4225 , 72.87 )
( 4226 , 72.58 )
( 4227 , 72.28 )
( 4228 , 72.38 )
( 4229 , 72.29 )
( 4230 , 72.18 )
( 4231 , 71.94 )
( 4232 , 71.88 )
( 4233 , 71.58 )
( 4234 , 71.28 )
( 4235 , 70.98 )
( 4236 , 70.70 )
( 4237 , 70.45 )
( 4238 , 70.20 )
( 4239 , 70.00 )
( 4240 , 69.77 )
( 4241 , 69.55 )
( 4242 , 69.31 )
( 4243 , 69.02 )
( 4244 , 68.71 )
( 4245 , 68.50 )
( 4246 , 68.29 )
( 4247 , 68.08 )
( 4248 , 67.79 )
( 4249 , 67.48 )
( 4250 , 67.27 )
( 4251 , 67.09 )
( 4252 , 66.79 )
( 4253 , 66.72 )
( 4254 , 66.45 )
( 4255 , 66.36 )
( 4256 , 66.35 )
( 4257 , 66.05 )
( 4258 , 65.81 )
( 4259 , 65.51 )
( 4260 , 65.38 )
( 4261 , 65.09 )
( 4262 , 64.79 )
( 4263 , 64.73 )
( 4264 , 64.66 )
( 4265 , 64.57 )
( 4266 , 64.42 )
( 4267 , 64.12 )
( 4268 , 63.82 )
( 4269 , 63.53 )
( 4270 , 63.23 )
( 4271 , 62.96 )
( 4272 , 62.85 )
( 4273 , 62.55 )
( 4274 , 62.25 )
( 4275 , 61.98 )
( 4276 , 61.91 )
( 4277 , 61.87 )
( 4278 , 61.81 )
( 4279 , 61.73 )
( 4280 , 61.57 )
( 4281 , 61.27 )
( 4282 , 60.97 )
( 4283 , 60.93 )
( 4284 , 60.84 )
( 4285 , 60.77 )
( 4286 , 60.67 )
( 4287 , 60.58 )
( 4288 , 60.29 )
( 4289 , 60.02 )
( 4290 , 59.79 )
( 4291 , 59.50 )
( 4292 , 59.20 )
( 4293 , 58.90 )
( 4294 , 58.91 )
( 4295 , 58.70 )
( 4296 , 58.39 )
( 4297 , 58.11 )
( 4298 , 57.81 )
( 4299 , 57.59 )
( 4300 , 57.30 )
( 4301 , 57.21 )
( 4302 , 56.91 )
( 4303 , 56.61 )
( 4304 , 56.55 )
( 4305 , 56.59 )
( 4306 , 56.50 )
( 4307 , 56.40 )
( 4308 , 56.12 )
( 4309 , 55.83 )
( 4310 , 55.53 )
( 4311 , 55.43 )
( 4312 , 55.28 )
( 4313 , 55.16 )
( 4314 , 55.02 )
( 4315 , 54.73 )
( 4316 , 54.53 )
( 4317 , 54.23 )
( 4318 , 54.14 )
( 4319 , 54.01 )
( 4320 , 53.71 )
( 4321 , 53.41 )
( 4322 , 53.54 )
( 4323 , 53.47 )
( 4324 , 53.17 )
( 4325 , 52.97 )
( 4326 , 52.67 )
( 4327 , 52.37 )
( 4328 , 52.07 )
( 4329 , 52.00 )
( 4330 , 51.71 )
( 4331 , 51.50 )
( 4332 , 51.29 )
( 4333 , 50.99 )
( 4334 , 50.89 )
( 4335 , 50.80 )
( 4336 , 50.70 )
( 4337 , 50.45 )
( 4338 , 50.16 )
( 4339 , 49.86 )
( 4340 , 49.61 )
( 4341 , 49.31 )
( 4342 , 49.01 )
( 4343 , 48.71 )
( 4344 , 48.92 )
( 4345 , 49.09 )
( 4346 , 49.27 )
( 4347 , 49.41 )
( 4348 , 49.51 )
( 4349 , 49.61 )
( 4350 , 49.71 )
( 4351 , 49.91 )
( 4352 , 50.13 )
( 4353 , 50.25 )
( 4354 , 50.38 )
( 4355 , 50.50 )
( 4356 , 50.64 )
( 4357 , 50.73 )
( 4358 , 50.76 )
( 4359 , 50.77 )
( 4360 , 50.74 )
( 4361 , 50.78 )
( 4362 , 50.75 )
( 4363 , 50.82 )
( 4364 , 50.88 )
( 4365 , 50.98 )
( 4366 , 51.11 )
( 4367 , 51.19 )
( 4368 , 51.15 )
( 4369 , 51.11 )
( 4370 , 51.06 )
( 4371 , 51.07 )
( 4372 , 50.96 )
( 4373 , 50.84 )
( 4374 , 50.75 )
( 4375 , 50.62 )
( 4376 , 50.88 )
( 4377 , 51.20 )
( 4378 , 51.42 )
( 4379 , 51.66 )
( 4380 , 51.91 )
( 4381 , 52.08 )
( 4382 , 52.28 )
( 4383 , 52.41 )
( 4384 , 52.64 )
( 4385 , 52.83 )
( 4386 , 53.14 )
( 4387 , 53.43 )
( 4388 , 53.81 )
( 4389 , 54.17 )
( 4390 , 54.56 )
( 4391 , 54.93 )
( 4392 , 55.29 )
( 4393 , 55.20 )
( 4394 , 55.08 )
( 4395 , 55.20 )
( 4396 , 55.39 )
( 4397 , 55.65 )
( 4398 , 55.81 )
( 4399 , 55.77 )
( 4400 , 55.80 )
( 4401 , 55.85 )
( 4402 , 55.80 )
( 4403 , 55.69 )
( 4404 , 55.56 )
( 4405 , 55.45 )
( 4406 , 55.38 )
( 4407 , 55.29 )
( 4408 , 55.29 )
( 4409 , 55.33 )
( 4410 , 55.43 )
( 4411 , 55.52 )
( 4412 , 55.55 )
( 4413 , 55.60 )
( 4414 , 55.67 )
( 4415 , 55.71 )
( 4416 , 55.60 )
( 4417 , 55.48 )
( 4418 , 55.36 )
( 4419 , 55.23 )
( 4420 , 55.11 )
( 4421 , 54.98 )
( 4422 , 54.86 )
( 4423 , 54.79 )
( 4424 , 54.73 )
( 4425 , 54.93 )
( 4426 , 55.05 )
( 4427 , 55.18 )
( 4428 , 55.43 )
( 4429 , 55.69 )
( 4430 , 55.99 )
( 4431 , 56.25 )
( 4432 , 56.50 )
( 4433 , 56.63 )
( 4434 , 56.75 )
( 4435 , 56.93 )
( 4436 , 57.06 )
( 4437 , 57.19 )
( 4438 , 57.28 )
( 4439 , 57.38 )
( 4440 , 57.53 )
( 4441 , 57.63 )
( 4442 , 57.73 )
( 4443 , 57.78 )
( 4444 , 57.67 )
( 4445 , 57.62 )
( 4446 , 57.53 )
( 4447 , 57.42 )
( 4448 , 57.50 )
( 4449 , 57.64 )
( 4450 , 57.73 )
( 4451 , 57.66 )
( 4452 , 57.78 )
( 4453 , 57.75 )
( 4454 , 57.64 )
( 4455 , 57.52 )
( 4456 , 57.64 )
( 4457 , 57.95 )
( 4458 , 58.08 )
( 4459 , 58.21 )
( 4460 , 58.34 )
( 4461 , 58.52 )
( 4462 , 58.74 )
( 4463 , 58.92 )
( 4464 , 59.11 )
( 4465 , 59.02 )
( 4466 , 58.95 )
( 4467 , 58.82 )
( 4468 , 58.92 )
( 4469 , 59.04 )
( 4470 , 59.13 )
( 4471 , 59.23 )
( 4472 , 59.33 )
( 4473 , 59.43 )
( 4474 , 59.55 )
( 4475 , 59.67 )
( 4476 , 59.81 )
( 4477 , 59.94 )
( 4478 , 60.06 )
( 4479 , 60.21 )
( 4480 , 60.18 )
( 4481 , 60.24 )
( 4482 , 60.23 )
( 4483 , 60.59 )
( 4484 , 60.94 )
( 4485 , 61.44 )
( 4486 , 61.72 )
( 4487 , 61.71 )
( 4488 , 61.72 )
( 4489 , 61.75 )
( 4490 , 61.74 )
( 4491 , 61.81 )
( 4492 , 61.84 )
( 4493 , 61.86 )
( 4494 , 62.00 )
( 4495 , 62.17 )
( 4496 , 62.38 )
( 4497 , 62.52 )
( 4498 , 62.73 )
( 4499 , 62.98 )
( 4500 , 63.20 )
( 4501 , 63.41 )
( 4502 , 63.46 )
( 4503 , 63.50 )
( 4504 , 63.62 )
( 4505 , 63.50 )
( 4506 , 63.38 )
( 4507 , 63.27 )
( 4508 , 63.19 )
( 4509 , 63.12 )
( 4510 , 63.39 )
( 4511 , 63.62 )
( 4512 , 63.88 )
( 4513 , 64.20 )
( 4514 , 64.49 )
( 4515 , 64.75 )
( 4516 , 65.01 )
( 4517 , 65.20 )
( 4518 , 65.38 )
( 4519 , 65.63 )
( 4520 , 65.76 )
( 4521 , 65.88 )
( 4522 , 66.09 )
( 4523 , 66.27 )
( 4524 , 66.46 )
( 4525 , 66.65 )
( 4526 , 66.83 )
( 4527 , 67.05 )
( 4528 , 67.18 )
( 4529 , 67.34 )
( 4530 , 67.47 )
( 4531 , 67.61 )
( 4532 , 67.78 )
( 4533 , 67.91 )
( 4534 , 68.04 )
( 4535 , 68.16 )
( 4536 , 68.29 )
( 4537 , 68.41 )
( 4538 , 68.30 )
( 4539 , 68.17 )
( 4540 , 68.05 )
( 4541 , 67.92 )
( 4542 , 67.88 )
( 4543 , 67.88 )
( 4544 , 67.75 )
( 4545 , 67.80 )
( 4546 , 67.84 )
( 4547 , 67.89 )
( 4548 , 67.77 )
( 4549 , 67.81 )
( 4550 , 67.69 )
( 4551 , 67.62 )
( 4552 , 67.50 )
( 4553 , 67.45 )
( 4554 , 67.33 )
( 4555 , 67.24 )
( 4556 , 67.16 )
( 4557 , 67.13 )
( 4558 , 67.09 )
( 4559 , 67.05 )
( 4560 , 67.08 )
( 4561 , 67.04 )
( 4562 , 67.03 )
( 4563 , 66.93 )
( 4564 , 66.88 )
( 4565 , 66.78 )
( 4566 , 66.67 )
( 4567 , 66.55 )
( 4568 , 66.59 )
( 4569 , 66.48 )
( 4570 , 66.35 )
( 4571 , 66.23 )
( 4572 , 66.12 )
( 4573 , 66.07 )
( 4574 , 65.95 )
( 4575 , 65.89 )
( 4576 , 65.84 )
( 4577 , 65.78 )
( 4578 , 65.73 )
( 4579 , 65.80 )
( 4580 , 65.92 )
( 4581 , 65.86 )
( 4582 , 65.85 )
( 4583 , 65.79 )
( 4584 , 65.82 )
( 4585 , 65.81 )
( 4586 , 65.81 )
( 4587 , 65.84 )
( 4588 , 65.84 )
( 4589 , 65.85 )
( 4590 , 65.89 )
( 4591 , 65.89 )
( 4592 , 65.89 )
( 4593 , 65.88 )
( 4594 , 65.88 )
( 4595 , 65.87 )
( 4596 , 65.90 )
( 4597 , 65.91 )
( 4598 , 65.91 )
( 4599 , 65.91 )
( 4600 , 65.88 )
( 4601 , 65.85 )
( 4602 , 65.95 )
( 4603 , 66.06 )
( 4604 , 66.16 )
( 4605 , 66.13 )
( 4606 , 66.08 )
( 4607 , 66.04 )
( 4608 , 65.98 )
( 4609 , 66.02 )
( 4610 , 66.06 )
( 4611 , 66.05 )
( 4612 , 66.13 )
( 4613 , 66.20 )
( 4614 , 66.24 )
( 4615 , 66.26 )
( 4616 , 66.20 )
( 4617 , 66.31 )
( 4618 , 66.43 )
( 4619 , 66.59 )
( 4620 , 66.70 )
( 4621 , 66.82 )
( 4622 , 66.91 )
( 4623 , 66.98 )
( 4624 , 66.91 )
( 4625 , 66.91 )
( 4626 , 66.89 )
( 4627 , 66.87 )
( 4628 , 66.88 )
( 4629 , 66.97 )
( 4630 , 67.05 )
( 4631 , 67.16 )
( 4632 , 67.17 )
( 4633 , 67.15 )
( 4634 , 67.31 )
( 4635 , 67.29 )
( 4636 , 67.27 )
( 4637 , 67.24 )
( 4638 , 67.06 )
( 4639 , 66.77 )
( 4640 , 66.62 )
( 4641 , 66.48 )
( 4642 , 66.27 )
( 4643 , 65.96 )
( 4644 , 65.71 )
( 4645 , 65.60 )
( 4646 , 65.53 )
( 4647 , 65.31 )
( 4648 , 65.03 )
( 4649 , 64.74 )
( 4650 , 64.45 )
( 4651 , 64.38 )
( 4652 , 64.09 )
( 4653 , 63.94 )
( 4654 , 63.64 )
( 4655 , 63.34 )
( 4656 , 63.04 )
( 4657 , 62.75 )
( 4658 , 62.46 )
( 4659 , 62.16 )
( 4660 , 62.01 )
( 4661 , 61.95 )
( 4662 , 61.76 )
( 4663 , 61.50 )
( 4664 , 61.21 )
( 4665 , 61.15 )
( 4666 , 61.19 )
( 4667 , 61.09 )
( 4668 , 60.80 )
( 4669 , 60.51 )
( 4670 , 60.27 )
( 4671 , 60.02 )
( 4672 , 59.75 )
( 4673 , 59.45 )
( 4674 , 59.16 )
( 4675 , 58.88 )
( 4676 , 58.62 )
( 4677 , 58.36 )
( 4678 , 58.05 )
( 4679 , 57.75 )
( 4680 , 57.45 )
( 4681 , 57.15 )
( 4682 , 56.96 )
( 4683 , 56.87 )
( 4684 , 56.73 )
( 4685 , 56.58 )
( 4686 , 56.28 )
( 4687 , 56.20 )
( 4688 , 56.06 )
( 4689 , 55.76 )
( 4690 , 55.80 )
( 4691 , 55.82 )
( 4692 , 55.75 )
( 4693 , 55.74 )
( 4694 , 55.59 )
( 4695 , 55.31 )
( 4696 , 55.01 )
( 4697 , 54.71 )
( 4698 , 54.61 )
( 4699 , 54.51 )
( 4700 , 54.42 )
( 4701 , 54.12 )
( 4702 , 53.82 )
( 4703 , 53.57 )
( 4704 , 53.31 )
( 4705 , 53.09 )
( 4706 , 52.86 )
( 4707 , 52.84 )
( 4708 , 52.75 )
( 4709 , 52.62 )
( 4710 , 52.32 )
( 4711 , 52.02 )
( 4712 , 51.72 )
( 4713 , 51.52 )
( 4714 , 51.22 )
( 4715 , 50.94 )
( 4716 , 50.64 )
( 4717 , 50.34 )
( 4718 , 50.04 )
( 4719 , 49.76 )
( 4720 , 49.47 )
( 4721 , 49.17 )
( 4722 , 49.11 )
( 4723 , 49.06 )
( 4724 , 49.00 )
( 4725 , 49.05 )
( 4726 , 49.07 )
( 4727 , 48.98 )
( 4728 , 48.68 )
( 4729 , 48.44 )
( 4730 , 48.14 )
( 4731 , 47.91 )
( 4732 , 47.80 )
( 4733 , 47.52 )
( 4734 , 47.33 )
( 4735 , 47.16 )
( 4736 , 47.15 )
( 4737 , 47.02 )
( 4738 , 46.97 )
( 4739 , 46.81 )
( 4740 , 46.55 )
( 4741 , 46.44 )
( 4742 , 46.35 )
( 4743 , 46.21 )
( 4744 , 46.00 )
( 4745 , 45.71 )
( 4746 , 45.41 )
( 4747 , 45.34 )
( 4748 , 45.26 )
( 4749 , 44.97 )
( 4750 , 44.67 )
( 4751 , 44.37 )
( 4752 , 44.07 )
( 4753 , 43.93 )
( 4754 , 43.83 )
( 4755 , 43.53 )
( 4756 , 43.29 )
( 4757 , 43.09 )
( 4758 , 43.00 )
( 4759 , 42.79 )
( 4760 , 42.55 )
( 4761 , 42.35 )
( 4762 , 42.05 )
( 4763 , 41.77 )
( 4764 , 41.50 )
( 4765 , 41.24 )
( 4766 , 41.02 )
( 4767 , 40.74 )
( 4768 , 40.68 )
( 4769 , 40.39 )
( 4770 , 40.10 )
( 4771 , 39.96 )
( 4772 , 39.66 )
( 4773 , 39.36 )
( 4774 , 39.06 )
( 4775 , 38.80 )
( 4776 , 38.71 )
( 4777 , 38.64 )
( 4778 , 38.55 )
( 4779 , 38.46 )
( 4780 , 38.36 )
( 4781 , 38.26 )
( 4782 , 38.22 )
( 4783 , 38.15 )
( 4784 , 38.14 )
( 4785 , 37.84 )
( 4786 , 37.54 )
( 4787 , 37.51 )
( 4788 , 37.48 )
( 4789 , 37.40 )
( 4790 , 37.50 )
( 4791 , 37.56 )
( 4792 , 37.43 )
( 4793 , 37.48 )
( 4794 , 37.35 )
( 4795 , 37.34 )
( 4796 , 37.24 )
( 4797 , 36.94 )
( 4798 , 36.64 )
( 4799 , 36.35 )
( 4800 , 36.25 )
( 4801 , 36.17 )
( 4802 , 35.88 )
( 4803 , 35.66 )
( 4804 , 35.39 )
( 4805 , 35.12 )
( 4806 , 34.83 )
( 4807 , 34.56 )
( 4808 , 34.46 )
( 4809 , 34.21 )
( 4810 , 33.92 )
( 4811 , 33.65 )
( 4812 , 33.35 )
( 4813 , 33.05 )
( 4814 , 32.75 )
( 4815 , 32.45 )
( 4816 , 32.48 )
( 4817 , 32.47 )
( 4818 , 32.45 )
( 4819 , 32.20 )
( 4820 , 31.90 )
( 4821 , 31.62 )
( 4822 , 31.39 )
( 4823 , 31.10 )
( 4824 , 30.88 )
( 4825 , 30.73 )
( 4826 , 30.71 )
( 4827 , 30.60 )
( 4828 , 30.40 )
( 4829 , 30.10 )
( 4830 , 29.80 )
( 4831 , 29.73 )
( 4832 , 29.43 )
( 4833 , 29.41 )
( 4834 , 29.44 )
( 4835 , 29.49 )
( 4836 , 29.23 )
( 4837 , 29.05 )
( 4838 , 28.97 )
( 4839 , 28.88 )
( 4840 , 28.57 )
( 4841 , 28.29 )
( 4842 , 28.22 )
( 4843 , 28.12 )
( 4844 , 28.10 )
( 4845 , 28.20 )
( 4846 , 28.07 )
( 4847 , 27.77 )
( 4848 , 27.84 )
( 4849 , 27.79 )
( 4850 , 27.83 )
( 4851 , 27.80 )
( 4852 , 28.00 )
( 4853 , 27.98 )
( 4854 , 27.68 )
( 4855 , 27.38 )
( 4856 , 27.35 )
( 4857 , 27.06 )
( 4858 , 26.76 )
( 4859 , 26.46 )
( 4860 , 26.17 )
( 4861 , 25.87 )
( 4862 , 25.64 )
( 4863 , 25.34 )
( 4864 , 25.35 )
( 4865 , 25.28 )
( 4866 , 25.19 )
( 4867 , 25.12 )
( 4868 , 24.93 )
( 4869 , 24.66 )
( 4870 , 24.36 )
( 4871 , 24.27 )
( 4872 , 24.17 )
( 4873 , 23.88 )
( 4874 , 23.83 )
( 4875 , 23.85 )
( 4876 , 23.72 )
( 4877 , 23.43 )
( 4878 , 23.14 )
( 4879 , 23.09 )
( 4880 , 22.89 )
( 4881 , 22.60 )
( 4882 , 22.36 )
( 4883 , 22.06 )
( 4884 , 21.76 )
( 4885 , 21.46 )
( 4886 , 21.16 )
( 4887 , 20.98 )
( 4888 , 20.70 )
( 4889 , 20.44 )
( 4890 , 20.14 )
( 4891 , 19.84 )
( 4892 , 19.54 )
( 4893 , 19.24 )
( 4894 , 19.30 )
( 4895 , 19.25 )
( 4896 , 19.17 )
( 4897 , 19.23 )
( 4898 , 19.15 )
( 4899 , 19.07 )
( 4900 , 18.97 )
( 4901 , 18.94 )
( 4902 , 18.79 )
( 4903 , 18.53 )
( 4904 , 18.23 )
( 4905 , 17.95 )
( 4906 , 17.83 )
( 4907 , 17.53 )
( 4908 , 17.28 )
( 4909 , 17.16 )
( 4910 , 17.11 )
( 4911 , 17.20 )
( 4912 , 17.07 )
( 4913 , 16.78 )
( 4914 , 16.48 )
( 4915 , 16.22 )
( 4916 , 15.92 )
( 4917 , 15.62 )
( 4918 , 15.42 )
( 4919 , 15.13 )
( 4920 , 14.83 )
( 4921 , 14.54 )
( 4922 , 14.24 )
( 4923 , 13.96 )
( 4924 , 13.86 )
( 4925 , 13.93 )
( 4926 , 13.84 )
( 4927 , 13.65 )
( 4928 , 13.48 )
( 4929 , 13.34 )
( 4930 , 13.30 )
( 4931 , 13.00 )
( 4932 , 13.26 )
( 4933 , 13.45 )
( 4934 , 13.59 )
( 4935 , 13.69 )
( 4936 , 13.79 )
( 4937 , 13.79 )
( 4938 , 13.79 )
( 4939 , 13.79 )
( 4940 , 13.84 )
( 4941 , 13.94 )
( 4942 , 14.09 )
( 4943 , 14.33 )
( 4944 , 14.33 )
( 4945 , 14.33 )
( 4946 , 14.33 )
( 4947 , 14.36 )
( 4948 , 14.36 )
( 4949 , 14.51 )
( 4950 , 14.51 )
( 4951 , 14.81 )
( 4952 , 15.00 )
( 4953 , 15.00 )
( 4954 , 15.01 )
( 4955 , 15.02 )
( 4956 , 15.02 )
( 4957 , 15.05 )
( 4958 , 15.07 )
( 4959 , 15.22 )
( 4960 , 15.23 )
( 4961 , 15.34 )
( 4962 , 15.39 )
( 4963 , 15.39 )
( 4964 , 15.52 )
( 4965 , 15.63 )
( 4966 , 15.69 )
( 4967 , 15.71 )
( 4968 , 15.71 )
( 4969 , 15.71 )
( 4970 , 16.07 )
( 4971 , 16.42 )
( 4972 , 16.72 )
( 4973 , 17.10 )
( 4974 , 17.57 )
( 4975 , 17.87 )
( 4976 , 18.28 )
( 4977 , 18.71 )
( 4978 , 18.99 )
( 4979 , 19.21 )
( 4980 , 19.32 )
( 4981 , 19.32 )
( 4982 , 19.32 )
( 4983 , 19.40 )
( 4984 , 19.40 )
( 4985 , 19.41 )
( 4986 , 19.51 )
( 4987 , 19.57 )
( 4988 , 19.63 )
( 4989 , 19.63 )
( 4990 , 19.63 )
( 4991 , 19.71 )
( 4992 , 19.82 )
( 4993 , 19.84 )
( 4994 , 19.84 )
( 4995 , 19.84 )
( 4996 , 20.28 )
( 4997 , 20.65 )
( 4998 , 21.09 )
( 4999 , 21.58 )
( 5000 , 21.97 )
( 5001 , 22.38 )
( 5002 , 22.81 )
( 5003 , 23.12 )
( 5004 , 23.40 )
( 5005 , 23.43 )
( 5006 , 23.43 )
( 5007 , 23.49 )
( 5008 , 23.53 )
( 5009 , 23.60 )
( 5010 , 23.67 )
( 5011 , 23.67 )
( 5012 , 23.75 )
( 5013 , 23.97 )
( 5014 , 24.18 )
( 5015 , 24.33 )
( 5016 , 24.34 )
( 5017 , 24.34 )
( 5018 , 24.47 )
( 5019 , 24.62 )
( 5020 , 24.87 )
( 5021 , 25.12 )
( 5022 , 25.26 )
( 5023 , 25.41 )
( 5024 , 25.56 )
( 5025 , 25.56 )
( 5026 , 25.76 )
( 5027 , 25.91 )
( 5028 , 26.06 )
( 5029 , 26.20 )
( 5030 , 26.38 )
( 5031 , 26.38 )
( 5032 , 26.53 )
( 5033 , 26.65 )
( 5034 , 26.77 )
( 5035 , 26.99 )
( 5036 , 27.21 )
( 5037 , 27.43 )
( 5038 , 27.78 )
( 5039 , 28.04 )
( 5040 , 28.33 )
( 5041 , 28.61 )
( 5042 , 28.83 )
( 5043 , 28.94 )
( 5044 , 28.99 )
( 5045 , 29.08 )
( 5046 , 29.13 )
( 5047 , 29.18 )
( 5048 , 29.33 )
( 5049 , 29.34 )
( 5050 , 29.58 )
( 5051 , 29.76 )
( 5052 , 29.87 )
( 5053 , 29.98 )
( 5054 , 30.05 )
( 5055 , 30.22 )
( 5056 , 30.37 )
( 5057 , 30.53 )
( 5058 , 30.56 )
( 5059 , 30.62 )
( 5060 , 30.69 )
( 5061 , 30.71 )
( 5062 , 30.71 )
( 5063 , 30.78 )
( 5064 , 30.78 )
( 5065 , 30.83 )
( 5066 , 30.88 )
( 5067 , 30.88 )
( 5068 , 30.90 )
( 5069 , 30.97 )
( 5070 , 30.98 )
( 5071 , 30.97 )
( 5072 , 31.02 )
( 5073 , 31.02 )
( 5074 , 30.93 )
( 5075 , 30.83 )
( 5076 , 30.77 )
( 5077 , 30.67 )
( 5078 , 30.66 )
( 5079 , 30.72 )
( 5080 , 30.74 )
( 5081 , 30.61 )
( 5082 , 30.31 )
( 5083 , 30.17 )
( 5084 , 29.87 )
( 5085 , 29.57 )
( 5086 , 29.52 )
( 5087 , 29.33 )
( 5088 , 29.03 )
( 5089 , 28.84 )
( 5090 , 28.64 )
( 5091 , 28.49 )
( 5092 , 28.35 )
( 5093 , 28.20 )
( 5094 , 28.17 )
( 5095 , 27.90 )
( 5096 , 27.67 )
( 5097 , 27.53 )
( 5098 , 27.29 )
( 5099 , 27.00 )
( 5100 , 26.79 )
( 5101 , 26.52 )
( 5102 , 26.24 )
( 5103 , 25.94 )
( 5104 , 25.79 )
( 5105 , 25.56 )
( 5106 , 25.41 )
( 5107 , 25.44 )
( 5108 , 25.50 )
( 5109 , 25.38 )
( 5110 , 25.28 )
( 5111 , 25.02 )
( 5112 , 24.82 )
( 5113 , 24.52 )
( 5114 , 24.46 )
( 5115 , 24.42 )
( 5116 , 24.50 )
( 5117 , 24.44 )
( 5118 , 24.14 )
( 5119 , 23.88 )
( 5120 , 23.60 )
( 5121 , 23.46 )
( 5122 , 23.21 )
( 5123 , 22.91 )
( 5124 , 22.94 )
( 5125 , 22.95 )
( 5126 , 22.94 )
( 5127 , 22.93 )
( 5128 , 22.97 )
( 5129 , 23.02 )
( 5130 , 22.90 )
( 5131 , 22.78 )
( 5132 , 22.65 )
( 5133 , 22.35 )
( 5134 , 22.05 )
( 5135 , 21.85 )
( 5136 , 21.66 )
( 5137 , 21.47 )
( 5138 , 21.34 )
( 5139 , 21.35 )
( 5140 , 21.27 )
( 5141 , 20.97 )
( 5142 , 20.88 )
( 5143 , 20.83 )
( 5144 , 20.69 )
( 5145 , 20.40 )
( 5146 , 20.10 )
( 5147 , 20.14 )
( 5148 , 20.06 )
( 5149 , 19.94 )
( 5150 , 19.81 )
( 5151 , 19.69 )
( 5152 , 19.64 )
( 5153 , 19.51 )
( 5154 , 19.53 )
( 5155 , 19.55 )
( 5156 , 19.52 )
( 5157 , 19.58 )
( 5158 , 19.60 )
( 5159 , 19.82 )
( 5160 , 19.82 )
( 5161 , 20.04 )
( 5162 , 20.27 )
( 5163 , 20.49 )
( 5164 , 20.79 )
( 5165 , 21.02 )
( 5166 , 21.29 )
( 5167 , 21.58 )
( 5168 , 21.82 )
( 5169 , 22.04 )
( 5170 , 22.19 )
( 5171 , 22.21 )
( 5172 , 22.21 )
( 5173 , 22.62 )
( 5174 , 23.03 )
( 5175 , 23.38 )
( 5176 , 23.73 )
( 5177 , 24.18 )
( 5178 , 24.56 )
( 5179 , 24.93 )
( 5180 , 25.32 )
( 5181 , 25.77 )
( 5182 , 26.22 )
( 5183 , 26.67 )
( 5184 , 27.02 )
( 5185 , 27.38 )
( 5186 , 27.72 )
( 5187 , 28.07 )
( 5188 , 28.42 )
( 5189 , 28.69 )
( 5190 , 29.04 )
( 5191 , 29.29 )
( 5192 , 29.57 )
( 5193 , 29.85 )
( 5194 , 30.07 )
( 5195 , 30.43 )
( 5196 , 30.80 )
( 5197 , 31.14 )
( 5198 , 31.37 )
( 5199 , 31.66 )
( 5200 , 32.00 )
( 5201 , 32.22 )
( 5202 , 32.44 )
( 5203 , 32.79 )
( 5204 , 33.14 )
( 5205 , 33.41 )
( 5206 , 33.42 )
( 5207 , 33.42 )
( 5208 , 33.43 )
( 5209 , 33.54 )
( 5210 , 33.64 )
( 5211 , 33.79 )
( 5212 , 34.01 )
( 5213 , 34.14 )
( 5214 , 34.27 )
( 5215 , 34.41 )
( 5216 , 34.38 )
( 5217 , 34.32 )
( 5218 , 34.37 )
( 5219 , 34.51 )
( 5220 , 34.60 )
( 5221 , 34.68 )
( 5222 , 34.91 )
( 5223 , 35.10 )
( 5224 , 35.08 )
( 5225 , 35.08 )
( 5226 , 35.17 )
( 5227 , 35.17 )
( 5228 , 35.30 )
( 5229 , 35.48 )
( 5230 , 35.61 )
( 5231 , 35.54 )
( 5232 , 35.43 )
( 5233 , 35.60 )
( 5234 , 35.64 )
( 5235 , 35.52 )
( 5236 , 35.73 )
( 5237 , 35.94 )
( 5238 , 36.06 )
( 5239 , 35.94 )
( 5240 , 35.81 )
( 5241 , 36.00 )
( 5242 , 36.12 )
( 5243 , 36.25 )
( 5244 , 36.38 )
( 5245 , 36.59 )
( 5246 , 36.79 )
( 5247 , 36.92 )
( 5248 , 36.79 )
( 5249 , 36.70 )
( 5250 , 36.59 )
( 5251 , 36.48 )
( 5252 , 36.41 )
( 5253 , 36.44 )
( 5254 , 36.52 )
( 5255 , 36.61 )
( 5256 , 36.69 )
( 5257 , 36.73 )
( 5258 , 36.65 )
( 5259 , 36.52 )
( 5260 , 36.57 )
( 5261 , 36.67 )
( 5262 , 36.55 )
( 5263 , 36.43 )
( 5264 , 36.31 )
( 5265 , 36.18 )
( 5266 , 36.09 )
( 5267 , 36.10 )
( 5268 , 35.98 )
( 5269 , 35.89 )
( 5270 , 35.76 )
( 5271 , 36.09 )
( 5272 , 36.30 )
( 5273 , 36.54 )
( 5274 , 36.74 )
( 5275 , 36.93 )
( 5276 , 36.81 )
( 5277 , 36.73 )
( 5278 , 36.62 )
( 5279 , 36.59 )
( 5280 , 36.55 )
( 5281 , 36.50 )
( 5282 , 36.57 )
( 5283 , 36.27 )
( 5284 , 36.12 )
( 5285 , 36.07 )
( 5286 , 35.93 )
( 5287 , 35.62 )
( 5288 , 35.35 )
( 5289 , 35.36 )
( 5290 , 35.45 )
( 5291 , 35.37 )
( 5292 , 35.09 )
( 5293 , 34.79 )
( 5294 , 34.64 )
( 5295 , 34.34 )
( 5296 , 34.04 )
( 5297 , 33.75 )
( 5298 , 33.45 )
( 5299 , 33.16 )
( 5300 , 32.97 )
( 5301 , 32.75 )
( 5302 , 32.52 )
( 5303 , 32.21 )
( 5304 , 31.91 )
( 5305 , 31.61 )
( 5306 , 31.31 )
( 5307 , 31.17 )
( 5308 , 31.06 )
( 5309 , 30.91 )
( 5310 , 30.77 )
( 5311 , 30.47 )
( 5312 , 30.38 )
( 5313 , 30.09 )
( 5314 , 29.79 )
( 5315 , 29.49 )
( 5316 , 29.24 )
( 5317 , 28.95 )
( 5318 , 28.74 )
( 5319 , 28.49 )
( 5320 , 28.19 )
( 5321 , 28.07 )
( 5322 , 27.97 )
( 5323 , 27.86 )
( 5324 , 28.04 )
( 5325 , 28.24 )
( 5326 , 28.45 )
( 5327 , 28.64 )
( 5328 , 29.02 )
( 5329 , 29.28 )
( 5330 , 29.54 )
( 5331 , 29.93 )
( 5332 , 30.32 )
( 5333 , 30.68 )
( 5334 , 30.88 )
( 5335 , 31.10 )
( 5336 , 31.30 )
( 5337 , 31.57 )
( 5338 , 31.77 )
( 5339 , 31.97 )
( 5340 , 32.22 )
( 5341 , 32.44 )
( 5342 , 32.62 )
( 5343 , 32.74 )
( 5344 , 32.87 )
( 5345 , 32.84 )
( 5346 , 32.81 )
( 5347 , 33.24 )
( 5348 , 33.64 )
( 5349 , 34.04 )
( 5350 , 34.44 )
( 5351 , 34.87 )
( 5352 , 35.27 )
( 5353 , 35.66 )
( 5354 , 36.12 )
( 5355 , 36.55 )
( 5356 , 36.95 )
( 5357 , 37.40 )
( 5358 , 37.83 )
( 5359 , 38.25 )
( 5360 , 38.68 )
( 5361 , 39.18 )
( 5362 , 39.69 )
( 5363 , 40.11 )
( 5364 , 40.54 )
( 5365 , 40.98 )
( 5366 , 41.43 )
( 5367 , 41.88 )
( 5368 , 42.33 )
( 5369 , 42.77 )
( 5370 , 43.18 )
( 5371 , 43.48 )
( 5372 , 43.78 )
( 5373 , 44.08 )
( 5374 , 44.33 )
( 5375 , 44.55 )
( 5376 , 44.82 )
( 5377 , 45.14 )
( 5378 , 45.49 )
( 5379 , 45.80 )
( 5380 , 46.12 )
( 5381 , 46.43 )
( 5382 , 46.39 )
( 5383 , 46.39 )
( 5384 , 46.48 )
( 5385 , 46.36 )
( 5386 , 46.27 )
( 5387 , 46.19 )
( 5388 , 46.06 )
( 5389 , 45.95 )
( 5390 , 45.84 )
( 5391 , 45.88 )
( 5392 , 45.93 )
( 5393 , 46.02 )
( 5394 , 46.09 )
( 5395 , 45.97 )
( 5396 , 45.84 )
( 5397 , 45.80 )
( 5398 , 45.68 )
( 5399 , 45.83 )
( 5400 , 46.00 )
( 5401 , 46.04 )
( 5402 , 46.21 )
( 5403 , 46.33 )
( 5404 , 46.43 )
( 5405 , 46.53 )
( 5406 , 46.62 )
( 5407 , 46.70 )
( 5408 , 46.57 )
( 5409 , 46.46 )
( 5410 , 46.39 )
( 5411 , 46.27 )
( 5412 , 46.21 )
( 5413 , 46.16 )
( 5414 , 46.12 )
( 5415 , 46.20 )
( 5416 , 46.20 )
( 5417 , 46.16 )
( 5418 , 46.14 )
( 5419 , 46.14 )
( 5420 , 46.10 )
( 5421 , 46.06 )
( 5422 , 46.00 )
( 5423 , 45.94 )
( 5424 , 45.93 )
( 5425 , 45.88 )
( 5426 , 45.98 )
( 5427 , 45.92 )
( 5428 , 45.87 )
( 5429 , 45.82 )
( 5430 , 45.77 )
( 5431 , 45.71 )
( 5432 , 45.66 )
( 5433 , 45.60 )
( 5434 , 45.61 )
( 5435 , 45.62 )
( 5436 , 45.61 )
( 5437 , 45.59 )
( 5438 , 45.54 )
( 5439 , 45.56 )
( 5440 , 45.55 )
( 5441 , 45.56 )
( 5442 , 45.59 )
( 5443 , 45.60 )
( 5444 , 45.73 )
( 5445 , 45.86 )
( 5446 , 45.98 )
( 5447 , 46.18 )
( 5448 , 46.34 )
( 5449 , 46.50 )
( 5450 , 46.45 )
( 5451 , 46.43 )
( 5452 , 46.38 )
( 5453 , 46.33 )
( 5454 , 46.28 )
( 5455 , 46.22 )
( 5456 , 46.21 )
( 5457 , 46.17 )
( 5458 , 46.12 )
( 5459 , 46.07 )
( 5460 , 46.01 )
( 5461 , 45.71 )
( 5462 , 45.57 )
( 5463 , 45.27 )
( 5464 , 44.98 )
( 5465 , 44.73 )
( 5466 , 44.43 )
( 5467 , 44.18 )
( 5468 , 43.99 )
( 5469 , 43.69 )
( 5470 , 43.39 )
( 5471 , 43.09 )
( 5472 , 42.81 )
( 5473 , 42.57 )
( 5474 , 42.27 )
( 5475 , 42.32 )
( 5476 , 42.41 )
( 5477 , 42.50 )
( 5478 , 42.38 )
( 5479 , 42.23 )
( 5480 , 42.05 )
( 5481 , 41.85 )
( 5482 , 41.55 )
( 5483 , 41.25 )
( 5484 , 40.95 )
( 5485 , 40.90 )
( 5486 , 40.81 )
( 5487 , 40.73 )
( 5488 , 40.52 )
( 5489 , 40.22 )
( 5490 , 39.92 )
( 5491 , 39.63 )
( 5492 , 39.34 )
( 5493 , 39.04 )
( 5494 , 38.86 )
( 5495 , 38.62 )
( 5496 , 38.33 )
( 5497 , 38.04 )
( 5498 , 37.75 )
( 5499 , 37.46 )
( 5500 , 37.47 )
( 5501 , 37.23 )
( 5502 , 36.93 )
( 5503 , 36.63 )
( 5504 , 36.33 )
( 5505 , 36.15 )
( 5506 , 35.91 )
( 5507 , 35.64 )
( 5508 , 35.55 )
( 5509 , 35.25 )
( 5510 , 35.04 )
( 5511 , 34.77 )
( 5512 , 34.76 )
( 5513 , 34.53 )
( 5514 , 34.23 )
( 5515 , 34.30 )
( 5516 , 34.06 )
( 5517 , 33.76 )
( 5518 , 33.88 )
( 5519 , 33.92 )
( 5520 , 34.08 )
( 5521 , 34.25 )
( 5522 , 34.44 )
( 5523 , 34.65 )
( 5524 , 34.79 )
( 5525 , 34.87 )
( 5526 , 34.91 )
( 5527 , 34.93 )
( 5528 , 34.93 )
( 5529 , 34.94 )
( 5530 , 34.95 )
( 5531 , 34.97 )
( 5532 , 34.97 )
( 5533 , 34.99 )
( 5534 , 35.06 )
( 5535 , 35.07 )
( 5536 , 35.07 )
( 5537 , 35.13 )
( 5538 , 35.13 )
( 5539 , 35.42 )
( 5540 , 35.71 )
( 5541 , 35.99 )
( 5542 , 36.27 )
( 5543 , 36.60 )
( 5544 , 36.89 )
( 5545 , 37.12 )
( 5546 , 37.34 )
( 5547 , 37.61 )
( 5548 , 37.91 )
( 5549 , 38.21 )
( 5550 , 38.49 )
( 5551 , 38.76 )
( 5552 , 39.07 )
( 5553 , 39.30 )
( 5554 , 39.54 )
( 5555 , 39.77 )
( 5556 , 40.11 )
( 5557 , 40.45 )
( 5558 , 40.80 )
( 5559 , 41.16 )
( 5560 , 41.39 )
( 5561 , 41.69 )
( 5562 , 41.69 )
( 5563 , 41.72 )
( 5564 , 41.72 )
( 5565 , 41.73 )
( 5566 , 41.73 )
( 5567 , 41.85 )
( 5568 , 41.85 )
( 5569 , 41.88 )
( 5570 , 41.88 )
( 5571 , 41.98 )
( 5572 , 42.01 )
( 5573 , 42.16 )
( 5574 , 42.30 )
( 5575 , 42.49 )
( 5576 , 42.55 )
( 5577 , 42.63 )
( 5578 , 42.63 )
( 5579 , 42.67 )
( 5580 , 42.71 )
( 5581 , 42.76 )
( 5582 , 42.84 )
( 5583 , 42.84 )
( 5584 , 42.85 )
( 5585 , 42.85 )
( 5586 , 43.21 )
( 5587 , 43.63 )
( 5588 , 44.04 )
( 5589 , 44.47 )
( 5590 , 44.82 )
( 5591 , 45.16 )
( 5592 , 45.51 )
( 5593 , 45.87 )
( 5594 , 46.27 )
( 5595 , 46.75 )
( 5596 , 47.08 )
( 5597 , 47.37 )
( 5598 , 47.64 )
( 5599 , 47.93 )
( 5600 , 48.15 )
( 5601 , 48.54 )
( 5602 , 48.89 )
( 5603 , 49.23 )
( 5604 , 49.51 )
( 5605 , 49.79 )
( 5606 , 50.07 )
( 5607 , 50.07 )
( 5608 , 50.12 )
( 5609 , 50.12 )
( 5610 , 50.19 )
( 5611 , 50.27 )
( 5612 , 50.38 )
( 5613 , 50.46 )
( 5614 , 50.46 )
( 5615 , 50.64 )
( 5616 , 50.79 )
( 5617 , 50.95 )
( 5618 , 51.13 )
( 5619 , 51.31 )
( 5620 , 51.46 )
( 5621 , 51.52 )
( 5622 , 51.52 )
( 5623 , 51.53 )
( 5624 , 51.53 )
( 5625 , 51.57 )
( 5626 , 51.63 )
( 5627 , 51.71 )
( 5628 , 51.80 )
( 5629 , 51.87 )
( 5630 , 51.89 )
( 5631 , 51.95 )
( 5632 , 52.00 )
( 5633 , 52.00 )
( 5634 , 52.01 )
( 5635 , 52.15 )
( 5636 , 52.15 )
( 5637 , 52.30 )
( 5638 , 52.30 )
( 5639 , 52.33 )
( 5640 , 52.35 )
( 5641 , 52.36 )
( 5642 , 52.59 )
( 5643 , 52.71 )
( 5644 , 52.77 )
( 5645 , 52.85 )
( 5646 , 52.97 )
( 5647 , 52.97 )
( 5648 , 52.91 )
( 5649 , 52.97 )
( 5650 , 53.06 )
( 5651 , 53.12 )
( 5652 , 53.07 )
( 5653 , 53.01 )
( 5654 , 52.95 )
( 5655 , 53.00 )
( 5656 , 53.18 )
( 5657 , 53.17 )
( 5658 , 53.14 )
( 5659 , 53.11 )
( 5660 , 53.18 )
( 5661 , 53.18 )
( 5662 , 53.19 )
( 5663 , 53.19 )
( 5664 , 53.20 )
( 5665 , 53.18 )
( 5666 , 53.18 )
( 5667 , 53.17 )
( 5668 , 53.32 )
( 5669 , 53.46 )
( 5670 , 53.71 )
( 5671 , 53.96 )
( 5672 , 54.20 )
( 5673 , 54.50 )
( 5674 , 54.80 )
( 5675 , 55.10 )
( 5676 , 55.34 )
( 5677 , 55.48 )
( 5678 , 55.62 )
( 5679 , 55.83 )
( 5680 , 56.05 )
( 5681 , 56.11 )
( 5682 , 56.18 )
( 5683 , 56.18 )
( 5684 , 56.18 )
( 5685 , 56.21 )
( 5686 , 56.21 )
( 5687 , 56.21 )
( 5688 , 56.45 )
( 5689 , 56.67 )
( 5690 , 56.90 )
( 5691 , 57.16 )
( 5692 , 57.42 )
( 5693 , 57.66 )
( 5694 , 57.89 )
( 5695 , 58.16 )
( 5696 , 58.40 )
( 5697 , 58.40 )
( 5698 , 58.41 )
( 5699 , 58.42 )
( 5700 , 58.44 )
( 5701 , 58.45 )
( 5702 , 58.46 )
( 5703 , 58.46 )
( 5704 , 58.49 )
( 5705 , 58.53 )
( 5706 , 58.53 )
( 5707 , 58.55 )
( 5708 , 58.56 )
( 5709 , 58.61 )
( 5710 , 58.76 )
( 5711 , 58.76 )
( 5712 , 58.93 )
( 5713 , 59.13 )
( 5714 , 59.30 )
( 5715 , 59.30 )
( 5716 , 59.34 )
( 5717 , 59.34 )
( 5718 , 59.34 )
( 5719 , 59.34 )
( 5720 , 59.48 )
( 5721 , 59.67 )
( 5722 , 59.83 )
( 5723 , 59.98 )
( 5724 , 60.12 )
( 5725 , 60.14 )
( 5726 , 60.20 )
( 5727 , 60.28 )
( 5728 , 60.40 )
( 5729 , 60.44 )
( 5730 , 60.45 )
( 5731 , 60.47 )
( 5732 , 60.48 )
( 5733 , 60.51 )
( 5734 , 60.51 )
( 5735 , 60.86 )
( 5736 , 61.21 )
( 5737 , 61.56 )
( 5738 , 61.92 )
( 5739 , 62.16 )
( 5740 , 62.38 )
( 5741 , 62.63 )
( 5742 , 62.85 )
( 5743 , 63.08 )
( 5744 , 63.30 )
( 5745 , 63.56 )
( 5746 , 63.79 )
( 5747 , 64.06 )
( 5748 , 64.49 )
( 5749 , 64.88 )
( 5750 , 65.16 )
( 5751 , 65.48 )
( 5752 , 65.80 )
( 5753 , 66.13 )
( 5754 , 66.41 )
( 5755 , 66.70 )
( 5756 , 66.98 )
( 5757 , 67.30 )
( 5758 , 67.60 )
( 5759 , 67.88 )
( 5760 , 68.17 )
( 5761 , 68.51 )
( 5762 , 68.78 )
( 5763 , 69.05 )
( 5764 , 69.37 )
( 5765 , 69.72 )
( 5766 , 70.02 )
( 5767 , 70.12 )
( 5768 , 70.16 )
( 5769 , 70.26 )
( 5770 , 70.48 )
( 5771 , 70.54 )
( 5772 , 70.59 )
( 5773 , 70.79 )
( 5774 , 70.91 )
( 5775 , 70.91 )
( 5776 , 70.92 )
( 5777 , 70.99 )
( 5778 , 70.99 )
( 5779 , 70.99 )
( 5780 , 71.00 )
( 5781 , 71.01 )
( 5782 , 71.01 )
( 5783 , 71.29 )
( 5784 , 71.52 )
( 5785 , 71.79 )
( 5786 , 72.07 )
( 5787 , 72.36 )
( 5788 , 72.70 )
( 5789 , 72.98 )
( 5790 , 73.20 )
( 5791 , 73.55 )
( 5792 , 73.88 )
( 5793 , 74.28 )
( 5794 , 74.51 )
( 5795 , 74.76 )
( 5796 , 75.01 )
( 5797 , 75.09 )
( 5798 , 75.27 )
( 5799 , 75.45 )
( 5800 , 75.60 )
( 5801 , 75.79 )
( 5802 , 75.80 )
( 5803 , 75.80 )
( 5804 , 75.82 )
( 5805 , 75.82 )
( 5806 , 76.04 )
( 5807 , 76.27 )
( 5808 , 76.49 )
( 5809 , 76.64 )
( 5810 , 76.83 )
( 5811 , 76.84 )
( 5812 , 76.86 )
( 5813 , 76.94 )
( 5814 , 76.98 )
( 5815 , 76.98 )
( 5816 , 76.98 )
( 5817 , 76.98 )
( 5818 , 77.20 )
( 5819 , 77.36 )
( 5820 , 77.38 )
( 5821 , 77.46 )
( 5822 , 77.53 )
( 5823 , 77.53 )
( 5824 , 77.54 )
( 5825 , 77.54 )
( 5826 , 77.69 )
( 5827 , 77.85 )
( 5828 , 78.09 )
( 5829 , 78.30 )
( 5830 , 78.45 )
( 5831 , 78.47 )
( 5832 , 78.47 )
( 5833 , 78.47 )
( 5834 , 78.47 )
( 5835 , 78.50 )
( 5836 , 78.58 )
( 5837 , 78.58 )
( 5838 , 78.60 )
( 5839 , 78.61 )
( 5840 , 78.62 )
( 5841 , 78.62 )
( 5842 , 78.93 )
( 5843 , 79.27 )
( 5844 , 79.60 )
( 5845 , 79.94 )
( 5846 , 80.25 )
( 5847 , 80.57 )
( 5848 , 80.89 )
( 5849 , 81.20 )
( 5850 , 81.48 )
( 5851 , 81.72 )
( 5852 , 81.95 )
( 5853 , 82.17 )
( 5854 , 82.51 )
( 5855 , 82.74 )
( 5856 , 83.01 )
( 5857 , 83.25 )
( 5858 , 83.47 )
( 5859 , 83.48 )
( 5860 , 83.48 )
( 5861 , 83.48 )
( 5862 , 83.48 )
( 5863 , 83.56 )
( 5864 , 83.63 )
( 5865 , 83.70 )
( 5866 , 83.70 )
( 5867 , 83.70 )
( 5868 , 83.80 )
( 5869 , 83.80 )
( 5870 , 83.88 )
( 5871 , 83.88 )
( 5872 , 83.88 )
( 5873 , 83.89 )
( 5874 , 83.89 )
( 5875 , 83.91 )
( 5876 , 83.91 )
( 5877 , 83.98 )
( 5878 , 83.98 )
( 5879 , 83.98 )
( 5880 , 83.98 )
( 5881 , 84.00 )
( 5882 , 84.00 )
( 5883 , 84.15 )
( 5884 , 84.30 )
( 5885 , 84.44 )
( 5886 , 84.44 )
( 5887 , 84.48 )
( 5888 , 84.57 )
( 5889 , 84.66 )
( 5890 , 84.67 )
( 5891 , 84.67 )
( 5892 , 84.67 )
( 5893 , 84.68 )
( 5894 , 84.68 )
( 5895 , 84.70 )
( 5896 , 84.73 )
( 5897 , 84.73 )
( 5898 , 84.76 )
( 5899 , 84.76 )
( 5900 , 84.80 )
( 5901 , 84.80 )
( 5902 , 84.80 )
( 5903 , 85.08 )
( 5904 , 85.38 )
( 5905 , 85.66 )
( 5906 , 85.91 )
( 5907 , 86.16 )
( 5908 , 86.39 )
( 5909 , 86.61 )
( 5910 , 86.88 )
( 5911 , 87.17 )
( 5912 , 87.40 )
( 5913 , 87.63 )
( 5914 , 87.91 )
( 5915 , 88.05 )
( 5916 , 88.05 )
( 5917 , 88.06 )
( 5918 , 88.06 )
( 5919 , 88.06 )
( 5920 , 88.06 )
( 5921 , 88.12 )
( 5922 , 88.12 )
( 5923 , 88.12 )
( 5924 , 88.19 )
( 5925 , 88.26 )
( 5926 , 88.28 )
( 5927 , 88.38 )
( 5928 , 88.41 )
( 5929 , 88.49 )
( 5930 , 88.52 )
( 5931 , 88.59 )
( 5932 , 88.78 )
( 5933 , 88.92 )
( 5934 , 89.08 )
( 5935 , 89.23 )
( 5936 , 89.30 )
( 5937 , 89.30 )
( 5938 , 89.42 )
( 5939 , 89.49 )
( 5940 , 89.70 )
( 5941 , 89.85 )
( 5942 , 90.05 )
( 5943 , 90.20 )
( 5944 , 90.27 )
( 5945 , 90.27 )
( 5946 , 90.30 )
( 5947 , 90.45 )
( 5948 , 90.45 )
( 5949 , 90.45 )
( 5950 , 90.54 )
( 5951 , 90.62 )
( 5952 , 90.70 )
( 5953 , 90.70 )
( 5954 , 90.77 )
( 5955 , 90.84 )
( 5956 , 90.95 )
( 5957 , 90.96 )
( 5958 , 90.98 )
( 5959 , 91.03 )
( 5960 , 91.07 )
( 5961 , 91.07 )
( 5962 , 91.20 )
( 5963 , 91.21 )
( 5964 , 91.27 )
( 5965 , 91.22 )
( 5966 , 91.16 )
( 5967 , 90.90 )
( 5968 , 90.62 )
( 5969 , 90.43 )
( 5970 , 90.23 )
( 5971 , 89.95 )
( 5972 , 89.67 )
( 5973 , 89.38 )
( 5974 , 89.23 )
( 5975 , 88.93 )
( 5976 , 88.84 )
( 5977 , 88.55 )
( 5978 , 88.25 )
( 5979 , 87.96 )
( 5980 , 87.75 )
( 5981 , 87.48 )
( 5982 , 87.27 )
( 5983 , 86.97 )
( 5984 , 86.67 )
( 5985 , 86.42 )
( 5986 , 86.18 )
( 5987 , 85.94 )
( 5988 , 85.72 )
( 5989 , 85.41 )
( 5990 , 85.11 )
( 5991 , 84.97 )
( 5992 , 84.76 )
( 5993 , 84.45 )
( 5994 , 84.16 )
( 5995 , 83.86 )
( 5996 , 83.61 )
( 5997 , 83.41 )
( 5998 , 83.20 )
( 5999 , 82.91 )
( 6000 , 82.80 )
( 6001 , 82.50 )
( 6002 , 82.20 )
( 6003 , 81.90 )
( 6004 , 81.59 )
( 6005 , 81.30 )
( 6006 , 81.01 )
( 6007 , 80.72 )
( 6008 , 80.43 )
( 6009 , 80.19 )
( 6010 , 79.99 )
( 6011 , 79.71 )
( 6012 , 79.41 )
( 6013 , 79.12 )
( 6014 , 78.83 )
( 6015 , 78.54 )
( 6016 , 78.45 )
( 6017 , 78.37 )
( 6018 , 78.29 )
( 6019 , 77.98 )
( 6020 , 77.84 )
( 6021 , 77.54 )
( 6022 , 77.34 )
( 6023 , 77.23 )
( 6024 , 76.98 )
( 6025 , 76.69 )
( 6026 , 76.38 )
( 6027 , 76.11 )
( 6028 , 75.96 )
( 6029 , 75.82 )
( 6030 , 75.62 )
( 6031 , 75.32 )
( 6032 , 75.02 )
( 6033 , 74.72 )
( 6034 , 74.42 )
( 6035 , 74.14 )
( 6036 , 73.84 )
( 6037 , 73.55 )
( 6038 , 73.24 )
( 6039 , 73.07 )
( 6040 , 72.88 )
( 6041 , 72.68 )
( 6042 , 72.48 )
( 6043 , 72.39 )
( 6044 , 72.38 )
( 6045 , 72.10 )
( 6046 , 71.81 )
( 6047 , 71.51 )
( 6048 , 71.20 )
( 6049 , 71.12 )
( 6050 , 71.02 )
( 6051 , 70.93 )
( 6052 , 70.84 )
( 6053 , 70.77 )
( 6054 , 70.63 )
( 6055 , 70.43 )
( 6056 , 70.13 )
( 6057 , 69.85 )
( 6058 , 69.55 )
( 6059 , 69.28 )
( 6060 , 68.98 )
( 6061 , 68.69 )
( 6062 , 68.38 )
( 6063 , 68.09 )
( 6064 , 67.78 )
( 6065 , 67.48 )
( 6066 , 67.29 )
( 6067 , 67.23 )
( 6068 , 67.13 )
( 6069 , 66.99 )
( 6070 , 66.71 )
( 6071 , 66.41 )
( 6072 , 66.21 )
( 6073 , 65.91 )
( 6074 , 65.82 )
( 6075 , 65.76 )
( 6076 , 65.46 )
( 6077 , 65.16 )
( 6078 , 65.02 )
( 6079 , 64.80 )
( 6080 , 64.58 )
( 6081 , 64.27 )
( 6082 , 64.15 )
( 6083 , 63.86 )
( 6084 , 63.93 )
( 6085 , 63.84 )
( 6086 , 63.74 )
( 6087 , 63.72 )
( 6088 , 63.65 )
( 6089 , 63.55 )
( 6090 , 63.46 )
( 6091 , 63.19 )
( 6092 , 62.89 )
( 6093 , 62.59 )
( 6094 , 62.30 )
( 6095 , 62.05 )
( 6096 , 61.74 )
( 6097 , 61.44 )
( 6098 , 61.30 )
( 6099 , 61.15 )
( 6100 , 61.19 )
( 6101 , 61.23 )
( 6102 , 61.26 )
( 6103 , 61.11 )
( 6104 , 60.96 )
( 6105 , 60.80 )
( 6106 , 60.50 )
( 6107 , 60.40 )
( 6108 , 60.46 )
( 6109 , 60.48 )
( 6110 , 60.18 )
( 6111 , 59.88 )
( 6112 , 59.79 )
( 6113 , 59.49 )
( 6114 , 59.39 )
( 6115 , 59.38 )
( 6116 , 59.29 )
( 6117 , 59.23 )
( 6118 , 59.08 )
( 6119 , 58.91 )
( 6120 , 58.85 )
( 6121 , 58.77 )
( 6122 , 58.62 )
( 6123 , 58.34 )
( 6124 , 58.13 )
( 6125 , 57.96 )
( 6126 , 57.75 )
( 6127 , 57.55 )
( 6128 , 57.42 )
( 6129 , 57.32 )
( 6130 , 57.30 )
( 6131 , 57.20 )
( 6132 , 57.13 )
( 6133 , 57.11 )
( 6134 , 57.02 )
( 6135 , 56.81 )
( 6136 , 56.55 )
( 6137 , 56.28 )
( 6138 , 56.03 )
( 6139 , 55.80 )
( 6140 , 55.78 )
( 6141 , 55.68 )
( 6142 , 55.41 )
( 6143 , 55.23 )
( 6144 , 55.04 )
( 6145 , 54.88 )
( 6146 , 54.64 )
( 6147 , 54.37 )
( 6148 , 54.09 )
( 6149 , 53.84 )
( 6150 , 53.64 )
( 6151 , 53.40 )
( 6152 , 53.09 )
( 6153 , 52.79 )
( 6154 , 52.49 )
( 6155 , 52.20 )
( 6156 , 51.91 )
( 6157 , 51.81 )
( 6158 , 51.56 )
( 6159 , 51.32 )
( 6160 , 51.02 )
( 6161 , 50.87 )
( 6162 , 50.82 )
( 6163 , 50.52 )
( 6164 , 50.30 )
( 6165 , 50.00 )
( 6166 , 49.70 )
( 6167 , 49.51 )
( 6168 , 49.21 )
( 6169 , 48.95 )
( 6170 , 49.07 )
( 6171 , 49.12 )
( 6172 , 48.84 )
( 6173 , 48.64 )
( 6174 , 48.47 )
( 6175 , 48.35 )
( 6176 , 48.20 )
( 6177 , 47.90 )
( 6178 , 47.93 )
( 6179 , 47.92 )
( 6180 , 47.62 )
( 6181 , 47.32 )
( 6182 , 47.18 )
( 6183 , 46.88 )
( 6184 , 46.78 )
( 6185 , 46.57 )
( 6186 , 46.30 )
( 6187 , 46.10 )
( 6188 , 45.82 )
( 6189 , 45.62 )
( 6190 , 45.44 )
( 6191 , 45.14 )
( 6192 , 44.84 )
( 6193 , 44.54 )
( 6194 , 44.48 )
( 6195 , 44.47 )
( 6196 , 44.38 )
( 6197 , 44.08 )
( 6198 , 43.78 )
( 6199 , 43.54 )
( 6200 , 43.25 )
( 6201 , 42.97 )
( 6202 , 42.68 )
( 6203 , 42.59 )
( 6204 , 42.49 )
( 6205 , 42.40 )
( 6206 , 42.10 )
( 6207 , 41.82 )
( 6208 , 41.54 )
( 6209 , 41.26 )
( 6210 , 41.17 )
( 6211 , 40.87 )
( 6212 , 40.74 )
( 6213 , 40.62 )
( 6214 , 40.58 )
( 6215 , 40.46 )
( 6216 , 40.34 )
( 6217 , 40.36 )
( 6218 , 40.33 )
( 6219 , 40.45 )
( 6220 , 40.44 )
( 6221 , 40.43 )
( 6222 , 40.29 )
( 6223 , 39.98 )
( 6224 , 39.69 )
( 6225 , 39.39 )
( 6226 , 39.09 )
( 6227 , 38.95 )
( 6228 , 38.65 )
( 6229 , 38.58 )
( 6230 , 38.53 )
( 6231 , 38.47 )
( 6232 , 38.37 )
( 6233 , 38.07 )
( 6234 , 37.86 )
( 6235 , 37.66 )
( 6236 , 37.36 )
( 6237 , 37.06 )
( 6238 , 36.80 )
( 6239 , 36.59 )
( 6240 , 36.49 )
( 6241 , 36.39 )
( 6242 , 36.30 )
( 6243 , 36.00 )
( 6244 , 36.09 )
( 6245 , 36.22 )
( 6246 , 36.36 )
( 6247 , 36.31 )
( 6248 , 36.25 )
( 6249 , 36.13 )
( 6250 , 36.17 )
( 6251 , 36.21 )
( 6252 , 36.30 )
( 6253 , 36.34 )
( 6254 , 36.27 )
( 6255 , 36.45 )
( 6256 , 36.63 )
( 6257 , 36.51 )
( 6258 , 36.42 )
( 6259 , 36.42 )
( 6260 , 36.37 )
( 6261 , 36.24 )
( 6262 , 36.14 )
( 6263 , 36.05 )
( 6264 , 36.11 )
( 6265 , 35.99 )
( 6266 , 36.05 )
( 6267 , 36.09 )
( 6268 , 36.16 )
( 6269 , 36.04 )
( 6270 , 35.99 )
( 6271 , 35.86 )
( 6272 , 35.87 )
( 6273 , 35.82 )
( 6274 , 35.79 )
( 6275 , 35.66 )
( 6276 , 35.54 )
( 6277 , 35.41 )
( 6278 , 35.31 )
( 6279 , 35.23 )
( 6280 , 35.25 )
( 6281 , 35.17 )
( 6282 , 35.05 )
( 6283 , 34.95 )
( 6284 , 34.94 )
( 6285 , 34.98 )
( 6286 , 35.07 )
( 6287 , 35.07 )
( 6288 , 35.15 )
( 6289 , 35.23 )
( 6290 , 35.39 )
( 6291 , 35.50 )
( 6292 , 35.49 )
( 6293 , 35.75 )
( 6294 , 36.00 )
( 6295 , 36.27 )
( 6296 , 36.61 )
( 6297 , 36.97 )
( 6298 , 37.17 )
( 6299 , 37.42 )
( 6300 , 37.62 )
( 6301 , 37.54 )
( 6302 , 37.46 )
( 6303 , 37.36 )
( 6304 , 37.23 )
( 6305 , 37.38 )
( 6306 , 37.49 )
( 6307 , 37.45 )
( 6308 , 37.46 )
( 6309 , 37.49 )
( 6310 , 37.36 )
( 6311 , 37.27 )
( 6312 , 37.18 )
( 6313 , 37.08 )
( 6314 , 37.20 )
( 6315 , 37.20 )
( 6316 , 37.08 )
( 6317 , 36.96 )
( 6318 , 37.01 )
( 6319 , 37.09 )
( 6320 , 37.20 )
( 6321 , 37.27 )
( 6322 , 37.30 )
( 6323 , 37.18 )
( 6324 , 37.05 )
( 6325 , 37.16 )
( 6326 , 37.29 )
( 6327 , 37.39 )
( 6328 , 37.64 )
( 6329 , 37.76 )
( 6330 , 38.00 )
( 6331 , 38.14 )
( 6332 , 38.31 )
( 6333 , 38.49 )
( 6334 , 38.50 )
( 6335 , 38.49 )
( 6336 , 38.45 )
( 6337 , 38.52 )
( 6338 , 38.47 )
( 6339 , 38.41 )
( 6340 , 38.36 )
( 6341 , 38.45 )
( 6342 , 38.53 )
( 6343 , 38.47 )
( 6344 , 38.20 )
( 6345 , 37.90 )
( 6346 , 37.75 )
( 6347 , 37.69 )
( 6348 , 37.70 )
( 6349 , 37.64 )
( 6350 , 37.58 )
( 6351 , 37.54 )
( 6352 , 37.48 )
( 6353 , 37.62 )
( 6354 , 37.74 )
( 6355 , 37.87 )
( 6356 , 37.97 )
( 6357 , 38.06 )
( 6358 , 38.16 )
( 6359 , 38.40 )
( 6360 , 38.52 )
( 6361 , 38.62 )
( 6362 , 38.72 )
( 6363 , 38.77 )
( 6364 , 38.84 )
( 6365 , 38.96 )
( 6366 , 39.00 )
( 6367 , 38.96 )
( 6368 , 38.93 )
( 6369 , 38.63 )
( 6370 , 38.35 )
( 6371 , 38.05 )
( 6372 , 37.75 )
( 6373 , 37.48 )
( 6374 , 37.24 )
( 6375 , 36.94 )
( 6376 , 36.65 )
( 6377 , 36.35 )
( 6378 , 36.34 )
( 6379 , 36.34 )
( 6380 , 36.12 )
( 6381 , 35.95 )
( 6382 , 35.74 )
( 6383 , 35.46 )
( 6384 , 35.16 )
( 6385 , 34.87 )
( 6386 , 34.72 )
( 6387 , 34.42 )
( 6388 , 34.12 )
( 6389 , 34.00 )
( 6390 , 33.89 )
( 6391 , 33.79 )
( 6392 , 33.66 )
( 6393 , 33.55 )
( 6394 , 33.36 )
( 6395 , 33.15 )
( 6396 , 32.85 )
( 6397 , 32.55 )
( 6398 , 32.26 )
( 6399 , 31.96 )
( 6400 , 31.85 )
( 6401 , 31.64 )
( 6402 , 31.34 )
( 6403 , 31.04 )
( 6404 , 31.03 )
( 6405 , 30.73 )
( 6406 , 30.43 )
( 6407 , 30.19 )
( 6408 , 29.90 )
( 6409 , 29.61 )
( 6410 , 29.42 )
( 6411 , 29.12 )
( 6412 , 28.81 )
( 6413 , 28.70 )
( 6414 , 28.60 )
( 6415 , 28.55 )
( 6416 , 28.51 )
( 6417 , 28.45 )
( 6418 , 28.35 )
( 6419 , 28.05 )
( 6420 , 27.75 )
( 6421 , 27.73 )
( 6422 , 27.62 )
( 6423 , 27.60 )
( 6424 , 27.54 )
( 6425 , 27.24 )
( 6426 , 26.99 )
( 6427 , 27.11 )
( 6428 , 26.97 )
( 6429 , 26.89 )
( 6430 , 26.75 )
( 6431 , 26.52 )
( 6432 , 26.22 )
( 6433 , 25.92 )
( 6434 , 25.69 )
( 6435 , 25.45 )
( 6436 , 25.19 )
( 6437 , 24.91 )
( 6438 , 24.61 )
( 6439 , 24.31 )
( 6440 , 24.01 )
( 6441 , 23.74 )
( 6442 , 23.44 )
( 6443 , 23.14 )
( 6444 , 23.10 )
( 6445 , 23.01 )
( 6446 , 22.72 )
( 6447 , 22.43 )
( 6448 , 22.15 )
( 6449 , 21.88 )
( 6450 , 21.58 )
( 6451 , 21.29 )
( 6452 , 20.99 )
( 6453 , 20.71 )
( 6454 , 20.66 )
( 6455 , 20.37 )
( 6456 , 20.18 )
( 6457 , 20.03 )
( 6458 , 19.87 )
( 6459 , 19.63 )
( 6460 , 19.33 )
( 6461 , 19.03 )
( 6462 , 18.73 )
( 6463 , 18.67 )
( 6464 , 18.71 )
( 6465 , 18.68 )
( 6466 , 18.38 )
( 6467 , 18.25 )
( 6468 , 17.98 )
( 6469 , 17.69 )
( 6470 , 17.55 )
( 6471 , 17.30 )
( 6472 , 17.03 )
( 6473 , 16.82 )
( 6474 , 16.52 )
( 6475 , 16.24 )
( 6476 , 16.17 )
( 6477 , 16.02 )
( 6478 , 15.75 )
( 6479 , 15.46 )
( 6480 , 15.16 )
( 6481 , 14.86 )
( 6482 , 14.76 )
( 6483 , 14.86 )
( 6484 , 14.65 )
( 6485 , 14.35 )
( 6486 , 14.11 )
( 6487 , 13.82 )
( 6488 , 13.55 )
( 6489 , 13.34 )
( 6490 , 13.12 )
( 6491 , 12.91 )
( 6492 , 12.61 )
( 6493 , 12.31 )
( 6494 , 12.00 )
( 6495 , 11.70 )
( 6496 , 11.72 )
( 6497 , 11.62 )
( 6498 , 11.35 )
( 6499 , 11.05 )
( 6500 , 10.85 )
( 6501 , 10.58 )
( 6502 , 10.28 )
( 6503 , 10.25 )
( 6504 , 9.951 )
( 6505 , 9.650 )
( 6506 , 9.525 )
( 6507 , 9.379 )
( 6508 , 9.087 )
( 6509 , 8.838 )
( 6510 , 8.537 )
( 6511 , 8.300 )
( 6512 , 8.211 )
( 6513 , 8.235 )
( 6514 , 7.965 )
( 6515 , 7.919 )
( 6516 , 7.823 )
( 6517 , 7.521 )
( 6518 , 7.465 )
( 6519 , 7.411 )
( 6520 , 7.448 )
( 6521 , 7.390 )
( 6522 , 7.332 )
( 6523 , 7.031 )
( 6524 , 6.900 )
( 6525 , 6.913 )
( 6526 , 6.702 )
( 6527 , 6.608 )
( 6528 , 6.310 )
( 6529 , 6.021 )
( 6530 , 5.791 )
( 6531 , 5.735 )
( 6532 , 5.529 )
( 6533 , 5.228 )
( 6534 , 5.104 )
( 6535 , 5.060 )
( 6536 , 5.135 )
( 6537 , 5.209 )
( 6538 , 5.209 )
( 6539 , 5.417 )
( 6540 , 5.564 )
( 6541 , 5.579 )
( 6542 , 5.610 )
( 6543 , 5.610 )
( 6544 , 5.664 )
( 6545 , 5.686 )
( 6546 , 5.735 )
( 6547 , 5.803 )
( 6548 , 5.803 )
( 6549 , 6.138 )
( 6550 , 6.360 )
( 6551 , 6.375 )
( 6552 , 6.266 )
( 6553 , 6.169 )
( 6554 , 5.913 )
( 6555 , 5.848 )
( 6556 , 5.751 )
( 6557 , 5.731 )
( 6558 , 5.430 )
( 6559 , 5.129 )
( 6560 , 4.839 )
( 6561 , 4.609 )
( 6562 , 4.413 )
( 6563 , 4.235 )
( 6564 , 3.935 )
( 6565 , 3.842 )
( 6566 , 3.783 )
( 6567 , 3.688 )
( 6568 , 3.387 )
( 6569 , 3.497 )
( 6570 , 3.543 )
( 6571 , 3.569 )
( 6572 , 3.513 )
( 6573 , 3.554 )
( 6574 , 3.663 )
( 6575 , 3.817 )
( 6576 , 3.969 )
( 6577 , 3.907 )
( 6578 , 3.850 )
( 6579 , 3.549 )
( 6580 , 3.528 )
( 6581 , 3.434 )
( 6582 , 3.206 )
( 6583 , 3.024 )
( 6584 , 2.779 )
( 6585 , 0.000 )
};



==> H565680 <==
\addplot[color=red] coordinates{
( 0 , 5.752 )
( 1 , 6.075 )
( 2 , 6.312 )
( 3 , 6.680 )
( 4 , 6.935 )
( 5 , 7.225 )
( 6 , 7.424 )
( 7 , 7.521 )
( 8 , 7.643 )
( 9 , 7.746 )
( 10 , 7.746 )
( 11 , 7.978 )
( 12 , 8.151 )
( 13 , 8.311 )
( 14 , 8.311 )
( 15 , 8.359 )
( 16 , 8.581 )
( 17 , 8.679 )
( 18 , 8.764 )
( 19 , 8.813 )
( 20 , 8.892 )
( 21 , 9.038 )
( 22 , 9.185 )
( 23 , 9.185 )
( 24 , 9.418 )
( 25 , 9.641 )
( 26 , 9.703 )
( 27 , 9.726 )
( 28 , 9.726 )
( 29 , 9.726 )
( 30 , 9.771 )
( 31 , 9.908 )
( 32 , 10.05 )
( 33 , 10.08 )
( 34 , 10.11 )
( 35 , 10.10 )
( 36 , 9.979 )
( 37 , 10.00 )
( 38 , 10.13 )
( 39 , 10.01 )
( 40 , 10.25 )
( 41 , 10.46 )
( 42 , 10.64 )
( 43 , 10.82 )
( 44 , 11.12 )
( 45 , 11.30 )
( 46 , 11.48 )
( 47 , 11.66 )
( 48 , 11.99 )
( 49 , 12.36 )
( 50 , 12.58 )
( 51 , 12.80 )
( 52 , 13.01 )
( 53 , 13.24 )
( 54 , 13.44 )
( 55 , 13.76 )
( 56 , 14.10 )
( 57 , 14.41 )
( 58 , 14.72 )
( 59 , 15.14 )
( 60 , 15.47 )
( 61 , 15.72 )
( 62 , 15.98 )
( 63 , 16.22 )
( 64 , 16.45 )
( 65 , 16.68 )
( 66 , 16.75 )
( 67 , 16.82 )
( 68 , 16.88 )
( 69 , 16.95 )
( 70 , 17.02 )
( 71 , 17.23 )
( 72 , 17.30 )
( 73 , 17.48 )
( 74 , 17.59 )
( 75 , 17.91 )
( 76 , 18.00 )
( 77 , 18.02 )
( 78 , 18.02 )
( 79 , 18.03 )
( 80 , 18.04 )
( 81 , 18.13 )
( 82 , 18.20 )
( 83 , 18.23 )
( 84 , 18.26 )
( 85 , 18.26 )
( 86 , 18.33 )
( 87 , 18.59 )
( 88 , 18.79 )
( 89 , 18.79 )
( 90 , 18.79 )
( 91 , 18.79 )
( 92 , 18.79 )
( 93 , 18.97 )
( 94 , 19.04 )
( 95 , 19.05 )
( 96 , 19.05 )
( 97 , 19.09 )
( 98 , 19.11 )
( 99 , 19.18 )
( 100 , 19.44 )
( 101 , 19.72 )
( 102 , 19.88 )
( 103 , 20.10 )
( 104 , 20.31 )
( 105 , 20.37 )
( 106 , 20.50 )
( 107 , 20.63 )
( 108 , 20.76 )
( 109 , 20.96 )
( 110 , 21.05 )
( 111 , 21.07 )
( 112 , 21.11 )
( 113 , 21.12 )
( 114 , 21.12 )
( 115 , 21.12 )
( 116 , 21.12 )
( 117 , 21.12 )
( 118 , 21.26 )
( 119 , 21.28 )
( 120 , 21.46 )
( 121 , 21.63 )
( 122 , 21.92 )
( 123 , 22.10 )
( 124 , 22.25 )
( 125 , 22.44 )
( 126 , 22.60 )
( 127 , 22.66 )
( 128 , 22.73 )
( 129 , 22.90 )
( 130 , 22.97 )
( 131 , 23.03 )
( 132 , 23.10 )
( 133 , 23.28 )
( 134 , 23.49 )
( 135 , 23.71 )
( 136 , 23.91 )
( 137 , 24.01 )
( 138 , 24.11 )
( 139 , 24.18 )
( 140 , 24.26 )
( 141 , 24.33 )
( 142 , 24.55 )
( 143 , 24.78 )
( 144 , 24.98 )
( 145 , 25.19 )
( 146 , 25.49 )
( 147 , 25.83 )
( 148 , 26.01 )
( 149 , 26.11 )
( 150 , 26.21 )
( 151 , 26.45 )
( 152 , 26.57 )
( 153 , 26.68 )
( 154 , 26.84 )
( 155 , 27.06 )
( 156 , 27.13 )
( 157 , 27.30 )
( 158 , 27.52 )
( 159 , 27.74 )
( 160 , 27.95 )
( 161 , 28.22 )
( 162 , 28.43 )
( 163 , 28.78 )
( 164 , 28.90 )
( 165 , 29.12 )
( 166 , 29.24 )
( 167 , 29.26 )
( 168 , 29.31 )
( 169 , 29.29 )
( 170 , 29.27 )
( 171 , 29.25 )
( 172 , 29.24 )
( 173 , 29.23 )
( 174 , 29.24 )
( 175 , 29.23 )
( 176 , 29.39 )
( 177 , 29.55 )
( 178 , 29.71 )
( 179 , 29.95 )
( 180 , 30.05 )
( 181 , 30.14 )
( 182 , 30.32 )
( 183 , 30.44 )
( 184 , 30.55 )
( 185 , 30.65 )
( 186 , 30.74 )
( 187 , 30.84 )
( 188 , 30.90 )
( 189 , 30.84 )
( 190 , 30.78 )
( 191 , 30.72 )
( 192 , 30.74 )
( 193 , 30.78 )
( 194 , 30.72 )
( 195 , 30.68 )
( 196 , 30.62 )
( 197 , 30.65 )
( 198 , 30.63 )
( 199 , 30.60 )
( 200 , 30.60 )
( 201 , 30.60 )
( 202 , 30.60 )
( 203 , 30.68 )
( 204 , 30.71 )
( 205 , 30.74 )
( 206 , 30.76 )
( 207 , 30.76 )
( 208 , 30.90 )
( 209 , 30.95 )
( 210 , 31.10 )
( 211 , 31.25 )
( 212 , 31.36 )
( 213 , 31.55 )
( 214 , 31.74 )
( 215 , 31.89 )
( 216 , 32.07 )
( 217 , 32.21 )
( 218 , 32.21 )
( 219 , 32.23 )
( 220 , 32.32 )
( 221 , 32.41 )
( 222 , 32.44 )
( 223 , 32.44 )
( 224 , 32.44 )
( 225 , 32.44 )
( 226 , 32.47 )
( 227 , 32.54 )
( 228 , 32.57 )
( 229 , 32.62 )
( 230 , 32.63 )
( 231 , 32.57 )
( 232 , 32.49 )
( 233 , 32.19 )
( 234 , 32.12 )
( 235 , 31.84 )
( 236 , 31.55 )
( 237 , 31.25 )
( 238 , 30.95 )
( 239 , 30.71 )
( 240 , 30.51 )
( 241 , 30.31 )
( 242 , 30.25 )
( 243 , 30.23 )
( 244 , 30.19 )
( 245 , 29.89 )
( 246 , 29.59 )
( 247 , 29.63 )
( 248 , 29.53 )
( 249 , 29.23 )
( 250 , 29.17 )
( 251 , 28.89 )
( 252 , 28.61 )
( 253 , 28.38 )
( 254 , 28.08 )
( 255 , 27.85 )
( 256 , 27.78 )
( 257 , 27.63 )
( 258 , 27.57 )
( 259 , 27.50 )
( 260 , 27.41 )
( 261 , 27.44 )
( 262 , 27.21 )
( 263 , 27.10 )
( 264 , 27.15 )
( 265 , 27.21 )
( 266 , 27.26 )
( 267 , 27.21 )
( 268 , 27.11 )
( 269 , 27.03 )
( 270 , 26.74 )
( 271 , 26.67 )
( 272 , 26.37 )
( 273 , 26.22 )
( 274 , 25.94 )
( 275 , 25.73 )
( 276 , 25.43 )
( 277 , 25.13 )
( 278 , 25.02 )
( 279 , 24.72 )
( 280 , 24.51 )
( 281 , 24.21 )
( 282 , 24.02 )
( 283 , 23.74 )
( 284 , 23.44 )
( 285 , 23.34 )
( 286 , 23.25 )
( 287 , 22.98 )
( 288 , 22.80 )
( 289 , 22.50 )
( 290 , 22.27 )
( 291 , 22.03 )
( 292 , 21.74 )
( 293 , 21.50 )
( 294 , 21.20 )
( 295 , 20.90 )
( 296 , 20.89 )
( 297 , 20.59 )
( 298 , 20.29 )
( 299 , 20.01 )
( 300 , 19.86 )
( 301 , 19.58 )
( 302 , 19.28 )
( 303 , 18.98 )
( 304 , 18.88 )
( 305 , 18.66 )
( 306 , 18.38 )
( 307 , 18.08 )
( 308 , 17.98 )
( 309 , 17.79 )
( 310 , 17.80 )
( 311 , 17.79 )
( 312 , 17.49 )
( 313 , 17.37 )
( 314 , 17.11 )
( 315 , 16.96 )
( 316 , 16.83 )
( 317 , 16.53 )
( 318 , 16.23 )
( 319 , 15.95 )
( 320 , 15.86 )
( 321 , 15.68 )
( 322 , 15.38 )
( 323 , 15.08 )
( 324 , 15.20 )
( 325 , 15.32 )
( 326 , 15.49 )
( 327 , 15.65 )
( 328 , 15.83 )
( 329 , 15.91 )
( 330 , 15.97 )
( 331 , 15.95 )
( 332 , 15.99 )
( 333 , 15.91 )
( 334 , 15.83 )
( 335 , 15.72 )
( 336 , 15.59 )
( 337 , 15.49 )
( 338 , 15.66 )
( 339 , 15.53 )
( 340 , 15.41 )
( 341 , 15.29 )
( 342 , 15.33 )
( 343 , 15.21 )
( 344 , 15.21 )
( 345 , 15.20 )
( 346 , 15.31 )
( 347 , 15.41 )
( 348 , 15.51 )
( 349 , 15.74 )
( 350 , 15.97 )
( 351 , 16.23 )
( 352 , 16.32 )
( 353 , 16.56 )
( 354 , 16.65 )
( 355 , 16.80 )
( 356 , 16.94 )
( 357 , 17.02 )
( 358 , 17.10 )
( 359 , 17.09 )
( 360 , 16.97 )
( 361 , 16.85 )
( 362 , 16.78 )
( 363 , 16.65 )
( 364 , 16.68 )
( 365 , 16.67 )
( 366 , 16.73 )
( 367 , 16.95 )
( 368 , 16.89 )
( 369 , 16.88 )
( 370 , 16.90 )
( 371 , 16.89 )
( 372 , 16.79 )
( 373 , 16.67 )
( 374 , 16.64 )
( 375 , 16.90 )
( 376 , 17.10 )
( 377 , 17.30 )
( 378 , 17.44 )
( 379 , 17.60 )
( 380 , 17.70 )
( 381 , 17.74 )
( 382 , 17.85 )
( 383 , 18.00 )
( 384 , 18.05 )
( 385 , 18.10 )
( 386 , 17.99 )
( 387 , 17.88 )
( 388 , 17.76 )
( 389 , 17.79 )
( 390 , 17.71 )
( 391 , 17.62 )
( 392 , 17.60 )
( 393 , 17.50 )
( 394 , 17.23 )
( 395 , 17.14 )
( 396 , 16.84 )
( 397 , 16.54 )
( 398 , 16.24 )
( 399 , 15.94 )
( 400 , 15.68 )
( 401 , 15.38 )
( 402 , 15.35 )
( 403 , 15.13 )
( 404 , 14.96 )
( 405 , 14.76 )
( 406 , 14.54 )
( 407 , 14.30 )
( 408 , 14.16 )
( 409 , 14.20 )
( 410 , 14.22 )
( 411 , 14.08 )
( 412 , 13.77 )
( 413 , 13.47 )
( 414 , 13.17 )
( 415 , 12.87 )
( 416 , 12.67 )
( 417 , 12.38 )
( 418 , 12.18 )
( 419 , 11.88 )
( 420 , 11.62 )
( 421 , 11.32 )
( 422 , 11.12 )
( 423 , 11.15 )
( 424 , 11.06 )
( 425 , 10.79 )
( 426 , 10.56 )
( 427 , 10.27 )
( 428 , 9.970 )
( 429 , 9.675 )
( 430 , 9.373 )
( 431 , 9.385 )
( 432 , 9.429 )
( 433 , 9.517 )
( 434 , 9.458 )
( 435 , 9.417 )
( 436 , 9.364 )
( 437 , 9.246 )
( 438 , 9.293 )
( 439 , 9.303 )
( 440 , 9.530 )
( 441 , 9.726 )
( 442 , 9.917 )
( 443 , 10.04 )
( 444 , 10.04 )
( 445 , 10.05 )
( 446 , 10.13 )
( 447 , 10.16 )
( 448 , 10.22 )
( 449 , 10.27 )
( 450 , 10.28 )
( 451 , 10.28 )
( 452 , 10.33 )
( 453 , 10.33 )
( 454 , 10.40 )
( 455 , 10.68 )
( 456 , 10.91 )
( 457 , 11.33 )
( 458 , 11.63 )
( 459 , 11.91 )
( 460 , 12.30 )
( 461 , 12.67 )
( 462 , 12.89 )
( 463 , 12.93 )
( 464 , 12.93 )
( 465 , 13.14 )
( 466 , 13.21 )
( 467 , 13.22 )
( 468 , 13.51 )
( 469 , 13.52 )
( 470 , 13.55 )
( 471 , 13.63 )
( 472 , 13.57 )
( 473 , 13.58 )
( 474 , 13.54 )
( 475 , 13.48 )
( 476 , 13.58 )
( 477 , 13.53 )
( 478 , 13.59 )
( 479 , 13.71 )
( 480 , 13.78 )
( 481 , 13.78 )
( 482 , 13.76 )
( 483 , 13.97 )
( 484 , 14.26 )
( 485 , 14.62 )
( 486 , 14.83 )
( 487 , 15.04 )
( 488 , 15.28 )
( 489 , 15.67 )
( 490 , 15.98 )
( 491 , 16.28 )
( 492 , 16.42 )
( 493 , 16.52 )
( 494 , 16.64 )
( 495 , 16.84 )
( 496 , 16.94 )
( 497 , 17.11 )
( 498 , 17.25 )
( 499 , 17.37 )
( 500 , 17.50 )
( 501 , 17.62 )
( 502 , 17.75 )
( 503 , 17.87 )
( 504 , 18.10 )
( 505 , 18.29 )
( 506 , 18.38 )
( 507 , 18.62 )
( 508 , 18.82 )
( 509 , 18.93 )
( 510 , 19.03 )
( 511 , 19.17 )
( 512 , 19.37 )
( 513 , 19.42 )
( 514 , 19.56 )
( 515 , 19.53 )
( 516 , 19.53 )
( 517 , 19.50 )
( 518 , 19.38 )
( 519 , 19.08 )
( 520 , 18.85 )
( 521 , 18.58 )
( 522 , 18.28 )
( 523 , 18.03 )
( 524 , 17.86 )
( 525 , 17.56 )
( 526 , 17.36 )
( 527 , 17.24 )
( 528 , 16.96 )
( 529 , 16.65 )
( 530 , 16.60 )
( 531 , 16.54 )
( 532 , 16.48 )
( 533 , 16.43 )
( 534 , 16.38 )
( 535 , 16.32 )
( 536 , 16.41 )
( 537 , 16.43 )
( 538 , 16.42 )
( 539 , 16.41 )
( 540 , 16.39 )
( 541 , 16.48 )
( 542 , 16.69 )
( 543 , 16.88 )
( 544 , 17.00 )
( 545 , 17.09 )
( 546 , 17.06 )
( 547 , 17.07 )
( 548 , 17.14 )
( 549 , 17.04 )
( 550 , 16.99 )
( 551 , 16.87 )
( 552 , 16.98 )
( 553 , 16.89 )
( 554 , 16.77 )
( 555 , 16.64 )
( 556 , 16.52 )
( 557 , 16.59 )
( 558 , 16.54 )
( 559 , 16.51 )
( 560 , 16.41 )
( 561 , 16.45 )
( 562 , 16.25 )
( 563 , 15.95 )
( 564 , 16.12 )
( 565 , 16.26 )
( 566 , 16.32 )
( 567 , 16.48 )
( 568 , 16.60 )
( 569 , 16.55 )
( 570 , 16.73 )
( 571 , 16.94 )
( 572 , 17.34 )
( 573 , 17.53 )
( 574 , 17.51 )
( 575 , 17.60 )
( 576 , 17.68 )
( 577 , 17.76 )
( 578 , 17.82 )
( 579 , 17.79 )
( 580 , 17.66 )
( 581 , 17.54 )
( 582 , 17.63 )
( 583 , 17.73 )
( 584 , 17.71 )
( 585 , 17.97 )
( 586 , 18.18 )
( 587 , 18.40 )
( 588 , 18.65 )
( 589 , 18.83 )
( 590 , 18.77 )
( 591 , 18.72 )
( 592 , 18.60 )
( 593 , 18.47 )
( 594 , 18.18 )
( 595 , 17.96 )
( 596 , 17.67 )
( 597 , 17.37 )
( 598 , 17.07 )
( 599 , 16.86 )
( 600 , 16.62 )
( 601 , 16.32 )
( 602 , 16.03 )
( 603 , 15.96 )
( 604 , 15.86 )
( 605 , 15.91 )
( 606 , 15.61 )
( 607 , 15.31 )
( 608 , 15.45 )
( 609 , 15.41 )
( 610 , 15.28 )
( 611 , 15.41 )
( 612 , 15.57 )
( 613 , 15.69 )
( 614 , 15.88 )
( 615 , 16.01 )
( 616 , 16.14 )
( 617 , 16.32 )
( 618 , 16.42 )
( 619 , 16.55 )
( 620 , 16.80 )
( 621 , 17.05 )
( 622 , 17.14 )
( 623 , 17.14 )
( 624 , 17.30 )
( 625 , 17.39 )
( 626 , 17.46 )
( 627 , 17.53 )
( 628 , 17.97 )
( 629 , 18.39 )
( 630 , 18.82 )
( 631 , 19.25 )
( 632 , 19.62 )
( 633 , 20.00 )
( 634 , 20.35 )
( 635 , 20.72 )
( 636 , 21.12 )
( 637 , 21.38 )
( 638 , 21.65 )
( 639 , 21.97 )
( 640 , 22.29 )
( 641 , 22.36 )
( 642 , 22.36 )
( 643 , 22.37 )
( 644 , 22.39 )
( 645 , 22.57 )
( 646 , 22.73 )
( 647 , 22.91 )
( 648 , 23.13 )
( 649 , 23.35 )
( 650 , 23.33 )
( 651 , 23.32 )
( 652 , 23.31 )
( 653 , 23.30 )
( 654 , 23.49 )
( 655 , 23.50 )
( 656 , 23.59 )
( 657 , 23.69 )
( 658 , 23.66 )
( 659 , 23.70 )
( 660 , 23.78 )
( 661 , 23.93 )
( 662 , 24.17 )
( 663 , 24.34 )
( 664 , 24.35 )
( 665 , 24.45 )
( 666 , 24.52 )
( 667 , 24.59 )
( 668 , 24.56 )
( 669 , 24.51 )
( 670 , 24.45 )
( 671 , 24.41 )
( 672 , 24.40 )
( 673 , 24.35 )
( 674 , 24.29 )
( 675 , 24.24 )
( 676 , 24.19 )
( 677 , 24.13 )
( 678 , 24.07 )
( 679 , 24.15 )
( 680 , 24.24 )
( 681 , 24.54 )
( 682 , 24.72 )
( 683 , 24.82 )
( 684 , 24.91 )
( 685 , 25.03 )
( 686 , 25.13 )
( 687 , 25.21 )
( 688 , 25.67 )
( 689 , 25.97 )
( 690 , 26.25 )
( 691 , 26.52 )
( 692 , 26.77 )
( 693 , 27.09 )
( 694 , 27.30 )
( 695 , 27.64 )
( 696 , 27.96 )
( 697 , 28.32 )
( 698 , 28.68 )
( 699 , 28.90 )
( 700 , 29.13 )
( 701 , 29.36 )
( 702 , 29.64 )
( 703 , 29.84 )
( 704 , 30.05 )
( 705 , 30.27 )
( 706 , 30.64 )
( 707 , 31.02 )
( 708 , 31.23 )
( 709 , 31.48 )
( 710 , 31.69 )
( 711 , 32.05 )
( 712 , 32.38 )
( 713 , 32.68 )
( 714 , 32.92 )
( 715 , 33.23 )
( 716 , 33.50 )
( 717 , 33.85 )
( 718 , 34.20 )
( 719 , 34.55 )
( 720 , 34.88 )
( 721 , 35.25 )
( 722 , 35.46 )
( 723 , 35.73 )
( 724 , 35.94 )
( 725 , 36.25 )
( 726 , 36.58 )
( 727 , 36.92 )
( 728 , 37.31 )
( 729 , 37.68 )
( 730 , 38.00 )
( 731 , 38.32 )
( 732 , 38.62 )
( 733 , 38.93 )
( 734 , 39.24 )
( 735 , 39.55 )
( 736 , 39.87 )
( 737 , 40.17 )
( 738 , 40.47 )
( 739 , 40.77 )
( 740 , 41.10 )
( 741 , 41.48 )
( 742 , 42.02 )
( 743 , 42.47 )
( 744 , 42.94 )
( 745 , 43.43 )
( 746 , 43.91 )
( 747 , 44.31 )
( 748 , 44.78 )
( 749 , 45.26 )
( 750 , 45.63 )
( 751 , 45.93 )
( 752 , 46.23 )
( 753 , 46.57 )
( 754 , 46.89 )
( 755 , 47.21 )
( 756 , 47.65 )
( 757 , 48.04 )
( 758 , 48.34 )
( 759 , 48.71 )
( 760 , 49.04 )
( 761 , 49.36 )
( 762 , 49.79 )
( 763 , 50.17 )
( 764 , 50.51 )
( 765 , 50.84 )
( 766 , 51.25 )
( 767 , 51.57 )
( 768 , 51.89 )
( 769 , 52.23 )
( 770 , 52.53 )
( 771 , 52.88 )
( 772 , 53.25 )
( 773 , 53.59 )
( 774 , 53.91 )
( 775 , 54.21 )
( 776 , 54.54 )
( 777 , 54.88 )
( 778 , 55.22 )
( 779 , 55.52 )
( 780 , 55.72 )
( 781 , 55.92 )
( 782 , 56.18 )
( 783 , 56.43 )
( 784 , 56.78 )
( 785 , 56.75 )
( 786 , 56.73 )
( 787 , 56.91 )
( 788 , 57.08 )
( 789 , 57.18 )
( 790 , 57.38 )
( 791 , 57.57 )
( 792 , 57.77 )
( 793 , 58.00 )
( 794 , 58.24 )
( 795 , 58.40 )
( 796 , 58.50 )
( 797 , 58.59 )
( 798 , 58.70 )
( 799 , 58.86 )
( 800 , 59.00 )
( 801 , 59.16 )
( 802 , 59.32 )
( 803 , 59.42 )
( 804 , 59.52 )
( 805 , 59.64 )
( 806 , 59.68 )
( 807 , 59.55 )
( 808 , 59.30 )
( 809 , 59.00 )
( 810 , 58.76 )
( 811 , 58.46 )
( 812 , 58.17 )
( 813 , 57.87 )
( 814 , 57.61 )
( 815 , 57.35 )
( 816 , 57.24 )
( 817 , 57.02 )
( 818 , 56.82 )
( 819 , 56.52 )
( 820 , 56.22 )
( 821 , 56.09 )
( 822 , 55.97 )
( 823 , 55.67 )
( 824 , 55.37 )
( 825 , 55.07 )
( 826 , 55.05 )
( 827 , 54.96 )
( 828 , 54.66 )
( 829 , 54.42 )
( 830 , 54.12 )
( 831 , 53.92 )
( 832 , 53.62 )
( 833 , 53.41 )
( 834 , 53.11 )
( 835 , 52.82 )
( 836 , 52.52 )
( 837 , 52.30 )
( 838 , 52.07 )
( 839 , 51.81 )
( 840 , 51.58 )
( 841 , 51.37 )
( 842 , 51.07 )
( 843 , 50.77 )
( 844 , 50.47 )
( 845 , 50.21 )
( 846 , 49.95 )
( 847 , 49.67 )
( 848 , 49.44 )
( 849 , 49.34 )
( 850 , 49.20 )
( 851 , 48.93 )
( 852 , 48.85 )
( 853 , 48.75 )
( 854 , 48.69 )
( 855 , 48.67 )
( 856 , 48.59 )
( 857 , 48.30 )
( 858 , 48.07 )
( 859 , 47.77 )
( 860 , 47.68 )
( 861 , 47.54 )
( 862 , 47.52 )
( 863 , 47.45 )
( 864 , 47.38 )
( 865 , 47.23 )
( 866 , 46.96 )
( 867 , 46.87 )
( 868 , 46.57 )
( 869 , 46.27 )
( 870 , 46.12 )
( 871 , 45.82 )
( 872 , 45.61 )
( 873 , 45.36 )
( 874 , 45.16 )
( 875 , 44.86 )
( 876 , 44.92 )
( 877 , 44.93 )
( 878 , 44.91 )
( 879 , 44.90 )
( 880 , 45.03 )
( 881 , 45.12 )
( 882 , 45.22 )
( 883 , 45.33 )
( 884 , 45.43 )
( 885 , 45.57 )
( 886 , 45.56 )
( 887 , 45.54 )
( 888 , 45.52 )
( 889 , 45.49 )
( 890 , 45.43 )
( 891 , 45.38 )
( 892 , 45.32 )
( 893 , 45.26 )
( 894 , 45.32 )
( 895 , 45.43 )
( 896 , 45.50 )
( 897 , 45.44 )
( 898 , 45.38 )
( 899 , 45.29 )
( 900 , 45.16 )
( 901 , 45.04 )
( 902 , 44.99 )
( 903 , 44.86 )
( 904 , 44.74 )
( 905 , 44.62 )
( 906 , 44.62 )
( 907 , 44.52 )
( 908 , 44.41 )
( 909 , 44.35 )
( 910 , 44.23 )
( 911 , 44.43 )
( 912 , 44.64 )
( 913 , 44.84 )
( 914 , 45.06 )
( 915 , 45.24 )
( 916 , 45.45 )
( 917 , 45.69 )
( 918 , 45.98 )
( 919 , 46.39 )
( 920 , 46.87 )
( 921 , 47.26 )
( 922 , 47.65 )
( 923 , 48.11 )
( 924 , 48.51 )
( 925 , 48.91 )
( 926 , 49.33 )
( 927 , 49.76 )
( 928 , 50.18 )
( 929 , 50.64 )
( 930 , 51.04 )
( 931 , 51.43 )
( 932 , 51.72 )
( 933 , 52.09 )
( 934 , 52.20 )
( 935 , 52.30 )
( 936 , 52.02 )
( 937 , 51.96 )
( 938 , 51.91 )
( 939 , 51.89 )
( 940 , 51.75 )
( 941 , 51.60 )
( 942 , 51.37 )
( 943 , 51.14 )
( 944 , 50.84 )
( 945 , 50.55 )
( 946 , 50.26 )
( 947 , 50.05 )
( 948 , 49.77 )
( 949 , 49.46 )
( 950 , 49.27 )
( 951 , 48.97 )
( 952 , 48.73 )
( 953 , 48.43 )
( 954 , 48.12 )
( 955 , 47.98 )
( 956 , 47.84 )
( 957 , 47.54 )
( 958 , 47.23 )
( 959 , 46.93 )
( 960 , 46.65 )
( 961 , 46.35 )
( 962 , 46.15 )
( 963 , 45.96 )
( 964 , 45.83 )
( 965 , 45.64 )
( 966 , 45.44 )
( 967 , 45.25 )
( 968 , 44.96 )
( 969 , 44.84 )
( 970 , 44.78 )
( 971 , 44.48 )
( 972 , 44.30 )
( 973 , 44.00 )
( 974 , 43.70 )
( 975 , 43.61 )
( 976 , 43.62 )
( 977 , 43.57 )
( 978 , 43.48 )
( 979 , 43.18 )
( 980 , 43.10 )
( 981 , 42.81 )
( 982 , 42.55 )
( 983 , 42.25 )
( 984 , 42.32 )
( 985 , 42.21 )
( 986 , 42.11 )
( 987 , 42.09 )
( 988 , 41.90 )
( 989 , 41.86 )
( 990 , 41.72 )
( 991 , 41.57 )
( 992 , 41.46 )
( 993 , 41.19 )
( 994 , 40.91 )
( 995 , 40.72 )
( 996 , 40.45 )
( 997 , 40.21 )
( 998 , 40.15 )
( 999 , 39.87 )
( 1000 , 39.57 )
( 1001 , 39.27 )
( 1002 , 38.97 )
( 1003 , 38.68 )
( 1004 , 38.38 )
( 1005 , 38.08 )
( 1006 , 38.11 )
( 1007 , 38.05 )
( 1008 , 38.02 )
( 1009 , 38.00 )
( 1010 , 37.97 )
( 1011 , 38.00 )
( 1012 , 37.98 )
( 1013 , 37.95 )
( 1014 , 38.20 )
( 1015 , 38.38 )
( 1016 , 38.55 )
( 1017 , 38.83 )
( 1018 , 39.10 )
( 1019 , 39.38 )
( 1020 , 39.55 )
( 1021 , 39.84 )
( 1022 , 40.08 )
( 1023 , 40.34 )
( 1024 , 40.62 )
( 1025 , 40.88 )
( 1026 , 41.11 )
( 1027 , 41.34 )
( 1028 , 41.57 )
( 1029 , 41.80 )
( 1030 , 42.02 )
( 1031 , 42.33 )
( 1032 , 42.59 )
( 1033 , 42.86 )
( 1034 , 43.09 )
( 1035 , 43.30 )
( 1036 , 43.51 )
( 1037 , 43.74 )
( 1038 , 43.95 )
( 1039 , 44.24 )
( 1040 , 44.46 )
( 1041 , 44.69 )
( 1042 , 44.90 )
( 1043 , 45.16 )
( 1044 , 45.32 )
( 1045 , 45.45 )
( 1046 , 45.66 )
( 1047 , 45.87 )
( 1048 , 46.11 )
( 1049 , 46.36 )
( 1050 , 46.61 )
( 1051 , 46.91 )
( 1052 , 47.04 )
( 1053 , 47.16 )
( 1054 , 47.36 )
( 1055 , 47.48 )
( 1056 , 47.61 )
( 1057 , 47.77 )
( 1058 , 47.90 )
( 1059 , 48.12 )
( 1060 , 48.29 )
( 1061 , 48.59 )
( 1062 , 48.86 )
( 1063 , 49.16 )
( 1064 , 49.32 )
( 1065 , 49.45 )
( 1066 , 49.57 )
( 1067 , 49.70 )
( 1068 , 49.93 )
( 1069 , 50.15 )
( 1070 , 50.33 )
( 1071 , 50.54 )
( 1072 , 50.66 )
( 1073 , 50.79 )
( 1074 , 50.96 )
( 1075 , 51.18 )
( 1076 , 51.38 )
( 1077 , 51.25 )
( 1078 , 50.95 )
( 1079 , 50.75 )
( 1080 , 50.71 )
( 1081 , 50.61 )
( 1082 , 50.61 )
( 1083 , 50.61 )
( 1084 , 50.59 )
( 1085 , 50.49 )
( 1086 , 50.39 )
( 1087 , 50.30 )
( 1088 , 50.00 )
( 1089 , 49.86 )
( 1090 , 49.71 )
( 1091 , 49.47 )
( 1092 , 49.32 )
( 1093 , 49.28 )
( 1094 , 49.20 )
( 1095 , 49.12 )
( 1096 , 49.03 )
( 1097 , 48.93 )
( 1098 , 48.87 )
( 1099 , 48.89 )
( 1100 , 48.91 )
( 1101 , 49.09 )
( 1102 , 49.16 )
( 1103 , 49.29 )
( 1104 , 49.37 )
( 1105 , 49.40 )
( 1106 , 49.36 )
( 1107 , 49.13 )
( 1108 , 49.04 )
( 1109 , 48.95 )
( 1110 , 48.80 )
( 1111 , 48.75 )
( 1112 , 48.64 )
( 1113 , 48.52 )
( 1114 , 48.39 )
( 1115 , 48.33 )
( 1116 , 48.43 )
( 1117 , 48.32 )
( 1118 , 48.06 )
( 1119 , 47.80 )
( 1120 , 47.50 )
( 1121 , 47.20 )
( 1122 , 47.10 )
( 1123 , 47.03 )
( 1124 , 46.73 )
( 1125 , 46.43 )
( 1126 , 46.13 )
( 1127 , 45.84 )
( 1128 , 45.69 )
( 1129 , 45.45 )
( 1130 , 45.16 )
( 1131 , 45.14 )
( 1132 , 45.10 )
( 1133 , 45.00 )
( 1134 , 44.90 )
( 1135 , 44.60 )
( 1136 , 44.46 )
( 1137 , 44.19 )
( 1138 , 43.91 )
( 1139 , 43.61 )
( 1140 , 43.30 )
( 1141 , 43.00 )
( 1142 , 42.85 )
( 1143 , 42.57 )
( 1144 , 42.28 )
( 1145 , 42.00 )
( 1146 , 41.79 )
( 1147 , 41.70 )
( 1148 , 41.66 )
( 1149 , 41.68 )
( 1150 , 41.46 )
( 1151 , 41.16 )
( 1152 , 41.02 )
( 1153 , 40.89 )
( 1154 , 40.59 )
( 1155 , 40.29 )
( 1156 , 40.05 )
( 1157 , 39.75 )
( 1158 , 39.51 )
( 1159 , 39.21 )
( 1160 , 39.00 )
( 1161 , 38.70 )
( 1162 , 38.40 )
( 1163 , 38.10 )
( 1164 , 37.95 )
( 1165 , 37.71 )
( 1166 , 37.75 )
( 1167 , 37.84 )
( 1168 , 37.80 )
( 1169 , 37.55 )
( 1170 , 37.29 )
( 1171 , 37.03 )
( 1172 , 36.80 )
( 1173 , 36.52 )
( 1174 , 36.46 )
( 1175 , 36.40 )
( 1176 , 36.34 )
( 1177 , 36.28 )
( 1178 , 35.99 )
( 1179 , 35.84 )
( 1180 , 35.55 )
( 1181 , 35.25 )
( 1182 , 34.95 )
( 1183 , 34.71 )
( 1184 , 34.41 )
( 1185 , 34.56 )
( 1186 , 34.69 )
( 1187 , 34.86 )
( 1188 , 35.07 )
( 1189 , 35.22 )
( 1190 , 35.22 )
( 1191 , 35.20 )
( 1192 , 35.19 )
( 1193 , 35.36 )
( 1194 , 35.36 )
( 1195 , 35.58 )
( 1196 , 35.80 )
( 1197 , 36.04 )
( 1198 , 36.25 )
( 1199 , 36.55 )
( 1200 , 36.81 )
( 1201 , 37.07 )
( 1202 , 37.33 )
( 1203 , 37.57 )
( 1204 , 37.82 )
( 1205 , 38.03 )
( 1206 , 38.23 )
( 1207 , 38.43 )
( 1208 , 38.63 )
( 1209 , 38.95 )
( 1210 , 39.22 )
( 1211 , 39.43 )
( 1212 , 39.63 )
( 1213 , 39.95 )
( 1214 , 40.28 )
( 1215 , 40.69 )
( 1216 , 40.95 )
( 1217 , 41.23 )
( 1218 , 41.50 )
( 1219 , 41.83 )
( 1220 , 42.10 )
( 1221 , 42.36 )
( 1222 , 42.65 )
( 1223 , 42.93 )
( 1224 , 43.24 )
( 1225 , 43.53 )
( 1226 , 43.80 )
( 1227 , 44.12 )
( 1228 , 44.38 )
( 1229 , 44.70 )
( 1230 , 44.96 )
( 1231 , 45.21 )
( 1232 , 45.47 )
( 1233 , 45.74 )
( 1234 , 46.00 )
( 1235 , 45.98 )
( 1236 , 46.00 )
( 1237 , 45.98 )
( 1238 , 45.96 )
( 1239 , 45.95 )
( 1240 , 45.93 )
( 1241 , 46.05 )
( 1242 , 46.27 )
( 1243 , 46.30 )
( 1244 , 46.29 )
( 1245 , 46.28 )
( 1246 , 46.26 )
( 1247 , 46.32 )
( 1248 , 46.32 )
( 1249 , 46.33 )
( 1250 , 46.32 )
( 1251 , 46.43 )
( 1252 , 46.42 )
( 1253 , 46.65 )
( 1254 , 46.97 )
( 1255 , 47.14 )
( 1256 , 47.28 )
( 1257 , 47.41 )
( 1258 , 47.54 )
( 1259 , 47.73 )
( 1260 , 47.89 )
( 1261 , 47.99 )
( 1262 , 48.15 )
( 1263 , 48.40 )
( 1264 , 48.50 )
( 1265 , 48.60 )
( 1266 , 48.71 )
( 1267 , 48.80 )
( 1268 , 48.96 )
( 1269 , 49.09 )
( 1270 , 49.19 )
( 1271 , 49.29 )
( 1272 , 49.53 )
( 1273 , 49.71 )
( 1274 , 49.88 )
( 1275 , 50.05 )
( 1276 , 50.20 )
( 1277 , 50.20 )
( 1278 , 50.20 )
( 1279 , 50.19 )
( 1280 , 50.24 )
( 1281 , 50.28 )
( 1282 , 50.25 )
( 1283 , 50.31 )
( 1284 , 50.32 )
( 1285 , 50.34 )
( 1286 , 50.32 )
( 1287 , 50.36 )
( 1288 , 50.41 )
( 1289 , 50.38 )
( 1290 , 50.36 )
( 1291 , 50.33 )
( 1292 , 50.20 )
( 1293 , 50.08 )
( 1294 , 50.10 )
( 1295 , 50.24 )
( 1296 , 50.41 )
( 1297 , 50.54 )
( 1298 , 50.64 )
( 1299 , 50.89 )
( 1300 , 50.99 )
( 1301 , 51.09 )
( 1302 , 51.20 )
( 1303 , 51.38 )
( 1304 , 51.49 )
( 1305 , 51.60 )
( 1306 , 51.73 )
( 1307 , 51.86 )
( 1308 , 51.96 )
( 1309 , 52.05 )
( 1310 , 52.17 )
( 1311 , 52.28 )
( 1312 , 52.39 )
( 1313 , 52.54 )
( 1314 , 52.64 )
( 1315 , 52.73 )
( 1316 , 52.89 )
( 1317 , 53.10 )
( 1318 , 53.29 )
( 1319 , 53.46 )
( 1320 , 53.80 )
( 1321 , 54.16 )
( 1322 , 54.50 )
( 1323 , 54.72 )
( 1324 , 54.95 )
( 1325 , 55.17 )
( 1326 , 55.43 )
( 1327 , 55.69 )
( 1328 , 55.93 )
( 1329 , 56.15 )
( 1330 , 56.54 )
( 1331 , 56.90 )
( 1332 , 57.27 )
( 1333 , 57.63 )
( 1334 , 57.91 )
( 1335 , 58.16 )
( 1336 , 58.38 )
( 1337 , 58.40 )
( 1338 , 58.46 )
( 1339 , 58.54 )
( 1340 , 58.53 )
( 1341 , 58.47 )
( 1342 , 58.41 )
( 1343 , 58.33 )
( 1344 , 58.21 )
( 1345 , 58.12 )
( 1346 , 58.00 )
( 1347 , 58.00 )
( 1348 , 58.07 )
( 1349 , 58.06 )
( 1350 , 58.01 )
( 1351 , 57.95 )
( 1352 , 57.96 )
( 1353 , 58.00 )
( 1354 , 58.06 )
( 1355 , 58.07 )
( 1356 , 58.07 )
( 1357 , 58.12 )
( 1358 , 58.12 )
( 1359 , 58.12 )
( 1360 , 58.12 )
( 1361 , 58.14 )
( 1362 , 58.16 )
( 1363 , 58.17 )
( 1364 , 58.17 )
( 1365 , 58.19 )
( 1366 , 58.41 )
( 1367 , 58.63 )
( 1368 , 58.91 )
( 1369 , 59.13 )
( 1370 , 59.42 )
( 1371 , 59.67 )
( 1372 , 59.89 )
( 1373 , 60.11 )
( 1374 , 60.34 )
( 1375 , 60.56 )
( 1376 , 60.78 )
( 1377 , 61.20 )
( 1378 , 61.65 )
( 1379 , 62.10 )
( 1380 , 62.51 )
( 1381 , 62.84 )
( 1382 , 62.88 )
( 1383 , 62.98 )
( 1384 , 63.02 )
( 1385 , 63.13 )
( 1386 , 63.20 )
( 1387 , 63.29 )
( 1388 , 63.33 )
( 1389 , 63.36 )
( 1390 , 63.40 )
( 1391 , 63.49 )
( 1392 , 63.74 )
( 1393 , 64.02 )
( 1394 , 64.02 )
( 1395 , 64.02 )
( 1396 , 64.02 )
( 1397 , 64.07 )
( 1398 , 64.12 )
( 1399 , 64.14 )
( 1400 , 64.14 )
( 1401 , 64.36 )
( 1402 , 64.57 )
( 1403 , 64.72 )
( 1404 , 64.76 )
( 1405 , 64.85 )
( 1406 , 64.85 )
( 1407 , 64.86 )
( 1408 , 64.86 )
( 1409 , 64.86 )
( 1410 , 64.88 )
( 1411 , 64.89 )
( 1412 , 65.02 )
( 1413 , 65.16 )
( 1414 , 65.27 )
( 1415 , 65.38 )
( 1416 , 65.48 )
( 1417 , 65.60 )
( 1418 , 65.70 )
( 1419 , 65.80 )
( 1420 , 65.95 )
( 1421 , 66.12 )
( 1422 , 66.30 )
( 1423 , 66.44 )
( 1424 , 66.60 )
( 1425 , 66.70 )
( 1426 , 66.82 )
( 1427 , 66.92 )
( 1428 , 67.09 )
( 1429 , 67.26 )
( 1430 , 67.38 )
( 1431 , 67.53 )
( 1432 , 67.63 )
( 1433 , 67.64 )
( 1434 , 67.63 )
( 1435 , 67.62 )
( 1436 , 67.62 )
( 1437 , 67.62 )
( 1438 , 67.78 )
( 1439 , 67.91 )
( 1440 , 68.03 )
( 1441 , 68.07 )
( 1442 , 68.12 )
( 1443 , 68.21 )
( 1444 , 68.20 )
( 1445 , 68.39 )
( 1446 , 68.65 )
( 1447 , 69.00 )
( 1448 , 69.35 )
( 1449 , 69.73 )
( 1450 , 70.10 )
( 1451 , 70.45 )
( 1452 , 70.81 )
( 1453 , 71.26 )
( 1454 , 71.57 )
( 1455 , 71.92 )
( 1456 , 72.27 )
( 1457 , 72.56 )
( 1458 , 72.87 )
( 1459 , 73.14 )
( 1460 , 73.23 )
( 1461 , 73.30 )
( 1462 , 73.36 )
( 1463 , 73.25 )
( 1464 , 73.38 )
( 1465 , 73.51 )
( 1466 , 73.64 )
( 1467 , 73.83 )
( 1468 , 74.01 )
( 1469 , 73.94 )
( 1470 , 73.81 )
( 1471 , 73.69 )
( 1472 , 73.48 )
( 1473 , 73.28 )
( 1474 , 73.12 )
( 1475 , 72.87 )
( 1476 , 72.61 )
( 1477 , 72.38 )
( 1478 , 72.15 )
( 1479 , 71.84 )
( 1480 , 71.55 )
( 1481 , 71.26 )
( 1482 , 71.13 )
( 1483 , 70.87 )
( 1484 , 70.56 )
( 1485 , 70.59 )
( 1486 , 70.53 )
( 1487 , 70.55 )
( 1488 , 70.71 )
( 1489 , 70.73 )
( 1490 , 70.78 )
( 1491 , 70.86 )
( 1492 , 70.91 )
( 1493 , 70.98 )
( 1494 , 70.92 )
( 1495 , 70.80 )
( 1496 , 70.76 )
( 1497 , 70.69 )
( 1498 , 70.62 )
( 1499 , 70.52 )
( 1500 , 70.42 )
( 1501 , 70.30 )
( 1502 , 70.19 )
( 1503 , 70.18 )
( 1504 , 70.05 )
( 1505 , 69.95 )
( 1506 , 69.85 )
( 1507 , 69.77 )
( 1508 , 69.68 )
( 1509 , 69.84 )
( 1510 , 70.05 )
( 1511 , 70.22 )
( 1512 , 70.38 )
( 1513 , 70.62 )
( 1514 , 70.94 )
( 1515 , 71.20 )
( 1516 , 71.30 )
( 1517 , 71.43 )
( 1518 , 71.55 )
( 1519 , 71.65 )
( 1520 , 71.79 )
( 1521 , 71.89 )
( 1522 , 72.09 )
( 1523 , 72.19 )
( 1524 , 72.28 )
( 1525 , 72.41 )
( 1526 , 72.52 )
( 1527 , 72.62 )
( 1528 , 72.73 )
( 1529 , 72.83 )
( 1530 , 72.99 )
( 1531 , 73.12 )
( 1532 , 73.25 )
( 1533 , 73.38 )
( 1534 , 73.49 )
( 1535 , 73.52 )
( 1536 , 73.55 )
( 1537 , 73.57 )
( 1538 , 73.30 )
( 1539 , 73.00 )
( 1540 , 72.70 )
( 1541 , 72.41 )
( 1542 , 72.15 )
( 1543 , 71.85 )
( 1544 , 71.62 )
( 1545 , 71.34 )
( 1546 , 71.07 )
( 1547 , 70.91 )
( 1548 , 70.62 )
( 1549 , 70.47 )
( 1550 , 70.17 )
( 1551 , 69.88 )
( 1552 , 69.83 )
( 1553 , 69.64 )
( 1554 , 69.48 )
( 1555 , 69.20 )
( 1556 , 69.06 )
( 1557 , 68.91 )
( 1558 , 68.87 )
( 1559 , 68.82 )
( 1560 , 68.84 )
( 1561 , 68.70 )
( 1562 , 68.41 )
( 1563 , 68.12 )
( 1564 , 67.92 )
( 1565 , 67.62 )
( 1566 , 67.32 )
( 1567 , 67.03 )
( 1568 , 66.73 )
( 1569 , 66.46 )
( 1570 , 66.34 )
( 1571 , 66.21 )
( 1572 , 65.91 )
( 1573 , 65.82 )
( 1574 , 65.67 )
( 1575 , 65.41 )
( 1576 , 65.23 )
( 1577 , 65.10 )
( 1578 , 64.91 )
( 1579 , 64.76 )
( 1580 , 64.77 )
( 1581 , 64.69 )
( 1582 , 64.39 )
( 1583 , 64.09 )
( 1584 , 64.02 )
( 1585 , 63.93 )
( 1586 , 63.84 )
( 1587 , 63.74 )
( 1588 , 63.64 )
( 1589 , 63.55 )
( 1590 , 63.34 )
( 1591 , 63.08 )
( 1592 , 62.78 )
( 1593 , 62.80 )
( 1594 , 62.71 )
( 1595 , 62.41 )
( 1596 , 62.35 )
( 1597 , 62.45 )
( 1598 , 62.57 )
( 1599 , 62.66 )
( 1600 , 62.73 )
( 1601 , 62.79 )
( 1602 , 62.64 )
( 1603 , 62.60 )
( 1604 , 62.46 )
( 1605 , 62.32 )
( 1606 , 62.03 )
( 1607 , 61.73 )
( 1608 , 61.43 )
( 1609 , 61.13 )
( 1610 , 60.89 )
( 1611 , 60.61 )
( 1612 , 60.35 )
( 1613 , 60.05 )
( 1614 , 59.75 )
( 1615 , 59.46 )
( 1616 , 59.16 )
( 1617 , 58.86 )
( 1618 , 58.59 )
( 1619 , 58.53 )
( 1620 , 58.23 )
( 1621 , 57.93 )
( 1622 , 57.63 )
( 1623 , 57.64 )
( 1624 , 57.55 )
( 1625 , 57.27 )
( 1626 , 56.98 )
( 1627 , 56.84 )
( 1628 , 56.56 )
( 1629 , 56.26 )
( 1630 , 55.96 )
( 1631 , 55.82 )
( 1632 , 55.67 )
( 1633 , 55.49 )
( 1634 , 55.22 )
( 1635 , 54.99 )
( 1636 , 54.84 )
( 1637 , 54.73 )
( 1638 , 54.54 )
( 1639 , 54.24 )
( 1640 , 53.94 )
( 1641 , 53.84 )
( 1642 , 53.65 )
( 1643 , 53.45 )
( 1644 , 53.23 )
( 1645 , 52.94 )
( 1646 , 52.79 )
( 1647 , 52.64 )
( 1648 , 52.40 )
( 1649 , 52.10 )
( 1650 , 51.80 )
( 1651 , 51.50 )
( 1652 , 51.33 )
( 1653 , 51.23 )
( 1654 , 51.26 )
( 1655 , 51.13 )
( 1656 , 50.83 )
( 1657 , 50.57 )
( 1658 , 50.38 )
( 1659 , 50.32 )
( 1660 , 50.04 )
( 1661 , 49.78 )
( 1662 , 49.48 )
( 1663 , 49.31 )
( 1664 , 49.01 )
( 1665 , 48.71 )
( 1666 , 48.42 )
( 1667 , 48.12 )
( 1668 , 47.82 )
( 1669 , 47.52 )
( 1670 , 47.38 )
( 1671 , 47.08 )
( 1672 , 46.86 )
( 1673 , 46.59 )
( 1674 , 46.46 )
( 1675 , 46.40 )
( 1676 , 46.45 )
( 1677 , 46.43 )
( 1678 , 46.13 )
( 1679 , 45.94 )
( 1680 , 45.65 )
( 1681 , 45.38 )
( 1682 , 45.25 )
( 1683 , 44.96 )
( 1684 , 44.67 )
( 1685 , 44.49 )
( 1686 , 44.20 )
( 1687 , 43.96 )
( 1688 , 43.66 )
( 1689 , 43.36 )
( 1690 , 43.06 )
( 1691 , 42.76 )
( 1692 , 42.46 )
( 1693 , 42.18 )
( 1694 , 41.91 )
( 1695 , 41.61 )
( 1696 , 41.31 )
( 1697 , 41.02 )
( 1698 , 40.96 )
( 1699 , 40.66 )
( 1700 , 40.37 )
( 1701 , 40.16 )
( 1702 , 39.86 )
( 1703 , 39.57 )
( 1704 , 39.27 )
( 1705 , 39.04 )
( 1706 , 38.78 )
( 1707 , 38.70 )
( 1708 , 38.60 )
( 1709 , 38.32 )
( 1710 , 38.23 )
( 1711 , 37.97 )
( 1712 , 37.67 )
( 1713 , 37.46 )
( 1714 , 37.16 )
( 1715 , 37.02 )
( 1716 , 36.72 )
( 1717 , 36.42 )
( 1718 , 36.29 )
( 1719 , 36.25 )
( 1720 , 36.12 )
( 1721 , 36.02 )
( 1722 , 35.72 )
( 1723 , 35.42 )
( 1724 , 35.36 )
( 1725 , 35.16 )
( 1726 , 34.86 )
( 1727 , 34.56 )
( 1728 , 34.44 )
( 1729 , 34.31 )
( 1730 , 34.59 )
( 1731 , 34.79 )
( 1732 , 34.92 )
( 1733 , 35.04 )
( 1734 , 35.17 )
( 1735 , 35.22 )
( 1736 , 35.14 )
( 1737 , 35.04 )
( 1738 , 34.93 )
( 1739 , 34.82 )
( 1740 , 34.69 )
( 1741 , 34.45 )
( 1742 , 34.16 )
( 1743 , 34.02 )
( 1744 , 33.96 )
( 1745 , 33.78 )
( 1746 , 33.48 )
( 1747 , 33.43 )
( 1748 , 33.25 )
( 1749 , 33.07 )
( 1750 , 32.77 )
( 1751 , 32.47 )
( 1752 , 32.17 )
( 1753 , 32.20 )
( 1754 , 31.90 )
( 1755 , 31.61 )
( 1756 , 31.50 )
( 1757 , 31.62 )
( 1758 , 31.74 )
( 1759 , 31.73 )
( 1760 , 31.53 )
( 1761 , 31.23 )
( 1762 , 30.93 )
( 1763 , 30.83 )
( 1764 , 30.53 )
( 1765 , 30.23 )
( 1766 , 29.93 )
( 1767 , 29.66 )
( 1768 , 29.37 )
( 1769 , 29.45 )
( 1770 , 29.39 )
( 1771 , 29.33 )
( 1772 , 29.03 )
( 1773 , 28.72 )
( 1774 , 28.43 )
( 1775 , 28.15 )
( 1776 , 27.88 )
( 1777 , 27.63 )
( 1778 , 27.54 )
( 1779 , 27.46 )
( 1780 , 27.16 )
( 1781 , 26.88 )
( 1782 , 26.65 )
( 1783 , 26.51 )
( 1784 , 26.27 )
( 1785 , 26.07 )
( 1786 , 25.86 )
( 1787 , 25.55 )
( 1788 , 25.25 )
( 1789 , 25.06 )
( 1790 , 24.85 )
( 1791 , 24.55 )
( 1792 , 24.54 )
( 1793 , 24.41 )
( 1794 , 24.29 )
( 1795 , 24.17 )
( 1796 , 24.04 )
( 1797 , 24.02 )
( 1798 , 23.99 )
( 1799 , 24.18 )
( 1800 , 24.35 )
( 1801 , 24.53 )
( 1802 , 24.74 )
( 1803 , 24.98 )
( 1804 , 25.21 )
( 1805 , 25.45 )
( 1806 , 25.68 )
( 1807 , 25.86 )
( 1808 , 25.97 )
( 1809 , 26.03 )
( 1810 , 25.94 )
( 1811 , 25.84 )
( 1812 , 25.71 )
( 1813 , 25.47 )
( 1814 , 25.23 )
( 1815 , 25.08 )
( 1816 , 24.79 )
( 1817 , 24.60 )
( 1818 , 24.54 )
( 1819 , 24.63 )
( 1820 , 24.35 )
( 1821 , 24.11 )
( 1822 , 23.88 )
( 1823 , 23.58 )
( 1824 , 23.62 )
( 1825 , 23.64 )
( 1826 , 23.58 )
( 1827 , 23.51 )
( 1828 , 23.41 )
( 1829 , 23.22 )
( 1830 , 22.93 )
( 1831 , 22.70 )
( 1832 , 22.43 )
( 1833 , 22.15 )
( 1834 , 21.85 )
( 1835 , 21.62 )
( 1836 , 21.51 )
( 1837 , 21.30 )
( 1838 , 21.00 )
( 1839 , 20.88 )
( 1840 , 21.00 )
( 1841 , 21.14 )
( 1842 , 21.31 )
( 1843 , 21.44 )
( 1844 , 21.65 )
( 1845 , 21.91 )
( 1846 , 22.08 )
( 1847 , 22.21 )
( 1848 , 22.41 )
( 1849 , 22.60 )
( 1850 , 22.79 )
( 1851 , 22.97 )
( 1852 , 23.16 )
( 1853 , 23.35 )
( 1854 , 23.47 )
( 1855 , 23.68 )
( 1856 , 23.88 )
( 1857 , 24.04 )
( 1858 , 24.17 )
( 1859 , 24.05 )
( 1860 , 23.94 )
( 1861 , 23.81 )
( 1862 , 23.75 )
( 1863 , 23.88 )
( 1864 , 23.85 )
( 1865 , 23.81 )
( 1866 , 23.85 )
( 1867 , 23.89 )
( 1868 , 23.81 )
( 1869 , 23.69 )
( 1870 , 23.57 )
( 1871 , 23.46 )
( 1872 , 23.42 )
( 1873 , 23.39 )
( 1874 , 23.26 )
( 1875 , 23.14 )
( 1876 , 23.04 )
( 1877 , 22.74 )
( 1878 , 22.44 )
( 1879 , 22.15 )
( 1880 , 21.96 )
( 1881 , 21.91 )
( 1882 , 21.81 )
( 1883 , 21.69 )
( 1884 , 21.38 )
( 1885 , 21.08 )
( 1886 , 20.79 )
( 1887 , 20.70 )
( 1888 , 20.61 )
( 1889 , 20.31 )
( 1890 , 20.05 )
( 1891 , 19.79 )
( 1892 , 19.53 )
( 1893 , 19.30 )
( 1894 , 19.07 )
( 1895 , 18.78 )
( 1896 , 18.52 )
( 1897 , 18.48 )
( 1898 , 18.20 )
( 1899 , 17.90 )
( 1900 , 17.69 )
( 1901 , 17.47 )
( 1902 , 17.29 )
( 1903 , 16.99 )
( 1904 , 16.69 )
( 1905 , 16.46 )
( 1906 , 16.19 )
( 1907 , 15.93 )
( 1908 , 15.72 )
( 1909 , 15.42 )
( 1910 , 15.34 )
( 1911 , 15.20 )
( 1912 , 14.97 )
( 1913 , 14.74 )
( 1914 , 14.73 )
( 1915 , 14.66 )
( 1916 , 14.45 )
( 1917 , 14.14 )
( 1918 , 13.87 )
( 1919 , 13.72 )
( 1920 , 13.42 )
( 1921 , 13.21 )
( 1922 , 12.98 )
( 1923 , 13.00 )
( 1924 , 12.85 )
( 1925 , 12.61 )
( 1926 , 12.30 )
( 1927 , 12.07 )
( 1928 , 11.77 )
( 1929 , 11.94 )
( 1930 , 12.03 )
( 1931 , 12.13 )
( 1932 , 12.23 )
( 1933 , 12.28 )
( 1934 , 12.17 )
( 1935 , 12.56 )
( 1936 , 12.91 )
( 1937 , 13.23 )
( 1938 , 13.61 )
( 1939 , 13.98 )
( 1940 , 14.36 )
( 1941 , 14.69 )
( 1942 , 14.91 )
( 1943 , 15.12 )
( 1944 , 15.39 )
( 1945 , 15.66 )
( 1946 , 15.88 )
( 1947 , 16.12 )
( 1948 , 16.34 )
( 1949 , 16.70 )
( 1950 , 16.97 )
( 1951 , 17.23 )
( 1952 , 17.52 )
( 1953 , 17.79 )
( 1954 , 17.99 )
( 1955 , 18.26 )
( 1956 , 18.46 )
( 1957 , 18.78 )
( 1958 , 18.98 )
( 1959 , 19.24 )
( 1960 , 19.60 )
( 1961 , 19.92 )
( 1962 , 20.18 )
( 1963 , 20.46 )
( 1964 , 20.72 )
( 1965 , 20.86 )
( 1966 , 20.77 )
( 1967 , 20.76 )
( 1968 , 20.72 )
( 1969 , 20.60 )
( 1970 , 20.53 )
( 1971 , 20.43 )
( 1972 , 20.39 )
( 1973 , 20.27 )
( 1974 , 20.43 )
( 1975 , 20.57 )
( 1976 , 20.70 )
( 1977 , 20.93 )
( 1978 , 21.06 )
( 1979 , 21.19 )
( 1980 , 21.42 )
( 1981 , 21.54 )
( 1982 , 21.67 )
( 1983 , 21.80 )
( 1984 , 21.68 )
( 1985 , 21.56 )
( 1986 , 21.43 )
( 1987 , 21.63 )
( 1988 , 21.54 )
( 1989 , 21.44 )
( 1990 , 21.33 )
( 1991 , 21.27 )
( 1992 , 21.25 )
( 1993 , 21.31 )
( 1994 , 21.56 )
( 1995 , 21.77 )
( 1996 , 21.97 )
( 1997 , 22.14 )
( 1998 , 22.31 )
( 1999 , 22.53 )
( 2000 , 22.65 )
( 2001 , 22.57 )
( 2002 , 22.45 )
( 2003 , 22.34 )
( 2004 , 22.33 )
( 2005 , 22.20 )
( 2006 , 22.10 )
( 2007 , 21.99 )
( 2008 , 21.92 )
( 2009 , 22.04 )
( 2010 , 21.94 )
( 2011 , 21.82 )
( 2012 , 21.69 )
( 2013 , 21.57 )
( 2014 , 21.44 )
( 2015 , 21.37 )
( 2016 , 21.25 )
( 2017 , 21.13 )
( 2018 , 21.00 )
( 2019 , 21.13 )
( 2020 , 21.01 )
( 2021 , 20.90 )
( 2022 , 20.77 )
( 2023 , 20.67 )
( 2024 , 20.55 )
( 2025 , 20.49 )
( 2026 , 20.43 )
( 2027 , 20.31 )
( 2028 , 20.21 )
( 2029 , 20.15 )
( 2030 , 20.10 )
( 2031 , 20.05 )
( 2032 , 20.00 )
( 2033 , 19.97 )
( 2034 , 19.92 )
( 2035 , 19.62 )
( 2036 , 19.81 )
( 2037 , 19.91 )
( 2038 , 20.15 )
( 2039 , 20.37 )
( 2040 , 20.50 )
( 2041 , 20.59 )
( 2042 , 20.85 )
( 2043 , 21.05 )
( 2044 , 21.15 )
( 2045 , 21.27 )
( 2046 , 21.40 )
( 2047 , 21.56 )
( 2048 , 21.74 )
( 2049 , 22.02 )
( 2050 , 22.19 )
( 2051 , 22.44 )
( 2052 , 22.69 )
( 2053 , 22.95 )
( 2054 , 23.12 )
( 2055 , 23.41 )
( 2056 , 23.74 )
( 2057 , 23.95 )
( 2058 , 24.21 )
( 2059 , 24.41 )
( 2060 , 24.64 )
( 2061 , 24.92 )
( 2062 , 25.14 )
( 2063 , 25.36 )
( 2064 , 25.59 )
( 2065 , 25.82 )
( 2066 , 26.09 )
( 2067 , 26.31 )
( 2068 , 26.58 )
( 2069 , 26.86 )
( 2070 , 27.09 )
( 2071 , 27.35 )
( 2072 , 27.56 )
( 2073 , 27.78 )
( 2074 , 27.99 )
( 2075 , 28.23 )
( 2076 , 28.44 )
( 2077 , 28.65 )
( 2078 , 28.99 )
( 2079 , 29.35 )
( 2080 , 29.30 )
( 2081 , 29.24 )
( 2082 , 29.26 )
( 2083 , 29.22 )
( 2084 , 29.20 )
( 2085 , 29.14 )
( 2086 , 29.08 )
( 2087 , 29.03 )
( 2088 , 29.05 )
( 2089 , 29.04 )
( 2090 , 29.02 )
( 2091 , 29.10 )
( 2092 , 29.04 )
( 2093 , 29.00 )
( 2094 , 28.95 )
( 2095 , 28.82 )
( 2096 , 28.70 )
( 2097 , 28.74 )
( 2098 , 28.62 )
( 2099 , 28.50 )
( 2100 , 28.37 )
( 2101 , 28.25 )
( 2102 , 28.19 )
( 2103 , 28.07 )
( 2104 , 27.95 )
( 2105 , 27.95 )
( 2106 , 27.99 )
( 2107 , 28.09 )
( 2108 , 28.13 )
( 2109 , 28.18 )
( 2110 , 28.06 )
( 2111 , 28.03 )
( 2112 , 27.90 )
( 2113 , 27.80 )
( 2114 , 27.73 )
( 2115 , 27.80 )
( 2116 , 27.85 )
( 2117 , 27.89 )
( 2118 , 27.99 )
( 2119 , 28.04 )
( 2120 , 28.05 )
( 2121 , 28.01 )
( 2122 , 27.99 )
( 2123 , 27.95 )
( 2124 , 27.96 )
( 2125 , 28.07 )
( 2126 , 28.14 )
( 2127 , 28.01 )
( 2128 , 27.75 )
( 2129 , 27.46 )
( 2130 , 27.25 )
( 2131 , 26.95 )
( 2132 , 26.65 )
( 2133 , 26.53 )
( 2134 , 26.26 )
( 2135 , 26.20 )
( 2136 , 26.16 )
( 2137 , 26.03 )
( 2138 , 25.84 )
( 2139 , 25.54 )
( 2140 , 25.24 )
( 2141 , 24.95 )
( 2142 , 24.68 )
( 2143 , 24.38 )
( 2144 , 24.08 )
( 2145 , 24.07 )
( 2146 , 24.04 )
( 2147 , 23.98 )
( 2148 , 23.92 )
( 2149 , 23.91 )
( 2150 , 23.90 )
( 2151 , 23.93 )
( 2152 , 24.22 )
( 2153 , 24.23 )
( 2154 , 24.17 )
( 2155 , 24.16 )
( 2156 , 24.13 )
( 2157 , 24.07 )
( 2158 , 24.08 )
( 2159 , 24.07 )
( 2160 , 24.06 )
( 2161 , 24.01 )
( 2162 , 24.05 )
( 2163 , 24.04 )
( 2164 , 23.98 )
( 2165 , 23.93 )
( 2166 , 23.90 )
( 2167 , 23.84 )
( 2168 , 23.80 )
( 2169 , 23.78 )
( 2170 , 23.72 )
( 2171 , 23.70 )
( 2172 , 23.80 )
( 2173 , 23.79 )
( 2174 , 23.76 )
( 2175 , 23.78 )
( 2176 , 23.78 )
( 2177 , 23.78 )
( 2178 , 23.79 )
( 2179 , 23.79 )
( 2180 , 24.02 )
( 2181 , 24.36 )
( 2182 , 24.62 )
( 2183 , 24.85 )
( 2184 , 25.19 )
( 2185 , 25.54 )
( 2186 , 25.78 )
( 2187 , 26.12 )
( 2188 , 26.36 )
( 2189 , 26.59 )
( 2190 , 26.86 )
( 2191 , 27.09 )
( 2192 , 27.38 )
( 2193 , 27.67 )
( 2194 , 27.67 )
( 2195 , 27.91 )
( 2196 , 28.27 )
( 2197 , 28.62 )
( 2198 , 28.85 )
( 2199 , 28.91 )
( 2200 , 28.99 )
( 2201 , 28.99 )
( 2202 , 28.99 )
( 2203 , 29.07 )
( 2204 , 29.08 )
( 2205 , 29.08 )
( 2206 , 29.31 )
( 2207 , 29.53 )
( 2208 , 29.79 )
( 2209 , 30.04 )
( 2210 , 30.45 )
( 2211 , 30.67 )
( 2212 , 31.11 )
( 2213 , 31.52 )
( 2214 , 31.80 )
( 2215 , 32.07 )
( 2216 , 32.30 )
( 2217 , 32.32 )
( 2218 , 32.32 )
( 2219 , 32.32 )
( 2220 , 32.36 )
( 2221 , 32.40 )
( 2222 , 32.41 )
( 2223 , 32.41 )
( 2224 , 32.41 )
( 2225 , 32.56 )
( 2226 , 32.71 )
( 2227 , 32.89 )
( 2228 , 32.89 )
( 2229 , 33.00 )
( 2230 , 33.09 )
( 2231 , 33.10 )
( 2232 , 33.10 )
( 2233 , 33.12 )
( 2234 , 33.34 )
( 2235 , 33.57 )
( 2236 , 33.90 )
( 2237 , 34.19 )
( 2238 , 34.48 )
( 2239 , 34.73 )
( 2240 , 35.02 )
( 2241 , 35.38 )
( 2242 , 35.70 )
( 2243 , 35.99 )
( 2244 , 36.39 )
( 2245 , 36.66 )
( 2246 , 36.95 )
( 2247 , 37.23 )
( 2248 , 37.53 )
( 2249 , 37.53 )
( 2250 , 37.53 )
( 2251 , 37.53 )
( 2252 , 37.58 )
( 2253 , 37.58 )
( 2254 , 37.58 )
( 2255 , 37.64 )
( 2256 , 37.92 )
( 2257 , 38.20 )
( 2258 , 38.47 )
( 2259 , 38.62 )
( 2260 , 38.62 )
( 2261 , 38.62 )
( 2262 , 38.62 )
( 2263 , 38.62 )
( 2264 , 38.66 )
( 2265 , 38.66 )
( 2266 , 38.80 )
( 2267 , 38.90 )
( 2268 , 38.94 )
( 2269 , 38.98 )
( 2270 , 39.00 )
( 2271 , 39.00 )
( 2272 , 39.02 )
( 2273 , 39.02 )
( 2274 , 39.09 )
( 2275 , 39.11 )
( 2276 , 39.12 )
( 2277 , 39.14 )
( 2278 , 39.25 )
( 2279 , 39.22 )
( 2280 , 39.34 )
( 2281 , 39.47 )
( 2282 , 39.62 )
( 2283 , 39.74 )
( 2284 , 39.84 )
( 2285 , 39.93 )
( 2286 , 40.04 )
( 2287 , 40.21 )
( 2288 , 40.29 )
( 2289 , 40.36 )
( 2290 , 40.46 )
( 2291 , 40.36 )
( 2292 , 40.23 )
( 2293 , 40.15 )
( 2294 , 40.09 )
( 2295 , 39.97 )
( 2296 , 39.86 )
( 2297 , 39.83 )
( 2298 , 39.70 )
( 2299 , 39.66 )
( 2300 , 39.54 )
( 2301 , 39.41 )
( 2302 , 39.29 )
( 2303 , 39.24 )
( 2304 , 39.11 )
( 2305 , 38.99 )
( 2306 , 38.90 )
( 2307 , 38.77 )
( 2308 , 38.68 )
( 2309 , 38.78 )
( 2310 , 38.67 )
( 2311 , 38.75 )
( 2312 , 38.79 )
( 2313 , 38.83 )
( 2314 , 38.88 )
( 2315 , 38.75 )
( 2316 , 38.72 )
( 2317 , 38.70 )
( 2318 , 38.78 )
( 2319 , 38.83 )
( 2320 , 38.96 )
( 2321 , 39.07 )
( 2322 , 38.98 )
( 2323 , 38.87 )
( 2324 , 38.80 )
( 2325 , 38.67 )
( 2326 , 38.55 )
( 2327 , 38.42 )
( 2328 , 38.55 )
( 2329 , 38.68 )
( 2330 , 38.82 )
( 2331 , 38.95 )
( 2332 , 39.13 )
( 2333 , 39.32 )
( 2334 , 39.49 )
( 2335 , 39.66 )
( 2336 , 39.83 )
( 2337 , 40.01 )
( 2338 , 40.24 )
( 2339 , 40.13 )
( 2340 , 40.01 )
( 2341 , 39.98 )
( 2342 , 40.01 )
( 2343 , 40.03 )
( 2344 , 40.09 )
( 2345 , 40.18 )
( 2346 , 40.30 )
( 2347 , 40.38 )
( 2348 , 40.37 )
( 2349 , 40.40 )
( 2350 , 40.47 )
( 2351 , 40.53 )
( 2352 , 40.53 )
( 2353 , 40.62 )
( 2354 , 40.64 )
( 2355 , 40.49 )
( 2356 , 40.36 )
( 2357 , 40.06 )
( 2358 , 39.83 )
( 2359 , 39.53 )
( 2360 , 39.30 )
( 2361 , 39.00 )
( 2362 , 38.75 )
( 2363 , 38.45 )
( 2364 , 38.36 )
( 2365 , 38.30 )
( 2366 , 38.20 )
( 2367 , 38.12 )
( 2368 , 38.25 )
( 2369 , 38.15 )
( 2370 , 38.23 )
( 2371 , 38.37 )
( 2372 , 38.35 )
( 2373 , 38.27 )
( 2374 , 38.16 )
( 2375 , 38.05 )
( 2376 , 37.93 )
( 2377 , 37.81 )
( 2378 , 37.72 )
( 2379 , 37.82 )
( 2380 , 37.90 )
( 2381 , 37.97 )
( 2382 , 37.85 )
( 2383 , 37.74 )
( 2384 , 37.66 )
( 2385 , 37.56 )
( 2386 , 37.82 )
( 2387 , 37.95 )
( 2388 , 38.07 )
( 2389 , 38.21 )
( 2390 , 38.34 )
( 2391 , 38.52 )
( 2392 , 38.71 )
( 2393 , 38.94 )
( 2394 , 39.18 )
( 2395 , 39.44 )
( 2396 , 39.70 )
( 2397 , 40.04 )
( 2398 , 40.32 )
( 2399 , 40.60 )
( 2400 , 40.87 )
( 2401 , 41.08 )
( 2402 , 41.28 )
( 2403 , 41.48 )
( 2404 , 41.68 )
( 2405 , 41.88 )
( 2406 , 42.14 )
( 2407 , 42.38 )
( 2408 , 42.59 )
( 2409 , 42.82 )
( 2410 , 43.02 )
( 2411 , 43.23 )
( 2412 , 43.43 )
( 2413 , 43.62 )
( 2414 , 43.87 )
( 2415 , 44.09 )
( 2416 , 44.35 )
( 2417 , 44.61 )
( 2418 , 44.80 )
( 2419 , 44.92 )
( 2420 , 45.04 )
( 2421 , 45.19 )
( 2422 , 45.20 )
( 2423 , 45.22 )
( 2424 , 45.32 )
( 2425 , 45.33 )
( 2426 , 45.35 )
( 2427 , 45.50 )
( 2428 , 45.64 )
( 2429 , 45.67 )
( 2430 , 45.67 )
( 2431 , 45.67 )
( 2432 , 45.68 )
( 2433 , 45.68 )
( 2434 , 45.74 )
( 2435 , 45.80 )
( 2436 , 45.82 )
( 2437 , 45.83 )
( 2438 , 45.84 )
( 2439 , 45.86 )
( 2440 , 45.88 )
( 2441 , 45.90 )
( 2442 , 46.10 )
( 2443 , 46.10 )
( 2444 , 46.10 )
( 2445 , 46.15 )
( 2446 , 46.17 )
( 2447 , 46.17 )
( 2448 , 46.17 )
( 2449 , 46.55 )
( 2450 , 46.98 )
( 2451 , 47.29 )
( 2452 , 47.59 )
( 2453 , 47.86 )
( 2454 , 48.23 )
( 2455 , 48.57 )
( 2456 , 48.90 )
( 2457 , 49.24 )
( 2458 , 49.61 )
( 2459 , 49.89 )
( 2460 , 50.18 )
( 2461 , 50.46 )
( 2462 , 50.84 )
( 2463 , 51.12 )
( 2464 , 51.34 )
( 2465 , 51.67 )
( 2466 , 51.98 )
( 2467 , 51.98 )
( 2468 , 51.99 )
( 2469 , 52.04 )
( 2470 , 52.07 )
( 2471 , 52.14 )
( 2472 , 52.22 )
( 2473 , 52.22 )
( 2474 , 52.57 )
( 2475 , 52.93 )
( 2476 , 53.29 )
( 2477 , 53.53 )
( 2478 , 53.77 )
( 2479 , 53.82 )
( 2480 , 53.89 )
( 2481 , 53.96 )
( 2482 , 53.98 )
( 2483 , 53.99 )
( 2484 , 54.02 )
( 2485 , 54.04 )
( 2486 , 54.20 )
( 2487 , 54.43 )
( 2488 , 54.59 )
( 2489 , 54.62 )
( 2490 , 54.65 )
( 2491 , 54.67 )
( 2492 , 54.67 )
( 2493 , 54.77 )
( 2494 , 54.97 )
( 2495 , 55.00 )
( 2496 , 55.04 )
( 2497 , 55.04 )
( 2498 , 55.07 )
( 2499 , 55.07 )
( 2500 , 55.07 )
( 2501 , 55.07 )
( 2502 , 55.07 )
( 2503 , 55.07 )
( 2504 , 55.07 )
( 2505 , 55.08 )
( 2506 , 55.08 )
( 2507 , 55.10 )
( 2508 , 55.12 )
( 2509 , 55.16 )
( 2510 , 55.16 )
( 2511 , 55.18 )
( 2512 , 55.21 )
( 2513 , 55.23 )
( 2514 , 55.23 )
( 2515 , 55.23 )
( 2516 , 55.24 )
( 2517 , 55.24 )
( 2518 , 55.27 )
( 2519 , 55.29 )
( 2520 , 55.29 )
( 2521 , 55.32 )
( 2522 , 55.32 )
( 2523 , 55.33 )
( 2524 , 55.33 )
( 2525 , 55.68 )
( 2526 , 55.91 )
( 2527 , 56.16 )
( 2528 , 56.44 )
( 2529 , 56.72 )
( 2530 , 56.98 )
( 2531 , 57.23 )
( 2532 , 57.49 )
( 2533 , 57.72 )
( 2534 , 57.98 )
( 2535 , 58.05 )
( 2536 , 58.16 )
( 2537 , 58.30 )
( 2538 , 58.37 )
( 2539 , 58.44 )
( 2540 , 58.51 )
( 2541 , 58.64 )
( 2542 , 58.77 )
( 2543 , 58.77 )
( 2544 , 58.78 )
( 2545 , 58.80 )
( 2546 , 59.00 )
( 2547 , 59.15 )
( 2548 , 59.30 )
( 2549 , 59.30 )
( 2550 , 59.35 )
( 2551 , 59.40 )
( 2552 , 59.40 )
( 2553 , 59.42 )
( 2554 , 59.45 )
( 2555 , 59.62 )
( 2556 , 59.77 )
( 2557 , 59.91 )
( 2558 , 60.13 )
( 2559 , 60.40 )
( 2560 , 60.62 )
( 2561 , 60.98 )
( 2562 , 61.20 )
( 2563 , 61.48 )
( 2564 , 61.71 )
( 2565 , 61.96 )
( 2566 , 62.21 )
( 2567 , 62.52 )
( 2568 , 62.80 )
( 2569 , 62.80 )
( 2570 , 62.83 )
( 2571 , 62.83 )
( 2572 , 62.84 )
( 2573 , 62.84 )
( 2574 , 62.94 )
( 2575 , 63.04 )
( 2576 , 63.11 )
( 2577 , 63.19 )
( 2578 , 63.32 )
( 2579 , 63.40 )
( 2580 , 63.47 )
( 2581 , 63.47 )
( 2582 , 63.47 )
( 2583 , 63.70 )
( 2584 , 63.92 )
( 2585 , 64.16 )
( 2586 , 64.39 )
( 2587 , 64.63 )
( 2588 , 64.86 )
( 2589 , 65.10 )
( 2590 , 65.33 )
( 2591 , 65.48 )
( 2592 , 65.48 )
( 2593 , 65.48 )
( 2594 , 65.48 )
( 2595 , 65.82 )
( 2596 , 66.18 )
( 2597 , 66.41 )
( 2598 , 66.43 )
( 2599 , 66.43 )
( 2600 , 66.50 )
( 2601 , 66.65 )
( 2602 , 66.66 )
( 2603 , 66.72 )
( 2604 , 66.72 )
( 2605 , 66.84 )
( 2606 , 66.89 )
( 2607 , 66.91 )
( 2608 , 66.91 )
( 2609 , 66.98 )
( 2610 , 67.00 )
( 2611 , 67.05 )
( 2612 , 67.10 )
( 2613 , 67.12 )
( 2614 , 67.16 )
( 2615 , 67.22 )
( 2616 , 67.28 )
( 2617 , 67.28 )
( 2618 , 67.28 )
( 2619 , 67.29 )
( 2620 , 67.31 )
( 2621 , 67.32 )
( 2622 , 67.38 )
( 2623 , 67.58 )
( 2624 , 67.85 )
( 2625 , 68.00 )
( 2626 , 68.22 )
( 2627 , 68.45 )
( 2628 , 68.72 )
( 2629 , 68.95 )
( 2630 , 69.12 )
( 2631 , 69.41 )
( 2632 , 69.72 )
( 2633 , 70.01 )
( 2634 , 70.24 )
( 2635 , 70.48 )
( 2636 , 70.71 )
( 2637 , 70.73 )
( 2638 , 70.73 )
( 2639 , 70.74 )
( 2640 , 70.76 )
( 2641 , 70.77 )
( 2642 , 70.92 )
( 2643 , 71.07 )
( 2644 , 71.07 )
( 2645 , 71.22 )
( 2646 , 71.41 )
( 2647 , 71.48 )
( 2648 , 71.52 )
( 2649 , 71.52 )
( 2650 , 71.52 )
( 2651 , 71.53 )
( 2652 , 71.53 )
( 2653 , 71.55 )
( 2654 , 71.70 )
( 2655 , 71.82 )
( 2656 , 71.84 )
( 2657 , 71.84 )
( 2658 , 71.91 )
( 2659 , 71.91 )
( 2660 , 71.99 )
( 2661 , 72.20 )
( 2662 , 72.34 )
( 2663 , 72.41 )
( 2664 , 72.42 )
( 2665 , 72.45 )
( 2666 , 72.51 )
( 2667 , 72.56 )
( 2668 , 72.56 )
( 2669 , 72.59 )
( 2670 , 72.60 )
( 2671 , 72.60 )
( 2672 , 72.66 )
( 2673 , 72.77 )
( 2674 , 72.84 )
( 2675 , 72.84 )
( 2676 , 72.84 )
( 2677 , 72.88 )
( 2678 , 72.95 )
( 2679 , 72.96 )
( 2680 , 72.96 )
( 2681 , 73.04 )
( 2682 , 73.04 )
( 2683 , 73.04 )
( 2684 , 73.10 )
( 2685 , 73.20 )
( 2686 , 73.22 )
( 2687 , 73.23 )
( 2688 , 73.25 )
( 2689 , 73.30 )
( 2690 , 73.36 )
( 2691 , 73.44 )
( 2692 , 73.44 )
( 2693 , 73.50 )
( 2694 , 73.53 )
( 2695 , 73.55 )
( 2696 , 73.62 )
( 2697 , 73.78 )
( 2698 , 73.95 )
( 2699 , 74.17 )
( 2700 , 74.22 )
( 2701 , 74.43 )
( 2702 , 74.43 )
( 2703 , 74.45 )
( 2704 , 74.51 )
( 2705 , 74.61 )
( 2706 , 74.61 )
( 2707 , 74.66 )
( 2708 , 74.75 )
( 2709 , 74.77 )
( 2710 , 74.80 )
( 2711 , 74.98 )
( 2712 , 75.12 )
( 2713 , 75.28 )
( 2714 , 75.50 )
( 2715 , 75.66 )
( 2716 , 75.82 )
( 2717 , 75.97 )
( 2718 , 76.12 )
( 2719 , 76.33 )
( 2720 , 76.41 )
( 2721 , 76.62 )
( 2722 , 76.64 )
( 2723 , 76.66 )
( 2724 , 76.87 )
( 2725 , 76.88 )
( 2726 , 76.91 )
( 2727 , 76.97 )
( 2728 , 77.19 )
( 2729 , 77.44 )
( 2730 , 77.73 )
( 2731 , 78.01 )
( 2732 , 78.23 )
( 2733 , 78.45 )
( 2734 , 78.67 )
( 2735 , 78.95 )
( 2736 , 79.09 )
( 2737 , 79.09 )
( 2738 , 79.09 )
( 2739 , 79.12 )
( 2740 , 79.12 )
( 2741 , 79.14 )
( 2742 , 79.14 )
( 2743 , 79.25 )
( 2744 , 79.35 )
( 2745 , 79.36 )
( 2746 , 79.36 )
( 2747 , 79.36 )
( 2748 , 79.50 )
( 2749 , 79.70 )
( 2750 , 79.87 )
( 2751 , 79.94 )
( 2752 , 79.95 )
( 2753 , 79.95 )
( 2754 , 79.95 )
( 2755 , 80.00 )
( 2756 , 80.00 )
( 2757 , 80.27 )
( 2758 , 80.53 )
( 2759 , 80.76 )
( 2760 , 80.98 )
( 2761 , 81.27 )
( 2762 , 81.61 )
( 2763 , 81.91 )
( 2764 , 82.20 )
( 2765 , 82.46 )
( 2766 , 82.70 )
( 2767 , 82.91 )
( 2768 , 83.14 )
( 2769 , 83.38 )
( 2770 , 83.68 )
( 2771 , 83.95 )
( 2772 , 84.25 )
( 2773 , 84.55 )
( 2774 , 84.84 )
( 2775 , 85.12 )
( 2776 , 85.43 )
( 2777 , 85.70 )
( 2778 , 85.98 )
( 2779 , 86.30 )
( 2780 , 86.62 )
( 2781 , 86.97 )
( 2782 , 87.32 )
( 2783 , 87.62 )
( 2784 , 87.63 )
( 2785 , 87.64 )
( 2786 , 87.66 )
( 2787 , 87.66 )
( 2788 , 87.66 )
( 2789 , 87.66 )
( 2790 , 87.66 )
( 2791 , 87.67 )
( 2792 , 87.70 )
( 2793 , 87.70 )
( 2794 , 87.70 )
( 2795 , 87.74 )
( 2796 , 87.79 )
( 2797 , 87.80 )
( 2798 , 87.86 )
( 2799 , 87.88 )
( 2800 , 87.88 )
( 2801 , 87.88 )
( 2802 , 88.07 )
( 2803 , 88.16 )
( 2804 , 88.23 )
( 2805 , 88.27 )
( 2806 , 88.35 )
( 2807 , 88.42 )
( 2808 , 88.43 )
( 2809 , 88.43 )
( 2810 , 88.43 )
( 2811 , 88.65 )
( 2812 , 88.88 )
( 2813 , 89.16 )
( 2814 , 89.38 )
( 2815 , 89.72 )
( 2816 , 89.99 )
( 2817 , 90.30 )
( 2818 , 90.60 )
( 2819 , 90.90 )
( 2820 , 91.19 )
( 2821 , 91.47 )
( 2822 , 91.74 )
( 2823 , 92.08 )
( 2824 , 92.39 )
( 2825 , 92.69 )
( 2826 , 92.97 )
( 2827 , 93.02 )
( 2828 , 93.09 )
( 2829 , 93.16 )
( 2830 , 93.17 )
( 2831 , 93.19 )
( 2832 , 93.28 )
( 2833 , 93.42 )
( 2834 , 93.57 )
( 2835 , 93.76 )
( 2836 , 93.80 )
( 2837 , 93.81 )
( 2838 , 93.85 )
( 2839 , 93.88 )
( 2840 , 93.88 )
( 2841 , 93.88 )
( 2842 , 93.96 )
( 2843 , 93.98 )
( 2844 , 93.98 )
( 2845 , 93.98 )
( 2846 , 93.99 )
( 2847 , 93.99 )
( 2848 , 94.01 )
( 2849 , 94.01 )
( 2850 , 94.03 )
( 2851 , 94.05 )
( 2852 , 94.06 )
( 2853 , 94.08 )
( 2854 , 94.20 )
( 2855 , 94.18 )
( 2856 , 94.16 )
( 2857 , 94.30 )
( 2858 , 94.45 )
( 2859 , 94.59 )
( 2860 , 94.73 )
( 2861 , 94.87 )
( 2862 , 95.00 )
( 2863 , 95.14 )
( 2864 , 95.27 )
( 2865 , 95.41 )
( 2866 , 95.52 )
( 2867 , 95.64 )
( 2868 , 95.73 )
( 2869 , 95.85 )
( 2870 , 95.95 )
( 2871 , 96.05 )
( 2872 , 96.17 )
( 2873 , 96.42 )
( 2874 , 96.62 )
( 2875 , 96.84 )
( 2876 , 97.00 )
( 2877 , 97.17 )
( 2878 , 97.33 )
( 2879 , 97.45 )
( 2880 , 97.56 )
( 2881 , 97.66 )
( 2882 , 97.87 )
( 2883 , 97.96 )
( 2884 , 98.07 )
( 2885 , 98.16 )
( 2886 , 98.27 )
( 2887 , 98.42 )
( 2888 , 98.47 )
( 2889 , 98.51 )
( 2890 , 98.60 )
( 2891 , 98.67 )
( 2892 , 98.66 )
( 2893 , 98.65 )
( 2894 , 98.38 )
( 2895 , 98.14 )
( 2896 , 97.85 )
( 2897 , 97.55 )
( 2898 , 97.26 )
( 2899 , 97.05 )
( 2900 , 96.78 )
( 2901 , 96.70 )
( 2902 , 96.55 )
( 2903 , 96.27 )
( 2904 , 96.08 )
( 2905 , 95.78 )
( 2906 , 95.51 )
( 2907 , 95.41 )
( 2908 , 95.35 )
( 2909 , 95.38 )
( 2910 , 95.37 )
( 2911 , 95.12 )
( 2912 , 94.88 )
( 2913 , 94.58 )
( 2914 , 94.28 )
( 2915 , 94.05 )
( 2916 , 93.82 )
( 2917 , 93.59 )
( 2918 , 93.31 )
( 2919 , 93.23 )
( 2920 , 93.15 )
( 2921 , 93.12 )
( 2922 , 93.13 )
( 2923 , 93.08 )
( 2924 , 93.05 )
( 2925 , 92.96 )
( 2926 , 92.90 )
( 2927 , 92.80 )
( 2928 , 92.83 )
( 2929 , 92.82 )
( 2930 , 92.62 )
( 2931 , 92.33 )
( 2932 , 92.03 )
( 2933 , 92.06 )
( 2934 , 92.16 )
( 2935 , 92.07 )
( 2936 , 92.07 )
( 2937 , 92.11 )
( 2938 , 92.05 )
( 2939 , 91.95 )
( 2940 , 91.86 )
( 2941 , 91.55 )
( 2942 , 91.25 )
( 2943 , 90.99 )
( 2944 , 90.70 )
( 2945 , 90.62 )
( 2946 , 90.59 )
( 2947 , 90.57 )
( 2948 , 90.61 )
( 2949 , 90.40 )
( 2950 , 90.10 )
( 2951 , 89.81 )
( 2952 , 89.53 )
( 2953 , 89.37 )
( 2954 , 89.30 )
( 2955 , 89.23 )
( 2956 , 89.13 )
( 2957 , 88.84 )
( 2958 , 88.54 )
( 2959 , 88.23 )
( 2960 , 88.09 )
( 2961 , 87.96 )
( 2962 , 88.11 )
( 2963 , 88.29 )
( 2964 , 88.43 )
( 2965 , 88.49 )
( 2966 , 88.51 )
( 2967 , 88.53 )
( 2968 , 88.61 )
( 2969 , 88.64 )
( 2970 , 88.63 )
( 2971 , 88.84 )
( 2972 , 88.98 )
( 2973 , 89.23 )
( 2974 , 89.48 )
( 2975 , 89.45 )
( 2976 , 89.43 )
( 2977 , 89.42 )
( 2978 , 89.48 )
( 2979 , 89.46 )
( 2980 , 89.43 )
( 2981 , 89.36 )
( 2982 , 89.23 )
( 2983 , 89.12 )
( 2984 , 89.00 )
( 2985 , 89.00 )
( 2986 , 88.96 )
( 2987 , 88.84 )
( 2988 , 88.73 )
( 2989 , 88.82 )
( 2990 , 88.86 )
( 2991 , 88.91 )
( 2992 , 88.95 )
( 2993 , 89.00 )
( 2994 , 89.04 )
( 2995 , 89.11 )
( 2996 , 89.17 )
( 2997 , 89.28 )
( 2998 , 89.32 )
( 2999 , 89.38 )
( 3000 , 89.45 )
( 3001 , 89.52 )
( 3002 , 89.40 )
( 3003 , 89.27 )
( 3004 , 89.16 )
( 3005 , 89.03 )
( 3006 , 88.91 )
( 3007 , 88.78 )
( 3008 , 88.72 )
( 3009 , 88.65 )
( 3010 , 88.66 )
( 3011 , 88.59 )
( 3012 , 88.47 )
( 3013 , 88.35 )
( 3014 , 88.23 )
( 3015 , 88.11 )
( 3016 , 88.02 )
( 3017 , 87.92 )
( 3018 , 87.88 )
( 3019 , 87.80 )
( 3020 , 87.73 )
( 3021 , 87.61 )
( 3022 , 87.55 )
( 3023 , 87.51 )
( 3024 , 87.45 )
( 3025 , 87.43 )
( 3026 , 87.40 )
( 3027 , 87.38 )
( 3028 , 87.39 )
( 3029 , 87.34 )
( 3030 , 87.33 )
( 3031 , 87.27 )
( 3032 , 87.21 )
( 3033 , 87.15 )
( 3034 , 87.10 )
( 3035 , 87.06 )
( 3036 , 87.00 )
( 3037 , 86.70 )
( 3038 , 86.40 )
( 3039 , 86.28 )
( 3040 , 86.13 )
( 3041 , 85.84 )
( 3042 , 85.78 )
( 3043 , 85.66 )
( 3044 , 85.52 )
( 3045 , 85.38 )
( 3046 , 85.24 )
( 3047 , 85.09 )
( 3048 , 84.82 )
( 3049 , 84.60 )
( 3050 , 84.39 )
( 3051 , 84.09 )
( 3052 , 83.79 )
( 3053 , 83.49 )
( 3054 , 83.27 )
( 3055 , 82.97 )
( 3056 , 82.68 )
( 3057 , 82.47 )
( 3058 , 82.24 )
( 3059 , 82.00 )
( 3060 , 81.76 )
( 3061 , 81.51 )
( 3062 , 81.20 )
( 3063 , 81.24 )
( 3064 , 81.20 )
( 3065 , 81.11 )
( 3066 , 80.81 )
( 3067 , 80.51 )
( 3068 , 80.38 )
( 3069 , 80.28 )
( 3070 , 80.23 )
( 3071 , 80.14 )
( 3072 , 80.05 )
( 3073 , 79.95 )
( 3074 , 79.91 )
( 3075 , 79.80 )
( 3076 , 79.73 )
( 3077 , 79.71 )
( 3078 , 79.62 )
( 3079 , 79.66 )
( 3080 , 79.35 )
( 3081 , 79.05 )
( 3082 , 79.04 )
( 3083 , 78.97 )
( 3084 , 78.92 )
( 3085 , 78.85 )
( 3086 , 78.73 )
( 3087 , 78.53 )
( 3088 , 78.23 )
( 3089 , 78.13 )
( 3090 , 78.12 )
( 3091 , 77.82 )
( 3092 , 77.52 )
( 3093 , 77.34 )
( 3094 , 77.15 )
( 3095 , 76.85 )
( 3096 , 76.55 )
( 3097 , 76.48 )
( 3098 , 76.38 )
( 3099 , 76.08 )
( 3100 , 75.87 )
( 3101 , 75.57 )
( 3102 , 75.37 )
( 3103 , 75.16 )
( 3104 , 74.97 )
( 3105 , 74.66 )
( 3106 , 74.41 )
( 3107 , 74.11 )
( 3108 , 73.84 )
( 3109 , 73.53 )
( 3110 , 73.23 )
( 3111 , 72.95 )
( 3112 , 72.83 )
( 3113 , 72.53 )
( 3114 , 72.23 )
( 3115 , 71.93 )
( 3116 , 71.63 )
( 3117 , 71.35 )
( 3118 , 71.16 )
( 3119 , 70.96 )
( 3120 , 70.67 )
( 3121 , 70.37 )
( 3122 , 70.58 )
( 3123 , 70.67 )
( 3124 , 70.77 )
( 3125 , 70.97 )
( 3126 , 71.07 )
( 3127 , 71.17 )
( 3128 , 71.29 )
( 3129 , 71.39 )
( 3130 , 71.49 )
( 3131 , 71.61 )
( 3132 , 71.75 )
( 3133 , 71.88 )
( 3134 , 71.95 )
( 3135 , 71.88 )
( 3136 , 71.76 )
( 3137 , 71.63 )
( 3138 , 71.51 )
( 3139 , 71.43 )
( 3140 , 71.36 )
( 3141 , 71.26 )
( 3142 , 71.13 )
( 3143 , 71.01 )
( 3144 , 71.05 )
( 3145 , 71.10 )
( 3146 , 71.00 )
( 3147 , 70.90 )
( 3148 , 70.82 )
( 3149 , 70.73 )
( 3150 , 70.65 )
( 3151 , 70.58 )
( 3152 , 70.45 )
( 3153 , 70.16 )
( 3154 , 69.88 )
( 3155 , 69.57 )
( 3156 , 69.27 )
( 3157 , 68.98 )
( 3158 , 68.67 )
( 3159 , 68.55 )
( 3160 , 68.31 )
( 3161 , 68.02 )
( 3162 , 67.97 )
( 3163 , 67.66 )
( 3164 , 67.40 )
( 3165 , 67.09 )
( 3166 , 66.80 )
( 3167 , 66.49 )
( 3168 , 66.29 )
( 3169 , 66.09 )
( 3170 , 65.80 )
( 3171 , 65.55 )
( 3172 , 65.34 )
( 3173 , 65.06 )
( 3174 , 64.96 )
( 3175 , 64.98 )
( 3176 , 65.01 )
( 3177 , 65.04 )
( 3178 , 65.05 )
( 3179 , 65.03 )
( 3180 , 64.94 )
( 3181 , 64.88 )
( 3182 , 64.83 )
( 3183 , 64.73 )
( 3184 , 64.63 )
( 3185 , 64.74 )
( 3186 , 64.66 )
( 3187 , 64.42 )
( 3188 , 64.12 )
( 3189 , 64.12 )
( 3190 , 64.05 )
( 3191 , 63.96 )
( 3192 , 63.93 )
( 3193 , 63.89 )
( 3194 , 63.89 )
( 3195 , 63.79 )
( 3196 , 63.50 )
( 3197 , 63.20 )
( 3198 , 62.91 )
( 3199 , 62.61 )
( 3200 , 62.65 )
( 3201 , 62.66 )
( 3202 , 62.67 )
( 3203 , 62.67 )
( 3204 , 62.67 )
( 3205 , 62.67 )
( 3206 , 62.74 )
( 3207 , 62.89 )
( 3208 , 63.04 )
( 3209 , 63.09 )
( 3210 , 63.09 )
( 3211 , 63.09 )
( 3212 , 63.09 )
( 3213 , 63.11 )
( 3214 , 63.15 )
( 3215 , 63.15 )
( 3216 , 63.15 )
( 3217 , 63.18 )
( 3218 , 63.22 )
( 3219 , 63.28 )
( 3220 , 63.43 )
( 3221 , 63.54 )
( 3222 , 63.54 )
( 3223 , 63.69 )
( 3224 , 63.69 )
( 3225 , 63.76 )
( 3226 , 63.89 )
( 3227 , 63.97 )
( 3228 , 63.97 )
( 3229 , 63.98 )
( 3230 , 63.98 )
( 3231 , 63.98 )
( 3232 , 63.98 )
( 3233 , 63.98 )
( 3234 , 64.10 )
( 3235 , 64.10 )
( 3236 , 64.12 )
( 3237 , 64.14 )
( 3238 , 64.14 )
( 3239 , 64.14 )
( 3240 , 64.30 )
( 3241 , 64.45 )
( 3242 , 64.66 )
( 3243 , 64.80 )
( 3244 , 64.80 )
( 3245 , 64.80 )
( 3246 , 64.85 )
( 3247 , 64.85 )
( 3248 , 65.25 )
( 3249 , 65.66 )
( 3250 , 65.88 )
( 3251 , 66.19 )
( 3252 , 66.49 )
( 3253 , 66.84 )
( 3254 , 67.13 )
( 3255 , 67.13 )
( 3256 , 67.14 )
( 3257 , 67.17 )
( 3258 , 67.27 )
( 3259 , 67.38 )
( 3260 , 67.46 )
( 3261 , 67.41 )
( 3262 , 67.37 )
( 3263 , 67.38 )
( 3264 , 67.32 )
( 3265 , 67.36 )
( 3266 , 67.30 )
( 3267 , 67.17 )
( 3268 , 67.07 )
( 3269 , 67.02 )
( 3270 , 66.96 )
( 3271 , 66.84 )
( 3272 , 66.73 )
( 3273 , 66.67 )
( 3274 , 66.62 )
( 3275 , 66.68 )
( 3276 , 66.73 )
( 3277 , 66.84 )
( 3278 , 66.92 )
( 3279 , 67.01 )
( 3280 , 67.00 )
( 3281 , 66.98 )
( 3282 , 66.95 )
( 3283 , 66.88 )
( 3284 , 66.87 )
( 3285 , 66.86 )
( 3286 , 66.81 )
( 3287 , 66.77 )
( 3288 , 66.71 )
( 3289 , 66.72 )
( 3290 , 66.74 )
( 3291 , 66.73 )
( 3292 , 66.73 )
( 3293 , 66.74 )
( 3294 , 66.76 )
( 3295 , 66.78 )
( 3296 , 66.77 )
( 3297 , 66.67 )
( 3298 , 66.55 )
( 3299 , 66.44 )
( 3300 , 66.44 )
( 3301 , 66.36 )
( 3302 , 66.30 )
( 3303 , 66.19 )
( 3304 , 66.06 )
( 3305 , 65.94 )
( 3306 , 65.84 )
( 3307 , 65.71 )
( 3308 , 65.59 )
( 3309 , 65.47 )
( 3310 , 65.35 )
( 3311 , 65.23 )
( 3312 , 65.27 )
( 3313 , 65.14 )
( 3314 , 65.20 )
( 3315 , 65.23 )
( 3316 , 65.25 )
( 3317 , 65.20 )
( 3318 , 65.07 )
( 3319 , 64.97 )
( 3320 , 65.02 )
( 3321 , 64.90 )
( 3322 , 64.79 )
( 3323 , 64.66 )
( 3324 , 64.68 )
( 3325 , 64.60 )
( 3326 , 64.52 )
( 3327 , 64.39 )
( 3328 , 64.30 )
( 3329 , 64.34 )
( 3330 , 64.37 )
( 3331 , 64.39 )
( 3332 , 64.27 )
( 3333 , 64.17 )
( 3334 , 64.06 )
( 3335 , 63.98 )
( 3336 , 63.90 )
( 3337 , 63.78 )
( 3338 , 63.82 )
( 3339 , 63.86 )
( 3340 , 63.78 )
( 3341 , 63.77 )
( 3342 , 63.67 )
( 3343 , 63.73 )
( 3344 , 63.62 )
( 3345 , 63.59 )
( 3346 , 63.47 )
( 3347 , 63.41 )
( 3348 , 63.39 )
( 3349 , 63.32 )
( 3350 , 63.25 )
( 3351 , 63.37 )
( 3352 , 63.25 )
( 3353 , 63.12 )
( 3354 , 62.83 )
( 3355 , 62.61 )
( 3356 , 62.56 )
( 3357 , 62.50 )
( 3358 , 62.44 )
( 3359 , 62.30 )
( 3360 , 62.00 )
( 3361 , 61.77 )
( 3362 , 61.58 )
( 3363 , 61.28 )
( 3364 , 60.98 )
( 3365 , 60.84 )
( 3366 , 60.88 )
( 3367 , 60.81 )
( 3368 , 60.77 )
( 3369 , 60.76 )
( 3370 , 60.61 )
( 3371 , 60.48 )
( 3372 , 60.34 )
( 3373 , 60.20 )
( 3374 , 60.06 )
( 3375 , 59.75 )
( 3376 , 59.45 )
( 3377 , 59.68 )
( 3378 , 59.68 )
( 3379 , 59.90 )
( 3380 , 60.18 )
( 3381 , 60.43 )
( 3382 , 60.67 )
( 3383 , 60.89 )
( 3384 , 61.11 )
( 3385 , 61.45 )
( 3386 , 61.74 )
( 3387 , 62.05 )
( 3388 , 62.08 )
( 3389 , 62.12 )
( 3390 , 62.12 )
( 3391 , 62.20 )
( 3392 , 62.27 )
( 3393 , 62.28 )
( 3394 , 62.28 )
( 3395 , 62.28 )
( 3396 , 62.51 )
( 3397 , 62.73 )
( 3398 , 63.13 )
( 3399 , 63.43 )
( 3400 , 63.65 )
( 3401 , 63.98 )
( 3402 , 64.34 )
( 3403 , 64.56 )
( 3404 , 64.78 )
( 3405 , 65.01 )
( 3406 , 65.24 )
( 3407 , 65.48 )
( 3408 , 65.71 )
( 3409 , 66.01 )
( 3410 , 66.01 )
( 3411 , 66.19 )
( 3412 , 66.20 )
( 3413 , 66.20 )
( 3414 , 66.20 )
( 3415 , 66.21 )
( 3416 , 66.24 )
( 3417 , 66.24 )
( 3418 , 66.41 )
( 3419 , 66.57 )
( 3420 , 66.73 )
( 3421 , 66.91 )
( 3422 , 67.06 )
( 3423 , 67.25 )
( 3424 , 67.27 )
( 3425 , 67.32 )
( 3426 , 67.33 )
( 3427 , 67.38 )
( 3428 , 67.47 )
( 3429 , 67.47 )
( 3430 , 67.47 )
( 3431 , 67.53 )
( 3432 , 67.62 )
( 3433 , 67.62 )
( 3434 , 67.68 )
( 3435 , 67.69 )
( 3436 , 67.73 )
( 3437 , 67.97 )
( 3438 , 68.24 )
( 3439 , 68.57 )
( 3440 , 68.85 )
( 3441 , 69.16 )
( 3442 , 69.49 )
( 3443 , 69.77 )
( 3444 , 70.05 )
( 3445 , 70.39 )
( 3446 , 70.71 )
( 3447 , 71.01 )
( 3448 , 71.29 )
( 3449 , 71.62 )
( 3450 , 72.04 )
( 3451 , 72.47 )
( 3452 , 72.62 )
( 3453 , 72.80 )
( 3454 , 72.89 )
( 3455 , 72.95 )
( 3456 , 72.97 )
( 3457 , 73.12 )
( 3458 , 73.26 )
( 3459 , 73.26 )
( 3460 , 73.27 )
( 3461 , 73.31 )
( 3462 , 73.34 )
( 3463 , 73.36 )
( 3464 , 73.38 )
( 3465 , 73.38 )
( 3466 , 73.38 )
( 3467 , 73.58 )
( 3468 , 73.81 )
( 3469 , 74.05 )
( 3470 , 74.23 )
( 3471 , 74.23 )
( 3472 , 74.51 )
( 3473 , 74.78 )
( 3474 , 74.79 )
( 3475 , 74.79 )
( 3476 , 74.80 )
( 3477 , 74.83 )
( 3478 , 74.83 )
( 3479 , 74.84 )
( 3480 , 74.88 )
( 3481 , 74.89 )
( 3482 , 74.94 )
( 3483 , 74.96 )
( 3484 , 74.99 )
( 3485 , 75.01 )
( 3486 , 75.01 )
( 3487 , 75.07 )
( 3488 , 75.22 )
( 3489 , 75.36 )
( 3490 , 75.36 )
( 3491 , 75.40 )
( 3492 , 75.46 )
( 3493 , 75.51 )
( 3494 , 75.54 )
( 3495 , 75.54 )
( 3496 , 75.60 )
( 3497 , 75.64 )
( 3498 , 75.66 )
( 3499 , 75.66 )
( 3500 , 75.70 )
( 3501 , 75.70 )
( 3502 , 75.75 )
( 3503 , 75.80 )
( 3504 , 75.80 )
( 3505 , 75.80 )
( 3506 , 75.95 )
( 3507 , 76.16 )
( 3508 , 76.33 )
( 3509 , 76.53 )
( 3510 , 76.73 )
( 3511 , 76.73 )
( 3512 , 76.75 )
( 3513 , 76.78 )
( 3514 , 76.78 )
( 3515 , 76.79 )
( 3516 , 76.90 )
( 3517 , 76.96 )
( 3518 , 77.05 )
( 3519 , 77.20 )
( 3520 , 77.28 )
( 3521 , 77.36 )
( 3522 , 77.36 )
( 3523 , 77.52 )
( 3524 , 77.66 )
( 3525 , 77.77 )
( 3526 , 77.78 )
( 3527 , 77.90 )
( 3528 , 77.91 )
( 3529 , 77.93 )
( 3530 , 77.98 )
( 3531 , 78.05 )
( 3532 , 78.05 )
( 3533 , 78.11 )
( 3534 , 78.14 )
( 3535 , 78.15 )
( 3536 , 78.16 )
( 3537 , 78.16 )
( 3538 , 78.16 )
( 3539 , 78.16 )
( 3540 , 78.20 )
( 3541 , 78.34 )
( 3542 , 78.34 )
( 3543 , 78.35 )
( 3544 , 78.38 )
( 3545 , 78.38 )
( 3546 , 78.45 )
( 3547 , 78.50 )
( 3548 , 78.66 )
( 3549 , 78.83 )
( 3550 , 78.97 )
( 3551 , 79.20 )
( 3552 , 79.42 )
( 3553 , 79.48 )
( 3554 , 79.48 )
( 3555 , 79.68 )
( 3556 , 79.72 )
( 3557 , 79.72 )
( 3558 , 79.73 )
( 3559 , 79.75 )
( 3560 , 79.79 )
( 3561 , 79.80 )
( 3562 , 79.88 )
( 3563 , 80.04 )
( 3564 , 80.19 )
( 3565 , 80.40 )
( 3566 , 80.67 )
( 3567 , 80.96 )
( 3568 , 81.15 )
( 3569 , 81.26 )
( 3570 , 81.26 )
( 3571 , 81.14 )
( 3572 , 81.02 )
( 3573 , 80.90 )
( 3574 , 80.83 )
( 3575 , 80.74 )
( 3576 , 80.67 )
( 3577 , 80.55 )
( 3578 , 80.60 )
( 3579 , 80.48 )
( 3580 , 80.41 )
( 3581 , 80.30 )
( 3582 , 80.18 )
( 3583 , 80.05 )
( 3584 , 79.95 )
( 3585 , 79.98 )
( 3586 , 79.86 )
( 3587 , 79.81 )
( 3588 , 79.69 )
( 3589 , 79.61 )
( 3590 , 79.48 )
( 3591 , 79.43 )
( 3592 , 79.27 )
( 3593 , 78.99 )
( 3594 , 78.70 )
( 3595 , 78.73 )
( 3596 , 78.59 )
( 3597 , 78.29 )
( 3598 , 77.99 )
( 3599 , 77.70 )
( 3600 , 77.55 )
( 3601 , 77.45 )
( 3602 , 77.36 )
( 3603 , 77.05 )
( 3604 , 76.83 )
( 3605 , 76.59 )
( 3606 , 76.30 )
( 3607 , 76.17 )
( 3608 , 76.06 )
( 3609 , 76.05 )
( 3610 , 75.94 )
( 3611 , 75.81 )
( 3612 , 75.70 )
( 3613 , 75.57 )
( 3614 , 75.48 )
( 3615 , 75.55 )
( 3616 , 75.68 )
( 3617 , 75.73 )
( 3618 , 75.87 )
( 3619 , 76.01 )
( 3620 , 76.16 )
( 3621 , 76.22 )
( 3622 , 76.12 )
( 3623 , 76.01 )
( 3624 , 75.91 )
( 3625 , 75.78 )
( 3626 , 75.67 )
( 3627 , 75.55 )
( 3628 , 75.44 )
( 3629 , 75.31 )
( 3630 , 75.19 )
( 3631 , 75.23 )
( 3632 , 75.11 )
( 3633 , 74.99 )
( 3634 , 74.91 )
( 3635 , 74.83 )
( 3636 , 74.87 )
( 3637 , 74.77 )
( 3638 , 74.64 )
( 3639 , 74.52 )
( 3640 , 74.41 )
( 3641 , 74.32 )
( 3642 , 74.23 )
( 3643 , 74.10 )
( 3644 , 74.00 )
( 3645 , 73.94 )
( 3646 , 73.89 )
( 3647 , 73.82 )
( 3648 , 73.73 )
( 3649 , 73.63 )
( 3650 , 73.38 )
( 3651 , 73.09 )
( 3652 , 72.79 )
( 3653 , 72.48 )
( 3654 , 72.19 )
( 3655 , 71.88 )
( 3656 , 71.83 )
( 3657 , 71.56 )
( 3658 , 71.27 )
( 3659 , 70.99 )
( 3660 , 70.93 )
( 3661 , 70.84 )
( 3662 , 70.53 )
( 3663 , 70.23 )
( 3664 , 69.93 )
( 3665 , 69.63 )
( 3666 , 69.34 )
( 3667 , 69.14 )
( 3668 , 68.92 )
( 3669 , 68.94 )
( 3670 , 68.88 )
( 3671 , 68.81 )
( 3672 , 68.51 )
( 3673 , 68.30 )
( 3674 , 68.13 )
( 3675 , 68.04 )
( 3676 , 67.91 )
( 3677 , 67.82 )
( 3678 , 67.73 )
( 3679 , 67.62 )
( 3680 , 67.66 )
( 3681 , 67.70 )
( 3682 , 67.77 )
( 3683 , 67.59 )
( 3684 , 67.33 )
( 3685 , 67.03 )
( 3686 , 66.73 )
( 3687 , 66.75 )
( 3688 , 66.61 )
( 3689 , 66.55 )
( 3690 , 66.41 )
( 3691 , 66.26 )
( 3692 , 66.03 )
( 3693 , 65.95 )
( 3694 , 65.84 )
( 3695 , 65.79 )
( 3696 , 65.87 )
( 3697 , 65.77 )
( 3698 , 65.55 )
( 3699 , 65.36 )
( 3700 , 65.34 )
( 3701 , 65.27 )
( 3702 , 64.97 )
( 3703 , 64.67 )
( 3704 , 64.46 )
( 3705 , 64.27 )
( 3706 , 64.08 )
( 3707 , 63.77 )
( 3708 , 63.47 )
( 3709 , 63.26 )
( 3710 , 62.96 )
( 3711 , 62.83 )
( 3712 , 62.56 )
( 3713 , 62.25 )
( 3714 , 61.95 )
( 3715 , 61.65 )
( 3716 , 61.35 )
( 3717 , 61.12 )
( 3718 , 60.88 )
( 3719 , 60.64 )
( 3720 , 60.35 )
( 3721 , 60.05 )
( 3722 , 59.84 )
( 3723 , 59.64 )
( 3724 , 59.34 )
( 3725 , 59.04 )
( 3726 , 58.74 )
( 3727 , 58.45 )
( 3728 , 58.14 )
( 3729 , 58.00 )
( 3730 , 57.94 )
( 3731 , 57.87 )
( 3732 , 57.99 )
( 3733 , 58.09 )
( 3734 , 58.10 )
( 3735 , 57.96 )
( 3736 , 57.81 )
( 3737 , 57.59 )
( 3738 , 57.40 )
( 3739 , 57.25 )
( 3740 , 57.12 )
( 3741 , 56.98 )
( 3742 , 56.74 )
( 3743 , 56.44 )
( 3744 , 56.14 )
( 3745 , 55.91 )
( 3746 , 55.61 )
( 3747 , 55.41 )
( 3748 , 55.18 )
( 3749 , 54.88 )
( 3750 , 54.78 )
( 3751 , 54.48 )
( 3752 , 54.31 )
( 3753 , 54.12 )
( 3754 , 53.82 )
( 3755 , 53.55 )
( 3756 , 53.25 )
( 3757 , 52.97 )
( 3758 , 52.67 )
( 3759 , 52.45 )
( 3760 , 52.16 )
( 3761 , 51.86 )
( 3762 , 51.68 )
( 3763 , 51.39 )
( 3764 , 51.09 )
( 3765 , 50.82 )
( 3766 , 50.52 )
( 3767 , 50.22 )
( 3768 , 49.92 )
( 3769 , 49.69 )
( 3770 , 49.39 )
( 3771 , 49.12 )
( 3772 , 48.89 )
( 3773 , 48.62 )
( 3774 , 48.36 )
( 3775 , 48.21 )
( 3776 , 48.10 )
( 3777 , 47.98 )
( 3778 , 47.90 )
( 3779 , 47.84 )
( 3780 , 47.71 )
( 3781 , 47.60 )
( 3782 , 47.40 )
( 3783 , 47.11 )
( 3784 , 46.81 )
( 3785 , 46.51 )
( 3786 , 46.23 )
( 3787 , 46.10 )
( 3788 , 45.95 )
( 3789 , 45.67 )
( 3790 , 45.37 )
( 3791 , 45.12 )
( 3792 , 44.88 )
( 3793 , 44.58 )
( 3794 , 44.28 )
( 3795 , 44.24 )
( 3796 , 44.18 )
( 3797 , 44.09 )
( 3798 , 44.02 )
( 3799 , 43.93 )
( 3800 , 43.78 )
( 3801 , 43.72 )
( 3802 , 43.73 )
( 3803 , 43.63 )
( 3804 , 43.33 )
( 3805 , 43.06 )
( 3806 , 42.76 )
( 3807 , 42.54 )
( 3808 , 42.24 )
( 3809 , 41.94 )
( 3810 , 42.10 )
( 3811 , 42.19 )
( 3812 , 42.39 )
( 3813 , 42.55 )
( 3814 , 42.66 )
( 3815 , 42.81 )
( 3816 , 42.92 )
( 3817 , 43.07 )
( 3818 , 43.20 )
( 3819 , 43.25 )
( 3820 , 43.28 )
( 3821 , 43.40 )
( 3822 , 43.35 )
( 3823 , 43.36 )
( 3824 , 43.33 )
( 3825 , 43.31 )
( 3826 , 43.29 )
( 3827 , 43.47 )
( 3828 , 43.70 )
( 3829 , 43.83 )
( 3830 , 43.88 )
( 3831 , 43.95 )
( 3832 , 43.95 )
( 3833 , 44.26 )
( 3834 , 44.62 )
( 3835 , 44.96 )
( 3836 , 45.29 )
( 3837 , 45.66 )
( 3838 , 46.00 )
( 3839 , 46.20 )
( 3840 , 46.18 )
( 3841 , 46.16 )
( 3842 , 46.11 )
( 3843 , 46.05 )
( 3844 , 46.00 )
( 3845 , 45.96 )
( 3846 , 45.90 )
( 3847 , 45.85 )
( 3848 , 45.80 )
( 3849 , 45.81 )
( 3850 , 45.76 )
( 3851 , 45.77 )
( 3852 , 45.71 )
( 3853 , 45.65 )
( 3854 , 45.61 )
( 3855 , 45.57 )
( 3856 , 45.48 )
( 3857 , 45.36 )
( 3858 , 45.32 )
( 3859 , 45.29 )
( 3860 , 45.16 )
( 3861 , 45.04 )
( 3862 , 44.92 )
( 3863 , 44.99 )
( 3864 , 45.05 )
( 3865 , 44.92 )
( 3866 , 44.93 )
( 3867 , 44.80 )
( 3868 , 44.71 )
( 3869 , 44.59 )
( 3870 , 44.46 )
( 3871 , 44.34 )
( 3872 , 44.24 )
( 3873 , 44.12 )
( 3874 , 44.31 )
( 3875 , 44.45 )
( 3876 , 44.66 )
( 3877 , 44.80 )
( 3878 , 44.92 )
( 3879 , 44.95 )
( 3880 , 44.97 )
( 3881 , 44.95 )
( 3882 , 44.91 )
( 3883 , 44.89 )
( 3884 , 44.91 )
( 3885 , 44.96 )
( 3886 , 44.93 )
( 3887 , 44.95 )
( 3888 , 44.93 )
( 3889 , 44.90 )
( 3890 , 44.85 )
( 3891 , 44.84 )
( 3892 , 44.78 )
( 3893 , 44.75 )
( 3894 , 44.73 )
( 3895 , 44.84 )
( 3896 , 44.78 )
( 3897 , 44.86 )
( 3898 , 44.80 )
( 3899 , 44.73 )
( 3900 , 44.65 )
( 3901 , 44.53 )
( 3902 , 44.43 )
( 3903 , 44.31 )
( 3904 , 44.18 )
( 3905 , 44.13 )
( 3906 , 44.09 )
( 3907 , 44.04 )
( 3908 , 43.99 )
( 3909 , 43.93 )
( 3910 , 43.93 )
( 3911 , 43.90 )
( 3912 , 43.91 )
( 3913 , 43.92 )
( 3914 , 43.86 )
( 3915 , 43.80 )
( 3916 , 43.92 )
( 3917 , 43.98 )
( 3918 , 43.92 )
( 3919 , 44.00 )
( 3920 , 43.98 )
( 3921 , 43.93 )
( 3922 , 43.89 )
( 3923 , 43.84 )
( 3924 , 43.79 )
( 3925 , 43.74 )
( 3926 , 43.61 )
( 3927 , 43.66 )
( 3928 , 43.70 )
( 3929 , 43.58 )
( 3930 , 43.46 )
( 3931 , 43.35 )
( 3932 , 43.24 )
( 3933 , 43.11 )
( 3934 , 42.99 )
( 3935 , 43.05 )
( 3936 , 43.07 )
( 3937 , 43.15 )
( 3938 , 43.10 )
( 3939 , 43.06 )
( 3940 , 43.08 )
( 3941 , 43.14 )
( 3942 , 43.22 )
( 3943 , 43.29 )
( 3944 , 43.42 )
( 3945 , 43.58 )
( 3946 , 43.57 )
( 3947 , 43.52 )
( 3948 , 43.47 )
( 3949 , 43.41 )
( 3950 , 43.42 )
( 3951 , 43.41 )
( 3952 , 43.38 )
( 3953 , 43.42 )
( 3954 , 43.41 )
( 3955 , 43.46 )
( 3956 , 43.35 )
( 3957 , 43.22 )
( 3958 , 43.10 )
( 3959 , 43.29 )
( 3960 , 43.49 )
( 3961 , 43.69 )
( 3962 , 44.00 )
( 3963 , 44.32 )
( 3964 , 44.67 )
( 3965 , 44.91 )
( 3966 , 45.17 )
( 3967 , 45.36 )
( 3968 , 45.24 )
( 3969 , 45.16 )
( 3970 , 45.04 )
( 3971 , 45.04 )
( 3972 , 45.04 )
( 3973 , 45.00 )
( 3974 , 44.87 )
( 3975 , 44.95 )
( 3976 , 45.00 )
( 3977 , 44.95 )
( 3978 , 44.93 )
( 3979 , 44.87 )
( 3980 , 44.87 )
( 3981 , 44.91 )
( 3982 , 44.91 )
( 3983 , 44.93 )
( 3984 , 44.93 )
( 3985 , 44.93 )
( 3986 , 44.94 )
( 3987 , 45.11 )
( 3988 , 45.28 )
( 3989 , 45.45 )
( 3990 , 45.66 )
( 3991 , 45.81 )
( 3992 , 45.84 )
( 3993 , 46.06 )
( 3994 , 46.19 )
( 3995 , 46.32 )
( 3996 , 46.42 )
( 3997 , 46.55 )
( 3998 , 46.71 )
( 3999 , 46.81 )
( 4000 , 46.92 )
( 4001 , 47.02 )
( 4002 , 47.24 )
( 4003 , 47.38 )
( 4004 , 47.52 )
( 4005 , 47.62 )
( 4006 , 47.74 )
( 4007 , 47.84 )
( 4008 , 47.94 )
( 4009 , 48.07 )
( 4010 , 48.19 )
( 4011 , 48.32 )
( 4012 , 48.45 )
( 4013 , 48.51 )
( 4014 , 48.47 )
( 4015 , 48.53 )
( 4016 , 48.69 )
( 4017 , 48.82 )
( 4018 , 48.85 )
( 4019 , 48.80 )
( 4020 , 48.75 )
( 4021 , 48.69 )
( 4022 , 48.66 )
( 4023 , 48.61 )
( 4024 , 48.57 )
( 4025 , 48.53 )
( 4026 , 48.61 )
( 4027 , 48.71 )
( 4028 , 48.68 )
( 4029 , 48.77 )
( 4030 , 48.75 )
( 4031 , 48.75 )
( 4032 , 48.79 )
( 4033 , 48.73 )
( 4034 , 48.75 )
( 4035 , 48.74 )
( 4036 , 48.68 )
( 4037 , 48.70 )
( 4038 , 48.71 )
( 4039 , 48.66 )
( 4040 , 48.67 )
( 4041 , 48.61 )
( 4042 , 48.60 )
( 4043 , 48.59 )
( 4044 , 48.54 )
( 4045 , 48.59 )
( 4046 , 48.55 )
( 4047 , 48.50 )
( 4048 , 48.44 )
( 4049 , 48.43 )
( 4050 , 48.37 )
( 4051 , 48.43 )
( 4052 , 48.52 )
( 4053 , 48.49 )
( 4054 , 48.43 )
( 4055 , 48.38 )
( 4056 , 48.18 )
( 4057 , 47.88 )
( 4058 , 47.82 )
( 4059 , 47.77 )
( 4060 , 47.74 )
( 4061 , 47.68 )
( 4062 , 47.81 )
( 4063 , 47.88 )
( 4064 , 47.95 )
( 4065 , 48.07 )
( 4066 , 48.12 )
( 4067 , 48.20 )
( 4068 , 48.14 )
( 4069 , 48.08 )
( 4070 , 48.04 )
( 4071 , 47.98 )
( 4072 , 48.05 )
( 4073 , 48.30 )
( 4074 , 48.50 )
( 4075 , 48.55 )
( 4076 , 48.64 )
( 4077 , 48.74 )
( 4078 , 48.88 )
( 4079 , 49.00 )
( 4080 , 49.10 )
( 4081 , 49.23 )
( 4082 , 49.32 )
( 4083 , 49.42 )
( 4084 , 49.59 )
( 4085 , 49.75 )
( 4086 , 49.92 )
( 4087 , 50.02 )
( 4088 , 50.12 )
( 4089 , 50.24 )
( 4090 , 50.38 )
( 4091 , 50.48 )
( 4092 , 50.73 )
( 4093 , 50.89 )
( 4094 , 50.99 )
( 4095 , 51.09 )
( 4096 , 51.19 )
( 4097 , 51.29 )
( 4098 , 51.59 )
( 4099 , 51.83 )
( 4100 , 51.95 )
( 4101 , 52.04 )
( 4102 , 52.18 )
( 4103 , 52.32 )
( 4104 , 52.44 )
( 4105 , 52.54 )
( 4106 , 52.64 )
( 4107 , 52.73 )
( 4108 , 52.89 )
( 4109 , 52.98 )
( 4110 , 53.09 )
( 4111 , 53.19 )
( 4112 , 53.49 )
( 4113 , 53.74 )
( 4114 , 53.86 )
( 4115 , 53.95 )
( 4116 , 54.12 )
( 4117 , 54.26 )
( 4118 , 54.38 )
( 4119 , 54.47 )
( 4120 , 54.57 )
( 4121 , 54.67 )
( 4122 , 54.81 )
( 4123 , 54.98 )
( 4124 , 55.09 )
( 4125 , 55.19 )
( 4126 , 55.29 )
( 4127 , 55.38 )
( 4128 , 55.48 )
( 4129 , 55.62 )
( 4130 , 55.73 )
( 4131 , 55.85 )
( 4132 , 55.97 )
( 4133 , 56.07 )
( 4134 , 56.07 )
( 4135 , 56.07 )
( 4136 , 56.07 )
( 4137 , 56.07 )
( 4138 , 56.11 )
( 4139 , 56.10 )
( 4140 , 56.10 )
( 4141 , 56.10 )
( 4142 , 56.24 )
( 4143 , 56.37 )
( 4144 , 56.55 )
( 4145 , 56.71 )
( 4146 , 56.81 )
( 4147 , 56.95 )
( 4148 , 57.04 )
( 4149 , 57.14 )
( 4150 , 57.24 )
( 4151 , 57.34 )
( 4152 , 57.45 )
( 4153 , 57.54 )
( 4154 , 57.72 )
( 4155 , 57.89 )
( 4156 , 57.98 )
( 4157 , 58.09 )
( 4158 , 58.18 )
( 4159 , 58.28 )
( 4160 , 58.38 )
( 4161 , 58.47 )
( 4162 , 58.64 )
( 4163 , 58.84 )
( 4164 , 59.07 )
( 4165 , 59.27 )
( 4166 , 59.38 )
( 4167 , 59.47 )
( 4168 , 59.67 )
( 4169 , 59.89 )
( 4170 , 60.01 )
( 4171 , 60.11 )
( 4172 , 60.23 )
( 4173 , 60.34 )
( 4174 , 60.44 )
( 4175 , 60.55 )
( 4176 , 60.65 )
( 4177 , 60.75 )
( 4178 , 60.87 )
( 4179 , 60.93 )
( 4180 , 60.97 )
( 4181 , 61.01 )
( 4182 , 61.05 )
( 4183 , 60.94 )
( 4184 , 60.83 )
( 4185 , 60.87 )
( 4186 , 60.75 )
( 4187 , 60.70 )
( 4188 , 60.62 )
( 4189 , 60.50 )
( 4190 , 60.38 )
( 4191 , 60.28 )
( 4192 , 60.20 )
( 4193 , 60.08 )
( 4194 , 59.95 )
( 4195 , 59.83 )
( 4196 , 59.70 )
( 4197 , 59.65 )
( 4198 , 59.58 )
( 4199 , 59.46 )
( 4200 , 59.34 )
( 4201 , 59.24 )
( 4202 , 59.12 )
( 4203 , 59.05 )
( 4204 , 58.96 )
( 4205 , 58.86 )
( 4206 , 58.77 )
( 4207 , 58.69 )
( 4208 , 58.73 )
( 4209 , 58.83 )
( 4210 , 58.78 )
( 4211 , 58.73 )
( 4212 , 58.61 )
( 4213 , 58.48 )
( 4214 , 58.39 )
( 4215 , 58.27 )
( 4216 , 58.15 )
( 4217 , 58.21 )
( 4218 , 58.27 )
( 4219 , 58.31 )
( 4220 , 58.36 )
( 4221 , 58.42 )
( 4222 , 58.30 )
( 4223 , 58.18 )
( 4224 , 58.05 )
( 4225 , 57.93 )
( 4226 , 58.06 )
( 4227 , 57.96 )
( 4228 , 57.84 )
( 4229 , 57.80 )
( 4230 , 57.69 )
( 4231 , 57.61 )
( 4232 , 57.52 )
( 4233 , 57.59 )
( 4234 , 57.66 )
( 4235 , 57.53 )
( 4236 , 57.64 )
( 4237 , 57.71 )
( 4238 , 57.76 )
( 4239 , 57.65 )
( 4240 , 57.57 )
( 4241 , 57.50 )
( 4242 , 57.45 )
( 4243 , 57.39 )
( 4244 , 57.34 )
( 4245 , 57.21 )
( 4246 , 57.25 )
( 4247 , 57.14 )
( 4248 , 57.02 )
( 4249 , 57.00 )
( 4250 , 56.88 )
( 4251 , 56.92 )
( 4252 , 56.96 )
( 4253 , 56.84 )
( 4254 , 56.88 )
( 4255 , 56.75 )
( 4256 , 56.90 )
( 4257 , 56.89 )
( 4258 , 56.80 )
( 4259 , 56.76 )
( 4260 , 56.72 )
( 4261 , 56.60 )
( 4262 , 56.48 )
( 4263 , 56.36 )
( 4264 , 56.24 )
( 4265 , 56.36 )
( 4266 , 56.49 )
( 4267 , 56.62 )
( 4268 , 56.79 )
( 4269 , 56.91 )
( 4270 , 57.04 )
( 4271 , 57.03 )
( 4272 , 56.90 )
( 4273 , 57.03 )
( 4274 , 57.09 )
( 4275 , 57.07 )
( 4276 , 57.09 )
( 4277 , 57.09 )
( 4278 , 57.08 )
( 4279 , 57.15 )
( 4280 , 57.14 )
( 4281 , 57.18 )
( 4282 , 57.16 )
( 4283 , 57.19 )
( 4284 , 57.33 )
( 4285 , 57.50 )
( 4286 , 57.64 )
( 4287 , 57.76 )
( 4288 , 57.90 )
( 4289 , 58.02 )
( 4290 , 58.25 )
( 4291 , 58.38 )
( 4292 , 58.50 )
( 4293 , 58.56 )
( 4294 , 58.59 )
( 4295 , 58.63 )
( 4296 , 58.60 )
( 4297 , 58.65 )
( 4298 , 58.53 )
( 4299 , 58.40 )
( 4300 , 58.28 )
( 4301 , 58.27 )
( 4302 , 58.25 )
( 4303 , 58.27 )
( 4304 , 58.25 )
( 4305 , 58.25 )
( 4306 , 58.22 )
( 4307 , 58.19 )
( 4308 , 58.24 )
( 4309 , 58.37 )
( 4310 , 58.49 )
( 4311 , 58.61 )
( 4312 , 58.73 )
( 4313 , 58.86 )
( 4314 , 58.84 )
( 4315 , 58.81 )
( 4316 , 58.80 )
( 4317 , 58.77 )
( 4318 , 58.75 )
( 4319 , 58.72 )
( 4320 , 58.70 )
( 4321 , 58.87 )
( 4322 , 59.05 )
( 4323 , 59.32 )
( 4324 , 59.49 )
( 4325 , 59.70 )
( 4326 , 59.88 )
( 4327 , 60.15 )
( 4328 , 60.37 )
( 4329 , 60.55 )
( 4330 , 60.73 )
( 4331 , 60.96 )
( 4332 , 61.17 )
( 4333 , 61.38 )
( 4334 , 61.57 )
( 4335 , 61.75 )
( 4336 , 61.93 )
( 4337 , 62.10 )
( 4338 , 62.28 )
( 4339 , 62.47 )
( 4340 , 62.66 )
( 4341 , 62.93 )
( 4342 , 63.18 )
( 4343 , 63.53 )
( 4344 , 63.77 )
( 4345 , 64.05 )
( 4346 , 64.37 )
( 4347 , 64.59 )
( 4348 , 64.81 )
( 4349 , 65.21 )
( 4350 , 65.59 )
( 4351 , 65.84 )
( 4352 , 66.17 )
( 4353 , 66.51 )
( 4354 , 66.77 )
( 4355 , 67.02 )
( 4356 , 67.30 )
( 4357 , 67.59 )
( 4358 , 67.96 )
( 4359 , 68.23 )
( 4360 , 68.36 )
( 4361 , 68.48 )
( 4362 , 68.41 )
( 4363 , 68.30 )
( 4364 , 68.17 )
( 4365 , 68.12 )
( 4366 , 67.99 )
( 4367 , 67.94 )
( 4368 , 67.88 )
( 4369 , 67.85 )
( 4370 , 68.09 )
( 4371 , 68.33 )
( 4372 , 68.53 )
( 4373 , 68.73 )
( 4374 , 68.99 )
( 4375 , 69.02 )
( 4376 , 69.01 )
( 4377 , 68.95 )
( 4378 , 68.83 )
( 4379 , 68.70 )
( 4380 , 68.59 )
( 4381 , 68.47 )
( 4382 , 68.41 )
( 4383 , 68.29 )
( 4384 , 68.16 )
( 4385 , 68.05 )
( 4386 , 67.93 )
( 4387 , 67.82 )
( 4388 , 67.77 )
( 4389 , 67.71 )
( 4390 , 67.68 )
( 4391 , 67.71 )
( 4392 , 67.67 )
( 4393 , 67.68 )
( 4394 , 67.62 )
( 4395 , 67.59 )
( 4396 , 67.52 )
( 4397 , 67.59 )
( 4398 , 67.57 )
( 4399 , 67.70 )
( 4400 , 67.83 )
( 4401 , 67.82 )
( 4402 , 67.79 )
( 4403 , 67.77 )
( 4404 , 67.73 )
( 4405 , 67.71 )
( 4406 , 67.68 )
( 4407 , 67.72 )
( 4408 , 67.71 )
( 4409 , 67.89 )
( 4410 , 67.94 )
( 4411 , 68.01 )
( 4412 , 68.19 )
( 4413 , 68.21 )
( 4414 , 68.20 )
( 4415 , 68.27 )
( 4416 , 68.26 )
( 4417 , 68.16 )
( 4418 , 68.05 )
( 4419 , 68.02 )
( 4420 , 67.93 )
( 4421 , 67.80 )
( 4422 , 67.77 )
( 4423 , 67.70 )
( 4424 , 67.66 )
( 4425 , 67.55 )
( 4426 , 67.60 )
( 4427 , 67.48 )
( 4428 , 67.35 )
( 4429 , 67.25 )
( 4430 , 67.15 )
( 4431 , 67.02 )
( 4432 , 66.90 )
( 4433 , 66.84 )
( 4434 , 66.71 )
( 4435 , 66.59 )
( 4436 , 66.62 )
( 4437 , 66.73 )
( 4438 , 66.84 )
( 4439 , 66.88 )
( 4440 , 66.75 )
( 4441 , 66.80 )
( 4442 , 66.67 )
( 4443 , 66.55 )
( 4444 , 66.42 )
( 4445 , 66.41 )
( 4446 , 66.39 )
( 4447 , 66.43 )
( 4448 , 66.56 )
( 4449 , 66.61 )
( 4450 , 66.66 )
( 4451 , 66.71 )
( 4452 , 66.82 )
( 4453 , 66.70 )
( 4454 , 66.74 )
( 4455 , 66.66 )
( 4456 , 66.53 )
( 4457 , 66.50 )
( 4458 , 66.45 )
( 4459 , 66.39 )
( 4460 , 66.41 )
( 4461 , 66.41 )
( 4462 , 66.43 )
( 4463 , 66.41 )
( 4464 , 66.39 )
( 4465 , 66.43 )
( 4466 , 66.56 )
( 4467 , 66.70 )
( 4468 , 66.84 )
( 4469 , 66.88 )
( 4470 , 66.87 )
( 4471 , 66.86 )
( 4472 , 66.73 )
( 4473 , 66.98 )
( 4474 , 67.24 )
( 4475 , 67.37 )
( 4476 , 67.24 )
( 4477 , 67.15 )
( 4478 , 67.08 )
( 4479 , 66.95 )
( 4480 , 66.83 )
( 4481 , 66.71 )
( 4482 , 66.84 )
( 4483 , 67.01 )
( 4484 , 67.21 )
( 4485 , 67.41 )
( 4486 , 67.54 )
( 4487 , 67.68 )
( 4488 , 67.80 )
( 4489 , 68.08 )
( 4490 , 68.33 )
( 4491 , 68.49 )
( 4492 , 68.62 )
( 4493 , 68.70 )
( 4494 , 68.76 )
( 4495 , 68.63 )
( 4496 , 68.77 )
( 4497 , 68.88 )
( 4498 , 69.18 )
( 4499 , 69.47 )
( 4500 , 69.73 )
( 4501 , 69.98 )
( 4502 , 70.30 )
( 4503 , 70.64 )
( 4504 , 71.00 )
( 4505 , 71.34 )
( 4506 , 71.62 )
( 4507 , 71.88 )
( 4508 , 72.14 )
( 4509 , 72.46 )
( 4510 , 72.77 )
( 4511 , 72.95 )
( 4512 , 73.12 )
( 4513 , 73.45 )
( 4514 , 73.80 )
( 4515 , 74.16 )
( 4516 , 74.41 )
( 4517 , 74.67 )
( 4518 , 74.98 )
( 4519 , 75.24 )
( 4520 , 75.49 )
( 4521 , 75.74 )
( 4522 , 75.92 )
( 4523 , 76.09 )
( 4524 , 76.27 )
( 4525 , 76.45 )
( 4526 , 76.65 )
( 4527 , 76.84 )
( 4528 , 77.19 )
( 4529 , 77.43 )
( 4530 , 77.61 )
( 4531 , 77.79 )
( 4532 , 77.98 )
( 4533 , 78.26 )
( 4534 , 78.44 )
( 4535 , 78.65 )
( 4536 , 78.88 )
( 4537 , 79.06 )
( 4538 , 79.30 )
( 4539 , 79.55 )
( 4540 , 79.78 )
( 4541 , 79.98 )
( 4542 , 80.14 )
( 4543 , 80.51 )
( 4544 , 80.84 )
( 4545 , 81.14 )
( 4546 , 81.46 )
( 4547 , 81.77 )
( 4548 , 82.07 )
( 4549 , 82.20 )
( 4550 , 82.32 )
( 4551 , 82.53 )
( 4552 , 82.72 )
( 4553 , 82.91 )
( 4554 , 83.09 )
( 4555 , 83.31 )
( 4556 , 83.45 )
( 4557 , 83.76 )
( 4558 , 84.07 )
( 4559 , 84.41 )
( 4560 , 84.72 )
( 4561 , 85.03 )
( 4562 , 85.35 )
( 4563 , 85.66 )
( 4564 , 85.98 )
( 4565 , 86.27 )
( 4566 , 86.45 )
( 4567 , 86.63 )
( 4568 , 86.83 )
( 4569 , 87.02 )
( 4570 , 87.15 )
( 4571 , 87.34 )
( 4572 , 87.48 )
( 4573 , 87.66 )
( 4574 , 87.80 )
( 4575 , 87.95 )
( 4576 , 88.07 )
( 4577 , 88.20 )
( 4578 , 88.08 )
( 4579 , 87.95 )
( 4580 , 87.89 )
( 4581 , 87.82 )
( 4582 , 87.87 )
( 4583 , 87.74 )
( 4584 , 87.62 )
( 4585 , 87.52 )
( 4586 , 87.39 )
( 4587 , 87.09 )
( 4588 , 86.92 )
( 4589 , 86.77 )
( 4590 , 86.47 )
( 4591 , 86.20 )
( 4592 , 85.91 )
( 4593 , 85.71 )
( 4594 , 85.41 )
( 4595 , 85.11 )
( 4596 , 84.80 )
( 4597 , 84.54 )
( 4598 , 84.23 )
( 4599 , 84.01 )
( 4600 , 83.88 )
( 4601 , 83.60 )
( 4602 , 83.32 )
( 4603 , 83.12 )
( 4604 , 83.07 )
( 4605 , 82.98 )
( 4606 , 82.88 )
( 4607 , 82.82 )
( 4608 , 82.73 )
( 4609 , 82.66 )
( 4610 , 82.72 )
( 4611 , 82.74 )
( 4612 , 82.61 )
( 4613 , 82.41 )
( 4614 , 82.22 )
( 4615 , 82.02 )
( 4616 , 82.09 )
( 4617 , 82.07 )
( 4618 , 82.01 )
( 4619 , 81.92 )
( 4620 , 81.69 )
( 4621 , 81.55 )
( 4622 , 81.44 )
( 4623 , 81.13 )
( 4624 , 80.84 )
( 4625 , 80.54 )
( 4626 , 80.27 )
( 4627 , 79.96 )
( 4628 , 79.92 )
( 4629 , 79.73 )
( 4630 , 79.43 )
( 4631 , 79.13 )
( 4632 , 78.83 )
( 4633 , 78.62 )
( 4634 , 78.34 )
( 4635 , 78.04 )
( 4636 , 77.75 )
( 4637 , 77.45 )
( 4638 , 77.22 )
( 4639 , 77.05 )
( 4640 , 76.81 )
( 4641 , 76.53 )
( 4642 , 76.23 )
( 4643 , 76.13 )
( 4644 , 76.03 )
( 4645 , 75.90 )
( 4646 , 75.97 )
( 4647 , 75.99 )
( 4648 , 76.03 )
( 4649 , 75.73 )
( 4650 , 75.46 )
( 4651 , 75.30 )
( 4652 , 75.01 )
( 4653 , 74.95 )
( 4654 , 74.80 )
( 4655 , 74.51 )
( 4656 , 74.41 )
( 4657 , 74.34 )
( 4658 , 74.30 )
( 4659 , 74.30 )
( 4660 , 74.30 )
( 4661 , 74.11 )
( 4662 , 74.01 )
( 4663 , 74.04 )
( 4664 , 74.06 )
( 4665 , 73.80 )
( 4666 , 73.49 )
( 4667 , 73.30 )
( 4668 , 73.03 )
( 4669 , 72.76 )
( 4670 , 72.47 )
( 4671 , 72.20 )
( 4672 , 72.10 )
( 4673 , 71.84 )
( 4674 , 71.55 )
( 4675 , 71.27 )
( 4676 , 70.98 )
( 4677 , 70.69 )
( 4678 , 70.46 )
( 4679 , 70.27 )
( 4680 , 70.21 )
( 4681 , 69.91 )
( 4682 , 69.62 )
( 4683 , 69.32 )
( 4684 , 69.03 )
( 4685 , 68.84 )
( 4686 , 68.84 )
( 4687 , 68.54 )
( 4688 , 68.29 )
( 4689 , 68.05 )
( 4690 , 67.74 )
( 4691 , 67.67 )
( 4692 , 67.52 )
( 4693 , 67.41 )
( 4694 , 67.33 )
( 4695 , 67.03 )
( 4696 , 66.82 )
( 4697 , 66.52 )
( 4698 , 66.23 )
( 4699 , 65.95 )
( 4700 , 65.64 )
( 4701 , 65.35 )
( 4702 , 65.05 )
( 4703 , 64.95 )
( 4704 , 64.66 )
( 4705 , 64.37 )
( 4706 , 64.07 )
( 4707 , 63.86 )
( 4708 , 63.56 )
( 4709 , 63.26 )
( 4710 , 62.96 )
( 4711 , 62.80 )
( 4712 , 62.50 )
( 4713 , 62.25 )
( 4714 , 61.95 )
( 4715 , 61.71 )
( 4716 , 61.41 )
( 4717 , 61.12 )
( 4718 , 60.91 )
( 4719 , 60.73 )
( 4720 , 60.43 )
( 4721 , 60.20 )
( 4722 , 59.91 )
( 4723 , 59.61 )
( 4724 , 59.39 )
( 4725 , 59.11 )
( 4726 , 59.02 )
( 4727 , 58.74 )
( 4728 , 58.50 )
( 4729 , 58.21 )
( 4730 , 57.91 )
( 4731 , 57.66 )
( 4732 , 57.36 )
( 4733 , 57.05 )
( 4734 , 56.80 )
( 4735 , 56.73 )
( 4736 , 56.50 )
( 4737 , 56.20 )
( 4738 , 55.99 )
( 4739 , 55.70 )
( 4740 , 55.39 )
( 4741 , 55.38 )
( 4742 , 55.36 )
( 4743 , 55.35 )
( 4744 , 55.35 )
( 4745 , 55.34 )
( 4746 , 55.38 )
( 4747 , 55.54 )
( 4748 , 55.71 )
( 4749 , 55.84 )
( 4750 , 55.81 )
( 4751 , 55.69 )
( 4752 , 55.57 )
( 4753 , 55.48 )
( 4754 , 55.62 )
( 4755 , 55.63 )
( 4756 , 55.52 )
( 4757 , 55.56 )
( 4758 , 55.44 )
( 4759 , 55.32 )
( 4760 , 55.28 )
( 4761 , 55.16 )
( 4762 , 55.04 )
( 4763 , 54.92 )
( 4764 , 54.79 )
( 4765 , 54.49 )
( 4766 , 54.40 )
( 4767 , 54.10 )
( 4768 , 53.90 )
( 4769 , 53.60 )
( 4770 , 53.37 )
( 4771 , 53.07 )
( 4772 , 52.93 )
( 4773 , 52.84 )
( 4774 , 52.77 )
( 4775 , 52.69 )
( 4776 , 52.59 )
( 4777 , 52.51 )
( 4778 , 52.49 )
( 4779 , 52.28 )
( 4780 , 51.98 )
( 4781 , 51.68 )
( 4782 , 51.38 )
( 4783 , 51.11 )
( 4784 , 50.84 )
( 4785 , 50.58 )
( 4786 , 50.28 )
( 4787 , 50.09 )
( 4788 , 49.79 )
( 4789 , 49.49 )
( 4790 , 49.35 )
( 4791 , 49.16 )
( 4792 , 48.97 )
( 4793 , 48.67 )
( 4794 , 48.58 )
( 4795 , 48.48 )
( 4796 , 48.41 )
( 4797 , 48.11 )
( 4798 , 47.81 )
( 4799 , 47.65 )
( 4800 , 47.35 )
( 4801 , 47.05 )
( 4802 , 46.77 )
( 4803 , 46.48 )
( 4804 , 46.25 )
( 4805 , 45.96 )
( 4806 , 45.76 )
( 4807 , 45.46 )
( 4808 , 45.16 )
( 4809 , 44.86 )
( 4810 , 44.55 )
( 4811 , 44.36 )
( 4812 , 44.30 )
( 4813 , 44.05 )
( 4814 , 43.77 )
( 4815 , 43.48 )
( 4816 , 43.36 )
( 4817 , 43.35 )
( 4818 , 43.34 )
( 4819 , 43.43 )
( 4820 , 43.54 )
( 4821 , 43.64 )
( 4822 , 43.74 )
( 4823 , 43.84 )
( 4824 , 43.98 )
( 4825 , 44.13 )
( 4826 , 44.12 )
( 4827 , 44.15 )
( 4828 , 44.12 )
( 4829 , 44.09 )
( 4830 , 44.22 )
( 4831 , 44.49 )
( 4832 , 44.75 )
( 4833 , 44.87 )
( 4834 , 45.16 )
( 4835 , 45.48 )
( 4836 , 45.77 )
( 4837 , 46.02 )
( 4838 , 46.30 )
( 4839 , 46.54 )
( 4840 , 46.77 )
( 4841 , 46.71 )
( 4842 , 46.69 )
( 4843 , 46.57 )
( 4844 , 46.46 )
( 4845 , 46.34 )
( 4846 , 46.33 )
( 4847 , 46.29 )
( 4848 , 46.16 )
( 4849 , 46.12 )
( 4850 , 46.11 )
( 4851 , 46.07 )
( 4852 , 46.12 )
( 4853 , 46.04 )
( 4854 , 45.92 )
( 4855 , 45.79 )
( 4856 , 45.67 )
( 4857 , 45.55 )
( 4858 , 45.25 )
( 4859 , 44.97 )
( 4860 , 44.70 )
( 4861 , 44.49 )
( 4862 , 44.19 )
( 4863 , 43.89 )
( 4864 , 43.80 )
( 4865 , 43.51 )
( 4866 , 43.25 )
( 4867 , 43.06 )
( 4868 , 42.81 )
( 4869 , 42.57 )
( 4870 , 42.37 )
( 4871 , 42.18 )
( 4872 , 41.87 )
( 4873 , 41.61 )
( 4874 , 41.31 )
( 4875 , 41.03 )
( 4876 , 40.73 )
( 4877 , 40.43 )
( 4878 , 40.49 )
( 4879 , 40.19 )
( 4880 , 39.98 )
( 4881 , 39.84 )
( 4882 , 39.54 )
( 4883 , 39.26 )
( 4884 , 39.03 )
( 4885 , 38.73 )
( 4886 , 38.58 )
( 4887 , 38.28 )
( 4888 , 38.20 )
( 4889 , 38.10 )
( 4890 , 38.08 )
( 4891 , 37.96 )
( 4892 , 38.01 )
( 4893 , 38.14 )
( 4894 , 38.13 )
( 4895 , 38.01 )
( 4896 , 37.93 )
( 4897 , 37.84 )
( 4898 , 37.78 )
( 4899 , 37.71 )
( 4900 , 37.65 )
( 4901 , 37.59 )
( 4902 , 37.54 )
( 4903 , 37.27 )
( 4904 , 37.30 )
( 4905 , 37.41 )
( 4906 , 37.54 )
( 4907 , 37.44 )
( 4908 , 37.34 )
( 4909 , 37.07 )
( 4910 , 36.78 )
( 4911 , 36.53 )
( 4912 , 36.22 )
( 4913 , 36.16 )
( 4914 , 36.04 )
( 4915 , 36.12 )
( 4916 , 36.20 )
( 4917 , 36.11 )
( 4918 , 36.00 )
( 4919 , 35.89 )
( 4920 , 35.77 )
( 4921 , 35.70 )
( 4922 , 35.48 )
( 4923 , 35.21 )
( 4924 , 34.96 )
( 4925 , 34.77 )
( 4926 , 34.46 )
( 4927 , 34.18 )
( 4928 , 33.94 )
( 4929 , 33.64 )
( 4930 , 33.59 )
( 4931 , 33.29 )
( 4932 , 33.10 )
( 4933 , 32.80 )
( 4934 , 32.68 )
( 4935 , 32.38 )
( 4936 , 32.37 )
( 4937 , 32.35 )
( 4938 , 32.06 )
( 4939 , 31.88 )
( 4940 , 31.60 )
( 4941 , 31.54 )
( 4942 , 31.44 )
( 4943 , 31.17 )
( 4944 , 30.87 )
( 4945 , 30.64 )
( 4946 , 30.37 )
( 4947 , 30.07 )
( 4948 , 29.77 )
( 4949 , 29.47 )
( 4950 , 29.23 )
( 4951 , 29.02 )
( 4952 , 28.72 )
( 4953 , 28.67 )
( 4954 , 28.69 )
( 4955 , 28.63 )
( 4956 , 28.56 )
( 4957 , 28.33 )
( 4958 , 28.03 )
( 4959 , 27.73 )
( 4960 , 27.69 )
( 4961 , 27.39 )
( 4962 , 27.09 )
( 4963 , 27.01 )
( 4964 , 26.72 )
( 4965 , 26.48 )
( 4966 , 26.34 )
( 4967 , 26.39 )
( 4968 , 26.33 )
( 4969 , 26.38 )
( 4970 , 26.34 )
( 4971 , 26.42 )
( 4972 , 26.51 )
( 4973 , 26.46 )
( 4974 , 26.54 )
( 4975 , 26.49 )
( 4976 , 26.44 )
( 4977 , 26.38 )
( 4978 , 26.32 )
( 4979 , 26.26 )
( 4980 , 26.21 )
( 4981 , 26.17 )
( 4982 , 26.11 )
( 4983 , 26.13 )
( 4984 , 26.16 )
( 4985 , 26.04 )
( 4986 , 25.91 )
( 4987 , 25.97 )
( 4988 , 26.03 )
( 4989 , 25.91 )
( 4990 , 25.85 )
( 4991 , 25.80 )
( 4992 , 25.74 )
( 4993 , 25.66 )
( 4994 , 25.54 )
( 4995 , 25.59 )
( 4996 , 25.66 )
( 4997 , 25.74 )
( 4998 , 25.78 )
( 4999 , 25.87 )
( 5000 , 25.91 )
( 5001 , 25.80 )
( 5002 , 25.68 )
( 5003 , 25.81 )
( 5004 , 25.93 )
( 5005 , 26.06 )
( 5006 , 26.18 )
( 5007 , 26.37 )
( 5008 , 26.55 )
( 5009 , 26.28 )
( 5010 , 25.98 )
( 5011 , 25.79 )
( 5012 , 25.49 )
( 5013 , 25.20 )
( 5014 , 24.90 )
( 5015 , 24.60 )
( 5016 , 24.65 )
( 5017 , 24.54 )
( 5018 , 24.42 )
( 5019 , 24.45 )
( 5020 , 24.43 )
( 5021 , 24.40 )
( 5022 , 24.38 )
( 5023 , 24.50 )
( 5024 , 24.64 )
( 5025 , 24.78 )
( 5026 , 24.80 )
( 5027 , 24.75 )
( 5028 , 24.69 )
( 5029 , 24.64 )
( 5030 , 24.63 )
( 5031 , 24.76 )
( 5032 , 24.78 )
( 5033 , 24.72 )
( 5034 , 24.66 )
( 5035 , 24.61 )
( 5036 , 24.55 )
( 5037 , 24.47 )
( 5038 , 24.35 )
( 5039 , 24.40 )
( 5040 , 24.46 )
( 5041 , 24.50 )
( 5042 , 24.37 )
( 5043 , 24.26 )
( 5044 , 24.14 )
( 5045 , 24.02 )
( 5046 , 23.92 )
( 5047 , 23.80 )
( 5048 , 23.69 )
( 5049 , 23.60 )
( 5050 , 23.48 )
( 5051 , 23.53 )
( 5052 , 23.58 )
( 5053 , 23.62 )
( 5054 , 23.66 )
( 5055 , 23.55 )
( 5056 , 23.51 )
( 5057 , 23.47 )
( 5058 , 23.43 )
( 5059 , 23.53 )
( 5060 , 23.41 )
( 5061 , 23.29 )
( 5062 , 23.05 )
( 5063 , 22.78 )
( 5064 , 22.48 )
( 5065 , 22.18 )
( 5066 , 22.12 )
( 5067 , 22.06 )
( 5068 , 22.07 )
( 5069 , 22.04 )
( 5070 , 22.04 )
( 5071 , 22.10 )
( 5072 , 22.05 )
( 5073 , 22.17 )
( 5074 , 22.30 )
( 5075 , 22.24 )
( 5076 , 22.19 )
( 5077 , 22.13 )
( 5078 , 22.08 )
( 5079 , 22.03 )
( 5080 , 22.02 )
( 5081 , 21.96 )
( 5082 , 22.01 )
( 5083 , 22.13 )
( 5084 , 22.26 )
( 5085 , 22.30 )
( 5086 , 22.23 )
( 5087 , 22.36 )
( 5088 , 22.48 )
( 5089 , 22.62 )
( 5090 , 22.75 )
( 5091 , 22.88 )
( 5092 , 23.04 )
( 5093 , 23.28 )
( 5094 , 23.48 )
( 5095 , 23.63 )
( 5096 , 23.84 )
( 5097 , 24.03 )
( 5098 , 23.91 )
( 5099 , 23.79 )
( 5100 , 23.70 )
( 5101 , 23.57 )
( 5102 , 23.45 )
( 5103 , 23.64 )
( 5104 , 23.83 )
( 5105 , 24.00 )
( 5106 , 24.19 )
( 5107 , 24.37 )
( 5108 , 24.54 )
( 5109 , 24.82 )
( 5110 , 25.06 )
( 5111 , 25.30 )
( 5112 , 25.48 )
( 5113 , 25.66 )
( 5114 , 25.93 )
( 5115 , 26.10 )
( 5116 , 26.28 )
( 5117 , 26.51 )
( 5118 , 26.76 )
( 5119 , 26.90 )
( 5120 , 27.04 )
( 5121 , 27.17 )
( 5122 , 27.35 )
( 5123 , 27.49 )
( 5124 , 27.38 )
( 5125 , 27.26 )
( 5126 , 27.13 )
( 5127 , 27.09 )
( 5128 , 27.09 )
( 5129 , 27.07 )
( 5130 , 27.01 )
( 5131 , 26.96 )
( 5132 , 26.90 )
( 5133 , 27.00 )
( 5134 , 27.10 )
( 5135 , 27.20 )
( 5136 , 27.35 )
( 5137 , 27.50 )
( 5138 , 27.81 )
( 5139 , 28.04 )
( 5140 , 28.13 )
( 5141 , 28.26 )
( 5142 , 28.43 )
( 5143 , 28.64 )
( 5144 , 28.70 )
( 5145 , 28.70 )
( 5146 , 28.81 )
( 5147 , 28.79 )
( 5148 , 28.56 )
( 5149 , 28.28 )
( 5150 , 27.98 )
( 5151 , 27.68 )
( 5152 , 27.59 )
( 5153 , 27.53 )
( 5154 , 27.50 )
( 5155 , 27.45 )
( 5156 , 27.39 )
( 5157 , 27.33 )
( 5158 , 27.33 )
( 5159 , 27.35 )
( 5160 , 27.29 )
( 5161 , 27.35 )
( 5162 , 27.44 )
( 5163 , 27.38 )
( 5164 , 27.42 )
( 5165 , 27.39 )
( 5166 , 27.50 )
( 5167 , 27.59 )
( 5168 , 27.71 )
( 5169 , 27.83 )
( 5170 , 28.01 )
( 5171 , 28.15 )
( 5172 , 28.33 )
( 5173 , 28.30 )
( 5174 , 28.32 )
( 5175 , 28.36 )
( 5176 , 28.39 )
( 5177 , 28.46 )
( 5178 , 28.43 )
( 5179 , 28.13 )
( 5180 , 27.83 )
( 5181 , 27.54 )
( 5182 , 27.29 )
( 5183 , 27.05 )
( 5184 , 26.75 )
( 5185 , 26.57 )
( 5186 , 26.27 )
( 5187 , 26.02 )
( 5188 , 25.71 )
( 5189 , 25.59 )
( 5190 , 25.53 )
( 5191 , 25.27 )
( 5192 , 24.97 )
( 5193 , 24.78 )
( 5194 , 24.56 )
( 5195 , 24.29 )
( 5196 , 24.09 )
( 5197 , 23.79 )
( 5198 , 23.49 )
( 5199 , 23.36 )
( 5200 , 23.27 )
( 5201 , 23.17 )
( 5202 , 23.13 )
( 5203 , 22.83 )
( 5204 , 22.53 )
( 5205 , 22.23 )
( 5206 , 21.96 )
( 5207 , 21.86 )
( 5208 , 21.56 )
( 5209 , 21.58 )
( 5210 , 21.44 )
( 5211 , 21.14 )
( 5212 , 20.84 )
( 5213 , 20.61 )
( 5214 , 20.58 )
( 5215 , 20.59 )
( 5216 , 20.58 )
( 5217 , 20.28 )
( 5218 , 20.13 )
( 5219 , 19.83 )
( 5220 , 19.53 )
( 5221 , 19.25 )
( 5222 , 18.97 )
( 5223 , 18.74 )
( 5224 , 18.64 )
( 5225 , 18.38 )
( 5226 , 18.07 )
( 5227 , 17.84 )
( 5228 , 17.54 )
( 5229 , 17.25 )
( 5230 , 16.97 )
( 5231 , 16.67 )
( 5232 , 16.38 )
( 5233 , 16.08 )
( 5234 , 15.78 )
( 5235 , 15.59 )
( 5236 , 15.31 )
( 5237 , 15.25 )
( 5238 , 15.10 )
( 5239 , 14.81 )
( 5240 , 14.72 )
( 5241 , 14.62 )
( 5242 , 14.38 )
( 5243 , 14.31 )
( 5244 , 14.27 )
( 5245 , 14.22 )
( 5246 , 14.25 )
( 5247 , 14.21 )
( 5248 , 13.92 )
( 5249 , 13.77 )
( 5250 , 13.68 )
( 5251 , 13.58 )
( 5252 , 13.48 )
( 5253 , 13.18 )
( 5254 , 12.88 )
( 5255 , 12.68 )
( 5256 , 12.41 )
( 5257 , 12.13 )
( 5258 , 11.91 )
( 5259 , 11.62 )
( 5260 , 11.39 )
( 5261 , 11.13 )
( 5262 , 10.88 )
( 5263 , 10.59 )
( 5264 , 10.32 )
( 5265 , 10.25 )
( 5266 , 9.953 )
( 5267 , 9.742 )
( 5268 , 9.664 )
( 5269 , 9.518 )
( 5270 , 9.324 )
( 5271 , 9.054 )
( 5272 , 9.023 )
( 5273 , 8.958 )
( 5274 , 8.669 )
( 5275 , 8.390 )
( 5276 , 8.112 )
( 5277 , 7.910 )
( 5278 , 7.609 )
( 5279 , 7.313 )
( 5280 , 7.037 )
( 5281 , 6.763 )
( 5282 , 6.667 )
( 5283 , 6.402 )
( 5284 , 6.206 )
( 5285 , 5.905 )
( 5286 , 5.777 )
( 5287 , 5.540 )
( 5288 , 5.429 )
( 5289 , 5.283 )
( 5290 , 5.103 )
( 5291 , 4.802 )
( 5292 , 4.843 )
( 5293 , 4.753 )
( 5294 , 4.752 )
( 5295 , 4.646 )
( 5296 , 4.521 )
( 5297 , 4.637 )
( 5298 , 4.513 )
( 5299 , 4.410 )
( 5300 , 4.535 )
( 5301 , 4.660 )
( 5302 , 4.702 )
( 5303 , 4.577 )
( 5304 , 4.452 )
( 5305 , 4.383 )
( 5306 , 3.766 )
( 5307 , 2.515 )
( 5308 , 2.053 )
( 5309 , 0.000 )
};


==> H696780 <==
\addplot[color=yellow] coordinates{
( 0 , 5.843 )
( 1 , 6.253 )
( 2 , 6.646 )
( 3 , 6.880 )
( 4 , 7.131 )
( 5 , 7.377 )
( 6 , 7.599 )
( 7 , 7.859 )
( 8 , 8.125 )
( 9 , 8.349 )
( 10 , 8.652 )
( 11 , 8.875 )
( 12 , 9.146 )
( 13 , 9.374 )
( 14 , 9.609 )
( 15 , 9.704 )
( 16 , 9.704 )
( 17 , 9.705 )
( 18 , 9.777 )
( 19 , 9.862 )
( 20 , 9.931 )
( 21 , 9.993 )
( 22 , 10.02 )
( 23 , 10.07 )
( 24 , 10.16 )
( 25 , 10.31 )
( 26 , 10.33 )
( 27 , 10.63 )
( 28 , 10.88 )
( 29 , 11.10 )
( 30 , 11.38 )
( 31 , 11.80 )
( 32 , 12.10 )
( 33 , 12.46 )
( 34 , 12.79 )
( 35 , 13.07 )
( 36 , 13.31 )
( 37 , 13.57 )
( 38 , 13.79 )
( 39 , 14.01 )
( 40 , 14.23 )
( 41 , 14.62 )
( 42 , 14.99 )
( 43 , 15.37 )
( 44 , 15.73 )
( 45 , 16.09 )
( 46 , 16.43 )
( 47 , 16.65 )
( 48 , 17.00 )
( 49 , 17.35 )
( 50 , 17.60 )
( 51 , 17.83 )
( 52 , 18.05 )
( 53 , 18.13 )
( 54 , 18.24 )
( 55 , 18.38 )
( 56 , 18.46 )
( 57 , 18.51 )
( 58 , 18.54 )
( 59 , 18.56 )
( 60 , 18.56 )
( 61 , 18.78 )
( 62 , 18.85 )
( 63 , 18.85 )
( 64 , 18.87 )
( 65 , 18.88 )
( 66 , 18.98 )
( 67 , 19.02 )
( 68 , 19.02 )
( 69 , 18.99 )
( 70 , 18.96 )
( 71 , 18.82 )
( 72 , 18.69 )
( 73 , 18.39 )
( 74 , 18.25 )
( 75 , 18.04 )
( 76 , 17.87 )
( 77 , 17.57 )
( 78 , 17.40 )
( 79 , 17.19 )
( 80 , 16.89 )
( 81 , 16.62 )
( 82 , 16.55 )
( 83 , 16.41 )
( 84 , 16.11 )
( 85 , 15.81 )
( 86 , 15.57 )
( 87 , 15.51 )
( 88 , 15.62 )
( 89 , 15.52 )
( 90 , 15.22 )
( 91 , 15.26 )
( 92 , 14.96 )
( 93 , 14.72 )
( 94 , 14.42 )
( 95 , 14.20 )
( 96 , 14.10 )
( 97 , 14.15 )
( 98 , 14.02 )
( 99 , 13.88 )
( 100 , 13.58 )
( 101 , 13.28 )
( 102 , 13.46 )
( 103 , 13.44 )
( 104 , 13.67 )
( 105 , 13.89 )
( 106 , 14.13 )
( 107 , 14.43 )
( 108 , 14.72 )
( 109 , 14.94 )
( 110 , 15.19 )
( 111 , 15.45 )
( 112 , 15.67 )
( 113 , 15.89 )
( 114 , 15.91 )
( 115 , 15.91 )
( 116 , 16.26 )
( 117 , 16.71 )
( 118 , 17.04 )
( 119 , 17.38 )
( 120 , 17.46 )
( 121 , 17.48 )
( 122 , 17.56 )
( 123 , 17.69 )
( 124 , 17.75 )
( 125 , 18.02 )
( 126 , 18.43 )
( 127 , 18.69 )
( 128 , 19.00 )
( 129 , 19.23 )
( 130 , 19.45 )
( 131 , 19.45 )
( 132 , 19.45 )
( 133 , 19.54 )
( 134 , 19.55 )
( 135 , 19.55 )
( 136 , 19.55 )
( 137 , 19.55 )
( 138 , 19.59 )
( 139 , 19.59 )
( 140 , 19.59 )
( 141 , 19.74 )
( 142 , 19.74 )
( 143 , 19.75 )
( 144 , 19.93 )
( 145 , 19.93 )
( 146 , 19.93 )
( 147 , 19.93 )
( 148 , 19.98 )
( 149 , 19.98 )
( 150 , 20.02 )
( 151 , 20.06 )
( 152 , 20.10 )
( 153 , 20.11 )
( 154 , 20.11 )
( 155 , 20.32 )
( 156 , 20.40 )
( 157 , 20.40 )
( 158 , 20.47 )
( 159 , 20.52 )
( 160 , 20.59 )
( 161 , 20.59 )
( 162 , 20.59 )
( 163 , 20.59 )
( 164 , 20.59 )
( 165 , 20.89 )
( 166 , 21.28 )
( 167 , 21.56 )
( 168 , 21.78 )
( 169 , 22.08 )
( 170 , 22.32 )
( 171 , 22.33 )
( 172 , 22.35 )
( 173 , 22.36 )
( 174 , 22.38 )
( 175 , 22.38 )
( 176 , 22.38 )
( 177 , 22.39 )
( 178 , 22.47 )
( 179 , 22.51 )
( 180 , 22.51 )
( 181 , 22.52 )
( 182 , 22.52 )
( 183 , 22.52 )
( 184 , 22.57 )
( 185 , 22.57 )
( 186 , 22.57 )
( 187 , 22.59 )
( 188 , 22.59 )
( 189 , 22.60 )
( 190 , 22.85 )
( 191 , 22.85 )
( 192 , 22.85 )
( 193 , 22.91 )
( 194 , 22.94 )
( 195 , 22.94 )
( 196 , 22.94 )
( 197 , 22.94 )
( 198 , 22.94 )
( 199 , 22.96 )
( 200 , 22.98 )
( 201 , 23.22 )
( 202 , 23.36 )
( 203 , 23.51 )
( 204 , 23.53 )
( 205 , 23.53 )
( 206 , 23.53 )
( 207 , 23.59 )
( 208 , 23.59 )
( 209 , 23.85 )
( 210 , 24.14 )
( 211 , 24.37 )
( 212 , 24.68 )
( 213 , 24.98 )
( 214 , 25.40 )
( 215 , 25.85 )
( 216 , 26.25 )
( 217 , 26.54 )
( 218 , 26.82 )
( 219 , 26.83 )
( 220 , 26.93 )
( 221 , 27.00 )
( 222 , 27.14 )
( 223 , 27.10 )
( 224 , 27.10 )
( 225 , 27.04 )
( 226 , 27.05 )
( 227 , 27.02 )
( 228 , 27.04 )
( 229 , 27.01 )
( 230 , 27.33 )
( 231 , 27.63 )
( 232 , 27.95 )
( 233 , 28.25 )
( 234 , 28.55 )
( 235 , 28.85 )
( 236 , 29.26 )
( 237 , 29.58 )
( 238 , 29.88 )
( 239 , 30.20 )
( 240 , 30.60 )
( 241 , 30.90 )
( 242 , 31.21 )
( 243 , 31.52 )
( 244 , 31.90 )
( 245 , 32.26 )
( 246 , 32.70 )
( 247 , 33.10 )
( 248 , 33.42 )
( 249 , 33.82 )
( 250 , 34.12 )
( 251 , 34.45 )
( 252 , 34.75 )
( 253 , 35.16 )
( 254 , 35.47 )
( 255 , 35.77 )
( 256 , 36.07 )
( 257 , 36.38 )
( 258 , 36.70 )
( 259 , 37.00 )
( 260 , 37.30 )
( 261 , 37.60 )
( 262 , 37.95 )
( 263 , 38.32 )
( 264 , 38.65 )
( 265 , 38.95 )
( 266 , 39.25 )
( 267 , 39.60 )
( 268 , 39.90 )
( 269 , 40.25 )
( 270 , 40.56 )
( 271 , 40.86 )
( 272 , 41.32 )
( 273 , 41.68 )
( 274 , 42.03 )
( 275 , 42.33 )
( 276 , 42.67 )
( 277 , 43.01 )
( 278 , 43.38 )
( 279 , 43.68 )
( 280 , 43.98 )
( 281 , 44.29 )
( 282 , 44.67 )
( 283 , 44.98 )
( 284 , 45.28 )
( 285 , 45.58 )
( 286 , 45.91 )
( 287 , 46.23 )
( 288 , 46.64 )
( 289 , 46.96 )
( 290 , 47.29 )
( 291 , 47.65 )
( 292 , 48.03 )
( 293 , 48.37 )
( 294 , 48.71 )
( 295 , 49.11 )
( 296 , 49.32 )
( 297 , 49.58 )
( 298 , 49.79 )
( 299 , 50.01 )
( 300 , 50.29 )
( 301 , 50.66 )
( 302 , 50.93 )
( 303 , 51.11 )
( 304 , 51.29 )
( 305 , 51.46 )
( 306 , 51.64 )
( 307 , 51.92 )
( 308 , 52.12 )
( 309 , 52.33 )
( 310 , 52.55 )
( 311 , 52.72 )
( 312 , 53.04 )
( 313 , 53.29 )
( 314 , 53.53 )
( 315 , 53.78 )
( 316 , 54.05 )
( 317 , 54.40 )
( 318 , 54.75 )
( 319 , 55.00 )
( 320 , 55.26 )
( 321 , 55.52 )
( 322 , 55.75 )
( 323 , 55.98 )
( 324 , 56.05 )
( 325 , 56.12 )
( 326 , 56.19 )
( 327 , 56.44 )
( 328 , 56.64 )
( 329 , 56.85 )
( 330 , 57.02 )
( 331 , 57.19 )
( 332 , 57.26 )
( 333 , 57.32 )
( 334 , 57.39 )
( 335 , 57.49 )
( 336 , 57.79 )
( 337 , 58.03 )
( 338 , 58.33 )
( 339 , 58.64 )
( 340 , 58.95 )
( 341 , 59.16 )
( 342 , 59.34 )
( 343 , 59.44 )
( 344 , 59.71 )
( 345 , 60.12 )
( 346 , 60.46 )
( 347 , 60.81 )
( 348 , 61.14 )
( 349 , 61.45 )
( 350 , 61.76 )
( 351 , 61.96 )
( 352 , 62.31 )
( 353 , 62.68 )
( 354 , 63.00 )
( 355 , 63.29 )
( 356 , 63.70 )
( 357 , 64.07 )
( 358 , 64.36 )
( 359 , 64.57 )
( 360 , 64.80 )
( 361 , 65.04 )
( 362 , 65.24 )
( 363 , 65.45 )
( 364 , 65.76 )
( 365 , 66.12 )
( 366 , 66.15 )
( 367 , 66.12 )
( 368 , 66.10 )
( 369 , 66.08 )
( 370 , 66.15 )
( 371 , 66.12 )
( 372 , 66.10 )
( 373 , 66.07 )
( 374 , 66.05 )
( 375 , 66.02 )
( 376 , 66.05 )
( 377 , 66.14 )
( 378 , 66.11 )
( 379 , 66.09 )
( 380 , 66.11 )
( 381 , 66.08 )
( 382 , 66.07 )
( 383 , 66.01 )
( 384 , 65.98 )
( 385 , 65.97 )
( 386 , 65.87 )
( 387 , 65.93 )
( 388 , 66.02 )
( 389 , 66.13 )
( 390 , 66.24 )
( 391 , 66.17 )
( 392 , 66.05 )
( 393 , 65.93 )
( 394 , 65.80 )
( 395 , 65.78 )
( 396 , 65.70 )
( 397 , 65.59 )
( 398 , 65.46 )
( 399 , 65.41 )
( 400 , 65.46 )
( 401 , 65.52 )
( 402 , 65.65 )
( 403 , 65.73 )
( 404 , 65.70 )
( 405 , 65.64 )
( 406 , 65.59 )
( 407 , 65.61 )
( 408 , 65.62 )
( 409 , 65.63 )
( 410 , 65.58 )
( 411 , 65.52 )
( 412 , 65.25 )
( 413 , 64.95 )
( 414 , 64.65 )
( 415 , 64.43 )
( 416 , 64.30 )
( 417 , 64.05 )
( 418 , 63.79 )
( 419 , 63.49 )
( 420 , 63.32 )
( 421 , 63.02 )
( 422 , 62.78 )
( 423 , 62.59 )
( 424 , 62.29 )
( 425 , 62.01 )
( 426 , 61.81 )
( 427 , 61.79 )
( 428 , 61.75 )
( 429 , 61.62 )
( 430 , 61.47 )
( 431 , 61.38 )
( 432 , 61.28 )
( 433 , 60.98 )
( 434 , 60.78 )
( 435 , 60.48 )
( 436 , 60.25 )
( 437 , 59.95 )
( 438 , 59.66 )
( 439 , 59.40 )
( 440 , 59.28 )
( 441 , 58.98 )
( 442 , 58.75 )
( 443 , 58.52 )
( 444 , 58.21 )
( 445 , 57.92 )
( 446 , 57.67 )
( 447 , 57.42 )
( 448 , 57.12 )
( 449 , 56.85 )
( 450 , 56.54 )
( 451 , 56.42 )
( 452 , 56.29 )
( 453 , 55.99 )
( 454 , 55.69 )
( 455 , 55.59 )
( 456 , 55.30 )
( 457 , 55.09 )
( 458 , 54.79 )
( 459 , 54.48 )
( 460 , 54.18 )
( 461 , 54.09 )
( 462 , 53.79 )
( 463 , 53.49 )
( 464 , 53.19 )
( 465 , 52.89 )
( 466 , 52.59 )
( 467 , 52.29 )
( 468 , 51.98 )
( 469 , 51.86 )
( 470 , 51.62 )
( 471 , 51.48 )
( 472 , 51.21 )
( 473 , 50.91 )
( 474 , 50.61 )
( 475 , 50.33 )
( 476 , 50.12 )
( 477 , 49.82 )
( 478 , 49.52 )
( 479 , 49.22 )
( 480 , 49.20 )
( 481 , 49.01 )
( 482 , 48.71 )
( 483 , 48.41 )
( 484 , 48.19 )
( 485 , 47.94 )
( 486 , 47.81 )
( 487 , 47.70 )
( 488 , 47.41 )
( 489 , 47.14 )
( 490 , 47.04 )
( 491 , 46.79 )
( 492 , 46.49 )
( 493 , 46.19 )
( 494 , 45.89 )
( 495 , 45.62 )
( 496 , 45.32 )
( 497 , 45.06 )
( 498 , 44.76 )
( 499 , 44.46 )
( 500 , 44.18 )
( 501 , 44.04 )
( 502 , 43.74 )
( 503 , 43.46 )
( 504 , 43.16 )
( 505 , 42.89 )
( 506 , 42.59 )
( 507 , 42.28 )
( 508 , 42.06 )
( 509 , 42.09 )
( 510 , 41.79 )
( 511 , 41.50 )
( 512 , 41.20 )
( 513 , 41.05 )
( 514 , 40.76 )
( 515 , 40.67 )
( 516 , 40.37 )
( 517 , 40.16 )
( 518 , 39.86 )
( 519 , 39.63 )
( 520 , 39.33 )
( 521 , 39.03 )
( 522 , 38.74 )
( 523 , 38.44 )
( 524 , 38.36 )
( 525 , 38.27 )
( 526 , 38.14 )
( 527 , 38.07 )
( 528 , 37.95 )
( 529 , 38.11 )
( 530 , 38.24 )
( 531 , 38.36 )
( 532 , 38.54 )
( 533 , 38.70 )
( 534 , 38.96 )
( 535 , 39.14 )
( 536 , 39.32 )
( 537 , 39.51 )
( 538 , 39.82 )
( 539 , 40.01 )
( 540 , 40.20 )
( 541 , 40.24 )
( 542 , 40.21 )
( 543 , 40.00 )
( 544 , 39.70 )
( 545 , 39.40 )
( 546 , 39.20 )
( 547 , 38.89 )
( 548 , 38.59 )
( 549 , 38.48 )
( 550 , 38.27 )
( 551 , 37.96 )
( 552 , 38.00 )
( 553 , 38.05 )
( 554 , 37.75 )
( 555 , 37.69 )
( 556 , 37.60 )
( 557 , 37.51 )
( 558 , 37.49 )
( 559 , 37.48 )
( 560 , 37.48 )
( 561 , 37.23 )
( 562 , 37.00 )
( 563 , 36.75 )
( 564 , 36.55 )
( 565 , 36.30 )
( 566 , 36.04 )
( 567 , 35.78 )
( 568 , 35.48 )
( 569 , 35.18 )
( 570 , 35.28 )
( 571 , 35.37 )
( 572 , 35.27 )
( 573 , 35.17 )
( 574 , 34.87 )
( 575 , 34.64 )
( 576 , 34.34 )
( 577 , 34.25 )
( 578 , 33.95 )
( 579 , 33.77 )
( 580 , 33.47 )
( 581 , 33.26 )
( 582 , 33.00 )
( 583 , 32.77 )
( 584 , 32.71 )
( 585 , 32.59 )
( 586 , 32.46 )
( 587 , 32.52 )
( 588 , 32.56 )
( 589 , 32.57 )
( 590 , 32.53 )
( 591 , 32.40 )
( 592 , 32.28 )
( 593 , 32.16 )
( 594 , 32.05 )
( 595 , 32.12 )
( 596 , 32.18 )
( 597 , 32.30 )
( 598 , 32.27 )
( 599 , 32.25 )
( 600 , 32.28 )
( 601 , 32.18 )
( 602 , 32.06 )
( 603 , 32.04 )
( 604 , 32.00 )
( 605 , 31.87 )
( 606 , 32.00 )
( 607 , 32.13 )
( 608 , 32.45 )
( 609 , 32.71 )
( 610 , 32.98 )
( 611 , 33.29 )
( 612 , 33.48 )
( 613 , 33.61 )
( 614 , 33.50 )
( 615 , 33.37 )
( 616 , 33.29 )
( 617 , 33.17 )
( 618 , 33.04 )
( 619 , 32.92 )
( 620 , 33.05 )
( 621 , 33.09 )
( 622 , 32.96 )
( 623 , 32.66 )
( 624 , 32.40 )
( 625 , 32.10 )
( 626 , 31.80 )
( 627 , 31.50 )
( 628 , 31.20 )
( 629 , 30.90 )
( 630 , 30.60 )
( 631 , 30.33 )
( 632 , 30.03 )
( 633 , 29.74 )
( 634 , 29.45 )
( 635 , 29.38 )
( 636 , 29.32 )
( 637 , 29.03 )
( 638 , 28.73 )
( 639 , 28.43 )
( 640 , 28.13 )
( 641 , 27.86 )
( 642 , 27.62 )
( 643 , 27.36 )
( 644 , 27.12 )
( 645 , 26.85 )
( 646 , 26.55 )
( 647 , 26.44 )
( 648 , 26.40 )
( 649 , 26.38 )
( 650 , 26.11 )
( 651 , 25.83 )
( 652 , 25.53 )
( 653 , 25.43 )
( 654 , 25.19 )
( 655 , 25.12 )
( 656 , 25.03 )
( 657 , 24.80 )
( 658 , 24.58 )
( 659 , 24.31 )
( 660 , 24.03 )
( 661 , 23.72 )
( 662 , 23.51 )
( 663 , 23.24 )
( 664 , 23.01 )
( 665 , 22.71 )
( 666 , 22.62 )
( 667 , 22.32 )
( 668 , 22.12 )
( 669 , 21.86 )
( 670 , 21.56 )
( 671 , 21.26 )
( 672 , 21.08 )
( 673 , 20.80 )
( 674 , 20.71 )
( 675 , 20.51 )
( 676 , 20.21 )
( 677 , 19.91 )
( 678 , 19.61 )
( 679 , 19.52 )
( 680 , 19.29 )
( 681 , 19.19 )
( 682 , 19.08 )
( 683 , 19.11 )
( 684 , 18.98 )
( 685 , 18.97 )
( 686 , 18.89 )
( 687 , 18.83 )
( 688 , 18.53 )
( 689 , 18.44 )
( 690 , 18.33 )
( 691 , 18.14 )
( 692 , 18.05 )
( 693 , 17.95 )
( 694 , 17.70 )
( 695 , 17.72 )
( 696 , 17.71 )
( 697 , 17.69 )
( 698 , 17.59 )
( 699 , 17.29 )
( 700 , 17.00 )
( 701 , 16.86 )
( 702 , 16.57 )
( 703 , 16.27 )
( 704 , 16.16 )
( 705 , 16.10 )
( 706 , 15.98 )
( 707 , 16.02 )
( 708 , 15.89 )
( 709 , 15.84 )
( 710 , 15.86 )
( 711 , 15.80 )
( 712 , 15.78 )
( 713 , 15.80 )
( 714 , 15.77 )
( 715 , 15.97 )
( 716 , 16.18 )
( 717 , 16.37 )
( 718 , 16.51 )
( 719 , 16.60 )
( 720 , 16.70 )
( 721 , 16.83 )
( 722 , 16.83 )
( 723 , 16.83 )
( 724 , 16.81 )
( 725 , 16.76 )
( 726 , 16.73 )
( 727 , 16.61 )
( 728 , 16.48 )
( 729 , 16.66 )
( 730 , 17.04 )
( 731 , 17.37 )
( 732 , 17.59 )
( 733 , 17.84 )
( 734 , 18.07 )
( 735 , 18.30 )
( 736 , 18.52 )
( 737 , 18.85 )
( 738 , 19.17 )
( 739 , 19.49 )
( 740 , 19.89 )
( 741 , 20.09 )
( 742 , 20.38 )
( 743 , 20.59 )
( 744 , 20.81 )
( 745 , 21.02 )
( 746 , 21.23 )
( 747 , 21.56 )
( 748 , 21.90 )
( 749 , 22.12 )
( 750 , 22.39 )
( 751 , 22.57 )
( 752 , 22.90 )
( 753 , 23.08 )
( 754 , 23.25 )
( 755 , 23.44 )
( 756 , 23.64 )
( 757 , 23.82 )
( 758 , 24.08 )
( 759 , 24.35 )
( 760 , 24.59 )
( 761 , 24.82 )
( 762 , 25.06 )
( 763 , 25.30 )
( 764 , 25.54 )
( 765 , 25.79 )
( 766 , 26.04 )
( 767 , 26.30 )
( 768 , 26.60 )
( 769 , 26.88 )
( 770 , 27.12 )
( 771 , 27.29 )
( 772 , 27.54 )
( 773 , 27.77 )
( 774 , 28.05 )
( 775 , 28.28 )
( 776 , 28.51 )
( 777 , 28.74 )
( 778 , 29.00 )
( 779 , 29.34 )
( 780 , 29.57 )
( 781 , 29.81 )
( 782 , 29.89 )
( 783 , 30.18 )
( 784 , 30.24 )
( 785 , 30.36 )
( 786 , 30.47 )
( 787 , 30.58 )
( 788 , 30.58 )
( 789 , 30.65 )
( 790 , 30.71 )
( 791 , 30.71 )
( 792 , 30.79 )
( 793 , 30.94 )
( 794 , 31.08 )
( 795 , 31.11 )
( 796 , 31.12 )
( 797 , 31.16 )
( 798 , 31.18 )
( 799 , 31.29 )
( 800 , 31.36 )
( 801 , 31.39 )
( 802 , 31.44 )
( 803 , 31.49 )
( 804 , 31.53 )
( 805 , 31.53 )
( 806 , 31.58 )
( 807 , 31.60 )
( 808 , 31.60 )
( 809 , 31.62 )
( 810 , 31.66 )
( 811 , 31.70 )
( 812 , 31.70 )
( 813 , 31.71 )
( 814 , 31.82 )
( 815 , 31.82 )
( 816 , 31.99 )
( 817 , 32.05 )
( 818 , 32.05 )
( 819 , 32.31 )
( 820 , 32.44 )
( 821 , 32.59 )
( 822 , 32.71 )
( 823 , 32.86 )
( 824 , 32.97 )
( 825 , 33.10 )
( 826 , 33.21 )
( 827 , 33.43 )
( 828 , 33.53 )
( 829 , 33.62 )
( 830 , 33.69 )
( 831 , 33.76 )
( 832 , 33.96 )
( 833 , 34.27 )
( 834 , 34.38 )
( 835 , 34.60 )
( 836 , 34.81 )
( 837 , 35.02 )
( 838 , 35.09 )
( 839 , 35.16 )
( 840 , 35.23 )
( 841 , 35.43 )
( 842 , 35.67 )
( 843 , 35.91 )
( 844 , 36.17 )
( 845 , 36.40 )
( 846 , 36.50 )
( 847 , 36.61 )
( 848 , 36.69 )
( 849 , 36.76 )
( 850 , 36.86 )
( 851 , 36.95 )
( 852 , 37.04 )
( 853 , 37.13 )
( 854 , 37.14 )
( 855 , 37.15 )
( 856 , 37.36 )
( 857 , 37.50 )
( 858 , 37.50 )
( 859 , 37.50 )
( 860 , 37.59 )
( 861 , 37.60 )
( 862 , 37.61 )
( 863 , 37.66 )
( 864 , 37.66 )
( 865 , 37.68 )
( 866 , 37.86 )
( 867 , 37.92 )
( 868 , 38.02 )
( 869 , 38.12 )
( 870 , 38.21 )
( 871 , 38.30 )
( 872 , 38.51 )
( 873 , 38.60 )
( 874 , 38.70 )
( 875 , 38.85 )
( 876 , 38.98 )
( 877 , 39.10 )
( 878 , 39.37 )
( 879 , 39.65 )
( 880 , 39.91 )
( 881 , 40.19 )
( 882 , 40.32 )
( 883 , 40.45 )
( 884 , 40.57 )
( 885 , 40.70 )
( 886 , 40.57 )
( 887 , 40.57 )
( 888 , 40.66 )
( 889 , 40.77 )
( 890 , 40.88 )
( 891 , 41.00 )
( 892 , 40.99 )
( 893 , 40.98 )
( 894 , 41.06 )
( 895 , 41.06 )
( 896 , 41.20 )
( 897 , 41.32 )
( 898 , 41.45 )
( 899 , 41.60 )
( 900 , 41.51 )
( 901 , 41.48 )
( 902 , 41.36 )
( 903 , 41.23 )
( 904 , 41.30 )
( 905 , 41.29 )
( 906 , 41.32 )
( 907 , 41.30 )
( 908 , 41.34 )
( 909 , 41.28 )
( 910 , 41.16 )
( 911 , 41.04 )
( 912 , 40.91 )
( 913 , 40.80 )
( 914 , 40.98 )
( 915 , 41.11 )
( 916 , 41.27 )
( 917 , 41.45 )
( 918 , 41.68 )
( 919 , 41.86 )
( 920 , 42.06 )
( 921 , 42.25 )
( 922 , 42.41 )
( 923 , 42.62 )
( 924 , 42.75 )
( 925 , 42.88 )
( 926 , 43.07 )
( 927 , 43.20 )
( 928 , 43.39 )
( 929 , 43.54 )
( 930 , 43.66 )
( 931 , 43.87 )
( 932 , 44.08 )
( 933 , 44.29 )
( 934 , 44.46 )
( 935 , 44.59 )
( 936 , 44.71 )
( 937 , 44.84 )
( 938 , 45.00 )
( 939 , 45.22 )
( 940 , 45.18 )
( 941 , 45.07 )
( 942 , 44.95 )
( 943 , 44.82 )
( 944 , 44.96 )
( 945 , 45.06 )
( 946 , 45.13 )
( 947 , 45.17 )
( 948 , 45.21 )
( 949 , 45.18 )
( 950 , 45.07 )
( 951 , 45.00 )
( 952 , 44.95 )
( 953 , 44.82 )
( 954 , 44.70 )
( 955 , 44.82 )
( 956 , 44.89 )
( 957 , 44.93 )
( 958 , 45.00 )
( 959 , 44.88 )
( 960 , 44.76 )
( 961 , 44.63 )
( 962 , 44.61 )
( 963 , 44.57 )
( 964 , 44.45 )
( 965 , 44.36 )
( 966 , 44.27 )
( 967 , 44.30 )
( 968 , 44.20 )
( 969 , 44.11 )
( 970 , 44.07 )
( 971 , 43.77 )
( 972 , 43.47 )
( 973 , 43.20 )
( 974 , 42.98 )
( 975 , 42.68 )
( 976 , 42.41 )
( 977 , 42.12 )
( 978 , 42.09 )
( 979 , 41.94 )
( 980 , 41.80 )
( 981 , 41.49 )
( 982 , 41.19 )
( 983 , 40.96 )
( 984 , 40.66 )
( 985 , 40.36 )
( 986 , 40.07 )
( 987 , 39.97 )
( 988 , 39.67 )
( 989 , 39.62 )
( 990 , 39.57 )
( 991 , 39.50 )
( 992 , 39.20 )
( 993 , 39.14 )
( 994 , 38.93 )
( 995 , 38.71 )
( 996 , 38.48 )
( 997 , 38.43 )
( 998 , 38.29 )
( 999 , 38.08 )
( 1000 , 37.81 )
( 1001 , 37.54 )
( 1002 , 37.26 )
( 1003 , 36.96 )
( 1004 , 36.77 )
( 1005 , 36.46 )
( 1006 , 36.39 )
( 1007 , 36.43 )
( 1008 , 36.33 )
( 1009 , 36.26 )
( 1010 , 35.98 )
( 1011 , 35.68 )
( 1012 , 35.38 )
( 1013 , 35.08 )
( 1014 , 34.96 )
( 1015 , 34.66 )
( 1016 , 34.36 )
( 1017 , 34.06 )
( 1018 , 33.76 )
( 1019 , 33.71 )
( 1020 , 33.62 )
( 1021 , 33.60 )
( 1022 , 33.36 )
( 1023 , 33.07 )
( 1024 , 32.80 )
( 1025 , 32.52 )
( 1026 , 32.34 )
( 1027 , 32.04 )
( 1028 , 31.97 )
( 1029 , 31.67 )
( 1030 , 31.38 )
( 1031 , 31.28 )
( 1032 , 31.26 )
( 1033 , 31.16 )
( 1034 , 30.86 )
( 1035 , 30.74 )
( 1036 , 30.44 )
( 1037 , 30.13 )
( 1038 , 29.98 )
( 1039 , 29.68 )
( 1040 , 29.38 )
( 1041 , 29.24 )
( 1042 , 28.95 )
( 1043 , 28.86 )
( 1044 , 28.63 )
( 1045 , 28.72 )
( 1046 , 28.63 )
( 1047 , 28.43 )
( 1048 , 28.25 )
( 1049 , 28.09 )
( 1050 , 27.79 )
( 1051 , 27.66 )
( 1052 , 27.47 )
( 1053 , 27.17 )
( 1054 , 27.31 )
( 1055 , 27.36 )
( 1056 , 27.36 )
( 1057 , 27.40 )
( 1058 , 27.37 )
( 1059 , 27.19 )
( 1060 , 26.90 )
( 1061 , 26.60 )
( 1062 , 26.30 )
( 1063 , 26.10 )
( 1064 , 25.83 )
( 1065 , 25.53 )
( 1066 , 25.58 )
( 1067 , 25.53 )
( 1068 , 25.53 )
( 1069 , 25.47 )
( 1070 , 25.46 )
( 1071 , 25.45 )
( 1072 , 25.39 )
( 1073 , 25.42 )
( 1074 , 25.41 )
( 1075 , 25.40 )
( 1076 , 25.27 )
( 1077 , 25.15 )
( 1078 , 25.27 )
( 1079 , 25.44 )
( 1080 , 25.66 )
( 1081 , 25.88 )
( 1082 , 26.01 )
( 1083 , 26.14 )
( 1084 , 26.35 )
( 1085 , 26.55 )
( 1086 , 26.71 )
( 1087 , 26.84 )
( 1088 , 27.09 )
( 1089 , 27.36 )
( 1090 , 27.66 )
( 1091 , 27.79 )
( 1092 , 27.97 )
( 1093 , 27.87 )
( 1094 , 27.75 )
( 1095 , 27.66 )
( 1096 , 27.57 )
( 1097 , 27.45 )
( 1098 , 27.33 )
( 1099 , 27.20 )
( 1100 , 26.97 )
( 1101 , 26.74 )
( 1102 , 26.44 )
( 1103 , 26.31 )
( 1104 , 26.22 )
( 1105 , 26.16 )
( 1106 , 26.06 )
( 1107 , 25.77 )
( 1108 , 25.54 )
( 1109 , 25.32 )
( 1110 , 25.02 )
( 1111 , 24.89 )
( 1112 , 25.09 )
( 1113 , 25.20 )
( 1114 , 25.34 )
( 1115 , 25.49 )
( 1116 , 25.66 )
( 1117 , 25.83 )
( 1118 , 26.04 )
( 1119 , 26.23 )
( 1120 , 26.22 )
( 1121 , 26.23 )
( 1122 , 26.11 )
( 1123 , 25.98 )
( 1124 , 25.95 )
( 1125 , 25.83 )
( 1126 , 25.76 )
( 1127 , 25.73 )
( 1128 , 25.71 )
( 1129 , 25.60 )
( 1130 , 25.48 )
( 1131 , 25.36 )
( 1132 , 25.23 )
( 1133 , 25.26 )
( 1134 , 25.31 )
( 1135 , 25.26 )
( 1136 , 25.21 )
( 1137 , 25.21 )
( 1138 , 25.08 )
( 1139 , 24.96 )
( 1140 , 25.30 )
( 1141 , 25.54 )
( 1142 , 25.75 )
( 1143 , 26.02 )
( 1144 , 26.25 )
( 1145 , 26.48 )
( 1146 , 26.68 )
( 1147 , 26.86 )
( 1148 , 27.04 )
( 1149 , 27.21 )
( 1150 , 27.39 )
( 1151 , 27.62 )
( 1152 , 27.81 )
( 1153 , 27.80 )
( 1154 , 27.71 )
( 1155 , 27.69 )
( 1156 , 27.66 )
( 1157 , 27.65 )
( 1158 , 27.61 )
( 1159 , 27.35 )
( 1160 , 27.06 )
( 1161 , 26.85 )
( 1162 , 26.55 )
( 1163 , 26.27 )
( 1164 , 26.40 )
( 1165 , 26.50 )
( 1166 , 26.41 )
( 1167 , 26.27 )
( 1168 , 26.13 )
( 1169 , 25.98 )
( 1170 , 25.84 )
( 1171 , 25.54 )
( 1172 , 25.42 )
( 1173 , 25.46 )
( 1174 , 25.37 )
( 1175 , 25.15 )
( 1176 , 25.06 )
( 1177 , 24.76 )
( 1178 , 24.46 )
( 1179 , 24.41 )
( 1180 , 24.11 )
( 1181 , 24.10 )
( 1182 , 24.01 )
( 1183 , 23.83 )
( 1184 , 23.57 )
( 1185 , 23.45 )
( 1186 , 23.14 )
( 1187 , 23.28 )
( 1188 , 23.30 )
( 1189 , 23.34 )
( 1190 , 23.28 )
( 1191 , 23.25 )
( 1192 , 23.29 )
( 1193 , 23.35 )
( 1194 , 23.40 )
( 1195 , 23.42 )
( 1196 , 23.47 )
( 1197 , 23.48 )
( 1198 , 23.49 )
( 1199 , 23.43 )
( 1200 , 23.38 )
( 1201 , 23.33 )
( 1202 , 23.33 )
( 1203 , 23.33 )
( 1204 , 23.36 )
( 1205 , 23.38 )
( 1206 , 23.42 )
( 1207 , 23.42 )
( 1208 , 23.58 )
( 1209 , 23.61 )
( 1210 , 23.61 )
( 1211 , 23.64 )
( 1212 , 23.64 )
( 1213 , 23.64 )
( 1214 , 23.64 )
( 1215 , 23.79 )
( 1216 , 23.94 )
( 1217 , 24.13 )
( 1218 , 24.29 )
( 1219 , 24.46 )
( 1220 , 24.62 )
( 1221 , 24.66 )
( 1222 , 24.68 )
( 1223 , 24.92 )
( 1224 , 25.26 )
( 1225 , 25.52 )
( 1226 , 25.74 )
( 1227 , 26.01 )
( 1228 , 26.01 )
( 1229 , 26.05 )
( 1230 , 26.07 )
( 1231 , 26.07 )
( 1232 , 26.09 )
( 1233 , 26.13 )
( 1234 , 26.13 )
( 1235 , 26.30 )
( 1236 , 26.45 )
( 1237 , 26.55 )
( 1238 , 26.55 )
( 1239 , 26.61 )
( 1240 , 26.69 )
( 1241 , 26.77 )
( 1242 , 26.79 )
( 1243 , 26.87 )
( 1244 , 26.92 )
( 1245 , 26.97 )
( 1246 , 26.99 )
( 1247 , 26.94 )
( 1248 , 26.88 )
( 1249 , 26.58 )
( 1250 , 26.28 )
( 1251 , 25.98 )
( 1252 , 25.68 )
( 1253 , 25.49 )
( 1254 , 25.40 )
( 1255 , 25.12 )
( 1256 , 24.97 )
( 1257 , 24.67 )
( 1258 , 24.48 )
( 1259 , 24.19 )
( 1260 , 23.89 )
( 1261 , 23.70 )
( 1262 , 23.39 )
( 1263 , 23.38 )
( 1264 , 23.12 )
( 1265 , 22.82 )
( 1266 , 22.80 )
( 1267 , 22.71 )
( 1268 , 22.72 )
( 1269 , 22.62 )
( 1270 , 22.53 )
( 1271 , 22.43 )
( 1272 , 22.41 )
( 1273 , 22.40 )
( 1274 , 22.23 )
( 1275 , 21.96 )
( 1276 , 21.87 )
( 1277 , 21.57 )
( 1278 , 21.48 )
( 1279 , 21.52 )
( 1280 , 21.43 )
( 1281 , 21.28 )
( 1282 , 21.24 )
( 1283 , 21.19 )
( 1284 , 21.04 )
( 1285 , 20.99 )
( 1286 , 20.99 )
( 1287 , 21.01 )
( 1288 , 21.08 )
( 1289 , 21.00 )
( 1290 , 20.92 )
( 1291 , 20.62 )
( 1292 , 20.58 )
( 1293 , 20.30 )
( 1294 , 20.11 )
( 1295 , 20.08 )
( 1296 , 20.07 )
( 1297 , 19.98 )
( 1298 , 19.97 )
( 1299 , 19.88 )
( 1300 , 19.58 )
( 1301 , 19.54 )
( 1302 , 19.61 )
( 1303 , 19.42 )
( 1304 , 19.12 )
( 1305 , 18.82 )
( 1306 , 19.12 )
( 1307 , 19.44 )
( 1308 , 19.68 )
( 1309 , 19.68 )
( 1310 , 20.01 )
( 1311 , 20.34 )
( 1312 , 20.33 )
( 1313 , 20.30 )
( 1314 , 20.25 )
( 1315 , 20.26 )
( 1316 , 20.26 )
( 1317 , 20.26 )
( 1318 , 20.32 )
( 1319 , 20.41 )
( 1320 , 20.48 )
( 1321 , 20.53 )
( 1322 , 20.48 )
( 1323 , 20.36 )
( 1324 , 20.23 )
( 1325 , 20.36 )
( 1326 , 20.49 )
( 1327 , 20.64 )
( 1328 , 20.80 )
( 1329 , 20.93 )
( 1330 , 21.25 )
( 1331 , 21.51 )
( 1332 , 21.64 )
( 1333 , 21.77 )
( 1334 , 21.89 )
( 1335 , 22.08 )
( 1336 , 22.25 )
( 1337 , 22.37 )
( 1338 , 22.51 )
( 1339 , 22.68 )
( 1340 , 22.83 )
( 1341 , 23.10 )
( 1342 , 23.38 )
( 1343 , 23.64 )
( 1344 , 23.77 )
( 1345 , 24.02 )
( 1346 , 24.15 )
( 1347 , 24.27 )
( 1348 , 24.15 )
( 1349 , 24.23 )
( 1350 , 24.30 )
( 1351 , 24.37 )
( 1352 , 24.12 )
( 1353 , 23.82 )
( 1354 , 23.53 )
( 1355 , 23.30 )
( 1356 , 23.01 )
( 1357 , 22.71 )
( 1358 , 22.41 )
( 1359 , 22.27 )
( 1360 , 22.15 )
( 1361 , 21.87 )
( 1362 , 21.60 )
( 1363 , 21.60 )
( 1364 , 21.50 )
( 1365 , 21.46 )
( 1366 , 21.20 )
( 1367 , 20.90 )
( 1368 , 20.64 )
( 1369 , 20.34 )
( 1370 , 20.04 )
( 1371 , 19.74 )
( 1372 , 19.82 )
( 1373 , 19.90 )
( 1374 , 20.07 )
( 1375 , 20.07 )
( 1376 , 20.07 )
( 1377 , 20.09 )
( 1378 , 20.09 )
( 1379 , 20.09 )
( 1380 , 20.24 )
( 1381 , 20.28 )
( 1382 , 20.48 )
( 1383 , 20.65 )
( 1384 , 20.82 )
( 1385 , 20.97 )
( 1386 , 21.14 )
( 1387 , 21.20 )
( 1388 , 21.27 )
( 1389 , 21.27 )
( 1390 , 21.44 )
( 1391 , 21.54 )
( 1392 , 21.55 )
( 1393 , 21.67 )
( 1394 , 21.61 )
( 1395 , 21.65 )
( 1396 , 21.70 )
( 1397 , 21.76 )
( 1398 , 21.82 )
( 1399 , 21.78 )
( 1400 , 21.81 )
( 1401 , 21.85 )
( 1402 , 22.00 )
( 1403 , 22.13 )
( 1404 , 22.07 )
( 1405 , 21.95 )
( 1406 , 21.85 )
( 1407 , 21.76 )
( 1408 , 21.63 )
( 1409 , 21.53 )
( 1410 , 21.41 )
( 1411 , 21.29 )
( 1412 , 21.16 )
( 1413 , 21.07 )
( 1414 , 20.98 )
( 1415 , 20.95 )
( 1416 , 20.83 )
( 1417 , 20.73 )
( 1418 , 20.44 )
( 1419 , 20.47 )
( 1420 , 20.32 )
( 1421 , 20.02 )
( 1422 , 19.72 )
( 1423 , 19.42 )
( 1424 , 19.12 )
( 1425 , 18.82 )
( 1426 , 18.53 )
( 1427 , 18.30 )
( 1428 , 18.00 )
( 1429 , 17.70 )
( 1430 , 17.56 )
( 1431 , 17.42 )
( 1432 , 17.36 )
( 1433 , 17.05 )
( 1434 , 16.75 )
( 1435 , 16.56 )
( 1436 , 16.53 )
( 1437 , 16.23 )
( 1438 , 16.22 )
( 1439 , 16.31 )
( 1440 , 16.30 )
( 1441 , 16.17 )
( 1442 , 16.34 )
( 1443 , 16.47 )
( 1444 , 16.35 )
( 1445 , 16.22 )
( 1446 , 16.24 )
( 1447 , 16.14 )
( 1448 , 15.95 )
( 1449 , 15.66 )
( 1450 , 15.37 )
( 1451 , 15.07 )
( 1452 , 14.77 )
( 1453 , 14.98 )
( 1454 , 15.20 )
( 1455 , 15.36 )
( 1456 , 15.62 )
( 1457 , 15.83 )
( 1458 , 15.94 )
( 1459 , 16.09 )
( 1460 , 16.21 )
( 1461 , 16.12 )
( 1462 , 16.02 )
( 1463 , 15.79 )
( 1464 , 15.49 )
( 1465 , 15.36 )
( 1466 , 15.43 )
( 1467 , 15.13 )
( 1468 , 15.15 )
( 1469 , 15.14 )
( 1470 , 15.08 )
( 1471 , 15.07 )
( 1472 , 15.13 )
( 1473 , 15.17 )
( 1474 , 15.18 )
( 1475 , 15.16 )
( 1476 , 15.35 )
( 1477 , 15.33 )
( 1478 , 15.30 )
( 1479 , 15.04 )
( 1480 , 14.74 )
( 1481 , 14.44 )
( 1482 , 14.14 )
( 1483 , 13.85 )
( 1484 , 13.56 )
( 1485 , 13.26 )
( 1486 , 12.96 )
( 1487 , 12.73 )
( 1488 , 12.44 )
( 1489 , 12.14 )
( 1490 , 12.12 )
( 1491 , 11.82 )
( 1492 , 11.84 )
( 1493 , 11.89 )
( 1494 , 11.94 )
( 1495 , 12.14 )
( 1496 , 12.28 )
( 1497 , 12.29 )
( 1498 , 12.29 )
( 1499 , 12.31 )
( 1500 , 12.46 )
( 1501 , 12.62 )
( 1502 , 12.80 )
( 1503 , 12.95 )
( 1504 , 13.09 )
( 1505 , 13.33 )
( 1506 , 13.54 )
( 1507 , 13.56 )
( 1508 , 13.57 )
( 1509 , 13.57 )
( 1510 , 13.84 )
( 1511 , 14.10 )
( 1512 , 14.32 )
( 1513 , 14.58 )
( 1514 , 14.91 )
( 1515 , 15.26 )
( 1516 , 15.55 )
( 1517 , 15.85 )
( 1518 , 16.12 )
( 1519 , 16.36 )
( 1520 , 16.60 )
( 1521 , 16.85 )
( 1522 , 17.08 )
( 1523 , 17.31 )
( 1524 , 17.58 )
( 1525 , 17.81 )
( 1526 , 18.10 )
( 1527 , 18.32 )
( 1528 , 18.54 )
( 1529 , 18.90 )
( 1530 , 19.22 )
( 1531 , 19.44 )
( 1532 , 19.70 )
( 1533 , 19.92 )
( 1534 , 20.15 )
( 1535 , 20.44 )
( 1536 , 20.70 )
( 1537 , 20.99 )
( 1538 , 21.31 )
( 1539 , 21.59 )
( 1540 , 21.88 )
( 1541 , 22.18 )
( 1542 , 22.44 )
( 1543 , 22.71 )
( 1544 , 22.95 )
( 1545 , 23.25 )
( 1546 , 23.54 )
( 1547 , 23.82 )
( 1548 , 24.10 )
( 1549 , 24.38 )
( 1550 , 24.69 )
( 1551 , 24.98 )
( 1552 , 25.20 )
( 1553 , 25.44 )
( 1554 , 25.82 )
( 1555 , 26.16 )
( 1556 , 26.52 )
( 1557 , 26.92 )
( 1558 , 27.29 )
( 1559 , 27.53 )
( 1560 , 27.86 )
( 1561 , 28.21 )
( 1562 , 28.43 )
( 1563 , 28.43 )
( 1564 , 28.46 )
( 1565 , 28.67 )
( 1566 , 28.82 )
( 1567 , 28.87 )
( 1568 , 28.89 )
( 1569 , 28.89 )
( 1570 , 29.27 )
( 1571 , 29.49 )
( 1572 , 29.79 )
( 1573 , 30.01 )
( 1574 , 30.23 )
( 1575 , 30.48 )
( 1576 , 30.74 )
( 1577 , 30.97 )
( 1578 , 31.25 )
( 1579 , 31.48 )
( 1580 , 31.76 )
( 1581 , 31.99 )
( 1582 , 32.38 )
( 1583 , 32.80 )
( 1584 , 33.23 )
( 1585 , 33.68 )
( 1586 , 34.14 )
( 1587 , 34.58 )
( 1588 , 34.88 )
( 1589 , 35.17 )
( 1590 , 35.40 )
( 1591 , 35.62 )
( 1592 , 35.91 )
( 1593 , 36.20 )
( 1594 , 36.42 )
( 1595 , 36.47 )
( 1596 , 36.50 )
( 1597 , 36.53 )
( 1598 , 36.59 )
( 1599 , 36.59 )
( 1600 , 36.60 )
( 1601 , 36.60 )
( 1602 , 36.60 )
( 1603 , 36.60 )
( 1604 , 36.60 )
( 1605 , 36.61 )
( 1606 , 36.61 )
( 1607 , 36.61 )
( 1608 , 36.66 )
( 1609 , 36.66 )
( 1610 , 36.87 )
( 1611 , 37.02 )
( 1612 , 37.17 )
( 1613 , 37.18 )
( 1614 , 37.18 )
( 1615 , 37.20 )
( 1616 , 37.20 )
( 1617 , 37.36 )
( 1618 , 37.56 )
( 1619 , 37.72 )
( 1620 , 37.90 )
( 1621 , 37.90 )
( 1622 , 37.90 )
( 1623 , 37.92 )
( 1624 , 37.92 )
( 1625 , 37.92 )
( 1626 , 37.92 )
( 1627 , 38.15 )
( 1628 , 38.37 )
( 1629 , 38.56 )
( 1630 , 38.72 )
( 1631 , 38.87 )
( 1632 , 38.87 )
( 1633 , 38.87 )
( 1634 , 39.09 )
( 1635 , 39.36 )
( 1636 , 39.62 )
( 1637 , 39.72 )
( 1638 , 39.85 )
( 1639 , 40.00 )
( 1640 , 40.00 )
( 1641 , 40.00 )
( 1642 , 40.21 )
( 1643 , 40.38 )
( 1644 , 40.55 )
( 1645 , 40.72 )
( 1646 , 40.90 )
( 1647 , 41.04 )
( 1648 , 41.05 )
( 1649 , 41.19 )
( 1650 , 41.39 )
( 1651 , 41.47 )
( 1652 , 41.56 )
( 1653 , 41.57 )
( 1654 , 41.59 )
( 1655 , 41.62 )
( 1656 , 41.77 )
( 1657 , 41.95 )
( 1658 , 42.02 )
( 1659 , 42.15 )
( 1660 , 42.22 )
( 1661 , 42.38 )
( 1662 , 42.40 )
( 1663 , 42.46 )
( 1664 , 42.53 )
( 1665 , 42.60 )
( 1666 , 42.68 )
( 1667 , 42.66 )
( 1668 , 42.62 )
( 1669 , 42.56 )
( 1670 , 42.51 )
( 1671 , 42.53 )
( 1672 , 42.52 )
( 1673 , 42.62 )
( 1674 , 42.65 )
( 1675 , 42.79 )
( 1676 , 42.78 )
( 1677 , 42.91 )
( 1678 , 43.04 )
( 1679 , 43.16 )
( 1680 , 43.35 )
( 1681 , 43.59 )
( 1682 , 43.79 )
( 1683 , 44.00 )
( 1684 , 44.12 )
( 1685 , 44.00 )
( 1686 , 43.87 )
( 1687 , 43.75 )
( 1688 , 43.62 )
( 1689 , 43.50 )
( 1690 , 43.31 )
( 1691 , 43.11 )
( 1692 , 42.81 )
( 1693 , 42.51 )
( 1694 , 42.21 )
( 1695 , 42.01 )
( 1696 , 41.99 )
( 1697 , 41.85 )
( 1698 , 41.90 )
( 1699 , 41.79 )
( 1700 , 41.48 )
( 1701 , 41.20 )
( 1702 , 40.90 )
( 1703 , 40.60 )
( 1704 , 40.38 )
( 1705 , 40.12 )
( 1706 , 39.82 )
( 1707 , 39.57 )
( 1708 , 39.38 )
( 1709 , 39.08 )
( 1710 , 38.79 )
( 1711 , 38.53 )
( 1712 , 38.23 )
( 1713 , 37.93 )
( 1714 , 37.62 )
( 1715 , 37.49 )
( 1716 , 37.43 )
( 1717 , 37.32 )
( 1718 , 37.02 )
( 1719 , 36.72 )
( 1720 , 36.63 )
( 1721 , 36.55 )
( 1722 , 36.42 )
( 1723 , 36.23 )
( 1724 , 35.93 )
( 1725 , 35.62 )
( 1726 , 35.32 )
( 1727 , 35.04 )
( 1728 , 34.77 )
( 1729 , 34.68 )
( 1730 , 34.38 )
( 1731 , 34.43 )
( 1732 , 34.52 )
( 1733 , 34.42 )
( 1734 , 34.31 )
( 1735 , 34.26 )
( 1736 , 34.13 )
( 1737 , 34.04 )
( 1738 , 33.73 )
( 1739 , 33.50 )
( 1740 , 33.29 )
( 1741 , 33.19 )
( 1742 , 32.89 )
( 1743 , 32.59 )
( 1744 , 32.29 )
( 1745 , 31.99 )
( 1746 , 31.68 )
( 1747 , 31.39 )
( 1748 , 31.11 )
( 1749 , 30.84 )
( 1750 , 30.64 )
( 1751 , 30.34 )
( 1752 , 30.04 )
( 1753 , 29.76 )
( 1754 , 29.46 )
( 1755 , 29.16 )
( 1756 , 28.93 )
( 1757 , 28.85 )
( 1758 , 28.71 )
( 1759 , 28.73 )
( 1760 , 28.72 )
( 1761 , 28.79 )
( 1762 , 28.78 )
( 1763 , 28.74 )
( 1764 , 28.45 )
( 1765 , 28.22 )
( 1766 , 28.20 )
( 1767 , 28.05 )
( 1768 , 27.88 )
( 1769 , 27.58 )
( 1770 , 27.28 )
( 1771 , 27.18 )
( 1772 , 26.88 )
( 1773 , 26.58 )
( 1774 , 26.28 )
( 1775 , 25.98 )
( 1776 , 25.70 )
( 1777 , 25.50 )
( 1778 , 25.23 )
( 1779 , 25.25 )
( 1780 , 25.21 )
( 1781 , 25.00 )
( 1782 , 24.77 )
( 1783 , 24.46 )
( 1784 , 24.16 )
( 1785 , 24.01 )
( 1786 , 23.72 )
( 1787 , 23.44 )
( 1788 , 23.30 )
( 1789 , 23.15 )
( 1790 , 22.96 )
( 1791 , 22.68 )
( 1792 , 22.43 )
( 1793 , 22.15 )
( 1794 , 21.85 )
( 1795 , 21.55 )
( 1796 , 21.25 )
( 1797 , 20.96 )
( 1798 , 20.66 )
( 1799 , 20.36 )
( 1800 , 20.21 )
( 1801 , 19.91 )
( 1802 , 19.61 )
( 1803 , 19.31 )
( 1804 , 19.01 )
( 1805 , 18.71 )
( 1806 , 18.68 )
( 1807 , 18.38 )
( 1808 , 18.11 )
( 1809 , 17.83 )
( 1810 , 17.62 )
( 1811 , 17.43 )
( 1812 , 17.41 )
( 1813 , 17.33 )
( 1814 , 17.37 )
( 1815 , 17.07 )
( 1816 , 17.01 )
( 1817 , 16.84 )
( 1818 , 16.55 )
( 1819 , 16.25 )
( 1820 , 15.95 )
( 1821 , 16.16 )
( 1822 , 16.30 )
( 1823 , 16.29 )
( 1824 , 16.49 )
( 1825 , 16.69 )
( 1826 , 16.70 )
( 1827 , 16.64 )
( 1828 , 16.62 )
( 1829 , 16.56 )
( 1830 , 16.51 )
( 1831 , 16.46 )
( 1832 , 16.47 )
( 1833 , 16.44 )
( 1834 , 16.38 )
( 1835 , 16.39 )
( 1836 , 16.38 )
( 1837 , 16.44 )
( 1838 , 16.57 )
( 1839 , 16.56 )
( 1840 , 16.62 )
( 1841 , 16.58 )
( 1842 , 16.52 )
( 1843 , 16.47 )
( 1844 , 16.42 )
( 1845 , 16.52 )
( 1846 , 16.63 )
( 1847 , 16.51 )
( 1848 , 16.38 )
( 1849 , 16.33 )
( 1850 , 16.31 )
( 1851 , 16.36 )
( 1852 , 16.30 )
( 1853 , 16.27 )
( 1854 , 16.21 )
( 1855 , 16.17 )
( 1856 , 16.14 )
( 1857 , 15.84 )
( 1858 , 15.54 )
( 1859 , 15.50 )
( 1860 , 15.42 )
( 1861 , 15.12 )
( 1862 , 14.91 )
( 1863 , 14.61 )
( 1864 , 14.70 )
( 1865 , 14.76 )
( 1866 , 14.64 )
( 1867 , 14.62 )
( 1868 , 14.60 )
( 1869 , 14.48 )
( 1870 , 14.42 )
( 1871 , 14.39 )
( 1872 , 14.78 )
( 1873 , 15.16 )
( 1874 , 15.60 )
( 1875 , 15.92 )
( 1876 , 16.17 )
( 1877 , 16.38 )
( 1878 , 16.59 )
( 1879 , 16.89 )
( 1880 , 17.21 )
( 1881 , 17.51 )
( 1882 , 17.92 )
( 1883 , 18.39 )
( 1884 , 18.73 )
( 1885 , 19.17 )
( 1886 , 19.47 )
( 1887 , 19.82 )
( 1888 , 20.13 )
( 1889 , 20.44 )
( 1890 , 20.74 )
( 1891 , 21.04 )
( 1892 , 21.34 )
( 1893 , 21.67 )
( 1894 , 21.99 )
( 1895 , 22.29 )
( 1896 , 22.59 )
( 1897 , 22.90 )
( 1898 , 23.20 )
( 1899 , 23.51 )
( 1900 , 23.81 )
( 1901 , 24.16 )
( 1902 , 24.46 )
( 1903 , 24.81 )
( 1904 , 25.15 )
( 1905 , 25.47 )
( 1906 , 25.78 )
( 1907 , 26.08 )
( 1908 , 26.43 )
( 1909 , 26.77 )
( 1910 , 27.18 )
( 1911 , 27.48 )
( 1912 , 27.79 )
( 1913 , 28.11 )
( 1914 , 28.46 )
( 1915 , 28.67 )
( 1916 , 28.89 )
( 1917 , 29.26 )
( 1918 , 29.63 )
( 1919 , 29.97 )
( 1920 , 30.35 )
( 1921 , 30.72 )
( 1922 , 31.06 )
( 1923 , 31.28 )
( 1924 , 31.49 )
( 1925 , 31.74 )
( 1926 , 32.02 )
( 1927 , 32.31 )
( 1928 , 32.57 )
( 1929 , 32.93 )
( 1930 , 33.21 )
( 1931 , 33.52 )
( 1932 , 33.77 )
( 1933 , 34.00 )
( 1934 , 34.21 )
( 1935 , 34.44 )
( 1936 , 34.65 )
( 1937 , 34.98 )
( 1938 , 35.20 )
( 1939 , 35.41 )
( 1940 , 35.64 )
( 1941 , 35.85 )
( 1942 , 36.07 )
( 1943 , 36.41 )
( 1944 , 36.71 )
( 1945 , 37.01 )
( 1946 , 36.91 )
( 1947 , 36.82 )
( 1948 , 36.73 )
( 1949 , 36.63 )
( 1950 , 36.53 )
( 1951 , 36.43 )
( 1952 , 36.34 )
( 1953 , 36.35 )
( 1954 , 36.26 )
( 1955 , 36.20 )
( 1956 , 36.10 )
( 1957 , 36.07 )
( 1958 , 35.79 )
( 1959 , 35.49 )
( 1960 , 35.30 )
( 1961 , 35.00 )
( 1962 , 35.05 )
( 1963 , 34.75 )
( 1964 , 34.82 )
( 1965 , 34.52 )
( 1966 , 34.43 )
( 1967 , 34.38 )
( 1968 , 34.41 )
( 1969 , 34.27 )
( 1970 , 34.30 )
( 1971 , 34.10 )
( 1972 , 33.91 )
( 1973 , 33.81 )
( 1974 , 33.75 )
( 1975 , 33.69 )
( 1976 , 33.39 )
( 1977 , 33.09 )
( 1978 , 32.79 )
( 1979 , 32.83 )
( 1980 , 32.89 )
( 1981 , 32.93 )
( 1982 , 33.01 )
( 1983 , 32.89 )
( 1984 , 32.76 )
( 1985 , 32.64 )
( 1986 , 32.57 )
( 1987 , 32.55 )
( 1988 , 32.50 )
( 1989 , 32.38 )
( 1990 , 32.11 )
( 1991 , 31.81 )
( 1992 , 31.51 )
( 1993 , 31.21 )
( 1994 , 31.00 )
( 1995 , 30.70 )
( 1996 , 30.67 )
( 1997 , 30.63 )
( 1998 , 30.65 )
( 1999 , 30.69 )
( 2000 , 30.69 )
( 2001 , 30.69 )
( 2002 , 30.80 )
( 2003 , 30.90 )
( 2004 , 30.99 )
( 2005 , 31.10 )
( 2006 , 31.39 )
( 2007 , 31.68 )
( 2008 , 31.95 )
( 2009 , 32.24 )
( 2010 , 32.55 )
( 2011 , 32.76 )
( 2012 , 32.84 )
( 2013 , 32.94 )
( 2014 , 32.89 )
( 2015 , 32.83 )
( 2016 , 32.78 )
( 2017 , 32.72 )
( 2018 , 32.69 )
( 2019 , 32.74 )
( 2020 , 32.73 )
( 2021 , 32.72 )
( 2022 , 32.66 )
( 2023 , 32.61 )
( 2024 , 32.70 )
( 2025 , 32.73 )
( 2026 , 32.77 )
( 2027 , 32.76 )
( 2028 , 32.77 )
( 2029 , 32.76 )
( 2030 , 32.75 )
( 2031 , 32.78 )
( 2032 , 32.84 )
( 2033 , 32.84 )
( 2034 , 32.92 )
( 2035 , 32.94 )
( 2036 , 32.96 )
( 2037 , 32.96 )
( 2038 , 32.90 )
( 2039 , 32.84 )
( 2040 , 32.78 )
( 2041 , 32.76 )
( 2042 , 32.73 )
( 2043 , 32.70 )
( 2044 , 32.67 )
( 2045 , 32.57 )
( 2046 , 32.52 )
( 2047 , 32.40 )
( 2048 , 32.27 )
( 2049 , 32.15 )
( 2050 , 32.19 )
( 2051 , 32.23 )
( 2052 , 32.12 )
( 2053 , 32.03 )
( 2054 , 31.90 )
( 2055 , 31.78 )
( 2056 , 31.66 )
( 2057 , 31.53 )
( 2058 , 31.41 )
( 2059 , 31.37 )
( 2060 , 31.25 )
( 2061 , 31.12 )
( 2062 , 31.50 )
( 2063 , 31.82 )
( 2064 , 32.14 )
( 2065 , 32.53 )
( 2066 , 32.87 )
( 2067 , 33.25 )
( 2068 , 33.55 )
( 2069 , 33.82 )
( 2070 , 34.04 )
( 2071 , 34.26 )
( 2072 , 34.61 )
( 2073 , 34.94 )
( 2074 , 35.31 )
( 2075 , 35.69 )
( 2076 , 36.02 )
( 2077 , 36.34 )
( 2078 , 36.54 )
( 2079 , 36.81 )
( 2080 , 37.01 )
( 2081 , 37.21 )
( 2082 , 37.52 )
( 2083 , 37.73 )
( 2084 , 37.95 )
( 2085 , 38.20 )
( 2086 , 38.42 )
( 2087 , 38.82 )
( 2088 , 39.19 )
( 2089 , 39.52 )
( 2090 , 39.79 )
( 2091 , 40.00 )
( 2092 , 40.22 )
( 2093 , 40.46 )
( 2094 , 40.69 )
( 2095 , 40.92 )
( 2096 , 41.20 )
( 2097 , 41.62 )
( 2098 , 41.98 )
( 2099 , 42.34 )
( 2100 , 42.76 )
( 2101 , 43.20 )
( 2102 , 43.47 )
( 2103 , 43.77 )
( 2104 , 43.99 )
( 2105 , 44.27 )
( 2106 , 44.58 )
( 2107 , 44.89 )
( 2108 , 45.16 )
( 2109 , 45.44 )
( 2110 , 45.72 )
( 2111 , 45.96 )
( 2112 , 46.16 )
( 2113 , 46.45 )
( 2114 , 46.65 )
( 2115 , 46.88 )
( 2116 , 47.08 )
( 2117 , 47.28 )
( 2118 , 47.57 )
( 2119 , 47.55 )
( 2120 , 47.53 )
( 2121 , 47.69 )
( 2122 , 47.88 )
( 2123 , 48.00 )
( 2124 , 48.03 )
( 2125 , 48.06 )
( 2126 , 48.16 )
( 2127 , 48.21 )
( 2128 , 48.27 )
( 2129 , 48.32 )
( 2130 , 48.52 )
( 2131 , 48.61 )
( 2132 , 48.59 )
( 2133 , 48.58 )
( 2134 , 48.46 )
( 2135 , 48.34 )
( 2136 , 48.29 )
( 2137 , 48.23 )
( 2138 , 48.29 )
( 2139 , 48.39 )
( 2140 , 48.32 )
( 2141 , 48.25 )
( 2142 , 48.14 )
( 2143 , 48.02 )
( 2144 , 48.06 )
( 2145 , 48.11 )
( 2146 , 48.10 )
( 2147 , 48.12 )
( 2148 , 48.11 )
( 2149 , 48.09 )
( 2150 , 48.04 )
( 2151 , 47.73 )
( 2152 , 47.45 )
( 2153 , 47.14 )
( 2154 , 46.93 )
( 2155 , 46.62 )
( 2156 , 46.36 )
( 2157 , 46.12 )
( 2158 , 46.05 )
( 2159 , 45.99 )
( 2160 , 45.90 )
( 2161 , 45.60 )
( 2162 , 45.30 )
( 2163 , 45.09 )
( 2164 , 44.88 )
( 2165 , 44.59 )
( 2166 , 44.35 )
( 2167 , 44.05 )
( 2168 , 43.76 )
( 2169 , 43.46 )
( 2170 , 43.16 )
( 2171 , 42.86 )
( 2172 , 42.57 )
( 2173 , 42.43 )
( 2174 , 42.34 )
( 2175 , 42.23 )
( 2176 , 42.17 )
( 2177 , 42.07 )
( 2178 , 41.96 )
( 2179 , 41.87 )
( 2180 , 41.84 )
( 2181 , 41.77 )
( 2182 , 41.67 )
( 2183 , 41.38 )
( 2184 , 41.07 )
( 2185 , 40.77 )
( 2186 , 40.49 )
( 2187 , 40.19 )
( 2188 , 39.95 )
( 2189 , 39.80 )
( 2190 , 39.52 )
( 2191 , 39.21 )
( 2192 , 38.91 )
( 2193 , 38.84 )
( 2194 , 38.61 )
( 2195 , 38.31 )
( 2196 , 38.02 )
( 2197 , 37.74 )
( 2198 , 37.46 )
( 2199 , 37.23 )
( 2200 , 36.98 )
( 2201 , 36.70 )
( 2202 , 36.40 )
( 2203 , 36.13 )
( 2204 , 35.83 )
( 2205 , 36.11 )
( 2206 , 36.23 )
( 2207 , 36.17 )
( 2208 , 36.04 )
( 2209 , 36.40 )
( 2210 , 36.61 )
( 2211 , 36.83 )
( 2212 , 37.02 )
( 2213 , 36.90 )
( 2214 , 36.77 )
( 2215 , 36.65 )
( 2216 , 36.61 )
( 2217 , 36.57 )
( 2218 , 36.61 )
( 2219 , 36.65 )
( 2220 , 36.70 )
( 2221 , 36.73 )
( 2222 , 36.62 )
( 2223 , 36.50 )
( 2224 , 36.62 )
( 2225 , 36.75 )
( 2226 , 36.94 )
( 2227 , 37.06 )
( 2228 , 37.19 )
( 2229 , 37.32 )
( 2230 , 37.50 )
( 2231 , 37.69 )
( 2232 , 37.82 )
( 2233 , 37.96 )
( 2234 , 38.08 )
( 2235 , 38.22 )
( 2236 , 38.40 )
( 2237 , 38.59 )
( 2238 , 38.72 )
( 2239 , 38.84 )
( 2240 , 39.02 )
( 2241 , 39.18 )
( 2242 , 39.37 )
( 2243 , 39.57 )
( 2244 , 39.70 )
( 2245 , 39.82 )
( 2246 , 39.70 )
( 2247 , 39.58 )
( 2248 , 39.50 )
( 2249 , 39.40 )
( 2250 , 39.30 )
( 2251 , 39.18 )
( 2252 , 39.05 )
( 2253 , 39.18 )
( 2254 , 39.05 )
( 2255 , 38.96 )
( 2256 , 38.83 )
( 2257 , 38.95 )
( 2258 , 39.05 )
( 2259 , 39.14 )
( 2260 , 39.25 )
( 2261 , 39.34 )
( 2262 , 39.54 )
( 2263 , 39.57 )
( 2264 , 39.56 )
( 2265 , 39.35 )
( 2266 , 39.14 )
( 2267 , 38.90 )
( 2268 , 38.66 )
( 2269 , 38.36 )
( 2270 , 38.34 )
( 2271 , 38.39 )
( 2272 , 38.44 )
( 2273 , 38.55 )
( 2274 , 38.54 )
( 2275 , 38.54 )
( 2276 , 38.53 )
( 2277 , 38.54 )
( 2278 , 38.58 )
( 2279 , 38.67 )
( 2280 , 38.66 )
( 2281 , 38.66 )
( 2282 , 38.63 )
( 2283 , 38.64 )
( 2284 , 38.59 )
( 2285 , 38.53 )
( 2286 , 38.47 )
( 2287 , 38.42 )
( 2288 , 38.40 )
( 2289 , 38.34 )
( 2290 , 38.33 )
( 2291 , 38.27 )
( 2292 , 38.26 )
( 2293 , 38.27 )
( 2294 , 38.21 )
( 2295 , 38.16 )
( 2296 , 38.14 )
( 2297 , 38.12 )
( 2298 , 38.03 )
( 2299 , 37.90 )
( 2300 , 38.03 )
( 2301 , 38.20 )
( 2302 , 38.32 )
( 2303 , 38.20 )
( 2304 , 38.25 )
( 2305 , 38.29 )
( 2306 , 38.38 )
( 2307 , 38.48 )
( 2308 , 38.62 )
( 2309 , 38.71 )
( 2310 , 38.81 )
( 2311 , 38.91 )
( 2312 , 39.02 )
( 2313 , 39.11 )
( 2314 , 39.23 )
( 2315 , 39.33 )
( 2316 , 39.48 )
( 2317 , 39.63 )
( 2318 , 39.79 )
( 2319 , 39.96 )
( 2320 , 40.14 )
( 2321 , 40.41 )
( 2322 , 40.51 )
( 2323 , 40.70 )
( 2324 , 40.80 )
( 2325 , 40.90 )
( 2326 , 41.00 )
( 2327 , 41.12 )
( 2328 , 41.24 )
( 2329 , 41.52 )
( 2330 , 41.82 )
( 2331 , 42.02 )
( 2332 , 42.17 )
( 2333 , 42.27 )
( 2334 , 42.46 )
( 2335 , 42.66 )
( 2336 , 42.78 )
( 2337 , 42.94 )
( 2338 , 43.04 )
( 2339 , 43.26 )
( 2340 , 43.36 )
( 2341 , 43.46 )
( 2342 , 43.57 )
( 2343 , 43.70 )
( 2344 , 43.96 )
( 2345 , 44.07 )
( 2346 , 44.27 )
( 2347 , 44.46 )
( 2348 , 44.69 )
( 2349 , 44.89 )
( 2350 , 45.13 )
( 2351 , 45.40 )
( 2352 , 45.61 )
( 2353 , 45.77 )
( 2354 , 45.93 )
( 2355 , 46.06 )
( 2356 , 46.26 )
( 2357 , 46.42 )
( 2358 , 46.52 )
( 2359 , 46.62 )
( 2360 , 46.66 )
( 2361 , 46.64 )
( 2362 , 46.69 )
( 2363 , 46.66 )
( 2364 , 46.63 )
( 2365 , 46.91 )
( 2366 , 47.17 )
( 2367 , 47.54 )
( 2368 , 47.52 )
( 2369 , 47.50 )
( 2370 , 47.48 )
( 2371 , 47.46 )
( 2372 , 47.43 )
( 2373 , 47.83 )
( 2374 , 48.11 )
( 2375 , 48.07 )
( 2376 , 48.23 )
( 2377 , 48.29 )
( 2378 , 48.33 )
( 2379 , 48.36 )
( 2380 , 48.34 )
( 2381 , 48.32 )
( 2382 , 48.46 )
( 2383 , 48.59 )
( 2384 , 48.71 )
( 2385 , 48.84 )
( 2386 , 48.96 )
( 2387 , 49.01 )
( 2388 , 49.06 )
( 2389 , 49.16 )
( 2390 , 49.13 )
( 2391 , 49.11 )
( 2392 , 49.08 )
( 2393 , 49.02 )
( 2394 , 49.12 )
( 2395 , 49.15 )
( 2396 , 49.09 )
( 2397 , 49.04 )
( 2398 , 49.05 )
( 2399 , 49.11 )
( 2400 , 49.05 )
( 2401 , 49.00 )
( 2402 , 48.92 )
( 2403 , 48.79 )
( 2404 , 48.70 )
( 2405 , 48.60 )
( 2406 , 48.31 )
( 2407 , 48.01 )
( 2408 , 47.73 )
( 2409 , 47.43 )
( 2410 , 47.12 )
( 2411 , 46.84 )
( 2412 , 46.71 )
( 2413 , 46.70 )
( 2414 , 46.39 )
( 2415 , 46.09 )
( 2416 , 45.98 )
( 2417 , 45.68 )
( 2418 , 45.38 )
( 2419 , 45.09 )
( 2420 , 44.80 )
( 2421 , 44.58 )
( 2422 , 44.45 )
( 2423 , 44.34 )
( 2424 , 44.29 )
( 2425 , 44.22 )
( 2426 , 44.11 )
( 2427 , 43.81 )
( 2428 , 43.51 )
( 2429 , 43.21 )
( 2430 , 43.11 )
( 2431 , 42.90 )
( 2432 , 42.75 )
( 2433 , 42.58 )
( 2434 , 42.28 )
( 2435 , 42.00 )
( 2436 , 41.70 )
( 2437 , 41.40 )
( 2438 , 41.12 )
( 2439 , 40.91 )
( 2440 , 40.85 )
( 2441 , 40.75 )
( 2442 , 40.66 )
( 2443 , 40.46 )
( 2444 , 40.16 )
( 2445 , 39.86 )
( 2446 , 39.71 )
( 2447 , 39.57 )
( 2448 , 39.38 )
( 2449 , 39.08 )
( 2450 , 38.79 )
( 2451 , 38.49 )
( 2452 , 38.19 )
( 2453 , 38.07 )
( 2454 , 37.77 )
( 2455 , 37.47 )
( 2456 , 37.17 )
( 2457 , 36.90 )
( 2458 , 36.60 )
( 2459 , 36.35 )
( 2460 , 36.09 )
( 2461 , 35.81 )
( 2462 , 35.54 )
( 2463 , 35.39 )
( 2464 , 35.09 )
( 2465 , 34.80 )
( 2466 , 34.50 )
( 2467 , 34.20 )
( 2468 , 33.93 )
( 2469 , 33.67 )
( 2470 , 33.41 )
( 2471 , 33.11 )
( 2472 , 32.85 )
( 2473 , 32.70 )
( 2474 , 32.62 )
( 2475 , 32.48 )
( 2476 , 32.18 )
( 2477 , 31.88 )
( 2478 , 31.63 )
( 2479 , 31.34 )
( 2480 , 31.05 )
( 2481 , 30.76 )
( 2482 , 30.46 )
( 2483 , 30.16 )
( 2484 , 30.21 )
( 2485 , 30.36 )
( 2486 , 30.52 )
( 2487 , 30.65 )
( 2488 , 30.77 )
( 2489 , 30.77 )
( 2490 , 30.83 )
( 2491 , 30.83 )
( 2492 , 30.99 )
( 2493 , 31.01 )
( 2494 , 31.04 )
( 2495 , 31.06 )
( 2496 , 31.36 )
( 2497 , 31.64 )
( 2498 , 31.79 )
( 2499 , 31.93 )
( 2500 , 32.08 )
( 2501 , 32.23 )
( 2502 , 32.23 )
( 2503 , 32.70 )
( 2504 , 33.13 )
( 2505 , 33.44 )
( 2506 , 33.76 )
( 2507 , 34.07 )
( 2508 , 34.36 )
( 2509 , 34.70 )
( 2510 , 35.03 )
( 2511 , 35.34 )
( 2512 , 35.63 )
( 2513 , 35.86 )
( 2514 , 36.10 )
( 2515 , 36.36 )
( 2516 , 36.60 )
( 2517 , 36.83 )
( 2518 , 37.07 )
( 2519 , 37.31 )
( 2520 , 37.54 )
( 2521 , 37.79 )
( 2522 , 38.02 )
( 2523 , 38.30 )
( 2524 , 38.54 )
( 2525 , 38.54 )
( 2526 , 38.64 )
( 2527 , 38.69 )
( 2528 , 38.74 )
( 2529 , 38.81 )
( 2530 , 38.82 )
( 2531 , 38.84 )
( 2532 , 38.86 )
( 2533 , 38.86 )
( 2534 , 39.01 )
( 2535 , 39.16 )
( 2536 , 39.19 )
( 2537 , 39.19 )
( 2538 , 39.19 )
( 2539 , 39.19 )
( 2540 , 39.27 )
( 2541 , 39.33 )
( 2542 , 39.34 )
( 2543 , 39.51 )
( 2544 , 39.61 )
( 2545 , 39.68 )
( 2546 , 39.91 )
( 2547 , 40.11 )
( 2548 , 40.18 )
( 2549 , 40.28 )
( 2550 , 40.34 )
( 2551 , 40.41 )
( 2552 , 40.49 )
( 2553 , 40.55 )
( 2554 , 40.62 )
( 2555 , 40.81 )
( 2556 , 40.93 )
( 2557 , 40.93 )
( 2558 , 40.95 )
( 2559 , 40.95 )
( 2560 , 41.08 )
( 2561 , 41.21 )
( 2562 , 41.32 )
( 2563 , 41.38 )
( 2564 , 41.39 )
( 2565 , 41.46 )
( 2566 , 41.48 )
( 2567 , 41.61 )
( 2568 , 41.62 )
( 2569 , 41.62 )
( 2570 , 41.92 )
( 2571 , 42.19 )
( 2572 , 42.46 )
( 2573 , 42.73 )
( 2574 , 42.90 )
( 2575 , 43.01 )
( 2576 , 43.08 )
( 2577 , 43.15 )
( 2578 , 43.21 )
( 2579 , 43.37 )
( 2580 , 43.50 )
( 2581 , 43.82 )
( 2582 , 44.16 )
( 2583 , 44.44 )
( 2584 , 44.60 )
( 2585 , 44.76 )
( 2586 , 44.89 )
( 2587 , 44.96 )
( 2588 , 44.96 )
( 2589 , 44.96 )
( 2590 , 44.97 )
( 2591 , 45.03 )
( 2592 , 45.16 )
( 2593 , 45.29 )
( 2594 , 45.45 )
( 2595 , 45.57 )
( 2596 , 45.70 )
( 2597 , 45.76 )
( 2598 , 45.77 )
( 2599 , 45.94 )
( 2600 , 46.11 )
( 2601 , 46.11 )
( 2602 , 46.12 )
( 2603 , 46.12 )
( 2604 , 46.18 )
( 2605 , 46.18 )
( 2606 , 46.26 )
( 2607 , 46.38 )
( 2608 , 46.45 )
( 2609 , 46.45 )
( 2610 , 46.59 )
( 2611 , 46.75 )
( 2612 , 46.76 )
( 2613 , 46.76 )
( 2614 , 46.76 )
( 2615 , 46.91 )
( 2616 , 46.93 )
( 2617 , 47.04 )
( 2618 , 47.18 )
( 2619 , 47.29 )
( 2620 , 47.41 )
( 2621 , 47.41 )
( 2622 , 47.59 )
( 2623 , 47.83 )
( 2624 , 47.84 )
( 2625 , 47.84 )
( 2626 , 47.87 )
( 2627 , 47.87 )
( 2628 , 47.88 )
( 2629 , 47.98 )
( 2630 , 48.10 )
( 2631 , 48.21 )
( 2632 , 48.32 )
( 2633 , 48.48 )
( 2634 , 48.64 )
( 2635 , 48.69 )
( 2636 , 48.70 )
( 2637 , 48.70 )
( 2638 , 48.75 )
( 2639 , 48.75 )
( 2640 , 48.89 )
( 2641 , 49.09 )
( 2642 , 49.24 )
( 2643 , 49.39 )
( 2644 , 49.54 )
( 2645 , 49.65 )
( 2646 , 49.70 )
( 2647 , 49.75 )
( 2648 , 49.80 )
( 2649 , 49.80 )
( 2650 , 49.88 )
( 2651 , 50.00 )
( 2652 , 50.00 )
( 2653 , 50.19 )
( 2654 , 50.34 )
( 2655 , 50.34 )
( 2656 , 50.49 )
( 2657 , 50.49 )
( 2658 , 50.49 )
( 2659 , 50.49 )
( 2660 , 50.49 )
( 2661 , 50.49 )
( 2662 , 50.50 )
( 2663 , 50.50 )
( 2664 , 50.50 )
( 2665 , 50.52 )
( 2666 , 50.53 )
( 2667 , 50.53 )
( 2668 , 50.75 )
( 2669 , 50.89 )
( 2670 , 51.04 )
( 2671 , 51.06 )
( 2672 , 51.09 )
( 2673 , 51.09 )
( 2674 , 51.11 )
( 2675 , 51.29 )
( 2676 , 51.37 )
( 2677 , 51.52 )
( 2678 , 51.58 )
( 2679 , 51.61 )
( 2680 , 51.67 )
( 2681 , 51.67 )
( 2682 , 51.85 )
( 2683 , 52.03 )
( 2684 , 52.09 )
( 2685 , 52.09 )
( 2686 , 52.09 )
( 2687 , 52.09 )
( 2688 , 52.11 )
( 2689 , 52.23 )
( 2690 , 52.36 )
( 2691 , 52.47 )
( 2692 , 52.52 )
( 2693 , 52.55 )
( 2694 , 52.58 )
( 2695 , 52.61 )
( 2696 , 52.61 )
( 2697 , 52.62 )
( 2698 , 52.62 )
( 2699 , 52.67 )
( 2700 , 52.67 )
( 2701 , 52.67 )
( 2702 , 52.78 )
( 2703 , 52.78 )
( 2704 , 52.80 )
( 2705 , 52.91 )
( 2706 , 53.04 )
( 2707 , 53.15 )
( 2708 , 53.39 )
( 2709 , 53.54 )
( 2710 , 53.69 )
( 2711 , 53.84 )
( 2712 , 53.84 )
( 2713 , 53.91 )
( 2714 , 53.91 )
( 2715 , 53.91 )
( 2716 , 53.91 )
( 2717 , 53.92 )
( 2718 , 54.09 )
( 2719 , 54.12 )
( 2720 , 54.23 )
( 2721 , 54.34 )
( 2722 , 54.50 )
( 2723 , 54.54 )
( 2724 , 54.54 )
( 2725 , 54.69 )
( 2726 , 54.77 )
( 2727 , 54.79 )
( 2728 , 54.80 )
( 2729 , 54.82 )
( 2730 , 54.82 )
( 2731 , 54.82 )
( 2732 , 54.84 )
( 2733 , 54.84 )
( 2734 , 54.88 )
( 2735 , 54.93 )
( 2736 , 54.93 )
( 2737 , 54.93 )
( 2738 , 55.07 )
( 2739 , 55.22 )
( 2740 , 55.39 )
( 2741 , 55.55 )
( 2742 , 55.70 )
( 2743 , 55.85 )
( 2744 , 56.04 )
( 2745 , 56.26 )
( 2746 , 56.44 )
( 2747 , 56.44 )
( 2748 , 56.63 )
( 2749 , 56.80 )
( 2750 , 57.10 )
( 2751 , 57.39 )
( 2752 , 57.55 )
( 2753 , 57.70 )
( 2754 , 57.84 )
( 2755 , 58.09 )
( 2756 , 58.42 )
( 2757 , 58.70 )
( 2758 , 58.82 )
( 2759 , 58.93 )
( 2760 , 59.08 )
( 2761 , 59.28 )
( 2762 , 59.43 )
( 2763 , 59.58 )
( 2764 , 59.75 )
( 2765 , 59.89 )
( 2766 , 59.89 )
( 2767 , 59.94 )
( 2768 , 59.97 )
( 2769 , 59.98 )
( 2770 , 59.98 )
( 2771 , 60.00 )
( 2772 , 60.00 )
( 2773 , 60.13 )
( 2774 , 60.27 )
( 2775 , 60.27 )
( 2776 , 60.30 )
( 2777 , 60.35 )
( 2778 , 60.35 )
( 2779 , 60.49 )
( 2780 , 60.50 )
( 2781 , 60.51 )
( 2782 , 60.57 )
( 2783 , 60.59 )
( 2784 , 60.76 )
( 2785 , 60.96 )
( 2786 , 61.15 )
( 2787 , 61.40 )
( 2788 , 61.71 )
( 2789 , 61.78 )
( 2790 , 61.86 )
( 2791 , 61.94 )
( 2792 , 62.01 )
( 2793 , 62.21 )
( 2794 , 62.29 )
( 2795 , 62.38 )
( 2796 , 62.45 )
( 2797 , 62.54 )
( 2798 , 62.60 )
( 2799 , 62.67 )
( 2800 , 62.73 )
( 2801 , 62.83 )
( 2802 , 62.89 )
( 2803 , 63.13 )
( 2804 , 63.30 )
( 2805 , 63.52 )
( 2806 , 63.64 )
( 2807 , 63.78 )
( 2808 , 63.91 )
( 2809 , 64.05 )
( 2810 , 63.96 )
( 2811 , 63.84 )
( 2812 , 63.71 )
( 2813 , 63.65 )
( 2814 , 63.59 )
( 2815 , 63.46 )
( 2816 , 63.41 )
( 2817 , 63.31 )
( 2818 , 63.20 )
( 2819 , 63.12 )
( 2820 , 63.01 )
( 2821 , 62.92 )
( 2822 , 62.80 )
( 2823 , 62.67 )
( 2824 , 62.55 )
( 2825 , 62.47 )
( 2826 , 62.43 )
( 2827 , 62.30 )
( 2828 , 62.27 )
( 2829 , 62.30 )
( 2830 , 62.20 )
( 2831 , 62.14 )
( 2832 , 62.02 )
( 2833 , 62.06 )
( 2834 , 62.08 )
( 2835 , 62.13 )
( 2836 , 62.26 )
( 2837 , 62.31 )
( 2838 , 62.36 )
( 2839 , 62.36 )
( 2840 , 62.55 )
( 2841 , 62.73 )
( 2842 , 63.00 )
( 2843 , 63.29 )
( 2844 , 63.58 )
( 2845 , 63.80 )
( 2846 , 63.99 )
( 2847 , 64.23 )
( 2848 , 64.46 )
( 2849 , 64.69 )
( 2850 , 64.98 )
( 2851 , 65.27 )
( 2852 , 65.45 )
( 2853 , 65.66 )
( 2854 , 65.91 )
( 2855 , 66.12 )
( 2856 , 66.34 )
( 2857 , 66.55 )
( 2858 , 66.79 )
( 2859 , 66.99 )
( 2860 , 67.19 )
( 2861 , 67.42 )
( 2862 , 67.70 )
( 2863 , 67.95 )
( 2864 , 68.16 )
( 2865 , 68.12 )
( 2866 , 68.08 )
( 2867 , 68.02 )
( 2868 , 68.02 )
( 2869 , 68.06 )
( 2870 , 68.16 )
( 2871 , 68.16 )
( 2872 , 68.16 )
( 2873 , 68.44 )
( 2874 , 68.77 )
( 2875 , 69.10 )
( 2876 , 69.44 )
( 2877 , 69.75 )
( 2878 , 70.19 )
( 2879 , 70.66 )
( 2880 , 70.95 )
( 2881 , 71.26 )
( 2882 , 71.28 )
( 2883 , 71.28 )
( 2884 , 71.28 )
( 2885 , 71.28 )
( 2886 , 71.34 )
( 2887 , 71.34 )
( 2888 , 71.35 )
( 2889 , 71.36 )
( 2890 , 71.36 )
( 2891 , 71.38 )
( 2892 , 71.38 )
( 2893 , 71.40 )
( 2894 , 71.41 )
( 2895 , 71.42 )
( 2896 , 71.45 )
( 2897 , 71.55 )
( 2898 , 71.55 )
( 2899 , 71.55 )
( 2900 , 71.55 )
( 2901 , 71.55 )
( 2902 , 71.58 )
( 2903 , 71.59 )
( 2904 , 71.63 )
( 2905 , 71.63 )
( 2906 , 71.77 )
( 2907 , 71.81 )
( 2908 , 71.96 )
( 2909 , 72.13 )
( 2910 , 72.35 )
( 2911 , 72.55 )
( 2912 , 72.55 )
( 2913 , 72.62 )
( 2914 , 72.62 )
( 2915 , 72.62 )
( 2916 , 72.62 )
( 2917 , 72.67 )
( 2918 , 72.69 )
( 2919 , 72.69 )
( 2920 , 72.70 )
( 2921 , 72.70 )
( 2922 , 72.70 )
( 2923 , 72.72 )
( 2924 , 72.73 )
( 2925 , 72.73 )
( 2926 , 72.73 )
( 2927 , 72.73 )
( 2928 , 72.75 )
( 2929 , 72.75 )
( 2930 , 72.76 )
( 2931 , 72.84 )
( 2932 , 72.84 )
( 2933 , 72.84 )
( 2934 , 72.99 )
( 2935 , 73.01 )
( 2936 , 73.12 )
( 2937 , 73.14 )
( 2938 , 73.29 )
( 2939 , 73.45 )
( 2940 , 73.66 )
( 2941 , 73.90 )
( 2942 , 74.05 )
( 2943 , 74.05 )
( 2944 , 74.09 )
( 2945 , 74.09 )
( 2946 , 74.11 )
( 2947 , 74.34 )
( 2948 , 74.57 )
( 2949 , 74.91 )
( 2950 , 75.23 )
( 2951 , 75.55 )
( 2952 , 75.85 )
( 2953 , 76.07 )
( 2954 , 76.30 )
( 2955 , 76.70 )
( 2956 , 77.11 )
( 2957 , 77.45 )
( 2958 , 77.82 )
( 2959 , 78.16 )
( 2960 , 78.52 )
( 2961 , 78.78 )
( 2962 , 79.00 )
( 2963 , 79.27 )
( 2964 , 79.64 )
( 2965 , 79.94 )
( 2966 , 80.26 )
( 2967 , 80.55 )
( 2968 , 80.84 )
( 2969 , 81.08 )
( 2970 , 81.34 )
( 2971 , 81.56 )
( 2972 , 81.78 )
( 2973 , 82.01 )
( 2974 , 82.27 )
( 2975 , 82.52 )
( 2976 , 82.74 )
( 2977 , 82.96 )
( 2978 , 82.98 )
( 2979 , 82.98 )
( 2980 , 83.00 )
( 2981 , 83.00 )
( 2982 , 83.04 )
( 2983 , 83.04 )
( 2984 , 83.24 )
( 2985 , 83.29 )
( 2986 , 83.32 )
( 2987 , 83.34 )
( 2988 , 83.35 )
( 2989 , 83.35 )
( 2990 , 83.39 )
( 2991 , 83.39 )
( 2992 , 83.40 )
( 2993 , 83.48 )
( 2994 , 83.53 )
( 2995 , 83.67 )
( 2996 , 83.86 )
( 2997 , 84.02 )
( 2998 , 84.02 )
( 2999 , 84.05 )
( 3000 , 84.09 )
( 3001 , 84.10 )
( 3002 , 84.10 )
( 3003 , 84.15 )
( 3004 , 84.15 )
( 3005 , 84.30 )
( 3006 , 84.45 )
( 3007 , 84.56 )
( 3008 , 84.57 )
( 3009 , 84.80 )
( 3010 , 85.13 )
( 3011 , 85.36 )
( 3012 , 85.64 )
( 3013 , 85.92 )
( 3014 , 86.21 )
( 3015 , 86.46 )
( 3016 , 86.68 )
( 3017 , 86.92 )
( 3018 , 87.14 )
( 3019 , 87.38 )
( 3020 , 87.38 )
( 3021 , 87.38 )
( 3022 , 87.39 )
( 3023 , 87.39 )
( 3024 , 87.46 )
( 3025 , 87.55 )
( 3026 , 87.64 )
( 3027 , 87.77 )
( 3028 , 87.95 )
( 3029 , 88.01 )
( 3030 , 88.06 )
( 3031 , 88.13 )
( 3032 , 88.18 )
( 3033 , 88.18 )
( 3034 , 88.18 )
( 3035 , 88.18 )
( 3036 , 88.26 )
( 3037 , 88.27 )
( 3038 , 88.27 )
( 3039 , 88.38 )
( 3040 , 88.38 )
( 3041 , 88.38 )
( 3042 , 88.38 )
( 3043 , 88.41 )
( 3044 , 88.50 )
( 3045 , 88.52 )
( 3046 , 88.52 )
( 3047 , 88.52 )
( 3048 , 88.58 )
( 3049 , 88.63 )
( 3050 , 88.68 )
( 3051 , 88.73 )
( 3052 , 88.73 )
( 3053 , 88.85 )
( 3054 , 88.92 )
( 3055 , 88.92 )
( 3056 , 88.93 )
( 3057 , 89.16 )
( 3058 , 89.16 )
( 3059 , 89.41 )
( 3060 , 89.70 )
( 3061 , 89.99 )
( 3062 , 90.38 )
( 3063 , 90.67 )
( 3064 , 90.92 )
( 3065 , 91.15 )
( 3066 , 91.16 )
( 3067 , 91.16 )
( 3068 , 91.16 )
( 3069 , 91.16 )
( 3070 , 91.19 )
( 3071 , 91.25 )
( 3072 , 91.30 )
( 3073 , 91.30 )
( 3074 , 91.56 )
( 3075 , 91.71 )
( 3076 , 91.71 )
( 3077 , 91.71 )
( 3078 , 91.92 )
( 3079 , 91.97 )
( 3080 , 91.98 )
( 3081 , 92.01 )
( 3082 , 92.18 )
( 3083 , 92.37 )
( 3084 , 92.59 )
( 3085 , 92.81 )
( 3086 , 92.98 )
( 3087 , 93.22 )
( 3088 , 93.41 )
( 3089 , 93.56 )
( 3090 , 93.74 )
( 3091 , 93.89 )
( 3092 , 93.89 )
( 3093 , 93.98 )
( 3094 , 94.03 )
( 3095 , 94.03 )
( 3096 , 94.20 )
( 3097 , 94.38 )
( 3098 , 94.55 )
( 3099 , 94.74 )
( 3100 , 94.91 )
( 3101 , 95.06 )
( 3102 , 95.06 )
( 3103 , 95.06 )
( 3104 , 95.09 )
( 3105 , 95.09 )
( 3106 , 95.17 )
( 3107 , 95.24 )
( 3108 , 95.24 )
( 3109 , 95.25 )
( 3110 , 95.25 )
( 3111 , 95.28 )
( 3112 , 95.28 )
( 3113 , 95.48 )
( 3114 , 95.68 )
( 3115 , 95.84 )
( 3116 , 95.99 )
( 3117 , 96.14 )
( 3118 , 96.16 )
( 3119 , 96.16 )
( 3120 , 96.29 )
( 3121 , 96.33 )
( 3122 , 96.33 )
( 3123 , 96.43 )
( 3124 , 96.47 )
( 3125 , 96.55 )
( 3126 , 96.72 )
( 3127 , 96.95 )
( 3128 , 97.14 )
( 3129 , 97.32 )
( 3130 , 97.18 )
( 3131 , 97.26 )
( 3132 , 97.13 )
( 3133 , 97.01 )
( 3134 , 96.86 )
( 3135 , 96.56 )
( 3136 , 96.34 )
( 3137 , 96.25 )
( 3138 , 96.19 )
( 3139 , 96.08 )
( 3140 , 95.95 )
( 3141 , 95.84 )
( 3142 , 95.64 )
( 3143 , 95.45 )
( 3144 , 95.30 )
( 3145 , 95.05 )
( 3146 , 94.80 )
( 3147 , 94.51 )
( 3148 , 94.20 )
( 3149 , 93.91 )
( 3150 , 93.61 )
( 3151 , 93.36 )
( 3152 , 93.05 )
( 3153 , 92.82 )
( 3154 , 92.52 )
( 3155 , 92.22 )
( 3156 , 92.12 )
( 3157 , 92.03 )
( 3158 , 91.73 )
( 3159 , 91.43 )
( 3160 , 91.13 )
( 3161 , 90.90 )
( 3162 , 90.60 )
( 3163 , 90.40 )
( 3164 , 90.15 )
( 3165 , 89.84 )
( 3166 , 89.55 )
( 3167 , 89.38 )
( 3168 , 89.16 )
( 3169 , 88.88 )
( 3170 , 88.58 )
( 3171 , 88.34 )
( 3172 , 88.05 )
( 3173 , 87.74 )
( 3174 , 87.45 )
( 3175 , 87.14 )
( 3176 , 86.88 )
( 3177 , 86.59 )
( 3178 , 86.31 )
( 3179 , 86.03 )
( 3180 , 85.79 )
( 3181 , 85.69 )
( 3182 , 85.59 )
( 3183 , 85.54 )
( 3184 , 85.23 )
( 3185 , 84.96 )
( 3186 , 84.82 )
( 3187 , 84.52 )
( 3188 , 84.23 )
( 3189 , 83.97 )
( 3190 , 83.72 )
( 3191 , 83.42 )
( 3192 , 83.12 )
( 3193 , 82.82 )
( 3194 , 82.52 )
( 3195 , 82.24 )
( 3196 , 81.95 )
( 3197 , 81.80 )
( 3198 , 81.70 )
( 3199 , 81.39 )
( 3200 , 81.30 )
( 3201 , 81.20 )
( 3202 , 80.99 )
( 3203 , 80.83 )
( 3204 , 80.62 )
( 3205 , 80.42 )
( 3206 , 80.26 )
( 3207 , 79.96 )
( 3208 , 79.66 )
( 3209 , 79.37 )
( 3210 , 79.07 )
( 3211 , 78.80 )
( 3212 , 78.50 )
( 3213 , 78.40 )
( 3214 , 78.31 )
( 3215 , 78.28 )
( 3216 , 78.22 )
( 3217 , 78.16 )
( 3218 , 77.98 )
( 3219 , 77.67 )
( 3220 , 77.55 )
( 3221 , 77.24 )
( 3222 , 77.10 )
( 3223 , 76.93 )
( 3224 , 76.62 )
( 3225 , 76.33 )
( 3226 , 76.27 )
( 3227 , 76.20 )
( 3228 , 75.92 )
( 3229 , 75.71 )
( 3230 , 75.67 )
( 3231 , 75.40 )
( 3232 , 75.12 )
( 3233 , 74.84 )
( 3234 , 74.54 )
( 3235 , 74.34 )
( 3236 , 74.27 )
( 3237 , 74.14 )
( 3238 , 73.86 )
( 3239 , 73.55 )
( 3240 , 73.30 )
( 3241 , 73.09 )
( 3242 , 72.84 )
( 3243 , 72.59 )
( 3244 , 72.44 )
( 3245 , 72.16 )
( 3246 , 71.98 )
( 3247 , 71.80 )
( 3248 , 71.81 )
( 3249 , 71.55 )
( 3250 , 71.24 )
( 3251 , 70.97 )
( 3252 , 70.67 )
( 3253 , 70.38 )
( 3254 , 70.12 )
( 3255 , 69.82 )
( 3256 , 69.52 )
( 3257 , 69.22 )
( 3258 , 68.92 )
( 3259 , 68.65 )
( 3260 , 68.39 )
( 3261 , 68.09 )
( 3262 , 67.91 )
( 3263 , 67.71 )
( 3264 , 67.54 )
( 3265 , 67.36 )
( 3266 , 67.05 )
( 3267 , 66.92 )
( 3268 , 66.64 )
( 3269 , 66.34 )
( 3270 , 66.04 )
( 3271 , 65.73 )
( 3272 , 65.44 )
( 3273 , 65.34 )
( 3274 , 65.04 )
( 3275 , 64.75 )
( 3276 , 64.48 )
( 3277 , 64.38 )
( 3278 , 64.31 )
( 3279 , 64.06 )
( 3280 , 63.76 )
( 3281 , 63.47 )
( 3282 , 63.35 )
( 3283 , 63.33 )
( 3284 , 63.21 )
( 3285 , 63.06 )
( 3286 , 62.92 )
( 3287 , 62.63 )
( 3288 , 62.33 )
( 3289 , 62.03 )
( 3290 , 61.97 )
( 3291 , 62.02 )
( 3292 , 62.05 )
( 3293 , 61.96 )
( 3294 , 61.98 )
( 3295 , 61.78 )
( 3296 , 61.61 )
( 3297 , 61.31 )
( 3298 , 61.34 )
( 3299 , 61.25 )
( 3300 , 61.24 )
( 3301 , 61.21 )
( 3302 , 61.04 )
( 3303 , 60.74 )
( 3304 , 60.44 )
( 3305 , 60.32 )
( 3306 , 60.28 )
( 3307 , 60.15 )
( 3308 , 60.03 )
( 3309 , 59.93 )
( 3310 , 59.85 )
( 3311 , 59.89 )
( 3312 , 59.83 )
( 3313 , 59.77 )
( 3314 , 59.64 )
( 3315 , 59.56 )
( 3316 , 59.44 )
( 3317 , 59.34 )
( 3318 , 59.24 )
( 3319 , 59.11 )
( 3320 , 58.99 )
( 3321 , 58.89 )
( 3322 , 58.88 )
( 3323 , 58.95 )
( 3324 , 58.84 )
( 3325 , 58.71 )
( 3326 , 58.87 )
( 3327 , 59.04 )
( 3328 , 59.18 )
( 3329 , 59.29 )
( 3330 , 59.39 )
( 3331 , 59.49 )
( 3332 , 59.66 )
( 3333 , 59.85 )
( 3334 , 59.95 )
( 3335 , 60.04 )
( 3336 , 60.20 )
( 3337 , 60.43 )
( 3338 , 60.62 )
( 3339 , 60.82 )
( 3340 , 61.05 )
( 3341 , 61.14 )
( 3342 , 61.27 )
( 3343 , 61.36 )
( 3344 , 61.46 )
( 3345 , 61.56 )
( 3346 , 61.77 )
( 3347 , 62.03 )
( 3348 , 62.23 )
( 3349 , 62.43 )
( 3350 , 62.66 )
( 3351 , 62.80 )
( 3352 , 62.94 )
( 3353 , 63.21 )
( 3354 , 63.48 )
( 3355 , 63.67 )
( 3356 , 63.79 )
( 3357 , 63.91 )
( 3358 , 64.02 )
( 3359 , 64.15 )
( 3360 , 64.34 )
( 3361 , 64.46 )
( 3362 , 64.51 )
( 3363 , 64.55 )
( 3364 , 64.61 )
( 3365 , 64.65 )
( 3366 , 64.79 )
( 3367 , 64.78 )
( 3368 , 64.79 )
( 3369 , 64.95 )
( 3370 , 65.02 )
( 3371 , 65.02 )
( 3372 , 65.18 )
( 3373 , 65.18 )
( 3374 , 65.16 )
( 3375 , 65.13 )
( 3376 , 65.25 )
( 3377 , 65.24 )
( 3378 , 65.28 )
( 3379 , 65.26 )
( 3380 , 65.34 )
( 3381 , 65.33 )
( 3382 , 65.38 )
( 3383 , 65.41 )
( 3384 , 65.38 )
( 3385 , 65.25 )
( 3386 , 65.12 )
( 3387 , 65.00 )
( 3388 , 64.88 )
( 3389 , 65.01 )
( 3390 , 65.13 )
( 3391 , 65.23 )
( 3392 , 65.39 )
( 3393 , 65.46 )
( 3394 , 65.45 )
( 3395 , 65.46 )
( 3396 , 65.49 )
( 3397 , 65.63 )
( 3398 , 65.75 )
( 3399 , 65.90 )
( 3400 , 66.03 )
( 3401 , 66.01 )
( 3402 , 66.20 )
( 3403 , 66.44 )
( 3404 , 66.63 )
( 3405 , 66.67 )
( 3406 , 66.65 )
( 3407 , 66.65 )
( 3408 , 66.66 )
( 3409 , 66.62 )
( 3410 , 66.77 )
( 3411 , 66.98 )
( 3412 , 67.22 )
( 3413 , 67.44 )
( 3414 , 67.68 )
( 3415 , 67.80 )
( 3416 , 67.79 )
( 3417 , 67.78 )
( 3418 , 67.75 )
( 3419 , 67.73 )
( 3420 , 67.77 )
( 3421 , 67.78 )
( 3422 , 67.75 )
( 3423 , 67.73 )
( 3424 , 67.70 )
( 3425 , 67.67 )
( 3426 , 67.73 )
( 3427 , 67.74 )
( 3428 , 67.84 )
( 3429 , 67.92 )
( 3430 , 68.12 )
( 3431 , 68.40 )
( 3432 , 68.70 )
( 3433 , 68.97 )
( 3434 , 69.23 )
( 3435 , 69.48 )
( 3436 , 69.46 )
( 3437 , 69.40 )
( 3438 , 69.33 )
( 3439 , 69.25 )
( 3440 , 69.39 )
( 3441 , 69.67 )
( 3442 , 69.97 )
( 3443 , 70.16 )
( 3444 , 70.34 )
( 3445 , 70.59 )
( 3446 , 70.84 )
( 3447 , 70.97 )
( 3448 , 71.02 )
( 3449 , 71.06 )
( 3450 , 71.10 )
( 3451 , 71.15 )
( 3452 , 71.19 )
( 3453 , 71.23 )
( 3454 , 71.27 )
( 3455 , 71.20 )
( 3456 , 71.07 )
( 3457 , 70.96 )
( 3458 , 70.84 )
( 3459 , 70.88 )
( 3460 , 70.76 )
( 3461 , 70.69 )
( 3462 , 70.84 )
( 3463 , 70.80 )
( 3464 , 70.67 )
( 3465 , 70.55 )
( 3466 , 70.59 )
( 3467 , 70.63 )
( 3468 , 70.70 )
( 3469 , 70.75 )
( 3470 , 70.80 )
( 3471 , 70.84 )
( 3472 , 70.98 )
( 3473 , 71.09 )
( 3474 , 71.20 )
( 3475 , 71.33 )
( 3476 , 71.26 )
( 3477 , 71.16 )
( 3478 , 71.04 )
( 3479 , 70.77 )
( 3480 , 70.51 )
( 3481 , 70.23 )
( 3482 , 69.94 )
( 3483 , 69.68 )
( 3484 , 69.40 )
( 3485 , 69.16 )
( 3486 , 68.91 )
( 3487 , 68.61 )
( 3488 , 68.41 )
( 3489 , 68.10 )
( 3490 , 68.04 )
( 3491 , 68.03 )
( 3492 , 67.98 )
( 3493 , 67.92 )
( 3494 , 67.62 )
( 3495 , 67.35 )
( 3496 , 67.16 )
( 3497 , 66.87 )
( 3498 , 66.67 )
( 3499 , 66.44 )
( 3500 , 66.32 )
( 3501 , 66.02 )
( 3502 , 65.72 )
( 3503 , 65.41 )
( 3504 , 65.19 )
( 3505 , 65.05 )
( 3506 , 64.75 )
( 3507 , 64.45 )
( 3508 , 64.16 )
( 3509 , 64.02 )
( 3510 , 63.89 )
( 3511 , 63.61 )
( 3512 , 63.35 )
( 3513 , 63.05 )
( 3514 , 62.75 )
( 3515 , 62.45 )
( 3516 , 62.25 )
( 3517 , 61.95 )
( 3518 , 61.67 )
( 3519 , 61.37 )
( 3520 , 61.07 )
( 3521 , 60.78 )
( 3522 , 60.59 )
( 3523 , 60.47 )
( 3524 , 60.32 )
( 3525 , 60.18 )
( 3526 , 60.05 )
( 3527 , 59.80 )
( 3528 , 59.50 )
( 3529 , 59.24 )
( 3530 , 58.94 )
( 3531 , 58.84 )
( 3532 , 58.79 )
( 3533 , 58.82 )
( 3534 , 58.52 )
( 3535 , 58.22 )
( 3536 , 57.99 )
( 3537 , 57.70 )
( 3538 , 57.40 )
( 3539 , 57.13 )
( 3540 , 56.86 )
( 3541 , 56.55 )
( 3542 , 56.25 )
( 3543 , 56.08 )
( 3544 , 55.78 )
( 3545 , 55.63 )
( 3546 , 55.55 )
( 3547 , 55.48 )
( 3548 , 55.18 )
( 3549 , 54.88 )
( 3550 , 55.08 )
( 3551 , 55.37 )
( 3552 , 55.66 )
( 3553 , 55.89 )
( 3554 , 55.99 )
( 3555 , 56.09 )
( 3556 , 56.25 )
( 3557 , 56.38 )
( 3558 , 56.50 )
( 3559 , 56.72 )
( 3560 , 56.86 )
( 3561 , 57.00 )
( 3562 , 57.12 )
( 3563 , 57.25 )
( 3564 , 57.35 )
( 3565 , 57.48 )
( 3566 , 57.62 )
( 3567 , 57.71 )
( 3568 , 57.84 )
( 3569 , 57.96 )
( 3570 , 58.09 )
( 3571 , 58.24 )
( 3572 , 58.30 )
( 3573 , 58.25 )
( 3574 , 58.29 )
( 3575 , 58.20 )
( 3576 , 58.07 )
( 3577 , 57.95 )
( 3578 , 57.82 )
( 3579 , 57.70 )
( 3580 , 57.57 )
( 3581 , 57.45 )
( 3582 , 57.38 )
( 3583 , 57.25 )
( 3584 , 57.13 )
( 3585 , 57.01 )
( 3586 , 57.05 )
( 3587 , 57.09 )
( 3588 , 56.96 )
( 3589 , 56.84 )
( 3590 , 56.90 )
( 3591 , 56.79 )
( 3592 , 56.70 )
( 3593 , 56.65 )
( 3594 , 56.58 )
( 3595 , 56.58 )
( 3596 , 56.46 )
( 3597 , 56.36 )
( 3598 , 56.40 )
( 3599 , 56.53 )
( 3600 , 56.49 )
( 3601 , 56.59 )
( 3602 , 56.71 )
( 3603 , 56.78 )
( 3604 , 56.72 )
( 3605 , 56.72 )
( 3606 , 56.67 )
( 3607 , 56.61 )
( 3608 , 56.47 )
( 3609 , 56.17 )
( 3610 , 55.94 )
( 3611 , 55.79 )
( 3612 , 55.80 )
( 3613 , 55.71 )
( 3614 , 55.62 )
( 3615 , 55.57 )
( 3616 , 55.42 )
( 3617 , 55.12 )
( 3618 , 54.95 )
( 3619 , 54.94 )
( 3620 , 54.86 )
( 3621 , 54.76 )
( 3622 , 54.66 )
( 3623 , 54.57 )
( 3624 , 54.48 )
( 3625 , 54.38 )
( 3626 , 54.29 )
( 3627 , 53.98 )
( 3628 , 53.70 )
( 3629 , 53.58 )
( 3630 , 53.28 )
( 3631 , 53.15 )
( 3632 , 53.03 )
( 3633 , 52.94 )
( 3634 , 52.82 )
( 3635 , 52.71 )
( 3636 , 52.59 )
( 3637 , 52.80 )
( 3638 , 53.05 )
( 3639 , 53.29 )
( 3640 , 53.47 )
( 3641 , 53.80 )
( 3642 , 54.03 )
( 3643 , 54.21 )
( 3644 , 54.40 )
( 3645 , 54.57 )
( 3646 , 54.75 )
( 3647 , 55.04 )
( 3648 , 55.22 )
( 3649 , 55.39 )
( 3650 , 55.57 )
( 3651 , 55.80 )
( 3652 , 56.02 )
( 3653 , 56.20 )
( 3654 , 56.40 )
( 3655 , 56.57 )
( 3656 , 56.85 )
( 3657 , 57.03 )
( 3658 , 57.20 )
( 3659 , 57.38 )
( 3660 , 57.58 )
( 3661 , 57.93 )
( 3662 , 58.27 )
( 3663 , 58.61 )
( 3664 , 58.94 )
( 3665 , 59.29 )
( 3666 , 59.61 )
( 3667 , 59.96 )
( 3668 , 59.94 )
( 3669 , 59.91 )
( 3670 , 59.88 )
( 3671 , 59.85 )
( 3672 , 59.79 )
( 3673 , 59.75 )
( 3674 , 59.69 )
( 3675 , 59.78 )
( 3676 , 59.86 )
( 3677 , 59.98 )
( 3678 , 59.98 )
( 3679 , 60.10 )
( 3680 , 60.22 )
( 3681 , 60.19 )
( 3682 , 60.26 )
( 3683 , 60.23 )
( 3684 , 60.22 )
( 3685 , 60.17 )
( 3686 , 60.11 )
( 3687 , 60.05 )
( 3688 , 60.04 )
( 3689 , 60.05 )
( 3690 , 60.09 )
( 3691 , 60.10 )
( 3692 , 60.12 )
( 3693 , 60.14 )
( 3694 , 60.11 )
( 3695 , 60.19 )
( 3696 , 60.16 )
( 3697 , 60.30 )
( 3698 , 60.33 )
( 3699 , 60.37 )
( 3700 , 60.34 )
( 3701 , 60.41 )
( 3702 , 60.50 )
( 3703 , 60.63 )
( 3704 , 60.73 )
( 3705 , 60.79 )
( 3706 , 60.82 )
( 3707 , 60.87 )
( 3708 , 60.75 )
( 3709 , 60.62 )
( 3710 , 60.71 )
( 3711 , 60.75 )
( 3712 , 60.81 )
( 3713 , 60.88 )
( 3714 , 60.95 )
( 3715 , 60.99 )
( 3716 , 60.95 )
( 3717 , 60.83 )
( 3718 , 60.75 )
( 3719 , 60.66 )
( 3720 , 60.54 )
( 3721 , 60.42 )
( 3722 , 60.30 )
( 3723 , 60.17 )
( 3724 , 60.21 )
( 3725 , 60.25 )
( 3726 , 60.25 )
( 3727 , 60.12 )
( 3728 , 60.14 )
( 3729 , 60.18 )
( 3730 , 60.12 )
( 3731 , 60.16 )
( 3732 , 60.12 )
( 3733 , 60.07 )
( 3734 , 60.02 )
( 3735 , 59.96 )
( 3736 , 59.90 )
( 3737 , 59.85 )
( 3738 , 59.79 )
( 3739 , 59.73 )
( 3740 , 59.68 )
( 3741 , 59.62 )
( 3742 , 59.57 )
( 3743 , 59.51 )
( 3744 , 59.48 )
( 3745 , 59.47 )
( 3746 , 59.46 )
( 3747 , 59.45 )
( 3748 , 59.61 )
( 3749 , 59.67 )
( 3750 , 59.66 )
( 3751 , 59.80 )
( 3752 , 59.95 )
( 3753 , 60.11 )
( 3754 , 60.26 )
( 3755 , 60.23 )
( 3756 , 60.21 )
( 3757 , 60.23 )
( 3758 , 60.20 )
( 3759 , 60.24 )
( 3760 , 60.21 )
( 3761 , 60.09 )
( 3762 , 59.96 )
( 3763 , 60.03 )
( 3764 , 60.11 )
( 3765 , 60.08 )
( 3766 , 60.02 )
( 3767 , 60.00 )
( 3768 , 59.94 )
( 3769 , 59.91 )
( 3770 , 59.89 )
( 3771 , 59.83 )
( 3772 , 59.77 )
( 3773 , 59.71 )
( 3774 , 59.70 )
( 3775 , 59.72 )
( 3776 , 59.89 )
( 3777 , 59.84 )
( 3778 , 59.82 )
( 3779 , 59.93 )
( 3780 , 60.08 )
( 3781 , 60.04 )
( 3782 , 59.92 )
( 3783 , 59.83 )
( 3784 , 59.70 )
( 3785 , 59.58 )
( 3786 , 59.55 )
( 3787 , 59.42 )
( 3788 , 59.31 )
( 3789 , 59.23 )
( 3790 , 59.10 )
( 3791 , 58.98 )
( 3792 , 58.77 )
( 3793 , 58.47 )
( 3794 , 58.18 )
( 3795 , 57.88 )
( 3796 , 57.61 )
( 3797 , 57.40 )
( 3798 , 57.10 )
( 3799 , 56.80 )
( 3800 , 56.70 )
( 3801 , 56.66 )
( 3802 , 56.59 )
( 3803 , 56.30 )
( 3804 , 56.01 )
( 3805 , 55.80 )
( 3806 , 55.70 )
( 3807 , 55.69 )
( 3808 , 55.66 )
( 3809 , 55.62 )
( 3810 , 55.48 )
( 3811 , 55.29 )
( 3812 , 55.05 )
( 3813 , 54.79 )
( 3814 , 54.49 )
( 3815 , 54.22 )
( 3816 , 53.92 )
( 3817 , 53.72 )
( 3818 , 53.43 )
( 3819 , 53.13 )
( 3820 , 52.86 )
( 3821 , 52.76 )
( 3822 , 52.46 )
( 3823 , 52.37 )
( 3824 , 52.34 )
( 3825 , 52.32 )
( 3826 , 52.23 )
( 3827 , 52.13 )
( 3828 , 52.07 )
( 3829 , 52.12 )
( 3830 , 52.02 )
( 3831 , 51.96 )
( 3832 , 51.91 )
( 3833 , 51.86 )
( 3834 , 51.76 )
( 3835 , 51.71 )
( 3836 , 51.66 )
( 3837 , 51.59 )
( 3838 , 51.54 )
( 3839 , 51.62 )
( 3840 , 51.48 )
( 3841 , 51.33 )
( 3842 , 51.09 )
( 3843 , 50.79 )
( 3844 , 50.50 )
( 3845 , 50.20 )
( 3846 , 50.07 )
( 3847 , 49.95 )
( 3848 , 49.91 )
( 3849 , 49.61 )
( 3850 , 49.33 )
( 3851 , 49.03 )
( 3852 , 48.90 )
( 3853 , 48.79 )
( 3854 , 48.68 )
( 3855 , 48.55 )
( 3856 , 48.25 )
( 3857 , 47.95 )
( 3858 , 47.64 )
( 3859 , 47.37 )
( 3860 , 47.09 )
( 3861 , 46.80 )
( 3862 , 46.51 )
( 3863 , 46.23 )
( 3864 , 46.08 )
( 3865 , 45.78 )
( 3866 , 45.66 )
( 3867 , 45.43 )
( 3868 , 45.13 )
( 3869 , 45.00 )
( 3870 , 44.70 )
( 3871 , 44.43 )
( 3872 , 44.18 )
( 3873 , 44.04 )
( 3874 , 43.81 )
( 3875 , 43.53 )
( 3876 , 43.46 )
( 3877 , 43.20 )
( 3878 , 42.89 )
( 3879 , 42.59 )
( 3880 , 42.29 )
( 3881 , 41.99 )
( 3882 , 41.69 )
( 3883 , 41.50 )
( 3884 , 41.23 )
( 3885 , 41.13 )
( 3886 , 41.18 )
( 3887 , 41.21 )
( 3888 , 41.12 )
( 3889 , 40.99 )
( 3890 , 40.70 )
( 3891 , 40.45 )
( 3892 , 40.15 )
( 3893 , 39.99 )
( 3894 , 39.79 )
( 3895 , 39.64 )
( 3896 , 39.34 )
( 3897 , 39.05 )
( 3898 , 38.87 )
( 3899 , 38.57 )
( 3900 , 38.45 )
( 3901 , 38.20 )
( 3902 , 37.91 )
( 3903 , 37.91 )
( 3904 , 37.83 )
( 3905 , 37.76 )
( 3906 , 37.46 )
( 3907 , 37.16 )
( 3908 , 36.85 )
( 3909 , 36.57 )
( 3910 , 36.26 )
( 3911 , 36.15 )
( 3912 , 35.96 )
( 3913 , 35.66 )
( 3914 , 35.36 )
( 3915 , 35.17 )
( 3916 , 34.90 )
( 3917 , 34.60 )
( 3918 , 34.54 )
( 3919 , 34.34 )
( 3920 , 34.11 )
( 3921 , 33.82 )
( 3922 , 33.79 )
( 3923 , 33.77 )
( 3924 , 33.75 )
( 3925 , 33.54 )
( 3926 , 33.33 )
( 3927 , 33.05 )
( 3928 , 32.75 )
( 3929 , 32.45 )
( 3930 , 32.23 )
( 3931 , 32.06 )
( 3932 , 31.87 )
( 3933 , 31.59 )
( 3934 , 31.29 )
( 3935 , 31.02 )
( 3936 , 30.73 )
( 3937 , 30.43 )
( 3938 , 30.13 )
( 3939 , 29.83 )
( 3940 , 29.53 )
( 3941 , 29.25 )
( 3942 , 28.95 )
( 3943 , 28.83 )
( 3944 , 28.70 )
( 3945 , 28.90 )
( 3946 , 28.77 )
( 3947 , 28.67 )
( 3948 , 28.56 )
( 3949 , 28.46 )
( 3950 , 28.36 )
( 3951 , 28.23 )
( 3952 , 28.11 )
( 3953 , 28.05 )
( 3954 , 27.99 )
( 3955 , 27.99 )
( 3956 , 27.95 )
( 3957 , 27.89 )
( 3958 , 27.95 )
( 3959 , 28.01 )
( 3960 , 28.02 )
( 3961 , 27.97 )
( 3962 , 27.95 )
( 3963 , 27.94 )
( 3964 , 27.95 )
( 3965 , 27.92 )
( 3966 , 27.87 )
( 3967 , 27.82 )
( 3968 , 27.76 )
( 3969 , 27.63 )
( 3970 , 27.51 )
( 3971 , 27.70 )
( 3972 , 27.93 )
( 3973 , 28.16 )
( 3974 , 28.38 )
( 3975 , 28.55 )
( 3976 , 28.79 )
( 3977 , 29.11 )
( 3978 , 29.43 )
( 3979 , 29.75 )
( 3980 , 30.08 )
( 3981 , 30.37 )
( 3982 , 30.55 )
( 3983 , 30.83 )
( 3984 , 31.00 )
( 3985 , 31.30 )
( 3986 , 31.58 )
( 3987 , 31.85 )
( 3988 , 32.06 )
( 3989 , 32.34 )
( 3990 , 32.62 )
( 3991 , 32.80 )
( 3992 , 32.97 )
( 3993 , 33.16 )
( 3994 , 33.34 )
( 3995 , 33.52 )
( 3996 , 33.74 )
( 3997 , 33.95 )
( 3998 , 34.16 )
( 3999 , 34.34 )
( 4000 , 34.59 )
( 4001 , 34.84 )
( 4002 , 35.10 )
( 4003 , 35.37 )
( 4004 , 35.60 )
( 4005 , 35.84 )
( 4006 , 36.07 )
( 4007 , 36.36 )
( 4008 , 36.61 )
( 4009 , 36.89 )
( 4010 , 37.17 )
( 4011 , 37.43 )
( 4012 , 37.37 )
( 4013 , 37.31 )
( 4014 , 37.29 )
( 4015 , 37.22 )
( 4016 , 37.16 )
( 4017 , 37.03 )
( 4018 , 37.07 )
( 4019 , 36.95 )
( 4020 , 36.89 )
( 4021 , 36.77 )
( 4022 , 36.73 )
( 4023 , 36.73 )
( 4024 , 36.60 )
( 4025 , 36.68 )
( 4026 , 36.79 )
( 4027 , 36.84 )
( 4028 , 36.89 )
( 4029 , 36.78 )
( 4030 , 36.74 )
( 4031 , 36.66 )
( 4032 , 36.55 )
( 4033 , 36.43 )
( 4034 , 36.38 )
( 4035 , 36.26 )
( 4036 , 36.14 )
( 4037 , 36.20 )
( 4038 , 36.07 )
( 4039 , 36.07 )
( 4040 , 36.25 )
( 4041 , 36.51 )
( 4042 , 36.82 )
( 4043 , 36.99 )
( 4044 , 37.17 )
( 4045 , 37.39 )
( 4046 , 37.56 )
( 4047 , 37.74 )
( 4048 , 38.01 )
( 4049 , 38.19 )
( 4050 , 38.41 )
( 4051 , 38.61 )
( 4052 , 38.79 )
( 4053 , 38.96 )
( 4054 , 39.14 )
( 4055 , 39.38 )
( 4056 , 39.57 )
( 4057 , 39.84 )
( 4058 , 40.07 )
( 4059 , 40.24 )
( 4060 , 40.44 )
( 4061 , 40.62 )
( 4062 , 40.85 )
( 4063 , 41.07 )
( 4064 , 41.25 )
( 4065 , 41.48 )
( 4066 , 41.66 )
( 4067 , 41.90 )
( 4068 , 42.15 )
( 4069 , 42.39 )
( 4070 , 42.63 )
( 4071 , 42.91 )
( 4072 , 43.09 )
( 4073 , 43.35 )
( 4074 , 43.64 )
( 4075 , 43.92 )
( 4076 , 44.34 )
( 4077 , 44.77 )
( 4078 , 45.18 )
( 4079 , 45.52 )
( 4080 , 45.74 )
( 4081 , 45.96 )
( 4082 , 46.29 )
( 4083 , 46.68 )
( 4084 , 47.03 )
( 4085 , 47.36 )
( 4086 , 47.72 )
( 4087 , 48.12 )
( 4088 , 48.50 )
( 4089 , 48.81 )
( 4090 , 49.15 )
( 4091 , 49.46 )
( 4092 , 49.79 )
( 4093 , 50.09 )
( 4094 , 50.39 )
( 4095 , 50.69 )
( 4096 , 50.99 )
( 4097 , 51.34 )
( 4098 , 51.70 )
( 4099 , 52.11 )
( 4100 , 52.54 )
( 4101 , 52.96 )
( 4102 , 53.29 )
( 4103 , 53.61 )
( 4104 , 53.91 )
( 4105 , 54.21 )
( 4106 , 54.52 )
( 4107 , 54.84 )
( 4108 , 55.17 )
( 4109 , 55.53 )
( 4110 , 55.88 )
( 4111 , 56.19 )
( 4112 , 56.49 )
( 4113 , 56.90 )
( 4114 , 57.21 )
( 4115 , 57.52 )
( 4116 , 57.94 )
( 4117 , 58.36 )
( 4118 , 58.77 )
( 4119 , 59.19 )
( 4120 , 59.64 )
( 4121 , 60.06 )
( 4122 , 60.54 )
( 4123 , 60.89 )
( 4124 , 60.89 )
( 4125 , 61.11 )
( 4126 , 61.33 )
( 4127 , 61.53 )
( 4128 , 61.73 )
( 4129 , 61.93 )
( 4130 , 62.26 )
( 4131 , 62.51 )
( 4132 , 62.80 )
( 4133 , 63.06 )
( 4134 , 63.47 )
( 4135 , 63.85 )
( 4136 , 64.23 )
( 4137 , 64.68 )
( 4138 , 65.13 )
( 4139 , 65.60 )
( 4140 , 65.98 )
( 4141 , 66.38 )
( 4142 , 66.77 )
( 4143 , 67.04 )
( 4144 , 67.02 )
( 4145 , 67.05 )
( 4146 , 67.09 )
( 4147 , 67.15 )
( 4148 , 67.12 )
( 4149 , 67.27 )
( 4150 , 67.39 )
( 4151 , 67.54 )
( 4152 , 67.70 )
( 4153 , 67.82 )
( 4154 , 67.86 )
( 4155 , 67.89 )
( 4156 , 67.88 )
( 4157 , 67.91 )
( 4158 , 67.95 )
( 4159 , 68.00 )
( 4160 , 68.04 )
( 4161 , 68.17 )
( 4162 , 68.27 )
( 4163 , 68.38 )
( 4164 , 68.44 )
( 4165 , 68.51 )
( 4166 , 68.55 )
( 4167 , 68.63 )
( 4168 , 68.63 )
( 4169 , 68.82 )
( 4170 , 68.81 )
( 4171 , 68.69 )
( 4172 , 68.61 )
( 4173 , 68.52 )
( 4174 , 68.64 )
( 4175 , 68.77 )
( 4176 , 68.89 )
( 4177 , 69.02 )
( 4178 , 68.90 )
( 4179 , 68.82 )
( 4180 , 68.73 )
( 4181 , 68.63 )
( 4182 , 68.55 )
( 4183 , 68.42 )
( 4184 , 68.30 )
( 4185 , 68.48 )
( 4186 , 68.80 )
( 4187 , 69.20 )
( 4188 , 69.53 )
( 4189 , 69.85 )
( 4190 , 70.18 )
( 4191 , 70.50 )
( 4192 , 70.83 )
( 4193 , 71.16 )
( 4194 , 71.49 )
( 4195 , 71.77 )
( 4196 , 72.02 )
( 4197 , 72.15 )
( 4198 , 72.19 )
( 4199 , 72.27 )
( 4200 , 72.20 )
( 4201 , 72.07 )
( 4202 , 72.04 )
( 4203 , 71.97 )
( 4204 , 71.84 )
( 4205 , 71.72 )
( 4206 , 71.63 )
( 4207 , 71.55 )
( 4208 , 71.43 )
( 4209 , 71.56 )
( 4210 , 71.70 )
( 4211 , 71.79 )
( 4212 , 72.01 )
( 4213 , 72.23 )
( 4214 , 72.45 )
( 4215 , 72.66 )
( 4216 , 72.76 )
( 4217 , 72.89 )
( 4218 , 73.02 )
( 4219 , 73.16 )
( 4220 , 73.27 )
( 4221 , 73.37 )
( 4222 , 73.47 )
( 4223 , 73.56 )
( 4224 , 73.69 )
( 4225 , 73.93 )
( 4226 , 74.12 )
( 4227 , 74.32 )
( 4228 , 74.42 )
( 4229 , 74.54 )
( 4230 , 74.66 )
( 4231 , 74.80 )
( 4232 , 74.93 )
( 4233 , 75.07 )
( 4234 , 75.18 )
( 4235 , 75.27 )
( 4236 , 75.41 )
( 4237 , 75.57 )
( 4238 , 75.71 )
( 4239 , 75.85 )
( 4240 , 76.00 )
( 4241 , 76.14 )
( 4242 , 76.18 )
( 4243 , 76.05 )
( 4244 , 75.98 )
( 4245 , 75.91 )
( 4246 , 75.79 )
( 4247 , 75.68 )
( 4248 , 75.59 )
( 4249 , 75.48 )
( 4250 , 75.45 )
( 4251 , 75.41 )
( 4252 , 75.48 )
( 4253 , 75.60 )
( 4254 , 75.66 )
( 4255 , 75.76 )
( 4256 , 75.80 )
( 4257 , 75.67 )
( 4258 , 75.55 )
( 4259 , 75.45 )
( 4260 , 75.41 )
( 4261 , 75.46 )
( 4262 , 75.51 )
( 4263 , 75.38 )
( 4264 , 75.27 )
( 4265 , 75.14 )
( 4266 , 75.04 )
( 4267 , 74.99 )
( 4268 , 74.87 )
( 4269 , 74.74 )
( 4270 , 74.72 )
( 4271 , 74.69 )
( 4272 , 74.43 )
( 4273 , 74.13 )
( 4274 , 73.85 )
( 4275 , 73.64 )
( 4276 , 73.34 )
( 4277 , 73.35 )
( 4278 , 73.41 )
( 4279 , 73.33 )
( 4280 , 73.27 )
( 4281 , 73.15 )
( 4282 , 73.20 )
( 4283 , 73.31 )
( 4284 , 73.38 )
( 4285 , 73.45 )
( 4286 , 73.48 )
( 4287 , 73.57 )
( 4288 , 73.45 )
( 4289 , 73.57 )
( 4290 , 73.73 )
( 4291 , 73.86 )
( 4292 , 73.80 )
( 4293 , 73.75 )
( 4294 , 73.70 )
( 4295 , 73.63 )
( 4296 , 73.62 )
( 4297 , 73.51 )
( 4298 , 73.45 )
( 4299 , 73.32 )
( 4300 , 73.21 )
( 4301 , 73.09 )
( 4302 , 73.12 )
( 4303 , 73.02 )
( 4304 , 72.90 )
( 4305 , 72.77 )
( 4306 , 72.89 )
( 4307 , 73.00 )
( 4308 , 73.15 )
( 4309 , 73.29 )
( 4310 , 73.46 )
( 4311 , 73.54 )
( 4312 , 73.58 )
( 4313 , 73.62 )
( 4314 , 73.68 )
( 4315 , 73.79 )
( 4316 , 73.88 )
( 4317 , 73.95 )
( 4318 , 73.99 )
( 4319 , 73.87 )
( 4320 , 73.84 )
( 4321 , 73.76 )
( 4322 , 73.63 )
( 4323 , 73.53 )
( 4324 , 73.24 )
( 4325 , 73.18 )
( 4326 , 72.88 )
( 4327 , 72.84 )
( 4328 , 72.71 )
( 4329 , 72.67 )
( 4330 , 72.56 )
( 4331 , 72.51 )
( 4332 , 72.48 )
( 4333 , 72.56 )
( 4334 , 72.44 )
( 4335 , 72.49 )
( 4336 , 72.54 )
( 4337 , 72.59 )
( 4338 , 72.62 )
( 4339 , 72.66 )
( 4340 , 72.67 )
( 4341 , 72.66 )
( 4342 , 72.66 )
( 4343 , 72.73 )
( 4344 , 72.79 )
( 4345 , 72.80 )
( 4346 , 72.88 )
( 4347 , 72.92 )
( 4348 , 72.96 )
( 4349 , 72.95 )
( 4350 , 72.93 )
( 4351 , 72.87 )
( 4352 , 72.76 )
( 4353 , 72.68 )
( 4354 , 72.55 )
( 4355 , 72.48 )
( 4356 , 72.36 )
( 4357 , 72.23 )
( 4358 , 72.17 )
( 4359 , 72.09 )
( 4360 , 71.99 )
( 4361 , 71.88 )
( 4362 , 72.02 )
( 4363 , 72.14 )
( 4364 , 72.27 )
( 4365 , 72.16 )
( 4366 , 72.03 )
( 4367 , 72.01 )
( 4368 , 71.91 )
( 4369 , 71.95 )
( 4370 , 71.82 )
( 4371 , 71.70 )
( 4372 , 71.59 )
( 4373 , 71.48 )
( 4374 , 71.35 )
( 4375 , 71.23 )
( 4376 , 71.11 )
( 4377 , 70.98 )
( 4378 , 70.86 )
( 4379 , 70.73 )
( 4380 , 70.66 )
( 4381 , 70.53 )
( 4382 , 70.41 )
( 4383 , 70.33 )
( 4384 , 70.20 )
( 4385 , 70.13 )
( 4386 , 70.09 )
( 4387 , 70.02 )
( 4388 , 69.90 )
( 4389 , 69.84 )
( 4390 , 69.72 )
( 4391 , 69.59 )
( 4392 , 69.47 )
( 4393 , 69.47 )
( 4394 , 69.46 )
( 4395 , 69.43 )
( 4396 , 69.43 )
( 4397 , 69.12 )
( 4398 , 68.93 )
( 4399 , 68.63 )
( 4400 , 68.34 )
( 4401 , 68.13 )
( 4402 , 67.84 )
( 4403 , 67.61 )
( 4404 , 67.45 )
( 4405 , 67.42 )
( 4406 , 67.23 )
( 4407 , 66.93 )
( 4408 , 66.84 )
( 4409 , 66.54 )
( 4410 , 66.23 )
( 4411 , 65.94 )
( 4412 , 65.63 )
( 4413 , 65.34 )
( 4414 , 65.24 )
( 4415 , 64.95 )
( 4416 , 64.80 )
( 4417 , 64.52 )
( 4418 , 64.23 )
( 4419 , 64.04 )
( 4420 , 63.96 )
( 4421 , 63.99 )
( 4422 , 63.69 )
( 4423 , 63.39 )
( 4424 , 63.30 )
( 4425 , 63.16 )
( 4426 , 63.01 )
( 4427 , 62.84 )
( 4428 , 62.82 )
( 4429 , 62.87 )
( 4430 , 62.57 )
( 4431 , 62.27 )
( 4432 , 62.02 )
( 4433 , 61.72 )
( 4434 , 61.67 )
( 4435 , 61.57 )
( 4436 , 61.50 )
( 4437 , 61.48 )
( 4438 , 61.49 )
( 4439 , 61.46 )
( 4440 , 61.40 )
( 4441 , 61.34 )
( 4442 , 61.04 )
( 4443 , 60.95 )
( 4444 , 60.88 )
( 4445 , 60.73 )
( 4446 , 60.49 )
( 4447 , 60.38 )
( 4448 , 60.24 )
( 4449 , 60.09 )
( 4450 , 59.95 )
( 4451 , 59.75 )
( 4452 , 59.69 )
( 4453 , 59.49 )
( 4454 , 59.19 )
( 4455 , 58.95 )
( 4456 , 58.86 )
( 4457 , 58.76 )
( 4458 , 58.61 )
( 4459 , 58.47 )
( 4460 , 58.26 )
( 4461 , 57.96 )
( 4462 , 57.66 )
( 4463 , 57.38 )
( 4464 , 57.07 )
( 4465 , 56.90 )
( 4466 , 56.66 )
( 4467 , 56.36 )
( 4468 , 56.21 )
( 4469 , 56.04 )
( 4470 , 55.84 )
( 4471 , 55.69 )
( 4472 , 55.68 )
( 4473 , 55.70 )
( 4474 , 55.68 )
( 4475 , 55.60 )
( 4476 , 55.54 )
( 4477 , 55.35 )
( 4478 , 55.30 )
( 4479 , 55.00 )
( 4480 , 54.81 )
( 4481 , 54.62 )
( 4482 , 54.61 )
( 4483 , 54.76 )
( 4484 , 54.78 )
( 4485 , 54.69 )
( 4486 , 54.71 )
( 4487 , 54.64 )
( 4488 , 54.35 )
( 4489 , 54.05 )
( 4490 , 53.85 )
( 4491 , 53.66 )
( 4492 , 53.57 )
( 4493 , 53.27 )
( 4494 , 52.98 )
( 4495 , 52.71 )
( 4496 , 52.59 )
( 4497 , 52.46 )
( 4498 , 52.31 )
( 4499 , 52.19 )
( 4500 , 51.89 )
( 4501 , 51.59 )
( 4502 , 51.38 )
( 4503 , 51.16 )
( 4504 , 50.91 )
( 4505 , 50.81 )
( 4506 , 50.54 )
( 4507 , 50.45 )
( 4508 , 50.27 )
( 4509 , 50.21 )
( 4510 , 50.15 )
( 4511 , 50.02 )
( 4512 , 49.88 )
( 4513 , 49.73 )
( 4514 , 49.63 )
( 4515 , 49.51 )
( 4516 , 49.32 )
( 4517 , 49.03 )
( 4518 , 48.93 )
( 4519 , 48.79 )
( 4520 , 48.82 )
( 4521 , 48.72 )
( 4522 , 48.71 )
( 4523 , 48.67 )
( 4524 , 48.43 )
( 4525 , 48.20 )
( 4526 , 47.89 )
( 4527 , 47.86 )
( 4528 , 47.77 )
( 4529 , 47.47 )
( 4530 , 47.54 )
( 4531 , 47.58 )
( 4532 , 47.62 )
( 4533 , 47.56 )
( 4534 , 47.64 )
( 4535 , 47.69 )
( 4536 , 47.50 )
( 4537 , 47.31 )
( 4538 , 47.01 )
( 4539 , 46.90 )
( 4540 , 46.64 )
( 4541 , 46.34 )
( 4542 , 46.04 )
( 4543 , 45.74 )
( 4544 , 45.45 )
( 4545 , 45.15 )
( 4546 , 44.89 )
( 4547 , 44.59 )
( 4548 , 44.29 )
( 4549 , 44.36 )
( 4550 , 44.44 )
( 4551 , 44.57 )
( 4552 , 44.53 )
( 4553 , 44.41 )
( 4554 , 44.34 )
( 4555 , 44.27 )
( 4556 , 44.16 )
( 4557 , 44.23 )
( 4558 , 44.27 )
( 4559 , 44.14 )
( 4560 , 44.02 )
( 4561 , 44.00 )
( 4562 , 44.06 )
( 4563 , 44.06 )
( 4564 , 44.04 )
( 4565 , 44.14 )
( 4566 , 44.23 )
( 4567 , 44.35 )
( 4568 , 44.45 )
( 4569 , 44.54 )
( 4570 , 44.64 )
( 4571 , 44.61 )
( 4572 , 44.62 )
( 4573 , 44.62 )
( 4574 , 44.57 )
( 4575 , 44.52 )
( 4576 , 44.46 )
( 4577 , 44.44 )
( 4578 , 44.48 )
( 4579 , 44.42 )
( 4580 , 44.16 )
( 4581 , 43.91 )
( 4582 , 43.61 )
( 4583 , 43.49 )
( 4584 , 43.25 )
( 4585 , 43.01 )
( 4586 , 42.80 )
( 4587 , 42.50 )
( 4588 , 42.20 )
( 4589 , 41.99 )
( 4590 , 41.79 )
( 4591 , 41.58 )
( 4592 , 41.30 )
( 4593 , 41.21 )
( 4594 , 40.91 )
( 4595 , 40.62 )
( 4596 , 40.32 )
( 4597 , 40.29 )
( 4598 , 40.27 )
( 4599 , 40.05 )
( 4600 , 39.94 )
( 4601 , 39.77 )
( 4602 , 39.71 )
( 4603 , 39.61 )
( 4604 , 39.48 )
( 4605 , 39.55 )
( 4606 , 39.62 )
( 4607 , 39.59 )
( 4608 , 39.49 )
( 4609 , 39.42 )
( 4610 , 39.27 )
( 4611 , 39.07 )
( 4612 , 38.86 )
( 4613 , 38.65 )
( 4614 , 38.67 )
( 4615 , 38.57 )
( 4616 , 38.27 )
( 4617 , 38.00 )
( 4618 , 37.78 )
( 4619 , 37.48 )
( 4620 , 37.36 )
( 4621 , 37.21 )
( 4622 , 36.92 )
( 4623 , 36.62 )
( 4624 , 36.32 )
( 4625 , 36.08 )
( 4626 , 35.81 )
( 4627 , 35.51 )
( 4628 , 35.21 )
( 4629 , 34.92 )
( 4630 , 34.62 )
( 4631 , 34.32 )
( 4632 , 34.41 )
( 4633 , 34.51 )
( 4634 , 34.62 )
( 4635 , 34.71 )
( 4636 , 34.88 )
( 4637 , 34.97 )
( 4638 , 35.09 )
( 4639 , 35.18 )
( 4640 , 35.28 )
( 4641 , 35.38 )
( 4642 , 35.54 )
( 4643 , 35.67 )
( 4644 , 35.77 )
( 4645 , 36.01 )
( 4646 , 36.24 )
( 4647 , 36.48 )
( 4648 , 36.77 )
( 4649 , 37.01 )
( 4650 , 37.16 )
( 4651 , 37.34 )
( 4652 , 37.34 )
( 4653 , 37.06 )
( 4654 , 36.91 )
( 4655 , 36.63 )
( 4656 , 36.43 )
( 4657 , 36.13 )
( 4658 , 35.83 )
( 4659 , 35.54 )
( 4660 , 35.23 )
( 4661 , 34.93 )
( 4662 , 34.87 )
( 4663 , 34.82 )
( 4664 , 34.73 )
( 4665 , 34.64 )
( 4666 , 34.34 )
( 4667 , 34.12 )
( 4668 , 34.05 )
( 4669 , 34.09 )
( 4670 , 33.99 )
( 4671 , 33.73 )
( 4672 , 33.64 )
( 4673 , 33.59 )
( 4674 , 33.48 )
( 4675 , 33.35 )
( 4676 , 33.23 )
( 4677 , 33.11 )
( 4678 , 32.98 )
( 4679 , 32.86 )
( 4680 , 32.73 )
( 4681 , 32.61 )
( 4682 , 32.49 )
( 4683 , 32.38 )
( 4684 , 32.71 )
( 4685 , 33.02 )
( 4686 , 33.41 )
( 4687 , 33.78 )
( 4688 , 33.86 )
( 4689 , 33.90 )
( 4690 , 33.78 )
( 4691 , 33.66 )
( 4692 , 33.53 )
( 4693 , 33.41 )
( 4694 , 33.73 )
( 4695 , 34.12 )
( 4696 , 34.55 )
( 4697 , 35.00 )
( 4698 , 35.39 )
( 4699 , 35.78 )
( 4700 , 36.18 )
( 4701 , 36.57 )
( 4702 , 37.04 )
( 4703 , 37.49 )
( 4704 , 37.86 )
( 4705 , 38.23 )
( 4706 , 38.64 )
( 4707 , 39.02 )
( 4708 , 39.46 )
( 4709 , 39.82 )
( 4710 , 40.28 )
( 4711 , 40.58 )
( 4712 , 40.90 )
( 4713 , 41.24 )
( 4714 , 41.55 )
( 4715 , 41.86 )
( 4716 , 42.21 )
( 4717 , 42.54 )
( 4718 , 42.84 )
( 4719 , 43.14 )
( 4720 , 43.44 )
( 4721 , 43.80 )
( 4722 , 44.10 )
( 4723 , 44.40 )
( 4724 , 44.75 )
( 4725 , 45.05 )
( 4726 , 45.37 )
( 4727 , 45.67 )
( 4728 , 46.03 )
( 4729 , 46.33 )
( 4730 , 46.68 )
( 4731 , 47.07 )
( 4732 , 47.39 )
( 4733 , 47.76 )
( 4734 , 48.15 )
( 4735 , 48.47 )
( 4736 , 48.81 )
( 4737 , 49.11 )
( 4738 , 49.45 )
( 4739 , 49.79 )
( 4740 , 50.09 )
( 4741 , 50.49 )
( 4742 , 50.79 )
( 4743 , 51.11 )
( 4744 , 51.49 )
( 4745 , 51.84 )
( 4746 , 52.17 )
( 4747 , 52.48 )
( 4748 , 52.78 )
( 4749 , 53.08 )
( 4750 , 53.39 )
( 4751 , 53.76 )
( 4752 , 54.06 )
( 4753 , 54.40 )
( 4754 , 54.75 )
( 4755 , 55.07 )
( 4756 , 55.38 )
( 4757 , 55.68 )
( 4758 , 56.01 )
( 4759 , 56.31 )
( 4760 , 56.70 )
( 4761 , 57.00 )
( 4762 , 57.32 )
( 4763 , 57.70 )
( 4764 , 58.00 )
( 4765 , 58.30 )
( 4766 , 58.61 )
( 4767 , 58.92 )
( 4768 , 59.22 )
( 4769 , 59.52 )
( 4770 , 59.87 )
( 4771 , 60.24 )
( 4772 , 60.62 )
( 4773 , 61.00 )
( 4774 , 61.35 )
( 4775 , 61.66 )
( 4776 , 61.89 )
( 4777 , 62.13 )
( 4778 , 62.48 )
( 4779 , 62.79 )
( 4780 , 63.06 )
( 4781 , 63.32 )
( 4782 , 63.57 )
( 4783 , 63.70 )
( 4784 , 63.86 )
( 4785 , 64.01 )
( 4786 , 64.21 )
( 4787 , 64.41 )
( 4788 , 64.58 )
( 4789 , 64.70 )
( 4790 , 64.84 )
( 4791 , 64.98 )
( 4792 , 65.10 )
( 4793 , 65.23 )
( 4794 , 65.40 )
( 4795 , 65.57 )
( 4796 , 65.76 )
( 4797 , 65.92 )
( 4798 , 66.05 )
( 4799 , 66.17 )
( 4800 , 66.15 )
( 4801 , 66.16 )
( 4802 , 66.07 )
( 4803 , 66.12 )
( 4804 , 66.27 )
( 4805 , 66.44 )
( 4806 , 66.57 )
( 4807 , 66.71 )
( 4808 , 66.84 )
( 4809 , 66.78 )
( 4810 , 66.73 )
( 4811 , 66.70 )
( 4812 , 66.64 )
( 4813 , 66.62 )
( 4814 , 66.61 )
( 4815 , 66.78 )
( 4816 , 66.93 )
( 4817 , 66.98 )
( 4818 , 67.05 )
( 4819 , 67.09 )
( 4820 , 67.24 )
( 4821 , 67.24 )
( 4822 , 67.12 )
( 4823 , 66.99 )
( 4824 , 66.96 )
( 4825 , 66.92 )
( 4826 , 66.80 )
( 4827 , 66.76 )
( 4828 , 66.63 )
( 4829 , 66.51 )
( 4830 , 66.57 )
( 4831 , 66.66 )
( 4832 , 66.74 )
( 4833 , 66.78 )
( 4834 , 66.68 )
( 4835 , 66.55 )
( 4836 , 66.48 )
( 4837 , 66.37 )
( 4838 , 66.29 )
( 4839 , 66.16 )
( 4840 , 66.11 )
( 4841 , 65.98 )
( 4842 , 65.86 )
( 4843 , 65.73 )
( 4844 , 65.84 )
( 4845 , 65.89 )
( 4846 , 65.88 )
( 4847 , 65.76 )
( 4848 , 65.65 )
( 4849 , 65.52 )
( 4850 , 65.43 )
( 4851 , 65.30 )
( 4852 , 65.23 )
( 4853 , 65.14 )
( 4854 , 65.05 )
( 4855 , 64.96 )
( 4856 , 64.86 )
( 4857 , 64.79 )
( 4858 , 64.70 )
( 4859 , 64.80 )
( 4860 , 64.92 )
( 4861 , 64.95 )
( 4862 , 64.97 )
( 4863 , 64.96 )
( 4864 , 64.87 )
( 4865 , 64.82 )
( 4866 , 64.53 )
( 4867 , 64.23 )
( 4868 , 64.34 )
( 4869 , 64.39 )
( 4870 , 64.34 )
( 4871 , 64.39 )
( 4872 , 64.42 )
( 4873 , 64.44 )
( 4874 , 64.38 )
( 4875 , 64.34 )
( 4876 , 64.28 )
( 4877 , 64.29 )
( 4878 , 64.30 )
( 4879 , 64.27 )
( 4880 , 64.23 )
( 4881 , 64.37 )
( 4882 , 64.33 )
( 4883 , 64.29 )
( 4884 , 64.37 )
( 4885 , 64.48 )
( 4886 , 64.55 )
( 4887 , 64.48 )
( 4888 , 64.57 )
( 4889 , 64.52 )
( 4890 , 64.46 )
( 4891 , 64.45 )
( 4892 , 64.45 )
( 4893 , 64.39 )
( 4894 , 64.52 )
( 4895 , 64.62 )
( 4896 , 64.70 )
( 4897 , 64.75 )
( 4898 , 64.86 )
( 4899 , 64.88 )
( 4900 , 64.88 )
( 4901 , 64.84 )
( 4902 , 64.83 )
( 4903 , 64.90 )
( 4904 , 64.84 )
( 4905 , 64.91 )
( 4906 , 64.98 )
( 4907 , 65.05 )
( 4908 , 64.98 )
( 4909 , 64.93 )
( 4910 , 64.93 )
( 4911 , 64.88 )
( 4912 , 64.84 )
( 4913 , 64.81 )
( 4914 , 64.88 )
( 4915 , 64.83 )
( 4916 , 64.77 )
( 4917 , 64.73 )
( 4918 , 64.70 )
( 4919 , 64.74 )
( 4920 , 64.73 )
( 4921 , 64.72 )
( 4922 , 64.72 )
( 4923 , 64.77 )
( 4924 , 64.77 )
( 4925 , 64.77 )
( 4926 , 64.76 )
( 4927 , 64.73 )
( 4928 , 64.86 )
( 4929 , 64.97 )
( 4930 , 65.23 )
( 4931 , 65.53 )
( 4932 , 65.70 )
( 4933 , 65.70 )
( 4934 , 65.77 )
( 4935 , 65.80 )
( 4936 , 65.85 )
( 4937 , 65.83 )
( 4938 , 65.88 )
( 4939 , 65.94 )
( 4940 , 65.91 )
( 4941 , 66.04 )
( 4942 , 66.16 )
( 4943 , 66.13 )
( 4944 , 66.00 )
( 4945 , 65.72 )
( 4946 , 65.42 )
( 4947 , 65.12 )
( 4948 , 64.88 )
( 4949 , 64.69 )
( 4950 , 64.50 )
( 4951 , 64.35 )
( 4952 , 64.20 )
( 4953 , 64.06 )
( 4954 , 63.95 )
( 4955 , 63.65 )
( 4956 , 63.35 )
( 4957 , 63.20 )
( 4958 , 62.93 )
( 4959 , 62.63 )
( 4960 , 62.46 )
( 4961 , 62.16 )
( 4962 , 61.87 )
( 4963 , 61.75 )
( 4964 , 61.46 )
( 4965 , 61.18 )
( 4966 , 60.88 )
( 4967 , 60.70 )
( 4968 , 60.43 )
( 4969 , 60.37 )
( 4970 , 60.40 )
( 4971 , 60.34 )
( 4972 , 60.20 )
( 4973 , 59.92 )
( 4974 , 59.68 )
( 4975 , 59.38 )
( 4976 , 59.11 )
( 4977 , 58.89 )
( 4978 , 58.68 )
( 4979 , 58.48 )
( 4980 , 58.27 )
( 4981 , 57.97 )
( 4982 , 57.67 )
( 4983 , 57.37 )
( 4984 , 57.23 )
( 4985 , 56.95 )
( 4986 , 56.69 )
( 4987 , 56.45 )
( 4988 , 56.35 )
( 4989 , 56.38 )
( 4990 , 56.40 )
( 4991 , 56.49 )
( 4992 , 56.52 )
( 4993 , 56.42 )
( 4994 , 56.32 )
( 4995 , 56.32 )
( 4996 , 56.12 )
( 4997 , 56.02 )
( 4998 , 55.95 )
( 4999 , 55.76 )
( 5000 , 55.46 )
( 5001 , 55.16 )
( 5002 , 54.86 )
( 5003 , 54.56 )
( 5004 , 54.27 )
( 5005 , 54.12 )
( 5006 , 54.00 )
( 5007 , 53.70 )
( 5008 , 53.40 )
( 5009 , 53.10 )
( 5010 , 53.01 )
( 5011 , 52.91 )
( 5012 , 52.61 )
( 5013 , 52.32 )
( 5014 , 52.02 )
( 5015 , 51.93 )
( 5016 , 51.83 )
( 5017 , 51.53 )
( 5018 , 51.26 )
( 5019 , 51.30 )
( 5020 , 51.29 )
( 5021 , 51.24 )
( 5022 , 51.00 )
( 5023 , 50.70 )
( 5024 , 50.40 )
( 5025 , 50.10 )
( 5026 , 49.80 )
( 5027 , 49.50 )
( 5028 , 49.20 )
( 5029 , 48.90 )
( 5030 , 48.60 )
( 5031 , 48.33 )
( 5032 , 48.03 )
( 5033 , 47.73 )
( 5034 , 47.64 )
( 5035 , 47.44 )
( 5036 , 47.14 )
( 5037 , 46.84 )
( 5038 , 46.64 )
( 5039 , 46.40 )
( 5040 , 46.10 )
( 5041 , 45.95 )
( 5042 , 45.88 )
( 5043 , 45.80 )
( 5044 , 45.73 )
( 5045 , 45.43 )
( 5046 , 45.25 )
( 5047 , 45.05 )
( 5048 , 44.88 )
( 5049 , 44.68 )
( 5050 , 44.54 )
( 5051 , 44.39 )
( 5052 , 44.12 )
( 5053 , 43.86 )
( 5054 , 43.55 )
( 5055 , 43.25 )
( 5056 , 43.05 )
( 5057 , 42.92 )
( 5058 , 42.82 )
( 5059 , 42.56 )
( 5060 , 42.28 )
( 5061 , 41.98 )
( 5062 , 41.68 )
( 5063 , 41.39 )
( 5064 , 41.09 )
( 5065 , 40.92 )
( 5066 , 40.63 )
( 5067 , 40.36 )
( 5068 , 40.15 )
( 5069 , 39.87 )
( 5070 , 39.58 )
( 5071 , 39.28 )
( 5072 , 38.98 )
( 5073 , 38.77 )
( 5074 , 38.51 )
( 5075 , 38.21 )
( 5076 , 37.92 )
( 5077 , 37.67 )
( 5078 , 37.58 )
( 5079 , 37.29 )
( 5080 , 37.22 )
( 5081 , 36.92 )
( 5082 , 36.84 )
( 5083 , 36.54 )
( 5084 , 36.45 )
( 5085 , 36.15 )
( 5086 , 35.94 )
( 5087 , 35.73 )
( 5088 , 35.52 )
( 5089 , 35.22 )
( 5090 , 34.92 )
( 5091 , 34.83 )
( 5092 , 34.75 )
( 5093 , 34.69 )
( 5094 , 34.59 )
( 5095 , 34.54 )
( 5096 , 34.44 )
( 5097 , 34.27 )
( 5098 , 34.04 )
( 5099 , 33.75 )
( 5100 , 33.45 )
( 5101 , 33.67 )
( 5102 , 33.75 )
( 5103 , 33.72 )
( 5104 , 33.70 )
( 5105 , 33.74 )
( 5106 , 33.86 )
( 5107 , 34.06 )
( 5108 , 34.30 )
( 5109 , 34.54 )
( 5110 , 34.59 )
( 5111 , 34.56 )
( 5112 , 34.28 )
( 5113 , 33.98 )
( 5114 , 33.68 )
( 5115 , 33.38 )
( 5116 , 33.08 )
( 5117 , 32.81 )
( 5118 , 32.51 )
( 5119 , 32.37 )
( 5120 , 32.08 )
( 5121 , 31.86 )
( 5122 , 31.68 )
( 5123 , 31.55 )
( 5124 , 31.43 )
( 5125 , 31.13 )
( 5126 , 31.07 )
( 5127 , 30.77 )
( 5128 , 30.47 )
( 5129 , 30.17 )
( 5130 , 29.96 )
( 5131 , 29.89 )
( 5132 , 29.62 )
( 5133 , 29.49 )
( 5134 , 29.31 )
( 5135 , 29.07 )
( 5136 , 28.84 )
( 5137 , 28.55 )
( 5138 , 28.26 )
( 5139 , 27.96 )
( 5140 , 27.83 )
( 5141 , 27.78 )
( 5142 , 27.63 )
( 5143 , 27.50 )
( 5144 , 27.25 )
( 5145 , 26.95 )
( 5146 , 26.65 )
( 5147 , 26.35 )
( 5148 , 26.21 )
( 5149 , 26.11 )
( 5150 , 26.01 )
( 5151 , 25.92 )
( 5152 , 25.62 )
( 5153 , 25.32 )
( 5154 , 25.03 )
( 5155 , 24.73 )
( 5156 , 24.73 )
( 5157 , 24.64 )
( 5158 , 24.54 )
( 5159 , 24.24 )
( 5160 , 23.96 )
( 5161 , 23.70 )
( 5162 , 23.40 )
( 5163 , 23.23 )
( 5164 , 23.04 )
( 5165 , 22.74 )
( 5166 , 22.44 )
( 5167 , 22.48 )
( 5168 , 22.18 )
( 5169 , 21.88 )
( 5170 , 21.75 )
( 5171 , 21.67 )
( 5172 , 21.44 )
( 5173 , 21.21 )
( 5174 , 21.11 )
( 5175 , 21.07 )
( 5176 , 20.85 )
( 5177 , 20.61 )
( 5178 , 20.61 )
( 5179 , 20.52 )
( 5180 , 20.22 )
( 5181 , 19.92 )
( 5182 , 19.62 )
( 5183 , 19.32 )
( 5184 , 19.07 )
( 5185 , 18.77 )
( 5186 , 18.47 )
( 5187 , 18.17 )
( 5188 , 18.25 )
( 5189 , 18.26 )
( 5190 , 18.20 )
( 5191 , 18.07 )
( 5192 , 17.95 )
( 5193 , 17.65 )
( 5194 , 17.45 )
( 5195 , 17.18 )
( 5196 , 16.88 )
( 5197 , 16.88 )
( 5198 , 16.92 )
( 5199 , 17.03 )
( 5200 , 17.10 )
( 5201 , 16.79 )
( 5202 , 16.52 )
( 5203 , 16.22 )
( 5204 , 15.92 )
( 5205 , 15.63 )
( 5206 , 15.33 )
( 5207 , 15.04 )
( 5208 , 14.80 )
( 5209 , 14.75 )
( 5210 , 14.77 )
( 5211 , 14.67 )
( 5212 , 14.54 )
( 5213 , 14.25 )
( 5214 , 14.28 )
( 5215 , 14.24 )
( 5216 , 14.14 )
( 5217 , 14.05 )
( 5218 , 14.07 )
( 5219 , 13.77 )
( 5220 , 13.71 )
( 5221 , 13.61 )
( 5222 , 13.35 )
( 5223 , 13.05 )
( 5224 , 12.75 )
( 5225 , 12.46 )
( 5226 , 12.38 )
( 5227 , 12.45 )
( 5228 , 12.35 )
( 5229 , 12.39 )
( 5230 , 12.39 )
( 5231 , 12.29 )
( 5232 , 11.99 )
( 5233 , 11.99 )
( 5234 , 11.92 )
( 5235 , 11.90 )
( 5236 , 11.81 )
( 5237 , 11.52 )
( 5238 , 11.37 )
( 5239 , 11.10 )
( 5240 , 11.02 )
( 5241 , 10.78 )
( 5242 , 10.71 )
( 5243 , 10.41 )
( 5244 , 10.11 )
( 5245 , 9.816 )
( 5246 , 9.549 )
( 5247 , 9.312 )
( 5248 , 9.102 )
( 5249 , 8.801 )
( 5250 , 8.511 )
( 5251 , 8.414 )
( 5252 , 8.493 )
( 5253 , 8.517 )
( 5254 , 8.432 )
( 5255 , 8.306 )
( 5256 , 8.012 )
( 5257 , 7.748 )
( 5258 , 7.609 )
( 5259 , 7.537 )
( 5260 , 7.514 )
( 5261 , 7.565 )
( 5262 , 7.618 )
( 5263 , 7.583 )
( 5264 , 7.282 )
( 5265 , 7.189 )
( 5266 , 6.977 )
( 5267 , 6.745 )
( 5268 , 6.449 )
( 5269 , 6.210 )
( 5270 , 5.909 )
( 5271 , 5.627 )
( 5272 , 5.343 )
( 5273 , 5.164 )
( 5274 , 4.882 )
( 5275 , 4.617 )
( 5276 , 4.443 )
( 5277 , 4.143 )
( 5278 , 3.875 )
( 5279 , 3.635 )
( 5280 , 3.540 )
( 5281 , 3.240 )
( 5282 , 3.323 )
( 5283 , 3.269 )
( 5284 , 3.291 )
( 5285 , 2.991 )
( 5286 , 3.150 )
( 5287 , 3.014 )
( 5288 , 2.841 )
( 5289 , 2.544 )
( 5290 , 2.595 )
( 5291 , 2.301 )
( 5292 , 2.423 )
( 5293 , 1.771 )
( 5294 , 0.000 )
};

